Robust Motion Planning in the Presence of Estimation Uncertainty

Motion planning is a fundamental problem and focuses on finding control inputs that enable a robot to reach a goal region while safely avoiding obstacles. However, in many situations, the state of the system may not be known but only estimated using, for instance, a Kalman filter. This results in a novel motion planning problem where safety must be ensured in the presence of state estimation uncertainty. Previous approaches to this problem are either conservative or integrate state estimates optimistically which leads to non-robust solutions. Optimistic solutions require frequent replanning to not endanger the safety of the system. We propose a new formulation to this problem with the aim to be robust to state estimation errors while not being overly conservative. In particular, we formulate a stochastic optimal control problem that contains robustified risk-aware safety constraints by incorporating robustness margins to account for state estimation errors. We propose a novel sampling-based approach that builds trees exploring the reachable space of Gaussian distributions that capture uncertainty both in state estimation and in future measurements. We provide robustness guarantees and show, both in theory and simulations, that the induced robustness margins constitute a trade-off between conservatism and robustness for planning under estimation uncertainty that allows to control the frequency of replanning.

==> Robust Motion Planning in the Presence of Estimation Uncertainty/algorithm2e.tex <==
%  algorithm2e.sty --- style file for algorithms
%                      almost everything can be customized by users. See the document for more explanations
%% Copyright 1996-2015 Christophe Fiorio
%
% This work may be distributed and/or modified under the conditions of the LaTeX Project
% Public License, either version 1.3 of this license or (at your option) any later version.
% The latest version of this license is in http://www.latex-project.org/lppl.txt and
% version 1.3 or later is part of all distributions of LaTeX version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is M. Christophe Fiorio
%
% This work consists of the files algorithm2e.sty and algorithm2e.tex 
% and the associated example files algorithm2e_exAlgoDisjdecomp.tex,
% algorithm2e_exIR.tex, algorithm2e_ex01.tex, algorithm2e_exProg.tex,
% algorithm2e_ex02.tex, algorithm2e_exfor.tex, algorithm2e_ex03.tex,
% algorithm2e_exgeneric.tex, algorithm2e_ex04.tex,  algorithm2e_exgeneric2.tex,
% algorithm2e_ex05.tex, algorithm2e_exnlsty.tex, algorithm2e_ex06.tex,
% algorithm2e_exrepeat.tex, algorithm2e_ex07.tex, algorithm2e_exswitch.tex
%  
%  Report bugs and comments to:
%  - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
%  - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
%  subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
%
%  $Id: algorithm2e.sty,v 5.1 2015/10/18 21:37:30 cfiorio Exp $
%
%  PACKAGES REQUIRED:
%
%  - float   (in contrib/supported/float)
%  - ifthen  (in base)
%  - xspace  (in packages/tools)
%  - relsize (in contrib/misc/relsize.sty)
%
%%%%%%%%%%%%%%%  Release 5.1
%
%   Package options: 
%   ---------------
%   - oldcommands                      : to use old command names
%   - french, english, german, ngerman
%      portuguese, czech, italiano,
%      slovak, croatian, spanish       : for the name of the algorithm and some keyword code
%   - onelanguage                      : to simply switch keyword from one language to another without changing
%                                        keyword commands
%   - boxed, boxruled, ruled, tworuled, 
%     algoruled, plain                 : layout of the algorithm
%   - algo2e                           : environment is algorithm2e instead of algorithms and \listofalgorithmes
%                                        instead of \listofalgorithms
%   - slide                            : to use when making slides
%   - noline,lined,vlined              : how block are designed.
%   - shortend, longend, noend         : short or long end keyword as endif for e.g.
%   - linesnumbered                    : auto numbering of the algorithm's lines
%   - linesnumberedhidden              : to hide autonumbered lines (show number on a line with \ShowLn
%   - commentsnumbered, inoutnumbered  : to autonumber comments and inout keywords (by defaut not numbered)
%   - rightnl                          : to have line number on the right instead of on the left as default
%   - algonl                           : line numbers preceded by algo number
%   - scright, scleft                  : right or left justified side comments
%   - fillcomment, nofillcomment       : end mark of comment is flushed to the right so comments fill the line
%   - dotocloa                         : add an entry in the toc for list of algorithms (require tocbibind package)
%   - endfloat                         : add algoendfloat environment pushing algorithm so written to the end of document
%   - resetcount, noresetcount         : start value of line numbers.
%   - algopart,algochapter,algosection : algo numbering within part, chapter or section
%   - titlenumbered,titlenotnumbered   : numbering of title set by \Titleofalgo
%   - figure                           : algorithms are figures, numbered as figures, and put in the list of figures.
%   - procnumbered                     : procedure or function are numbered as algorithm
%   - nokwfunc                         : procedure or function name doens't become a command
%   - norelsize                        : don't use relsize package (useful if it breaks the compatibily)
%   - displayblockmarkers              : display begin, end keywords at start of each block
%  
%   defaults are; english,plain,resetcount,titlenotnumbered
%
%%%%%%%%%%%%%%
%
%   Short summary  
%   -------------
%  
%   algorithm is an environment for writing algorithm in LaTeX2e.
%   Almost all is customizable. You can add keywords, change style, change the layout, ...
%   It provide macros that allow you to create differents sorts of key words, therefore a set of predefined key
%   word is gived.
%
%   IT should be used as follows
%
%   \begin{algorithm}
%       ...
%       ...
%   \end{algorithm}
%
%
%   IMPORTANT : each line MUST end with \;
%
%   Note that if you define macros outside algorithm environment they
%   are avaible in all the document and particulary you can use then
%   inside all algorithms without re-define them.
%  
%   an example:
%
%   \begin{algorithm}
%     \SetAlgoLined
%     \KwIn{this text}
%     \KwOut{how to write algorithm with \LaTeX2e }
%     
%     initialization\;
%     \While{not at end of this document}{
%       read current section\;
%       \eIf{understand}{
%         go to next section\;
%         current section becomes this one\;
%         }{
%         go back to the beginning of current section\;
%         }
%       }
%     \caption{How to write algorithm}
%   \end{algorithm}
%
%
%%%%%%%%%%%%%%         predefined keywords
%
%     \KwIn{input}
%     \KwOut{output}
%     \KwData{input}
%     \KwResult{output}
%     \KwTo                                       % a simple keyword
%     \KwFrom                                     % a simple keyword
%     \KwRet{[value]}
%     \Return{[value]}
%     \Begin{block inside}
%     \eIf{condition}{Then Block}{Else block}     % in blocks
%     \If{condition}{Then block}                  % in a block
%     \uIf{condition}{Then block}                 % in a block unended
%     \lIf{condition}{Else text}                  % on the same line
%     \Else{inside Else}                          % in a block
%     \lElse{Else text}                           % on the same line        
%     \uElse{Else text}                           % in a block unended
%     \ElseIf{inside Elseif}                      % in a block
%     \lElseIf{Elseif text}                       % on the same line        
%     \uElseIf{Elseif text}                       % in a block unended
%     \Switch{Condition}{Switch block}
%     \Case{a case}{case block}                   % in a block
%     \lCase{a case}{case text}                   % on the same line
%     \Other{otherwise block}                     % in a block
%     \lOther{otherwise block}                    % on the same line
%     \For{condition}{text loop}                  % in a block
%     \lFor{condition}{text}                      % on the same line
%     \ForEach{condition}{text loop}              % in a block
%     \lForEach{condition}{text}                  % on the same line
%     \ForPar{condition}{text loop}               % in a block
%     \lForPar{condition}{text}                   % on the same line
%     \While{condition}{text loop}                % in a block
%     \lWhile{condition}{text loop}               % on the same line
%     \Repeat{End condition}{text loop}           % in a block
%     \lRepeat{condition}{text}                   % on the same line
%
%%%%%%%%%%%%%%
%
%   History: 
%
%   -  October 19 2015 - revision 5.1
%                   * CHANGE/ADD: l commands  (the ones as \lIf) can now be used with a
%                              star. If done, no end of line are done, so you can enclose
%                              l command into another one. For example, you can write:
%                              \lForEach{$i$}{\lIf*{foo}{bar}}.
%                               Note that when you use a star, side comments are not allowed.
%                   * CHANGE/ADD: Now you can have a side comment at end of macros which
%                               have a block. For example you can do : 
%                               \Begin(\tcc*[h]{side comment for begin}{text}(\tcc*[h]{side comment after end})
%                               Note: there are some side effects for some commands:
%                              \SetKwProg : macro defined thanks to \SetKwProg are allowed
%                                                   to have no end marker. In this case,
%                                                   beware to end side comment, this can
%                                                   do weird output (but no error)
%                   * CHANGE: \SetKwSwitch defines also an \uOther command which was not
%                               the case until this release.
%                   * CHANGE: \SetStartEndCondition{typo1}{typo2}{typo3} defined two end
%                               conditions (type2 and typo3) : typo3 is no more used for
%                               case condition as typo2 is used which is more consistent
%                               since there is a condition followed by a keyword as for
%                               if-then or other command that are defined using typo2.
%                   * CHANGE: keywords was not language dependant to allow to use multiple
%                               languages in the same document, but some keywords in
%                               different language were having the same keyword that lead
%                               last one declared to replace first one and so you could have some
%                               spanish keywords printed as you were in portuguese. So
%                               this behavior is changed from now:
%                               - localized keywords are defined if according language
%                                  option is defined ; 
%                               - if you want to keep old behaviour and use localized
%                                  keywords without using language option (keep old
%                                  behavior), you can use languagekw option
%                                  (e.g. frenchkw, germankw, ...). Note that you can use
%                                  multiple languagekw options at the same time, in
%                                  contrary of language option. Note also that if you use
%                                  multiple languagekw options, you can get back the same
%                                  problem as previously when keywords was not language
%                                  dependant.
%                   * ADD: new typo styles:
%                               - Arguments of functions have now their own style. By
%                                  default, FuncArgSty is the same as ArgSty. 
%                               - Name of KwProg have now their own sty (they used ArgSty
%                                  previously). By default, ProgSty is still ArgSty.
%                               As usual, \SetFuncArgSty{}, FuncArgSty{} and
%                               \SetProgSty{}, ProgSty{} are macros to set and use these
%                               typo styles.
%                   * ADD: Options to manage algorithm hangindent
%                            Until this revision, long statement acts as classical text and
%                            continue on next line starting from the same point. This makes
%                            difficult to notice that the new lines of text is not a new
%                            statement. Now, hangindent is managed and when a long
%                            statement continue on next lines, lines, except the first,
%                            are indented.
%                            Option: noalgohanging
%                               By default, long statement are indented on subsequent
%                               lines; with this option you get old behavior and lines are
%                               no more indented
%                            Option: hangingcomment 
%                               Comment that are alone on a line (not side comment) are
%                               not driven by algo hanging: subsequent lines of long
%                               comments are indented according to width of start comment
%                               marker. With this option, comment are indented like normal
%                               statement.
%                            Option: hanginginout
%                               As for comment, by default, in/out keywords and input
%                               keywords (defined by \SetKwInOut or \SetKwInput) are not
%                               indented by algorithm hangindent. They are indented
%                               according to width of input keyword. If you want that these
%                               keywords acts like normal statement, use this option.
%                            \SetAlgoHangIndent{length}
%                               This macro allows you to set your own indent length. By
%                               default, \SetAlgoHangIndent{0.5em}
%                   * ADD: Group markers. 
%                            This option is related to block markers of release 5.0. Some
%                            have ask to put also block markers for single line
%                            command. This new feature has been implemented to do this.
%                            So, you can now ask package to put begin and end keywords
%                            automatically at start and end of single line command (see
%                            example in documentation).
%                            These new group markers macros are:
%                            - \AlgoDisplayGroupMarkers and \AlgoDontDisplayGroupMarkers
%                            Note that a new option has also been added: displaygroupmarkers
%                   * ADD: \SetCustomAlgoRuledWidth{length}
%                             set a custom ruled width of ruled and algoruled options ;
%                             note that by the moment you use this macro, rules will have
%                             this fixed length: this can cause strange behavior in
%                             multicolumn mode or other layout that change the line
%                             width. 
%                   * ADD: turkish language option
%                   * FIX: a spurious whitespace which results in a spurious indent in the
%                            user's text right after the end of the algorithm environment
%                            was introduced  in release 5.0. This is fixed now thanks to
%                            Alexander Malkis.
%                   * FIX: there was a problem with margins in caption when option figure
%                            was use with caption package. This is fixed.
%                   * FIX: when changing font size in caption with, interline skip stayed
%                            unchanged and so with a small font was to large. This is fixed.
%                   * FIX: in contrary of that is written in the documentation, ':' what
%                            not in KwSty typo for KwIn and KwOut command. This is fixed. 
%                   * FIX: strange behaviour with label and lines numbered: @currentlabel
%                            was updated according to algo line number not in all
%                            situation. For e.g, with hyperref package, always updated ;
%                            with \nlset also updated, but with \nl or linesnumbered
%                            option, not updated. This "feature" causes different output
%                            with \label command according to options used which is not
%                            that one want. This is solved now, and @currentlabel is
%                            always updated so \label command works always is the same way.
%                   * FIX: some czech keywords
%                   * FIX: some spanish keywords
%                   * FIX: some croatian keywords
%                   * FIX: krantz class changes definition of chapter and get one more
%                            option that classical classes as book.cls or report.cls and
%                            broke fix for hyperref on chapter definition. This is now
%                            fixed and algorithm detects use of krantz class and use then
%                            a definition of chapter working with krantz class.
%                   * FIX: an issue with internal macro which causes ([Q]) use as argument
%                            of some environment to be misprinted (thanks to Martin Schr?der).
%                   * FIX: mispelled name of hyperrefcounter inside internal macro.
%
%   - January 06 2013 - revision 5.0
%                     * CHANGE: SetKwSwitch takes now 9 args: 9th arg is the same as
%                                previous 8th arg ('end of switch' keyword). New 8th arg is
%                                'end of case' keyword. This is due to change of release
%                                3.2 which introduce end after case block... as I never
%                                test with longend option, I never see that the 'end
%                                switch' used for case was not good.
%                     * CHANGE: when no end keyword is defined in a block macro, then
%                                algorithm2e does no more try to print it. So even with lined or noline
%                                option, no empty line is printed (before: a blank end was
%                                printed, so a blank line appeared)
%                     * Internal Change: add some internal function to improve readibility
%                                        (thanks to Philip K. F. H\?lzenspies)
%                     * ADD: Block markers. 
%                            You can now ask package to put begin and end keywords automatically at begin
%                            and end of blocks, it means each group of commands shifted and enclosed in
%                            braces.
%                            This is tricky to use but, combined with \SetStartEndCondition and
%                            redefinition of keywords, you should be abble to simulate any syntax. See
%                            examples in documentation where a generic example is derived in pseudo-code,
%                            python and C by keeping code and changing only style using block markers
%                            macros, \SetStartEndCondition and some redefinition of keywords.
%                            These new block markers macros are:
%                            - \AlgoDisplayBlockMarkers and \AlgoDontDisplayBlockMarkers
%                            - \SetAlgoBlockMarkers{begin marker}{end marker}
%                            - \BlockMarkersSty{text} and \SetBlockMarkersSty
%                            Note that a new option has also been added: displayblockmarkers
%                     * ADD: \leIf macro automatically defined by \SetKwIF: allow to define
%                            an if-then-else on a single line.
%                     * ADD: new macro \SetStartEndCondition{typo1}{typo2}{typo3} which
%                            sets typo around condition in For, If, Switch, Case and
%                            Repeat macros. First two are used around For, If, Swith
%                            conditions, First and third are used for Case and Repeat
%                            condition where condition ends the line. Default definition
%                            is \SetStartEndCondition{ }{ }{}. 
%                            A common alternative is \SetStartEndCondition{ (}{) }{)}
%                            Can also be used to remove space around condition, for
%                            example if you want python style commands:
%                            \SetStartEndCondition{ }{}{} and \SetKwFor{For}{for}{:}{}
%                     * ADD: new environment algomathdisplay which allow display math (like inside \[ \] or $$ $$) 
%                            handling end line and line number
%                     * ADD: new command \SetKwProg{Env}{Title}{is}{end} which defines a macro
%                            \Env{args}{text}. Env is a block with 'Title' (in \CapSty) at the beginning
%                            followed by args followed by 'is' then 'text' is put below inside a block ended
%                            by 'end'. If no 'end' is specified, nothing is written (no
%                            blank line is inserted). Useful to typeset function or prog for example:
%                            \SetKwProg{Fn}{Function}{ is}{end} makes \Fn{afunc(i: int) : int}{return 0\;}                    
%                            writes: 
%                            Function afunc(i: int) : int is
%                            | return 0;
%                            end
%                            or \SetKwProg{Def}{def}{:}{} makes \Def{afunc(i: int)}{return 0\;} writes:
%                            def afunc(i: int):
%                            | return 0
%                            Tip: combine it with \SetKwFunction to write recursive function algorithm. With
%                            example above, you could define \SetKwFunction{\Afunc}{afunc} and then write:
%                            \Def{\Afunc{i:int}{\eIf{i>0}{\KwRet \Afunc{i-1}}{\KwRet 0\;}} that writes:
%                            def afunc(i: int):
%                            | if(i>0):
%                            |     return afunc(i-1)
%                            | else:
%                            |     return 0
%                            with appropriate typo.
%                     * ADD: option croatian: croatian keywords (thanks to Ivan Gavran)
%                     * ADD: option ngerman: same as german option but so can be used with global option ngerman
%                            of babel
%                     * ADD: option spanish: Spanish support (thanks to Mario Abarca)
%                     * ADD: unterminated block: useful to add part separator that doesn't necessary need an end
%                            keyword.  
%                            Designed on the pattern of unterminated if (see \uIf macro) allowing to
%                            add a block that is not terminated by a keyword. Such block are defined in the same
%                            time as a block is defined by adding a macro beginning with u. So, for example,
%                            predefined \SetKwBlock{Begin}{begin}{end} defines now two commands:
%                            - \Begin{} as previously which print a begin - end block
%                            - \uBegin{} that defines a begin only block
%                     * FIX: problem when numbering line inside until condition of
%                            \SetKwRepeat macro: line number was not correctly aligned.
%                     * FIX: dotocloa option which was broken
%                     * FIX: uIf and uCase didn't have same behavior when used with
%                            noline, vlined or lined option. This is fixed. Side effect: no empty
%                            line after an uIf or uCase when used with options lined or vlined
%                     * FIX: a bug with Repeat Until command when use with side comment on Until
%                     * FIX: a bug with side text -- text put into () -- of command macro (SetKwIf and so on)
%                            which was always setting a ';' even after a \DontPrintSemicolon
%                     * FIX: a bug with hyperref and chapter definition (thanks to Hubert Meier)
%                     * FIX: bugs with l macro and side comment
%                     * FIX: revision number
%                     * FIX: fix non ascii character (utf8 not yet recognized by all latex engine)
%                     * FIX: fnum@algocf had an useless parameter which sometimes broke expansion and output an error
%                     * FIX: works now with multicol package
%
%   - december 14 2009 - revision 4.1
%                     * ADD: new command \SetKwHangingKw{Name}{text} (hanging indent with keyword): This creates a
%                            hanging indent much like \texttt{SetKwInput}, except that it removes the trailing `:'
%                            and does not reset numbering (thanks to Nathan Tallent)
%
%   - november 17 2009  - revision 4.00 -
%
%                      * CHANGE: IMPORTANT: some commands have been renamed to have consistent naming (CamlCase
%                                syntax) and old commands are no more available. If you doesn't want to change
%                                your mind or use old latex files, you can use oldcommands option to enable old
%                                commands back.
%                                text. Here are these commands:
%                                - \SetNoLine becomes \SetAlgoNoLine
%                                - \SetVline  becomes \SetAlgoVlined
%                                - \Setvlineskip  becomes \SetVlineSkip
%                                - \SetLine   becomes \SetAlgoLined
%                                - \dontprintsemicolon becomes \DontPrintSemicolon
%                                - \printsemicolon becomes \PrintSemicolon
%                                - \incmargin becomes \IncMargin
%                                - \decmargin becomes \DecMargin
%                                - \setnlskip becomes \SetNlSkip
%                                - \Setnlskip becomes \SetNlSkip
%                                - \setalcapskip becomes \SetAlCapSkip
%                                - \setalcaphskip becomes \SetAlCapHSkip
%                                - \nlSty becomes \NlSty
%                                - \Setnlsty becomes \SetNlSty
%                                - \linesnumbered becomes \LinesNumbered
%                                - \linesnotnumbered becomes \LinesNotNumbered
%                                - \linesnumberedhidden becomes \LinesNumberedHidden
%                                - \showln becomes \ShowLn
%                                - \showlnlabel becomes \ShowLnLabel
%                                - \nocaptionofalgo becomes \NoCaptionOfAlgo
%                                - \restorecaptionofalgo becomes \RestoreCaptionOfAlgo
%                                - \restylealgo becomes \RestyleAlgo
%                                - gIf macros and so on do no more exist
%                      * NEW: - Compatibily with other packages improven by changing name of internal
%                               macros. Algorithm2e can now be used with arabtex for example, if this last is
%                               loaded after algorithm2e package.
%                      * ADD: - OPTION endfloat: endfloat packages doesn't allow float environment inside other
%                               environment. So using it with figure option of algorithm2e makes error. This
%                               option enables a new environment algoendfloat to be used instead of algorithm
%                               environment that put algorithm at the end. algoendfloat environment make
%                               algorithm acting as endfloat figures. This option requires endfloat packages.
%                      * ADD: - OPTION norelsize: starting from this release (v4.00), algorithm2e package uses
%                               relsize package in order to get relative size for lines numbers; but it seems
%                               that some rare classes (such as inform1.cls) are not compatible with relsize; to
%                               have algorithm2e working, this option makes algorithm2e not to load relsize
%                               package and go back to previous definition by using \scriptsize font for lines
%                               numbers.
%                      * ADD: - OPTION onelanguage: allow, if using standard keywords listed below, to switch
%                               from one language to another without changing keywords by using appropriate
%                               language option:
%                               . KwIn, KwOut, KwData, KwResult
%                               . KwTo KwFrom
%                               . KwRet, Return
%                               . Begin
%                               . Repeat
%                               . If, ElseIf, Else
%                               . Switch, Case, Other
%                               . For, ForPar, ForEach, ForAll, While
%                               .
%                      * ADD: - OPTION rightnl: put lines numbers to the right of the algorithm instead of left.
%                      * ADD:   new commands \setRightLinesNumbers and \setLeftLinesNumbers which sets the lines
%                               numbers to the right or to the left of the algorithm.
%                      * ADD: - new kind of keywords: KwArray used to define arrays:
%                               \SetKwArray{Kw}{array} defines an array keywords Kw called array and printed in
%                               DataSty style when call with \Kw. It can be used with one argument which
%                               denotes the element index: \Kw{n} prints array[n] with array in DataSty and n in
%                               ArgSty.
%                      * ADD/FIX: rules of ruled, algoruled, tworuled styles used rules of different sizes! This
%                                 is now fixed. Moreover size of the rules is now controlled by a length and so
%                                 can be customized by the user.
%                                 \algoheightrule is the height of the rules and can be changed via \setlength
%                                 \algoheightruledefault is the default height of he rules (0.8pt)
%                                 \algotitleheightrule is the height of the rule that comes just after the
%                                 caption in ruled and algoruled style; it can be changed via \setlength
%                                 \algotitleheightruledefault is the default height of this rules (0.8pt)
%                                 Thanks to Philippe Dumas who reports the bug and make the suggestion.
%                      * ADD: - \SetAlgoCaptionSeparator which sets the separator between Algorithm 1 and the
%                               title. By default it's ':' and caption looks like "Algorithm 2: title" but now
%                               you can change it by using for example \SetAlgoCaptionSeparator{.} which will
%                               give "Algorithm 3. title"
%                      * ADD: - \SetAlgoLongEnd and \SetAlgoShortEnd and \SetAlgoNoEnd commands which act as
%                               corresponding package options
%                      * ADD: - OPTIONS italiano and slovak as new language (thanks to Roberto Posenato and
%                               Miroslav Binas) 
%                      * CHANGE: - Fnt and Sty macro to have consistent use and naming (see below)
%                      * ADD: - \AlCapSty, \AlCapNameSty, \AlCapFnt, \AlCapNameFnt, \ProcSty, \ProcFnt,
%                               \ProcNameSty, \ProcNameFnt, \ProcArgSty, ProcArgFnt and corresponding "set macro" 
%                               \SetAlCapSty, \SetAlCapNameSty, \SetAlCapFnt, \SetAlCapNameFnt, \SetProcSty,
%                               \SetProcFnt, \SetProcNameSty, \SetProcNameFnt, \SetProcArgSty, \SetProcArgFnt which
%                               control the way caption is printed. Sty macro use command taking one parameter as
%                               argument, Fnt macros use directly command. In Fact caption is printed as follow:
%                               \AlCapSty{\AlCapFnt Algorithm 1:}\AlCapNameSty{\AlCapNameFnt my algorithm}
%                               By default, \AlCapSty is textbf and \AlCapFnt is nothing. \AlCapNameSty keep text 
%                               as it is, and \AlCapNameFnt do nothing also.
%                               You can redefine \AlCapFnt and \AlCapNameFnt by giving macro to \Set commands. For
%                               example, you can do \SetAlCapFnt{\large} to see Algorithm printed in \large font.
%                               You can redefine \AlCapSty, \AlCapFnt, \AlCapNameSty and \AlCapNameFnt with the
%                               corresponding \Set command. For the Sty commands, you have to give in parameter
%                               name of a macro (whithout \)  which takes one argument. For example,
%                               \SetAlCapFnt{textbf} defines the default behaviour. If you want to do more
%                               complicated thing, you should define your own macro and give it to \SetAlCapFnt or
%                               \SetAlCapNameFnt. Here are two examples:
%                               - \newcommand{\mycapsty}[1]{\tiny #1}\SetAlCapNameSty{mycapsty}
%                               - \newcommand{\mycapsty}[1]{\textsl{\small #1}}\SetAlCapNameSty{mycapsty}
%                               Or you can combine the two, for the last example you can also do:
%                               \SetAlCapNameSty{textsl}\SetAlCapNameFnt{\small}
%                               Thanks to Jan Stilhammer who gives me the idea of \AlCapNameFnt.
%                      * CHANGE \AlTitleFnt to match definition of all other Fnt macros and add a \AlTitleSty 
%                               macro (see below) . Now you set \AlTitleFnt by calling \SetAlTitleFnt with 
%                               directly a macro without parameter in argument:
%                               Example: \SetAlTitleFnt{\small} to set title in small font.
%                      * ADD: - \AlTitleSty and \SetAlTitleSty commands to set a style for title. These commands
%                               are defined from a macro taking the text in argument, as \textbf for example. 
%                               To set the TitleSty you have to give name of the macro (without the '\') 
%                               to \SetAlTitleSty. For example \SetAlTitleSty{textbf} to set \textbf style.
%                      * ADD: - new command \SetAlgorithmName{algorithmname}{list of algorithms name} which
%                               redefines name of the algorithms and the sentence list of algorithms. Second
%                               argument is the name that \autoref, from hyperref package, will use. Example:
%                               \SetAlgorithmName{Protocol}{List of protocols} if you prefer protocol than
%                               algorithm.
%                      * ADD: - new \SetAlgoRefName{QXY} which change the default ref (number of the algorithm) by
%                               the name given in parameter (QXY in the example). 
%                      * ADD: - new command \SetAlgoRefRelativeSize{-2} which sets the output size of refs, defined
%                               by \SetAlgoRefName, used in list of algorithms.
%                      * ADD: - two dimensions to control the layout of caption in ruled, algoruled and boxruled
%                               algorithms:
%                               - interspacetitleruled (2pt by defaut) which controls the vertical space between
%                                 rules and title in ruled and algoruled algorithms.
%                               - interspaceboxruled (2\lineskip by default) which controls the vertical space
%                                 between rules and title in boxruled algorithms.
%                               These two dimensions can be changed by using \setlength command.
%                      * ADD: - With the fix (see below) of procedure and function environments, a new feature has
%                               been added: the name of the procedure or function set in caption is automatically
%                               defined as a KwFunction and so can be used as a macro. For example, if inside a
%                               procedure environment you set \caption{myproc()}, you can use \myproc macro in you
%                               main text. Beware that the macro is only defined after the \caption!
%                      * ADD: - OPTION nokwfunc to unable the new feature described above in function and
%                               procedure environment. Useful if you use name of procedure or function that cannot
%                               be a command name as a math display for example.
%                      * ADD: - \SetAlgoNlRelativeSize{number} command which sets the relative size of line
%                               numbers. By default, line numbers are two size smaller than algorithm text. Use
%                               this macro to change this behavior. For example, \SetAlgoNlRelativeSize{0} sets it
%                               to the same size, \SetAlgoNlRelativeSize{-1} to one size smaller and
%                               \SetAlgoNlRelativeSize{1} to one size bigger
%                      * ADD: - \SetAlgoProcName{aname} command which sets the name of Procedure printed by
%                               procedure environment (the environment prints Procedure by default). Second
%                               argument is the name that \autoref, from hyperref package, will use.
%                      * ADD: - \SetAlgoFuncName{aname} command which sets the name of Function printed by
%                               procedure environment (the environment prints Function by default). Second
%                               argument is the name that \autoref, from hyperref package, will use. 
%                      * ADD: - \SetAlgoCaptionLayout{style} command which sets style of the caption; style must
%                               be the name of a macro taking one argument (the text of the caption). Examples
%                               below show how to use it:
%                               . \SetAlgoCaptionLayout{centerline} to have centered caption
%                               . \SetAlgoCaptionLayout{textbf} to have bold caption
%                               If you want to apply two styles in the same time, such as centered bold, you have
%                               to define you own macro and then use \SetAlgoCaptionLayout with its name.
%                      * ADD: - OPTION procnumbered: which makes the procedure and function to be numbered as
%                               algorithm
%                      * ADD: - OPTIONS tworuled and boxruled
%                               these are two new layouts: tworuled acts like ruled but doesn't put a line after
%                               caption ; boxruled surround algorithm by a box, puts caption above and add a line
%                               after caption.
%                      * REMOVE: - SetKwInParam has been deleted since not useful itself because of different
%                                macros which can do the same in a better and a more consistent way as
%                                SetKwFunction or SetKw.
%                      * FIX: - line number is now correctly vertically aligned with math display.
%                      * FIX: - references with hyperref. No more same identifier or missing name error. BUT now
%                               you must NOT use naturalnames option of hyperref packages if you do PdfLaTeX
%                      * FIX: - autoref with hyperref package (thanks to J?rg Sommer who notices the problem).
%                      * FIX: - titlenumbered was not working! fixed.
%                      * FIX: - Else(){} acted like uElse. Corrected.
%                      * FIX: - noend management: when a block was inside another and end of block was following
%                               each other, a blank line was added: it's now corrected.
%                      * FIX: - Function and Procedure environment was no more working as defined originally: the
%                               label was no more name of the procedure, it acts always as if procumbered option
%                               has been used.
%                      * FIX: - line numbers had a fixed size which can be bigger than algorithm text accordingly
%                               to \AlFnt set (see also new command \SetAlgoNlRelativeSize above)
%                      * FIX: - semicolon in comments when dontprintsemicolon is used.
%                      * FIX: - listofalgorithms adds a vertical space before first algo of a chapter as for
%                               listoffigures or listoftables
%                      * FIX: - listofalgorithms with twocolumns mode and some classes which don't allow onecolumn
%                               and so don't define \if@restonecol as prescribed in LaTeX (sig-alternate for
%                               example)
%                      * FIX: - algorithm2e now works with elsart cls and some more classes.
%                      * FIX: - blocks defined by SetKwBlock act now as other blocks (if for instance) and don't
%                               write end in vlined mode, instead they print a small horizontal line as required
%                               by the option.
%                      * FIX: - underfull hbox warning at each end of algorithm environment removed.
%
%                      * INTERNAL CHANGE: - short end keyword are deduce from long end keyword by keeping the
%                                           first one. Allows to avoid double definition.
%                      * INTERNAL CHANGE: - procedure, function and algorithm are now resolved by the same
%                               environment to avoid code duplication. 
%
%   - October  04 2005  - revision 3.9 -
%                      * ADD: - \setalcaphskip command which sets the horizontal skip before Algorithm: in caption
%                               when used in ruled algorithm.
%                      * ADD: - \SetAlgoInsideSkip command which allows to add an extra vertical space before and
%                               after the core of the algorithm (ie: \SetAlgoInsideSkip{bigskip}) 
%                      * CHANGE: - caption, when used with figure option, is no more controlled by algorithm2e
%                                  package and so follows the exact behaviour of figures. The drawback is that you
%                                  cannot change the typo with AlTitleFnt or CapFnt. The avantage is that if you
%                                  use caption package, it works.
%                      * FIX: - problem with numbering line and pdflatex
%                      * FIX: - error when algorithm2e package was used with beamer and listings together
%   - February 12 2005  - revision 3.8 -
%                      * FIX: - extra line with noend option.
%   - February 10 2005  - revision 3.7 -
%                      * ADD: - sidecomment: different macros allowing to put text right after code on the same
%                               line. They are defined in the same time comment macros are defined with a star
%                               after the macro name. By default comments are right justified but this can be
%                               change with appropriate option in the macro. Ex:
%                               . default: \tcc*{side comment}
%                               . same as previous: \tcc*[r]{side comment}
%                               . left justify: \tcc*[l]{side comment}
%                               . here: \tcc*[h]{side comment} don't put the end of line mark before
%                                       comment (; by default) and don't end the line.
%                               . flushed: \tcc*[f]{side comment} same as the precedent but right
%                                 justified
%                      * ADD: - OPTION scright (default): right justified side comments (side comments
%                               are flushed to the righr)
%                      * ADD: - OPTION scleft: left justified side comments (side comments are put right after the
%                               code line)
%                      * ADD: - \SetSideCommentLeft acts as scleft option
%                      * ADD: - \SetSideCommentRight acts as scright option
%                      * ADD: - block like macro side text: all macro defining a block allows now to put text right
%                               after key words by putting text into (). Done to be used with sidecomment macros,
%                               but all text can be used. 
%                               Ex: \eIf(\tcc*[f]{then comment}){test}{then text}(else side text){else text}
%                      * ADD: - OPTION fillcomment (default): end mark of comment is flushed to the right so
%                               comments fill all the width of text.
%                      * ADD: - OPTION nofillcomment: end mark of comment is put right after the comment.
%                      * ADD: - \SetNoFillComment acts as nofillcomment option.
%                      * ADD: - \SetFillComment acts as fillcomment option.
%                      * ADD: - OPTION dotocloa: which adds an entry in the toc for the list of algorithms. This
%                               option load package tocbibind if not already done and so list of figures and list
%                               of tables are also added in the toc. If you want to control which ones of the lists
%                               will be added in the toc, please load package tocbibind before package algorithm
%                               and give it the options you want.
%                      * FIX: - vertical spacing for uif macro with noend option
%                      * FIX: - all the compatibility problems between caption and other packages
%                      * FIX: - typographical differences between list of algorithms and other lists  when in
%                               report or book 
%
%   - January 24 2005  - revision 3.6 -
%                      * FIX: - vertical spacing and space characters at the beginning or end of comments.
%                               line numbers of comments not in the NlSty.
%                               Thanks to Arnaud Giersch for his comments and suggestions.
%                      * FIX: - Set*Sty macro: the styles defined was not protected and was modified by surrounding
%                               context. For example KwTo in a \For{}{} was in bold AND italic instead of just in
%                               bold.
%                      * FIX: - line number misplacement after \Indp
%
%   - January 21 2005  - revision 3.5 -
%                      * ADD: - hidden numbering of the lines. Lines are auto-numbered but numbers are shown only
%                               on lines you specify:
%                               * linesnumberedhidden option or \LinesNumberedHidden macro activate this
%                                 functionnality.
%                               * \ShowLn and \ShowLnLabel{lab} macros make the number visible on the
%                               line. \ShowLnLabel{lab} allows to set a label for this line. 
%                               Thanks to Samson de Jager who makes this suggestion and provides the macros.
%                      * ADD: - \AlCapFnt and \SetAlCapFnt which allow to have a different font for
%                               caption. Works like \AlFnt and \SetAlFnt and by default is the same.
%                      * ADD: - \AlCapSkip skip length. This vertical space is added before caption in plain ou
%                               boxed mode. It allows to change distance between text and caption.
%                      * FIX: - caption compatible with IEEEtran class. 
%                      * FIX: - some vertical spacing error with \uIf macros (Thanks to Arnaud Giersch)
%                      * FIX: - Procedure and Function: lines are also numbered like algorithms
%                      * FIX: - CommentSty was not used for Comments
%
%   - January 10 2005  - revision 3.4 -
%                      * FIX: - caption compatible with new release of Beamer class. 
%
%   - June 16 2004     - revision 3.3 - 
%                      * FIX: - Hyperlink references of Hyperref package works now if compiled with pdflatex 
%                               and [naturalnames] option of hyperref package is used.
%                      * FIX: - algorithm[H] had problem in an list environment - corrected
%                      * FIX: - interline was not so regular in nested blocks - corrected
%                      * ADD  - \SetVlineSkip macro which sets the vertical skip after the little horizontal 
%                               rule which closes a block in Vlined mode. By default 0.8ex
%
%   - June 11 2004     - revision 3.2 - AUTO NUMBERING LINES !!!
%                      * ADD: auto numbering of the lines (the so asked and so long awaiting feature)
%                             this feature is managed by 3 options and 3 commands:
%                             - linesnumbered option: lines of the algo are numbered except for comments and
%                               input/output (KwInput and KwInOut)
%                             - commentsnumbered option: makes comments be numbered
%                             - inoutnumbered option: makes data input/output be numbered
%                             - \nllabel{lab} labels the line so you can cite with \ref{lab}
%                             - \LinesNumbered make the following algorithms having auto-numbered lines
%                             - \linesnotnumbered make the following algorithms having no auto-numbered lines
%                      * Change: algo2e option renames listofalgorithms in listofalgorithmes
%                      * FIX: new solution for compatibility with color package, more robust and not tricky.
%                             Many thanks to David Carlisle for his advices
%
%   - June 09 2004     - revision 3.1 -
%                      * Change: \SetKwSwitch command defines an additionnal macro \uCase and \Case prints end
%                      * Change: now macros SetKw* do a renewcommand if the keyword is already defined. So you can
%                                redefine default definition at your own convenience or change your definition
%                                without introducing a new macro and changing your text.
%                      * ADD: new macro \SetKwIF which do \SetKwIf and
%                             \SetKwIfElseIf.The following default definition has been added:
%                             \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
%                             and so you get the macros;
%                             \If \eIf \lIf \uIf \ElseIf \uElseIf \lElseIf \Else \uElse \lElse
%                      * ADD: new macro \SetAlgoSkip which allow to fix the vertical skip before and after the
%                             algorithms. Default is smallskip, do \SetAlgoSkip{} if you don't want an extra space
%                             or \SetAlgoSkip{medskip} or \SetAlgoSkip{bigskip} if you want bigger space.
%                      * ADD: macro \SetKwIf defines in addition a new macro \uElse  (depending on wat name you
%                             have given in #2 arg).
%                      * ADD: macro \SetKwIfElseIf defines in addition a new macro \uElse and \ugElseIf (depending
%                             on what name you have given in #2 and #3 arg).
%                      * Change: baseline of algorithm is now top, so two algorithms can be put side by side.
%                      * FIX: Compatibility with color package solved. The problem was due to a redefinition of
%                             standard macros by color package. This solves compatibility problem with other
%                             packages as pstcol or colortbl. (notified by Dirk Fressmann, Antti Tarvainen and Koby
%                             Crammer)
%                      * Fix: extra little shift to the right with boxed style algorithm removed (notified by
%                             P. Tanovski)
%                      * Fix: algoln option was buggy (notified bye Jiaying Shen)
%                      * Fix: german and portuges option didn't work due to bad typo (notified by Martin Sievers,
%                             Thorsten Vitt and Jeronimo Pellegrini)
%                      
%   - February 13 2004 - revision 3.0 -
%                      * Major revision which makes the package independent from float.sty, so now
%                        - algorithm* works better, in particular can be used in multicols environments
%                        - (known bug corrected)
%                          [H] works now for all sort of environment but is handled differently for classic
%                          environment and star environment (algorithm, figure, procedure and function). For star
%                          environment, H acts like for classical figure environment, so it doesn't stay here
%                          absolutely.
%                        - (known bug corrected)
%                          you can use now floatflt package with algorithm package and even with figure
%                          option. Beware that if you want to put an algorithm inside a floatingfigure, it cannot
%                          be floating, so [H] is required and then figure option should not be used, since
%                          standard figure[H] are still floating with LaTeX.
%                      * boxruled: a new style added. Possible now since no style no more defined by the float
%                        package.
%                      * nocaptionofalgo: dosen't print Algorithm #: in the caption for algorithm in ruled or
%                        algoruled style.
%                        note: this is just documentation of a macro which was already in the package.
%   - December 14 2003 - revision 2.52 -
%                      * output message shorter
%                      * French keyword macro \PourTous was missing for longend option, it has been added.
%                      * TitleofAlgo prints Function or Procedure in corresponding environments.
%
%   - October 27 2003  - revision 2.51 - Revision submitted to CTAN archive
%                      * correction of a minor which make caption in procedure
%                        and function to be blanck with pdfscreen package
%                        (thanks to Joel Gossens for the notification)
%                      * add two internal definition to avoid some errors when
%                        used with Hyperref package (Hyperref package need to
%                        define new counter macro from existing ones, and
%                        don't do it for algorithm2e package, so we do it)
%
%   - October 17 2003  - revision 2.50 - first revision for CTAN archive
%                      * add \AlFnt and \SetAlFnt{font} macros: \AlFnt is used at the beginning of the caption and
%                        the body of algorithm in order to define the fonts used for typesetting algorithms. You
%                        can use it elsewhere you want to typeset text as algorithm. For example you can do
%                        \SetAlFnt{\small\sf} to have algorithms typeset in small sf font. Default is nothing so
%                        algorithm is typeset as the text of the document.
%                      * add \AlTitleFnt{text} and \SetAlTitleFnt{font} macros: The {Algorithm: } in the caption is
%                        typeset with \AlTitleFnt{Algorithm:}. You can use it to have text typeset as {Algorithm:}
%                        of captions. Default is textbf.  Default can be redefined by \SetAlTitleFnt{font}, for
%                        example you can do \SetAlTitleFnt{emph}
%                      * add CommentSty typo for text comment.  
%                      * add some compatibility with hyperref package (still an error on multiply defined refs but
%                        pdf correctly generated)
%                      * flush text to left in order to have correct indentation even with class as amsart which
%                        center all figures
%                      * add german, portuguese and czech options for title of algorithms and typo.
%                      * add portuguese translation of predefined keywords * add czech translation of some
%                        predefined keywords
%
%   - December 23 2002 - revision 2.40
%                      * add some French keyword missing
%                      * add function* and procedure* environment like algorithme* environment: print in one column
%                        even if twocolumn option is specified for the document.
%                      * add a new macro \SetKwComment to define macro which writes comments in the text. First
%                        argument is the name of the macro, second is the text put before the comment, third is the
%                        text put at the end of the comment.Default are \tcc and \tcp
%                      * add new options to change the way algo are numbered:
%                        [algopart] algo are numbered within part (counter must exist)
%                        [algochapter] algo are numbered within chapter
%                        [algosection] algo are numbered within section
%
%   - March 27 2002   - revision 2.39
%                      * Gilles Geeraerts: added the \SetKwIfElseIf to manage
%                        if (c)
%                             i;
%                        else if (c)
%                             i;
%                        ...
%                        else
%                             i;
%                        end
%                      * Also added \gIf \gElseIf \gElse.
%
%   - January 02 2001 - revision 2.38
%                      * bugs related to the caption in procedure and function
%                        environment are corrected.
%                      * bug related to option noend (extra vertical space added
%                        after block command as If or For) is corrected.
%                      * czech option language added (thanks to Libor Bus: l.bus@sh.cvut.cz).
%  
%   - October 16 2000 - revision 2.37
%                      * option algo2e added: change the name of environment
%                        algorithm into algorithm2e. So allow to use the package
%                        with some journal style which already define an algorithm
%                        environment.
%  
%   - September 13 2000 - revision 2.36
%                      * option slide added: require package color
%                      * Hack for slide class in order to have correct
%                        margins
%  
%   - November 25 1999 - revision 2.35
%                      * revision number match RCS number
%                      * Thanks to David A. Bader, a new option is added:
%                        noend: no end keywords are printed.
%  
%   - November 19 1999 - revision 2.32
%                      * minor bug on longend option corrected.
%  
%   - August 26 1999 - revision 2.31
%                      * add an option: figure
%                        this option makes algorithms be figure and so are numbered
%                        as figures, have Figure as caption and are put in 
%                        the \listoffigures
%  
%   - January 21 1999 - revision 2.3 beta
%                    add 2 new environments: procedure and function.
%                    These environments works like algorithm environment but:
%                    - the ruled (or algoruled) style is imperative.
%                    - the caption now writes Procedure name....
%                    - the syntax of the \caption command is restricted as
%                      follow: you MUST put a name followed by 2 braces like
%                      this ``()''. You can put arguments inside the braces and
%                      text after. If no argument is given, the braces will be
%                      removed in the title. 
%                    - label now puts the name (the text before the braces in the
%                      caption) of the procedure or function as reference (not
%                      the number like a classic algorithm environment).
%                    There are also two new styles: ProcNameSty and
%                    ProcArgSty. These style are by default the same as FuncSty
%                    and ArgSty but are used in the caption of a procedure or a
%                    function.
%                    
%   - November 28 1996 - revision 2.22
%                    add a new macro \SetKwInParam{arg1}{arg2}{arg3}:
%                    it defines a macro \arg1{name}{arg} which prints name in keyword
%                    style followed byt arg surrounded by arg2 and arg3. The main
%                    application is to a function working as \SetKwInput to be used
%                    in the head of the algorithm. For example
%                    \SetKwInParam{Func}{(}{)} allows
%                    \Func{functionname}{list of arguments} which prints:
%                    \KwSty{functioname(}list of arguments\KwSty{)}
%       
%
%   - November 27 1996 - revision 2.21:
%                    minor bug in length of InOut boxes fixed.
%                    add algorithm* environment.
%
%   - July 12 1996 - revision 2.2: \SetArg and \SetKwArg macros removed.
%                        
%                    \SetArg has been removed since it never has been
%                    documented.
%                    \SetKwArg has been removed since \SetKw can now
%                    take an argument in order to be consistent with
%                    \SetKwData and \SetKwFunction macros.
%
%   - July 04 1996 - revision 2.1: still more LaTeX2e! Minor compatibility break
%
%                    Macros use now \newcommand instead of \def, use of \setlength, 
%                    \newsavebox, ... and other LaTeX2e specific stuff.
%                    The compatibility break:
%                    - \SetData becomes \SetKwData to be more consistent. So the old 
%                      \SetKwData becomes \SetKwInput
%                    - old macros \titleofalgo, \Freetitleofalgo and \freetitleofalgo
%                      from LaTeX209 version which did print a warning message and call 
%                      \Titleofalgo in version 2.0 are now removed!
%
%   - March 13 1996 - revision 2.0: first official major revision.
%   
%
%%%%%%%%%%%%%%
%
%   Known bugs: 
%   -----------
%   - horizontal spacing (indent) doesn't work with revtex4 class.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% for more complete informations you can see algorithm2e.tex
%
%
%%%%%%%%%%%%%%%%%%%%%%%% Identification Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
%
\ProvidesPackage{algorithm2e}[2013/01/06 v5.00 algorithms environments]
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Initial Code %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\@makeother\*% some package redefined it as a letter (as color.sty)
\def\@firstword#1 #2\@nil{#1}% an useful fonction
%%%%%%% Utilities:
% \ifArgumentEmpty<c><t><e> ; if c is empty, i.e. {}, then t, else e.
%    Function used internally, but may as well expose it to the user; it's useful
\begingroup
\catcode`\Q=3
\catcode`\T=3
\long\gdef\ALGOCF@argemptyaux#1#2Q#3#4#5T{#4}
\long\gdef\ifArgumentEmpty#1{%
  \begingroup\long\edef\@tempa{\endgroup
    \ALGOCF@argemptyaux#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T%
  }\@tempa
}
\endgroup
% \long\def\ifArgumentEmpty#1{\bgroup
% 	\catcode`\Q=3
% 	\catcode`\T=3
% 	\long\def\@tempa##1##2Q##3##4##5T{##4}%
% 	\xdef\@tempa{\@tempa#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T}%
% \egroup\@tempa}
%%%%%%%%%%%
%
% \algocf@longdef -> shorthand to reduce
%    \expandafter\long\expandafter\def
% to
%    \expandafter\algocf@longdef
% may look insignificant, but reads that much better ;)
\def\algocf@longdef{\long\def}
%
% \algocf@newcommand (and helper \algocf@new@command) behaves like LaTeX's newcommand,
% with two differences:
%  - the argument is not "\<name>", but rather "<name>"; i.e. one level of indirection
%  - if the command exists already, then \renewcommand, rather than \newcommand
\def\algocf@newcommand#1{\expandafter\algocf@new@command\csname#1\endcsname}
\def\algocf@new@command#1{%
	\begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
	\expandafter\@ifundefined\@gtempa\newcommand\renewcommand#1}%
%
% \algocf@newcmdside<name><arity><body>
%   The largest time-saver; many commands we define have the pattern:
%     \<name>(<side_text>)<argX><argY>...
%   where "(<side_text>)" is optional. By defining them with this function,
%   the arguments are parsed and renumbered, i.e. the body works as if the
%   command was:
%     \<name><side_text><argX><argY>...
%   and can use \ifArgumentEmpty to see whether its #1 exists (default case
%   for the side text is (), so there's no difference between calling
%     \foo{bar}
%   or
%     \foo(){bar}
%   Technically this is new behaviour, but it shouldn't really occur...
\algocf@longdef\algocf@newcmdside#1#2#3{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3}%
}
%
% a serie of newcmdside macro for block that allows a comment after the end
%     \<name>(<side_text>)<argX><argY>...(<side_text>)% 
%
% 1. kind of begin-end : for command with only one block as begin-end 
\algocf@longdef\algocf@newcmdside@kobe#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2{\csname algocf@#1checkcomfol\endcsname{##1}{##2}}%
  % now check for last side comment; args are : <first side com (could be empty)>, <body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}}{\csname algocf@#1noendcom\endcsname{##1}{##2}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2(##3){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2{%
    \csname algocf@#1main\endcsname{##1}{##2}{}}%
  \algocf@newcommand{algocf@#1main}[3]{#2}%
}%
%
% 2. kind of if-else : for command with two blocks as if-then-else 
\algocf@longdef\algocf@newcmdside@koif#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2##3{\csname algocf@#1checkcomfol\endcsname{##1}{##2}{##3}}%
  % now check for last side comment; args are : <1st side com>, <1st body of cmd>, <2nd body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2##3{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}{##3}}{\csname algocf@#1noendcom\endcsname{##1}{##2}{##3}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2##3(##4){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{##4}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2##3{%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{}}%
  \algocf@newcommand{algocf@#1main}[4]{#2}%
}%
%
% \algocf@newcmdsides<name><arity><body><tail><closing>
%   Like the command above, but with an optional side text at the end
%   of the command as well, i.e.:
%     \<name>(<side_text>)<argX><argY>(<end_text>)
%   It may be a bit confusing that <arity> doesn't count <end_text>,
%   but since it is for internal use, the naming can be a little more
%   fuzzy. This function behaves as if:
%     <body'> = <body><if end_text: tail{end_text}><closing>
\algocf@longdef\algocf@newcmdsides#1#2#3#4#5{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3\@ifnextchar({\csname algocf@#1end\endcsname}{#4#5}}%
	\expandafter\algocf@longdef\csname algocf@#1end\endcsname(##1){#4{##1}\strut\par}%
}%
%
% definition of commands which can be redefined in options of the package.
%
\newcounter{AlgoLine}%
\setcounter{AlgoLine}{0}%
%
\newcommand{\algocf@algocfref}{\relax}%
\newcommand{\listalgorithmcfname}{}%
\newcommand{\algorithmcfname}{}%
\@ifundefined{algorithmautorefname}{\newcommand{\algorithmautorefname}{algorithm}}{\renewcommand{\algorithmautorefname}{algorithm}}%
\newcommand{\algorithmcflinename}{}%
\newcommand{\algocf@typo}{}%
\newcommand{\@algocf@procname}{}\newcommand{\procedureautorefname}{}%
\newcommand{\SetAlgoProcName}[2]{\renewcommand{\@algocf@procname}{#1}\renewcommand{\procedureautorefname}{#2}}%
\newcommand{\@algocf@funcname}{}\newcommand{\functionautorefname}{}%
\newcommand{\SetAlgoFuncName}[2]{\renewcommand{\@algocf@funcname}{#1}\renewcommand{\functionautorefname}{#2}}%
\newcommand{\@algocf@titleofalgoname}{\algorithmcfname}%
\newcommand{\@algocf@algotitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algorithmcfname}}%
\newcommand{\@algocf@proctitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algocf@procname}}%
%
\newcommand{\algocf@style}{plain}%
\newcommand{\@ResetCounterIfNeeded}{}%
\newcommand{\@titleprefix}{}%
%
\newcommand{\algocf@numbering}[1]{\newcommand{\algocf@within}{#1}}%
%
\newcommand{\defaultsmacros@algo}{\algocf@defaults@shortend}%
%
\newcommand{\algocf@list}{loa}%
\newcommand{\algocf@float}{algocf}%
%
\newcommand{\algocf@envname}{algorithm}%
\newcommand{\algocf@listofalgorithms}{listofalgorithms}%
%
%
%% redefine chapter so that it adds a vspace in the loa as the original does for lof and lot
% \let\algocf@original@chapter=\chapter%
% \def\chapter{\expandafter\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}%
%
% bug correction with hyperref submitted by Hubert Meier
\begingroup\expandafter\expandafter\expandafter\endgroup 
\expandafter\ifx\csname @chapter\endcsname\relax\else 
% \let\algocf@original@chapter=\chapter% 
% \def\chapter{\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}% 
\let\algocf@original@chapter=\@chapter%
\@ifclassloaded{krantz}{%
\def\@chapter[#1][#2]#3{\algocf@original@chapter[#1][#2]{#3}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}{%
\def\@chapter[#1]#2{\algocf@original@chapter[#1]{#2}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}%
\fi
%
%% if@restonecol is defined in article and book but some other classes don't define it and we need it, so we do
\ifx\if@restonecol\relax\else\newif\if@restonecol\fi%
%
%
%%%%%%%%%%%%%%%%%%%%%% Declaration of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\RequirePackage{ifthen}%
%
\newboolean{algocf@displayblockmarkers}\setboolean{algocf@displayblockmarkers}{false}%
\DeclareOption{displayblockmarkers}{%
  \setboolean{algocf@displayblockmarkers}{true}%
}
\newboolean{algocf@displaygroupmarkers}{\setboolean{algocf@displaygroupmarkers}{false}
\DeclareOption{displaygroupmarkers}{%
  \setboolean{algocf@displaygroupmarkers}{true}%
}
%
\newboolean{algocf@nokwfunc}\setboolean{algocf@nokwfunc}{false}%
\DeclareOption{nokwfunc}{%
  \setboolean{algocf@nokwfunc}{true}%
}%
%
\newboolean{algocf@oldcommands}\setboolean{algocf@oldcommands}{false}%
\DeclareOption{oldcommands}{%
  \setboolean{algocf@oldcommands}{true}%
}%
%
\newboolean{algocf@leftlinenumber}\setboolean{algocf@leftlinenumber}{true}%
\newcommand{\setLeftLinesNumbers}{\setboolean{algocf@leftlinenumber}{true}}%
\newcommand{\setRightLinesNumbers}{\setboolean{algocf@leftlinenumber}{false}}%
\DeclareOption{rightnl}{%
  \setRightLinesNumbers%
}%
%
\newboolean{algocf@endfloat}\setboolean{algocf@endfloat}{false}%
\DeclareOption{endfloat}{%
  \setboolean{algocf@endfloat}{true}%
  \newcounter{postalgo}\setcounter{postalgo}{0}%
}%
%
\newboolean{algocf@procnumbered}\setboolean{algocf@procnumbered}{false}%
\DeclareOption{procnumbered}{%
  \setboolean{algocf@procnumbered}{true}%
}%
%
\DeclareOption{algo2e}{%
  \renewcommand{\algocf@envname}{algorithm2e}%
  \renewcommand{\algocf@listofalgorithms}{listofalgorithmes}%
}%
%
\newboolean{algocf@slide}\setboolean{algocf@slide}{false}%
\DeclareOption{slide}{%
  \setboolean{algocf@slide}{true}%
}%
%
\newboolean{algocf@figurecaption}\setboolean{algocf@figurecaption}{false}%
\DeclareOption{figure}{%
\renewcommand{\algocf@list}{lof}%
\renewcommand{\algocf@float}{figure}%
\AtBeginDocument{\@ifpackageloaded{caption}{\setboolean{algocf@figurecaption}{true}}{}}%
}%
%
\newboolean{algocf@optonelanguage}\setboolean{algocf@optonelanguage}{false}%
\DeclareOption{onelanguage}{\setboolean{algocf@optonelanguage}{true}}%
%
\newcommand{\algocf@languagechoosen}{english}%
\newboolean{algocf@localkw@english}\setboolean{algocf@localkw@english}{true}%
\DeclareOption{englishkw}{%
\setboolean{algocf@localkw@english}{true}%
}%
%
\DeclareOption{english}{%
\renewcommand{\listalgorithmcfname}{List of Algorithms}%
\renewcommand{\algorithmcfname}{Algorithm}%
\renewcommand{\algorithmautorefname}{algorithm}%
\renewcommand{\algorithmcflinename}{line}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedure}%
\renewcommand{\@algocf@funcname}{Function}%
\renewcommand{\procedureautorefname}{procedure}%
\renewcommand{\functionautorefname}{function}%
\renewcommand{\algocf@languagechoosen}{english}%
}%
%
%----
\newboolean{algocf@localkw@french}\setboolean{algocf@localkw@french}{false}%
\DeclareOption{frenchkw}{%
\setboolean{algocf@localkw@french}{true}%
}%
%
\DeclareOption{french}{%
\renewcommand{\listalgorithmcfname}{Liste des Algorithmes}%
\renewcommand{\algorithmcfname}{Algorithme}%
\renewcommand{\algorithmautorefname}{algorithme}%
\renewcommand{\algorithmcflinename}{ligne}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Proc\'edure}%
\renewcommand{\@algocf@funcname}{Fonction}%
\renewcommand{\procedureautorefname}{proc\'edure}%
\renewcommand{\functionautorefname}{fonction}%
\renewcommand{\algocf@languagechoosen}{french}%
}%
%
%----
\newboolean{algocf@localkw@czech}\setboolean{algocf@localkw@czech}{false}%
\DeclareOption{czechkw}{%
\setboolean{algocf@localkw@czech}{true}%
}%
%
\DeclareOption{czech}{%
\renewcommand{\listalgorithmcfname}{Seznam algoritm\r{u}}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkce}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{czech}%
}%
%
%----
\newboolean{algocf@localkw@german}\setboolean{algocf@localkw@german}{false}%
\DeclareOption{germankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{german}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\DeclareOption{ngermankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{ngerman}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\newboolean{algocf@localkw@portuguese}\setboolean{algocf@localkw@portuguese}{false}%
\DeclareOption{portuguesekw}{%
\setboolean{algocf@localkw@portuguese}{true}%
}%
%
\DeclareOption{portuguese}{%
\renewcommand{\listalgorithmcfname}{Lista de Algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{linha}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimento}%
\renewcommand{\@algocf@funcname}{Fun\c{c}\~{a}o}%
\renewcommand{\procedureautorefname}{procedimento}%
\renewcommand{\functionautorefname}{fun\c{c}\~{a}o}%
\renewcommand{\algocf@languagechoosen}{portuguese}%
}%
%
%----
\newboolean{algocf@localkw@italiano}\setboolean{algocf@localkw@italiano}{false}%
\DeclareOption{italianokw}{%
\setboolean{algocf@localkw@italiano}{true}%
}%
%
\DeclareOption{italiano}{%
\renewcommand{\listalgorithmcfname}{Elenco degli algoritmi}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{riga}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funzione}%
\renewcommand{\procedureautorefname}{procedura}%
\renewcommand{\functionautorefname}{funzione}%
\renewcommand{\algocf@languagechoosen}{italiano}%
}%
%----
\newboolean{algocf@localkw@spanish}\setboolean{algocf@localkw@spanish}{false}%
\DeclareOption{spanishkw}{%
\setboolean{algocf@localkw@spanish}{true}%
}%
%
\DeclareOption{spanish}{%
\renewcommand{\listalgorithmcfname}{\'Indice de algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{l\'inea}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimiento}%
\renewcommand{\@algocf@funcname}{Funci\'on}%
\renewcommand{\procedureautorefname}{procedimiento}%
\renewcommand{\functionautorefname}{funci\'on}%
\renewcommand{\algocf@languagechoosen}{spanish}%
}%
%----
\newboolean{algocf@localkw@slovak}\setboolean{algocf@localkw@slovak}{false}%
\DeclareOption{slovakkw}{%
\setboolean{algocf@localkw@slovak}{true}%
}%
%
\DeclareOption{slovak}{%
\renewcommand{\listalgorithmcfname}{Zoznam algoritmov}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Proced\'{u}ra}%
\renewcommand{\@algocf@funcname}{Funkcia}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{slovak}%
}%
%
%----
\newboolean{algocf@localkw@croatian}\setboolean{algocf@localkw@croatian}{false}%
\DeclareOption{croatiankw}{%
\setboolean{algocf@localkw@croatian}{true}%
}%
%
\DeclareOption{croatian}{%
\renewcommand{\listalgorithmcfname}{Popis algoritama}%
\renewcommand{\algorithmcfname}{Algoritam}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{redak}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkcija}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{croatian}%
}%
%%% adding 'turkish' option customization
%
%----
\newboolean{algocf@localkw@turkish}\setboolean{algocf@localkw@turkish}{false}%
\DeclareOption{turkishkw}{%
\setboolean{algocf@localkw@turkish}{true}%
}%
\DeclareOption{turkish}{%
\renewcommand{\listalgorithmcfname}{Algoritma Listesi}%
\renewcommand{\algorithmcfname}{Algoritma}%
\renewcommand{\algorithmautorefname}{algoritma}%
\renewcommand{\algorithmcflinename}{?izgi}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Prosed?r}%
\renewcommand{\@algocf@funcname}{Fonksiyon}%
\renewcommand{\procedureautorefname}{prosed?r}%
\renewcommand{\functionautorefname}{fonksiyon}%
\renewcommand{\algocf@languagechoosen}{turkish}%
}%
%
% OPTIONs plain, boxed, ruled, algoruled & boxruled
%
\newcommand{\algocf@style@plain}{\renewcommand{\algocf@style}{plain}}%
\newcommand{\algocf@style@boxed}{\renewcommand{\algocf@style}{boxed}}%
\newcommand{\algocf@style@ruled}{\renewcommand{\algocf@style}{ruled}}%
\newcommand{\algocf@style@algoruled}{\renewcommand{\algocf@style}{algoruled}}%
\newcommand{\algocf@style@boxruled}{\renewcommand{\algocf@style}{boxruled}}%
\newcommand{\algocf@style@tworuled}{\renewcommand{\algocf@style}{tworuled}}%
\newcommand{\algocf@style@plainruled}{\renewcommand{\algocf@style}{plainruled}}%
\newcommand{\RestyleAlgo}[1]{\csname algocf@style@#1\endcsname}%
\DeclareOption{plain}{\algocf@style@plain}%
\DeclareOption{plainruled}{\algocf@style@plainruled}%
\DeclareOption{boxed}{\algocf@style@boxed}%
\DeclareOption{ruled}{\algocf@style@ruled}%
\DeclareOption{algoruled}{\algocf@style@algoruled}%
\DeclareOption{boxruled}{\algocf@style@boxruled}%
\DeclareOption{tworuled}{\algocf@style@tworuled}%
%
% OPTIONs algopart,algochapter & algosection
%
\DeclareOption{algopart}{\algocf@numbering{part}}%       %algo part numbered
\DeclareOption{algochapter}{\algocf@numbering{chapter}}% %algo chapter numbered
\DeclareOption{algosection}{\algocf@numbering{section}}% %algo section numbered
%
% OPTIONs resetcount & noresetcount
%
\DeclareOption{resetcount}{\renewcommand{\@ResetCounterIfNeeded}{\setcounter{AlgoLine}{0}}}%
\DeclareOption{noresetcount}{\renewcommand{\@ResetCounterIfNeeded}{}}%
%
% OPTIONs algorithm hanging for long lines
%
\newlength{\algocf@hangindent}\setlength{\algocf@hangindent}{.5em}
\newcommand{\SetAlgoHangIndent}[1]{\setlength{\algocf@hangindent}{#1}}
%
\newboolean{algocf@hanging}\setboolean{algocf@hanging}{true}% hanging is handle by default
\newboolean{algocf@hanginginout}\setboolean{algocf@hanginginout}{false}% inout are managed as previously: hanging set by inout keywords
\newboolean{algocf@hangingcomment}\setboolean{algocf@hangingcomment}{false}% comment that are not side comment are indented accordingly to comment mark, not as normal text
\newcommand{\algocf@everyparnl}{\relax}%
\newcommand{\algocf@everyparhanging}{\hangafter=1\hangindent=\algocf@hangindent\relax}%
\newcommand{\algocf@everypar}{\algocf@everyparnl\algocf@everyparhanging}%
\newcommand{\algocf@seteverypar}{%
  \ifthenelse{\boolean{algocf@hanging}}{\everypar{\algocf@everypar}}{\relax}%
}%
%
\newcommand{\algocf@seteveryparnl}[1]{\renewcommand{\algocf@everyparnl}{#1}\everypar{\algocf@everypar}}%
\newcommand{\algocf@seteveryparhanging}[1]{%
\let\algocf@oldeveryparhanging=\algocf@everyparhanging%
\renewcommand{\algocf@everyparhanging}{#1}\everypar{\algocf@everypar}%
}%
\newcommand{\algocf@reseteveryparhanging}{%
\let\algocf@everyparhanging=\algocf@oldeveryparhanging%
\everypar{\algocf@everypar}%
}%
\DeclareOption{hanginginout}{\setboolean{algocf@hanginginout}{true}}%
\DeclareOption{hangingcomment}{\setboolean{algocf@hangingcomment}{true}}%
\DeclareOption{noalgohanging}{%
  \setboolean{algocf@hanginginout}{false}%
  \setboolean{algocf@hangingcomment}{false}%
  \setboolean{algocf@hanging}{false}%
}%
%\newcommand{
%
%
% OPTION linesnumbered
%
\newboolean{algocf@linesnumbered}\setboolean{algocf@linesnumbered}{false}%
\newcommand{\algocf@linesnumbered}{\relax}%
\DeclareOption{linesnumbered}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}%
}%
%
% OPTION linesnumberedhidden
%
\DeclareOption{linesnumberedhidden}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}%
}%
%
% OPTION commentsnumbered inoutnumbered
%
\newboolean{algocf@commentsnumbered}\setboolean{algocf@commentsnumbered}{false}%
\DeclareOption{commentsnumbered}{\setboolean{algocf@commentsnumbered}{true}}%
\newboolean{algocf@inoutnumbered}\setboolean{algocf@inoutnumbered}{false}%
\DeclareOption{inoutnumbered}{\setboolean{algocf@inoutnumbered}{true}}%
%
% OPTIONs titlenumbered & titlenotnumbered
%
\DeclareOption{titlenumbered}{%
  \renewcommand{\@titleprefix}{%
    \refstepcounter{\algocf@float}%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\ \expandafter\csname the\algocf@float\endcsname\algocf@typo: }%
  }%
}%
%
\DeclareOption{titlenotnumbered}{\renewcommand{\@titleprefix}{%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\algocf@typo: }}%
}%
%
% OPTIONs algonl
% line numbered with the counter of the algorithm
%
\DeclareOption{algonl}{\renewcommand{\theAlgoLine}{\expandafter\csname the\algocf@float\endcsname.\arabic{AlgoLine}}}%
%
% OPTIONs lined, vlined & noline
%
\DeclareOption{lined}{\AtBeginDocument{\SetAlgoLined}}%   \SetAlgoLined (default)
\DeclareOption{vlined}{\AtBeginDocument{\SetAlgoVlined}}% \SetAlgoVlined
\DeclareOption{noline}{\AtBeginDocument{\SetAlgoNoLine}}%\SetAlgoNoLine
%
% OPTIONs longend, shotend & noend
%
\DeclareOption{longend}{\AtBeginDocument{\SetAlgoLongEnd}}%  \SetAlgoLongEnd
\DeclareOption{shortend}{\AtBeginDocument{\SetAlgoShortEnd}}%\SetAlgoShortEnd
\DeclareOption{noend}{\AtBeginDocument{\SetAlgoNoEnd}}%      \SetAlgoNoEnd
%
\DeclareOption{nosemicolon}{\AtBeginDocument{\DontPrintSemicolon}}%      \SetAlgoNoEnd
%
% OPTION dotoc
%
\newboolean{algocf@dotocloa}\setboolean{algocf@dotocloa}{false}%
\DeclareOption{dotocloa}{%
  \setboolean{algocf@dotocloa}{true}%
}
%
% OPTION comments
%
\newboolean{algocf@optfillcomment}\setboolean{algocf@optfillcomment}{true}%
\DeclareOption{nofillcomment}{%
  \setboolean{algocf@optfillcomment}{false}%
}%
\DeclareOption{fillcomment}{%
  \setboolean{algocf@optfillcomment}{true}%
}%
%
% OPTION sidecommments
%
\newboolean{algocf@scleft}\setboolean{algocf@scleft}{false}%
\DeclareOption{scleft}{%
  \setboolean{algocf@scleft}{true}%
}%
\DeclareOption{sright}{% default
  \setboolean{algocf@scleft}{false}%
}%
%
% OPTION norelsize
%
\newboolean{algocf@norelsize}\setboolean{algocf@norelsize}{false}%
\DeclareOption{norelsize}{%
  \setboolean{algocf@norelsize}{true}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%% Execution of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ExecuteOptions{english,plain,resetcount,titlenotnumbered,lined,shortend}%
%
\ProcessOptions%
%
\@algocf@algotitleofalgo% fix name for \TitleOfAlgo to \algorithmcfname by default
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Package Loading %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\RequirePackage{xspace}%
%
\ifthenelse{\boolean{algocf@endfloat}}{%
  \RequirePackage{endfloat}%
}{\relax}%
%
\ifthenelse{\boolean{algocf@norelsize}}{%
  \newcommand{\relsize}[1]{\scriptsize}%
}{%
  \RequirePackage{relsize}%
}%
%
\ifthenelse{\boolean{algocf@slide}}{\RequirePackage{color}}{}%
%
%
\AtEndOfPackage{%
  \ifthenelse{\boolean{algocf@dotocloa}}{%
    \renewcommand{\listofalgorithms}{\tocfile{\listalgorithmcfname}{loa}}%
  }{\relax}%
}%
%
% if loa in toc required, load tocbibind package if not already done.
\ifthenelse{\boolean{algocf@dotocloa}}{%
  \ifx\@tocextra\undefined%
  \RequirePackage{tocbibind}%
  \fi%
}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Main Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\algocf@name}{algorithm2e}%
\newcommand{\algocf@date}{october 19 2015}%
\newcommand{\algocf@version}{Release 5.1}%
\newcommand{\algocf@id}{\algocf@version\space -- \algocf@date\space --}%
\typeout{********************************************************^^JPackage `\algocf@name'\space\algocf@id^^J%
         - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
         - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
         subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
         - Author: Christophe Fiorio (christophe.fiorio@umontpellier.fr)^^J********************************************************}%
%%
%%
%%
%%
%%
%%
%%%% hyperref compatibility tricks: Hyperref package defines H counters from
   % standard counters (i.e \theHpage from \thepage) and check some particular
   % counters of some packages, unfortunately it doesn't do the same for
   % algorithm2e package but act as Hcounter was defined. To avoid errors we
   % defined \theHalgocf ourself
%%%%
%
\@ifundefined{theHalgocf}{\def\theHalgocf{\thealgocf}}{}%
\@ifundefined{theHAlgoLine}{\def\theHAlgoLine{\theAlgoLine}}{}%
\@ifundefined{theHalgocfproc}{\def\theHalgocfproc{0}}{}%
\@ifundefined{theHalgocffunc}{\def\theHalgocffunc{0}}{}%
\@ifundefined{toclevel@algocf}{\def\toclevel@algocf{0}}{}%
%
% autoref from hyperref needs an autorefname, so we give it.
\def\AlgoLineautorefname{\algorithmcflinename}%
\def\algocfautorefname{\algorithmautorefname}%
\def\algocfprocautorefname{\procedureautorefname}%
\def\algocffuncautorefname{\functionautorefname}%
%%
%%
%%
\newcommand{\@defaultskiptotal}{0.5em}%
\newskip\skiptotal\skiptotal=0.5em%
\newskip\skiplinenumber\skiplinenumber=\hsize\advance\skiplinenumber by-\skiptotal%
\newskip\skiprule%
\newskip\skiphlne%
\newskip\skiptext%
\newskip\skiplength%
\newskip\algomargin%
\newskip\skipalgocfslide\skipalgocfslide=1em%
\newdimen\algowidth%
\newdimen\inoutsize%
\newdimen\inoutindent%
\newdimen\interspacetitleruled\setlength{\interspacetitleruled}{2pt}%
\newdimen\interspacealgoruled\setlength{\interspacealgoruled}{2pt}%
\newdimen\interspacetitleboxruled\setlength{\interspacetitleboxruled}{2\lineskip}%
%
\newcommand{\@algoskip}{\smallskip}%
\newcommand{\SetAlgoSkip}[1]{\renewcommand{\@algoskip}{\csname#1\endcsname}}%
\newcommand{\@algoinsideskip}{\relax}%
\newcommand{\SetAlgoInsideSkip}[1]{\renewcommand{\@algoinsideskip}{\csname#1\endcsname}}%
%
% ruledwidth
%
\newlength{\algocf@ruledwidth}\setlength{\algocf@ruledwidth}{\linewidth}%
\newboolean{algocf@customruledwidth}\setboolean{algocf@customruledwidth}{false}%
\newcommand{\SetCustomAlgoRuledWidth}[1]{%
  \setboolean{algocf@customruledwidth}{true}%
  \ifthenelse{\boolean{algocf@customruledwidth}}{\setlength{\algocf@ruledwidth}{#1}}{\relax}%
}%
%
\newsavebox{\algocf@inoutbox}%
\newsavebox{\algocf@inputbox}%
%%
%%
\newcommand{\arg@e}{}%
\newcommand{\arg@space}{\ }%
\newcommand{\BlankLine}{\vskip 1ex}%
%%
\newcommand{\vespace}{1ex}%
\newcommand{\SetInd}[2]{%
\skiprule=#1%
\skiptext=#2%
\skiplength=\skiptext\advance\skiplength by \skiprule\advance\skiplength by 0.4pt}%
\SetInd{0.5em}{1em}
\algomargin=\leftskip\advance\algomargin by \parindent%
\newcommand{\IncMargin}[1]{\advance\algomargin by #1}%
\newcommand{\DecMargin}[1]{\advance\algomargin by -#1}%
\newcommand{\SetNlSkip}[1]{%
  \renewcommand{\@defaultskiptotal}{#1}%
  \setlength{\skiptotal}{#1}}%
%%
\newskip\AlCapSkip\AlCapSkip=0ex%
\newskip\AlCapHSkip\AlCapSkip=0ex%
\newcommand{\SetAlCapSkip}[1]{\setlength{\AlCapSkip}{#1}}%
\newcommand{\SetAlCapHSkip}[1]{\setlength{\AlCapHSkip}{#1}}%
\SetAlCapHSkip{.5\algomargin}%
%%
%%
\newskip\algoskipindent
\newcommand{\algocf@adjustskipindent}{%
  \algoskipindent=\skiprule%
  \advance\algoskipindent by \skiptext\advance\algoskipindent by 0.4pt}
\algocf@adjustskipindent%
%
\newcommand{\Indentp}[1]{\advance\leftskip by #1}%
\newcommand{\Indp}{\algocf@adjustskipindent\advance\leftskip by \algoskipindent}
\newcommand{\Indpp}{\advance\leftskip by 0.5em}%
\newcommand{\Indm}{\algocf@adjustskipindent\advance\leftskip by -\algoskipindent}
\newcommand{\Indmm}{\advance\leftskip by -0.5em}%
%
%%
%%
%% Line Numbering
%%
%%
% number line style
\newcommand{\algocf@nlrelsize}{-2}\newcommand{\SetAlgoNlRelativeSize}[1]{\renewcommand{\algocf@nlrelsize}{#1}}%
\newcommand{\NlSty}[1]{\textnormal{\textbf{\relsize{\algocf@nlrelsize}#1}}}% default definition
\newcommand{\SetNlSty}[3]{\renewcommand{\NlSty}[1]{\textnormal{\csname#1\endcsname{\relsize{\algocf@nlrelsize}#2##1#3}}}}%
%
% nl definitions
%
\newsavebox{\algocf@nlbox}%
\newcommand{\algocf@printnl}[1]{%
  \ifthenelse{\boolean{algocf@leftlinenumber}}{%
    \skiplinenumber=\skiptotal\advance\skiplinenumber by\leftskip%
    \strut\raisebox{0pt}{\llap{\NlSty{#1}\kern\skiplinenumber}}\ignorespaces%
  }{%
    \sbox\algocf@nlbox{\NlSty{#1}}%
    \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip\advance\skiplinenumber by-\skiptext%
    \advance\skiplinenumber by\algomargin\advance\skiplinenumber by.3em\advance\skiplinenumber by-\wd\algocf@nlbox%
    % to handle particular case of until: printnl is after 'until' keyword has been writen, so we need to substract length of this keyword
    \advance\skiplinenumber by-\algocf@skipuntil%
    \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\NlSty{#1\ignorespaces}}}\ignorespaces%
  }%
}%
\newcommand{\algocf@nl@sethref}[1]{%
  \renewcommand{\theHAlgoLine}{\thealgocfproc.#1}%
  \hyper@refstepcounter{AlgoLine}\gdef\@currentlabel{#1}%
}%
\newcommand{\nl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \algocf@printnl{\theAlgoLine}%
}%
%
\newcommand{\nllabel}[1]{\label{#1}}%
%
\newcommand{\enl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip%
  \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\strut\NlSty{\theAlgoLine}}}\ignorespaces%
}%
%% nlset
\newcommand{\nlset}[1]{%
  \@ifundefined{hyper@refstepcounter}{\protected@edef\@currentlabel{#1}}{\algocf@nl@sethref{#1}}\algocf@printnl{#1}%
}%
%
%% lnl definitions
\newcommand{\lnl}[1]{\nl\label{#1}\ignorespaces}%
%
%% lnlset
\newcommand{\lnlset}[2]{\nlset{#2}\label{#1}}%
%
% set char put at end of each line
%
\newcommand{\algocf@endline}{\string;}
\newcommand{\SetEndCharOfAlgoLine}[1]{\renewcommand{\algocf@endline}{#1}}
%
% end of line definition
%
\newcommand{\@endalgocfline}{\algocf@endline}% default definition: printsemicolon
\newcommand{\DontPrintSemicolon}{\renewcommand{\@endalgocfline}{\relax}}%
\newcommand{\PrintSemicolon}{\renewcommand{\@endalgocfline}{\algocf@endline}}%
\newcommand{\@endalgoln}{\@endalgocfline\hfill\strut\par}%
%
% line numbering
%
\newcommand{\LinesNumbered}{\setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}}%
\newcommand{\LinesNotNumbered}{%
  \setboolean{algocf@linesnumbered}{false}%
  \renewcommand{\algocf@linesnumbered}{\relax}%
}%
%
\newcommand{\LinesNumberedHidden}{%
  \setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}}%
\newcommand{\ShowLn}{\nlset{\theAlgoLine}\ignorespaces}% display the line number on this line (without labelling)
\newcommand{\ShowLnLabel}[1]{\lnlset{#1}{\theAlgoLine}\ignorespaces}% display the line number and label this line
%
%%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Styling text commands
%
\newcommand{\AlFnt}{\relax}% default definition
\newcommand{\SetAlFnt}[1]{\renewcommand{\AlFnt}{#1}}%
\newcommand{\AlTitleFnt}{\relax}% default definition
\newcommand{\SetAlTitleFnt}[1]{\renewcommand{\AlTitleFnt}{#1}}%
%
\newcommand{\AlCapFnt}{\relax}% default definition
\newcommand{\SetAlCapFnt}[1]{\renewcommand{\AlCapFnt}{#1}}%
\newcommand{\AlCapNameFnt}{\relax}% default definition
\newcommand{\SetAlCapNameFnt}[1]{\renewcommand{\AlCapNameFnt}{#1}}%
%
\newcommand{\ProcFnt}{\relax}% default definition
\newcommand{\SetProcFnt}[1]{\renewcommand{\ProcFnt}{#1}}%
\newcommand{\ProcNameFnt}{\relax}% default definition
\newcommand{\SetProcNameFnt}[1]{\renewcommand{\ProcNameFnt}{#1}}%
\newcommand{\ProcArgFnt}{\relax}% default definition
\newcommand{\SetProcArgFnt}[1]{\renewcommand{\ProcArgFnt}{#1}}%
%
\newcommand{\AlTitleSty}[1]{\textbf{#1}\unskip}% default definition
\newcommand{\SetAlTitleSty}[1]{\renewcommand{\AlTitleSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetAlCapSty}[1]{\renewcommand{\AlCapSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapNameSty}[1]{\textnormal{#1}\unskip}% default definition
\newcommand{\SetAlCapNameSty}[1]{\renewcommand{\AlCapNameSty}[1]{\textnormal{\csname #1\endcsname{##1}}\unskip}}%
%
\newcommand{\ProcSty}[1]{\AlCapSty{#1}}%
\newcommand{\SetProcSty}[1]{\renewcommand{\ProcSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcNameSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcNameSty}[1]{\renewcommand{\ProcNameSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcArgSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcArgSty}[1]{\renewcommand{\ProcArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
\newcommand{\KwSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetKwSty}[1]{\renewcommand{\KwSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetArgSty{emph}
\newcommand{\SetArgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetFuncArgSty{emph}
\newcommand{\SetFuncArgSty}[1]{\renewcommand{\FuncArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncSty}[1]{\textnormal{\texttt{#1}}\unskip}%\SetFuncSty{texttt}
\newcommand{\SetFuncSty}[1]{\renewcommand{\FuncSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetProgSty{emphg}
\newcommand{\SetProgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\DataSty}[1]{\textnormal{\textsf{#1}}\unskip}%%\SetDataSty{textsf}
\newcommand{\SetDataSty}[1]{\renewcommand{\DataSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\CommentSty}[1]{\textnormal{\texttt{#1}}\unskip}%%\SetDataSty{texttt}
\newcommand{\SetCommentSty}[1]{\renewcommand{\CommentSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\TitleSty}[1]{#1\unskip}%\SetTitleSty{}{}
\newcommand{\SetTitleSty}[2]{\renewcommand{\TitleSty}[1]{%
\csname#1\endcsname{\csname#2\endcsname##1}}\unskip}%
\newcommand{\BlockMarkersSty}[1]{\KwSty{#1}}%
\newcommand{\SetBlockMarkersSty}[1]{\renewcommand{\BlockMarkersSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Block basic commands
%
\newcommand{\algocf@push}[1]{\advance\skiptotal by #1\moveright #1}%
\newcommand{\algocf@pop}[1]{\advance\skiptotal by -#1}%
\newcommand{\algocf@addskiptotal}{\advance\skiptotal by 0.4pt\advance\hsize by -0.4pt\advance\hsize by -\skiplength}% 0.4 pt=width of \vrule
\newcommand{\algocf@subskiptotal}{\advance\skiptotal by -0.4pt\advance\hsize by 0.4pt\advance\hsize by \skiplength}% 0.4 pt=width of \vrule
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% group of instructions definition
%
\skiphlne=.8ex%
\newcommand{\SetVlineSkip}[1]{\skiphlne=#1}%
\newcommand{\algocf@bblock}{\BlockMarkersSty{begin}}%
\newcommand{\algocf@eblock}{\BlockMarkersSty{end}}%
\newcommand{\AlgoDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{true}}%
\newcommand{\AlgoDontDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{false}}%
\newcommand{\AlgoDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{true}}%
\newcommand{\AlgoDontDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{false}}%
\newcommand{\algocf@bblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@bblock\par}{\relax}%
}%
\newcommand{\algocf@eblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@eblock\par}{\relax}%
}%
\newcommand{\algocf@bgroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@bblock}{\relax}%
}%
\newcommand{\algocf@egroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@eblock}{\relax}%
}%
\newcommand{\SetAlgoBlockMarkers}[2]{%
  \ifArgumentEmpty{#1}{%
    \renewcommand{\algocf@bblock}{\relax}%
  }{%
    \renewcommand{\algocf@bblock}{\BlockMarkersSty{#1}}%
  }% begin marker set
  \ifArgumentEmpty{#2}{%
    \renewcommand{\algocf@eblock}{\relax}%
  }{%
    \renewcommand{\algocf@eblock}{\BlockMarkersSty{#2}}%
  }% end marker set
}
%
%%%%%%%%% block with a vertical line end by a little horizontal line
\newcommand{\algocf@Vline}[1]{%     no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}\Hlne}}\vskip\skiphlne% inside the block
  \algocf@pop{\skiprule}%\algocf@subskiptotal% restore indentation
  \nointerlineskip}% no vskip after
%
%%%%%%%%% block with a vertical line
\newcommand{\algocf@Vsline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%               the vertical rule
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}% restore indentation
  \algocf@eblockcode%
}
%
\newcommand{\algocf@Hlne}{\hrule height 0.4pt depth 0pt width .5em}%
%
%%%%%%%%%  block without line
\newcommand{\algocf@Noline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%
  \hbox{%
    \vtop{\algocf@push{\skiptext}%
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}%
  \algocf@eblockcode%
  % \nointerlineskip% no vskip after
}%
%%%%%%%%%
%
%% default=NoLine
%
\newcommand{\algocf@group}[1]{\algocf@Noline{#1}}% group: set of instruction depending from another (ex: then part of the If)
\newcommand{\algocf@@@eblock}[2]{#1\ifArgumentEmpty{#2}{\relax}{\KwSty{\@algocf@endoption{#2}}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@@block}[3]{#1\ifArgumentEmpty{#2}{\ifArgumentEmpty{#3}{\relax}{ #3\relax}}{\KwSty{\@algocf@endoption{#2}}\ifArgumentEmpty{#3}{\relax}{ #3}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@block}[3]{\algocf@@@block{#1}{#2}{#3}}% block: group with a end keyword.
\newcommand{\algocf@block}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
%\newcommand{\algocf@nblock}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
\newcommand{\algocf@setBlock}{%
  \ifthenelse{\boolean{algocf@optnoend}}{%     if no end option
    \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%     block will be a group
  }{%                                          else
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}% block stays a block
  }%
}%
%
\newcommand{\Hlne}{}% little hrizontal line ending a block in vline mode
%
\newcommand{\@algocf@endoption}[1]{#1}%
\newboolean{algocf@optnoend}\setboolean{algocf@optnoend}{false}%
%
\newcommand{\SetAlgoLongEnd}{%%%%%%%%%%%%%%%%%%%%%%%%% Long End
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{##1}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoShortEnd}{%%%%%%%%%%%%%%%%%%%%%%%% ShortEnd
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{\@firstword##1 \@nil}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoEnd}{%%%%%%%%%%%%%%%%%%%%%%%%%%% NoEnd
  \setboolean{algocf@optnoend}{true}%
  \renewcommand{\@algocf@endoption}[1]{}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoLine}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\algocf@Noline{##1}}{##2}}%
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetAlgoVlined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Vline
\renewcommand{\algocf@@block}[2]{\algocf@Vline{##1}}%
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{\algocf@Hlne}}%
%
\newcommand{\SetAlgoLined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\strut\algocf@Vsline{##1}}{##2}}% no skip after a block so garantie at least one line
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetNothing}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@Noline{##1}\par}%
%\long
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
%%
%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ``Input:'''s like command 
%
%%%
% text staying at the right of the longer keyword of KwInOut commands 
% (text of KwInOut commands are all vertically aligned)
%
\newcommand{\algocf@newinout}{\par\parindent=\inoutindent}% to put right indentation after a \\ in the KwInOut
\newcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2\algocf@typo:}}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else% else keep the larger dimension
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi% the dimension of the box is now defined.
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
%
%% allow to ajust the skip size of InOut
%%
\newcommand{\ResetInOut}[1]{%
  \sbox\algocf@inoutbox{\hbox{\KwSty{#1\algocf@typo:}\ }}%
  \setlength{\inoutsize}{\wd\algocf@inoutbox}%
  }%
%
% 
%%%
% text staying at the right of the keyword.
%
\newcommand{\algocf@newinput}{\par\parindent=\wd\algocf@inputbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwInput}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@inputbox{\hbox{\KwSty{#2\algocf@typo:} }}%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
    {\let\\\algocf@newinput\hangindent=\wd\algocf@inputbox\hangafter=1\unhbox\algocf@inputbox##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
\newcommand{\SetKwData}[2]{%
  \algocf@newcommand{@#1}[1]{\DataSty{#2(}\ArgSty{##1}\DataSty{)}}%
  \algocf@newcommand{#1}{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
  }%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tallent:
%
% Add following macros:
%   \SetKwHangingKw:  [kw] ------------   <= hanging determined by [kw]
%                          ------------
% Should act like a combination of \SetKwInput and \SetKw.
% Based on \SetKwInput:
%   - remove ':' at end of keyword
%   - do not reset numbering
%   - use separate savebox
\newsavebox{\algocf@hangingbox}
\newcommand{\algocf@newhanging}{\par\parindent=\wd\algocf@hangingbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwHangingKw}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@hangingbox{\hbox{\KwSty{#2}\algocf@typo\ }}%
    {\let\\\algocf@newhanging\hangindent=\wd\algocf@hangingbox\hangafter=1\unhbox\algocf@hangingbox##1\;}%
  }%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Comments macros
%
%%%%
% comment in the text, first argument is the name of the macro, second is
% the text put before the comment, third is the text put at the end of the
% comment.
%
% first side comment justification
\newcommand{\SetSideCommentLeft}{\setboolean{algocf@scleft}{true}}%
\newcommand{\SetSideCommentRight}{\setboolean{algocf@scleft}{false}}%
\newcommand{\SetNoFillComment}{\setboolean{algocf@optfillcomment}{false}}%
\newcommand{\SetFillComment}{\setboolean{algocf@optfillcomment}{true}}%
%
% next comment and side comment
%
\newcommand{\algocf@endmarkcomment}{\relax}%
\newcommand{\algocf@fillcomment}{%
  \ifthenelse{\boolean{algocf@optfillcomment}}{\hfill}{\relax}}%
%
\newcommand{\algocf@startcomment}{%
  \hangindent=\wd\algocf@inputbox\hangafter=1\usebox\algocf@inputbox}%
\newcommand{\algocf@endcomment}{\algocf@fillcomment\algocf@endmarkcomment\ignorespaces\par}%
\newcommand{\algocf@endstartcomment}{\algocf@endcomment\algocf@startcomment\ignorespaces}%
%
\newboolean{algocf@sidecomment}%
\newboolean{algocf@altsidecomment}\setboolean{algocf@altsidecomment}{false}%
\newcommand{\algocf@scpar}{\ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\par}}%
\newcommand{\algocf@sclfill}{\ifthenelse{\boolean{algocf@scleft}}{\algocf@fillcomment}{\relax}}%
\newcommand{\algocf@scrfill}{\ifthenelse{\boolean{algocf@scleft}}{\relax}{\hfill}}%
\newcommand{\algocf@startsidecomment}{\usebox\algocf@inputbox}%
\newcommand{\algocf@endsidecomment}{\algocf@endmarkcomment\algocf@scpar}%
\newcommand{\algocf@endstartsidecomment}{%
  \algocf@sclfill\algocf@endsidecomment%
  \algocf@scrfill\algocf@startsidecomment\ignorespaces}%
%
\newcommand{\SetKwComment}[3]{%
  \algocf@newcommand{#1}{\@ifstar{\csname algocf@#1@star\endcsname}{\csname algocf@#1\endcsname}}%
	\algocf@newcommand{algocf@#1}[1]{%
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@seteveryparhanging{\relax}}%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {\renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartcomment%
        \algocf@startcomment\CommentSty{%
          \strut\ignorespaces##1\strut\algocf@fillcomment#3}\par}%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@reseteveryparhanging}%
    }%
  %%% side comment definitions
	\algocf@newcommand{algocf@#1@star}[2][]{%
      \ifArgumentEmpty{##1}\relax{% TODO: Is this even necessary, with all those \ifx's?
        \ifthenelse{\boolean{algocf@scleft}}{\setboolean{algocf@sidecomment}{true}}{\setboolean{algocf@sidecomment}{false}}%
        \ifx##1h\setboolean{algocf@altsidecomment}{true}\SetSideCommentLeft\fi%
        \ifx##1f\setboolean{algocf@altsidecomment}{true}\SetSideCommentRight\fi%
        \ifx##1l\setboolean{algocf@altsidecomment}{false}\SetSideCommentLeft\fi%
        \ifx##1r\setboolean{algocf@altsidecomment}{false}\SetSideCommentRight\fi%
      }%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {%
        \renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartsidecomment%
        % here is the comment
        \ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\@endalgocfline\ }%
        \algocf@scrfill\algocf@startsidecomment\CommentSty{%
          \strut\ignorespaces##2\strut\algocf@sclfill#3}\algocf@scpar%
      }%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifArgumentEmpty{##1}\relax{%
        \ifthenelse{\boolean{algocf@sidecomment}}{\setboolean{algocf@scleft}{true}}{\setboolean{algocf@scleft}{false}}%
        \setboolean{algocf@altsidecomment}{false}%
      }%
	}%
  }%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwProg
%
\newcommand{\SetKwProg}[4]{%\SetKwProg{Env}{Title}{is}{end} 
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\ifArgumentEmpty{#2}\relax{\ }\ProgSty{##2}\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode\@endalgocfline\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Kw
%
\newcommand{\SetKw}[2]{%
	\algocf@newcommand{@#1}[1]{\KwSty{#2} \ArgSty{##1}}
	\algocf@newcommand{#1}{\@ifnextchar\bgroup{\csname @#1\endcsname}{\KwSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwFunction
%
\newcommand{\SetKwFunction}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\FuncSty{#2(}\FuncArgSty{##1}\FuncSty{)}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\FuncSty{#2}\xspace}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwTab
%
\newcommand{\SetKwArray}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\DataSty{#2[}\ArgSty{##1}\DataSty{]}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwBlock
%
\newcommand{\SetKwBlock}[3]{%
	\algocf@newcmdside@kobe{#1}%
    {\KwSty{#2}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#3}{##3}\par}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% condition typo
%
\newcommand{\algocf@scond}{\ }
\newcommand{\algocf@econd}{\ }
\newcommand{\algocf@ucond}{}
\newcommand{\SetStartEndCondition}[3]{%
  \renewcommand{\algocf@scond}{#1}\renewcommand{\algocf@econd}{#2}\renewcommand{\algocf@ucond}{#3}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For Switch
%
\newcommand{\SetKwSwitch}[9]{% #1=\Switch #2=\Case #3=\Other #4=switch #5=do #6=case #7=otherwise #8=endcase #9=endsw
%	\algocf@newcmdside{#1}{3}%
	\algocf@newcmdside@koif{#1}%
		{\KwSty{#4}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#9} {##4\relax}}%
%%%% Case
	\algocf@newcmdside@koif{#2}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#8}{##4\relax}}%
    %uCase
	\algocf@newcmdside{u#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##3}}%
    %lcase
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\ \relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
%%%% Other 
	\algocf@newcmdside@kobe{#3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#8}{##3\relax}}%
    %lOther
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\algocf@egroupcode}%
    %uOther
	\algocf@newcmdside{u#3}{3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##2}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% If macros
%
\newcommand{\SetKwIF}[8]{% #1=\If #2=\ElseIf #3=\Else #4=if #5=then #6=elseif #7=else #8=endif
% 
% common text
	\algocf@newcommand{#1@ifthen}[1]{\KwSty{#4}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#1@endif} [2]{\algocf@block{##1}{#8}{##2}}%
	\algocf@newcommand{#1@noend} [1]{\algocf@group{##1}}%
	\algocf@newcommand{#1@else}  [1]{\algocf@group{##1}\KwSty{#7}}%
	\algocf@newcommand{#2@elseif}[1]{\KwSty{#6}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#3@else}     {\KwSty{#7}}%
%%%% If then { } endif
	\algocf@newcmdside@koif{#1}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% If then {} else {} endif
    % first command to handle optional side comment of else (so just after first braces)
 	\algocf@newcmdside@kobe{algocf@e#1thenelse}{\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##2}{##3}}%
    % the definition of if-then-else command using command above 
	\algocf@newcmdside{e#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@else\endcsname{##3}\csname algocf@e#1thenelse\endcsname}%
    %%% leif
    \algocf@newcommand{le#1}{\@ifstar{\csname algocf@le#1star\endcsname}{\csname algocf@le#1\endcsname}}%
    \algocf@newcmdside{algocf@le#1}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\@endalgocfline\ \algocf@egroupcode\ifArgumentEmpty{##1}\relax{##1}\strut\par}%
    \algocf@newcmdside{algocf@le#1star}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\algocf@egroupcode}%
%%%% If then 
	% \algocf@newcmdside{l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\
    % ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@noend\endcsname{##3}}%
%%%% ElseIf {} endif
	\algocf@newcmdside@koif{#2}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% ElseIf
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#2}{3}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{##1}\csname #1@noend\endcsname{##3}}%
%%%% Else {} endif
	\algocf@newcmdside@kobe{#3}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ ##1\csname #1@endif\endcsname{##2}{##3\relax}}%
%%%% Else 
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\algocf@egroupcode}%
	\algocf@newcmdside{u#3}{2}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ {##1\relax}\csname #1@noend\endcsname{##2}}%
}% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For macros
%
\newcommand{\SetKwFor}[4]{%
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4\relax}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Repeat macros
%
\newsavebox{\algocf@untilbox}% to handle width of until keyword needed to have good skip
  % for line numbers
\newskip\algocf@skipuntil
\newcommand{\SetKwRepeat}[3]{%
	\algocf@newcmdsides{#1}{3}{%
      \sbox\algocf@untilbox{\KwSty{#3}\algocf@scond}\algocf@skipuntil=\wd\algocf@untilbox%
      \KwSty{#2}\ifArgumentEmpty{##1}\relax{##1}\algocf@group{##3}%
      \KwSty{#3}\algocf@scond% until keyword and start condition typo
      %\advance\skiptotal by\algocf@skipuntil%
      \ArgSty{##2}%
      %\advance\skiptotal by-\algocf@skipuntil%
      \algocf@ucond%
      \algocf@skipuntil=0pt% reset counter
    }{\@endalgocfline}{\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond\@endalgocfline\ifArgumentEmpty{##1}\relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond}%
}%
%
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%        Environments definitions     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%
%% Caption management
%%
% for the following macros:
% #1 is given by caption and is equal to fnum@algocf
% #2 is the text given in argument by the user in the \caption macro
%
%%%%% text of caption
\newcommand{\algocf@captionlayout}[1]{#1}%
\newcommand{\SetAlgoCaptionLayout}[1]{%
  \renewcommand{\algocf@captionlayout}[1]{\csname #1\endcsname{##1}}}%
\newcommand{\algocf@capseparator}{:}%
\newcommand{\SetAlgoCaptionSeparator}[1]{\renewcommand{\algocf@capseparator}{#1}}%
\newcommand{\algocf@captiontext}[2]{%
  \algocf@captionlayout{\AlCapSty{\AlCapFnt #1\algocf@typo\algocf@capseparator}\nobreakspace%
    \AlCapNameSty{\AlCapNameFnt{}#2\endgraf}}}% text of caption
%
%%%%% default caption of algorithm: used if no specific style caption is defined
\newcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}%
%
\newsavebox\algocf@capbox%
\newcommand{\algocf@makecaption@plain}[2]{%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}}%
\newcommand{\algocf@makecaption@boxed}[2]{%
  \addtolength{\hsize}{-\algomargin}%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}%
  \addtolength{\hsize}{\algomargin}%
 }%
%
\newcommand{\algocf@makecaption@plainruled}[2]{\algocf@makecaption@plain{#1}{#2}}%
\newcommand{\algocf@makecaption@tworuled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@algoruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@boxruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@ruled}[2]{%
  \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}}% then caption is not centered
}%
%
\newlength{\algoheightruledefault}\setlength{\algoheightruledefault}{0.8pt}%
\newlength{\algoheightrule}\setlength{\algoheightrule}{\algoheightruledefault}%
\newlength{\algotitleheightruledefault}\setlength{\algotitleheightruledefault}{0.8pt}%
\newlength{\algotitleheightrule}\setlength{\algotitleheightrule}{\algotitleheightruledefault}%
\newcommand{\algocf@caption@plain}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@plainruled}{\algocf@caption@plain}%
\newcommand{\algocf@caption@boxed}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@ruled}{\box\algocf@capbox\kern\interspacetitleruled\hrule
  width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@tworuled}{\box\algocf@capbox\hrule  height0pt depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@algoruled}{\algocf@caption@ruled}%
\newcommand{\algocf@caption@boxruled}{%
  \addtolength{\hsize}{-0.8pt}%
  \hbox to\hsize{%
    \vrule%\hskip-0.35pt%
    \vbox{%
      \hrule\vskip\interspacetitleboxruled%
      \hbox to\hsize{\unhbox\algocf@capbox\hfill}\vskip\interspacetitleboxruled%
    }% 
    %\hskip-0.35pt%
    \vrule%
  }\nointerlineskip%
  \addtolength{\hsize}{0.8pt}%
}%
%
%
%%%% set caption for the environment
\newcommand{\algocf@captionref}{%
  \renewcommand{\fnum@algocf}[1]{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\algocf@algocfref}}%
  \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
  \let\old@thealgocf=\thealgocf\renewcommand{\thealgocf}{{\relsize{\algocf@refrelsize}\algocf@algocfref}}%
  \gdef\@currentlabel{\algocf@algocfref}% let the label use the new ref
}%
%
% Unfortunatly, we also need our own caption to set some specific stuff for special references. But after these
% settings, we call the original caption.
%
\long\def\algocf@caption@algo#1[#2]#3{%
  \ifthenelse{\equal{\algocf@algocfref}{\relax}}{}{\algocf@captionref}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\equal{\algocf@algocfref}{\relax}}{\renewcommand{\theHalgocf}{\thealgocf}}{% take algocf as Href
      \renewcommand{\theHalgocf}{\algocf@algocfref}}%else if SetAlgoRefName done, take this name as ref.
    \hyper@refstepcounter{algocf}%set algocf as category of ref
  }%
   \algocf@latexcaption{#1}[{#2}]{{#3}}% call original caption
}%
%
% beamer define is own caption overrinding latex caption!
% as we need it, we have put here the original definition
% to handle manual ref, unfortunately we have to add one line to handle algocf@algocfref
\long\def\algocf@latexcaption#1[#2]#3{% original definition of caption
  \par%
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
  {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup%
  \@parboxrestore%
  \if@minipage%
    \@setminipage%
  \fi%
  \normalsize%
  \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par%
  \endgroup%
}%
%
% \ifx\beamer@makecaption\undefined%
% \else% beamer detected
\ifx\@makecaption\undefined%
\newcommand{\@makecaption}[2]{\relax}%
\fi%
%%

%
% more and more packages redefine \@caption instead of just \@makecaption which makes algorithm2e
% caption not works since based on standard \@caption. So we force the definition of \@caption to be
% the standard one (the one from LaTeX) inside algorithm environment.
%
% unfortunately, makecaption is called with \ignorespace #3 so 
% we can't do the @currentlabel definition inside \algocf@captionproctext
\long\def\algocf@caption@proc#1[#2]#3{%
  \ifthenelse{\boolean{algocf@nokwfunc}}{\relax}{%
    \SetKwFunction{\algocf@captname#3@}{\algocf@captname#3@}%
  }%
  % we tell hyperref to use algocfproc as category and to take the appropriate ref.
  \ifthenelse{\boolean{algocf@func}}{\def\@proc@func{algocffunc}}{\def\@proc@func{algocfproc}}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\boolean{algocf@procnumbered}}{% 
      \expandafter\def\csname theH\@proc@func\endcsname{\thealgocf}%if procnumbered, take \thealgocf as ref
    }{%
      \expandafter\def\csname theH\@proc@func\endcsname{\algocf@captname#3@}%else take procedure or function name
    }%
    \hyper@refstepcounter{\@proc@func}%
  }%
  \ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
    \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
    \gdef\@currentlabel{\algocf@captname#3@}% let the label be the name of the function, not the counter
  }%
  \ifthenelse{\equal{\algocf@captparam#2@}{\arg@e}}{% if no paramater, we remove the ()
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace\algocf@captname#2@]{#3}%
  }{%                                                 else we give the complete name
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace#2]{#3}%
  }%
}%
%%
%%% setcaption
\newcommand{\algocf@setcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment, caption text must be changed
    \let\algocf@oldcaptiontext=\algocf@captiontext%
    \renewcommand{\algocf@captiontext}[2]{%
      \algocf@captionproctext{##1}{##2}%
    }%
  }{}%
  \let\algocf@savecaption=\@caption%
  \ifthenelse{\boolean{algocf@procenvironment}}{\let\@caption=\algocf@caption@proc}{\let\@caption=\algocf@caption@algo}%
  \let\algocf@oldmakecaption=\@makecaption%
  \renewcommand{\@makecaption}[2]{%
    \expandafter\csname algocf@makecaption@\algocf@style\endcsname{##1}{##2}%
  }%
}%
%
%%%%% reset caption
%
% since we have force the LaTeX caption for algorithm environment, we must go back to the caption
% used in the text.
\newcommand{\algocf@resetcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment
    \let\thealgocf=\old@thealgocf% restore normal counter printing
    \let\algocf@captiontext=\algocf@oldcaptiontext% restore normal caption text
  }{}%
  \let\@caption=\algocf@savecaption% now restore caption outside algo/proc/func environment
  \let\@makecaption=\algocf@oldmakecaption% and restore makecaption outside outside algo/proc/func environment
  \algocf@resetfnum%
}%
%
%%%%% nocaptionofalgo and restorecaptionofalgo --
\newcommand{\NoCaptionOfAlgo}{%
  \let\@old@algocf@captiontext=\algocf@captiontext%
  \renewcommand{\algocf@captiontext}[2]{\AlCapNameSty{\AlCapNameFnt{}##2}}%
}%
\newcommand{\RestoreCaptionOfAlgo}{%
  \let\algocf@captiontext=\@old@algocf@captiontext%
}%
%
% ----------------------  algocf environment
%
\newcounter{algocfline}%                    % new counter to make lines numbers be internally 
\setcounter{algocfline}{0}%                 % different in different algorithms
\newcounter{algocfproc}% counter to count all algo environment (proc, func), just used by hyperref to avoir "same
\setcounter{algocfproc}{0}% identifier" error caused by algocf being set to '-' for procedure or function or not
  % changed if no caption is given.
%
\expandafter\ifx\csname algocf@within\endcsname\relax% if \algocf@within doesn't exist
\newcounter{algocf}%                        % just define a new counter
\renewcommand{\thealgocf}{\@arabic\c@algocf}% and the way it is printed
\else%                                     else
\newcounter{algocf}[\algocf@within]%        % counter is numbered within \algocf@within
\renewcommand\thealgocf{\csname the\algocf@within\endcsname.\@arabic\c@algocf}%
\fi%
%
\def\fps@algocf{htbp}%        % default
\def\ftype@algocf{10}%        % float type
\def\ext@algocf{\algocf@list} % loa by default, lof if figure option used
\newcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}%
\newcommand{\algocf@resetfnum}{\renewcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}}%
\newenvironment{algocf}%      % float environment for algorithms
               {\@float{algocf}}%
               {\end@float}%
\newenvironment{algocf*}%     % float* environment for algorithms
               {\@dblfloat{algocf}}%
               {\end@dblfloat}%
%
\def\algocf@seclistalgo{}%
\ifx\l@chapter\undefined\let\algocf@seclistalgo=\section\else\let\algocf@seclistalgo=\chapter\fi%
\@ifundefined{if@restonecol}{\newif\if@restonecol}\relax%
\newcommand\listofalgocfs{%
     \ifx\algocf@seclistalgo\chapter%
      \if@twocolumn\@restonecoltrue\onecolumn\else\@restonecolfalse\fi%
    \fi%
     \algocf@seclistalgo*{\listalgorithmcfname}%
       \@mkboth{\MakeUppercase\listalgorithmcfname}%
               {\MakeUppercase\listalgorithmcfname}%
     \@starttoc{loa}%
    \ifx\algocf@seclistalgo\chapter%
      \if@restonecol\twocolumn\fi%
    \fi%
}
%
\newcommand*\l@algocf{\@dottedtocline{1}{1em}{2.3em}}% line of the list
%
% ----------------------  algorithm environment
%
%%%%%%%
%%
%% Algorithm environment definition
%%
%%%%%%%
%%
%
\newsavebox\algocf@algoframe%
\def\@algocf@pre@plain{\relax}%  action to be done before printing the algo.
\def\@algocf@post@plain{\relax}% action to be done after printing the algo.
\def\@algocf@capt@plain{bottom}% where the caption should be localized.
\def\@algocf@pre@boxed{\noindent\begin{lrbox}{\algocf@algoframe}}
\def\@algocf@post@boxed{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxed{under}%
\def\@algocf@pre@ruled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@ruled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@ruled{top}%
\def\@algocf@pre@algoruled{\hrule width\algocf@ruledwidth height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@algoruled{\kern\interspacealgoruled\hrule width\algocf@ruledwidth height\algoheightrule \relax}%
\def\@algocf@capt@algoruled{top}%
\def\@algocf@pre@tworuled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@tworuled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@tworuled{top}%
\def\@algocf@pre@boxruled{\noindent\begin{lrbox}{\algocf@algoframe}}%
\def\@algocf@post@boxruled{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxruled{above}%
\def\@algocf@pre@plainruled{\@algocf@pre@ruled}%  action to be done before printing the algo.
\def\@algocf@post@plainruled{\@algocf@post@ruled\kern\interspacealgoruled}%  action to be done before printing the algo.
\def\@algocf@capt@plainruled{under}%
%
\newcommand{\noalgocaption}{\def\@algocf@capt@ruled{none}}
%
%% before algocf environment (not figure environment)
\newcommand{\@algocf@init@caption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if we are inside a procedure/function environment
    \@algocf@proctitleofalgo% set Titleofalgo to Procedure: or Function:
                            % accordingly to the environment
    \let\old@thealgocf=\thealgocf\ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
      \renewcommand{\thealgocf}{-}}%
  }{% else inside environment algorithm
    \@algocf@algotitleofalgo% fix name for \Titleofalgo to \algorithmcfname
  }%
  \algocf@setcaption%       set caption to our caption style
}%
%
\newcommand{\@algofloatboxreset}{\@setminipage}
\newcommand{\@algocf@init}{%
  \refstepcounter{algocfline}%
  \stepcounter{algocfproc}%to have a different counter for each environment and being abble to make the difference
    %between href of algoline in different algorithms.
  \ifthenelse{\boolean{algocf@optnoend}}{%
      \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%
    }{%
      \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
    }%
}%
%% after the end of algocf or figure environment
\newcommand{\@algocf@term@caption}{%
  \algocf@resetcaption% restore original caption
}%
%
\newcommand{\@algocf@term}{%
  \setboolean{algocf@algoH}{false}% no H by default
  \ifthenelse{\boolean{algocf@optnoend}}{%
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
  }{%
    \renewcommand{\algocf@block}[2]{\algocf@group{##1}}%
  }%
  \SetAlgoRefName{\relax}%
}%
%
%%%%%%%%%%%%%%%%%
%% makethealgo: macro which print effectively the algo in its box
%% 
\newsavebox\algocf@algobox%
\newcommand{\algocf@makethealgo}{%
  \vtop{%
    % place caption above if needed  bye the style
    \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{above}}%
    {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    % precommand according to the style
    \csname @algocf@pre@\algocf@style\endcsname%
    % place caption at top if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{top}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    \box\algocf@algobox% the algo
    % place caption at bottom if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{bottom}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    % postcommand according to the style
    \csname @algocf@post@\algocf@style\endcsname%
    % place caption under if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{under}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
  }%
}%
%%%%%%%%%%%%%%%%%%%
%
%% at the beginning of algocf or figure environment
\newenvironment{algomathdisplay}{\[}{\@endalgocfline\]\ifthenelse{\boolean{algocf@linesnumbered}}{\nl}{\relax}}%
\newcommand{\@algocf@start}{%
  \@algoskip%
  \begin{lrbox}{\algocf@algobox}%
  \setlength{\algowidth}{\hsize}%
  \vbox\bgroup% save all the algo in a box
  \hbox to\algowidth\bgroup\hbox to \algomargin{\hfill}\vtop\bgroup%
  \ifthenelse{\boolean{algocf@slide}}{\parskip 0.5ex\color{black}}{}%
  % initialization
  \addtolength{\hsize}{-1.5\algomargin}%
  \let\@mathsemicolon=\;\def\;{\ifmmode\@mathsemicolon\else\@endalgoln\fi}%
  \raggedright\AlFnt{}%
  \ifthenelse{\boolean{algocf@slide}}{\IncMargin{\skipalgocfslide}}{}%
  \@algoinsideskip%
%   \let\@emathdisplay=\]\def\]{\algocf@endline\@emathdisplay\nl}%
}%
%
%% at the end of algocf or figure environment
\newcommand{\@algocf@finish}{%
  \@algoinsideskip%
  \egroup%end of vtop which contain all the text
  \hfill\egroup%end of hbox wich contains [margin][vtop]
  \ifthenelse{\boolean{algocf@slide}}{\DecMargin{\skipalgocfslide}}{}%
  %
  \egroup%end of main vbox
  \end{lrbox}%
  \algocf@makethealgo% print the algo
  \@algoskip%
  % restore dimension and macros
  \setlength{\hsize}{\algowidth}%
  \lineskip\normallineskip\setlength{\skiptotal}{\@defaultskiptotal}%
  \let\;=\@mathsemicolon%  
  \let\]=\@emathdisplay%
}%
%
%%%%%%%%%%%%%%%%%%%%
%% basic definition of the environment algorithm
%%
%
\newboolean{algocf@procenvironment}\setboolean{algocf@procenvironment}{false}%
\newboolean{algocf@func}\setboolean{algocf@func}{false}%
\newboolean{algocf@algoH}\setboolean{algocf@algoH}{false}%
\newboolean{algocf@algostar}\setboolean{algocf@algostar}{false}%
%
%%% environment for {algorithm}[H]
\newenvironment{algocf@Here}{\noindent%
  \def\@captype{algocf}% if not defined, caption exit with an error
  \begin{minipage}{\hsize}%
}{%
  \end{minipage}%\par%
}%
%%% real algorithm environment which manages H and * option
%    \let\algocf@originalfloatboxreset=\@floatboxreset%
%    \let\@floatboxreset=\@algofloatboxreset%
\newenvironment{algocf@algorithm}[1][htbp]{%
   \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@figurecaption}}{\captionsetup{margin={-\algomargin,\algomargin}}}{}%
   }{}%
   \@algocf@init%
   \ifthenelse{\equal{\algocf@float}{figure}}{% if option figure set
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \begin{figure*}[#1]% call figure*
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else algorithm environment with figure option
       \begin{figure}[#1]%  call figure
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
          \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }%
   }{% else normal algorithm environment
     \@algocf@init@caption%
     \ifthenelse{\equal{#1}{H}}{% if [H] algorithm
       \if@twocolumn\@latex@error{[H] in two columns mode is not allowed for algorithms}\fi% TODO: SCREAM if H in two colums!
       \setboolean{algocf@algoH}{true}\begin{algocf@Here}% call corresponding environment
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \begin{algocf*}[#1]% call algocf*
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }{% else algorithm environment
         \begin{algocf}[#1]%  call algcf
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }%
     }%
   }% fin test option figure ou pas
   \@algocf@start% 
   \@ResetCounterIfNeeded%
   \algocf@linesnumbered\ignorespaces%
}{%
  \@algocf@finish%
  \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure*}% call figure*
     }{% else algorithm environment with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure}%  call figure
     }%
  }{%
    \@algocf@term@caption%
    \ifthenelse{\boolean{algocf@algoH}}{% if [H] algorithm
      \let\everypar=\algocf@oldeverypar%
      \end{algocf@Here}\par% call corresponding environment
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \let\everypar=\algocf@oldeverypar%
         \end{algocf*}% call algocf*
       }{% else algorithm environment
         \let\everypar=\algocf@oldeverypar%
         \end{algocf}%  call algocf
       }%
     }%
  }%
  \@algocf@term\ignorespacesafterend%
}%
%
%%% user algorithm environment
\newenvironment{\algocf@envname}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%%% user algorithm* environment
\newenvironment{\algocf@envname*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%
%%%
%
\expandafter\newcommand\csname\algocf@listofalgorithms\endcsname{%
  \ifthenelse{\equal{\algocf@float}{figure}}{\listoffigures}{\listofalgocfs}%
}%
%%%
%%%
%
% ----------------------  procedure and function environments
%
%
% -- new style (used in particular in the caption of function and procedure environments)
%
% three macros to extract parts of the caption
\gdef\algocf@captname#1(#2)#3@{#1}  % keep characters before the first brace
\gdef\algocf@captparam#1(#2)#3@{#2} % keep character in between the braces
\gdef\algocf@captother#1(#2)#3@{#3} % keep character after the braces
%
%%% Text of caption for Procedure or Function
\newcommand{\algocf@captionproctext}[2]{%
  {%
    \ProcSty{\ProcFnt\algocf@procname\ifthenelse{\boolean{algocf@procnumbered}}{\nobreakspace\thealgocf\algocf@typo\algocf@capseparator}{\relax}}%
    \nobreakspace\ProcNameSty{\ProcNameFnt\algocf@captname #2@}% Name of the procedure in ProcName Style. 
    \ifthenelse{\equal{\algocf@captparam #2@}{\arg@e}}{}{% if no argument, write nothing
      \ProcNameSty{\ProcNameFnt(}\ProcArgSty{\ProcArgFnt\algocf@captparam #2@}\ProcNameSty{\ProcNameFnt)}%else put arguments in ProcArgSty:
    }% endif
    \algocf@captother #2@%
  }%
}%
%
%
% -- procedure and function environments are defined from algocf@algorithm environment
%
\newenvironment{procedure}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
\newenvironment{procedure*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%
%%%%%%%%%%%%%%%%%%%%
%% definition of algondfloat environment
%%
\ifthenelse{\boolean{algocf@endfloat}}{% if endfloat option then
\newcommand{\algoplace}{% macro which is used to writhe algorithm about there
   \begin{center}%
     [\algorithmcfname~\thepostfig\ about here.]%
   \end{center}%
}%
\newcommand{\algoendfloat}{% use as a \begin{algoendfloat} environment to start scanning of line
%  \immediate\openout\@mainfff\jobname.fff%
  \efloat@condopen{fff}
  \efloat@iwrite{fff}{\string\begin{\algocf@envname}}%
    \if@domarkers%
       \ifthenelse{\equal{\algocf@list}{lof}}{%
         \addtocounter{postfig}{1}%
       }{%
         \addtocounter{postalgo}{1}%
       }%
       \algoplace%
    \fi%
    \bgroup%
    \let\do\ef@makeinnocent\dospecials%
    \ef@makeinnocent\^^L% and whatever other special cases
    \endlinechar`\^^M \catcode`\^^M=12 \ef@xalgocfendfloat}%
}{\relax}%%%% end of endfloat option ifthenelse
%% some macros useful for endfloat option that cannot be defined inside the ifthenelse
%scan algoendfloat algorithm and write the text into .fff file
{\catcode`\^^M=12 \endlinechar=-1 %
 \gdef\ef@xalgocfendfloat#1^^M{% scan the lines inside algoendfloat environment being read by latex
   \def\test{#1}% test is the line being currently scan by latex
   \ifx\test\ef@endalgocftest% if it is \end{algoendfloat}
     \def\next{% define next as to not continue the scan and write \end{algorithm} into .fff file
       \egroup\end{algoendfloat}%
       \efloat@iwrite{fff}{\string\end{\algocf@envname}}%
       \efloat@iwrite{fff}{\string\efloatseparator}%
       \efloat@iwrite{fff}{ }%
     }%
     \else% else write the current line being scanned by latex and set next to continue the scan
       \efloat@iwrite{fff}{#1}%
       \let\next\ef@xalgocfendfloat%
     \fi% endif
     \next}% next is continue if it was else condition, else it does not continue the scan and write end to file
}%
% test if the scan is finish by looking at the string \end{algoendfloat}
{\escapechar=-1%
 \xdef\ef@endalgocftest{\string\\end\string\{algoendfloat\string\}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
\newcommand{\TitleOfAlgo}[1]{\@titleprefix\ 
  \TitleSty{#1}\par\smallskip}%
%
\newcommand{\SetAlgorithmName}[3]{%
  \renewcommand{\listalgorithmcfname}{#3}%
  \renewcommand{\algorithmcfname}{#1}%
  \renewcommand{\algorithmautorefname}{#2}%
}%
%
\newcommand{\algocf@refrelsize}{-2}\newcommand{\SetAlgoRefRelativeSize}[1]{\renewcommand{\algocf@refrelsize}{#1}}%
\newcommand{\SetAlgoRefName}[1]{%
  \renewcommand{\algocf@algocfref}{#1}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
% -------------------------   Default Definitions
%
%%
%%
%
\SetKwComment{tcc}{/* }{ */}%
\SetKwComment{tcp}{// }{}%
%
%\newcommand{\algocf@defaults@common}{
%
%
% english keywords (default)
%
\SetKwHangingKw{KwHData}{Data$\rightarrow$}
\SetKwInput{KwIn}{Input}%
\SetKwInput{KwOut}{Output}%
\SetKwInput{KwData}{Data}%
\SetKwInput{KwResult}{Result}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
%
% French keywords
%
\ifthenelse{\boolean{algocf@localkw@french}\OR\equal{\algocf@languagechoosen}{french}}{%
%\SetKwInOut{AlgDonnees}{Donn\'ees}\SetKwInOut{AlgRes}{R\'esultat}
\SetKwHangingKw{HDonnees}{Donnees$\rightarrow$}
\SetKwInput{Donnees}{Donn\'ees}%
\SetKwInput{Res}{R\'esultat}%
\SetKwInput{Entree}{Entr\'ees}%
\SetKwInput{Sortie}{Sorties}%
\SetKw{KwA}{\`a}%
\SetKw{Retour}{retourner}%
\SetKwBlock{Deb}{d\'ebut}{fin}%
\SetKwRepeat{Repeter}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{Si}{SinonSi}{Sinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Suivant}{Cas}{Autre}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{Pour}{pour}{faire}{fin pour}%
\SetKwFor{PourPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{PourCh}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{PourTous}{pour tous les}{faire}{fin pour tous}%
\SetKwFor{Tq}{tant que}{faire}{fin tq}%
}{}%
%
% --- German keywords
%
\ifthenelse{\boolean{algocf@localkw@german}\OR\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{Ein}{Eingabe}%KwIn
\SetKwInput{Aus}{Ausgabe}%KwOut
\SetKwInput{Daten}{Daten}%KwData
\SetKwInput{Ergebnis}{Ergebnis}%KwResult
\SetKw{Bis}{bis}%KwTo
\SetKw{KwZurueck}{zur\"uck}%KwRet
\SetKw{Zurueck}{zur\"uck}%Return
\SetKwBlock{Beginn}{Beginn}{Ende}%Begin
\SetKwRepeat{Wiederh}{wiederhole}{bis}%Repeat
%
\SetKwIF{Wenn}{SonstWenn}{Sonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Unterscheide}{Fall}{Anderes}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{Fuer}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{FuerPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{FuerJedes}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{FuerAlle}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{Solange}{solange}{tue}{Ende solange}%While
}{}%
%
% --- Czech keywords
%
\ifthenelse{\boolean{algocf@localkw@czech}\OR\equal{\algocf@languagechoosen}{czech}}{%
\SetKwInput{Vst}{Vstup}%
\SetKwInput{Vyst}{V\'{y}stup}%
\SetKwInput{Vysl}{V\'{y}sledek}%
}{}%
%
% --- Portuguese keywords
%
\ifthenelse{\boolean{algocf@localkw@portuguese}\OR\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{Entrada}{Entrada}%
\SetKwInput{Saida}{Sa\'{i}da}%
\SetKwInput{Dados}{Dados}%
\SetKwInput{Resultado}{Resultado}%
\SetKw{Ate}{at\'{e}}
\SetKw{KwRetorna}{retorna}%
\SetKw{Retorna}{retorna}%
\SetKwBlock{Inicio}{in\'{i}cio}{fim}%
\SetKwRepeat{Repita}{repita}{at\'{e}}%
%
\SetKwIF{Se}{SenaoSe}{Senao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Selec}{Caso}{Outro}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{Para}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ParaPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ParaCada}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ParaTodo}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{Enqto}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
%
% --- Italian keywords
%
\ifthenelse{\boolean{algocf@localkw@italiano}\OR\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIng}{Ingresso}%
\SetKwInput{KwUsc}{Uscita}%
\SetKwInput{KwDati}{Dati}%
\SetKwInput{KwRisult}{Risultato}%
\SetKw{KwA}{a}%
\SetKw{KwRitorna}{ritorna}%
\SetKw{Ritorna}{ritorna}%
\SetKwBlock{Inizio}{inizio}{fine}%
\SetKwRepeat{Ripeti}{ripeti}{finch\'e}%
%
\SetKwIF{Sea}{AltSe}{Altrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{Per}{per}{fai}{fine per}%
\SetKwFor{PerPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{PerCiascun}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{PerTutti}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{Finche}{finch\'e}{fai}{fine finch\'e}%
}{}%
%
% --- Spanish keywords
%
\ifthenelse{\boolean{algocf@localkw@spanish}\OR\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{Datos}{Datos}
\SetKwInput{Resultado}{Resultado}
\SetKwInput{Entrada}{Entrada}
\SetKwInput{Salida}{Salida}
\SetKw{KwA}{a}
\SetKw{KwDevolver}{devolver}
\SetKw{Devolver}{devolver}
\SetKwBlock{Inicio}{inicio}{fin}
\SetKwIF{SSi}{EnOtroCasoSi}{EnOtroCaso}{si}{entonces}{sin\'o, si}{sin\'o}{fin si}
\SetKwSwitch{Seleccionar}{Caso}{Otro}{seleccionar}{hacer}{caso}{sin\'o}{fin caso}{fin seleccionar}
\SetKwFor{Para}{para}{hacer}{fin para}
\SetKwFor{ParaPara}{par}{hacer en paralelo}{fin para}
\SetKwFor{EnParalelo}{para}{hacer en paralelo}{fin para}
\SetKwFor{Mientras}{mientras}{hacer}{fin mientras}
\SetKwFor{ParaCada}{para cada}{hacer}{fin para cada}
\SetKwFor{ParaTodo}{para todo}{hacer}{fin para todo}
\SetKwRepeat{Repetir}{repetir}{hasta que}
}{}%
%
% Croatian keywords
%
\ifthenelse{\boolean{algocf@localkw@croatian}\OR\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwUlaz}{Ulaz}%KwIn
\SetKwInput{KwIzlaz}{Izlaz}%KwOut
\SetKwInput{KwPodaci}{Podaci}%KwData
\SetKwInput{KwRezultat}{Rezultat}%KwResult
\SetKw{KwDo}{do}%KwTo
\SetKw{KwVrati}{vrati}%KwRet
\SetKw{Vrati}{vrati}%Return
\SetKwBlock{Pocetak}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Ponavljaj}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{Ako}{InaceAko}{Inace}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Granaj}{Slucaj}{OstaliSlucajevi}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{Za}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ZaPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ZaSvaki}{za svaki}{\v{c}ini}{kraj za svaki}%mForEach
\SetKwFor{ZaSvaku}{za svaku}{\v{c}ini}{kraj za svaku}%fForEach
\SetKwFor{ZaSvako}{za svako}{\v{c}ini}{kraj za svako}%nForEach
\SetKwFor{ZaSve}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{Dok}{dok}{\v{c}ini}{kraj dok}%While
}{}%

%
% --- Turkish keywords
%
\ifthenelse{\boolean{algocf@localkw@turkish}\OR\equal{\algocf@languagechoosen}{turkish}}{%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
% %
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
% --- End 
%}
%
%\algocf@defaults@common
%
% option onelanguage redefinition
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{french}}{%
\SetKwInput{KwIn}{Entr\'ees}%
\SetKwInput{KwOutSortie}{Sorties}%
\SetKwInput{KwData}{Donn\'ees}%
\SetKwInput{KwResult}{R\'esultat}%
\SetKw{KwTo}{\`a}%
\SetKw{KwRet}{retourner}%
\SetKw{Return}{retourner}%
\SetKwBlock{Begin}{d\'ebut}{fin}%
\SetKwRepeat{Repeat}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Switch}{Case}{Other}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{For}{pour}{faire}{fin pour}%
\SetKwFor{ForPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{ForEach}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{ForAll}{pour tous}{faire}{fin pour tous}%
\SetKwFor{While}{tant que}{faire}{fin tq}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{KwIn}{Eingabe}%KwIn
\SetKwInput{KwOut}{Ausgabe}%KwOut
\SetKwInput{KwData}{Daten}%KwData
\SetKwInput{KwResult}{Ergebnis}%KwResult
\SetKw{KwTo}{bis}%KwTo
\SetKw{KwRet}{zur\"uck}%KwRet
\SetKw{Return}{zur\"uck}%Return
\SetKwBlock{Begin}{Beginn}{Ende}%Begin
\SetKwRepeat{Repeat}{wiederhole}{bis}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Switch}{Case}{Other}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{For}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{ForPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{ForEach}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{ForAll}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{While}{solange}{tue}{Ende solange}%While
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Sa\'{i}da}%
\SetKwInput{KwData}{Dados}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{at\'{e}}
\SetKw{KwRet}{retorna}%
\SetKw{Return}{retorna}%
\SetKwBlock{Begin}{in\'{i}cio}{fim}%
\SetKwRepeat{Repeat}{repita}{at\'{e}}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Switch}{Case}{Other}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{For}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ForPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ForEach}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ForAll}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{While}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIn}{Ingresso}%
\SetKwInput{KwOut}{Uscita}%
\SetKwInput{KwData}{Dati}%
\SetKwInput{KwResult}{Risultato}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{ritorna}%
\SetKw{Return}{ritorna}%
\SetKwBlock{Begin}{inizio}{fine}%
\SetKwRepeat{Repeat}{ripeti}{finch\'e}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{For}{per}{fai}{fine per}%
\SetKwFor{ForPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{ForEach}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{ForAll}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{While}{finch\'e}{fai}{fine finch\'e}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Salida}%
\SetKwInput{KwData}{Datos}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{devolver}%
\SetKw{Return}{devolver}%
\SetKwBlock{Begin}{inicio}{fin}%
\SetKwRepeat{Repeat}{repetir}{hasta que}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{entonces}{si no, si}{en otro caso}{fin si}
\SetKwSwitch{Switch}{Case}{Other}{seleccionar}{hacer}{caso}{si no}{fin caso}{fin seleccionar}
\SetKwFor{For}{para}{hacer}{fin para}%
\SetKwFor{ForPar}{para}{hacer in paralelo}{fin para}%
\SetKwFor{ForEach}{para cada}{hacer}{fin para cada}
\SetKwFor{ForAll}{para todo}{hacer}{fin para todo}
\SetKwFor{While}{mientras}{hacer}{fin mientras}
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwIn}{Ulaz}%KwIn
\SetKwInput{KwOut}{Izlaz}%KwOut
\SetKwInput{KwData}{Podaci}%KwData
\SetKwInput{KwResult}{Rezultat}%KwResult
\SetKw{KwTo}{do}%KwTo
\SetKw{KwRet}{vrati}%KwRet
\SetKw{Return}{vrati}%Return
\SetKwBlock{Begin}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Repeat}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Switch}{Case}{Other}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{For}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ForPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ForEach}{za svaki}{\v{c}ini}{kraj za svaki}%ForEach
\SetKwFor{ForAll}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{While}{dok}{\v{c}ini}{kraj dok}%While
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{turkish}}{%
%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
%
%%%% old commands compatibility
%
\ifthenelse{\boolean{algocf@oldcommands}}{%
\newcommand{\SetNoLine}{\SetAlgoNoLine}%
\newcommand{\SetNoline}{\SetAlgoNoLine}%
\newcommand{\SetVline}{\SetAlgoVlined}%
\newcommand{\SetLine}{\SetAlgoLined}%
%
\newcommand{\dontprintsemicolon}{\DontPrintSemicolon}%
\newcommand{\printsemicolon}{\PrintSemicolon}%
\newcommand{\incmargin}[1]{\IncMargin{#1}}%
\newcommand{\decmargin}[1]{\DecMargin{-#1}}%
\newcommand{\setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\Setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\setalcapskip}[1]{\SetAlCapSkip{#1}}%
\newcommand{\setalcaphskip}[1]{\SetAlCapHSkip{#1}}%
\newcommand{\nlSty}[1]{\NlSty{#1}}%
\newcommand{\Setnlsty}[3]{\SetNlSty{#1}{#2}{#3}}%
\newcommand{\linesnumbered}{\LinesNumbered}%
\newcommand{\linesnotnumbered}{\LinesNotNumbered}%
\newcommand{\linesnumberedhidden}{\LinesNumberedHidden}%
\newcommand{\showln}{\ShowLn}%
\newcommand{\showlnlabel}[1]{\ShowLnLabel{#1}}%
\newcommand{\nocaptionofalgo}{\NoCaptionOfAlgo}%
\newcommand{\restorecaptionofalgo}{\RestoreCaptionOfAlgo}%
\newcommand{\restylealgo}[1]{\RestyleAlgo{#1}}%
%
\newcommand{\Titleofalgo}[1]{\TitleOfAlgo{#1}}%
% \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
\newcommand{\SetKwIf}[6]{\SetKwIF{#1}{#2#1}{#2}{#3}{#4}{#5 #1}{#5}{#6}}
%
\SetKwIF{gSi}{gSinonSi}{gSinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwIF{gIf}{gElsIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gIf}{gElseIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gWenn}{gSonstWenn}{gSonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwIF{gSe}{gSenaoSe}{gSenao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwIF{gSea}{gAltSe}{gAltrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKw{Ret}{return}%
\SetKwInput{Data}{Data}%
\SetKwInput{Result}{Result}%
}{%
  \relax%
}%
%
%
%
%%
%%%
%%%% END

==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/Intro.tex <==
%\red{(needs to be polished quite a bit..)}


Temporal logic motion planning has emerged as one of the main approaches for specifying a richer class of robot tasks than the classical point-to-point navigation and can capture temporal and Boolean requirements, such as sequencing, surveillance or coverage
\cite{fainekos2005hybrid,kress2007s,smith2011optimal,tumova2016multi,chen2012formal,ulusoy2013optimality,ulusoy2014optimal,shoukry2017linear,shoukry2018smc,vasile2013sampling,kantaros2017Csampling,kantaros2018text}. Common in these works is that they typically assume robots with \textit{known} dynamics operating in \textit{known} environments that are modeled using discrete abstractions, e.g., transition systems. 
%Nevertheless, constructing expressive discrete abstractions makes the synthesis problem computationally expensive. 
As a result, these methods cannot be applied to scenarios where the environment is initially unknown and, therefore, online re-planning may be required as environmental maps are constructed;  resulting in limited applicability. To mitigate this issue, learning-based approaches have also been proposed that consider robots with \textit{unknown} dynamics operating in \textit{unknown} environments. These approaches learn policies that directly map on-board sensor readings to control commands in a trial-and-error fashion; see e.g., \cite{dorsa2014learning,li2017reinforcement,jones,gao2019reduced,hasanbeig2019reinforcement}. However, learning approaches, in addition to being data inefficient, are specialized to the  environment they were trained on and do not generalize well to previously unseen environments. %On the other hand, learning-free approaches typically rely on repeatedly re-planning trajectories towards intermediate goals within the robot’s known environment, with the expectation that the robot will eventually fulfill its assigned mission \cite{bekris2007greedy,guo2013revising,guo2015multi}. However, such planning strategies are not necessarily complete, i.e., a solution may not be found even if it exists, and their computational cost increases as the size of the environment or the number of robots increases which restricts their applicability.

%is shortsighted in that it does not reason about the map beyond the observed environment, resulting in greedy and inefficient trajectories


%%%%%

This paper addresses a motion planning problem for multiple robots with \textit{known} dynamics that need to accomplish collaborative complex tasks in \textit{unknown} environments. We consider robots that are tasked with accomplishing collaborative tasks captured by global Linear Temporal Logic (LTL) formulas in complex environments with unknown obstacles. To address this problem, we propose the first reactive, abstraction-free, and distributed temporal logic planning algorithm for complex mission planning in unknown environments. The robots are equipped with sensors that allow them to continuously learn an individual or shared occupancy grid map of the environment, using existing Simultaneous Localization and Mapping (SLAM) methods \cite{elfes1989using,thrun2001learning,thrun2005probabilistic,grisetti2007improved}, while reacting and adapting mission planning to the updated map.
%
Furthermore, the proposed algorithm is abstraction-free i.e., it does not rely on any discrete abstraction of the robot dynamics (e.g., transition systems) and distributed in the sense that the temporal logic task is decomposed into local point-to-point navigation tasks. These local tasks are formulated online based on the continuously learned map and can be solved using existing approaches 
\cite{karaman2011sampling,guzzi2013human,liu2016high,otte2016rrtx,bansal2019combining,vasilopoulos2018sensor,ryll2019efficient,tordesillas2020faster}.
%\cite{karaman2011sampling,guzzi2013human,pivtoraiko2013incremental,liu2016high,otte2016rrtx,bansal2019combining,ryll2019efficient,elhafsi2019map,zhai2019path,tordesillas2020faster}. 
The decomposition of the global LTL task into local reachability tasks allows for efficient re-planning as the robots can make decisions locally to accomplish the assigned LTL task while communicating intermittently with each other when new reachability tasks need to be designed. 
%, a task that is particularly challenging in unknown environments.
%To achieve that, we first translate the LTL specification into an automaton which is then pruned by removing transitions that can never be enabled (e.g., transitions that are enabled if a robot is simultaneously present in more than one location). Then, as the robots navigate the workspace they collaboratively select the automaton state they should reach next so that they move closer to the accepting/final automaton states (i.e., so that they make progress towards accomplishing the assigned task). By appropriately decomposing the Boolean formula that enables this automaton transition, every robot selects locations that they need to visit next to reach the desired automaton state. Then, every robot solves a \textit{local} shortest-path optimal control problem to design paths that reach the desired location in space and, consequently, the desired automaton state. These paths are locally revised online as  the map of the environment is updated as per sensor measurements. 
%Unlike the majority of relevant works, we show that by appropriately introducing delays in the execution of the synthesized motion plans, the robots can move asynchronously in the workspace. 
Theoretically, we show there exists a fragment of LTL formulas for which decomposition into local reachability tasks is always possible. Furthermore, we show that the paths designed to address these reachability sub-tasks can be executed asynchronously(?) across the robots. Finally, we prove that under mild assumptions on the coarse structure of the environment and the sensor model, the proposed planning algorithm is complete. 

%\subsection{Temporal Logic Planning in Known Environments}
%Control synthesis for mobile robots under complex tasks, captured by LTL formulas, build upon either bottom-up approaches when independent LTL expressions are assigned to robots \cite{kress2009temporal,kress2007s,bhatia2010sampling,smith2011optimal,fu2016optimal,tumova2016multi} or top-down approaches when a global LTL formula describing a collaborative task is assigned to a team of robots \cite{chen2011synthesis,chen2012formal,kloetzer2010automatic,ulusoy2012robust,ulusoy2013optimality,ulusoy2014optimal}, as in this work. %Common in the above works is that they rely on model checking tools \cite{baier2008principles,clarke1999model} to design correct-by-construction paths that satisfy the LTL tasks. 
%Common in these works is that optimal paths are synthesized for every robot using the individual transition systems that capture robot mobility and an automaton that represents the global LTL specification. Specifically, by taking the synchronous product among the transition systems and the NBA, a synchronous product automaton can be constructed \cite{baier2008principles,clarke1999model}. Then, representing the latter automaton as a graph and using graph-search techniques, optimal motion plans can be derived that satisfy the global LTL specification and optimize a cost function. As the number of robots or the size of the automaton increases, the state-space of the product automaton grows exponentially and, as a result, graph-search techniques become intractable. Consequently, these motion planning algorithms scale poorly with the number of robots and the complexity of the assigned task. Temporal logic planning algorithms for large-scale multi-robot systems have recently been proposed that rely on decomposing the automaton into local smaller automata \cite{schillinger2016decomposition}, SMT methods \cite{shoukry2017linear,shoukry2018smc}, or sampling-based techniques \cite{vasile2013sampling,kantaros2017Csampling,kantaros2018text,kantaros2018temporal}. Common in all the above works is that they assume that the environment is \textit{a priori} known, and, therefore, motion plans can be synthesized offline. 


%{\bf{Temporal Logic Tasks in Unknown Environments:}} 
%{\bf{Related Research:}}
\subsection{Related Research}
%Temporal logic planning has been studied extensively in \cite{fainekos2005hybrid,kress2007s,smith2011optimal,tumova2016multi,chen2012formal,ulusoy2013optimality,ulusoy2014optimal,shoukry2017linear,shoukry2018smc,vasile2013sampling,kantaros2017Csampling,kantaros2018text}. Common in these works is that they consider known environments while the majority of them rely on the application of graph search methods on a product automaton to compute correct-by-construction paths. Due to the centralized nature of these algorithms, their computational cost increases as the number of robots, the complexity of the task, or the size of the environment increases. 
%of these temporal logic planning approaches As a result, their application in unknown environments raises computational challenges, since they need to be re-executed online to design new robot paths as the environmental map is learned.\footnote{\red{[this paragraph is possibly not needed]}}%In fact, their computational cost increases as the number of robots, the complexity of the task, or the size of the environment increases. 

Reactive temporal logic planning algorithms that can account for map uncertainty in terms of incomplete environment models have been developed  in \cite{guo2013revising,guo2015multi,maly2013iterative,lahijanian2016iterative,livingston2012backtracking,livingston2013patching,kress2009temporal,alonso2018reactive}. Particularly, \cite{guo2013revising,guo2015multi} model the environment as transition systems which are partially known. Then discrete controllers are designed by applying graph search methods on a product automaton. As the environment, i.e., the transition system, is updated, the product automaton is locally updated as well, and new paths are re-designed by applying graph search approaches on the revised automaton. %However, construction of a product automaton and application of graph search techniques is computationally expensive.
A conceptually similar approach is proposed in \cite{maly2013iterative,lahijanian2016iterative} as well. The works in \cite{livingston2012backtracking,livingston2013patching} propose methods to locally patch paths as transition systems, modeling the environment, change so that GR(1) (General Reactivity of Rank 1) specifications are satisfied. Reactive to LTL specifications planning algorithms are proposed in \cite{kress2009temporal,alonso2018reactive}, as well. Specifically, in \cite{kress2009temporal,alonso2018reactive} the robot reacts to the environment while the task specification captures this reactivity. Correctness of these algorithms is guaranteed if the robot operates in an environment that satisfies the assumptions that were explicitly modeled in the task specification. 
%
Common in all these works is that, unlike our approach, they rely on discrete abstractions of the robot dynamics  \cite{belta2005discrete,pola2008approximately}. Thus, correctness of the generated motion plans is guaranteed with respect to the discrete abstractions resulting in a gap between  the generated discrete motion plans and their physical low-level implementation \cite{desaisoter}.
%
Moreover, the reactive algorithms proposed in \cite{guo2013revising,guo2015multi,maly2013iterative,lahijanian2016iterative,livingston2012backtracking,livingston2013patching,kress2009temporal,alonso2018reactive} are centralized as they rely on constructing a product automaton among all robots to synthesize motion plans. As a result, their their computational cost for online re-planning increases as the number of robots, the complexity of the task, or the size of the environment increase.
%also supported by our comparative simulation studies.
To the contrary, our algorithm is highly scalable due to its distributed nature and the fact that it avoids altogether the construction of a product automaton. %Specifically, we show that there exists a fragment of LTL that can decomposed into a sequence of \textit{local} reachability tasks that can be efficiently solved online as the map of the environment is learned using existing methods  \cite{karaman2011sampling,guzzi2013human,otte2016rrtx,bansal2019combining,ryll2019efficient,elhafsi2019map,zhai2019path,tordesillas2020faster}. 
%
%
Finally, note that decomposition of fragments of LTL formulas into reachability tasks has been investigated in \cite{fainekos2006translating,bisoffi2018hybrid,jagtap2019formal}, as well, assuming robots that operate in known environments. %For instance, \cite{fainekos2006translating} considers flat LTL formulas while \cite{bisoffi2018hybrid,jagtap2019formal}  considers safe-LTL formulas satisfied by finite traces. 
Common in these works is that temporal logic tasks are decomposed into \textit{global/multi-agent} reachability tasks. As a result, these methods face scaling challenges as the number of robots increases and require synchronous motion among all agents. Our proposed method mitigates these issues by decomposing temporal logic tasks  into \textit{local} reachability tasks. %We emphasize that this is the first temporal logic planning algorithm over continuously learned occupancy grid maps.

%cite{fainekos2006translating} as well. However, in these works temporal logic tasks are decomposed into \textit{global/multi-agent} reachability tasks while the computational cost of solving global reachability tasks increases as the number of robots increases. %As a result, it is computationally
%
%To the contrary, our approach does not rely on abstractions of the robot dynamics and, therefore, avoids altogether the construction of a product automaton and scales well with the number of robots. 

\subsection{Contribution}
%{\bf{Contributions:}}
The contribution of this paper can be summarized as follows.
\textit{First}, we propose the \textit{first} temporal logic planning algorithm over continuously learned occupancy grid maps. The proposed algorithm is reactive, distributed, and abstraction-free. \textit{Second}, we show that the proposed algorithm is complete under assumptions on the coarse structure of the environment and the sensor model. \textit{Third}, we provide extensive comparative simulation studies and hardware experiments that corroborate the efficacy and scalability of the proposed algorithm.



%The rest of the paper is organized as follows. The problem formulation is presented Section \ref{sec:PF} while the proposed distributed algorithm for LTL planning is presented in Section \ref{sec:planning}. Correctness of the proposed algorithm is dicussed in Section \ref{sec:complOpt}. In Section \ref{sec:Sim}, we provide numerical experiments. Conclusive remarks are provided in the last section.

==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/PF.tex <==

% ------------------------------------------------------------------------------- %
%\subsection{Robot \& Sensor Model}
Consider $N$ mobile robots that reside in an environment $\Omega\subset \reals^d$ with non-overlapping and known regions of interest, denoted  by $\ell_i\subset \Omega$, and \textit{static} but \textit{unknown} obstacles $O\subset\Omega$, where $d$ is the dimension of the workspace. The robots are governed by the following dynamics: $\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$,
% 
%\begin{equation}\label{eq:rdynamics}
%\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t)),
%\end{equation}
for all $j\in\ccalN:=\{1,\dots,N\}$, where $\bbp_{j}(t) \in\mathbb{R}^n$ stands for the state (e.g., position and orientation) of robot $j$ at time $t\geq 0$, $\bbu_{j}(t)$. %stands for a control input in a \textit{finite} space of admissible controls $\ccalU_j$. %\NA{state that time is discrete}
%Note that the state $\bbp_{j}$ may belong to a higher dimensional space than $\Omega_{\text{free}}$. For example, this is the case if $\bbp_j(t)$ includes the position and the orientation of robot $j$. Nevertheless, throughout the rest of the paper, for simplicity of notations we denote $\bbp_{j}(t) \in \Omega_{\text{free}}$.\BS{Can we make this into a  remark or just remove it? It's extra clutter for something that is fairly straightforward.} 
%Also, note that the considered dynamics can range from simple graph-based dynamics to arbitrary nonlinear discrete dynamics\NA{This sentence could be removed}. 
Hereafter, we compactly denote the dynamics of all robots as 
\begin{equation}\label{eq:rdynamics}
\bbp(t+1)=\bbf(\bbp(t),\bbu(t)),
\end{equation}
where $\bbp(t)\in \mathbb{R}^{n\times N}$, $\forall t\geq 0$. %, and $\bbu(t)\in\ccalU:=\ccalU_1\times\dots\times\ccalU_N$.

Moreover, we assume that the robots are equipped with sensors (e.g., LiDAR or camera) to detect if a given location $\bbq\in\Omega$ belongs to the obstacle-free space. Specifically, we consider the following deterministic sensor model:
\begin{equation}\label{eq:sensor}
   s(\bbp_j(t),\bbq)=
            \begin{cases}
               1~\text{if~}(\bbq\in O) \wedge (\lVert \bbp_j(t)-\bbq \rVert\leq R),\\
              0~\text{otherwise}.
            \end{cases} 
\end{equation}

\noindent In words, given a location $\bbq\in\Omega$ that lies within the sensing range $R$ of robot $j$, we have that $s(\bbp_j(t),\bbq)=1$ if $\bbq$ belongs to the obstacle-space, i.e., $\bbq\in O$; otherwise, $s(\bbp_j(t),\bbq)=0$. 

Using sensor measurements as per \eqref{eq:sensor}, the robots collectively build a shared (binary) occupancy grid map defined as follows. First, the workspace $\Omega$ is partitioned into $K$ grid cells denoted by $c_i\subset\Omega$. Then, given $C=\{c_1,c_2,\dots,c_K\}$, we define
a function a function $g: C\times \bbs_{0:t} \rightarrow \set{0,1}^K$ that maps each grid cell $c_i$ to $0$ or $1$, given all robot measurements up to time $t$, denoted by $\bbs_{0:t}$. 
%
The function $g$ is defined as follows:
\begin{equation}\label{eq:updMap}
   g(c_i,\bbs_{0:t})=
            \begin{cases}
               1~\text{if~}\exists j, \bbq\in c_i,~t'\leq t~\text{s.t}~s(\bbp_j(t'),\bbq)=1,\\
              0~\text{otherwise}.
            \end{cases} 
\end{equation}
In words, if there exists at least one robot $j$ that took a measurement at any past time instant $t'\leq t$ indicating that there exists an obstacle within the grid cell $c_i$ (i.e., $s(\bbp_j(t'),\bbq)=1$), then $g(c_i,\bbs_{0:t})=1$, i.e., $c_i$ is considered an obstacle. Otherwise, $g(c_i,\bbs_{0:t})=0$, which means that $c_i$ is either obstacle-free or no measurement associated with $c_i$ has been taken up to the current time instant $t$. As a result, $g$ produces a binary occupancy grid map $M(t)=\{m_1(t),m_2(t),\dots,m_K(t)\}$, where (i) $m_i(t)=1$ if $g(c_i,\bbs_{0:t})=1$ (ii) and $m_i(t)=0$ if $g(c_i,\bbs_{0:t})=0$. 
%
%
%
%For simplicity of notation, we assume that all robots can exchange their sensor measurements at any time $t$ through a connected communication network and, therefore, they have access to same global map $M(t)$.\footnote{The proposed algorithm can straightforwardly be extended to the case where each robot $j$ builds its own map $M_j$ and adapts its planning to $M_j$.} %if $\bbq$ belongs to the obstacle-free space, for all locations $\bbq$ that lie with the sensing range $R$ of robot $i$.
%\red{here we need to define the occupancy grid map that we build... otherwise it is unlcear what exactly $q$ is.}
Note that the occupancy grid map is constructed as per \eqref{eq:updMap} assuming deterministic and noiseless sensor models as in \eqref{eq:sensor}. In practice, to account for noisy sensors, the function $g$ in \eqref{eq:updMap} can be determined by inference methods (e.g., particle filters) giving rise to probabilistic maps which are then thresholded yielding binary maps $M(t)$ as e.g., in \cite{elfes1989using,thrun2001learning,thrun2005probabilistic,grisetti2007improved}. Moreover, for simplicity of notation, we assume that all robots build a shared map $M(t)$. This can be relaxed by allowing each robot to build its own local map $M_j(t)$, based on its individual sensor measurements.
%in \eqref{eq:updMap} we assume that all robots can exchange their sensor measurements at any time through a connected communication network and, therefore, they have access to same global map $M(t)$. Nevertheless, this can be relaxed by allowing each robot to build its own local map $M_j$, based on its individual sensor measurements. %Also, in Section \ref{sec:Sim}, we show that the proposed algorithm can be applied even without building maps, by leveraging recently proposed algorithms that consider point-to-point navigation problems in the presence of unknown obstacles \cite{guzzi2013human,vasilopoulos2018sensor,bansal2019combining}.
%, and adapt its planning to $M_j$ instead of $M$ 
%\footnote{The proposed algorithm can straightforwardly be extended to the case where each robot $j$ builds its own map $M_j$ and adapts its planning to $M_j$.} 
%Second, we consider deterministic and noiseless sensor models in \eqref{eq:sensor}. In practice, to account for noisy sensors, the function $g$ can be determined by inference methods (e.g., particle filters) giving rise to probabilistic maps which are then thresholded yielding binary maps $M(t)$ as e.g., in \cite{elfes1989using,thrun2001learning,thrun2005probabilistic,grisetti2007improved}. 

%\subsection{Task Specification using Linear Temporal Logic}
The goal of the robots is to accomplish a complex collaborative task captured by a global Linear Temporal Logic (LTL) specification $\phi$. The assigned task $\phi$ is defined over a set of atomic propositions $\mathcal{AP}=\cup_{\forall j}\mathcal{AP}_j$ where $\mathcal{AP}_j=\cup_i\set{\pi_{j}^{\ell_i},\pi_j^{O}}$, and $\pi_{j}^{\ell_i}$ and $\pi_{j}^{O}$ are atomic predicates that are true when robot $j$ is within region $\ell_i$ and hits an obstacle, respectively.
%
In what follows, we briefly present the syntax and semantics of LTL. A detailed overview of this theory can be found in \cite{baier2008principles}. The basic ingredients of LTL are a set of atomic propositions $\mathcal{AP}$, the boolean operators, i.e., conjunction $\wedge$, and negation $\neg$, and two temporal operators, next $\bigcirc$ and until $\mathcal{U}$. LTL formulas over a set $\mathcal{AP}$ can be constructed based on the following grammar: $\phi::=\text{true}~|~\pi~|~\phi_1\wedge\phi_2~|~\neg\phi~|~\bigcirc\phi~|~\phi_1~\mathcal{U}~\phi_2$, where $\pi\in\mathcal{AP}$. For brevity we abstain from presenting the derivations of other Boolean and temporal operators, e.g., \textit{always} $\square$, \textit{eventually} $\lozenge$, \textit{implication} $\Rightarrow$, which can be found in \cite{baier2008principles}. 
%
%An infinite \textit{word} $\sigma$ over the alphabet $2^{\mathcal{AP}}$ is defined as an infinite sequence  $\sigma=\pi_0\pi_1\pi_2\dots\in (2^{\mathcal{AP}})^{\omega}$, where $\omega$ denotes an infinite repetition and $\pi_k\in2^{\mathcal{AP}}$, $\forall k\in\mathbb{N}$. The language $\texttt{Words}(\phi)=\left\{\sigma\in (2^{\mathcal{AP}})^{\omega}|\sigma\models\phi\right\}$ is defined as the set of words that satisfy the LTL formula $\phi$, where $\models\subseteq (2^{\mathcal{AP}})^{\omega}\times\phi$ is the satisfaction relation.
%
%Any LTL formula $\phi$ can be translated into a Nondeterministic B$\ddot{\text{u}}$chi Automaton (NBA) over $(2^{\mathcal{AP}})^{\omega}$ denoted by $B$ \cite{vardi1986automata}, which is defined as follows:
%\begin{definition}
%A \textit{Nondeterministic B$\ddot{\text{u}}$chi Automaton} (NBA) $B$ over $2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\Sigma,\rightarrow_B,\mathcal{Q}_B^F\right)$, where $\ccalQ_{B}$ is the set of states, $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is a set of initial states, $\Sigma=2^{\mathcal{AP}}$ is an alphabet, $\rightarrow_{B}\subseteq\ccalQ_{B}\times \Sigma\times\ccalQ_{B}$ is the transition relation, and $\ccalQ_B^F\subseteq\ccalQ_{B}$ is a set of accepting/final states. 
%\end{definition}
%
%An \textit{infinite run} $\rho_B$ of $B$ over an infinite word $\sigma=\pi_0\pi_1\pi_2\dots$, where $\pi_k\in\Sigma$, for all $ k\in\mathbb{N}$, is a sequence $\rho_B=q_B^0q_B^1q_B^2\dots$ such that $q_B^0\in\ccalQ_B^0$ and $(q_B^{k},\pi_k,q_B^{k+1})\in\rightarrow_{B}$, $\forall k\in\mathbb{N}$. An infinite run $\rho_B$ is called \textit{accepting} if $\texttt{Inf}(\rho_B)\cap\ccalQ_B^F\neq\varnothing$, where $\texttt{Inf}(\rho_B)$ represents the set of states that appear in $\rho_B$ infinitely often. The words $\sigma$ that result in an accepting run of $B$ constitute the accepted language of $B$, denoted by $\ccalL_B$. It is proven \cite{baier2008principles} that the accepted language of $B$ is equivalent to the words of $\phi$, i.e., $\ccalL_B=\texttt{Words}(\phi)$. 
%
%Hereafter, we assume that in $\Omega$ there are non-overlapping regions of interest, denoted by $\ell_i\subseteq \Omega$ with known locations.\footnote{\red{explain why it is trivial to consider overlapping regions..}} However, the locations of obstacles are \textit{a priori} unknown. 
An example of an LTL specification is: $\phi=\Diamond(\pi_1^{\ell_1}\wedge (\pi_1^{\ell_2}\wedge (\Diamond \pi_1^{\ell_3}))) \wedge\Box (\neg(\pi_1^{O}\vee \pi_{1}^{\ell_{4}})) $, which requires the robot to (i) eventually visit locations $\ell_1$, $\ell_2$, and $\ell_{3}$ in this order; and (ii) avoid all a priori unknown obstacles and region $\ell_{4}$ since hostile units may exist there. %until robot $2$ visit location $\ell_3$, captured by $\neg\pi_1^{\ell_1}\ccalU \pi_1^{\ell_3}$; and (iii) both robots to avoid hitting any obstacle captured by $\Box (\wedge_{j}(\vee_{\ell_{\text{obs}}}\pi_j^{\ell_{\text{obs}}}))$. %Note that the robots know the coordinates of the target locations $\ell_1$ and $\ell_3$ but they are not aware of the locations of obstacles denoted by $\ell_{\text{obs}}$. Specifically, throughout the paper, we assume that the coordinates of all target locations $\ell_i$ are known but the coordinates of obstacles are completely unknown.
%
Hereafter, we exclude the `next' operator $\bigcirc$ from the syntax, since it is not meaningful for practical robotics applications; this is common in relevant works, see, e.g., \cite{kloetzer2008fully} and the references therein. LTL formulas are satisfied by discrete plans $\tau$ that are
infinite sequences of locations of $N$ robots in $\Omega$. i.e., $\tau=\bbp(0),\bbp(1),\dots,\bbp(t),\dots$ \cite{baier2008principles}. %Given an LTL formula $\phi$, if there exists a plan $\tau$ satisfying $\phi$, then it can be written in a finite representation, called prefix-suffix structure, i.e., $\tau=\tau_{\text{pre}}[\tau_{\text{suf}}]^{\omega}$, where the  prefix part $\tau_{\text{pre}}=\bbp(0),\bbp(1),\dots,\bbp(K)$ is executed only once followed by the indefinite execution of the suffix part $\tau_{\text{suf}}=\bbp(K+1),\bbp(\bbp(K+2)),\dots,\bbp(K+S)$, where $\bbp(K+S)=\bbp(K)$ and $\omega$ denotes the indefinite execution of $\tau_{\text{suf}}$. 
%
%In order to interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times M(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current robot system state $\bbp(t)\in\mathbb{R}^{n\times N}$ and the current map $M(t)$ of the environment.
%%%%%%%%%%%%%%
%
%\subsection{Mission Planning Problem in Unknown Environments}
%Given a task specification $\phi$, our goal is to select a stopping time $H$ and a sequence $\bbu_{0:H}$ of control inputs $\bbu(t)$, for all $t\in\set{0,\dots,H}$, that satisfies $\phi$ while minimizing a motion cost. This gives rise to the following optimal control problem:
%
%\footnotesize
%\begin{subequations}
%\label{eq:Prob2}
%\begin{align}
%& \min_{\substack{H, \bbu_{0:H}}} \left[J(H,\bbu_{0:H}) = %\int_{t=0}^{H}  w(\bbp(t),\bbu(t))dt \right] \label{obj2}\\
%& \ \ \ \ \ \ \ \ \ \ \  \bbp_{0:H}\models\phi  \label{constr1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \dot{\bbp}(t) = \bbf(\bbp(t),\bbu(t)). %\label{constr2}
%\end{align}
%\end{subequations}
%
%\normalsize
%where $w(\bbp(t),\bbu(t))\geq 0$ is a motion cost function that captures e.g., the energy consumption or control effort, and $\bbp_{0:H}$ is the path of the multi-robot system until the time instant $H$. 
The problem addressed in this paper can be summarized as follows:
\begin{problem} \label{prob}
Given an initial robot configuration $\bbp(0)$ in an environment with unknown obstacles, the robot dynamics \eqref{eq:rdynamics}, sensor models \eqref{eq:sensor}, and a task specification captured by an LTL formula $\phi$ (which also requires obstacle avoidance), compute a plan $\tau$ that satisfies $\phi$ and respects the robot dynamics.% as per \eqref{eq:Prob2}.
\end{problem}

Problem \ref{prob} can be solved by applying existing abstraction-free approaches for LTL planning, e.g., \cite{vasile2013sampling,luo2019abstraction}, at runtime to continuously update the robot paths as the map of the environment is continuously learned. These methods require searching over a large product automaton space, a task that is computationally challenging to perform at runtime. To mitigate this challenge, we propose a new reactive LTL planning algorithm that does not rely on searching over a product automaton space. In particular, in Section \ref{sec:aut}, we decompose the temporal logic task into a sequence of local point-to-point navigation problems which allows for efficient and fast re-planning. These navigation problems are formulated and solved online while adapting to the updated map of the environment; see Sec. \ref{sec:planning}.

%\begin{rem}
%Note that in this section, we made two main assumptions. First, we assume that all robots can exchange their sensor measurements at any time through a connected communication network and, therefore, they have access to same global map $M(t)$. This can be relaxed by allowing each robot to build its own local map $M_j$, based on its individual sensor measurements. %Also, in Section \ref{sec:Sim}, we show that the proposed algorithm can be applied even without building maps, by leveraging recently proposed algorithms that consider point-to-point navigation problems in the presence of unknown obstacles \cite{guzzi2013human,vasilopoulos2018sensor,bansal2019combining}.
%, and adapt its planning to $M_j$ instead of $M$ 
%\footnote{The proposed algorithm can straightforwardly be extended to the case where each robot $j$ builds its own map $M_j$ and adapts its planning to $M_j$.} 
%Second, we consider deterministic and noiseless sensor models in \eqref{eq:sensor}. In practice, to account for noisy sensors, the function $g$ can be determined by inference methods (e.g., particle filters) giving rise to probabilistic maps which are then thresholded yielding binary maps $M(t)$ as e.g., in \cite{elfes1989using,thrun2001learning,thrun2005probabilistic,grisetti2007improved}. 
%\end{rem}

==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/alg_April8_2020.tex <==
%
In this section, we provide an algorithm to decompose global LTL task into local reachability tasks. This process occurs offline i.e., before deploying the robots in the unknown environment. Specifically, in Section \ref{sec:nba} we translate the LTL formula into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA). In Section \ref{sec:prune} we prune this automaton by removing infeasible transitions i.e., transitions that can be activated only if a robot is present in more than one location simultaneously. Then, in Section \ref{sec:dec} we provide conditions under which feasible NBA transitions can be enabled by solving local reachability tasks. Such transitions are called decomposable. In Section \ref{sec:dist}, using the definition of feasible and decomposable transitions, we define a distance metric over the NBA that measures how far the robots are from fulfilling the assigned mission. This metric will be used in Section \ref{sec:planning} to guide and adapt planning to the continuously learned map of the environment.


\subsection{From LTL formulas to Automata}\label{sec:nba}

First, we translate the specification $\phi$, constructed using a set of atomic predicates $\mathcal{AP}$, into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA), defined as follows \cite{baier2008principles}. %Given a temporal logic formula $\phi$ , with syntax and semantics as described in Definitions \ref{syntax} and \ref{semantics}, respectively, a DFA is defined as follows:

\begin{definition}[NBA]
A Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\delta_B, \ccalQ_F\right)$, where (i) $\ccalQ_{B}$ is the set of states;
(ii) $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is the initial state; (iii) $\delta_B:\ccalQ_B\times\Sigma\rightarrow\ccalQ_B$ is a non-deterministic transition relation, and $\ccalQ_F\subseteq\ccalQ_{B}$ is a set of accepting/final state. 
\end{definition}

To interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times M(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current multi-robot state $\bbp(t)\in\mathbb{R}^{n\times N}$ and the current map $M(t)$ of the environment. An infinite-length discrete plan $\tau=\bbp(0)\bbp(1)\dots$ satisfies $\phi$, denoted by $\tau\models\phi$, if the word $\sigma=L(\bbp(0), M(0))L(\bbp(1),M(1))\dots$ yields an accepting NBA run defined as follows. First, a run of $\rho_B$ of $B$ over an infinite word $\sigma=\sigma(1)\sigma(2)\dots\sigma(t)\dots\in(2^{\mathcal{AP}})^{\omega}$, is a sequence $\rho_B=q_B(0)q_B(1)q_B(2)\dots,q_B(t),\dots$, where $q_B(0)\in\ccalQ_B^0$ and $\delta_B(q_B(t),\sigma(t),q_B(t+1)$, $\forall t\in\mathbb{N}$. %Hereafter, we equivalently denote $\delta_B(q_B(t),\sigma(t),q_B(t+1)$ as $q_B(t)\rightarrow_B q_B(t+1)$.
A run $\rho_B$ is called \textit{accepting} if at least one final state appears infinitely often in it. In words, an infinite-length discrete plan $\tau$ satisfies an LTL formula $\phi$ if it can generate at least one accepting NBA run. Hereafter, for simplicity we replace $L(\bbp(t),M(t))$ with $L(\bbp(t))$.
%The symbols $\sigma$ that result in an accepting run of $D$ constitute the accepted language of $D$.

%The proposed reactive algorithm builds online (i.e., as the robots navigate the environment) paths that live in the infinite-dimensional space $\Omega^N\times\ccalQ_D$. The synthesized paths are updated as the map of the environment is updated. 

%Specifically, let $q_B(t)\in\ccalQ_B$ denote the NBA state that the multi-robot system has reached at time $t$ given all observations that have been made (i.e., all atomic predicates that have been satisfied) until $t$, where $q_B(0)\in\ccalQ_B^0$ [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. 

%In Section \ref{sec:planning}, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task. Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task. To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that (i) it is  one-hop reachable from $q_B(t)$, (ii) the transition from $q_B(t)$ to $q_B^{\text{next}}$ is feasible, i.e., observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously, and (iii) $q_B^{\text{next}}$ is `closer' to the final states than $q_B(t)$ is. %Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. 
%In what follows, we describe these steps in detail.
%In Section \ref{sec:prune} we define when an NBA transition is feasible and when it is decomposable i.e., it can be enabled via solving local reachability-avoidance problems. In Section \ref{sec:dist}, we define a distance metric over the NBA that measures how far each NBA state is from the set of final states.

%Next, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task; see Algorithm \ref{alg:RRT}. Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task. To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that it is (i) one-hop reachable from $q_B(t)$, (ii) `closer' to the final states than $q_B(t)$ is according to a distance function defined over the NBA, and (iii) observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously. Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. In what follows, we describe these steps in detail.


%Once this transition is enabled, the robots update the target DFA state $q_D^{\text{next}}$ until they reach a final DFA state.%\footnote{In case the DFA has more than one initial state, then there is more than one state $\bbq(0)$ that can be used as a root. In this case, a separate tree is build for each one of possible roots.}
%For this, we assume that the initial robot configuration allows the robots to stay in $q_B(0)$.
%

%By convention the cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = 0$, while the cost of a node $\bbq(t+1)=[\bbp(t+1), q_D]\in\ccalV$, given its parent node $\bbq(t)=[\bbp(t),q_D']\in\ccalV$, is computed as 
%\begin{equation}\label{eq:costUpd}
%J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq(t)) +  w(\bbp(t),\bbp(t+1)).
%\end{equation}
%Observe that by applying \eqref{eq:costUpd} recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:Prob2}.

 
%Given the current DFA state $q_D(t)$, the robots first select a DFA state $q_D^{\text{next}}\in\ccalQ_D$ that is `closer' to the final state $q_F$ than $q_D(t)$ is and observations that generate a transition from $q_D(t)$ to $q_D^{\text{next}}$ can be generated. Therefore,
%\subsection{Selecting the Next DFA State}\label{sec:targetDFA}

%{\bf{Pruning the DFA:}}
\subsection{Pruning Infeasible NBA Transitions}\label{sec:prune}
%Given the current NBA state $q_B(t)$, a new state $q_B^{\text{next}}$ is selected so that it is closer to the final states. Thus, to select $q_B^{\text{next}}$, we need to define a distance function over the state-space of the NBA that measures how far each state is from the final state. %(in terms of the number feasible transitions/hops required to reach $q_F$). 
%To achieve that, we first prune the NBA $B$ by removing transitions that cannot be enabled [line \ref{rrt:prune}, Alg. \ref{alg:RRT}]. %This is required to define a distance function over the state-space of the DFA. %
%
%Specifically, the pruned NBA is constructed by removing all infeasible NBA transitions. 
In what follows, we define the \textit{feasible/infeasible} NBA transitions $\delta_B(q_B,\cdot,q_B')$. Transitions that are infeasible are removed giving rise to a pruned automaton. To formally define the \textit{feasible} NBA transitions we first need to introduce the following definitions. %\cite{kantaros2018text}.
%
%We also rewrite $b^{\text{inv}}^{q_D}$ and $b^{\text{next}}^{q_D,q_D'}$ as follows:
%\begin{equation}\label{eq:eq1}
%    b^{\text{inv}}^{q_D} = b^{\text{inv}}^{\text{goal}} \triangle (\neg b^{\text{inv}}^{\text{avoid}} ),
%\end{equation}

%\begin{equation}\label{eq:eq2}
%    b^{\text{next}}^{q_D,q_D'} = b^{\text{next}}^{\text{goal}} \triangle (\neg b^{\text{next}}^{\text{avoid}} ),
%\end{equation}
%where in the Boolean formulas  $b^{\text{next}}^{\text{goal}}$, $b^{\text{next}}^{\text{avoid}}$, $b^{\text{inv}}^{\text{goal}}$ and $b^{\text{inv}}^{\text{avoid}}$ the negation operator does not appear in front of any atomic proposition. Also, in \eqref{eq:eq1} and \eqref{eq:eq2}, $\triangle$ denotes either the logical AND ($\wedge$) or the logical OR $(\vee)$ operator.

% defined in \ref{defn:wTS}.%\footnote{Recall from Definition \ref{defn:wTS} that $\text{wTS}_i$ is defined over $\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma_i=2^{\mathcal{AP}_i}$. Also, recall from Definition \ref{def:pts} that the PTS is defined over $\mathcal{AP}=\bigcup_{i=1}^N\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma=2^{\mathcal{AP}}$. Also, throughout the paper, we denote the finite symbols by $\sigma^*\in\Sigma$ and the infinite symbols by $\sigma\in\Sigma^{\omega}$.}
\begin{definition}[Feasible symbols $\sigma_j\in\Sigma_j$]\label{defn:infTSi}
A symbol $\sigma_j\in\Sigma_j:=2^{\mathcal{AP}_j}$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, where $b_j^{\text{inf}}$ is a Boolean formula defined as 
\begin{equation}\label{bInfTSi}
b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e}(\pi_j^{r_i}\wedge\pi_j^{r_e})).
%b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e})),
\end{equation}
where $b_j^{\text{inf}}$ requires robot $j$ to be present simultaneously in more than one disjoint region.
\end{definition}

%We also need to define when a symbol $\sigma\in\Sigma$ is \textit{feasible}, i.e., when it can be generated by the multi-robot system. To this end, we first need to define the
%In other symbols $\sigma_j\in\Sigma_j=2^{\mathcal{AP}_j}$ that are feasible, i.e, the symbols that can be generated by robot $j$ \cite{kantaros2018text}. 


Note that the Boolean formula $b_j^{\text{inf}}$ is satisfied by any finite symbol $\sigma_j\in\Sigma_j$ that requires robot $j$ to be present in two or more disjoint regions, simultaneously. For instance, the symbol $\sigma_j=\pi_j^{r_i}\pi_j^{r_e}$ satisfies $b_j^{\text{inf}}$ if $r_i$ and $r_e$ are disjoint regions. %\footnote{Note that if we consider regions $r_i$ that are not necessarily disjoint, then the Boolean formula $b_j^{\text{inf}}$ is defined as $b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e}))$. Note also that definition of infeasible symbols depends on the problem at hand, i.e, the definition of atomic propositions included in the sets $\mathcal{AP}_j$.} % if there is an overlap between regions $r_i$ and $r_e$. 
Next, we define the feasible symbols $\sigma\in\Sigma$.

\begin{definition}[Feasible symbols $\sigma\in\Sigma$]\label{defn:infPTS}
A symbol $\sigma\in\Sigma$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, for all robots $j$,
where $\sigma_j=\Pi|_{\Sigma_j}\sigma$, $b_j^{\text{inf}}$ is defined in \eqref{bInfTSi}, and $\Pi|_{\Sigma_j}\sigma$ stands for the projection of the symbol $\sigma$ onto $\Sigma_j$.\footnote{For instance, $\Pi|_{\Sigma_j}(\pi_j^{r_e}\pi_m^{r_h})=\pi_j^{r_e}$.} We denote by $\Sigma_{\text{feas}}\subseteq\Sigma$ the set of all feasible symbols $\sigma\in\Sigma$. 
\end{definition}


%%%
%%%
%Next, we define the $\Sigma(q_D)=\{s\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D)\in\rightarrow_D)\}$ that collects all symbols that the robots can generate to remain in the state $q_D$. We also define the set $\Sigma(q_D,q_D')=\{\sigma\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D')\in\rightarrow_D)\}$ that collects all symbols that enable a transition from $q_D$ to $q_D'$.
%
%Moreover, for each state $q_D$, we define the set $\Sigma(q_D|p)$ that collects all symbols $\sigma$ that robots may observe if they reach $q_D$ through a path $p=q_D^0,\dots,q_D$, i.e., a sequence of states in $\ccalQ_D$ that starts at the initial state $q_D^0$ and ends at the state $q_D$. Note that there may be multiple paths that can reach $q_D$ from $q_D^0$ and, therefore, each state $q_D$ may be associated with more than one set $\Sigma(q_D|p)$. For the initial state, $q_D^0$, there is only one such set  defined as $\Sigma(q_D^0|p)=\Sigma(q_D^0)$, since in a DFA the only path $p$ to reach $q_D^0$ from $q_D^0$ is the self-loop of $q_D^0$.

%To prune the DFA we need first to construct the sets $\Sigma(q_D|p)$. Starting from $q_D^{0}$, we execute the following process for each state $q_D$ that is reachable within one hop from $q_D^0$

%First, we select a state $q_D\in\ccalQ_D$, for which all corresponding sets $\Sigma(q_D|p)$ have been constructed
%%%
%%%
%\red{unclear here..}
%To solve Problem \ref{prob}, we first decompose the assigned task into local point-to-point planning problems. Motion plans that solve these point-to-point navigation problems are locally designed online while adapting to the map of the environment that is built by the robots. The proposed algorithm is summarized in Algorithm \ref{alg:RRT}. 
%


%\begin{algorithm}[t]
%%\footnotesize
%\caption{Pruning a NBA}
%\LinesNumbered
%\label{alg:prune}
%\KwIn{NBA}
%\KwOut{Pruned NBA}
%Remove infeasible transitions (see Definition \ref{def:feas1})\label{prune:inf}\;
%Add auxiliary states and transitions\label{prune:aux}\;
%Initialize $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$, $\ccalQ_B^\text{checked}=\emptyset$, $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$\;\label{prune:init}
%Compute $\ccalQ_{q_B}^{\text{next}}$ for all $q_B\in\ccalQ_B^\text{loop}$\;
%\While{$|\ccalQ_B^{\text{not-checked}}|\neq\emptyset$}{
%    \For{$q_B\in\ccalQ_B^{\text{not-checked}}$}{
%        Compute $\ccalQ_{q_B}^{\text{next}}$\;\label{prune:nextS}
%        \For{$q_B^K\in\ccalQ_{q_B}^{\text{next}}$}{\label{prune:FornextS}
%            Replicate transition $\delta_B^K(q_B,q_B^K)$\;\label{prune:repl}
%            \If{$\delta_B^K(q_B,q_B^K)$ is decomposable (Def. \ref{def:feas})}{
%                $\ccalQ_B^{\text{dec}}=\ccalQ_B^{\text{dec}}\cup\{q_B^K\}$\;\label{prune:UpdLoop} 
%            }
%            \Else{
%                Remove transition $\delta_B^K(q_B,\cdot,q_B^K)$ from the NBA and the set $\ccalP_{q_B}^{\text{next}}$\;\label{prune:remNonDec}
%            }
%        }
%        One-hop transitions $\delta_B(q_B,\cdot,q_B')$ that are not part of any run in $\ccalP_{q_B}^{\text{next}}$ are removed\;\label{prune:prune2}
%    }
%    $\ccalQ_{B}^{\text{checked}}=\ccalQ_{B}^{\text{not-checked}}$\;
%    $\ccalQ_{B}^{\text{not-checked}}=\ccalQ_B^{\text{dec}}\setminus\ccalQ_{B}^{\text{checked}}$\;
%}
%%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
%\end{algorithm}

\begin{algorithm}[t]
%\footnotesize
\caption{Computing Decomposable Transitions}
\LinesNumbered
\label{alg:prune}
\KwIn{Pruned NBA}
\KwOut{Sets $\ccalQ_{q_B}^{\text{next}}$, $\Sigma^{q_B,q_B'}_{\text{dec}}$, $\forall q_B\in\ccalD_{q_B^\text{aux}}$}
%Remove infeasible transitions (see Definition \ref{def:feas1})\label{prune:inf}\;
Add auxiliary states and transitions\label{prune:aux}\;
Compute the set $\ccalD_{q_B^{\text{aux}}}$\;\label{prune:reachAux}
\For{$q_B\in\ccalD_{q_B^{\text{aux}}}$}{
    Initialize $\ccalQ_{q_B}^{\text{next}}=\emptyset$\;
    \For{each run \eqref{eq:run}}{\label{prune:forRun}%that ends in a state $q_B'\in\ccalD_{q_B^{\text{aux}}}$
        \If{$\delta_B^m(q_B,\cdot,q_B')$ is decomposable (Def. \ref{def:feas1})}{\label{prune:ifDec}
        $\ccalQ_{q_B}^{\text{next}}=\ccalQ_{q_B}^{\text{next}}\cup\{q_B'\}$\;\label{prune:upd1}
        }
         Collect in $\Sigma^{q_B,q_B'}_{\text{dec}}$ all symbols $\sigma^{q_B,q_B'}$ that satisfy Def. \ref{def:feas1} \;\label{prune:upd2}
        }

    }
$\ccalQ_B^{\text{dec}}=\bigcup_{q_B\in\ccalD_{q_B^{\text{aux}}}}\ccalQ_{q_B}^{\text{next}}$\;
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}





Next, we define the sets that collect all feasible symbols that enable a transition from an NBA state $q_B$ to another, not necessarily different, NBA state $q_B'$; see also Example \ref{ex:exFeasSets}. This definition relies on the fact that transition from a state $q_B$ to a state $q_B'$ is enabled if a Boolean formula, denoted by $b^{q_B,q_B'}$ and defined over the set of atomic predicates $\mathcal{AP}$, is satisfied.  %The set of all atomic predicates associated with robots $j\in\mathcal{N}_{q_B,q_B'}$ is defined by $\mathcal{AP}_{q_B,q_B'}=\bigcup_{j\in\mathcal{N}_{q_B,q_B'}}\mathcal{AP}_j$.

\begin{definition}[Sets of Feasible Symbols]
Let $\mathcal{AP}_{q_B,q_B'}$ be a set that collects all atomic predicates that appear in the Boolean formula $b^{q_B,q_B'}$ associated with an NBA transition $\delta_B(q_B,\cdot, q_B')$. Given $b^{q_B,q_B'}$, we define the set $\Sigma^{q_B,q_B'}\subseteq 2^{\mathcal{AP}_{q_B,q_B'}}$ 
that collects all symbols $\sigma$ that (i) satisfy the corresponding Boolean formula $b^{q_B,q_B'}$, i.e., $\sigma\models b^{q_B,q_B'}$; and (ii) $\sigma\in\Sigma_{\text{feas}}$. %; and (iii) are associated with robots that appear in $b^{q_B,q_B'}$. 
%If the empty symbol $\varnothing$ satisfies (i), then $\Sigma^{q_B,q_B'}=\set{\varnothing}$. 
%The set $\mathcal{AP}_{q_B,q_B'}$ collects all atomic predicates that appear in $b^{q_B,q_B'}$.
\label{defn:feasSet}
\end{definition}

%Moreover, let $b^{\text{inv}}^{q_D}$ denote the Boolean formula that needs to be satisfied to enable a loop around $q_D$, i.e., a transition from $q_D$ to $q_D$.\footnote{Note that $b^{\text{inv}}^{q_D}$ exists for all states $q_D$, since the `next' operator is excluded from the syntax. Also, the Boolean formulas that should be satisfied to enable a  transition from a state $q_D$ to $q_D'$ can be provided by tools that convert temporal logic formulas to automata.} Let also $\Sigma^{\text{inv}}^{q_D}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b^{\text{inv}}^{q_D}$. 
%
%Let also $b^{\text{next}}^{q_D,q_D'}$ denote the Boolean formula that needs to be satisfied to enable a transition from $q_D$ to $q_D'$ and $\Sigma^{\text{next}}^{q_D,q_D'}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b^{\text{next}}^{q_D,q_D'}$.
%Also, from $\Sigma_{\text{text}}^{q_D,q_D'}$, we exclude symbols associated with robots that do not play any role in satisfying $b^{\text{next}}^{q_D,q_D'}$. For instance, if $b^{\text{next}}^{q_D,q_D'}=\pi_j^{r_e}\vee\pi_j^{r_m}$, then $\Sigma_{\text{text}}^{q_D,q_D'}$ is defined as $\Sigma_{\text{text}}^{q_D,q_D'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$, i.e., it does not include any symbol associated with other robots $i\neq j$ that may also satisfy $b^{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_i^{r_f}$). The same also holds for $\Sigma^{\text{inv}}^{q_D}$; see also Example \ref{ex:feas}. %Additionally, in case the empty symbol, denoted by $\varnothing$ belongs to 
%

Given the sets $\Sigma^{q_B,q_B'}$, we define the infeasible NBA transitions defined as follows:

\begin{definition}[Infeasible NBA Transitions]\label{def:feas1}
A transition $\delta_B(q_B,\cdot,q_B')$ is infeasible if $\Sigma^{q_B,q_B'}=\emptyset$.
\end{definition}

In words, an NBA transition is infeasible if it is enabled only when at least one robot is present in more than one location in the environment simultaneously. All infeasible NBA transitions are pruned; see e.g., Figure \ref{fig:prune}. % line \ref{prune:inf}, Alg. \ref{alg:prune}]. 
%we remove all NBA transitions with $\Sigma_{q_B,q_B'}=\emptyset$, i.e., all transitions that are enabled if at least one robot is present in more than one location in the environment simultaneously [. 



%Next we remove NBA transitions that require robots to move from one region of interest $\ell_i$ to another one $\ell_e$ without visiting any location $\bbq$ in the environment outside $\ell_i$. Such transitions are considered infeasible as they require robots to `jump' from one region of interest to another one. For instance, consider the LTL formula $\phi=\pi_1^{r_1}\ccalU\pi_1^{r_2}$ that requires robot $1$ to be in region $r_1$ until it enters $r_2$. The corresponding NBA is illustrated in Figure \ref{fig:NBA1}. Assume that the initial condition of the robot satisfies $b^{q_B^0,q_B^0}=\pi_1^{r_1}$, i.e., that robot $1$ is initially located in $r_1$. Then the transition from the initial to the final state is considered infeasible as it requires the robot to `jump' from one region of interest to another one. 


\begin{figure}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Original NBA]{
    \label{fig:origNBA}
  \includegraphics[width=0.46\linewidth]{figures/feas1_bf.png}}
  \subfigure[Pruned NBA (Def. \ref{def:feas1})]{
    \label{fig:feas1}
  \includegraphics[width=0.38\linewidth]{figures/NBA2.png}}
%  \caption{FEASIBLE 1}
%  \label{fig:tow7}
%\end{figure}
%
%\begin{figure}[t]
%  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      %\subfigure[Replicating NBA states]{
    %\label{fig:repl}
 % \includegraphics[width=0.3\linewidth]{figures/NBA3.png}}
  \caption{Graphical illustration of Algorithm \ref{alg:prune} applied to the NBA corresponding to $\phi=\square\Diamond(\pi_1^{\ell_1})\wedge\square\Diamond(\pi_1^{\ell_2})$. This formula requires robot $1$ to visit infinitely often $\ell_1$ and $\ell_2$. Figure \ref{fig:origNBA} shows the original NBA where the states $q_B^0$ and $q_F$ correspond to the initial and final state of the NBA. The red dashed transitions are infeasible, as per Definition \ref{def:feas}, as they require robot $1$ to be in $\ell_1$ and $\ell_2$ simultaneously.  These transitions are removed  yielding the pruned NBA shown in Figure \ref{fig:feas1}. An auxiliary state $q_B^{\text{aux}}$ is added to the pruned NBA; see Figure \ref{fig:feas1}.
  Observe in Figure \ref{fig:feas1} that $\ccalD_{q_B^{\text{aux}}}=\{q_B^{\text{aux}},q_B^0,q_B\}$. Also, there are two runs in the form \eqref{eq:run} originating from $q_B$: $\rho_1=q_Bq_B$ and $\rho_2=q_B q_F q_B^0$. Note that the run $\rho=q_B q_F q_B$ cannot be generated as there is no feasible symbol that satisfies $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$. In fact, this run requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$ instantaneously. %Due to $\rho_2$, the intermediate state $q_F$ is replicated so that it has one incoming transition from $q_B$ and one outgoing transition to $q_B^0$; see Figure \ref{fig:repl}. The transition from $q_B$ to the original $q_F$ is removed. 
  Thus $\ccalQ_{q_B}^{\text{next}}=\{q_B,q_B^0\}$. Similarly, for $q_B^0$ there are two runs in the form \eqref{eq:run}: $\rho_1=q_B^0q_B^0$ and $\rho_2=q_B^0 q_B$ and $\ccalQ_{q_B^0}^{\text{next}}=\{q_B,q_B^0\}$.% The set $\ccalQ_B^{\text{dec}}$  constructed by alg. \ref{alg:prune} is $\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}},q_B^0,q_B\}$. 
  %
  %Observe in Figure \ref{fig:feas1} that there is no self-loop for the final state $q_F$. Thus, $q_F$ is replicated twice since it has one incoming and two outgoing transitions as shown in Figure \ref{fig:repl}. In Figure \ref{fig:repl} the multi-hop transition $q_B\rightarrow_B q_F\rightarrow_B q_B$ is removed since there are no symbols that satisfy $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$ (condition (i)-Defn. \ref{def:feas}); in fact this transition requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$. The resulting pruned NBA generated by Algorithm \ref{alg:prune} is shown in Figure \ref{fig:finalPrune}.  
  }
  \label{fig:prune}
\end{figure}

\begin{figure}
    \centering
     %\includegraphics[width=0.6\linewidth]{figures/p1Up2.png}
       \subfigure[Original NBA]{
    \label{fig:origNBAU}
  \includegraphics[width=0.45\linewidth]{figures/NBA1u.png}}
    \subfigure[Pruned NBA]{
    \label{fig:finalNBA2}
  \includegraphics[width=0.45\linewidth]{figures/NBAU.png}}
    %\subfigure[Pruned NBA]{
   % \label{fig:finalNBA3}
  %\includegraphics[width=0.3\linewidth]{figures/nba3u.png}}
    \caption{Effect of the initial robot state in computing decomposable transitions. Figure \ref{fig:origNBAU} depicts the NBA corresponding to $\phi=\pi_1^{\ell_1}\ccalU\pi_1^{\ell_2}$. All transitions are feasible as per Def. \ref{def:feas1}. Observe in Figure \ref{fig:finalNBA2} that if the initial robot state $\bbp(0)=\ell_1$, then $\ccalD_{q_B^{\text{aux}}}=\{q_B^{\text{aux}},q_B^0\}$. Note that the final state $q_F$ is not reachable from $q_B^0$. Also, $\ccalQ_{q_B^{\text{aux}}}^{\text{next}}=\{q_B^0,q_B^{\text{aux}}\}$ and $\ccalQ_{q_B^0}^{\text{next}}=\{q_B^0\}$. Note that the transition from $q_B^0$ to $q_F$ (red dashed line) does not satisfy Def. \ref{def:feas} and therefore the final state $q_F$ is not reachable. %In this case $\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}},q_B^0\}$. 
    If $\bbp(0)=\ell_2$, then $\ccalD_{q_B^{\text{aux}}}=\{q_B^{\text{aux}},q_F\}$, $\ccalQ_{q_B^{\text{aux}}}^{\text{next}}=\{q_B^{\text{aux}},q_F\}$, and $\ccalQ_{q_{F}}^{\text{next}}=\{q_F\}$. %, and $\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}},q_F\}$.
    %$\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}},q_B^0\}$. Also, there only decomposable transition originating from $q_B^0$ is its self-loop. As a result, the transition   Transition from the initial state $q_B^0$ to the final state $q_B^F$ is infeasible as robot $1$ is required to `jump' from $\ell_1$ to $\ell_2$ while $\ell_1$ and $\ell_2$ are disjoint regions.
    }
    \label{fig:NBA1}
\end{figure}


\subsection{Computing Decomposable NBA Transitions}\label{sec:dec}

In this section, we discuss when an NBA transition can be enabled by requiring each robot to solve a local reachability problem; such transitions are called decomposable. The process of determining which NBA transitions are decomposable is summarized in Algorithm \ref{alg:prune} and illustrated in Figures \ref{fig:prune}-\ref{fig:NBA1}.

First, to take into account the initial multi-robot state in this process, we introduce an auxiliary state $q_B^{\text{aux}}$ and transitions from $q_B^{\text{aux}}$ to all initial states $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=\wedge_{j\in\ccalN} L(\bbp_j(0))$, i.e., transition from $q_B^\text{aux}$ to $q_B^0$ can always be enabled; see also Figure \ref{fig:NBA1} [line \ref{prune:aux}, Alg. \ref{alg:prune}]. Hereafter, the auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA. %The set $\ccalQ_B^{\text{dec}}$ is initialized as $\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}}\}$ [line \ref{prune:init}, Alg. \ref{alg:prune}].


Let $\ccalD_{q_B^{\text{aux}}}$ a set that collects all NBA states $q_B$ with a feasible self-loop, as per Definition \ref{def:feas1}, for which there exists a finite and feasible word $w$, i.e., a finite sequence of feasible symbols, that can incur a finite NBA run $\rho_w$ that ends in $q_B$ and activate the self-loop of $q_B$ [line \ref{prune:reachAux}, Alg. \ref{alg:prune}]. In math, $\ccalD_{q_B^{\text{aux}}}$ is defined as:
%$\ccalD_{q_B^{\text{aux}}}$ is defined as:
\begin{align}\label{eq:reach}
    \ccalD_{q_B^{\text{aux}}}=&\{q_B\in\ccalQ_B|\\&(\Sigma^{q_B,q_B}\neq\emptyset)\wedge(\exists w~\text{s.t.}~\rho_{w}=q_B^{\text{aux}}\dots \bar{q}_B q_Bq_B)\nonumber\}.
\end{align}

By definition of $q_B^{\text{aux}}$, we have that $q_B^{\text{aux}}\in\ccalD_{q_B^{\text{aux}}}$. Consider any two states $q_B, q_B'\in\ccalD_{q_B^{\text{aux}}}$ for which there exists a symbol, denoted by $\sigma^{q_B,q_B'}$, the following run, starting from $q_B$, will be generated: 
\begin{equation}\label{eq:run}
    \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}q_B^{K},
\end{equation}
where $q_B'=q_B^K$. In \eqref{eq:run}, the run is defined so that (i) $q_B^k\neq q_B^{k+1}$, for all $k\in\{1,K-1\}$; (ii) $\delta_B(q_B^k,\sigma^{q_B,q_B'},q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$, i.e., the robots cannot remain in any of the intermediate states (if any) that connect $q_B$ to $q_B'$ either because a feasible self-loop does not exist or because $\sigma^{q_B,q_B'}$ cannot activate this self-loop; and (iii) $\delta_B(q_B',\sigma^{q_B,q_B'},q_B')$ i.e., there is a feasible loop associated with $q_B'$ that is activated by $\sigma^{q_B,q_B'}$ and, therefore, the robots can remain in $q_B'$ as long as $\sigma^{q_B,q_B'}$ is generated. The fact that the finite repetition of a \textit{single} symbol needs to generate the run \eqref{eq:run} precludes multi-hop transitions from $q_B$ to $q_B'$ that require a robot to jump from one region of interest to another one instantaneously as such transitions are not meaningful as discussed in Section \ref{sec:PF}; see e.g., Fig. \ref{fig:feas1}. Hereafter, we denote the multi-hop transition incurred due to the run \eqref{eq:run} by  $\delta_{B}^m(q_B,\cdot,q_B')$.

%Hereafter, we denote by $\delta_B^K(q_B,\cdot,q_B^K)$ the multi-hop NBA transition corresponding to the run \eqref{eq:run}. 
%
The symbol $\sigma^{q_B,q_B'}$ is selected from $\Sigma^{q_B,q_B'}$ that is constructed from the Boolean formula \eqref{eq:b} as per Definition \ref{defn:feasSet}.
\begin{equation}\label{eq:b}
   b^{q_B,q_B'}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}.  
\end{equation}
By definition of \eqref{eq:b}, if there exists a symbol $\sigma^{q_B,q_B'}$ that satisfies $b^{q_B,q_B'}$ then the finite word generated by repeating $K+1$ times the symbol $\sigma^{q_B,q_B'}$ can yield the run in \eqref{eq:run}. 
%
%
%
%Note that such a state $q_B^{K}$ can always be reached (assuming $\phi$ is satisfiable), since 
Note that given a state $q_B$, finding a symbol $\sigma^{q_B,q_B'}$ and a state $q_B'$ can be accomplished by viewing the NBA as a directed graph and applying graph-search methods on it.


%Next we define the decomposable transitions $\delta_B^{K_i}(q_B,q_B^{K_i})$; for simplicity of notation, when it is clear from the context we drop the index $i$. If $\delta_B^{K}(q_B,q_B^K)$ is not decomposable, then the multi-hop transition $\delta_B^{K}(q_B,q_B^{K})$ is removed. To define the decomposable transitions, we need first to introduce the following definition. 


%THE ROBOTS IN $\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$ GET OUT OF THEIR CURRENT REGIONS!
%q_B^K\in\ccalQ_B^{\text{dec}}

Next, we define when the multi-hop transition from $q_B$ to $q_B'$ is decomposable. To define this we need first to introduce the following definitions. First, given the Boolean formula $b^{q_B,q_B'}$ in \eqref{eq:b}, we define the set $\ccalN^{q_B,q_B'}\subseteq\ccalN$ that collects the indices of all robots that appear in $b^{q_B,q_B'}$. Also, given a symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$, we define the set $\ccalR^{q_B,q_B'}\subseteq\ccalN^{q_B,q_B'}$ that collects the indices $j$ of the robots that are involved in generating $\sigma^{q_B,q_B'}$. Also, we denote by $L_{j}^{q_B,q_B'}$ the location that robot $j\in\ccalN^{q_B,q_B'}$ should be located to generate $\sigma^{q_B,q_B'}$. Note that for robots $j\in\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$, $L_{j}^{q_B,q_B'}$ corresponds to any location $\bbq\in\Omega$ where no atomic predicates are satisfied; see also Example \ref{ex:exFeasSets}. 



\begin{definition}[Decomposable NBA transitions]\label{def:feas}
A transition $\delta_{B}^m(q_B,\cdot,q_B')$ corresponding to a run as in \eqref{eq:run} is decomposable if for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$, there exists at least one symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$
such that either (A) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}=\emptyset$ or (B) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B'}$.
\end{definition}

Observe that Definition \ref{def:feas} allows us to cast transition from $q_B$ to states $q_B'$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B'}$ needs to move to a region of interest $L_{j}^{q_B,q_B'}$ while avoiding obstacles and/or other regions of interest so that the symbol $\sigma^{q_B,q_B'}$ is generated; this will be discussed in detail in Section \ref{sec:planning}. This decomposition of the temporal logic task allows for computationally and efficient re-planning as the map of the environment is continuously learned.

Moreover, note that there may be more than one (if any) decomposable transitions originating from $q_B\in\ccalD_{q_B^{\text{aux}}}$ [line \ref{prune:forRun}, Alg. \ref{alg:prune}]. Hereafter, we collect all these states in a set $\ccalQ_{q_B}^{\text{next}}$ [line \ref{prune:upd1}, Alg. \ref{alg:prune}], i.e.,
\begin{equation}
    \ccalQ_{q_B}^{\text{next}}=\{q_B'\in\ccalD_{q_B^{\text{aux}}}~|~\delta_B^m(q_B,\cdot,q_B')~\text{is decomposable}\}.
\end{equation}

Also, there may be more than one symbol $\sigma^{q_B,q_B'}$ that satisfies both $b^{q_B,q_B'}$ in \eqref{eq:b} and Definition \ref{def:feas}. As a result, there may be more than one symbol $\sigma^{q_B,q_B'}$ that can enable the decomposable transition from $q_B$ to $q_B'$.  Hereafter, we collect all these symbols in the set $\Sigma_{\text{dec}}^{q_B,q_B'}\subseteq \Sigma^{q_B,q_B'}$ [line \ref{prune:upd2}, Alg. \ref{alg:prune}]. 

\begin{figure}
    \centering
     \includegraphics[width=1\linewidth]{figures/conserv.png}
    \caption{Decomposing global LTL tasks into local reachability tasks is not always possible. This figure shows the NBA corresponding to $\phi=\square(\pi_1^{\ell_0}\vee\pi_2^{\ell_0}) \wedge \Diamond \pi_2^{\ell_1}\wedge \Diamond \pi_2^{\ell_1}$. This formula requires either robot $1$ or $2$ to always be in $\ell_0$ and eventually robots $1$ and $2$ to visit, not necessarily simultaneously, $\ell_1$. Transition from $q_B^0$ to $q_B^F$ is removed as it requires robots to visit more than one location at the same time. Observe that the transitions from $q_B$ to $q_F$ and from $q_B'$ to $q_F$ do not satisfy  Definition \ref{def:feas}, i.e., $\ccalQ_{q_B}^{\text{next}}=\{q_B\}$ and $\ccalQ_{q_B'}^{\text{next}}=\{q_B'\}$, resulting in a disconnected graph $\ccalG$. For instance, consider the transition from $q_B$ to $q_F$. 
    %Assuming that both robots are initially in $\ell_0$, 
    Observe that transition from $q_B$ to $q_F$ cannot be cast as two independent reachability-avoidance problems. In fact, it requires coordination among the robots that is specific to the Boolean formula $b^{q_B,q_F}$. Specifically, when the robots reach $q_B$, we have that robot $1$ is in $\ell_0$ and robot $2$ is in $\ell_1$. To eventually satisfy $b^{q_B,q_F}=(\pi_1^{\ell_0}\wedge\pi_2^{\ell_1})\vee(\pi_2^{\ell_0}\wedge\pi_2^{\ell_1})$, first robot $2$ is required to return in $\ell_0$ while in the meantime robot $1$ should stay in $\ell_0$. Once robot $2$ returns in $\ell_0$, robot $1$ should move to $\ell_1$ enabling the transition to the final state $q_F$.}
    \label{fig:conserv}
\end{figure}
%Nevertheless, a solution exists, as these two transitions can be enabled in practice. 

\begin{rem}[Definition \ref{def:feas}]
Consider any transition $\delta_B^{m}(q_B,\cdot,q_B')$ associated with the finite run \eqref{eq:run}. If $\delta_B^{m}(q_B,\cdot,q_B')$ does not satisfy Definition \ref{def:feas} then this means that the transition from $q_B$ to $q_B'$ may be either feasible to enable but not in a local-reachability fashion (see Figure \ref{fig:conserv}) or impossible to activate as it may require robots to jump from one region of interest to another one (see Figure \ref{fig:NBA1}). %Conditions under which Definition \ref{def:feas} is not conservative are discussed in Section \ref{sec:complOpt}. Specifically, we show that there exists a fragment of LTL so that if Definition \ref{def:feas} is not satisfied then transition from $q_B$ to $q_B'$ is impossible to activate as it requires robots to instantaneously jump from one region of interest to another one.
%Nevertheless, conservative pruning ensures that when the robots reach a state $q_D$, they will always be able to make progress towards accomplishing their task (i.e., reach a new state $q_D'$) regardless of the symbols they have generated to reach $q_D$ by solving local point-to-point navigation problems. A fragment of LTL for which the proposed approach is not conservative is discussed in Section \ref{sec:complOpt}.
\end{rem}

\begin{ex}(Sets of Feasible Symbols)
(a) Consider the Boolean formula $b^{q_B,q_B'}=(\pi_j^{\ell_e}\vee\pi_j^{\ell_m})\wedge(\neg \pi_i^{\ell_e})$, then $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\pi_j^{\ell_e},\pi_j^{\ell_m}, \pi_j^{\ell_e}\pi_j^{\ell_m}\}$. %, i.e., it does not include any symbol associated with other robots $k\neq j$ that may also satisfy $b^{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{\ell_e}\pi_k^{\ell_f}$).
Given the Boolean formula $b^{q_B,q_B'}$, we have that $\ccalN^{q_B,q_B'}=\set{j,i}$.
%
Also, for $\sigma^{q_B,q_B'}=\pi_j^{\ell_e}$, we have that $\ccalR^{q_B,q_B'}=\set{j}$, $L_{j}^{q_B,q_B'}=\ell_e$. (b) Consider the Boolean formula $b^{q_B,q_B'}=\neg \pi_i^{\ell_e}$. In this case $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\varnothing\}$, where $\varnothing$ denotes an empty symbol and is generated when a robot is outside all regions interests and does hit any obstacles. Also, we have that $\ccalN^{q_B,q_B'}=\set{i}$, $\sigma^{q_B,q_B'}=\varnothing$, $\ccalR^{q_B,q_B'}=\emptyset$, and while $L_{i}^{q_B,q_B'}$ corresponds to any location $\bbq$ in the workspace where no atomic predicates are satisfied. 
\label{ex:exFeasSets}
\end{ex}

%\begin{ex}[Feasible DFA transitions]\label{ex:feas}
%(a) Consider the case, where $b^{q_B,q_B}=1$ and $b^{q_B,q_B'}=\pi_j^{\ell_{m}}$. By definition of $\Sigma^{q_B,q_B}$ and $\Sigma^{q_B,q_B'}$, we have that $\Sigma^{q_B,q_B}=\{\varnothing\}$, where $\varnothing$ stands for the empty symbol, and $\Sigma^{q_B,q_B'} =\{\pi_j^{\ell_{m}}\}$. Transition from $q_B$ to $q_B'$ is feasible as per Definition \ref{def:feas}. Recall that the sets $\Sigma^{q_B,q_B}, \Sigma^{q_B,q_B'}$ collect symbols that are associated with robots that play a role in satisfying the respective Boolean formulas. This precludes cases where, e.g., a symbol $\pi_j^{\ell_e}$, $e\neq m$ is included in $\Sigma^{q_B,q_B}$ resulting in erroneously characterizing the transition from $q_D$ to $q_D'$ as infeasible due to condition (iii). 
%%%(b) Consider the following Boolean conditions: $b^{\text{inv}}^{q_D}=b^{\text{inv}}^{q_D'}=\pi_j^{\ell_i}$ and $b^{\text{next}}^{q_D,q_D'}=\pi_j^{\ell_i}\wedge \pi_m^{\ell_h}$. Then the transition from $q_D$ to $q_D'$ is feasible since it satisfies Definition \ref{def:feas}. 
%(b) Consider also the Boolean formulas  $b^{q_B,q_B}=b^{q_B',q_B'}=\pi_j^{\ell_i}$ and $b^{q_B,q_B'}=\pi_j^{\ell_e}\wedge \pi_m^{\ell_h}$, then the transition from $q_B$ to $q_B'$ is infeasible, since it holds that $j\in \ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and, $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. In fact, transition from $q_B$ to $q_B'$ requires robot $j$ to instantaneously move from $\ell_i$ to $\ell_e$ which is not possible given that $\ell_i$ and $\ell_e$ are disjoint regions. 
%\end{ex}

\subsection{Distance Metric Over the Pruned NBA}\label{sec:dist}
Given the pruned NBA, we define a function to compute how far an NBA state is from the set of final states. This metric will be used in Section \ref{sec:planning} to guide planning towards NBA states that are closer to the final states.
%By construction of the pruned automaton, for every a state $q_B\in\ccalQ_B^{\text{dec}}$ there exists a symbol that if repeated a finite number of times then another state $q_B'\in\ccalQ_B^{\text{dec}}$ can be visited while this symbol allows to remain in $q_B'$. Also, as discussed before, transition from $q_B$ to $q_B'$ will occur while possibly going through intermediate states but self-loops are
To this end, we construct a directed graph $\ccalG=\{\ccalV,\ccalE\}$ where $\ccalV$ is the set of nodes defined as $\ccalV=\ccalD_{q_B^{\text{aux}}}$ and $\ccalE\subseteq\ccalV\times\ccalV$ is the set of edges. Specifically, there exists an edge from node $q_B\in\ccalV$ to $q_B'\in\ccalV$ if $\Sigma^{q_B,q_B'}_{\text{dec}}\neq\emptyset$, i.e., if there exists a decomposable transition from $q_B$ to $q_B'$ as per Definition \ref{def:feas}; see Figure \ref{fig:graphG}. 

Given the graph $\ccalG$, we define the distance metric
$d:\ccalV\times\ccalV\rightarrow \mathbb{N}$ that returns the minimum number of transitions among states in $\ccalV$ that are required to reach a state $q_B'\in\ccalV$ starting from a state $q_B\in\ccalV$. %This function will be used to guide the robots towards locations in the workspace so that eventually a final DFA state is visited, i.e., the LTL formula is satisfied.
%
Particularly, we define the distance function $d: \ccalV \times \ccalV \rightarrow \mathbb{N}$ as follows
\begin{equation}\label{eq:dist}
d(q_B,q_B')=\left\{
                \begin{array}{ll}
                  |SP_{q_B,q_B'}|, \mbox{if $SP_{q_B,q_B'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_B,q_B'}$ denotes the shortest path (in terms of hops) in $\ccalG$ from $q_B$ to $q_B'$ and $|SP_{q_B,q_B'}|$ stands for its cost (number of hops). %\footnote{In Section \ref{sec:complOpt}, we provide conditions under which if $d(q_D^0,q_F)=\infty$ then the assigned co-safe LTL task is infeasible}. %; see Sections \ref{sec:targetDFA}-\ref{sec:paths}.
%
Next, we define the final/accepting edges in $\ccalG$.
\begin{definition}[Final/Accepting Edges]\label{def:accEdges}
An edge $(q_B,q_B')\in\ccalE$ is called final or accepting if the corresponding multi-hop NBA transition $\delta_B^m(q_B,\cdot,q_B')$ includes at least one final state $q_F\in\ccalQ_F$.
\end{definition}

Based on the definition of accepting edges, we define the set $\ccalV_F\subseteq \ccalV$ that collects all states $q_B\in\ccalV$ from which an accepting edge originates, i.e.,
\begin{equation}\label{eq:accNode}
    \ccalV_F = \{q_B\in\ccalV~|~\exists~ \text{accepting edge}~(q_B,q_B')\in\ccalE \}.
\end{equation}
By definition of the accepting condition of the NBA, we have that if at least one of the accepting edges is traversed infinitely often, then the corresponding LTL formula is satisfied. %States $q_B\in\ccalQ_B^{\text{dec}}$ for which there are accepting edges $(q_B,q_B')\in\ccalE$ are collected in a set $\ccalQ_F^{\text{dec}}$.%, i.e.,

Similar to \cite{bisoffi2018hybrid}, we define the distance of any state $q_B\in\ccalV$ to the set $\ccalV_F\subseteq \ccalV$ as
\begin{equation}\label{eq:distF}
d_F(q_B,\ccalV_F)=\min_{q_B'\in\ccalV_F}d(q_B,q_B'),
\end{equation}
where $d(q_B,q_B')$ is defined in \eqref{eq:dist} and $\ccalV_F$ is defined in \eqref{eq:accNode}; see Figure \ref{fig:graphG}.

\begin{figure}
    \centering
     %\includegraphics[width=0.6\linewidth]{figures/p1Up2.png}
  \includegraphics[width=0.7\linewidth]{figures/graphG.png}
    \caption{Graph $\ccalG$ constructed for the NBA shown in Figure \ref{fig:feas1}. The red dashed line corresponds to an accepting edge. Also, we have that $\ccalV_F=\{q_B\}$, $d_F(q_B^{\text{aux}},\ccalV_F)=2$, $d_F(q_B^{0},\ccalV_F)=1$, and $d_F(q_B,\ccalV_F)=0$.
    }
    \label{fig:graphG}
\end{figure}

\section{From Automata to Reactive Planning\\in Unknown Occupancy Grid Maps}\label{sec:planning}

%The pruning process described in Section \ref{sec:prune} occurs offline, i.e., before deploying the robots in the workspace. In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

In this section, we present a distributed reactive temporal logic algorithm for robots that operate in unknown environments modeled as occupancy grid maps. The proposed algorithm is summarized in Algorithm \ref{alg:RRT} and requires as an input the output of the Algorithm \ref{alg:prune} that was executed offline. The main idea of Algorithm \ref{alg:RRT} is that the robots select NBA states they should visit next, using the continuously learned map, so that the distance to the final states as per \eqref{eq:distF} decreases over time giving rise to local reachability planning problems. %sets $\ccalQ_{q_B}^{\text{next}}$ and the set of of symbols $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, for all $q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}$ and for all $q_B\in\ccalV$. 
%Recall that $\ccalQ_{q_B}^{\text{next}}$ collects all states, denoted by $q_B^{\text{next}}$, that can reached from $q_B$ in a decomposable fashion, as per Definition \ref{def:feas}, using a symbol selected from $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$. These sets are computed offline by Algorithm \ref{alg:prune} described in Section \ref{sec:aut}.

%for all $q_B\in\ccalQ_B^{\text{dec}}$,  In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

\subsection{Distributed Construction of Robot Paths}\label{sec:paths}
Let $q_B(t)\in\ccalV$ be the NBA state that the robots have reached at time $t$ after following paths, denoted by $\bbp_{j,[0:t]}$ so that the robots can remain in $q_B(t)$ using the current symbol $L(\bbp(t))$, i.e., $L(\bbp(t))\models b^{q_{B}(t),q_{B}(t)}$.
%
At time $t=0$, $q_B(t)$ is initialized to be the initial/auxiliary state $q_B^{\text{aux}}$, introduced in Section \ref{sec:prune} [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. Recall that $q_B^{\text{aux}}\in\ccalV$ and $L(\bbp(0))\models b^{q_{B}(0),q_{B}(0)}$, by definition of $q_B^{\text{aux}}$. 
%


\begin{algorithm}[t]
%\footnotesize
\caption{Distributed LTL Control in Unknown Occupancy Grid Maps}
\LinesNumbered
\label{alg:RRT}
\KwIn{ (i) Initial robot configuration $\bbp(0)$, (ii) Sets $\ccalQ_{q_B}^{\text{next}}$, $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, $\forall q_B\in\ccalV$ provided by Alg. \ref{alg:prune}}
%\KwOut{Terminal horizon $H$, and control inputs $\bbu_{0:H}$}
%Convert $\phi$ into a DFA\label{rrt:dfa}\;
%Initial state $\bbq(0)=[\bbp(0), q_D^0]$;\label{rrt:init}
Initialize $t=0$, $q_B(0)=q_B^{\text{aux}}$\;\label{rrt:t0}
%Update current DFA state as $q_D(0)=\delta(q_D^0,L(\bbp(0)))$\;
%Prune DFA\;\label{rrt:prune}
%Select an initial state $q_D(0)=q_D^0$ and a feasible final state $q_F^{\text{feas}}$\;\label{rrt:feasFinal}
%Current DFA state $q_D(t)=q_D^0$\;\label{rrt:init}
%Compute distance from $q_D(t)$ to $q_D^F$\;
%\If{$d(q_D^0, q_F)= \infty$}{\label{rrt:unsat1}
%Error message: \textit{$\phi$ cannot be satisfied (see Proposition \ref{prop:sat})}\;}\label{rrt:unsat2}
%Initialize $\texttt{updateLoc}=0$ and $\texttt{updateDFA}=0$\;
Select the next NBA state $q_B^{\text{next}}\in\ccalQ_{q_B(t)}^{\text{next}}$\; Select $\sigma^{\text{next}}\in\Sigma_{\text{dec}}^{q_B(t),q_B^{\text{next}}}$\;\label{rrt:selTarget}%(see
Using $\sigma^{\text{next}}$, compute $\ccalN^{\text{next}}$\;\label{rrt:compN}
\While{accepting condition of NBA is not satisfied}{\label{rrt:sat}
%
%\For{$j\in\ccalN^{\text{next}}$}{\label{rrt:for1})
%Using $\sigma^{\text{next}}$, check if $j\in\ccalN^{\text{next}}$ $L_j^{\text{next}}$ \label{rrt:goals}\;
%and the set of robots $\ccalN^{\text{next}}$\;
\For{$j\in\ccalN^{\text{next}}$}{\label{rrt:for1}
Compute paths $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$; see \eqref{eq:localProb}\;\label{rrt:compPaths}%}
Follow paths, re-plan if needed, and update map\;\label{rrt:ExecReplan}%(see Section \ref{sec:exec})
%
\If{$\bbp_j(t)\in L_j^{\text{next}}$}{\label{rrt:T}
Wait until all other robots $j\in\ccalN^{\text{next}}$ reach their goal regions.\;}\label{rrt:wait}
\If{$\bbp_j(t)\in L_j^{\text{next}}, \forall i\in\ccalN^{\text{next}}$}{\label{rrt:nowait}
Update $q_B(t)=q_B^{\text{next}}$\;\label{rrt:updNBA}
Select a new NBA state $q_B^{\text{next}}$ and  $\sigma^{\text{next}}$\;\label{rrt:updTarget}
Using $\sigma^{\text{next}}$, update $\ccalN^{\text{next}}$\;\label{rrt:updN}
%
%Compute new $L_j^{\text{next}}$ and the set of robots $\ccalN^{\text{next}}$\;\label{rrt:UpdGoals}
}
}
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\normalsize

Given the current NBA state $\bbq_B(t)$, the robots coordinate to select a new NBA state, denoted by $q_B^{\text{next}}\in\ccalV$ that they should reach next to make progress towards accomplishing their task [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. This state is selected so that the transition from $q_B$ to $q_B^{\text{next}}$ is decomposable, as per Definition \ref{def:feas}, and progress towards reaching a final state is made. Therefore, the state $q_B^{\text{next}}$ is selected from the set $\ccalQ_{q_B(t)}^{\text{next}}$ based on the following two cases.
%
If $q_B(t)\notin \ccalV_F$, where $\ccalV_F$ is defined in \eqref{eq:accNode}, then among all the states in $\ccalQ_{q_B(t)}^{\text{next}}$ we select one that satisfies
%$q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}\subseteq \ccalQ_B^{\text{dec}}$
\begin{equation}\label{eq:minDist}
d_F(q_B^{\text{next}},\ccalV_F) =  d_F(q_B(t),\ccalV_F)-1,  
\end{equation}
i.e., a state that is one hop closer to the set $\ccalV_F$ than $q_B(t)$ is where $d_F$ is defined in \eqref{eq:distF}.  Under this policy of selecting $q_B^{\text{next}}$, we have that eventually $q_B(t)=\ccalV_F$; design of robot paths to ensure this property will be discussed next. If $q_B(t)\in\ccalV_F$, then the state $q_B^{\text{next}}$ is selected so that $(q_B(t),q_B^{\text{next}})$ is an accepting edge as per Definition \ref{def:accEdges}. This way we ensure that accepting edges are traversed infinitely often and, therefore, the assigned LTL task is satisfied.

%Note that there exists at least one $q_B^{\text{next}}$ that satisfies \eqref{eq:minDist} since any path (including the shortest path) in the pruned NBA that connects $q_B(t)$ to $q_F^{\text{feas}}$ goes through one of the states in $\ccalQ_{q_B(t)}^{\text{next}}$ by construction of the pruned automaton. %and the definition of the distance metric in \eqref{eq:dist}. 
%If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}].

%Given $q_B^{\text{next}}$


%every robot $j$ needs to locally design a path so that a DFA state that is closer to the final state $q_F$ than the current DFA state $q_D(t)$ is eventually reached. 
%The NBA state $q_B^{\text{next}}$ is selected as follows. First, we compute the distance $d(q_B(t),q_F^{\text{feas}})$, where $q_F^{\text{feas}}$ is a final NBA state that is selected offline and is reachable from its initial state $q_B^0$ in the pruned NBA, i.e., $d(q_B^0,q_F^{\text{feas}})\neq\infty$. Then, we select as $q_B^{\text{next}}$ a state that satisfies $d(q_B^{\text{next}},q_F^{\text{feas}}) < d(q_B(t),q_F^{\text{feas}})$,
%\begin{equation}\label{eq:targetDFA}
%   d(q_D^{\text{next}},q_F) = d(q_D(t),q_F) -1, 
%\end{equation}
%i.e., a state that is one hop closer to $q_F^{\text{feas}}$ than $q_B(t)$ is. If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}]. %; see  Sections \ref{sec:paths}. %or realize that a transition from $q_D(t)$ to $q_D^{\text{next}}$ is in fact infeasible; see next section.


%{\bf{Local Construction of Robot Paths:}}

To reach $q_B^{\text{next}}\in\ccalQ_{q_B(t)}^{\text{next}}$ the robots need to eventually generate a symbol from the set $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$; this symbol can be selected randomly. By construction of this symbol, we have that once the robots reach $q_B^{\text{next}}$ they will be able to stay in it as long as they keep generating this symbol; see \eqref{eq:b}.  %Among all such symbols $\sigma^{\text{next}}$, we select the one that yields the smallest set $\ccalN^{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
With slight abuse of notation, we denote the selected symbol by $\sigma^{\text{next}}$ [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. Also, for simplicity of notation we replace $b^{q_B(t),q_B^{\text{next}}}$ and $b^{q_B(t),q_B(t)}$ with $b^{\text{next}}$ and $b^{\text{inv}}$. The same simplification extends to all notation with the same superscripts.
%the corresponding set of robots $\ccalR^{q_B(t),q_B^{\text{next}}}$, $\ccalN^{q_B(t),q_B^{\text{next}}}$, $\ccalR^{q_B(t),q_B(t)}$, and $\ccalN^{q_B(t),q_B(t)}$.

%with $\ccalR^{\text{next}}$ and $\ccalN^{\text{next}}$.


In what follows, we discuss how to design robot paths $\bbp_{j,t:T_j}$, for all robots $j$, that should be followed within a time interval $[t,T_j]$ to ensure that eventually $\sigma^{\text{next}}$ is generated. Given $\sigma^{\text{next}}$, we compute for each robot $j\in\ccalN^{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma^{\text{next}}$. Recall that for robots $j\in\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma^{\text{next}}$  while for robots $j\in\ccalN^{\text{next}}\setminus\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%
Every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%the state $q_B^{\text{next}}$ will be eventually reached and once $q_B^{\text{next}}$ is reached the robots can remain in $q_B^{\text{next}}$ until new observations are made (i.e., until atomic predicates are satisfied/violated). 
%
%For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b^{\text{inv}}$ and $b^{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.
%
%Given the NBA state $q_B^{\text{next}}$, our goal is to design paths $\bbp_{j,t:T_j}$, for all robots $j$ that should be followed within a time interval $[t,T_j]$ so that the NBA transition from $q_B(t)$ to $q_B^{\text{next}}$ is activated. %%\footnote{With slight abuse of notation the subscript in $\bbp_{j,t:T_j}$ denotes the index of robot and the time interval $[t,T_j]$ within which the path should be followed.} 
%To achieve that, it suffices to ensure that the robots follow paths that (i) satisfy the Boolean formula $b^{q_B(t),q_B(t)}$ that allows them to stay in the current NBA state $q_B(t)$, until (ii) the Boolean formula $b^{q_B(t),q_B^{\text{next}}}$ that enables transition from $q_B(t)$ to $q_B^{\text{next}}$ is satisfied while (iii) while never satisfying Boolean formulas $b^{q_B(t),q_B''}$ other than the ones that are satisfied at time $t$.\footnote{At time $t$, the Boolean formula $b^{q_B(t),q_B(t)}$ is satisfied by construction of the pruned automaton. Nevertheless, other Boolean formulas $b^{q_B(t),q_B''}$ may be satisfied as well due to the non-deterministic nature of the NBA.}  For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b^{\text{inv}}$ and $b^{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.
%
%\red{[add reference to lines of the algorithm]}
%To design paths $\bbp_{j,t:T_j}$, \textit{first} the robots $j\in\ccalN^{\text{next}}$ \textit{communicate} to select a symbol $\sigma^{\text{next}}$ that satisfies conditions (i)-(ii) of Definition \ref{def:feas} given the current symbol  $\sigma^{\text{inv}}=L(\bbp(t))$ they are generating. %; see also Example \ref{ex3}. Note that such a symbol exists by construction of the pruned NBA for any symbol $\sigma^{\text{inv}}$. 
%%% \footnote{Note that it is possible that given the symbol that the robots generated to reach $q_D$ there may not exist a pair of symbols $\sigma^{\text{inv}}$ and $\sigma^{\text{next}}$ to reach a state $q_D^{\text{next}}$ that satisfy condition (iii) of Def. \ref{def:feas}. In other words, transition from $q_D$ to $q_D^{\text{next}}$ may not be cast as a point-to-point navigation problem as in \eqref{eq:localProb}.
%Consider e.g., the DFA that corresponds to $\phi=\square(\pi_1^{\ell_0}\vee\pi_2^{\ell_0})\wedge\Diamond(\pi_1^{\ell_1})\wedge\Diamond(\pi_2^{\ell_2})$. 
%Existence of such symbols is always guaranteed for a sub-class of co-safe LTL formulas as discussed in Lemma \ref{lem:cnt}.} %that satisfy $b^{\text{inv}}$ and $b^{\text{next}}$, respectively, i.e., $\sigma^{\text{next}}\models b^{\text{next}}$. This pair of symbols is selected so that condition (ii) of Definition \ref{def:feas} is satisfied; 
%Among all such symbols $\sigma^{\text{next}}$, we select the one that yields the smallest set $\ccalN^{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
%
%Given $\sigma^{\text{next}}$, we compute the set $\ccalR^{\text{next}}$ that collect the robots that need to move towards certain regions of interest $r_e$ in workspace to generate $\sigma^{\text{next}}$. 
%
%\textit{Second}, given $\sigma^{\text{next}}$,  we compute for each robot $j\in\ccalN^{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma^{\text{next}}$. Recall that for robots $j\in\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma^{\text{next}}$  while for robots $j\in\ccalN^{\text{next}}\setminus\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%\textit{Third}, we design the paths $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ for all robots $j\in\ccalN^{\text{next}}$. %First, all robots $j\notin\ccalR^{\text{inv}}$ stay put at their current locations until the state $q_B^{\text{next}}$ is reached. %
%\textit{Third}, every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%that if followed the symbol  $\sigma^{\text{next}}\models b^{\text{next}}$ is generated and the DFA state $q_D^{\text{next}}$ is reached
%In Section \ref{sec:complOpt}, we show that the multi-robot state $\bbp(t)$ already generates a symbol that satisfies $b^{\text{inv}}$. We also show that if (i) the robots that are involved in generating $\sigma^{\text{inv}}$, collected in a set $\ccalR^{\text{inv}}$, stay idle at their current locations $\bbp_j(t)$ and (ii) all other robots 
%
%
%\footnotesize
\begin{subequations}
\label{eq:localProb}
\begin{align}
%& \min_{\substack{T_j, \bbu_{j,t:T_j}}} \left[J(T_j,\bbu_{j,t:T_j}) = \int_{t'=t}^{T_j}  w(\bbp_j(t'),\bbu_j(t'))dt \right] \label{ObjLoc2}\\
& \text{Compute:~}{T_j, \bbu_{j,t:T_j}}~\text{such that}  \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ [L(\bbp_j(t'))=L(\bbp_j(t))] \vee [L(\bbp_j(t'))=\varnothing] \nonumber\\
%& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \vee [L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}],~\forall t'\in[t,T_j] \label{constrLoc1} \\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \cup_i\set{r_i}\setminus (R_j^t\cup L_j^{\text{next}}), \forall t'\in[t,T_j] \label{constrLoc1}\\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \hat{O}(t), \forall t'\in[t,T_j] \label{constrLocObs}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j) \in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin \ccalA_j^{\text{avoid}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
\end{align}
\end{subequations}
%\normalsize

\noindent In \eqref{constrLoc1}, $R_j^t$ denotes the region that robot $j$ lies in at time $t$. The first constraint \eqref{constrLoc1} requires that robot $j$ should not visit any region $r_i$ excluding $R_j^t$ and the target region $L_j^{\text{next}}$, for all $t'\in[t,T_j]$. If at time $t$ robot $j$ does not lie in any of the regions $r_i$, then $R_j^t=\emptyset$. This ensures that the multi-robot system can always remain in $q_B(t)$ as the robots $j\in\ccalN^{\text{next}}$ navigate the workspace; see Lemma \ref{lem:binv}. This constraint can be relaxed by requiring  robot $j\in\ccalN^{\text{next}}$ to always avoid only regions that may result in violating $b^{\text{inv}}$. For instance, if $b^{\text{next}}=\neg(\pi_j^{r_e}\wedge\pi_i^{r_e}$), then it suffices to require robot $j$ to never visit $r_e$.  %\footnote{$T_j^{-}$ denotes a time instant right before $T_j$, i.e., $T_j^{-}=T_j-\epsilon$, for an arbitrarily small $\epsilon>0$.} 
Similarly, the second constraint in \eqref{constrLocObs} requires robot $j$ to avoid all obstacles, collected in $\hat{O}(t)$, that are known up to the time instant $t$. The third constraint in \eqref{constrLoc2} requires robot $j$ to be in region $L_j^{\text{next}}$ at a time instant $T_j\geq t$. %so that it generates $L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}$.%\footnote{Note that this prevents the robot from visiting parts of $L_j^{\text{next}}$ that are shared with other regions $r_i$.} 
This is required to eventually generate the symbol $\sigma^{\text{next}}$. The last constraint in \eqref{constrLoc3} captures the robot dynamics. Note that among all paths that satisfy these constraints, the optimal one, as a per a user-specified motion cost function, can be selected. 
%\textit{Third}, every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%In words, the optimal control problem \eqref{eq:localProb} requires robot $j$ to design a path $\bbp_{j,t:T_j}$ that reaches $L_j^{\text{next}}$ (see \eqref{constrLoc2}) while avoiding certain regions $r_i$ (see \eqref{constrLoc1}) and all detected obstacles denoted by $\hat{O}(t)$ (see \eqref{constrLocObs}). %Note that the robots that do not belong to $\ccalR^{\text{inv}}$ and also are not responsible to generate $\sigma^{\text{next}}$ do not have a target region $L_{j}^{\text{next}}$. These robots remain stationary in their current locations and they do not need to solve \eqref{eq:localProb}.
%
Observe that \eqref{eq:localProb} is a local reachability problem, and, therefore, existing point-to-point navigation algorithms can be used to solve it, e.g., \cite{karaman2011sampling}. Finally observe that given $L_j^{\text{next}}$, robot $j$ locally solves \eqref{eq:localProb} without communicating with any other robot. %Also, since the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable as per Definition \ref{def:feas}, there are no conflicts where a robot would have to stay idle at its current location and at the same time move towards a new location as per the solution to \eqref{eq:localProb}; see also Lemma \ref{lem:binv}. %there is no robot $j$ that belongs to $\ccalR^{\text{inv}}$ that is required to stay idle
%
%Correctness of Alg. \ref{alg:RRT} is discussed in Sec. \ref{sec:complOpt}. %Feasibility of such this problem is examined in 

%We design such paths in two stages. In the first stage, we design subpaths $\bbp_{j,t:\bar{T}_j}$ for some $t<\bar{T}_j<T$ and in the second stage we design paths $\bbp_{j,\bar{T}_j:T_j}$. In particular, \textit{in the first stage} all robots that are involved in generating $\sigma^{\text{inv}}$, collected in a set $\ccalR^{\text{inv}}$, and all other robots $j$ for which it hold $L(\bbp_j(t))=\varnothing$ (i.e., they are outside of all regions $r_i$) stay idle at their current locations $\bbp_j(t)$, i.e., $\bar{T}_j=t+1$ and $\bbp_{j,t:\bar{T}_j}=[\bbp_j(t),\bbp_j(t)]$ All other robots $j$ (i.e., the ones that satisfy $j\notin\ccalR^{\text{inv}}$ and $L(\bbp_j(t))\neq \varnothing$) solve the following optimal control problem to design paths $\bbp_{j,t:\bar{T}_j}$ that if followed then the robots will move outside the regions that they are currently located. %As it will bbe discusses in Section \ref{sec:exec}, these subpaths will be executed so that the robots will move outside their current regions simultaneously.

%\begin{subequations}
%\label{eq:localProb1}
%\begin{align}
%& \min_{\substack{\bar{T}_j, \bbu_{t:\bar{T}_j}}} \left[J(\bar{T}_j,\bbu_{t:\bar{T}_j}) = \sum_{t'=t}^{\bar{T}_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc1}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in R_j(t), \forall t\in\set{t,\dots,\bar{T}_j-1} \label{constrLoc1a} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in \ccalR_j^{\text{inv}}, \forall t\in\set{t,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(\bar{T}_j))=\varnothing \label{constrLoc2a}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   %\bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc2}
%\end{align}
%\end{subequations}
%where $R_j(t)$ denotes the region $r_i$ that robot $j$ lies in at time $t$. Observe that the first two constraints \eqref{constrLoc1a}-\eqref{constrLoc2a} require robot $j$ to move outside the region $\ccalR_j(t)$ where it is located at the time instant $t$. This happens at a time instant $\bar{T}_j$, i.e., $L(\bbp_j(\bar{T}_j))=\varnothing$. Note that robot $j$ locally solves \label{eq:localProb1} with communicating with other robots. Observe that execution of these subpaths ensures that the robots remain in the DFA state $q_D(t)$ since $b^{\text{inv}}$ is always satisfied as the robots $\ccalR^{\text{inv}}$ remain stationary in their current locations that generates  $\sigma^{\text{inv}}\models b^{\text{inv}}$.

%since the robots in $\ccalR^{\text{inv}}$

%In the \textit{second} stage, we construct the subpaths $\bbp_{j,\bar{T}_j:T_j}$ that will enable the transition from $q_D(t)$ to $q_D^{\text{next}}$. For robots $j\in\ccalR^{\text{inv}}$, we select $T_j=\bar{T}_j+1$ and $\bbp_{j,\bar{T}_j:T_j}=[\bbp_{j}(t),\bbp_{j}(t)]$, i.e., these robots still stay idle. In fact, due to the deterministic structure of the DFA, this ensures that the robots remain in the DFA state $q_D(t)$ until the symbol $\sigma^{\text{next}}$ is generated which will activate the transition towards $q_D^{\text{next}}$. To generate the symbol  $\sigma^{\text{next}}$, all other robots $j\notin\ccalR^{\text{inv}}$ design paths $\bbp_{j,\bar{T}_j:T_j}$ by solving the following optimal control problem:

%\begin{subequations}
%\label{eq:localProb}
%\begin{align}
%& \min_{\substack{T_j, \bbu_{\bar{T}_j:T_j}}} \left[J(T_j,\bbu_{\bar{T}_j:T_j}) = \sum_{t'=\bar{T}_j}^{T_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ L(\bbp_j(t'))=\varnothing, \forall t'\in\set{\bar{T}_j,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
%\end{align}
%\end{subequations}



 %This ensures that  transition to a DFA state $q_D'\neq q_D(t)$ that is not $q_D^{\text{next}}$. 
%In the meantime the robots in $\ccalR^{\text{inv}}$ ensure that the current DFA state remain the same in $[t,\bar{T}-1]$, since they stay idle and generate the symbol $\sigma^{\text{inv}}$. Also note that robots in $\ccalR^{\text{inv}}$ do not belong to the set of robots that need to move to another location to generate the symbol $\sigma$, since that would create a conflict; see also Remark \ref{rem:invariant}. 
%The second constraint in \eqref{constrLoc2} requires that at time instant $T_j$, all robots should be in their corresponding locations $L_j^\textbf{}$. Once this happens the symbol $\sigma^{\text{next}}$ is generated and the target DFA state is reached.
%
%Note that infeasibility of \eqref{eq:localProb} is due to the facts (i) the environment is unknown and, therefore, it is not possible to check offline which DFA transitions cannot be enabled because e.g., of the robot dynamics or the existence of obstacles.%; and (ii) the LTL formula $\phi$ is decomposed into local sub-tasks Problem \ref{prob} is solved in a distributed the proposed algorithm is distributed nature of the proposed 

%What if the problem is infeasible? update $\sigma$ i.e., $L_j$. If no other $L_j$. update target DFA state. If no other target DFA state report `current method failed (this does not mean that the task is unsatisfiable though)'

%\begin{ex}[Selection of $\sigma^{\text{next}}$ and $\sigma^{\text{inv}}$]\label{ex3}
%Consider the Boolean formulas $b^{\text{inv}}=\neg \pi_{\text{obs}}$ and $b^{\text{next}}=(\pi_j^{r_1}\vee \pi_j^{r_3} )\wedge\pi_e^{r_2}\wedge (\neg \pi_j^{r_2}) \wedge (\neg (\pi_j^{r_1}\wedge \pi_e^{r_1}))$, where the atomic predicate $\pi_{\text{obs}}$ is true of at least one robot hits an obstacle. A symbol $\sigma^{\text{next}}$ that satisfies $b^{\text{next}}$ is $\sigma^{\text{next}}=\pi_j^{r_1}\pi_e^{r_2}$ while $b^{\text{inv}}$ is satisfied by an empty string, i.e., $\sigma^{\text{inv}}=\varnothing$. Given this pair of symbols, we have that $\ccalR^{\text{inv}}=\emptyset$, $\ccalR^{\text{next}}=\set{j,e}$, $L_j^{\text{next}}=r_1$, and $L_e^{\text{next}}=r_2$.
%\end{ex}

%\begin{ex}[Construction of $\sigma^{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b^{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$. Then, we have that $\sigma^{\text{inv}}=\pi_j^{r_1}$ and $\ccalR^{\text{inv}}=\set{j}$. Similarly, if $b^{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma^{\text{inv}}$ is an empty string and $\ccalR^{\text{inv}}=\emptyset$.
%\end{ex}

%\begin{ex}
%--add automaton figure--and explain--
%\end{ex}
%\begin{rem}[Initialization of $q_B(t)$]
%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}
%\end{rem}
\subsection{Reacting to Map Uncertainty}\label{sec:replan}
%{\bf{Reactive Planning to Map Uncertainty:}}

As the robots follow their paths $\bbp_{j,t:T_j}$, the map $M(t)$ is continuously updated, as per \eqref{eq:updMap}, and the robot paths need to be accordingly revised [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. In fact, reactivity to the environment is required in two cases. First, as the robots follow their paths $\bbp_{j,t:T_j}$, they may discover new obstacles based on their sensor measurements; see \eqref{eq:sensor}. If the discovered obstacles intersect with their paths $\bbp_{j,t:T_j}$, for some $j\in\ccalR^{\text{next}}$, then these robots $j$ locally re-solve \eqref{eq:localProb} using the updated map to design new paths. Note that existing reactive planning algorithms that can address reachability navigation problems in the presence of unknown obstacles can also be used to solve \eqref{eq:localProb}; see e.g., \cite{karaman2011sampling,guzzi2013human,otte2016rrtx,bansal2019combining,ryll2019efficient,elhafsi2019map,zhai2019path,tordesillas2020faster}.

%is not reachable e.g., due to the robot dynamics or 
Second, as the the map $M(t)$ is constructed, goal regions $L_j^{\text{next}}$ may become unreachable because of the structure of the environment (e.g., regions of interest may be surrounded by obstacles). In this case, robots $j$ that cannot reach $L_j^{\text{next}}$ communicate with all other robots so that a new symbol $\sigma^{\text{next}}$ is selected. This process is repeated until a reachable region $L_j^{\text{next}}$ is selected.  %that makes \eqref{eq:localProb} feasible. 
If such a symbol $\sigma^{\text{next}}$ does not exist, then this means that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$, due to the a-priori unknown structure of the environment. Then, the graph $\ccalG$ is updated by removing this transition and a new NBA state $q_B^{\text{next}}$ is selected. If there do not exist any candidate NBA states to be selected as $q_B^{\text{next}}$, then the assigned task cannot be accomplished given the current multi-robot and NBA state. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
In fact, there may exist another sequence of NBA states for which Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible (i.e., paths towards selected goal regions always exist) and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.

%\begin{rem}[Feasibility of \eqref{eq:localProb}]
%Observe that \eqref{eq:localProb} may be \textit{infeasible}. This can be the case e.g., if the region $L_j^{\text{next}}$ is not reachable e.g., due to the robot dynamics or the structure of the environment. In this case, robot $j$ needs to communicate with all other robots so that a new symbol $\sigma^{\text{next}}$ is selected. This process is repeated until regions $L_j^{\text{next}}$ are selected that make \eqref{eq:localProb} feasible. If such a symbol $\sigma^{\text{next}}$ does not exist, then this means that the transition from $q_D(t)$ to $q_D^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$. Then, the pruned DFA is updated by removing this transition. Next, a new target DFA state is selected that is closer to the final state $q_F$ than $q_D(t)$ is. If there do not exist such DFA states then the robots cannot accomplish the assigned task. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
%In fact, there may exist another sequence of DFA states for which  Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
%Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.
%\end{rem}

%{\bf{Asynchronous Execution of Paths:}} 
\subsection{Asynchronous Execution of Paths}\label{sec:exec}
The robots $j\in\ccalR^{\text{next}}$ follow their paths $\bbp_{j,t:T_j}$ to eventually reach their goal regions $L_j^{\text{next}}$. By construction of these paths, the robots may not arrive at the same discrete time instant at their goal regions. To account for this, when a robot $j$ has traversed its path and has reached its goal region, it waits until
all other robots $e\in\ccalR^{\text{next}}$ reach their respective goal regions $L_e^{\text{next}}$ as well [line \ref{rrt:wait}, Alg. \ref{alg:RRT}]. When this happens, the symbol $\sigma^{\text{next}}$ is generated and the NBA state $q_B^{\text{next}}$ is reached as it will be shown in Section \ref{sec:complOpt}. Then a new NBA state is selected [lines \ref{rrt:nowait}-\ref{rrt:updN}, Alg. \ref{alg:RRT}]. This process is repeated indefinitely so that a final state is reached infinitely often [line \ref{rrt:sat}, Alg. \ref{alg:RRT}]. Note also that the robots can execute their paths asynchronously in the sense that the (continuous) time required to move from $\bbp_j(t)$ to $\bbp_j(t+1)$ may differ across the robots; see Sec. \ref{sec:complOpt}.

%transition  the paths can be executed since the robots are allowed to not arrive at the same discrete-time instant at their goal locations, 



%\textit{asynchronously}, i.e., the robots do not need to reach their goal regions at the same (continuous) time instant [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. In fact, when a robot $j$ has traversed its  path and has reached its goal region $L_j^{\text{next}}$, it has to wait until all other robots $e\in\ccalR^{\text{next}}$ reach their respective goal regions $L_e^{\text{next}}$ [line \ref{rrt:wait}, Alg. \ref{alg:RRT}]. When this happens, the symbol $\sigma^{\text{next}}$ is generated and the NBA state $q_B^{\text{next}}$ is reached as it will be shown in Section \ref{sec:complOpt}. Then a new NBA state is selected [lines \ref{rrt:nowait}-\ref{rrt:updN}, Alg. \ref{alg:RRT}]. This process is repeated indefinitely so that a final state is reached infinitely often [line \ref{rrt:sat}, Alg. \ref{alg:RRT}].

%The robots $j\in\ccalR^{\text{next}}$ execute their paths $\bbp_{j,t:T_j}$ \textit{asynchronously}, i.e., the robots do not need to reach their goal regions at the same (continuous) time instant [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. In fact, when a robot $j$ has traversed its  path and has reached its goal region $L_j^{\text{next}}$, it has to wait until all other robots $e\in\ccalR^{\text{next}}$ reach their respective goal regions $L_e^{\text{next}}$ [line \ref{rrt:wait}, Alg. \ref{alg:RRT}]. When this happens, the symbol $\sigma^{\text{next}}$ is generated and the NBA state $q_B^{\text{next}}$ is reached as it will be shown in Section \ref{sec:complOpt}. Then a new NBA state is selected [lines \ref{rrt:nowait}-\ref{rrt:updN}, Alg. \ref{alg:RRT}]. This process is repeated indefinitely so that a final state is reached infinitely often [line \ref{rrt:sat}, Alg. \ref{alg:RRT}].
%In Section \ref{sec:complOpt}, we show the robots remain in the NBA state $q_B(t)$ for all  $t'\in [t, T-1]$ and transition to $q_B^{\text{next}}$ occurs at the time instant $T$. Once this happens, the robots update their current DFA state and select the next DFA state [lines \ref{rrt:T}-\ref{rrt:UpdGoals}]. This process is repeated until the final state $q_F$ is reached.

%
%\begin{rem}\label{rem:invariant}
%Note that once the robots reach a new DFA $q_D$, they satisfy its respective Boolean condition $b^{\text{inv}}$, since the `next' temporal operator is excluded from the task specification. Particularly, if $b^{\text{inv}}$ is not satisfied this implies that once the robots are at locations that generate a symbol that triggers the transition to $q_D$, the robots should immediately leave their locations, which is impossible to specify unless the next operator is included in the specification language. 

%Recall that $\sigma^{\text{inv}}$ is selected to have the minimum length, this means that the minimum number of robots are involved to generate it. Therefore, robots that are required to generate the symbol $\sigma$ are not included in the set $\ccalR^{\text{inv}}$; see also Remark \ref{rem:invariant}.
%Similarly, robots that are responsible to satisfy $b^{\text{next}}$ cannot be responsible for generating the symbol $\sigma^{\text{inv}}$, since the next operator does not exist and all regions are assumed to be disjoint. %(unless there is an overlap..)
%\end{rem}


%\subsection{Online Re-planning}\label{sec:replan}






\begin{rem}[Communication]
%Note that Algorithm \ref{alg:RRT} requires all-time communication to ensure that all robots always have access to the same map $M(t)$. Nevertheless, this requirement can be straightforwardly relaxed by allowing each robot to build their local map $M_j(t)$. Moreover, 
Execution of the paths $\bbp_{j,t:T_j}$ does not require all-time communication among robots, which is typically the case in relevant temporal logic algorithms. Instead, communication is intermittent and is required only in the following two cases: (i) all robots need to communicate with each other to select and update the symbol $\sigma^{\text{next}}$ (ii) every robot $j\in\ccalR^{\text{next}}$ needs to send a message to all other robots in $\ccalR^{\text{next}}$ once it has reached region $L_{j}^{\text{next}}$. %; see Section \ref{sec:exec}.
\end{rem}

%Next, we define the set $\ccalL_j$ that collects all robot positions $\bbp_j$ that violate $b^{\text{inv}}$ regardless of the state of all other robots. For instance, if $b^{\text{inv}}=\neg (\pi_j^{r_e}\wedge \pi_z^{r_h})$, then $\ccalL_j=\emptyset$. On the other hand, if $b^{\text{inv}}=\neg (\pi_j^{r_e})\wedge (\neg \pi_z^{r_h})$ then  $\ccalL_j=\set{r_e}$. Formally, to construct the set, we express the negation of $b^{\text{inv}}$, denoted by $\bar{b}^{\text{inv}}=\neg b^{\text{inv}}$ as


\begin{rem}[Conservativeness]\label{rem:conserv}
Recall that once the robots reach a state $q_B(t)\in\ccalV$ a new state $q_B^{\text{next}}\in\ccalV$ is selected to be reached next.
%
This state is selected from the set $\ccalQ_{q_B(t)}^{\text{next}}\subseteq\ccalV$ that collects all states $q_B^{\text{next}}$ for which the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable, as per Definition \ref{def:feas}, and therefore, this transition can be enabled by solving local reachability tasks as per \eqref{eq:localProb}. Note that there may be states that can be reached from $q_B(t)$ but not in a local-reachability fashion according to Definition \ref{def:feas}; see e.g., Figure \ref{fig:conserv}. As a result, such states are not included in the set $\ccalQ_{q_B(t)}^{\text{next}}$ and, therefore, a solution to Problem \ref{prob} may not be found even if it exists. 
%
\end{rem}
%In Section \ref{sec:complOpt}, we show that there exists a fragment of LTL so that if Definition \ref{def:feas} is not satisfied for a transition $\delta_B^m(q_B,\cdot,q_B')$, then transition from $q_B$ to $q_B'$ is impossible to activate as it requires robots to instantaneously jump from one region of interest to another one. 

%Definition \ref{def:feas} is conservative %Particularly, there may exist (feasible) symbols $\sigma^{q_B,q_B'}$ that satisfy \eqref{eq:b} but they do not satisfy Definition \ref{def:feas}; see e.g., Figure \ref{fig:conserv}. 
%in the sense that if is not satisfied then transition from $q_B$ to $q_B'$ may be either possible but not in a local-reachability fashion (see Figure \ref{fig:conserv}) or impossible as it may require robots to jump from one region of interest to another one (see Figure \ref{fig:NBA1}). Conditions under which Definition \ref{def:feas} is not conservative are discussed in Section \ref{sec:complOpt}. Specifically, we show that there exists a fragment of LTL so that if Definition \ref{def:feas} is not satisfied then transition from $q_B$ to $q_B'$ is impossible to activate as it requires robots to instantaneously jump from one region of interest to another one.
%Nevertheless, conservative pruning ensures that when the robots reach a state $q_D$, they will always be able to make progress towards accomplishing their task (i.e., reach a new state $q_D'$) regardless of the symbols they have generated to reach $q_D$ by solving local point-to-point navigation problems. A fragment of LTL for which the proposed approach is not conservative is discussed in Section \ref{sec:complOpt}.

==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/alg_Mar31_2020.tex <==
%
In this section, we provide an algorithm to decompose an LTL task into reachability tasks. This process occurs offline i.e., before deploying the robots in the unknown environment. Specifically, in Section \ref{sec:nba} we translate the LTL formula into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA). In Section \ref{sec:prune} we prune this automaton by removing infeasible transitions i.e., transitions that are activated if a robot is present in more than one location simultaneously. Then, in Section \ref{sec:dec} we provide conditions under which feasible NBA transitions can be enabled by solving local reachability tasks. Such transitions are called decomposable. Using the definition of feasible and decomposable transitions, in Section \ref{sec:dist} we define a distance metric over the NBA that measures how far the robots are from fulfilling the assigned mission. This metric will be used in Section \ref{sec:planning} to guide and adapt planning to the continuously learned map of the environment.


\subsection{From LTL formulas to Automata}\label{sec:nba}

First, we translate the specification $\phi$, constructed using a set of atomic predicates $\mathcal{AP}$, into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA), defined as follows \cite{baier2008principles} [line \ref{rrt:dfa}, Alg. \ref{alg:RRT}]. %Given a temporal logic formula $\phi$ , with syntax and semantics as described in Definitions \ref{syntax} and \ref{semantics}, respectively, a DFA is defined as follows:

\begin{definition}[NBA]
A Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\rightarrow_B, \ccalQ_F\right)$, where (i) $\ccalQ_{B}$ is the set of states;
(ii) $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is the initial state; (iii) $\delta_B:\ccalQ_B\times\Sigma\rightarrow\ccalQ_B$ is a non-deterministic transition relation, and $\ccalQ_F\subseteq\ccalQ_{B}$ is a set of accepting/final state. 
\end{definition}

To interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times M(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current multi-robot state $\bbp(t)\in\mathbb{R}^{n\times N}$ and the current map $M(t)$ of the environment. An infinite-length discrete plan $\tau=\bbp(0)\bbp(1)\dots$ satisfies $\phi$, denoted by $\tau\models\phi$, if the word $\sigma=L(\bbp(0), M(0))L(\bbp(1),M(1))\dots$ yields an accepting NBA run defined as follows. First, a run of $\rho_B$ of $B$ over an infinite word $\sigma=\sigma(1)\sigma(2)\dots\sigma(t)\dots\in(2^{\mathcal{AP}})^{\omega}$, is a sequence $\rho_B=q_B(0)q_B(1)q_B(2)\dots,q_B(t),\dots$, where $q_B(0)\in\ccalQ_B^0$ and $\delta_B(q_B(t),\sigma(t),q_B(t+1)$, $\forall t\in\mathbb{N}$. %Hereafter, we equivalently denote $\delta_B(q_B(t),\sigma(t),q_B(t+1)$ as $q_B(t)\rightarrow_B q_B(t+1)$.
A run $\rho_B$ is called \textit{accepting} if $\texttt{Inf}(\rho_B)\cap\ccalQ_F\neq\emptyset$, where $\texttt{Inf}(\rho_B)$ represents the set of states that appear infinitely often in $\rho_B$. In words, an infinite-length discrete plan $\tau$ satisfies an LTL formula $\phi$ if it can generate at least one accepting NBA run. Hereafter, for simplicity we replace $L(\bbp(t),M(t))$ with $L(\bbp(t))$.
%The symbols $\sigma$ that result in an accepting run of $D$ constitute the accepted language of $D$.

%The proposed reactive algorithm builds online (i.e., as the robots navigate the environment) paths that live in the infinite-dimensional space $\Omega^N\times\ccalQ_D$. The synthesized paths are updated as the map of the environment is updated. 

%Specifically, let $q_B(t)\in\ccalQ_B$ denote the NBA state that the multi-robot system has reached at time $t$ given all observations that have been made (i.e., all atomic predicates that have been satisfied) until $t$, where $q_B(0)\in\ccalQ_B^0$ [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. 

%In Section \ref{sec:planning}, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task. Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task. To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that (i) it is  one-hop reachable from $q_B(t)$, (ii) the transition from $q_B(t)$ to $q_B^{\text{next}}$ is feasible, i.e., observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously, and (iii) $q_B^{\text{next}}$ is `closer' to the final states than $q_B(t)$ is. %Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. 
%In what follows, we describe these steps in detail.
%In Section \ref{sec:prune} we define when an NBA transition is feasible and when it is decomposable i.e., it can be enabled via solving local reachability-avoidance problems. In Section \ref{sec:dist}, we define a distance metric over the NBA that measures how far each NBA state is from the set of final states.

%Next, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task; see Algorithm \ref{alg:RRT}. Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task. To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that it is (i) one-hop reachable from $q_B(t)$, (ii) `closer' to the final states than $q_B(t)$ is according to a distance function defined over the NBA, and (iii) observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously. Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. In what follows, we describe these steps in detail.


%Once this transition is enabled, the robots update the target DFA state $q_D^{\text{next}}$ until they reach a final DFA state.%\footnote{In case the DFA has more than one initial state, then there is more than one state $\bbq(0)$ that can be used as a root. In this case, a separate tree is build for each one of possible roots.}
%For this, we assume that the initial robot configuration allows the robots to stay in $q_B(0)$.
%

%By convention the cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = 0$, while the cost of a node $\bbq(t+1)=[\bbp(t+1), q_D]\in\ccalV$, given its parent node $\bbq(t)=[\bbp(t),q_D']\in\ccalV$, is computed as 
%\begin{equation}\label{eq:costUpd}
%J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq(t)) +  w(\bbp(t),\bbp(t+1)).
%\end{equation}
%Observe that by applying \eqref{eq:costUpd} recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:Prob2}.

 
%Given the current DFA state $q_D(t)$, the robots first select a DFA state $q_D^{\text{next}}\in\ccalQ_D$ that is `closer' to the final state $q_F$ than $q_D(t)$ is and observations that generate a transition from $q_D(t)$ to $q_D^{\text{next}}$ can be generated. Therefore,
%\subsection{Selecting the Next DFA State}\label{sec:targetDFA}

%{\bf{Pruning the DFA:}}
\subsection{Pruning Infeasible NBA Transitions}\label{sec:prune}
%Given the current NBA state $q_B(t)$, a new state $q_B^{\text{next}}$ is selected so that it is closer to the final states. Thus, to select $q_B^{\text{next}}$, we need to define a distance function over the state-space of the NBA that measures how far each state is from the final state. %(in terms of the number feasible transitions/hops required to reach $q_F$). 
%To achieve that, we first prune the NBA $B$ by removing transitions that cannot be enabled [line \ref{rrt:prune}, Alg. \ref{alg:RRT}]. %This is required to define a distance function over the state-space of the DFA. %
%
%Specifically, the pruned NBA is constructed by removing all infeasible NBA transitions. 
In what follows, we define the \textit{feasible/infeasible} NBA transitions $\delta_B(q_B,\cdot,q_B')$. Transitions that are infeasible are removed giving rise to a pruned automaton. To formally define the \textit{feasible} NBA transitions we first need to introduce the following definitions. %\cite{kantaros2018text}.
%
%We also rewrite $b^{\text{inv}}^{q_D}$ and $b^{\text{next}}^{q_D,q_D'}$ as follows:
%\begin{equation}\label{eq:eq1}
%    b^{\text{inv}}^{q_D} = b^{\text{inv}}^{\text{goal}} \triangle (\neg b^{\text{inv}}^{\text{avoid}} ),
%\end{equation}

%\begin{equation}\label{eq:eq2}
%    b^{\text{next}}^{q_D,q_D'} = b^{\text{next}}^{\text{goal}} \triangle (\neg b^{\text{next}}^{\text{avoid}} ),
%\end{equation}
%where in the Boolean formulas  $b^{\text{next}}^{\text{goal}}$, $b^{\text{next}}^{\text{avoid}}$, $b^{\text{inv}}^{\text{goal}}$ and $b^{\text{inv}}^{\text{avoid}}$ the negation operator does not appear in front of any atomic proposition. Also, in \eqref{eq:eq1} and \eqref{eq:eq2}, $\triangle$ denotes either the logical AND ($\wedge$) or the logical OR $(\vee)$ operator.

% defined in \ref{defn:wTS}.%\footnote{Recall from Definition \ref{defn:wTS} that $\text{wTS}_i$ is defined over $\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma_i=2^{\mathcal{AP}_i}$. Also, recall from Definition \ref{def:pts} that the PTS is defined over $\mathcal{AP}=\bigcup_{i=1}^N\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma=2^{\mathcal{AP}}$. Also, throughout the paper, we denote the finite symbols by $\sigma^*\in\Sigma$ and the infinite symbols by $\sigma\in\Sigma^{\omega}$.}
\begin{definition}[Feasible symbols $\sigma_j\in\Sigma_j$]\label{defn:infTSi}
A symbol $\sigma_j\in\Sigma_j:=2^{\mathcal{AP}_j}$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, where $b_j^{\text{inf}}$ is a Boolean formula defined as 
\begin{equation}\label{bInfTSi}
b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e}(\pi_j^{r_i}\wedge\pi_j^{r_e})).
%b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e})),
\end{equation}
where $b_j^{\text{inf}}$ requires robot $j$ to be present simultaneously in more than one disjoint region.
\end{definition}

%We also need to define when a symbol $\sigma\in\Sigma$ is \textit{feasible}, i.e., when it can be generated by the multi-robot system. To this end, we first need to define the
%In other symbols $\sigma_j\in\Sigma_j=2^{\mathcal{AP}_j}$ that are feasible, i.e, the symbols that can be generated by robot $j$ \cite{kantaros2018text}. 


Note that the Boolean formula $b_j^{\text{inf}}$ is satisfied by any finite symbol $\sigma_j\in\Sigma_j$ that requires robot $j$ to be present in two or more disjoint regions, simultaneously. For instance, the symbol $\sigma_j=\pi_j^{r_i}\pi_j^{r_e}$ satisfies $b_j^{\text{inf}}$ if $r_i$ and $r_e$ are disjoint regions. %\footnote{Note that if we consider regions $r_i$ that are not necessarily disjoint, then the Boolean formula $b_j^{\text{inf}}$ is defined as $b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e}))$. Note also that definition of infeasible symbols depends on the problem at hand, i.e, the definition of atomic propositions included in the sets $\mathcal{AP}_j$.} % if there is an overlap between regions $r_i$ and $r_e$. 
Next, we define the feasible symbols $\sigma\in\Sigma$.

\begin{definition}[Feasible symbols $\sigma\in\Sigma$]\label{defn:infPTS}
A symbol $\sigma\in\Sigma$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, for all robots $j$,
where $\sigma_j=\Pi|_{\Sigma_j}\sigma$, $b_j^{\text{inf}}$ is defined in \eqref{bInfTSi}, and $\Pi|_{\Sigma_j}\sigma$ stands for the projection of the symbol $\sigma$ onto $\Sigma_j$.\footnote{For instance, $\Pi|_{\Sigma_j}(\pi_j^{r_e}\pi_m^{r_h})=\pi_j^{r_e}$.} We denote by $\Sigma_{\text{feas}}\subseteq\Sigma$ the set of all feasible symbols $\sigma\in\Sigma$. 
\end{definition}


%%%
%%%
%Next, we define the $\Sigma(q_D)=\{s\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D)\in\rightarrow_D)\}$ that collects all symbols that the robots can generate to remain in the state $q_D$. We also define the set $\Sigma(q_D,q_D')=\{\sigma\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D')\in\rightarrow_D)\}$ that collects all symbols that enable a transition from $q_D$ to $q_D'$.
%
%Moreover, for each state $q_D$, we define the set $\Sigma(q_D|p)$ that collects all symbols $\sigma$ that robots may observe if they reach $q_D$ through a path $p=q_D^0,\dots,q_D$, i.e., a sequence of states in $\ccalQ_D$ that starts at the initial state $q_D^0$ and ends at the state $q_D$. Note that there may be multiple paths that can reach $q_D$ from $q_D^0$ and, therefore, each state $q_D$ may be associated with more than one set $\Sigma(q_D|p)$. For the initial state, $q_D^0$, there is only one such set  defined as $\Sigma(q_D^0|p)=\Sigma(q_D^0)$, since in a DFA the only path $p$ to reach $q_D^0$ from $q_D^0$ is the self-loop of $q_D^0$.

%To prune the DFA we need first to construct the sets $\Sigma(q_D|p)$. Starting from $q_D^{0}$, we execute the following process for each state $q_D$ that is reachable within one hop from $q_D^0$

%First, we select a state $q_D\in\ccalQ_D$, for which all corresponding sets $\Sigma(q_D|p)$ have been constructed
%%%
%%%
%\red{unclear here..}
%To solve Problem \ref{prob}, we first decompose the assigned task into local point-to-point planning problems. Motion plans that solve these point-to-point navigation problems are locally designed online while adapting to the map of the environment that is built by the robots. The proposed algorithm is summarized in Algorithm \ref{alg:RRT}. 
%


%\begin{algorithm}[t]
%%\footnotesize
%\caption{Pruning a NBA}
%\LinesNumbered
%\label{alg:prune}
%\KwIn{NBA}
%\KwOut{Pruned NBA}
%Remove infeasible transitions (see Definition \ref{def:feas1})\label{prune:inf}\;
%Add auxiliary states and transitions\label{prune:aux}\;
%Initialize $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$, $\ccalQ_B^\text{checked}=\emptyset$, $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$\;\label{prune:init}
%Compute $\ccalQ_{q_B}^{\text{next}}$ for all $q_B\in\ccalQ_B^\text{loop}$\;
%\While{$|\ccalQ_B^{\text{not-checked}}|\neq\emptyset$}{
%    \For{$q_B\in\ccalQ_B^{\text{not-checked}}$}{
%        Compute $\ccalQ_{q_B}^{\text{next}}$\;\label{prune:nextS}
%        \For{$q_B^K\in\ccalQ_{q_B}^{\text{next}}$}{\label{prune:FornextS}
%            Replicate transition $\delta_B^K(q_B,q_B^K)$\;\label{prune:repl}
%            \If{$\delta_B^K(q_B,q_B^K)$ is decomposable (Def. \ref{def:feas})}{
%                $\ccalQ_{B}^{\text{loop}}=\ccalQ_{B}^{\text{loop}}\cup\{q_B^K\}$\;\label{prune:UpdLoop} 
%            }
%            \Else{
%                Remove transition $\delta_B^K(q_B,\cdot,q_B^K)$ from the NBA and the set $\ccalP_{q_B}^{\text{next}}$\;\label{prune:remNonDec}
%            }
%        }
%        One-hop transitions $\delta_B(q_B,\cdot,q_B')$ that are not part of any run in $\ccalP_{q_B}^{\text{next}}$ are removed\;\label{prune:prune2}
%    }
%    $\ccalQ_{B}^{\text{checked}}=\ccalQ_{B}^{\text{not-checked}}$\;
%    $\ccalQ_{B}^{\text{not-checked}}=\ccalQ_{B}^{\text{loop}}\setminus\ccalQ_{B}^{\text{checked}}$\;
%}
%%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
%\end{algorithm}

\begin{algorithm}[t]
%\footnotesize
\caption{Computing Decomposable Transitions}
\LinesNumbered
\label{alg:prune}
\KwIn{Pruned NBA}
\KwOut{Sets $\ccalQ_{B}^{\text{loop}}$, $\ccalQ_{q_B}^{\text{next}}$, $\forall q_B\in\ccalQ_{B}^{\text{loop}}$}
%Remove infeasible transitions (see Definition \ref{def:feas1})\label{prune:inf}\;
Add auxiliary states and transitions\label{prune:aux}\;
Initialize $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$, $\ccalQ_B^\text{checked}=\emptyset$, $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$\;\label{prune:init}
Compute $\ccalQ_{q_B}^{\text{next}}$ for all $q_B\in\ccalQ_B^\text{loop}$\;
\While{$|\ccalQ_B^{\text{not-checked}}|\neq\emptyset$}{
    \For{$q_B\in\ccalQ_B^{\text{not-checked}}$}{
        $\ccalQ_{q_B}^{\text{next}}=\emptyset$\;\label{prune:initNext}
        Compute all runs \eqref{eq:run} starting from $q_B$\;\label{prune:run}
        \For{all runs}{\label{prune:FornextS}
            %Replicate transition $\delta_B^K(q_B,q_B^K)$\;\label{prune:repl}
            \If{$\delta_B^K(q_B,q_B^K)$ is decomposable (Def. \ref{def:feas})}{
                $\ccalQ_{B}^{\text{loop}}=\ccalQ_{B}^{\text{loop}}\cup\{q_B^K\}$\;\label{prune:UpdLoop1} 
                $\ccalQ_{q_B}^{\text{next}}=\ccalQ_{q_B}^{\text{next}}\cup\{q_B^K\}$\;\label{prune:UpdLoop2} 
            }
            %\Else{
             %   Remove transition $\delta_B^K(q_B,\cdot,q_B^K)$ from the NBA and the set $\ccalP_{q_B}^{\text{next}}$\;\label{prune:remNonDec}
            %}
        }
        %One-hop transitions $\delta_B(q_B,\cdot,q_B')$ that are not part of any run in $\ccalP_{q_B}^{\text{next}}$ are removed\;\label{prune:prune2}
    }
    $\ccalQ_{B}^{\text{checked}}=\ccalQ_{B}^{\text{not-checked}}$\;\label{prune:checked} 
    $\ccalQ_{B}^{\text{not-checked}}=\ccalQ_{B}^{\text{loop}}\setminus\ccalQ_{B}^{\text{checked}}$\;\label{prune:notchecked} 
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}





Next, we define the sets that collect all feasible symbols that enable a transition from an NBA state $q_B$ to another, not necessarily different, NBA state $q_B'$; see also Example \ref{ex:exFeasSets}. This definition relies on the fact that transition from a state $q_B$ to a state $q_B'$ is enabled if a Boolean formula, denoted by $b^{q_B,q_B'}$ and defined over the set of atomic predicates $\mathcal{AP}$, is satisfied.  %The set of all atomic predicates associated with robots $j\in\mathcal{N}_{q_B,q_B'}$ is defined by $\mathcal{AP}_{q_B,q_B'}=\bigcup_{j\in\mathcal{N}_{q_B,q_B'}}\mathcal{AP}_j$.

\begin{definition}[Sets of Feasible Symbols]
Let $\mathcal{AP}_{q_B,q_B'}$ be a set that collects all atomic predicates that appear in the Boolean formula $b^{q_B,q_B'}$ associated with an NBA transition $\delta_B(q_B,\cdot, q_B')$. Given $b^{q_B,q_B'}$, we define the set $\Sigma^{q_B,q_B'}\subseteq 2^{\mathcal{AP}_{q_B,q_B'}}$ 
that collects all symbols $\sigma$ that (i) satisfy the corresponding Boolean formula $b^{q_B,q_B'}$, i.e., $\sigma\models b^{q_B,q_B'}$; and (ii) $\sigma\in\Sigma_{\text{feas}}$. %; and (iii) are associated with robots that appear in $b^{q_B,q_B'}$. 
%If the empty symbol $\varnothing$ satisfies (i), then $\Sigma^{q_B,q_B'}=\set{\varnothing}$. 
%The set $\mathcal{AP}_{q_B,q_B'}$ collects all atomic predicates that appear in $b^{q_B,q_B'}$.
\label{defn:feasSet}
\end{definition}

%Moreover, let $b^{\text{inv}}^{q_D}$ denote the Boolean formula that needs to be satisfied to enable a loop around $q_D$, i.e., a transition from $q_D$ to $q_D$.\footnote{Note that $b^{\text{inv}}^{q_D}$ exists for all states $q_D$, since the `next' operator is excluded from the syntax. Also, the Boolean formulas that should be satisfied to enable a  transition from a state $q_D$ to $q_D'$ can be provided by tools that convert temporal logic formulas to automata.} Let also $\Sigma^{\text{inv}}^{q_D}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b^{\text{inv}}^{q_D}$. 
%
%Let also $b^{\text{next}}^{q_D,q_D'}$ denote the Boolean formula that needs to be satisfied to enable a transition from $q_D$ to $q_D'$ and $\Sigma^{\text{next}}^{q_D,q_D'}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b^{\text{next}}^{q_D,q_D'}$.
%Also, from $\Sigma_{\text{text}}^{q_D,q_D'}$, we exclude symbols associated with robots that do not play any role in satisfying $b^{\text{next}}^{q_D,q_D'}$. For instance, if $b^{\text{next}}^{q_D,q_D'}=\pi_j^{r_e}\vee\pi_j^{r_m}$, then $\Sigma_{\text{text}}^{q_D,q_D'}$ is defined as $\Sigma_{\text{text}}^{q_D,q_D'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$, i.e., it does not include any symbol associated with other robots $i\neq j$ that may also satisfy $b^{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_i^{r_f}$). The same also holds for $\Sigma^{\text{inv}}^{q_D}$; see also Example \ref{ex:feas}. %Additionally, in case the empty symbol, denoted by $\varnothing$ belongs to 
%

Given the sets $\Sigma^{q_B,q_B'}$, we define the infeasible NBA transitions defined as follows:

\begin{definition}[Infeasible NBA Transitions]\label{def:feas1}
A transition $\delta_B(q_B,\cdot,q_B')$ is infeasible if $\Sigma_{q_B,q_B'}=\emptyset$.
\end{definition}

In words, an NBA transition is infeasible if it is enabled only when at least one robot is present in more than one location in the environment simultaneously. All infeasible NBA transitions are pruned; see e.g., Figure \ref{fig:prune}. % line \ref{prune:inf}, Alg. \ref{alg:prune}]. 
%we remove all NBA transitions with $\Sigma_{q_B,q_B'}=\emptyset$, i.e., all transitions that are enabled if at least one robot is present in more than one location in the environment simultaneously [. 



%Next we remove NBA transitions that require robots to move from one region of interest $\ell_i$ to another one $\ell_e$ without visiting any location $\bbq$ in the environment outside $\ell_i$. Such transitions are considered infeasible as they require robots to `jump' from one region of interest to another one. For instance, consider the LTL formula $\phi=\pi_1^{r_1}\ccalU\pi_1^{r_2}$ that requires robot $1$ to be in region $r_1$ until it enters $r_2$. The corresponding NBA is illustrated in Figure \ref{fig:NBA1}. Assume that the initial condition of the robot satisfies $b^{q_B^0,q_B^0}=\pi_1^{r_1}$, i.e., that robot $1$ is initially located in $r_1$. Then the transition from the initial to the final state is considered infeasible as it requires the robot to `jump' from one region of interest to another one. 


\begin{figure}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Original NBA]{
    \label{fig:origNBA}
  \includegraphics[width=0.46\linewidth]{figures/feas1_bf.png}}
  \subfigure[Pruned NBA (Def. \ref{def:feas1})]{
    \label{fig:feas1}
  \includegraphics[width=0.38\linewidth]{figures/NBA2.png}}
%  \caption{FEASIBLE 1}
%  \label{fig:tow7}
%\end{figure}
%
%\begin{figure}[t]
%  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      %\subfigure[Replicating NBA states]{
    %\label{fig:repl}
 % \includegraphics[width=0.3\linewidth]{figures/NBA3.png}}
  \caption{Graphical illustration of Algorithm \ref{alg:prune} applied to the NBA corresponding to $\phi=\square\Diamond(\pi_1^{\ell_1})\wedge\square\Diamond(\pi_1^{\ell_2})$. This formula requires robot $1$ to visit infinitely often $\ell_1$ and $\ell_2$. Figure \ref{fig:origNBA} shows the original NBA where the states $q_B^0$ and $q_F$ correspond to the initial and final state of the NBA. The red dashed transitions are infeasible, as per Definition \ref{def:feas}, as they require robot $1$ to be in $\ell_1$ and $\ell_2$ simultaneously.  These transitions are removed  yielding the pruned NBA shown in Figure \ref{fig:feas1}. An auxiliary state $q_B^{\text{aux}}$ is added to the pruned NBA; see Figure \ref{fig:feas1}. Observe in Figure \ref{fig:feas1} that there are two runs in the form \eqref{eq:run} originating from $q_B$: $\rho_1=q_Bq_B$ and $\rho_2=q_B q_F q_B^0$. Note that the run $\rho=q_B q_F q_B$ cannot be generated as there is no feasible symbol that satisfies $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$. In fact, this run requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$ instantaneously. %Due to $\rho_2$, the intermediate state $q_F$ is replicated so that it has one incoming transition from $q_B$ and one outgoing transition to $q_B^0$; see Figure \ref{fig:repl}. The transition from $q_B$ to the original $q_F$ is removed. 
  Thus $\ccalQ_{q_B}^{\text{next}}={q_B,q_B^0}$. Similarly, for $q_B^0$ there are two runs in the form \eqref{eq:run}: $\rho_1=q_B^0q_B^0$ and $\rho_2=q_B^0 q_B$. The set $\ccalQ_{B}^{\text{loop}}$  constructed by alg. \ref{alg:prune} is $\ccalQ_{B}^{\text{loop}}=\{q_B^{\text{aux}},q_B^0,q_B\}$. 
  %
  %Observe in Figure \ref{fig:feas1} that there is no self-loop for the final state $q_F$. Thus, $q_F$ is replicated twice since it has one incoming and two outgoing transitions as shown in Figure \ref{fig:repl}. In Figure \ref{fig:repl} the multi-hop transition $q_B\rightarrow_B q_F\rightarrow_B q_B$ is removed since there are no symbols that satisfy $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$ (condition (i)-Defn. \ref{def:feas}); in fact this transition requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$. The resulting pruned NBA generated by Algorithm \ref{alg:prune} is shown in Figure \ref{fig:finalPrune}.  
  }
  \label{fig:prune}
\end{figure}

\begin{figure}
    \centering
     %\includegraphics[width=0.6\linewidth]{figures/p1Up2.png}
       \subfigure[Original NBA]{
    \label{fig:origNBAU}
  \includegraphics[width=0.45\linewidth]{figures/NBA1u.png}}
    \subfigure[Pruned NBA]{
    \label{fig:finalNBA2}
  \includegraphics[width=0.45\linewidth]{figures/NBAU.png}}
    %\subfigure[Pruned NBA]{
   % \label{fig:finalNBA3}
  %\includegraphics[width=0.3\linewidth]{figures/nba3u.png}}
    \caption{Effect of the initial robot state in computing decomposable transitions. Figure \ref{fig:origNBAU} depicts the NBA corresponding to $\phi=\pi_1^{\ell_1}\ccalU\pi_1^{\ell_2}$. All transitions are feasible as per Def. \ref{def:feas1}. Observe in Figure \ref{fig:finalNBA2} that if the initial robot state $\bbp(0)=\pi_1^{\ell_1}$, then $\ccalQ_{q_B^{\text{aux}}}^{\text{next}}=\{q_B^0,q_B^{\text{aux}}\}$ and $\ccalQ_{q_B^0}^{\text{next}}=\{q_B^0\}$. In other words, the transition from $q_B^0$ to $q_F$ (red dashed line) does not satisfy Def. \ref{def:feas} and therefore the final state $q_F$ is not reachable. In this case $\ccalQ_{B}^{\text{loop}}=\{q_B^{\text{aux}},q_B^0\}$. If $\bbp(0)=\pi_1^{\ell_2}$, then $\ccalQ_{q_B^{\text{aux}}}^{\text{next}}=\{q_B^{\text{aux}},q_F\}$, $\ccalQ_{q_B^{F}}^{\text{next}}=\{q_F\}$, and $\ccalQ_{B}^{\text{loop}}=\{q_B^{\text{aux}},q_F\}$.
    %$\ccalQ_{B}^{\text{loop}}=\{q_B^{\text{aux}},q_B^0\}$. Also, there only decomposable transition originating from $q_B^0$ is its self-loop. As a result, the transition   Transition from the initial state $q_B^0$ to the final state $q_B^F$ is infeasible as robot $1$ is required to `jump' from $\ell_1$ to $\ell_2$ while $\ell_1$ and $\ell_2$ are disjoint regions.
    }
    \label{fig:NBA1}
\end{figure}


\subsection{Computing Decomposable NBA Transitions}\label{sec:dec}

Given any Boolean formula $b^{q_B,q_B'}$, we define the set $\ccalN^{q_B,q_B'}\subseteq\ccalN$ that collects the indices of all robots that appear in $b^{q_B,q_B'}$. Also, given a symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$, we define the set $\ccalR^{q_B,q_B'}\subseteq\ccalN^{q_B,q_B'}$ that collects the indices $j$ of the robots that are involved in generating $\sigma_{q_B,q_B'}$. Also, we denote by $L_{j}^{q_B,q_B'}$ the location that robot $j\in\ccalN^{q_B,q_B'}$ should be located to generate $\sigma^{q_B,q_B'}$. Note that for robots $j\in\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$, $L_{j}^{q_B,q_B'}$ corresponds to any location $\bbq\in\Omega$ where no atomic predicates are satisfied; see also Example \ref{ex:exFeasSets}. 

Consider an NBA state $q_B$ with a feasible self-loop, as per Definition \ref{def:feas1}, that is reachable from the initial state. Given $q_B$, compute a finite $K\geq 1$ so that if a symbol, denoted by $\sigma^{q_B,q_B^K}$, is repeated $K$ times the following finite run will be generated:
\begin{equation}\label{eq:run}
    \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K},
\end{equation}
starting from $q_B$. In \eqref{eq:run}, the run is defined so that (i) $q_B^k\neq q_B^{k+1}$, for all $k\in\{1,K-1\}$; (ii) $\delta_B(q_B^k,\sigma^{q_B,q_B^K},q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$, i.e., the robots cannot remain in any of the intermediate states (if any) that connect $q_B$ to $q_B^K$ either because a feasible self-loop does not exist or because $\sigma^{q_B,q_B^K}$ cannot activate this self-loop; and (iii) $\delta_B(q_B^K,\sigma^{q_B,q_B^K},q_B^{K})$ i.e., there is a feasible loop associated with $q_B^K$ that is activated by $\sigma^{q_B,q_B^K}$ and, therefore, the robots can remain in $q_B^K$ as long as $\sigma^{q_B,q_B^K}$ is generated. The fact that the finite repetition of a \textit{single} symbol needs to generate the run \eqref{eq:run} precludes multi-hop transitions from $q_B$ to $q_B^K$ that require a robot to jump from one region of interest to another one instantaneously as such transitions are not meaningful as discussed in Section \ref{sec:PF}; see e.g., Fig. \ref{fig:feas1}. 

%Hereafter, we denote by $\delta_B^K(q_B,\cdot,q_B^K)$ the multi-hop NBA transition corresponding to the run \eqref{eq:run}. 
%
The symbol $\sigma^{q_B,q_B^K}$ is selected from $\Sigma^{q_B,q_B^K}$ that is constructed from the Boolean formula \eqref{eq:b} as per Definition \ref{defn:feasSet}.
\begin{equation}\label{eq:b}
   b^{q_B,q_B^K}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}.  
\end{equation}
By definition of \eqref{eq:b}, if there exists a symbol $\sigma^{q_B,q_B^K}$ that satisfies $b^{q_B,q_B^K}$ then the finite word generated by repeating $K$ times the symbol $\sigma^{q_B,q_B^K}$ will yield the run in \eqref{eq:run}. 
%
%
%
%Note that such a state $q_B^{K}$ can always be reached (assuming $\phi$ is satisfiable), since 
Finding such a symbol $\sigma^{q_B,q_B^K}$ and a state $q_B^K$ can be accomplished by viewing the NBA as a directed graph and applying graph-search methods on it.


%Next we define the decomposable transitions $\delta_B^{K_i}(q_B,q_B^{K_i})$; for simplicity of notation, when it is clear from the context we drop the index $i$. If $\delta_B^{K}(q_B,q_B^K)$ is not decomposable, then the multi-hop transition $\delta_B^{K}(q_B,q_B^{K})$ is removed. To define the decomposable transitions, we need first to introduce the following definition. 


%THE ROBOTS IN $\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$ GET OUT OF THEIR CURRENT REGIONS!
%q_B^K\in\ccalQ_B^{\text{loop}}
\begin{definition}[Decomposable NBA transitions]\label{def:feas}
A transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ corresponding to a run as in \eqref{eq:run} is decomposable if for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$, there exists at least one symbols $\sigma^{q_B,q_B^{K}}\in\Sigma^{q_B,q_B^K}$
such that $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^K}$.
\end{definition}

Observe that Definition \ref{def:feas} allows us to cast transition from $q_B$ to states $q_B^K$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B^K}$ needs to move to a region of interest $L_{j}^{q_B,q_B^K}$ while avoiding obstacles and/or other regions of interest. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is continuously learned; see Section \ref{sec:planning}. 
%
Moreover, note that it is possible that there is more than one such state $q_B^{K}$ that can be reached from $q_B$ and possibly more than one paths/runs to reach the same $q_B^K$. All (feasible) symbols that can generate a run in the form of \eqref{eq:run} towards a state $q_B^K$ are collected in a set $\Sigma^{q_B,q_B^{K}}_{\text{dec}}$.


Recall that Definition \ref{def:feas} is applied to all states $q_B\in\ccalQ_B^{\text{loop}}$ with feasible self-loops that can be reached from the initial state.  In what follows, we discuss how to compute the set $\ccalQ_B^{\text{loop}}$ which is summarized in Algorithm \ref{alg:prune}. As discussed before, the $\ccalQ_B^{\text{loop}}$ is initialized as $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$ [line \ref{prune:init}, Alg. \ref{alg:prune}]. 
%
All states $q_B\in\ccalQ_B^{\text{loop}}$ for which Definition \ref{def:feas} has been checked are collected in the set $\ccalQ_B^{\text{checked}}\subseteq\ccalQ_B^{\text{loop}}$ and the remaining states of $\ccalQ_B^{\text{loop}}$ are collected in $\ccalQ_B^{\text{not-checked}}$, i.e., $\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$. 
%
These sets are initialized as $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$ and $\ccalQ_B^\text{checked}=\emptyset$  [line \ref{prune:init}, Alg. \ref{alg:prune}]. Next we compute all possible finite runs starting from $q_B$ as defined in \eqref{eq:run} [line \ref{prune:run}, Alg. \ref{alg:prune}]. For each run \eqref{eq:run}, we examine if the corresponding multi-hop transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ is decomposable as per Definition \ref{def:feas} [lines \ref{prune:FornextS}-\ref{prune:UpdLoop2}, Alg. \ref{alg:prune}]. If it is decomposable then we update the set $\ccalQ_B^{\text{loop}}$ as: $\ccalQ_B^{\text{loop}}=\ccalQ_B^{\text{loop}}\cup\{q_B^K\}$ [line \ref{prune:UpdLoop1}, Alg. \ref{alg:prune}]. Also, we update the set $\ccalQ_B^{\text{next}}$ as $\ccalQ_B^{\text{next}}=\ccalQ_B^{\text{next}}\cup\{q_B^K\}$ [line \ref{prune:UpdLoop2}, Alg. \ref{alg:prune}]. The set $\ccalQ_B^{\text{next}}$ is initialized as $\ccalQ_B^{\text{next}}=\emptyset$ and collects all states $q_B^K\in\ccalQ_B^{\text{loop}}$ associated with $q_B$. 
%
Once all runs are examined, we update the set $\ccalQ_B^{\text{checked}}$ as $\ccalQ_B^{\text{checked}}=\ccalQ_B^{\text{checked}}\cup\ccalQ_B^{\text{checked}}\cup\{q_B\}$ and the set $\ccalQ_B^{\text{not-checked}}$ as
$\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$ [lines \ref{prune:checked}-\ref{prune:notchecked}, Alg. \ref{alg:prune}]. This process is repeated for all states $q_B\in\ccalQ_B^{\text{not-checked}}$ and terminates when $\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}=\emptyset$.


%Let also $ \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}$ be a run/path in the NBA that connects. Let also $ \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}$ be a $K$-hop path in the automaton (after removing infeasible transitions) that connect $q_B$ to $q_B^K=q_B'$. Hereafter, we denote a $K$-hop NBA transition as $\delta_B(q_B,\cdot,q_B^K)$. 

---------------------
%Let $q_B$ and $q_B'$ be NBA states with feasible self-loops, i.e., $\Sigma_{q_B,q_B}=\emptyset$ and $\Sigma_{q_B',q_B'}=\emptyset$. Let also $ \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}$ be a $K$-hop path in the automaton (after removing infeasible transitions) that connect $q_B$ to $q_B^K=q_B'$. Hereafter, we denote a $K$-hop NBA transition as $\delta_B(q_B,\cdot,q_B^K)$. 

In Section \ref{sec:planning}, we use the pruned NBA to guide planning as follows. Specifically, assume that at time $t$ the robots reach a state $q_B$ with a feasible self-loop that is activated, i.e., $L(\bbp(t))\models b^{q_B,q_B}$ (i.e., the current observations allow the robots to remain in $q_B$). Then the robots coordinate to select a new state $q_B'\neq q_B$ with a feasible self-loop that will also be activated when the robots reach it at a time $t'>t$. The state $q_B'$ is selected so that progress towards accomplishing the assigned mission is made; this process will be discussed in detail in Section \ref{sec:planning}. Such transitions are called decomposable. Note that transition from $q_B$ to $q_B'$ may be a multi-hop NBA transition. Hereafter, we denote a $K$-hop NBA transition from $q_B$ to $q_B'$ as $\delta_B^K(q_B,\cdot,q_B^K)$, where $q_B^K=q_B'$. %
%
In this section, we define conditions under which transition from $q_B$ to $q_B'$ is decomposable. 
%Transitions $\delta_B^K(q_B,\cdot,q_B^K)$ that cannot be enabled by solving local reachability-avoidance planning problems are called non-decomposable. %and are removed from the NBA.
%
%Next, we remove a transition $\delta_B(q_B,\cdot,q_B')$ only if transition from $q_B$ to $q_B'$ and from $q_B'$ to $q_B'$ can be decomposed into local reachability-avoid tasks per robot. This concept is formalized next. To take into account the initial multi-robot state in this pruning process, first, we introduce auxiliary states $q_B^{\text{aux}}$ and transitions $q_B^{\text{aux}}\rightarrow_B q_B^0$ for all $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=\wedge_j\in\ccalN L(\bbp_j(0))$, i.e., transition from $q_B^\text{aux}$ to $q_B^0$ can always be enabled. Hereafter, the auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA %and are introduced to take into account the initial multi-robot state as it may also result in infeasible NBA transitions; see e.g., Figure \ref{fig:NBA1}. 
%
%Consider any NBA state $q_B$ for which a feasible self-loop (as per Definition \ref{def:feas1}) exists. Also assume that there exists a sequence of observations, i.e., atomic predicates, that the robots can satisfy to reach $q_B$ from an initial state and stay in it, i.e., activate its self-loop. All such states $q_B$ are collected in the set $\ccalQ_B^{\text{loop}}$; computation of $\ccalQ_B^{\text{loop}}$ will be discussed later and summarized in Algorithm \ref{alg:prune}. %Let $q_B^1$ be an NBA state that is within one-hop reachable from $q_B$. %The following process is repeated for all such states $q_B$ and for each transition $\delta_{B}(q_B,\cdot,q_B^1)$ that originates from $q_B$. 
%In what follows, we discuss when $\delta_{B}(q_B,\cdot,q_B^1)$ is non-decomposable and therefore it should be removed. 


All states $q_B$ with feasible self-loops (Definition \ref{def:feas1}) that can reached from the initial state by following decomposable transitions and then stay in it, i.e., activate its self loop, are collected in a set denoted $\ccalQ_B^{\text{loop}}$. Construction of this set is summarized in Algorithm \ref{alg:prune} and will be discussed later. In what follows, we examine if there any decomposable transitions $\delta_{B}^K(q_B,\cdot,q_B^K)$ from a state $q_B\in\ccalQ_B^{\text{loop}}$ towards states $q_B'=q_B^K\in\ccalQ_B^{\text{loop}}$. 
%collects all NBA states with feasible self-loops (Definition \ref{def:feas1}) that can reached from the initial state by following decomposable transitions (Definition \ref{def:feas}).
%If there are no decomposable transitions originating from $q_B\in\ccalQ_B^{\text{loop}}$,
Examples illustrating this process are provided in Figures \ref{fig:prune} and \ref{fig:NBA1}.    %All one-hop transitions $\delta_{B}(q_B,\cdot,q_B')$ that are not part of any decomposable transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ are removed. 

First, to take into account the initial multi-robot state in this process, we introduce auxiliary states $q_B^{\text{aux}}$ and transitions $\delta_B(q_B^{\text{aux}},\cdot, q_B^0)$ for all $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=\wedge_{j\in\ccalN} L(\bbp_j(0))$, i.e., transition from $q_B^\text{aux}$ to $q_B^0$ can always be enabled; see also Figure \ref{fig:NBA1} [line \ref{prune:aux}, Alg. \ref{alg:prune}]. Hereafter, the auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA. The set $\ccalQ_B^{\text{loop}}$ is initialized as $\ccalQ_B^{\text{loop}}=\{q_B^{\text{aux}}\}$ [line \ref{prune:init}, Alg. \ref{alg:prune}].

Given any state $q_B\in\ccalQ_B^{\text{loop}}$, we compute a finite $K\geq 1$ so that if a symbol, denoted by $\sigma^{q_B,q_B^K}$, is repeated $K$ times the following finite run will be generated:
\begin{equation}\label{eq:run}
    \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K},
\end{equation}
starting from $q_B$. In \eqref{eq:run}, the run is defined so that (i) $q_B^k\neq q_B^{k+1}$, for all $k\in\{1,K-1\}$; (ii) $\delta_B(q_B^k,\sigma^{q_B,q_B^K},q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$, i.e., the robots cannot remain in any of the intermediate states (if any) that connect $q_B$ to $q_B^K$ either because a feasible self-loop does not exist or because $\sigma^{q_B,q_B^K}$ cannot activate this self-loop; and (iii) $\delta_B(q_B^K,\sigma^{q_B,q_B^K},q_B^{K})$ i.e., there is a feasible loop associated with $q_B^K$ that is activated by $\sigma^{q_B,q_B^K}$ and, therefore, the robots can remain in $q_B^K$ as long as $\sigma^{q_B,q_B^K}$ is generated. The fact that the finite repetition of a \textit{single} symbol needs generate the run \eqref{eq:run} precludes multi-hop transitions from $q_B$ to $q_B^K$ that require a robot to jump from one region of interest to another one instantaneously as such transitions are not meaningful as discussed in Section \ref{sec:PF}; see e.g., Fig. \ref{fig:feas1}. 

%Hereafter, we denote by $\delta_B^K(q_B,\cdot,q_B^K)$ the multi-hop NBA transition corresponding to the run \eqref{eq:run}. 
%
The symbol $\sigma^{q_B,q_B^K}$ is selected from $\Sigma^{q_B,q_B^K}$ that is constructed from the Boolean formula 
\begin{equation}\label{eq:b}
   b^{q_B,q_B^K}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}.  
\end{equation}
By definition of \eqref{eq:b}, if there exists a symbol $\sigma^{q_B,q_B^K}$ that satisfies $b^{q_B,q_B^K}$ then the finite word generated by repeating $K$ times the symbol $\sigma^{q_B,q_B^K}$ will yield the run in \eqref{eq:run}. 
%
%
%
%Note that such a state $q_B^{K}$ can always be reached (assuming $\phi$ is satisfiable), since 
Finding such a symbol $\sigma^{q_B,q_B^K}$ and a state $q_B^K$ can be accomplished  by viewing the NBA as a directed graph and applying graph-search methods on it.


To define when a transition $\delta_B^K(q_B,\cdot,q_B^K)$ is decomposable, we need first to introduce the following definitions. Given a Boolean formula $b^{q_B,q_B'}$, we define the set $\ccalN^{q_B,q_B'}\subseteq\ccalN$ that collects the indices of all robots that appear in $b^{q_B,q_B'}$. Also, given a symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$, we define the set $\ccalR^{q_B,q_B'}\subseteq\ccalN^{q_B,q_B'}$ that collects the indices $j$ of the robots that are involved in generating $\sigma_{q_B,q_B'}$. Also, we denote by $L_{j}^{q_B,q_B'}$ the location that robot $j\in\ccalN^{q_B,q_B'}$ should be located to generate $\sigma^{q_B,q_B'}$. Note that for robots $j\in\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$, $L_{j}^{q_B,q_B'}$ corresponds to any location $\bbq\in\Omega$ where no atomic predicates are satisfied; see also Example \ref{ex:exFeasSets}.   

%Next we define the decomposable transitions $\delta_B^{K_i}(q_B,q_B^{K_i})$; for simplicity of notation, when it is clear from the context we drop the index $i$. If $\delta_B^{K}(q_B,q_B^K)$ is not decomposable, then the multi-hop transition $\delta_B^{K}(q_B,q_B^{K})$ is removed. To define the decomposable transitions, we need first to introduce the following definition. 


%THE ROBOTS IN $\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$ GET OUT OF THEIR CURRENT REGIONS!
%q_B^K\in\ccalQ_B^{\text{loop}}
\begin{definition}[Decomposable NBA transitions]\label{def:feas}
A transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ corresponding to a run as in \eqref{eq:run} is decomposable if for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$, there exists at least one symbols $\sigma^{q_B,q_B^{K}}\in\Sigma^{q_B,q_B^K}$
such that $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^K}$.
\end{definition}

Observe that Definition \ref{def:feas} allows us to cast transition from $q_B$ to states $q_B^K$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B^K}$ needs to move to a region of interest $L_{j}^{q_B,q_B^K}$ while avoiding obstacles and/or other regions of interest. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is continuously learned; see Section \ref{sec:planning}. 
%
Moreover, note that it is possible that there is more than one such state $q_B^{K}$ that can be reached from $q_B$ and possibly more than one paths/runs to reach the same $q_B^K$. All (feasible) symbols that can generate a run in the form of \eqref{eq:run} towards a state $q_B^K$ are collected in a set $\Sigma^{q_B,q_B^{K}}_{\text{dec}}$.

%All such states are appended to $\ccalQ_{B}^{\text{loop}}$. Thus, the above process is repeated for all finite runs in the form of \eqref{eq:run}. Also, 
%Thus, we define the set $\ccalP_{q_B}^{\text{next}}$ that collects all finite runs, denoted by $\rho_i=q_B q_B^{1,i}\dots q_B^{k_i}\dots q_B^{K_i}$, in the form of \eqref{eq:run} that originate from $q_B\in\ccalQ_B^{\text{loop}}$ and the set $\ccalQ_{q_B}^{\text{next}}$ that collects all states $q_B^{K_i}$. Also, there may be more than one word that can yield the same run $\rho_i$. Thus, we collect in a set $\Sigma^{q_B,q_B^{K_i}}$ all symbols that can yield the run $\rho_i$, i.e., all symbols that satisfy the corresponding formula \eqref{eq:b}. Next, we delete the transition from $q_B$ to $q_B^{1,i}$ and we replicate all intermediate states that connect $q_B$ to $q_B^{K_i}$ so that for each state $q_B^{k_i}$ there is only one incoming transition from $q_B^{k_i-1}$ and one outgoing transition to $q_B^{k_i+1}$. This step allows us to examine each multi-hop transition independently as it is possible that more than one multi-hop transition shares common states.

%or more than one symbol that can be used to reach $q_B^{K}$. For every state $q_B\in\ccalQ_B^{\text{loop}}$, we define the set $\ccalP_{q_B}^{\text{next}}$ that collects all pairs of sets of feasible symbols and states, where the $i$-th pair is denoted by $(\Sigma^{q_B,q_B^{K_i}},q_B^{K_i})$, so that a symbol $\sigma^{q_B,q_B^{K_i}}\in\Sigma^{q_B,q_B^{K_i}}$ satisfies the corresponding formula \eqref{eq:b}, i.e.,
%\begin{align}\label{eq:pairs}
%    \ccalP_{q_B}^{\text{next}} = \{&(\Sigma^{q_B,q_B^{K_i}},q_B^{K_i})~|~\nonumber\\&\sigma^{q_B,q_B^{K_i}}\models b^{q_B,q_B^{K_i}}, \forall \sigma^{q_B,q_B^{K_i}}\in\Sigma^{q_B,q_B^{K_i}}\}
%\end{align}
%


%conditions under which conditions a symbol $\sigma^{q_B,q_B^{K_i}}$ can be generated by solving local/independent reachability-avoid tasks for each robot. If $\sigma^{q_B,q_B^{K_i}}$ can be generated in this way then we call the multi-hop transition from $q_B$ to $q_B^{K_i}$, denoted by $\delta_B^K(q_B,q_B^{K_i})$






%This concept is formalized in lines ??? in Algorithm \ref{alg:prune}. First, we introduce auxiliary states $q_B^{\text{aux}}$ and transitions $q_B^{\text{aux}}\rightarrow_B q_B^0$ for all $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=L(\bbp(0))$. The auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA and are introduced to take into account the initial multi-robot state as it may also result in infeasible NBA transitions; see e.g., Figure \ref{fig:NBA1}. 
%
%The key idea in lines ?? -?? is the following. Consider an NBA $q_B$ for which a feasible self-loop (as per Def??) exists. Assume that there exists a sequence of observations, i.e., atomic predicates that the robots can satisfy to reach $q_B$ from $q_B^{\text{aux}}$. Determining which states $q_B$ satisfy this condition will be discussed later. The following process is repeated for all such states $q_B$. We remove transitions $\delta_{B}(q_B,\cdot,q_B^1)$ (i) if after enabling this transition the robots are required to `jump' from one region of interest to another one so that they eventually visit and remain in another state with a feasible self-loop or (ii) if activation of $\delta_{B}(q_B,\cdot,q_B^1)$ cannot be cast as local reachability-avoid planning tasks per robot; as it will be discussed next condition (ii) is conservative. The latter is formalized in the following definition.

%\begin{definition}[Feasible NBA transitions]\label{def:feas}
%A transition $\delta_{B}(q_B,\cdot,q_B^1)$, $q_B\neq q_B^1$ is feasible if the following two conditions hold. (i) There exists at least one symbol denoted by $\sigma^{q_B,q_B^K}$ and a finite $K\geq 1$ so that the infinite word $w=[\sigma^{q_B,q_B^K}]^\omega$ enables either (A) a run of the form $\rho=q_B q_B^1\dots q_B^{K-1}[q_B^{K}]^\omega$, where $\delta_B(q_B^k,w(k),q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$ or (B) an accepting run $\rho$. The symbol $\sigma^{q_B,q_B^K}$ is selected from $\Sigma^{q_B,q_B^K}$ that is constructed from the Boolean formula $b^{q_B,q_B^K}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}$.
%%$\rho=q_B q_B^1\dots q_B^{m-1}[q_B^{m}\dots q_B^{K-1}q_B^{K}]^\omega$, where $\delta_B(q_B^k,w(k),q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K\}$ and at least one of the final states is appears infinitely often in $\rho$. 
%(ii) For all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$, there exists at least one of the symbols $\sigma^{q_B,q_B^K}$ that satisfy condition (i) and either (A) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^1}$. %%The symbol $\sigma^{q_B,q_B^K}$ is selected from $\Sigma^{q_B,q_B^K}$ which %If $K=0$, conditions (i)-(ii) are applied by replacing $q_B^1$ with $q_B'$. %conditions (i)-(ii) assume
%\end{definition}

%If $\delta_{B}(q_B,\cdot,q_B^1)$ does not satisfy Definition \ref{def:feas}, then it is removed. Note that condition (i)-(A) requires that once robots reach a state $q_B$ with a self-loop and remain in this state, they will always be able to make progress towards accomplishing the assigned task by moving towards a new NBA state $q_B^K$ with a self-loop and remain in it as well. If such states $q_B^K$ do not exist, i.e., if after enabling a transition from $q_B$ to $q_B^1$ the robots will never be able to reach and remain in a state with self-loop, then this means final states can be reached by `instantaneously' moving from one NBA state to another one. Clearly, this requires the robots to jump from one region of interest to enable such transitions unless there is a symbol that if repeated indefinitely, at least one final state will be visited infinitely often. This is captured by condition (i)-(B).  Condition (ii) allows us to cast transition from $q_B$ to states $q_B^K$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B^K}$ needs to move to a region of interest while avoiding certain regions and obstacles. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is continuously learned. 
%
%Also, by construction of the pruned automaton we have that once the robots reach an NBA state $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$, i.e., an NBA state for which a self-loop exists, the robots can remain in this state given their current observations. To enforce this property from $t=0$, we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$. This property will be used in Section \ref{sec:planning} to design robot paths.


Recall that Definition \ref{def:feas} is applied to all states $q_B\in\ccalQ_B^{\text{loop}}$ with feasible self-loops that can be reached from the initial state.  In what follows, we discuss how to compute the set $\ccalQ_B^{\text{loop}}$ which is summarized in Algorithm \ref{alg:prune}. As discussed before, the $\ccalQ_B^{\text{loop}}$ is initialized as $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$ [line \ref{prune:init}, Alg. \ref{alg:prune}]. 
%
All states $q_B\in\ccalQ_B^{\text{loop}}$ for which Definition \ref{def:feas} has been checked are collected in the set $\ccalQ_B^{\text{checked}}\subseteq\ccalQ_B^{\text{loop}}$ and the remaining states of $\ccalQ_B^{\text{loop}}$ are collected in $\ccalQ_B^{\text{not-checked}}$, i.e., $\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$. 
%
These sets are initialized as $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$ and $\ccalQ_B^\text{checked}=\emptyset$  [line \ref{prune:init}, Alg. \ref{alg:prune}]. Next we compute all possible finite runs starting from $q_B$ as defined in \eqref{eq:run} [line \ref{prune:run}, Alg. \ref{alg:prune}]. For each run \eqref{eq:run}, we examine if the corresponding multi-hop transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ is decomposable as per Definition \ref{def:feas} [lines \ref{prune:FornextS}-\ref{prune:UpdLoop2}, Alg. \ref{alg:prune}]. If it is decomposable then we update the set $\ccalQ_B^{\text{loop}}$ as: $\ccalQ_B^{\text{loop}}=\ccalQ_B^{\text{loop}}\cup\{q_B^K\}$ [line \ref{prune:UpdLoop1}, Alg. \ref{alg:prune}]. Also, we update the set $\ccalQ_B^{\text{next}}$ as $\ccalQ_B^{\text{next}}=\ccalQ_B^{\text{next}}\cup\{q_B^K\}$ [line \ref{prune:UpdLoop2}, Alg. \ref{alg:prune}]. The set $\ccalQ_B^{\text{next}}$ is initialized as $\ccalQ_B^{\text{next}}=\emptyset$ and collects all states $q_B^K\in\ccalQ_B^{\text{loop}}$ associated with $q_B$. 
%
Once all runs are examined, we update the set $\ccalQ_B^{\text{checked}}$ as $\ccalQ_B^{\text{checked}}=\ccalQ_B^{\text{checked}}\cup\ccalQ_B^{\text{checked}}\cup\{q_B\}$ and the set $\ccalQ_B^{\text{not-checked}}$ as
$\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$ [lines \ref{prune:checked}-\ref{prune:notchecked}, Alg. \ref{alg:prune}]. This process is repeated for all states $q_B\in\ccalQ_B^{\text{not-checked}}$ and terminates when $\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}=\emptyset$.
%all states $q_B^{K}$ that exist in $\ccalQ_{q_B}^{\text{next}}$ and can be reached through a symbol that satisfies Definition \ref{def:feas}. 
%Once all states in $\ccalQ_B^{\text{not-checked}}$ are examined, we update the set   $\ccalQ_B^{\text{not-checked}}$ as $\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$. This process is repeated until $\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}=\emptyset$. %Definition \ref{def:feas} has been applied to all transitions originated from states with feasible self-loops that can be reached from $q_B^{\text{aux}}$. 
Algorithm \ref{alg:prune} will terminate due to the finite set of NBA states and transitions. By construction of Algorithm \ref{alg:prune}, $\ccalQ_B^{\text{loop}}$ collects all NBA states with feasible self-loops (Definition \ref{def:feas1}) that can reached from the initial state by following decomposable transitions (Definition \ref{def:feas}).

%\begin{rem}[Non-emptiness of $\ccalQ_{q_B}^{\text{next}}$]
%Note that $\ccalQ_{q_B}^{\text{next}}\setminus\{q_B\}\neq\emptyset$ for all states $q_B\in\ccalQ_B^{\text{loop}}$ (assuming $\phi$ is satisfiable), since otherwise the only way to visit the final state after visiting $q_B$ is by instantaneously jumping from one NBA state to another one i.e., without staying in any of them. Nevertheless, such transitions cannot exist, as they would require new observations to be made every time a new NBA state is visited which is impossible to specify given that the `next' operator is omitted. %In case $\ccalQ_{q_B}^{\text{next}}=\emptyset$, then $\delta_B(q_B,\cdot,q_B^1)$ is removed.
%\end{rem}

%\begin{rem}[Conflict-free pruning]
%Note that if $\delta_{B}^K(q_B,\cdot,q_B^K)$ is decomposable as per Definition \ref{def:feas} then this means that there may exist states $q_B^k$, $k\in\{1,\dots,K-1\}$, with feasible self-loops without being activated by $\sigma^{q_B,q_B^K}$. Note that none of the transitions $\delta_B(q_B^k,\cdot,q_B^{k+1})$ should be removed at subsequent iterations of Algorithm \ref{alg:prune} since otherwise  $q_B^K$ may not be reachable from $q_B$. However, if there is a sequence of observations so that $q_B^k$ is reached from the initial state, then Definition \ref{def:feas} will be applied to the transition $\delta_B(q_B^k,\cdot,q_B^{k+1})$. If Definition \ref{def:feas} is not satisfied, then $\delta_B(q_B^k,\cdot,q_B^{k+1})$ should be removed which creates a conflict. To avoid such conflicts, if $\delta_{B}^K(q_B,\cdot,q_B^K)$ is decomposable, then we replicate all states $q_B^k$ with self-loops so that they have only one incoming transition which is  $\delta_{B}(q_B^{k-1},\cdot,q_B^k)$ and one outgoing transition which is $\delta_{B}(q_B^{k},\cdot,q_B^{k+1})$. By construction, the replicated state can be reached only through $q_B$ and therefore, it will never be removed. This is applied to all states $q_B^K$ collected in $\ccalQ_{q_B}^{\text{next}}$. Note that in our conducted experiments such conflicts never occurred.
%\end{rem}

%END END END


%In words, a transition from $q_B$ to $q_B'$ is feasible and, therefore, it is not removed (a) if the set $\Sigma^{q_B,q_B}$ is non-empty, i.e., there are feasible symbols that allow the robots to stay in state $q_B$; and (ii) for each possible symbol in $\Sigma^{q_B,q_B}$ that the robots may generate to reach $q_B'$, there exists a feasible symbol that will enable the robots to eventually reach a new state $q_B'$ from $q_B$ and stay in $q_B'$. Also, in (iii) we require the set of robots in $\ccalN^{q_B,q_B'}$ that to be either (a) disjoint from the set of robots in $\ccalR^{q_B,q_B}$ or (b) if there exist robots $j\in \ccalR^{q_B,q_B}\cap\ccalN^{\text{next}}^{q_B,q_B'}\neq\emptyset$ then these robots should suffice to stay in their current locations, i.e., $L_{j}^{q_B,q_B'}=L_{j}^{q_B,q_B}$, to `contribute' to satisfaction of $b^{\text{next}}^{q_D,q_D'}$. As it will be discussed later, this allows us to cast transition from $q_B$ to $q_B'$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalN^{q_B,q_B'}$ needs to move to a region of interest while avoiding certain regions and obstacles. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is learned.

%IN THE PRUNED AUTOMATON WE HAVE THAT ONCE WE VISIT A SELF-LOOP STATE WE CAN STAY IN IT MAKE PROGRESS I.E. VISIT NEW TASKS. This essentially allows us to avoid cases WHERE ROBOTS HAVE TO 'JUMP' FROM ONE REGION OF INTEREST TO ANOTHER ONE. WE USE THIS PROPERTY FOR PLANNING IN SECTION ?. TO ENFORCE THIS PROPERTY AT T=0, WE ASSUME THAT THE INITIAL CONDITION ALWAYS SATISFIES THE INITIAL SELF-LOOP IF IT EXISTS. 

%OR AVOID IT AND MENTION IT IN THE THEOREMS!!!

%IT IS POSSIBLE THAT THE INIT STATE DOES NOT HAVE A SELF LOOP OR THE INIT ROBOT STATE DOES NOT SATISFY.

%SAY HERE THAT OUR GOAL IS THAT ONCE WE VISIT A STATE WITH SELF LOOPS TO SATISFY THE RESPECTIVE CONDITION UNTIL WE MAKE NEW OBSERVATIONS THAT WILL ALLOWS US TO MAKE PROGRESS IE VISIT NEW TASKS


%\begin{ex}[Conservative Pruning]
%-Add figure and explain-
%\end{ex}
\begin{figure}
    \centering
     \includegraphics[width=1\linewidth]{figures/conserv.png}
    \caption{Example of conservativeness of Definition \ref{def:feas} for the NBA corresponding to $\phi=\square(\pi_1^{r_0}\vee\pi_1^{r_0}) \wedge \Diamond \pi_2^{r_1}\wedge \Diamond \pi_2^{r_1}$. This formula requires either robot $1$ or $2$ to always be in $\ell_0$ and eventually robots $1$ and $2$ to visit, not necessarily simultaneously, $\ell_1$. Transition from $q_B^0$ to $q_B^F$ is removed as it requires robots to visit more than one location at the same time. Transitions from $q_B$ to $q_F$ and from $q_B'$ to $q_F$ are removed as they violate both conditions of Definition \ref{def:feas} resulting in a disconnected pruned NBA, i.e., Algorithm \ref{alg:RRT} will not be able to find a solution. Nevertheless, a solution exists, as these two transitions can be enabled in practice. For instance, consider the transition from $q_B$ to $q_F$. %Assuming that both robots are initially in $\ell_0$, 
    Observe that transition from $q_B$ to $q_F$ cannot be cast as two independent reachability-avoidance problems. In fact, it requires coordination among the robots that is specific to the Boolean formula $b^{q_B,q_F}$. Specifically, when the robots reach $q_B$, we have that robot $1$ is in $\ell_0$ and robot $2$ is in $\ell_1$. To eventually satisfy $b^{q_B,q_F}=(\pi_1^{\ell_0}\wedge\pi_2^{\ell_1})\vee(\pi_2^{\ell_0}\wedge\pi_2^{\ell_1})$, first robot $2$ is required 
    to return in $\ell_0$ while in the meantime robot $1$ should stay in $\ell_0$. Once robot $2$ returns in $\ell_0$, robot $1$ should move to $\ell_1$ enabling the transition to the final state $q_F$.}
    \label{fig:conserv}
\end{figure}
%
%Conditions under which Definition \ref{def:feas} is not conservative are presented in Section \ref{sec:complOpt}.%, and/or (c) if it is (physically) impossible for the robots to stay in $q_D$ until the symbol $\sigma^{\text{next}}$, that triggers transition to $q_D'$, is generated; the latter happens if condition (iii) is not true (see also Ex. \ref{ex:feas}). 


\begin{rem}[Conservativeness]\label{rem:conserv}
%First, note that requiring a multi-hop transition to be enabled if the Boolean formula \eqref{eq:b} is satisfied is not conservative, since if \eqref{eq:b} is not satisfied then, this means that to enable this transition at least one robot has to instantaneously move from o
Algorithm \ref{alg:prune} is conservatice due to Definition \ref{def:feas}. Particularly, there may exist (feasible) symbols $\sigma^{q_B,q_B^K}$ that satisfy \eqref{eq:b} but they do not satisfy Definition \ref{def:feas}; see e.g., Figure \ref{fig:conserv}. Conditions under which Definition \ref{def:feas} and, consequently Algorithm \ref{alg:prune}, is not conservative are discussed in Section \ref{sec:complOpt}.
%Nevertheless, conservative pruning ensures that when the robots reach a state $q_D$, they will always be able to make progress towards accomplishing their task (i.e., reach a new state $q_D'$) regardless of the symbols they have generated to reach $q_D$ by solving local point-to-point navigation problems. A fragment of LTL for which the proposed approach is not conservative is discussed in Section \ref{sec:complOpt}.
\end{rem}

\begin{ex}(Sets of Feasible Symbols)
(a) Consider the Boolean formula $b^{q_B,q_B'}=(\pi_j^{r_e}\vee\pi_j^{r_m})\wedge(\neg \pi_i^{r_e})$, then $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$. %, i.e., it does not include any symbol associated with other robots $k\neq j$ that may also satisfy $b^{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_k^{r_f}$).
Given the Boolean formula $b^{q_B,q_B'}$, we have that $\ccalN^{q_B,q_B'}=\set{j,i}$.
%
Also, for $\sigma^{q_B,q_B'}=\pi_j^{r_e}$, we have that $\ccalR^{q_B,q_B'}=\set{j}$, $L_{j}^{q_B,q_B'}=r_e$. (b) Consider the Boolean formula $b^{q_B,q_B'}=\neg \pi_i^{r_e}$. In this case $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\varnothing\}$, where $\varnothing$ denotes an empty symbol and is generated when a robot is outside all regions interests and does hit any obstacles. Also, we have that $\ccalN^{q_B,q_B'}=\set{i}$, $\sigma^{q_B,q_B'}=\varnothing$, $\ccalR^{q_B,q_B'}=\emptyset$, and while $L_{i}^{q_B,q_B'}$ corresponds to any location $\bbq$ in the workspace where no atomic predicates are satisfied. 
\label{ex:exFeasSets}
\end{ex}

\subsection{Distance Metric Over the Pruned NBA}\label{sec:dist}
Given the pruned NBA, we define a function to compute how far two NBA states that belong to $\ccalQ_B^{\text{loop}}$ are. This metric will be used in Section \ref{sec:planning} to guide planning towards states in $\ccalQ_B^{\text{loop}}$ that are closer to the final states.
%By construction of the pruned automaton, for every a state $q_B\in\ccalQ_B^{\text{loop}}$ there exists a symbol that if repeated a finite number of times then another state $q_B'\in\ccalQ_B^{\text{loop}}$ can be visited while this symbol allows to remain in $q_B'$. Also, as discussed before, transition from $q_B$ to $q_B'$ will occur while possibly going through intermediate states but self-loops are
To this end, we construct a directed graph $\ccalG=\{\ccalV,\ccalE\}$ where $\ccalV$ is the set of nodes defined as $\ccalV=\ccalQ_B^{\text{loop}}$ and $\ccalE\subseteq\ccalV\times\ccalV$ is the set of edges. Specifically, there exists an edge from node $q_B\in\ccalV$ to $q_B'\in\ccalV$ if $\Sigma^{q_B,q_B^{K}}_{\text{dec}}\neq\emptyset$, i.e., if there exists a decomposable transition from $q_B$ to $q_B'$ as per Definition \ref{def:feas}. 

Given the graph $\ccalG$, we define the distance metric
$d:\ccalV\times\ccalV\rightarrow \mathbb{N}$ that returns the minimum number of transitions among states in $\ccalQ_B^{\text{loop}}$ that are required to reach a state $q_B'\in\ccalQ_B^{\text{loop}}$ starting from a state $q_B\in\ccalQ_B^{\text{loop}}$. %This function will be used to guide the robots towards locations in the workspace so that eventually a final DFA state is visited, i.e., the LTL formula is satisfied.
%
Particularly, we define the distance function $d: \ccalQ_B^{\text{loop}} \times \ccalQ_B^{\text{loop}} \rightarrow \mathbb{N}$ as follows
\begin{equation}\label{eq:dist}
d(q_B,q_B')=\left\{
                \begin{array}{ll}
                  |SP_{q_B,q_B'}|, \mbox{if $SP_{q_B,q_B'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_B,q_B'}$ denotes the shortest path (in terms of hops) in $\ccalG$ from $q_B$ to $q_B'$ and $|SP_{q_B,q_B'}|$ stands for its cost (number of hops).%\footnote{In Section \ref{sec:complOpt}, we provide conditions under which if $d(q_D^0,q_F)=\infty$ then the assigned co-safe LTL task is infeasible}. %; see Sections \ref{sec:targetDFA}-\ref{sec:paths}.

Next, we define the final/accepting edges in $\ccalG$.
\begin{definition}[Final/Accepting Edges]\label{def:accEdges}
An edge $(q_B,q_B')\in\ccalE$ is called final or accepting if the corresponding multi-hop NBA transition $\delta_B^K(q_B,\cdot,q_B')$ includes at least one final state $q_F$.
\end{definition}

Based on the definition of accepting edges, we define the set $\ccalQ_{F}^{\text{loop}}\subseteq \ccalQ_{B}^{\text{loop}}$ that collects all states $q_B\in\ccalQ_B^{\text{loop}}$ from which an accepting edge originates, i.e.,
\begin{equation}\label{eq:accNode}
    \ccalQ_{F}^{\text{loop}} = \{q_B\in\ccalQ_B^{\text{loop}}~|~\exists~ \text{accepting edge}~(q_B,q_B')\in\ccalE \}.
\end{equation}
By definition of the accepting condition of the NBA, we have that if at least one of the accepting edges is traversed infinitely often, then the corresponding LTL formula is satisfied. %States $q_B\in\ccalQ_{B}^{\text{loop}}$ for which there are accepting edges $(q_B,q_B')\in\ccalE$ are collected in a set $\ccalQ_{F}^{\text{loop}}$.%, i.e.,





%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}

%\begin{ex}[Feasible DFA transitions]\label{ex:feas}
%(a) Consider the case, where $b^{q_B,q_B}=1$ and $b^{q_B,q_B'}=\pi_j^{r_{m}}$. By definition of $\Sigma^{q_B,q_B}$ and $\Sigma^{q_B,q_B'}$, we have that $\Sigma^{q_B,q_B}=\{\varnothing\}$, where $\varnothing$ stands for the empty symbol, and $\Sigma^{q_B,q_B'} =\{\pi_j^{r_{m}}\}$. Transition from $q_B$ to $q_B'$ is feasible as per Definition \ref{def:feas}. Recall that the sets $\Sigma^{q_B,q_B}, \Sigma^{q_B,q_B'}$ collect symbols that are associated with robots that play a role in satisfying the respective Boolean formulas. This precludes cases where, e.g., a symbol $\pi_j^{r_e}$, $e\neq m$ is included in $\Sigma^{q_B,q_B}$ resulting in erroneously characterizing the transition from $q_D$ to $q_D'$ as infeasible due to condition (iii). 
%%%(b) Consider the following Boolean conditions: $b^{\text{inv}}^{q_D}=b^{\text{inv}}^{q_D'}=\pi_j^{r_i}$ and $b^{\text{next}}^{q_D,q_D'}=\pi_j^{r_i}\wedge \pi_m^{r_h}$. Then the transition from $q_D$ to $q_D'$ is feasible since it satisfies Definition \ref{def:feas}. 
%(b) Consider also the Boolean formulas  $b^{q_B,q_B}=b^{q_B',q_B'}=\pi_j^{r_i}$ and $b^{q_B,q_B'}=\pi_j^{r_e}\wedge \pi_m^{r_h}$, then the transition from $q_B$ to $q_B'$ is infeasible, since it holds that $j\in \ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and, $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. In fact, transition from $q_B$ to $q_B'$ requires robot $j$ to instantaneously move from $r_i$ to $r_e$ which is not possible given that $r_i$ and $r_e$ are disjoint regions. 
%\end{ex}




%\subsection{Selecting a Feasible DFA Final State}\label{sec:feasFinal}
%Given the pruned DFA, the distance function, and an initial DFA state $q_D(0)$, our next step is to select a \textit{feasible} final state $q_{F}\in\ccalQ_F$, i.e., a final state that is reachable from $q_D(0)$ in the pruned DFA [line \ref{rrt:feasFinal}, Alg. \ref{alg:RRT}]. In math, given an initial state  $q_D(0)$ feasible final states are the ones that satisfy  $d(q_D(0),q_{F})\neq \infty$. Among all final states that satisfy this condition, we select one randomly denoted by $q_F^{\text{feas}}$. If there do not exist such final states given the state $q_D(0)$, then we select another initial DFA state $q_D(0)$ from $\ccalQ_D^0$. If there do not exist initial states such that $d(q_D^0,q_{F})\neq \infty$, then the LTL formula can not be satisfied since the in the pruning process, only the DFA transitions that are impossible to enable are removed (i.e., the ones that require the robots to be physically present at more than one region simultaneously) [lines \ref{rrt:unsat1}-\ref{rrt:unsat2}, Alg. \ref{alg:RRT}].
%Next at any time $t\geq 0$, given the current DFA state $q_D(t)$, we select a target DFA state, denoted by $q_D^{\text{next}}$, that the robots should reach next. This state is selected so that it is one hop closer to $q_F^{\text{feas}}$ than $q_D(t)$ is, i.e.,

%\subsection{Selecting the Next NBA State}
%{\bf{Selecting the Next NBA State:}} 

\section{From Feasible Automata to Reactive Planning}\label{sec:planning}

%The pruning process described in Section \ref{sec:prune} occurs offline, i.e., before deploying the robots in the workspace. In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

In this section, we present a distributed reactive algorithm for LTL tasks. The proposed algorithm is summarized in Algorithm \ref{alg:RRT} and requires as input the sets $\ccalQ_{q_B}^{\text{next}}$ and the set of of symbols $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, for all $q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}$ and for all $q_B\in\ccalQ_B^{\text{loop}}$. Recall that $\ccalQ_{q_B}^{\text{next}}$ collects all states, denoted by $q_B^{\text{next}}$, that can reached from $q_B$ in a decomposable fashion, as per Definition \ref{def:feas}, using a symbol selected from $\Sigma_{\text{dec}}^{q_B,qq_B^{\text{next}}}$. These sets are computed offline by Algorithm \ref{alg:prune} described in Section \ref{sec:aut}.

%for all $q_B\in\ccalQ_B^{\text{loop}}$,  In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

\subsection{Distributed Construction of Robot Paths}\label{sec:paths}
Let $q_B(t)\in\ccalQ_B^{\text{loop}}$ be the NBA state that the robots have reached at time $t$ after following paths, denoted by $\bbp_{j,[0:t]}$. Assume also that $L(\bbp(t))\models b^{q_{B(t)},q_{B(t)}}$ i.e., the robots can remain in $q_B(t)$ as long as they remain idle in their current locations.
%
At time $t=0$, $q_B(t)$ is initialized to be the initial/auxiliary state $q_B^{\text{aux}}$, introduced in Section \ref{sec:prune} [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. Recall that $q_B^{\text{aux}}\in\ccalQ_B^{\text{loop}}$ and $L(\bbp(0))\models b^{q_{B(0)},q_{B(0)}}$, by definition of $q_B^{\text{aux}}$. 
%


\begin{algorithm}[t]
%\footnotesize
\caption{LTL Planning in Unknown Occupancy Grid Maps}
\LinesNumbered
\label{alg:RRT}
\KwIn{ (i) initial robot configuration $\bbp(0)$, (ii) Sets $\ccalQ_{q_B}^{\text{next}}$, $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, $\forall q_B\in\ccalQ_{B}^{\text{loop}}$}
%\KwOut{Terminal horizon $H$, and control inputs $\bbu_{0:H}$}
%Convert $\phi$ into a DFA\label{rrt:dfa}\;
%Initial state $\bbq(0)=[\bbp(0), q_D^0]$;\label{rrt:init}
Initialize $t=0$, $q_B(0)=q_B^{\text{aux}}$\;\label{rrt:t0}
%Update current DFA state as $q_D(0)=\delta(q_D^0,L(\bbp(0)))$\;
%Prune DFA\;\label{rrt:prune}
%Select an initial state $q_D(0)=q_D^0$ and a feasible final state $q_F^{\text{feas}}$\;\label{rrt:feasFinal}
%Current DFA state $q_D(t)=q_D^0$\;\label{rrt:init}
%Compute distance from $q_D(t)$ to $q_D^F$\;
%\If{$d(q_D^0, q_F)= \infty$}{\label{rrt:unsat1}
%Error message: \textit{$\phi$ cannot be satisfied (see Proposition \ref{prop:sat})}\;}\label{rrt:unsat2}
Select the next NBA state $q_B^{\text{next}}$ and select $\sigma^{\text{next}}$\;\label{rrt:selTarget}%(see \eqref{eq:targetDFA})
Compute $L_j^{\text{next}}$ and the set of robots $\ccalN^{\text{next}}$\;\label{rrt:goals}
%Initialize $\texttt{updateLoc}=0$ and $\texttt{updateDFA}=0$\;
\While{accepting condition of NBA is not satisfied}{\label{rrt:sat}
%
\For{$j\in\ccalN^{\text{next}}$}{\label{rrt:for1}
Using $\sigma^{\text{next}}$ compute $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$; see \eqref{eq:localProb}\;}\label{rrt:compPaths}
Follow $\bbp_{j,t:T_j}$, re-plan if needed, and update  $M(t)$\;\label{rrt:ExecReplan}%(see Section \ref{sec:exec})
%
\If{$t=T$}{\label{rrt:T}
Update $q_B(t)=q_B^{\text{next}}$\;\label{rrt:updcurDFA}
Select a new NBA state $q_B^{\text{next}}$ and  $\sigma^{\text{next}}$\;\label{rrt:updTarget}
%
Compute new $L_j^{\text{next}}$ and the set of robots $\ccalN^{\text{next}}$\;\label{rrt:UpdGoals}
}
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\normalsize

Given the current NBA state $\bbq_B(t)$, the robots coordinate to select a new NBA state, denoted by $q_B^{\text{next}}$ that they should reach next to make progress towards accomplishing their task [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. This state is selected so that the transition from $q_B$ to $q_B^{\text{next}}$ is decomposable, as per Definition \ref{def:feas}, and progress towards reaching a final state is made. Therefore, the state $q_B^{\text{next}}$ is selected from the set $\ccalQ_{q_B(t)}^{\text{next}}$ based on the following two cases.
%
If $q_B(t)\notin \ccalQ_F^{\text{loop}}$, where $\ccalQ_F^{\text{loop}}$ is defined in \eqref{eq:accNode}, then among all the states in $\ccalQ_{q_B(t)}^{\text{next}}$ we select one that satisfies
%$q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}\subseteq \ccalQ_{B}^{\text{loop}}$

\begin{equation}\label{eq:minDist}
d(q_B^{\text{next}},q_F^{\text{loop}}) =  d(q_B(t),q_F^{\text{loop}})-1,    
\end{equation}
i.e., a state that is one hop closer to a given state $q_F^{\text{loop}}\in\ccalQ_F^{\text{loop}}$ than $q_B(t)$ is. The state $q_F^{\text{loop}}\in\ccalQ_F^{\text{loop}}$ is selected offline and used to guide planning towards traversing accepting edges infinitely often; see Definition \ref{def:accEdges}. Recall that $q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}\subseteq \ccalQ_{B}^{\text{loop}}$ and therefore, $d(q_B^{\text{next}},q_F)$ is well defined; see \eqref{eq:dist}. Under this policy of selecting $q_B^{\text{next}}$, we have that eventually $q_B(t)=q_F$; design of robot paths to ensure this property will be discussed next. If $q_B(t)=q_F^{\text{loop}}$, then the state $q_B^{\text{next}}$ is selected so that $(q_B(t),q_B^{\text{next}})$ is an accepting edge as per Definition \ref{def:accEdges}. This way we ensure that accepting edges are traversed infinitely often and, therefore, the assigned LTL task is satisfied.

%Note that there exists at least one $q_B^{\text{next}}$ that satisfies \eqref{eq:minDist} since any path (including the shortest path) in the pruned NBA that connects $q_B(t)$ to $q_F^{\text{feas}}$ goes through one of the states in $\ccalQ_{q_B(t)}^{\text{next}}$ by construction of the pruned automaton. %and the definition of the distance metric in \eqref{eq:dist}. 
%If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}].

%Given $q_B^{\text{next}}$


%every robot $j$ needs to locally design a path so that a DFA state that is closer to the final state $q_F$ than the current DFA state $q_D(t)$ is eventually reached. 
%The NBA state $q_B^{\text{next}}$ is selected as follows. First, we compute the distance $d(q_B(t),q_F^{\text{feas}})$, where $q_F^{\text{feas}}$ is a final NBA state that is selected offline and is reachable from its initial state $q_B^0$ in the pruned NBA, i.e., $d(q_B^0,q_F^{\text{feas}})\neq\infty$. Then, we select as $q_B^{\text{next}}$ a state that satisfies $d(q_B^{\text{next}},q_F^{\text{feas}}) < d(q_B(t),q_F^{\text{feas}})$,
%\begin{equation}\label{eq:targetDFA}
%   d(q_D^{\text{next}},q_F) = d(q_D(t),q_F) -1, 
%\end{equation}
%i.e., a state that is one hop closer to $q_F^{\text{feas}}$ than $q_B(t)$ is. If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}]. %; see  Sections \ref{sec:paths}. %or realize that a transition from $q_D(t)$ to $q_D^{\text{next}}$ is in fact infeasible; see next section.


%{\bf{Local Construction of Robot Paths:}}

To reach $q_B^{\text{next}}\in\ccalQ_{q_B(t)}^{\text{next}}$ the robots need to eventually generate a symbol from the set $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$; this symbol can be selected randomly. %Among all such symbols $\sigma^{\text{next}}$, we select the one that yields the smallest set $\ccalN^{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
With slight abuse of notation, we denote the selected symbol by $\sigma^{\text{next}}$ [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. Also, for simplicity of notation we replace $b^{q_B(t),q_B^{\text{next}}}$ and $b^{q_B(t),q_B(t)}$ with $b^{\text{next}}$ and $b^{\text{inv}}$. The same notation extends to  the corresponding set of robots $\ccalR^{q_B(t),q_B^{\text{next}}}$, $\ccalN^{q_B(t),q_B^{\text{next}}}$, $\ccalR^{q_B(t),q_B(t)}$, and $\ccalN^{q_B(t),q_B(t)}$.

%with $\ccalR^{\text{next}}$ and $\ccalN^{\text{next}}$.


In what follows, we discuss how to design robot paths $\bbp_{j,t:T_j}$, for all robots $j$, that should be followed within a time interval $[t,T_j]$ to ensure that eventually $\sigma^{\text{next}}$ is generated. Given $\sigma^{\text{next}}$, we compute for each robot $j\in\ccalN^{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma^{\text{next}}$. Recall that for robots $j\in\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma^{\text{next}}$  while for robots $j\in\ccalN^{\text{next}}\setminus\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%
Every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%the state $q_B^{\text{next}}$ will be eventually reached and once $q_B^{\text{next}}$ is reached the robots can remain in $q_B^{\text{next}}$ until new observations are made (i.e., until atomic predicates are satisfied/violated). 
%
%For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b^{\text{inv}}$ and $b^{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.
%
%Given the NBA state $q_B^{\text{next}}$, our goal is to design paths $\bbp_{j,t:T_j}$, for all robots $j$ that should be followed within a time interval $[t,T_j]$ so that the NBA transition from $q_B(t)$ to $q_B^{\text{next}}$ is activated. %%\footnote{With slight abuse of notation the subscript in $\bbp_{j,t:T_j}$ denotes the index of robot and the time interval $[t,T_j]$ within which the path should be followed.} 
%To achieve that, it suffices to ensure that the robots follow paths that (i) satisfy the Boolean formula $b^{q_B(t),q_B(t)}$ that allows them to stay in the current NBA state $q_B(t)$, until (ii) the Boolean formula $b^{q_B(t),q_B^{\text{next}}}$ that enables transition from $q_B(t)$ to $q_B^{\text{next}}$ is satisfied while (iii) while never satisfying Boolean formulas $b^{q_B(t),q_B''}$ other than the ones that are satisfied at time $t$.\footnote{At time $t$, the Boolean formula $b^{q_B(t),q_B(t)}$ is satisfied by construction of the pruned automaton. Nevertheless, other Boolean formulas $b^{q_B(t),q_B''}$ may be satisfied as well due to the non-deterministic nature of the NBA.}  For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b^{\text{inv}}$ and $b^{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.
%
%\red{[add reference to lines of the algorithm]}
%To design paths $\bbp_{j,t:T_j}$, \textit{first} the robots $j\in\ccalN^{\text{next}}$ \textit{communicate} to select a symbol $\sigma^{\text{next}}$ that satisfies conditions (i)-(ii) of Definition \ref{def:feas} given the current symbol  $\sigma^{\text{inv}}=L(\bbp(t))$ they are generating. %; see also Example \ref{ex3}. Note that such a symbol exists by construction of the pruned NBA for any symbol $\sigma^{\text{inv}}$. 
%%% \footnote{Note that it is possible that given the symbol that the robots generated to reach $q_D$ there may not exist a pair of symbols $\sigma^{\text{inv}}$ and $\sigma^{\text{next}}$ to reach a state $q_D^{\text{next}}$ that satisfy condition (iii) of Def. \ref{def:feas}. In other words, transition from $q_D$ to $q_D^{\text{next}}$ may not be cast as a point-to-point navigation problem as in \eqref{eq:localProb}.
%Consider e.g., the DFA that corresponds to $\phi=\square(\pi_1^{r_0}\vee\pi_2^{r_0})\wedge\Diamond(\pi_1^{r_1})\wedge\Diamond(\pi_2^{r_2})$. 
%Existence of such symbols is always guaranteed for a sub-class of co-safe LTL formulas as discussed in Lemma \ref{lem:cnt}.} %that satisfy $b^{\text{inv}}$ and $b^{\text{next}}$, respectively, i.e., $\sigma^{\text{next}}\models b^{\text{next}}$. This pair of symbols is selected so that condition (ii) of Definition \ref{def:feas} is satisfied; 
%Among all such symbols $\sigma^{\text{next}}$, we select the one that yields the smallest set $\ccalN^{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
%
%Given $\sigma^{\text{next}}$, we compute the set $\ccalR^{\text{next}}$ that collect the robots that need to move towards certain regions of interest $r_e$ in workspace to generate $\sigma^{\text{next}}$. 
%
%\textit{Second}, given $\sigma^{\text{next}}$,  we compute for each robot $j\in\ccalN^{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma^{\text{next}}$. Recall that for robots $j\in\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma^{\text{next}}$  while for robots $j\in\ccalN^{\text{next}}\setminus\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%\textit{Third}, we design the paths $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ for all robots $j\in\ccalN^{\text{next}}$. %First, all robots $j\notin\ccalR^{\text{inv}}$ stay put at their current locations until the state $q_B^{\text{next}}$ is reached. %
%\textit{Third}, every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%that if followed the symbol  $\sigma^{\text{next}}\models b^{\text{next}}$ is generated and the DFA state $q_D^{\text{next}}$ is reached
%In Section \ref{sec:complOpt}, we show that the multi-robot state $\bbp(t)$ already generates a symbol that satisfies $b^{\text{inv}}$. We also show that if (i) the robots that are involved in generating $\sigma^{\text{inv}}$, collected in a set $\ccalR^{\text{inv}}$, stay idle at their current locations $\bbp_j(t)$ and (ii) all other robots 
%
%
%\footnotesize
\begin{subequations}
\label{eq:localProb}
\begin{align}
%& \min_{\substack{T_j, \bbu_{j,t:T_j}}} \left[J(T_j,\bbu_{j,t:T_j}) = \int_{t'=t}^{T_j}  w(\bbp_j(t'),\bbu_j(t'))dt \right] \label{ObjLoc2}\\
& \text{Compute:~}{T_j, \bbu_{j,t:T_j}}~\text{such that}  \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ [L(\bbp_j(t'))=L(\bbp_j(t))] \vee [L(\bbp_j(t'))=\varnothing] \nonumber\\
%& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \vee [L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}],~\forall t'\in[t,T_j] \label{constrLoc1} \\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \cup_i\set{r_i}\setminus (R_j^t\cup L_j^{\text{next}}), \forall t'\in[t,T_j] \label{constrLoc1}\\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \hat{O}(t), \forall t'\in[t,T_j] \label{constrLocObs}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j) \in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin \ccalA_j^{\text{avoid}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'+1),\bbu_j(t'+1)), \label{constrLoc3}
\end{align}
\end{subequations}
%\normalsize

\noindent In \eqref{constrLoc1}, $R_j^t$ denotes the region that robot $j$ lies in at time $t$. The first constraint \eqref{constrLoc1} requires that robot $j$ should not visit any region $r_i$ excluding $R_j^t$ and the target region $L_j^{\text{next}}$, for all $t'\in[t,T_j]$. If at time $t$ robot $j$ does not lie in any of the regions $r_i$, then $R_j^t=\emptyset$. This ensures that the multi-robot system can always remain in $q_B(t)$ as the robots $j\in\ccalN^{\text{next}}$ navigate the workspace; see Lemma \ref{lem:binv}. This constraint can be relaxed by requiring  robot $j\in\ccalN^{\text{next}}$ to always avoid only regions that may result in violating $b^{\text{inv}}$. For instance, if $b^{\text{next}}=\neg(\pi_j^{r_e}\wedge\pi_i^{r_e}$), then it suffices to require robot $j$ to never visit $r_e$.  %\footnote{$T_j^{-}$ denotes a time instant right before $T_j$, i.e., $T_j^{-}=T_j-\epsilon$, for an arbitrarily small $\epsilon>0$.} 
Similarly, the second constraint in \eqref{constrLocObs} requires robot $j$ to avoid all obstacles, collected in $\hat{O}(t)$, that are known up to the time instant $t$. The third constraint in \eqref{constrLoc2} requires robot $j$ to be in region $L_j^{\text{next}}$ at a time instant $T_j\geq t$. %so that it generates $L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}$.%\footnote{Note that this prevents the robot from visiting parts of $L_j^{\text{next}}$ that are shared with other regions $r_i$.} 
This is required to eventually generate the symbol $\sigma^{\text{next}}$. The last constraint in \eqref{constrLoc3} captures the robot dynamics. Note that among all paths that satisfy these constraints, the optimal one, as a per a user-specified motion cost function, can be selected. 
%\textit{Third}, every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%In words, the optimal control problem \eqref{eq:localProb} requires robot $j$ to design a path $\bbp_{j,t:T_j}$ that reaches $L_j^{\text{next}}$ (see \eqref{constrLoc2}) while avoiding certain regions $r_i$ (see \eqref{constrLoc1}) and all detected obstacles denoted by $\hat{O}(t)$ (see \eqref{constrLocObs}). %Note that the robots that do not belong to $\ccalR^{\text{inv}}$ and also are not responsible to generate $\sigma^{\text{next}}$ do not have a target region $L_{j}^{\text{next}}$. These robots remain stationary in their current locations and they do not need to solve \eqref{eq:localProb}.
%
Observe that \eqref{eq:localProb} is a  point-to-point navigation problem, and, therefore, any of the traditional motion planning algorithms, such as $\text{A}^*$, RRT, $\text{RRT}^*$, RRG, or PRM, can be used to solve it \cite{karaman2011sampling}. Finally observe that given $L_j^{\text{next}}$, robot $j$ locally solves \eqref{eq:localProb} without communicating with any other robot. %Also, since the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable as per Definition \ref{def:feas}, there are no conflicts where a robot would have to stay idle at its current location and at the same time move towards a new location as per the solution to \eqref{eq:localProb}; see also Lemma \ref{lem:binv}. %there is no robot $j$ that belongs to $\ccalR^{\text{inv}}$ that is required to stay idle
%
%Correctness of Alg. \ref{alg:RRT} is discussed in Sec. \ref{sec:complOpt}. %Feasibility of such this problem is examined in 

%We design such paths in two stages. In the first stage, we design subpaths $\bbp_{j,t:\bar{T}_j}$ for some $t<\bar{T}_j<T$ and in the second stage we design paths $\bbp_{j,\bar{T}_j:T_j}$. In particular, \textit{in the first stage} all robots that are involved in generating $\sigma^{\text{inv}}$, collected in a set $\ccalR^{\text{inv}}$, and all other robots $j$ for which it hold $L(\bbp_j(t))=\varnothing$ (i.e., they are outside of all regions $r_i$) stay idle at their current locations $\bbp_j(t)$, i.e., $\bar{T}_j=t+1$ and $\bbp_{j,t:\bar{T}_j}=[\bbp_j(t),\bbp_j(t)]$ All other robots $j$ (i.e., the ones that satisfy $j\notin\ccalR^{\text{inv}}$ and $L(\bbp_j(t))\neq \varnothing$) solve the following optimal control problem to design paths $\bbp_{j,t:\bar{T}_j}$ that if followed then the robots will move outside the regions that they are currently located. %As it will bbe discusses in Section \ref{sec:exec}, these subpaths will be executed so that the robots will move outside their current regions simultaneously.

%\begin{subequations}
%\label{eq:localProb1}
%\begin{align}
%& \min_{\substack{\bar{T}_j, \bbu_{t:\bar{T}_j}}} \left[J(\bar{T}_j,\bbu_{t:\bar{T}_j}) = \sum_{t'=t}^{\bar{T}_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc1}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in R_j(t), \forall t\in\set{t,\dots,\bar{T}_j-1} \label{constrLoc1a} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in \ccalR_j^{\text{inv}}, \forall t\in\set{t,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(\bar{T}_j))=\varnothing \label{constrLoc2a}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   %\bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc2}
%\end{align}
%\end{subequations}
%where $R_j(t)$ denotes the region $r_i$ that robot $j$ lies in at time $t$. Observe that the first two constraints \eqref{constrLoc1a}-\eqref{constrLoc2a} require robot $j$ to move outside the region $\ccalR_j(t)$ where it is located at the time instant $t$. This happens at a time instant $\bar{T}_j$, i.e., $L(\bbp_j(\bar{T}_j))=\varnothing$. Note that robot $j$ locally solves \label{eq:localProb1} with communicating with other robots. Observe that execution of these subpaths ensures that the robots remain in the DFA state $q_D(t)$ since $b^{\text{inv}}$ is always satisfied as the robots $\ccalR^{\text{inv}}$ remain stationary in their current locations that generates  $\sigma^{\text{inv}}\models b^{\text{inv}}$.

%since the robots in $\ccalR^{\text{inv}}$

%In the \textit{second} stage, we construct the subpaths $\bbp_{j,\bar{T}_j:T_j}$ that will enable the transition from $q_D(t)$ to $q_D^{\text{next}}$. For robots $j\in\ccalR^{\text{inv}}$, we select $T_j=\bar{T}_j+1$ and $\bbp_{j,\bar{T}_j:T_j}=[\bbp_{j}(t),\bbp_{j}(t)]$, i.e., these robots still stay idle. In fact, due to the deterministic structure of the DFA, this ensures that the robots remain in the DFA state $q_D(t)$ until the symbol $\sigma^{\text{next}}$ is generated which will activate the transition towards $q_D^{\text{next}}$. To generate the symbol  $\sigma^{\text{next}}$, all other robots $j\notin\ccalR^{\text{inv}}$ design paths $\bbp_{j,\bar{T}_j:T_j}$ by solving the following optimal control problem:

%\begin{subequations}
%\label{eq:localProb}
%\begin{align}
%& \min_{\substack{T_j, \bbu_{\bar{T}_j:T_j}}} \left[J(T_j,\bbu_{\bar{T}_j:T_j}) = \sum_{t'=\bar{T}_j}^{T_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ L(\bbp_j(t'))=\varnothing, \forall t'\in\set{\bar{T}_j,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
%\end{align}
%\end{subequations}



 %This ensures that  transition to a DFA state $q_D'\neq q_D(t)$ that is not $q_D^{\text{next}}$. 
%In the meantime the robots in $\ccalR^{\text{inv}}$ ensure that the current DFA state remain the same in $[t,\bar{T}-1]$, since they stay idle and generate the symbol $\sigma^{\text{inv}}$. Also note that robots in $\ccalR^{\text{inv}}$ do not belong to the set of robots that need to move to another location to generate the symbol $\sigma$, since that would create a conflict; see also Remark \ref{rem:invariant}. 
%The second constraint in \eqref{constrLoc2} requires that at time instant $T_j$, all robots should be in their corresponding locations $L_j^\textbf{}$. Once this happens the symbol $\sigma^{\text{next}}$ is generated and the target DFA state is reached.
%
%Note that infeasibility of \eqref{eq:localProb} is due to the facts (i) the environment is unknown and, therefore, it is not possible to check offline which DFA transitions cannot be enabled because e.g., of the robot dynamics or the existence of obstacles.%; and (ii) the LTL formula $\phi$ is decomposed into local sub-tasks Problem \ref{prob} is solved in a distributed the proposed algorithm is distributed nature of the proposed 

%What if the problem is infeasible? update $\sigma$ i.e., $L_j$. If no other $L_j$. update target DFA state. If no other target DFA state report `current method failed (this does not mean that the task is unsatisfiable though)'

%\begin{ex}[Selection of $\sigma^{\text{next}}$ and $\sigma^{\text{inv}}$]\label{ex3}
%Consider the Boolean formulas $b^{\text{inv}}=\neg \pi_{\text{obs}}$ and $b^{\text{next}}=(\pi_j^{r_1}\vee \pi_j^{r_3} )\wedge\pi_e^{r_2}\wedge (\neg \pi_j^{r_2}) \wedge (\neg (\pi_j^{r_1}\wedge \pi_e^{r_1}))$, where the atomic predicate $\pi_{\text{obs}}$ is true of at least one robot hits an obstacle. A symbol $\sigma^{\text{next}}$ that satisfies $b^{\text{next}}$ is $\sigma^{\text{next}}=\pi_j^{r_1}\pi_e^{r_2}$ while $b^{\text{inv}}$ is satisfied by an empty string, i.e., $\sigma^{\text{inv}}=\varnothing$. Given this pair of symbols, we have that $\ccalR^{\text{inv}}=\emptyset$, $\ccalR^{\text{next}}=\set{j,e}$, $L_j^{\text{next}}=r_1$, and $L_e^{\text{next}}=r_2$.
%\end{ex}

%\begin{ex}[Construction of $\sigma^{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b^{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$. Then, we have that $\sigma^{\text{inv}}=\pi_j^{r_1}$ and $\ccalR^{\text{inv}}=\set{j}$. Similarly, if $b^{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma^{\text{inv}}$ is an empty string and $\ccalR^{\text{inv}}=\emptyset$.
%\end{ex}

%\begin{ex}
%--add automaton figure--and explain--
%\end{ex}
%\begin{rem}[Initialization of $q_B(t)$]
%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}
%\end{rem}
\subsection{Reacting to Map Uncertainty}\label{sec:exec}
%{\bf{Reactive Planning to Map Uncertainty:}}

As the robots follow their paths $\bbp_{j,t:T_j}$, the map $M(t)$ is continuously updated, as per \eqref{eq:updMap}, and the robot paths need to be accordingly revised [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. In fact, reactivity to the environment is required in two cases. First, as the robots follow their paths $\bbp_{j,t:T_j}$, they may discover new obstacles based on their sensor measurements; see \eqref{eq:sensor}. If the discovered obstacles intersect with their paths $\bbp_{j,t:T_j}$, for some $j\in\ccalR^{\text{next}}$, then these robots $j$ locally re-solve \eqref{eq:localProb} using the updated map to design new paths. Note that existing reactive planning algorithms that can address reachability navigation problems in the presence of unknown obstacles can also be used to solve \eqref{eq:localProb}; see e.g., \cite{guzzi2013human,vasilopoulos2018sensor,bansal2019combining,ryll2019efficient}.

%is not reachable e.g., due to the robot dynamics or 
Second, as the the map $M(t)$ is constructed, goal regions $L_j^{\text{next}}$ may become unreachable because of the structure of the environment (e.g., regions of interest may be surrounded by obstacles). In this case, robots $j$ that cannot reach $L_j^{\text{next}}$ communicate with all other robots so that a new symbol $\sigma^{\text{next}}$ is selected. This process is repeated until a reachable region $L_j^{\text{next}}$ is selected.  %that makes \eqref{eq:localProb} feasible. 
If such a symbol $\sigma^{\text{next}}$ does not exist, then this means that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$, due to the a-priori unknown structure of the environment. Then, the pruned NBA is updated by removing this transition and a new NBA state $q_B^{\text{next}}$ is selected. If there do not exist any candidate NBA states to be selected as $q_B^{\text{next}}$, then the assigned task cannot be accomplished given the current multi-robot and NBA state. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
In fact, there may exist another sequence of NBA states for which Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible (i.e., paths towards selected goal regions always exist) and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.

%\begin{rem}[Feasibility of \eqref{eq:localProb}]
%Observe that \eqref{eq:localProb} may be \textit{infeasible}. This can be the case e.g., if the region $L_j^{\text{next}}$ is not reachable e.g., due to the robot dynamics or the structure of the environment. In this case, robot $j$ needs to communicate with all other robots so that a new symbol $\sigma^{\text{next}}$ is selected. This process is repeated until regions $L_j^{\text{next}}$ are selected that make \eqref{eq:localProb} feasible. If such a symbol $\sigma^{\text{next}}$ does not exist, then this means that the transition from $q_D(t)$ to $q_D^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$. Then, the pruned DFA is updated by removing this transition. Next, a new target DFA state is selected that is closer to the final state $q_F$ than $q_D(t)$ is. If there do not exist such DFA states then the robots cannot accomplish the assigned task. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
%In fact, there may exist another sequence of DFA states for which  Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
%Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.
%\end{rem}

%{\bf{Asynchronous Execution of Paths:}} 
\subsection{Asynchronous Execution of Paths}
The robots $j\in\ccalR^{\text{next}}$ execute their paths $\bbp_{j,t:T_j}$ \textit{asynchronously} until the time instant $T_j$, i.e., until they reach their respective target regions $L_j^{\text{next}}$ [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. At time $T_j$, robot $j$ waits for all other robots $e\in\ccalR^{\text{next}}$ with $T_e>T_j$. At time instant $T=\max_{j\in\ccalN^{\text{next}}}\{T_j\}$, i.e., when \textit{all} robots $j\in\ccalN^{\text{next}}$ have reached their respective regions $L_j^{\text{next}}$, the symbol $\sigma^{\text{next}}$ is generated. Then, the multi-robot system reaches the NBA state $q_B^{\text{next}}$ and a new NBA state is selected [lines \ref{rrt:T}-\ref{rrt:UpdGoals}, Alg. \ref{alg:RRT}]. This process is repeated indefinitely so that a final state is reached infinitely often [line \ref{rrt:sat}, Alg. \ref{alg:RRT}].
%In Section \ref{sec:complOpt}, we show the robots remain in the NBA state $q_B(t)$ for all  $t'\in [t, T-1]$ and transition to $q_B^{\text{next}}$ occurs at the time instant $T$. Once this happens, the robots update their current DFA state and select the next DFA state [lines \ref{rrt:T}-\ref{rrt:UpdGoals}]. This process is repeated until the final state $q_F$ is reached.

%
%\begin{rem}\label{rem:invariant}
%Note that once the robots reach a new DFA $q_D$, they satisfy its respective Boolean condition $b^{\text{inv}}$, since the `next' temporal operator is excluded from the task specification. Particularly, if $b^{\text{inv}}$ is not satisfied this implies that once the robots are at locations that generate a symbol that triggers the transition to $q_D$, the robots should immediately leave their locations, which is impossible to specify unless the next operator is included in the specification language. 

%Recall that $\sigma^{\text{inv}}$ is selected to have the minimum length, this means that the minimum number of robots are involved to generate it. Therefore, robots that are required to generate the symbol $\sigma$ are not included in the set $\ccalR^{\text{inv}}$; see also Remark \ref{rem:invariant}.
%Similarly, robots that are responsible to satisfy $b^{\text{next}}$ cannot be responsible for generating the symbol $\sigma^{\text{inv}}$, since the next operator does not exist and all regions are assumed to be disjoint. %(unless there is an overlap..)
%\end{rem}


%\subsection{Online Re-planning}\label{sec:replan}






\begin{rem}[Communication]
%Note that Algorithm \ref{alg:RRT} requires all-time communication to ensure that all robots always have access to the same map $M(t)$. Nevertheless, this requirement can be straightforwardly relaxed by allowing each robot to build their local map $M_j(t)$. Moreover, 
Execution of the paths $\bbp_{j,t:T_j}$ does not require all-time communication among robots, which is typically the case in relevant temporal logic algorithms. Instead, communication is intermittent and is required only in the following two cases: (i) all robots need to communicate with each other to select and update the symbol $\sigma^{\text{next}}$ (ii) every robot $j\in\ccalR^{\text{next}}$ needs to send a message to all other robots in $\ccalR^{\text{next}}$ once it has reached region $L_{j}^{\text{next}}$. %; see Section \ref{sec:exec}.
\end{rem}

%Next, we define the set $\ccalL_j$ that collects all robot positions $\bbp_j$ that violate $b^{\text{inv}}$ regardless of the state of all other robots. For instance, if $b^{\text{inv}}=\neg (\pi_j^{r_e}\wedge \pi_z^{r_h})$, then $\ccalL_j=\emptyset$. On the other hand, if $b^{\text{inv}}=\neg (\pi_j^{r_e})\wedge (\neg \pi_z^{r_h})$ then  $\ccalL_j=\set{r_e}$. Formally, to construct the set, we express the negation of $b^{\text{inv}}$, denoted by $\bar{b}^{\text{inv}}=\neg b^{\text{inv}}$ as




==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/alg_final.tex <==




%ASSUMPTIONS

%Disjoint regions? no reachable regions? not in the PF but possibly needed to ensure completeness separable regions? only for completeness


%%%%%%%%







%%%%%%%%%


%\subsection{Planning for Information Acquisition}
%\red{(we need figures)}

Problem \ref{prob} can be solved by applying existing abstraction-free approaches for LTL planning, e.g., \cite{vasile2013sampling,luo2019abstraction}, at runtime to continuously update the robot paths as the map of the environment is continuously learned. Nevertheless, such methods require searching over a large product automaton space, a task that is computationally challenging to perform at runtime. To mitigate this challenge, we propose a new reactive LTL planning algorithm summarized in Algorithm \ref{alg:RRT} that does not rely on searching over a product automaton space. The main idea of Algorithm \ref{alg:RRT} is to decompose the temporal logic task into a sequence of local point-to-point navigation problems that are formulated and solved online while adapting to the updated map $M(t)$ of the environment.
%

\subsection{From LTL formulas to Automata}



To this end, first, we translate the specification $\phi$, constructed using a set of atomic predicates $\mathcal{AP}$, into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA), defined as follows \cite{baier2008principles} [line \ref{rrt:dfa}, Alg. \ref{alg:RRT}]. %Given a temporal logic formula $\phi$ , with syntax and semantics as described in Definitions \ref{syntax} and \ref{semantics}, respectively, a DFA is defined as follows:

\begin{definition}[NBA]
A Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\rightarrow_B, \ccalQ_F\right)$, where (i) $\ccalQ_{B}$ is the set of states;
(ii) $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is the initial state; (iii) $\rightarrow_B:\ccalQ_B\times\Sigma\rightarrow\ccalQ_B$ is a non-deterministic transition relation, and $\ccalQ_F\subseteq\ccalQ_{B}$ is a set of accepting/final state. 
\end{definition}

To interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times M(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current multi-robot state $\bbp(t)\in\mathbb{R}^{n\times N}$ and the current map $M(t)$ of the environment. An infinite-length discrete plan $\tau=\bbp(0)\bbp(1)\dots$ satisfies $\phi$, denoted by $\tau\models\phi$, if the word $\sigma=L(\bbp(0), M(0))L(\bbp(1),M(1))\dots$ yields an accepting NBA run defined as follows.\footnote{Hereafter, for simplicity we denote $L(\bbp(t),M(t))$ by $L(\bbp(t))$.} First, a run of $\rho_B$ of $B$ over an infinite word $\sigma=\sigma(1)\sigma(2)\dots\sigma(t)\dots\in(2^{\mathcal{AP}})^{\omega}$, is a sequence $\rho_B=q_B(0)q_B(1)q_B(2)\dots,q_B(t),\dots$, where $q_B(0)\in\ccalQ_B^0$ and $(q_B(t),\sigma(t),q_B(t+1)\in\rightarrow_B$, $\forall t\in\mathbb{N}$. Hereafter, we equivalently denote $(q_B(t),\sigma(t),q_B(t+1)\in\rightarrow_B$ as $q_B(t)\rightarrow_B q_B(t+1)$. A run $\rho_B$ is called \textit{accepting} if $\texttt{Inf}(\rho_B)\cap\ccalQ_F\neq\emptyset$, where $\texttt{Inf}(\rho_B)$ represents the set of states that appear infinitely often in $\rho_B$. In words, an infinite-length discrete plan $\tau$ satisfies an LTL formula $\phi$ if its corresponding NBA run visits at least one of the final states infinitely often.
%The symbols $\sigma$ that result in an accepting run of $D$ constitute the accepted language of $D$.

%The proposed reactive algorithm builds online (i.e., as the robots navigate the environment) paths that live in the infinite-dimensional space $\Omega^N\times\ccalQ_D$. The synthesized paths are updated as the map of the environment is updated. 
Next, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task; see Algorithm \ref{alg:RRT}. %Specifically, let $q_B(t)\in\ccalQ_B$ denote the NBA state that the multi-robot system has reached at time $t$ given all observations that have been made (i.e., all atomic predicates that have been satisfied) until $t$, where $q_B(0)\in\ccalQ_B^0$ [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. 
Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task.
%eventually visit a new NBA state, denoted by $q_B^{\text{next}}$, i.e., they make progress towards accomplishing the assigned task. 
To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that it is (i) one-hop reachable from $q_B(t)$, (ii) `closer' to the final states than $q_B(t)$ is according to a distance function defined over the NBA, and (iii) observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously. Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. In what follows, we describe these steps in detail.%Once this transition is enabled, the robots update the target DFA state $q_D^{\text{next}}$ until they reach a final DFA state.%\footnote{In case the DFA has more than one initial state, then there is more than one state $\bbq(0)$ that can be used as a root. In this case, a separate tree is build for each one of possible roots.}
%For this, we assume that the initial robot configuration allows the robots to stay in $q_B(0)$.
%

%By convention the cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = 0$, while the cost of a node $\bbq(t+1)=[\bbp(t+1), q_D]\in\ccalV$, given its parent node $\bbq(t)=[\bbp(t),q_D']\in\ccalV$, is computed as 
%\begin{equation}\label{eq:costUpd}
%J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq(t)) +  w(\bbp(t),\bbp(t+1)).
%\end{equation}
%Observe that by applying \eqref{eq:costUpd} recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:Prob2}.

 
%Given the current DFA state $q_D(t)$, the robots first select a DFA state $q_D^{\text{next}}\in\ccalQ_D$ that is `closer' to the final state $q_F$ than $q_D(t)$ is and observations that generate a transition from $q_D(t)$ to $q_D^{\text{next}}$ can be generated. Therefore,
%\subsection{Selecting the Next DFA State}\label{sec:targetDFA}

%{\bf{Pruning the DFA:}}
\subsection{Pruning the NBA}\label{sec:prune}
Given the current NBA state $q_B(t)$, a new state $q_B^{\text{next}}$ is selected so that it is closer to the final states. Thus, to select $q_B^{\text{next}}$, we need to define a distance function over the state-space of the NBA that measures how far each state is from the final state. %(in terms of the number feasible transitions/hops required to reach $q_F$). 
To achieve that, we first prune the NBA $B$ by removing transitions that cannot be enabled [line \ref{rrt:prune}, Alg. \ref{alg:RRT}]. %This is required to define a distance function over the state-space of the DFA. %
%
Specifically, the pruned NBA is constructed by removing all infeasible NBA transitions. To formally define the \textit{feasible/infeasible} DFA transitions we first need to introduce the following definitions. %\cite{kantaros2018text}.
%
%We also rewrite $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$ as follows:
%\begin{equation}\label{eq:eq1}
%    b_{\text{inv}}^{q_D} = b_{\text{inv}}^{\text{goal}} \triangle (\neg b_{\text{inv}}^{\text{avoid}} ),
%\end{equation}

%\begin{equation}\label{eq:eq2}
%    b_{\text{next}}^{q_D,q_D'} = b_{\text{next}}^{\text{goal}} \triangle (\neg b_{\text{next}}^{\text{avoid}} ),
%\end{equation}
%where in the Boolean formulas  $b_{\text{next}}^{\text{goal}}$, $b_{\text{next}}^{\text{avoid}}$, $b_{\text{inv}}^{\text{goal}}$ and $b_{\text{inv}}^{\text{avoid}}$ the negation operator does not appear in front of any atomic proposition. Also, in \eqref{eq:eq1} and \eqref{eq:eq2}, $\triangle$ denotes either the logical AND ($\wedge$) or the logical OR $(\vee)$ operator.

% defined in \ref{defn:wTS}.%\footnote{Recall from Definition \ref{defn:wTS} that $\text{wTS}_i$ is defined over $\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma_i=2^{\mathcal{AP}_i}$. Also, recall from Definition \ref{def:pts} that the PTS is defined over $\mathcal{AP}=\bigcup_{i=1}^N\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma=2^{\mathcal{AP}}$. Also, throughout the paper, we denote the finite symbols by $\sigma^*\in\Sigma$ and the infinite symbols by $\sigma\in\Sigma^{\omega}$.}
\begin{definition}[Feasible symbols $\sigma_j\in\Sigma_j$]\label{defn:infTSi}
A symbol $\sigma_j\in\Sigma_j:=2^{\mathcal{AP}_j}$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, where $b_j^{\text{inf}}$ is a Boolean formula defined as 
\begin{equation}\label{bInfTSi}
b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e}(\pi_j^{r_i}\wedge\pi_j^{r_e})).
%b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e})),
\end{equation}
where $b_j^{\text{inf}}$ requires robot $j$ to be present simultaneously in more than one disjoint region.
\end{definition}

%We also need to define when a symbol $\sigma\in\Sigma$ is \textit{feasible}, i.e., when it can be generated by the multi-robot system. To this end, we first need to define the
%In other symbols $\sigma_j\in\Sigma_j=2^{\mathcal{AP}_j}$ that are feasible, i.e, the symbols that can be generated by robot $j$ \cite{kantaros2018text}. 


Note that the Boolean formula $b_j^{\text{inf}}$ is satisfied by any finite symbol $\sigma_j\in\Sigma_j$ that requires robot $j$ to be present in two or more disjoint regions, simultaneously. For instance, the symbol $\sigma_j=\pi_j^{r_i}\pi_j^{r_e}$ satisfies $b_j^{\text{inf}}$ if $r_i$ and $r_e$ are disjoint regions. %\footnote{Note that if we consider regions $r_i$ that are not necessarily disjoint, then the Boolean formula $b_j^{\text{inf}}$ is defined as $b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e}))$. Note also that definition of infeasible symbols depends on the problem at hand, i.e, the definition of atomic propositions included in the sets $\mathcal{AP}_j$.} % if there is an overlap between regions $r_i$ and $r_e$. 
Next, we define the feasible symbols $\sigma\in\Sigma$.

\begin{definition}[Feasible symbols $\sigma\in\Sigma$]\label{defn:infPTS}
A symbol $\sigma\in\Sigma$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, for all robots $j$,
where $\sigma_j=\Pi|_{\Sigma_j}\sigma$, $b_j^{\text{inf}}$ is defined in \eqref{bInfTSi}, and $\Pi|_{\Sigma_j}\sigma$ stands for the projection of the symbol $\sigma$ onto $\Sigma_j$.\footnote{For instance, $\Pi|_{\Sigma_j}(\pi_j^{r_e}\pi_m^{r_h})=\pi_j^{r_e}$.} We denote by $\Sigma_{\text{feas}}\subseteq\Sigma$ the set of all feasible symbols $\sigma\in\Sigma$. 
\end{definition}


%%%
%%%
%Next, we define the $\Sigma(q_D)=\{s\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D)\in\rightarrow_D)\}$ that collects all symbols that the robots can generate to remain in the state $q_D$. We also define the set $\Sigma(q_D,q_D')=\{\sigma\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D')\in\rightarrow_D)\}$ that collects all symbols that enable a transition from $q_D$ to $q_D'$.
%
%Moreover, for each state $q_D$, we define the set $\Sigma(q_D|p)$ that collects all symbols $\sigma$ that robots may observe if they reach $q_D$ through a path $p=q_D^0,\dots,q_D$, i.e., a sequence of states in $\ccalQ_D$ that starts at the initial state $q_D^0$ and ends at the state $q_D$. Note that there may be multiple paths that can reach $q_D$ from $q_D^0$ and, therefore, each state $q_D$ may be associated with more than one set $\Sigma(q_D|p)$. For the initial state, $q_D^0$, there is only one such set  defined as $\Sigma(q_D^0|p)=\Sigma(q_D^0)$, since in a DFA the only path $p$ to reach $q_D^0$ from $q_D^0$ is the self-loop of $q_D^0$.

%To prune the DFA we need first to construct the sets $\Sigma(q_D|p)$. Starting from $q_D^{0}$, we execute the following process for each state $q_D$ that is reachable within one hop from $q_D^0$

%First, we select a state $q_D\in\ccalQ_D$, for which all corresponding sets $\Sigma(q_D|p)$ have been constructed
%%%
%%%
%\red{unclear here..}
%To solve Problem \ref{prob}, we first decompose the assigned task into local point-to-point planning problems. Motion plans that solve these point-to-point navigation problems are locally designed online while adapting to the map of the environment that is built by the robots. The proposed algorithm is summarized in Algorithm \ref{alg:RRT}. 
%


\begin{algorithm}[t]
%\footnotesize
\caption{Pruning a NBA}
\LinesNumbered
\label{alg:prune}
\KwIn{NBA}
\KwOut{Pruned NBA}
Remove transitions that are activated only by infeasible symbols (see Definition \ref{defn:infPTS})\label{prune:inf}\;
Collect all states $q_B\in\ccalQ_B$ for which a self-loop does not exist in the set $\hat{\ccalQ}_B$\label{prune:noloop}\;
Collect in a set $\ccalP_{q_B}=\{[(q_B^{\text{in},n},q_B),(q_B,q_B^{\text{out},m})]\}_{n=1,m=1}^{n=\bar{n},m=\bar{m}}$ \;%all possible pairs of incoming and outgoing transitions associated with
\For{$q_B\in\ccalQ_B$}{\label{prune:for1}
    \For{each pair in $\ccalP_{q_B}$}{
    Replicate $q_B$ so that its copy has only one incoming and only one outgoing transition as per the selected pair of edges\;\label{prune:repl}
    Remove the pair of edges from $\ccalP_{q_B}$\;\label{prune:rem}} 
}
\For {$q_B\in\ccalQ_B$ with $\Sigma^{q_B,q_B}\neq\emptyset$}{
Apply Definition \ref{def:feas}
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\begin{algorithm}[t]
%\footnotesize
\caption{LTL Planning in Unknown Environments}
\LinesNumbered
\label{alg:RRT}
\KwIn{ (i) initial robot configuration $\bbp(0)\models b^{q_B^0,q_B^0}$, (ii) LTL formula $\phi$}
%\KwOut{Terminal horizon $H$, and control inputs $\bbu_{0:H}$}
Convert $\phi$ into a DFA\label{rrt:dfa}\;
%Initial state $\bbq(0)=[\bbp(0), q_D^0]$;\label{rrt:init}
Initialize $t=0$, $q_D(0)=q_D^0$\;\label{rrt:t0}
%Update current DFA state as $q_D(0)=\delta(q_D^0,L(\bbp(0)))$\;
Prune DFA\;\label{rrt:prune}
%Select an initial state $q_D(0)=q_D^0$ and a feasible final state $q_F^{\text{feas}}$\;\label{rrt:feasFinal}
%Current DFA state $q_D(t)=q_D^0$\;\label{rrt:init}
%Compute distance from $q_D(t)$ to $q_D^F$\;
%\If{$d(q_D^0, q_F)= \infty$}{\label{rrt:unsat1}
%Error message: \textit{$\phi$ cannot be satisfied (see Proposition \ref{prop:sat})}\;}\label{rrt:unsat2}
Select the next DFA state $q_D^{\text{next}}$ that should be reached\;\label{rrt:selTarget}%(see \eqref{eq:targetDFA})
Compute $L_j^{\text{next}}$ and the set of robots $\ccalR_{\text{next}}$\;\label{rrt:goals}
%Initialize $\texttt{updateLoc}=0$ and $\texttt{updateDFA}=0$\;
\While{$q_B(t)\neq q_F$}{
%
\For{$j\in\ccalR_{\text{next}}$}{\label{rrt:for1}
Compute $\bbp_{j,t:T_j}$ as per \eqref{eq:localProb}\;}\label{rrt:compPaths}
Execute paths $\bbp_{j,t:T_j}$, re-plan if needed, and update map $M(t)$\;\label{rrt:ExecReplan}%(see Section \ref{sec:exec})
%
\If{$t=T$}{\label{rrt:T}
Update $q_D(t)=q_D^{\text{next}}$\;\label{rrt:updcurDFA}
Select a new DFA state $q_D^{\text{next}}$\;\label{rrt:updTarget}
%
Compute new $L_j^{\text{next}}$ and the set of robots $\ccalR_{\text{next}}$\;\label{rrt:UpdGoals}
}
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\normalsize


Next, we define the sets that collect all feasible symbols that enable a transition from an NBA state $q_B$ to another, not necessarily different, NBA state $q_B'$. This definition relies on the fact that transitions among automaton states are enabled if Boolean formulas, denoted by $b^{q_B,q_B'}$ and defined over the set of atomic predicates $\mathcal{AP}$, are satisfied.  %The set of all atomic predicates associated with robots $j\in\mathcal{N}_{q_B,q_B'}$ is defined by $\mathcal{AP}_{q_B,q_B'}=\bigcup_{j\in\mathcal{N}_{q_B,q_B'}}\mathcal{AP}_j$.

\begin{definition}[Sets of Feasible Symbols]
Let $\mathcal{AP}_{q_B,q_B'}$ be a set that collects all atomic predicates that appear in the Boolean formula $b^{q_B,q_B'}$ associated with an NBA transition $q_B\rightarrow q_B'$. Given $b^{q_B,q_B'}$, we define the set $\Sigma^{q_B,q_B'}\subseteq 2^{\mathcal{AP}_{q_B,q_B'}}$ 
that collects all symbols $\sigma$ that (i) satisfy the corresponding Boolean formula $b^{q_B,q_B'}$, i.e., $\sigma\models b^{q_B,q_B'}$; and (ii) $\sigma\in\Sigma_{\text{feas}}$. %; and (iii) are associated with robots that appear in $b^{q_B,q_B'}$. 
%If the empty symbol $\varnothing$ satisfies (i), then $\Sigma^{q_B,q_B'}=\set{\varnothing}$. 
%The set $\mathcal{AP}_{q_B,q_B'}$ collects all atomic predicates that appear in $b^{q_B,q_B'}$.
\label{defn:feasSet}
\end{definition}

%Moreover, let $b_{\text{inv}}^{q_D}$ denote the Boolean formula that needs to be satisfied to enable a loop around $q_D$, i.e., a transition from $q_D$ to $q_D$.\footnote{Note that $b_{\text{inv}}^{q_D}$ exists for all states $q_D$, since the `next' operator is excluded from the syntax. Also, the Boolean formulas that should be satisfied to enable a  transition from a state $q_D$ to $q_D'$ can be provided by tools that convert temporal logic formulas to automata.} Let also $\Sigma_{\text{inv}}^{q_D}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b_{\text{inv}}^{q_D}$. 
%
%Let also $b_{\text{next}}^{q_D,q_D'}$ denote the Boolean formula that needs to be satisfied to enable a transition from $q_D$ to $q_D'$ and $\Sigma_{\text{next}}^{q_D,q_D'}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b_{\text{next}}^{q_D,q_D'}$.
%Also, from $\Sigma_{\text{text}}^{q_D,q_D'}$, we exclude symbols associated with robots that do not play any role in satisfying $b_{\text{next}}^{q_D,q_D'}$. For instance, if $b_{\text{next}}^{q_D,q_D'}=\pi_j^{r_e}\vee\pi_j^{r_m}$, then $\Sigma_{\text{text}}^{q_D,q_D'}$ is defined as $\Sigma_{\text{text}}^{q_D,q_D'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$, i.e., it does not include any symbol associated with other robots $i\neq j$ that may also satisfy $b_{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_i^{r_f}$). The same also holds for $\Sigma_{\text{inv}}^{q_D}$; see also Example \ref{ex:feas}. %Additionally, in case the empty symbol, denoted by $\varnothing$ belongs to 
%
Given a Boolean formula $b^{q_B,q_B'}$, we define the set $\ccalN^{q_B,q_B'}\subseteq\ccalN$ that collects the indices of all robots that appear in $b^{q_B,q_B'}$. Also, given a symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$, we define the set $\ccalR^{q_B,q_B'}\subseteq\ccalN^{q_B,q_B'}$ that collects the indices $j$ of the robots that are involved in generating $\sigma_{q_B,q_B'}$. Also, we denote by $L_{j}^{q_B,q_B'}$ the location that robot $j\in\ccalN^{q_B,q_B'}$ should be located to generate $\sigma^{q_B,q_B'}$. Note that for robots $j\in\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$, $L_{j}^{q_B,q_B'}$ corresponds to any location $\bbq\in\Omega$ where no atomic predicates are satisfied; see also Example \ref{ex:exFeasSets}. 


%THE ROBOTS IN $\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$ GET OUT OF THEIR CURRENT REGIONS!

\begin{ex}(Sets of Feasible Symbols)
(a) Consider the Boolean formula $b^{q_B,q_B'}=(\pi_j^{r_e}\vee\pi_j^{r_m})\wedge(\neg \pi_i^{r_e})$, then $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$. %, i.e., it does not include any symbol associated with other robots $k\neq j$ that may also satisfy $b_{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_k^{r_f}$).
Given the Boolean formula $b^{q_B,q_B'}$, we have that $\ccalN^{q_B,q_B'}=\set{j,i}$.
%
Also, for $\sigma^{q_B,q_B'}=\pi_j^{r_e}$, we have that $\ccalR^{q_B,q_B'}=\set{j}$, $L_{j}^{q_B,q_B'}=r_e$. (b) Consider the Boolean formula $b^{q_B,q_B'}=\neg \pi_i^{r_e}$. In this case $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\varnothing\}$, where $\varnothing$ denotes an empty symbol and is generated when a robot is outside all regions interests and does hit any obstacles. Also, we have that $\ccalN^{q_B,q_B'}=\set{i}$, $\sigma^{q_B,q_B'}=\varnothing$, $\ccalR^{q_B,q_B'}=\emptyset$, and while $L_{i}^{q_B,q_B'}$ corresponds to any location $\bbq$ in the workspace where no atomic predicates are satisfied. 
\label{ex:exFeasSets}
\end{ex}

Given the sets $\Sigma_{q_B,q_B'}$, we remove all NBA transitions with $\Sigma_{q_B,q_B'}=\emptyset$, i.e., all transitions that are require robots to be present in more than one locations in the environment simultaneously [line \ref{prune:inf}, Alg. \ref{alg:prune}]. Next we remove NBA transitions that require robots to move from one region of interest $\ell_i$ to another one $\ell_e$ without visiting any location $\bbq$ in the environment outside $\ell_i$. Such transitions are considered infeasible as they require robots to `jump' from one region of interest to another one.
%without robots to move to new regions of interest. Such transitions are removed as in practice they cannot be activated given that the regions of interest are disjoint. 
For instance, consider the LTL formula $\phi=\pi_1^{r_1}\ccalU\pi_1^{r_2}$ that requires robot $1$ to be in region $r_1$ until it enters $r_2$. The corresponding NBA is illustrated in Figure \ref{fig:NBA1}. Assume that the initial condition of the robot satisfies $b^{q_B^0,q_B^0}=\pi_1^{r_1}$, i.e., that robot $1$ is initially located in $r_1$. Then the transition from the initial to the final state is considered infeasible as it requires the robot to `jump' from one region of interest to another one. 

\begin{figure}
    \centering
     \includegraphics[width=0.6\linewidth]{figures/p1Up2.png}
    \caption{Example of an infeasible transition in the NBA corresponding to $\phi=\pi_1^{r_1}\ccalU\pi_1^{r_2}$. Transition from the initial state $q_B^0$ to the final state $q_B^F$ is infeasible as robot $1$ is required to `jump' from $\ell_1$ to $\ell_2$ while $\ell_1$ and $\ell_2$ are disjoint regions.}
    \label{fig:NBA1}
\end{figure}

\begin{figure}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Original NBA]{
    \label{fig:origNBA}
  \includegraphics[width=0.48\linewidth]{figures/feas1_bf.png}}
  \subfigure[Pruned NBA (Def. \ref{defn:feasSet})]{
    \label{fig:feas1}
  \includegraphics[width=0.34\linewidth]{figures/feas1_after.png}}
%  \caption{FEASIBLE 1}
%  \label{fig:tow7}
%\end{figure}
%
%\begin{figure}[t]
%  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Replicating NBA states]{
    \label{fig:repl}
  \includegraphics[width=0.5\linewidth]{figures/feas2_after.png}}
  \subfigure[Pruned NBA (Def. \ref{def:feas})]{
    \label{fig:finalPrune}
  \includegraphics[width=0.42\linewidth]{figures/feas2_pruned.png}}
  \caption{Graphical illustration of Algorithm \ref{alg:prune} applied to the NBA corresponding to $\phi=\square\Diamond(\pi_1^{\ell_1})\wedge\square\Diamond(\pi_1^{\ell_2})$. This formula requires robot $1$ to visit infinitely often $\ell_1$ and $\ell_2$. Figure \ref{fig:origNBA} shows the NBA   where the red dashed transitions are removed, as per Definition \ref{defn:feasSet}, as they require robot $1$ to be in $\ell_1$ and $\ell_2$ simultaneously yielding the pruned NBA shown in Figure \ref{fig:feas1}. Observe in Figure \ref{fig:feas1} that there is no self-loop for the final state $q_F$. Thus, $q_F$ is replicated twice since it has one incoming and two outgoing transitions as shown in Figure \ref{fig:repl}. In Figure \ref{fig:repl} the multi-hop transition $q_B\rightarrow_B q_F\rightarrow_B q_B$ is removed since there are no symbols that satisfy $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$ (condition (i)-Defn. \ref{def:feas}); in fact this transition requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$. The resulting pruned NBA generated by Algorithm \ref{alg:prune} is shown in Figure \ref{fig:finalPrune}.  
  }
  \label{fig:prune}
\end{figure}



To formalize this concept, we first %need to take into account the initial multi-robot state as it may also result in infeasible NBA transitions; see e.g., Figure \ref{fig:NBA1}. To this end, we introduce auxiliary states $q_B^{\text{aux}}$ and transitions $q_B^{\text{aux}}\rightarrow_B q_B^0$ for all $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=L(\bbp(0))$. The auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA. For
%In this way, we also ensure that the robots can remain in the initial states 
define the set $\hat{\ccalQ}_B\subseteq\ccalQ_B$ that collects all NBA states $q_B$ for which there exist feasible symbols (as per Definition \ref{defn:infPTS}) that allow a transition from $q_B$ to $q_B$, i.e., $\Sigma^{q_B,q_B}\neq\emptyset$, i.e., 
\begin{equation}
    \hat{\ccalQ}_B=\{q_B\in\ccalQ_B|\Sigma^{q_B,q_B}\neq\emptyset\},
\end{equation}
where $\Sigma^{q_B,q_B}$ is defined in Definition \ref{defn:feasSet}. Let $i_{q_B}$ and $o_{q_B}$ be the number of incoming and outgoing transitions for $q_B\in\hat{\ccalQ}_B$. For each state $q_B\in\hat{\ccalQ}_B$, we define the set $\ccalP_{q_B}$ that collects all possible pairs of incoming and outgoing transitions for $q_B$, i.e.,  
\begin{equation}\label{eq:pairs}
    \ccalP_{q_B}=\{[(q_B^{\text{in},i},q_B),(q_B,q_B^{\text{out},o})]\}_{i=1,o=1}^{i_{q_B},o_{q_B}}
\end{equation}
where with slight abuse of notation $(q_B^{\text{in},i},q_B)$ and $(q_B,q_B^{\text{out},o})$ denote an incoming and outgoing transition for $q_B$ respectively.
%$\ccalP_{q_B}=\{[(q_B^{\text{in},n},q_B),(q_B,q_B^{\text{out},m})]\}_{n=1,m=1}^{n=\bar{n},m=\bar{m}}$ that collects all possible pairs of incoming and outgoing transitions for $q_B$. 
Next we replicate all states $q_B\in\hat{\ccalQ}_B$ $i_{q_B}\times o_{q_B}$ times, so that each copy of $q_B$ has only one and unique pair of incoming and outgoing transitions; see Example \red{(????)}. 

Next for each state $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$ we compute all, possibly multi-hop, transitions that start from $q_B$ and end at states $q_B'\in q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$, $q_B'\neq q_B$ so that all, if any, intermediate NBA states that connect $q_B$ to $q_B'$ belong to $\hat{\ccalQ}_B$. Formally, these multi-hop transitions are defined as $q_B\rightarrow_B q_B^1\rightarrow_B q_B^2\rightarrow_B\dots\rightarrow_B q_B^K\rightarrow_B q_B'$, where $q_B^k\in\hat{\ccalQ}_B, k\in\{1,\dots,K\}$, and $K\geq 0$; see also Figure \red{(????)}. We compactly denote such a multi hop transition by $q_B\rightarrow_B^K q_B'$.%\footnote{Note that $q_B\rightarrow_B^0 q_B'$ corresponds to the one hop transition $q_B\rightarrow_B q_B'$.}

Given the above definitions, we define the feasible NBA transitions as follows; see also Example \ref{ex:feas}.
\begin{definition}[Feasible NBA transitions]\label{def:feas}
A transition $q_B\rightarrow_B^K q_B'$, where $q_B,q_B'\in\ccalQ_B\setminus\hat{\ccalQ}_B$, is feasible if (i) for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$ there exists at least one symbol $\sigma^{q_B,q_B^1}\in\Sigma^{q_B,q_B^1}$ that enables the multi-hop transition $q_B\rightarrow_B^K q_B'$, i.e.,
$\sigma^{q_B,q_B^1}\models b^{q_B,q_B'}_K$, where 
$b^{q_B,q_B'}_K=b^{q_B,q_B^1}\wedge b^{q_B^1,q_B^{2}}\wedge\dots\wedge b^{q_B^{K-1},q_B^{K}}\wedge b^{q_B^K,q_B'}\wedge b^{q_B',q_B'}$; and 
%
(ii) at least one of the symbols $\sigma^{q_B,q_B^1}$ that satisfy condition (i) should satisfy either (a) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^1}=\emptyset$ or (b) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^1}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^1}$. If $K=0$, conditions (i)-(ii) are applied by replacing $q_B^1$ with $q_B'$. %conditions (i)-(ii) assume
\end{definition}
%A transition $(q_B,\cdot,q_B')$ is feasible if (i) $\Sigma^{q_B,q_B}\neq \emptyset$; (ii) for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$ there exists at least one symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$ such that $\sigma^{q_B,q_B'}\models b^{q_B',q_B'}$; and (iii) at least one of the symbols $\sigma^{q_B,q_B'}$ that satisfy condition (ii) should satisfy either (a) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}=\emptyset$ or (b) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}\neq\emptyset$ and $L_{j}^{q_B,q_B'}=L_{j}^{q_B,q_B}$.

Then, we prune the NBA by removing transitions that are not feasible, as per Definition \ref{def:feas}. Note that condition (i) ensures that once robots reach a state $q_B$, they will always be able to make progress towards accomplishing the assigned task by moving towards a new NBA state $q_B'$. Also, due to condition (i), this will be achieved without requiring robots to be present in more than one location simultaneously (since $\sigma^{q_B,q_B^1}\in\Sigma^{q_B,q_B^1}$) or jump from one region of interest to another (since $\sigma^{q_B,q_B^1}\models b^{q_B,q_B'}_K$). Also, condition (ii) allows us to cast transition from $q_B$ to $q_B'$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B'}$ needs to move to a region of interest while avoiding certain regions and obstacles. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is continuously learned. 
%
Also, by construction of the pruned automaton we have that once the robots reach an NBA state $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$, i.e., an NBA state for which a self-loop exists, the robots can remain in this state given their current observations. To enforce this property from $t=0$, we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$. This property will be used in Section \ref{sec:planning} to design robot paths.
\begin{assumption}[Initial Robot State]
Assume that the initial multi-robot state $\bbp(0)$ satisfies $b^{q_B^0,q_B^0}$, i.e, $L(\bbp(0))\models b^{q_B^0,q_B^0}$ for at least one initial state $q_B^0\in\ccalQ_B^0$.
\end{assumption}

%In words, a transition from $q_B$ to $q_B'$ is feasible and, therefore, it is not removed (a) if the set $\Sigma^{q_B,q_B}$ is non-empty, i.e., there are feasible symbols that allow the robots to stay in state $q_B$; and (ii) for each possible symbol in $\Sigma^{q_B,q_B}$ that the robots may generate to reach $q_B'$, there exists a feasible symbol that will enable the robots to eventually reach a new state $q_B'$ from $q_B$ and stay in $q_B'$. Also, in (iii) we require the set of robots in $\ccalN^{q_B,q_B'}$ that to be either (a) disjoint from the set of robots in $\ccalR^{q_B,q_B}$ or (b) if there exist robots $j\in \ccalR^{q_B,q_B}\cap\ccalN_{\text{next}}^{q_B,q_B'}\neq\emptyset$ then these robots should suffice to stay in their current locations, i.e., $L_{j}^{q_B,q_B'}=L_{j}^{q_B,q_B}$, to `contribute' to satisfaction of $b_{\text{next}}^{q_D,q_D'}$. As it will be discussed later, this allows us to cast transition from $q_B$ to $q_B'$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalN^{q_B,q_B'}$ needs to move to a region of interest while avoiding certain regions and obstacles. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is learned.

%IN THE PRUNED AUTOMATON WE HAVE THAT ONCE WE VISIT A SELF-LOOP STATE WE CAN STAY IN IT MAKE PROGRESS I.E. VISIT NEW TASKS. This essentially allows us to avoid cases WHERE ROBOTS HAVE TO 'JUMP' FROM ONE REGION OF INTEREST TO ANOTHER ONE. WE USE THIS PROPERTY FOR PLANNING IN SECTION ?. TO ENFORCE THIS PROPERTY AT T=0, WE ASSUME THAT THE INITIAL CONDITION ALWAYS SATISFIES THE INITIAL SELF-LOOP IF IT EXISTS. 

%OR AVOID IT AND MENTION IT IN THE THEOREMS!!!

%IT IS POSSIBLE THAT THE INIT STATE DOES NOT HAVE A SELF LOOP OR THE INIT ROBOT STATE DOES NOT SATISFY.

%SAY HERE THAT OUR GOAL IS THAT ONCE WE VISIT A STATE WITH SELF LOOPS TO SATISFY THE RESPECTIVE CONDITION UNTIL WE MAKE NEW OBSERVATIONS THAT WILL ALLOWS US TO MAKE PROGRESS IE VISIT NEW TASKS


%\begin{ex}[Conservative Pruning]
%-Add figure and explain-
%\end{ex}
\begin{figure}
    \centering
     \includegraphics[width=1\linewidth]{figures/conserv.png}
    \caption{Example of conservative pruning for the NBA corresponding to $\phi=\square(\pi_1^{r_0}\vee\pi_1^{r_0}) \wedge \Diamond \pi_2^{r_1}\wedge \Diamond \pi_2^{r_1}$. This formula requires either robot $1$ or $2$ to always be in $\ell_0$ and eventually robots $1$ and $2$ to visit, not necessarily simultaneously, $\ell_1$. Transition from $q_B^0$ to $q_B^F$ is removed as it requires robots to visit more than one location at the same time. Transitions from $q_B$ to $q_F$ and from $q_B'$ to $q_F$ are removed as they violate both conditions of Definition \ref{def:feas} resulting in a disconnected pruned NBA, i.e., Algorithm \ref{alg:RRT} will not be able to find a solution. Nevertheless, a solution exists, as these two transitions can be enabled in practice. For instance, consider the transition from $q_B$ to $q_F$. %Assuming that both robots are initially in $\ell_0$, 
    Observe that transition from $q_B$ to $q_F$ cannot be cast as two independent reachability-avoidance problems (condition (ii)). Instead it requires coordination among the robots that is specific to the Boolean formula $b^{q_B,q_F}$. Specifically, when the robots reach $q_B$, we have that robot $1$ is in $\ell_0$ and robot $2$ is in $\ell_1$. To eventually satisfy $b^{q_B,q_F}=(\pi_1^{\ell_0}\wedge\pi_2^{\ell_1})\vee(\pi_2^{\ell_0}\wedge\pi_2^{\ell_1})$, first robot $2$ is required 
    to return in $\ell_0$ while in the meantime robot $1$ should stay in $\ell_0$. Once robot $2$ returns in $\ell_0$, robot $1$ should move to $\ell_1$ enabling the transition to the final state $q_F$.}
    \label{fig:conserv}
\end{figure}
%
%Conditions under which Definition \ref{def:feas} is not conservative are presented in Section \ref{sec:complOpt}.%, and/or (c) if it is (physically) impossible for the robots to stay in $q_D$ until the symbol $\sigma_{\text{next}}$, that triggers transition to $q_D'$, is generated; the latter happens if condition (iii) is not true (see also Ex. \ref{ex:feas}). 

On the pruned DFA, we define a function $d:\ccalQ_D\times\ccalQ_D\rightarrow \mathbb{N}$ that returns the minimum number of \textit{feasible} DFA transitions that are required to reach a state $q_D'\in\ccalQ_D$ starting from a state $q_D\in\ccalQ_D$. %This function will be used to guide the robots towards locations in the workspace so that eventually a final DFA state is visited, i.e., the LTL formula is satisfied.
%
Particularly, we define the distance function $d: \ccalQ_D \times \ccalQ_D \rightarrow \mathbb{N}$ as follows
\begin{equation}
d(q_D,q_D')=\left\{
                \begin{array}{ll}
                  |SP_{q_D,q_D'}|, \mbox{if $SP_{q_D,q_D'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_D,q_D'}$ denotes the shortest path (in terms of hops) in the  pruned DFA from $q_D$ to $q_D'$ and $|SP_{q_D,q_D'}|$ stands for its cost (number of hops).%\footnote{In Section \ref{sec:complOpt}, we provide conditions under which if $d(q_D^0,q_F)=\infty$ then the assigned co-safe LTL task is infeasible}. %; see Sections \ref{sec:targetDFA}-\ref{sec:paths}.
\begin{rem}[Conservative Pruning]\label{rem:conserv}
Notice that the proposed pruning approach for the NBA, as per Definition \ref{def:feas}, is conservative. For instance, there may exist feasible symbols (as per Definition \ref{defn:infPTS}) that enable a transition from $q_B$ to $q_B'$ that may not satisfy conditions (i)-(ii); see e.g., Figure \ref{fig:conserv}. Conditions under which the proposed pruning approach is not conservative are discussed in Section \ref{sec:complOpt}.
%Nevertheless, conservative pruning ensures that when the robots reach a state $q_D$, they will always be able to make progress towards accomplishing their task (i.e., reach a new state $q_D'$) regardless of the symbols they have generated to reach $q_D$ by solving local point-to-point navigation problems. A fragment of LTL for which the proposed approach is not conservative is discussed in Section \ref{sec:complOpt}.
\end{rem}


%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}

%\begin{ex}[Feasible DFA transitions]\label{ex:feas}
%(a) Consider the case, where $b^{q_B,q_B}=1$ and $b^{q_B,q_B'}=\pi_j^{r_{m}}$. By definition of $\Sigma^{q_B,q_B}$ and $\Sigma^{q_B,q_B'}$, we have that $\Sigma^{q_B,q_B}=\{\varnothing\}$, where $\varnothing$ stands for the empty symbol, and $\Sigma^{q_B,q_B'} =\{\pi_j^{r_{m}}\}$. Transition from $q_B$ to $q_B'$ is feasible as per Definition \ref{def:feas}. Recall that the sets $\Sigma^{q_B,q_B}, \Sigma^{q_B,q_B'}$ collect symbols that are associated with robots that play a role in satisfying the respective Boolean formulas. This precludes cases where, e.g., a symbol $\pi_j^{r_e}$, $e\neq m$ is included in $\Sigma^{q_B,q_B}$ resulting in erroneously characterizing the transition from $q_D$ to $q_D'$ as infeasible due to condition (iii). 
%%%(b) Consider the following Boolean conditions: $b_{\text{inv}}^{q_D}=b_{\text{inv}}^{q_D'}=\pi_j^{r_i}$ and $b_{\text{next}}^{q_D,q_D'}=\pi_j^{r_i}\wedge \pi_m^{r_h}$. Then the transition from $q_D$ to $q_D'$ is feasible since it satisfies Definition \ref{def:feas}. 
%(b) Consider also the Boolean formulas  $b^{q_B,q_B}=b^{q_B',q_B'}=\pi_j^{r_i}$ and $b^{q_B,q_B'}=\pi_j^{r_e}\wedge \pi_m^{r_h}$, then the transition from $q_B$ to $q_B'$ is infeasible, since it holds that $j\in \ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and, $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. In fact, transition from $q_B$ to $q_B'$ requires robot $j$ to instantaneously move from $r_i$ to $r_e$ which is not possible given that $r_i$ and $r_e$ are disjoint regions. 
%\end{ex}




%\subsection{Selecting a Feasible DFA Final State}\label{sec:feasFinal}
%Given the pruned DFA, the distance function, and an initial DFA state $q_D(0)$, our next step is to select a \textit{feasible} final state $q_{F}\in\ccalQ_F$, i.e., a final state that is reachable from $q_D(0)$ in the pruned DFA [line \ref{rrt:feasFinal}, Alg. \ref{alg:RRT}]. In math, given an initial state  $q_D(0)$ feasible final states are the ones that satisfy  $d(q_D(0),q_{F})\neq \infty$. Among all final states that satisfy this condition, we select one randomly denoted by $q_F^{\text{feas}}$. If there do not exist such final states given the state $q_D(0)$, then we select another initial DFA state $q_D(0)$ from $\ccalQ_D^0$. If there do not exist initial states such that $d(q_D^0,q_{F})\neq \infty$, then the LTL formula can not be satisfied since the in the pruning process, only the DFA transitions that are impossible to enable are removed (i.e., the ones that require the robots to be physically present at more than one region simultaneously) [lines \ref{rrt:unsat1}-\ref{rrt:unsat2}, Alg. \ref{alg:RRT}].
%Next at any time $t\geq 0$, given the current DFA state $q_D(t)$, we select a target DFA state, denoted by $q_D^{\text{next}}$, that the robots should reach next. This state is selected so that it is one hop closer to $q_F^{\text{feas}}$ than $q_D(t)$ is, i.e.,

%\subsection{Selecting the Next NBA State}
%{\bf{Selecting the Next NBA State:}} 
\subsection{Distributed Construction of Robot Paths}\label{sec:paths}
The pruning process described in Section \ref{sec:prune} occurs offline, i.e., before deploying the robots in the workspace. In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

Let $q_B(t)$ be the NBA state that the robots have reached at time $t$ after following paths, denoted by $\bbp_{j,[0:t]}$, and starting from an initial NBA state $q_B^0\in\ccalQ_B^0$. At time $t=0$, $q_B(0)$ is initialized to be one of the initial states $q_B^0$ of the NBA. Given the current NBA state $\bbq_B(t)$, the robots coordinate to select a new NBA state, denoted by $q_B^{\text{next}}$, that they should reach next to make progress towards accomplishing their task.
%every robot $j$ needs to locally design a path so that a DFA state that is closer to the final state $q_F$ than the current DFA state $q_D(t)$ is eventually reached. 
The NBA state $q_B^{\text{next}}$ is selected as follows. First, we compute the distance $d(q_BB(t),q_F^{\text{feas}})$, where $q_F^{\text{feas}}$ is a final NBA state that is reachable from its initial state $q_B^0$ in the pruned NBA, i.e., $d(q_B^0,q_F^{\text{feas}})\neq\infty$. Then, we select as $q_B^{\text{next}}$ a state that satisfies $d(q_B^{\text{next}},q_F^{\text{feas}}) = d(q_B(t),q_F^{\text{feas}}) -1$,
%\begin{equation}\label{eq:targetDFA}
%   d(q_D^{\text{next}},q_F) = d(q_D(t),q_F) -1, 
%\end{equation}
i.e., a state that is one hop closer to $q_F^{\text{feas}}$ than $q_B(t)$ is. If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}]. %; see  Sections \ref{sec:paths}. %or realize that a transition from $q_D(t)$ to $q_D^{\text{next}}$ is in fact infeasible; see next section.


%{\bf{Local Construction of Robot Paths:}}
Given the NBA state $q_B^{\text{next}}$, our goal is to design paths $\bbp_{j,t:T_j}$, for all robots $j$ that should be followed within a time interval $[t,T_j]$ so that the NBA transition from $q_B(t)$ to $q_B^{\text{next}}$ is activated. %\footnote{With slight abuse of notation the subscript in $\bbp_{j,t:T_j}$ denotes the index of robot and the time interval $[t,T_j]$ within which the path should be followed.} 
To achieve that, it suffices to ensure that the robots follow paths that (i) satisfy the Boolean formula $b^{q_B(t),q_B(t)}$ that allows them to stay in the current NBA state $q_B(t)$, until (ii) the Boolean formula $b^{q_B(t),q_B^{\text{next}}}$ that enables transition from $q_B(t)$ to $q_B^{\text{next}}$ is satisfied while (iii) while never satisfying Boolean formulas $b^{q_B(t),q_B''}$ other than the ones that are satisfied at time $t$.\footnote{At time $t$, the Boolean formula $b^{q_B(t),q_B(t)}$ is satisfied by construction of the pruned automaton. Nevertheless, other Boolean formulas $b^{q_B(t),q_B''}$ may be satisfied as well due to the non-deterministic nature of the NBA.} 
For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b_{\text{inv}}$ and $b_{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.

\red{[add reference to lines of the algorithm]}
To design paths $\bbp_{j,t:T_j}$, \textit{first} the robots $j\in\ccalN_{\text{next}}$ \textit{communicate} to select a symbol $\sigma_{\text{next}}$ that satisfies conditions (i)-(ii) of Definition \ref{def:feas} given the current symbol  $\sigma_{\text{inv}}=L(\bbp(t))$ they are generating. %; see also Example \ref{ex3}. 
Note that such a symbol exists by construction of the pruned NBA for any symbol $\sigma_{\text{inv}}$. % \footnote{Note that it is possible that given the symbol that the robots generated to reach $q_D$ there may not exist a pair of symbols $\sigma_{\text{inv}}$ and $\sigma_{\text{next}}$ to reach a state $q_D^{\text{next}}$ that satisfy condition (iii) of Def. \ref{def:feas}. In other words, transition from $q_D$ to $q_D^{\text{next}}$ may not be cast as a point-to-point navigation problem as in \eqref{eq:localProb}.
%Consider e.g., the DFA that corresponds to $\phi=\square(\pi_1^{r_0}\vee\pi_2^{r_0})\wedge\Diamond(\pi_1^{r_1})\wedge\Diamond(\pi_2^{r_2})$. 
%Existence of such symbols is always guaranteed for a sub-class of co-safe LTL formulas as discussed in Lemma \ref{lem:cnt}.} %that satisfy $b_{\text{inv}}$ and $b_{\text{next}}$, respectively, i.e., $\sigma_{\text{next}}\models b_{\text{next}}$. This pair of symbols is selected so that condition (ii) of Definition \ref{def:feas} is satisfied; 
Among all such symbols $\sigma_{\text{next}}$, we select the one that yields the smallest set $\ccalN_{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
%
%Given $\sigma_{\text{next}}$, we compute the set $\ccalR_{\text{next}}$ that collect the robots that need to move towards certain regions of interest $r_e$ in workspace to generate $\sigma_{\text{next}}$. 
%
\textit{Second}, given $\sigma_{\text{next}}$,  we compute for each robot $j\in\ccalN_{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma_{\text{next}}$. Recall that for robots $j\in\ccalR_{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma_{\text{next}}$  while for robots $j\in\ccalN_{\text{next}}\setminus\ccalR_{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%\textit{Third}, we design the paths $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ for all robots $j\in\ccalN_{\text{next}}$. %First, all robots $j\notin\ccalR_{\text{inv}}$ stay put at their current locations until the state $q_B^{\text{next}}$ is reached. %
\textit{Third}, every robot $j\in\ccalN_{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%that if followed the symbol  $\sigma_{\text{next}}\models b_{\text{next}}$ is generated and the DFA state $q_D^{\text{next}}$ is reached
%In Section \ref{sec:complOpt}, we show that the multi-robot state $\bbp(t)$ already generates a symbol that satisfies $b_{\text{inv}}$. We also show that if (i) the robots that are involved in generating $\sigma_{\text{inv}}$, collected in a set $\ccalR_{\text{inv}}$, stay idle at their current locations $\bbp_j(t)$ and (ii) all other robots 
%
%
%\footnotesize
\begin{subequations}
\label{eq:localProb}
\begin{align}
%& \min_{\substack{T_j, \bbu_{j,t:T_j}}} \left[J(T_j,\bbu_{j,t:T_j}) = \int_{t'=t}^{T_j}  w(\bbp_j(t'),\bbu_j(t'))dt \right] \label{ObjLoc2}\\
& \text{Compute:~}{T_j, \bbu_{j,t:T_j}}~\text{such that}  \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ [L(\bbp_j(t'))=L(\bbp_j(t))] \vee [L(\bbp_j(t'))=\varnothing] \nonumber\\
%& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \vee [L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}],~\forall t'\in[t,T_j] \label{constrLoc1} \\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \cup_i\set{r_i}\setminus (R_j^t\cup L_j^{\text{next}}), \forall t'\in[t,T_j] \label{constrLoc1}\\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \hat{O}(t), \forall t'\in[t,T_j] \label{constrLocObs}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j) \in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin \ccalA_j^{\text{avoid}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'+1),\bbu_j(t'+1)), \label{constrLoc3}
\end{align}
\end{subequations}
%\normalsize

\noindent In \eqref{constrLoc1}, $R_j^t$ denotes the region that robot $j$ lies in at time $t$. The first constraint \eqref{constrLoc1} requires that robot $j$ should not visit any region $r_i$ excluding $R_j^t$ and the target region $L_j^{\text{next}}$, for all $t'\in[t,T_j]$. If at time $t$ robot $j$ does not lie in any of the regions $r_i$, then $R_j^t=\emptyset$. This ensures that the multi-robot system can always remain in $q_B(t)$ as the robots $j\in\ccalN_{\text{next}}$ navigate the workspace; see Lemma \ref{lem:binv}. This constraint can be relaxed by requiring  robot $j\in\ccalN_\text{next}$ to always avoid only regions that may result in violating $b_{\text{inv}}$. For instance, if $b_{\text{next}}=\neg(\pi_j^{r_e}\wedge\pi_i^{r_e}$), then it suffices to require robot $j$ to never visit $r_e$.  %\footnote{$T_j^{-}$ denotes a time instant right before $T_j$, i.e., $T_j^{-}=T_j-\epsilon$, for an arbitrarily small $\epsilon>0$.} 
Similarly, the second constraint in \eqref{constrLocObs} requires robot $j$ to avoid all obstacles, collected in $\hat{O}(t)$, that are known up to the time instant $t$. The third constraint in \eqref{constrLoc2} requires robot $j$ to be in region $L_j^{\text{next}}$ at a time instant $T_j\geq t$. %so that it generates $L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}$.%\footnote{Note that this prevents the robot from visiting parts of $L_j^{\text{next}}$ that are shared with other regions $r_i$.} 
This is required to eventually generate the symbol $\sigma_{\text{next}}$. The last constraint in \eqref{constrLoc3} captures the robot dynamics. Note that among all paths that satisfy these constraints, the optimal one, as a per a user-specified motion cost function, can be selected. %In words, the optimal control problem \eqref{eq:localProb} requires robot $j$ to design a path $\bbp_{j,t:T_j}$ that reaches $L_j^{\text{next}}$ (see \eqref{constrLoc2}) while avoiding certain regions $r_i$ (see \eqref{constrLoc1}) and all detected obstacles denoted by $\hat{O}(t)$ (see \eqref{constrLocObs}). %Note that the robots that do not belong to $\ccalR_{\text{inv}}$ and also are not responsible to generate $\sigma_{\text{next}}$ do not have a target region $L_{j}^{\text{next}}$. These robots remain stationary in their current locations and they do not need to solve \eqref{eq:localProb}.
%
Observe that \eqref{eq:localProb} is a  point-to-point navigation problem, and, therefore, any of the traditional motion planning algorithms, such as $\text{A}^*$, RRT, $\text{RRT}^*$, RRG, or PRM, can be used to solve it \cite{karaman2011sampling}. Finally observe that given $L_j^{\text{next}}$, robot $j$ locally solves \eqref{eq:localProb} without communicating with any other robot. %Correctness of Alg. \ref{alg:RRT} is discussed in Sec. \ref{sec:complOpt}. %Feasibility of such this problem is examined in 

%We design such paths in two stages. In the first stage, we design subpaths $\bbp_{j,t:\bar{T}_j}$ for some $t<\bar{T}_j<T$ and in the second stage we design paths $\bbp_{j,\bar{T}_j:T_j}$. In particular, \textit{in the first stage} all robots that are involved in generating $\sigma_{\text{inv}}$, collected in a set $\ccalR_{\text{inv}}$, and all other robots $j$ for which it hold $L(\bbp_j(t))=\varnothing$ (i.e., they are outside of all regions $r_i$) stay idle at their current locations $\bbp_j(t)$, i.e., $\bar{T}_j=t+1$ and $\bbp_{j,t:\bar{T}_j}=[\bbp_j(t),\bbp_j(t)]$ All other robots $j$ (i.e., the ones that satisfy $j\notin\ccalR_{\text{inv}}$ and $L(\bbp_j(t))\neq \varnothing$) solve the following optimal control problem to design paths $\bbp_{j,t:\bar{T}_j}$ that if followed then the robots will move outside the regions that they are currently located. %As it will bbe discusses in Section \ref{sec:exec}, these subpaths will be executed so that the robots will move outside their current regions simultaneously.

%\begin{subequations}
%\label{eq:localProb1}
%\begin{align}
%& \min_{\substack{\bar{T}_j, \bbu_{t:\bar{T}_j}}} \left[J(\bar{T}_j,\bbu_{t:\bar{T}_j}) = \sum_{t'=t}^{\bar{T}_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc1}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in R_j(t), \forall t\in\set{t,\dots,\bar{T}_j-1} \label{constrLoc1a} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in \ccalR_j^{\text{inv}}, \forall t\in\set{t,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(\bar{T}_j))=\varnothing \label{constrLoc2a}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   %\bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc2}
%\end{align}
%\end{subequations}
%where $R_j(t)$ denotes the region $r_i$ that robot $j$ lies in at time $t$. Observe that the first two constraints \eqref{constrLoc1a}-\eqref{constrLoc2a} require robot $j$ to move outside the region $\ccalR_j(t)$ where it is located at the time instant $t$. This happens at a time instant $\bar{T}_j$, i.e., $L(\bbp_j(\bar{T}_j))=\varnothing$. Note that robot $j$ locally solves \label{eq:localProb1} with communicating with other robots. Observe that execution of these subpaths ensures that the robots remain in the DFA state $q_D(t)$ since $b_{\text{inv}}$ is always satisfied as the robots $\ccalR_{\text{inv}}$ remain stationary in their current locations that generates  $\sigma_{\text{inv}}\models b_{\text{inv}}$.

%since the robots in $\ccalR_{\text{inv}}$

%In the \textit{second} stage, we construct the subpaths $\bbp_{j,\bar{T}_j:T_j}$ that will enable the transition from $q_D(t)$ to $q_D^{\text{next}}$. For robots $j\in\ccalR_{\text{inv}}$, we select $T_j=\bar{T}_j+1$ and $\bbp_{j,\bar{T}_j:T_j}=[\bbp_{j}(t),\bbp_{j}(t)]$, i.e., these robots still stay idle. In fact, due to the deterministic structure of the DFA, this ensures that the robots remain in the DFA state $q_D(t)$ until the symbol $\sigma_{\text{next}}$ is generated which will activate the transition towards $q_D^{\text{next}}$. To generate the symbol  $\sigma_{\text{next}}$, all other robots $j\notin\ccalR_{\text{inv}}$ design paths $\bbp_{j,\bar{T}_j:T_j}$ by solving the following optimal control problem:

%\begin{subequations}
%\label{eq:localProb}
%\begin{align}
%& \min_{\substack{T_j, \bbu_{\bar{T}_j:T_j}}} \left[J(T_j,\bbu_{\bar{T}_j:T_j}) = \sum_{t'=\bar{T}_j}^{T_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ L(\bbp_j(t'))=\varnothing, \forall t'\in\set{\bar{T}_j,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
%\end{align}
%\end{subequations}



 %This ensures that  transition to a DFA state $q_D'\neq q_D(t)$ that is not $q_D^{\text{next}}$. 
%In the meantime the robots in $\ccalR_{\text{inv}}$ ensure that the current DFA state remain the same in $[t,\bar{T}-1]$, since they stay idle and generate the symbol $\sigma_{\text{inv}}$. Also note that robots in $\ccalR_{\text{inv}}$ do not belong to the set of robots that need to move to another location to generate the symbol $\sigma$, since that would create a conflict; see also Remark \ref{rem:invariant}. 
%The second constraint in \eqref{constrLoc2} requires that at time instant $T_j$, all robots should be in their corresponding locations $L_j^\textbf{}$. Once this happens the symbol $\sigma_{\text{next}}$ is generated and the target DFA state is reached.
%
%Note that infeasibility of \eqref{eq:localProb} is due to the facts (i) the environment is unknown and, therefore, it is not possible to check offline which DFA transitions cannot be enabled because e.g., of the robot dynamics or the existence of obstacles.%; and (ii) the LTL formula $\phi$ is decomposed into local sub-tasks Problem \ref{prob} is solved in a distributed the proposed algorithm is distributed nature of the proposed 

%What if the problem is infeasible? update $\sigma$ i.e., $L_j$. If no other $L_j$. update target DFA state. If no other target DFA state report `current method failed (this does not mean that the task is unsatisfiable though)'

%\begin{ex}[Selection of $\sigma_{\text{next}}$ and $\sigma_{\text{inv}}$]\label{ex3}
%Consider the Boolean formulas $b_{\text{inv}}=\neg \pi_{\text{obs}}$ and $b_{\text{next}}=(\pi_j^{r_1}\vee \pi_j^{r_3} )\wedge\pi_e^{r_2}\wedge (\neg \pi_j^{r_2}) \wedge (\neg (\pi_j^{r_1}\wedge \pi_e^{r_1}))$, where the atomic predicate $\pi_{\text{obs}}$ is true of at least one robot hits an obstacle. A symbol $\sigma_{\text{next}}$ that satisfies $b_{\text{next}}$ is $\sigma_{\text{next}}=\pi_j^{r_1}\pi_e^{r_2}$ while $b_{\text{inv}}$ is satisfied by an empty string, i.e., $\sigma_{\text{inv}}=\varnothing$. Given this pair of symbols, we have that $\ccalR_{\text{inv}}=\emptyset$, $\ccalR_{\text{next}}=\set{j,e}$, $L_j^{\text{next}}=r_1$, and $L_e^{\text{next}}=r_2$.
%\end{ex}

%\begin{ex}[Construction of $\sigma_{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b_{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$. Then, we have that $\sigma_{\text{inv}}=\pi_j^{r_1}$ and $\ccalR_{\text{inv}}=\set{j}$. Similarly, if $b_{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma_{\text{inv}}$ is an empty string and $\ccalR_{\text{inv}}=\emptyset$.
%\end{ex}

%\begin{ex}
%--add automaton figure--and explain--
%\end{ex}
%\begin{rem}[Initialization of $q_B(t)$]
%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}
%\end{rem}
\subsection{Reacting to Map Uncertainty}\label{sec:exec}
%{\bf{Reactive Planning to Map Uncertainty:}}

The robots need to adapt their control actions to the continuously learned occupancy grid map. In fact, reactivity to the environment is required in two cases. First, as the robots follow their paths $\bbp_{j,t:T_j}$, they may discover new obstacles based on their sensor measurements; see \eqref{eq:sensor}. If the discovered obstacles intersect with their paths $\bbp_{j,t:T_j}$, for some $j\in\ccalR_{\text{next}}$, then these robots $j$ locally re-solve \eqref{eq:localProb} using the updated map to design new paths. Note that existing reactive planning algorithms that can address reachability navigation problems in the presence of unknown obstacles can also be used to solve \eqref{eq:localProb}; see e.g., \cite{guzzi2013human,vasilopoulos2018sensor,bansal2019combining,ryll2019efficient}.

%is not reachable e.g., due to the robot dynamics or 
Second, as the the map $M(t)$ is constructed, goal regions $L_j^{\text{next}}$ may become unreachable because of the structure of the environment (e.g., regions of interest may be surrounded by obstacles). In this case, robots $j$ that cannot reach $L_j^{\text{next}}$ communicate with all other robots so that a new symbol $\sigma_{\text{next}}$ is selected. This process is repeated until a reachable region $L_j^{\text{next}}$ is selected.  %that makes \eqref{eq:localProb} feasible. 
If such a symbol $\sigma_{\text{next}}$ does not exist, then this means that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$, due to the a-priori unknown structure of the environment. Then, the pruned NBA is updated by removing this transition and a new NBA state $q_B^{\text{next}}$. If there do not exist any candidate NBA states to be selected as $q_B^{\text{next}}$, then the assigned task cannot be accomplished given the current multi-robot and NBA state. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
In fact, there may exist another sequence of NBA states for which  Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible (i.e., paths towards selected goal regions always exist) and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.

%\begin{rem}[Feasibility of \eqref{eq:localProb}]
%Observe that \eqref{eq:localProb} may be \textit{infeasible}. This can be the case e.g., if the region $L_j^{\text{next}}$ is not reachable e.g., due to the robot dynamics or the structure of the environment. In this case, robot $j$ needs to communicate with all other robots so that a new symbol $\sigma_{\text{next}}$ is selected. This process is repeated until regions $L_j^{\text{next}}$ are selected that make \eqref{eq:localProb} feasible. If such a symbol $\sigma_{\text{next}}$ does not exist, then this means that the transition from $q_D(t)$ to $q_D^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$. Then, the pruned DFA is updated by removing this transition. Next, a new target DFA state is selected that is closer to the final state $q_F$ than $q_D(t)$ is. If there do not exist such DFA states then the robots cannot accomplish the assigned task. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
%In fact, there may exist another sequence of DFA states for which  Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
%Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.
%\end{rem}

%{\bf{Asynchronous Execution of Paths:}} 
\subsection{Asynchronous Execution of Paths}
The robots $j\in\ccalR_{\text{next}}$ execute their paths $\bbp_{j,t:T_j}$ \textit{asynchronously} until the time instant $T_j$, i.e., until they reach their respective target regions $L_j^{\text{next}}$ [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. At time $T_j$, robot $j$ waits for all other robots $e\in\ccalR_{\text{next}}$ with $T_e>T_j$. At time instant $T=\max_{j\in\ccalN_{\text{next}}}\{T_j\}$, i.e., when \textit{all} robots $j\in\ccalN_{\text{next}}$ have reached their respective regions $L_j^{\text{next}}$, the symbol $\sigma_{\text{next}}$ is generated. Then, the multi-robot system reaches the NBA state $q_B^{\text{next}}$ and a new NBA state is selected [lines \ref{rrt:T}-\ref{rrt:UpdGoals}]. This process is repeated indefinitely so that a final state is reached infinitely often.
%In Section \ref{sec:complOpt}, we show the robots remain in the NBA state $q_B(t)$ for all  $t'\in [t, T-1]$ and transition to $q_B^{\text{next}}$ occurs at the time instant $T$. Once this happens, the robots update their current DFA state and select the next DFA state [lines \ref{rrt:T}-\ref{rrt:UpdGoals}]. This process is repeated until the final state $q_F$ is reached.

%
%\begin{rem}\label{rem:invariant}
%Note that once the robots reach a new DFA $q_D$, they satisfy its respective Boolean condition $b_{\text{inv}}$, since the `next' temporal operator is excluded from the task specification. Particularly, if $b_{\text{inv}}$ is not satisfied this implies that once the robots are at locations that generate a symbol that triggers the transition to $q_D$, the robots should immediately leave their locations, which is impossible to specify unless the next operator is included in the specification language. 

%Recall that $\sigma_{\text{inv}}$ is selected to have the minimum length, this means that the minimum number of robots are involved to generate it. Therefore, robots that are required to generate the symbol $\sigma$ are not included in the set $\ccalR_{\text{inv}}$; see also Remark \ref{rem:invariant}.
%Similarly, robots that are responsible to satisfy $b_{\text{next}}$ cannot be responsible for generating the symbol $\sigma_{\text{inv}}$, since the next operator does not exist and all regions are assumed to be disjoint. %(unless there is an overlap..)
%\end{rem}


%\subsection{Online Re-planning}\label{sec:replan}






\begin{rem}[Communication]
%Note that Algorithm \ref{alg:RRT} requires all-time communication to ensure that all robots always have access to the same map $M(t)$. Nevertheless, this requirement can be straightforwardly relaxed by allowing each robot to build their local map $M_j(t)$. Moreover, 
Execution of the paths $\bbp_{j,t:T_j}$ does not require all-time communication among robots, which is typically the case in relevant temporal logic algorithms. Instead, communication is intermittent and is required only in the following two cases: (i) all robots need to communicate with each other to select the symbol $\sigma_{\text{next}}$ (ii) every robot $j\in\ccalR_{\text{next}}$ needs to send a message to all other robots in $\ccalR_{\text{next}}$ once it is ready to step into the region $L_{j}^{\text{next}}$. %; see Section \ref{sec:exec}.
\end{rem}

%Next, we define the set $\ccalL_j$ that collects all robot positions $\bbp_j$ that violate $b_{\text{inv}}$ regardless of the state of all other robots. For instance, if $b_{\text{inv}}=\neg (\pi_j^{r_e}\wedge \pi_z^{r_h})$, then $\ccalL_j=\emptyset$. On the other hand, if $b_{\text{inv}}=\neg (\pi_j^{r_e})\wedge (\neg \pi_z^{r_h})$ then  $\ccalL_j=\set{r_e}$. Formally, to construct the set, we express the negation of $b_{\text{inv}}$, denoted by $\bar{b}_{\text{inv}}=\neg b_{\text{inv}}$ as




==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/proof2.tex <==
%In this section we provide the proof of Lemma \ref{lem:binv} required to prove that Algorithm \ref{alg:RRT} is complete. To prove this result, we need first to state the following results.

%First, we show that once the robots reach a DFA state $q_D^{\text{next}}$ they can remain in this state if they stay in their current configuration.

%\begin{lem}[Feasibility]\label{lem:feas}
%Assume that the robots reach a configuration $\bbp(t)$ that generates a word $\sigma=L(\bbp(t))$ which enables a transition to the DFA state $q_D^{\text{next}}$. Then, it holds that $\sigma\models b^{\text{inv}}$, where $b^{\text{inv}}$ is a Boolean formula that needs to be satisfied to remain in $q_D^{\text{next}}$. 
%\end{lem}

%\begin{proof}
%This result follows directly from the fact that the `next' operator is excluded from the syntax of the task specification language. Particularly, let $q_D^{\text{next}}$ denote the DFA state that the robots will reach from   $q_D^{\text{next}}$ if they stay put in $\bbp(t)$. In what follows, we show by contradiction that $q^{\text{next}}$ exists (i.e., staying in $\bbp(t)$ does not violate $\phi$) and  $q_D^{\text{next}}=q_D^{\text{next}}$. Assume that $q_D^{\text{next}}$ does not exist. This means that once the robots reach $\bbp(t)$ and the current DFA state becomes $q_D^{\text{next}}$, we have that $\delta(L(\bbp(t)),q_D^{\text{next}})=\varnothing$. This means that once the robots reach $\bbp(t)$ they should immediately leave it, beause otherwise the LTL formula is violated. This implies the existence of the `next' operator in the specification language which is not the case. Therefore, we conclude that $q_D^{\text{next}}$ exists.

%Next, we show that $q_D^{\text{next}}=q_D^{\text{next}}$. Assume $q_D^{\text{next}}\neq q_D^{\text{next}}$. This implies that once $L(\bbp(t))$ is generated and $q_D^{\text{next}}$ is reached, the robots should leave $\bbp(t)$ immediately in order to stay in $q_D^{\text{next}}$; otherwise $L(\bbp(t))$ will enable a subsequent transition to $q_D^{\text{next}}\neq q_D^{\text{next}}$. This also implies the existence of the `next' operator in the specification language which is not the case completing the proof.
%\end{proof}

%This implies that the same word $L(\bbp(t))$ enables first a transition from a DFA state $q_D$ to $q_D^{\text{next}}$ and second, once this happens, a transition from $q_D^{\text{next}}$ to $q_D^{\text{next}}$ is enabled immediately. This means that $q_D^{\text{next}}$ is a `dummy' state in the DFA which cannot happen 
%$\ccalR=\set{q\in\ccalQ_D~|~q=(L(\bbp(t)),q_D^{\text{next}})}$.
%
%if $\sigma\not\models b^{\text{inv}}$, then this means that once the robots reach the configuration $\bbp(t)$ and the current DFA state becomes $q_D(t)=q_D^{\text{next}}$, the robots should immediately leave from this configuration in order to stay in $q_D(t)$. This implies the existence of the `next' operator in the specification language which is not the case completing the proof.

%Next, let $\sigma_{\text{cur}}$ denote the word that the multi-robot system currently generates, i.e., $\sigma_{\text{cur}}=L(\bbp(t))$. Assume also that $\sigma_{\text{cur}}$ enables a transition from $q_D(t)$ to $q_D'\neq q_D(t)$. Let $b^{\text{inv}}$ be the Boolean formula that the robots should satisfy in order to remain in $q_D'$. Recall that in Lemma \ref{lem:feas}, we showed that  $\sigma_{\text{cur}}\models b^{\text{inv}}$, i.e., the robots can stay in the DFA state $q_D'$ as long as they stay idle. Next, we define the $\sigma^{\text{inv}}$ that is constructed by replacing in $\sigma_{\text{cur}}$ the maximum possible number of symbols with the empty string, so that $\sigma^{\text{inv}}$ still satisfies $b^{\text{inv}}$, i.e., $\sigma^{\text{inv}}\models b^{\text{inv}}$; see also Example \ref{ex4}. Let $\ccalR^{\text{inv}}$ be the robots that appear in $\sigma^{\text{inv}}$ and let $L_j^{\text{inv}}$ be the regions that robots $j\in\ccalR^{\text{inv}}$ have to belong to in order to generate $\sigma^{\text{inv}}$; see also Example \ref{ex4}. In the following lemma, we show that $\ccalR^{\text{inv}}$ and $\ccalR^{\text{next}}$ are disjoint sets.

%\begin{lem}[Conflict-free]\label{lem:confl}
%Let sets $\ccalR^{\text{inv}}$ be the set of robots that are responsible  and $\ccalR^{\text{next}}$ are disjoint. %If $\phi$ is satisfiable, then Algorithm \ref{alg:RRT} is conflict-free i.e., a robot $j\in\ccalR^{\text{inv}}$ that is required to stay idle will never have to solve \eqref{eq:localProb} to design a path towards a new region. 
%\end{lem}

%\begin{proof}
%Recall first that $\sigma^{\text{inv}}$ is the word with the minimum length that satisfies $b^{\text{inv}}$. This means that $\ccalR^{\text{inv}}$ does not involve `unnecessary' robots whose presence in a region $r_i$ does not affect the satisfaction of $b^{\text{inv}}$. The respective result also holds for $\sigma^{\text{next}}$. Note that this is important since otherwise, it is trivial to see that $\ccalR^{\text{inv}}$ and $\ccalR^{\text{next}}$ may not be disjoint.
%Given words $\sigma^{\text{inv}}$ and $\sigma^{\text{next}}$, assume that there exist a robot $j\in\ccalR^{\text{inv}}\cap\ccalR^{\text{next}}$. This means that according to the LTL task, robot $j$ has to be present in the region $L_j^{\text{inv}}$ for all time instants $t'\in[t,T)$ and in $L_{j}^{\text{next}}$ at the time instant $T$. Nevertheless, this is impossible to specify given that the `next' operator is not included in the task specification language.
%\end{proof}

 
%\begin{ex}[Construction of $\sigma^{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b^{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi_w^{r_2})\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$ (i.e., $\bbp_{j}\in r_1\cap r_2$). Then, we have that $\sigma^{\text{inv}}=\pi_j^{r_1}$, $\ccalR^{\text{inv}}=\set{j}$, and $L_j^{\text{inv}}=r_1$. Similarly, if $b^{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma^{\text{inv}}$ is an empty string and $\ccalR^{\text{inv}}=\emptyset$.
%\end{ex}
%, i.e., Algorithm \ref{alg:prune} will remove the multi-hop transition $q_B\rightarrow_B^K$ only if 

\subsection{Proof of Lemma \ref{lem:fragmentLTL}}
%\begin{proof}
To show this result, first we express all Boolean formulas $b^{q_B,q_B'}$ associated with any NBA transition $\delta(q_B,\cdot,q_B')$ in CNF, i.e., as a conjunction of $F$ Boolean formulas $b_f$, for some $F>0$, where $b_f$ is a disjunction of literals, i.e.,
\begin{equation}\label{eq:bqbqb}
    b^{q_B,q_B'}=\bigwedge_{f=1}^F b_f.
\end{equation}
%Assume that all literals in a clause $b_f$ are associated with only one robot, for all $f\in\{1,\dots,F\}$. 
%In what follows, we show by contradiction that Algorithm \ref{alg:prune} is not conservative if every clause $b_f$ is associated with only one robot, for all $f\in\{1,\dots,F\}$.
By Assumption \ref{as:cnf} we have that every clause $b_f$ is associated with only one robot, for all $f\in\{1,\dots,F\}$. Let $\ccalF_j$ be a set that collects all indices $f\in\{1,\dots,F\}$ to formulas $b_f$ that are associated with robot $j$, where $\ccalF_j\cap\ccalF_i=\emptyset$, for all $i,j\in\ccalN$, by definition of $b_f$. Next we define the Boolean formula 
\begin{equation}\label{eq:dj}
    d_j^{q_B,q_B'}=\bigwedge_{j\in\ccalF_j}b_f,
\end{equation}
which is a conjunction of all Boolean formulas $b_f$ associated with robot $j$ that appear in \eqref{eq:bqbqb}. Using \eqref{eq:dj} and the fact that $\ccalF_j\cap\ccalF_i=\emptyset$, for all $i,j\in\ccalN$, we can re-write \eqref{eq:bqbqb} as 
\begin{equation}\label{eq:bqbqb2}
    b^{q_B,q_B'}=\bigwedge_{j=1}^N d_j^{q_B,q_B'}.
\end{equation}
Thus, if Assumption \ref{as:cnf} holds, then the Boolean formula $b^{q_B,q_B'}$ defined in \eqref{eq:b} can be decomposed into local/decoupled sub-formulas $d_j^{q_B,q_B'}$ as in \eqref{eq:bqbqb2}. In other words, robot $j$ can make decisions to contribute to satisfaction of $b^{q_B,q_B'}$ independent from other robots by considering only the sub-formula $d_j^{q_B,q_B'}$. 

Due to the decomposition of \eqref{eq:b} as per \eqref{eq:bqbqb2}, we can apply Definition \ref{def:feas} locally to each robot as follows. %
Specifically, a transition $\delta_B^m(q_B,\cdot,q_B')$ is decomposable if the following condition holds for all robots $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$. For all symbols $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}_j$, there should exist at least one symbol $\sigma^{q_B,q_B'}_j$ that satisfies $d_j^{q_B,q_B^K}$ (i) and either (A) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B'}$. 
%Note that since symbols $\sigma^{q_B,q_B^K}$ that satisfy condition (i) exist, this means $L_{j}^{q_B,q_B^K}$ is unique/well-defined for all robots $j\in\ccalR^{q_B,q_B^K}$.
Assume that there exists at least one robot $j$ for which this condition is not satisfied i.e., there exists at least one symbol $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}_j$ for which there are no such $\sigma^{q_B,q_B'}_j$. This means that there exists $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. Since $j\in\ccalR^{q_B,q_B}$, we have that transition towards the state $q_B$ was enabled because robot $j$ reached a region of interest $L_{j}^{q_B,q_B}$. Also, since $j\in\ccalR^{q_B,q_B'}$, we get that transition from $q_B$ to $q_B'$ will be enabled only if robot $j$ visits a region of interest denoted by $L_{j}^{q_B,q_B'}$. By assumption we have that $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. Therefore, we conclude that if Definition \ref{def:feas} is not satisfied then transition from $q_B$ to $q_B'$ can be enabled only if robot $j$ keeps being in a region of interest $L_{j}^{q_B,q_B}$ until it reaches another region $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$, which is impossible given that all regions of interest are disjoint completing the proof.
%\end{proof}
%(i.e. the only NBA transitions that will be removed are the ones that require a robot does not include any Boolean subformula of the form $\vee_{j\ccalR}(\pi_j)$

%\subsection{Proof of Lemma \ref{thm:nonexist}}
%We show this result by contradiction. Assume that there exists a solution to Problem \ref{prob}. If there exists a solution to Problem \ref{prob} and Assumption (b) holds then we have that in $\ccalG$ there are states $q_B,q_B'\in\ccalV$ for which there does not exist a corresponding edge $(q_B,q_B')\notin\ccalE$ while the corresponding transitions $\delta_B^m(q_B,\cdot,q_B')$ can be enabled by the robots, i.e., without requiring them to instantaneously jump from one location to another one or being present in more than one location at the same time. Let $\delta_B^m(q_B,\cdot,q_B')$ be such a transition.
%
%Since $(q_B,q_B')\notin\ccalE$ this means that either (i) there does not exists a (feasible) symbol $\sigma^{q_B,q_B'}$ that satisfies $b^{q_B,q_B'}$ defined in \eqref{eq:b} or (ii) there exist symbols $\sigma^{q_B,q_B'}$ that satisfy $b^{q_B,q_B'}$ but none of them satisfies Definition \ref{def:feas}. By definition of $b^{q_B,q_B'}$ we have that in case (i), the state  $q_B'$ can be reached from $q_B$ only if the robots can instantaneously jump from one location to another one. Nevertheless, this contradicts the assumption that $\delta_B^m(q_B,\cdot,q_B')$ can be enabled without requiring the robots to instantaneously jump from one location to another one. Thus, case (i) cannot happen i.e., there exists at least one symbol  $\sigma^{q_B,q_B'}$ that satisfies $b^{q_B,q_B'}$. Due to assumption (a) and since case (i) cannot happen, we get from Lemma \ref{lem:fragmentLTL} that $\delta_B^m(q_B,\cdot,q_B')$ satisfies the condition mentioned in Definition \ref{def:feas} and, therefore, case (ii) cannot happen either. Thus, $\ccalG$ collects all edges that correspond to transitions $\delta_B^m(q_B,\cdot,q_B')$ that can be enabled by the robots which contradicts the assumption that there exists a solution to Problem \ref{prob}.

\subsection{Proof Of Proposition \ref{thm:completeness}}

To prove that Algorithm \ref{alg:RRT} is complete, we need first to state the following Lemma. The proof is omitted due to space limitations.
%Given the above results, we can state the following result.
\begin{lem}\label{lem:binv}
Assume that at time $t$ the robots reach a state $q_B(t)\in\ccalV$ and design paths $\bbp_{j,t:T_j}$ to reach  $q_B^{\text{next}}\in\ccalV$.
%Assume that there are no regions $r_i$ and $r_j$, such that $r_i\subseteq r_j$. Then,  %% condition for feasibility
If the robots execute and update the paths $\bbp_{j,t:T_j}$, as per Section \ref{sec:exec}, and eventually they reach their goal regions $L_j^{\text{next}}$ then the transition from $q_B$ to $q_B^{\text{next}}$ will be activated. % at the time instant $T=\max_{j\in\ccalN^{\text{next}}} \{T_j\}$.
\end{lem}


\begin{proof}
For simplicity of notation, let $b^{\text{inv}}$ and $b^{\text{next}}$ denote the Boolean formulas that should be true to enable a transition from $q_B$ to $q_B$ and from $q_B$ to $q_B^{\text{next}}$, respectively. Once the robots reach $q_B(t)$, they coordinate to select symbol $\sigma^{\text{next}}$ that satisfies $b^{\text{next}}$. By assumption, all robots will eventually reach their assigned locations $L_{j}^{\text{next}}$ but not necessarily at the same time instant. When this happens, a time instant $T$, the symbol $\sigma^{\text{next}}$ that satisfies $b^{\text{next}}$ will be generated.
%By construction of Algorithm \ref{alg:RRT} there exists a time instant $T$ when the symbol $\sigma^{\text{next}}$ will be generated. Specifically, since the environment is static, we have that re-planning will be required a finite number of times. As a result, all robots $\ccalN^{\text{next}}$ will eventually reach their assigned locations $L_{j}^{\text{next}}$ and the symbol $\sigma^{\text{next}}$ will be generated. 
Thus, to show that at time $T$ the transition from $q_B$ to $q_B^{\text{next}}$ will be enabled, it suffices to show that $b^{\text{inv}}$ is satisfied for all $t'\in [t,T)$.\footnote{Note that the transition from $q_B$ to $q_B^{\text{next}}$ is, in general, a multi-hop transition; see \eqref{eq:run}. Thus, formally, if the length of the this transition is $K$ hops, then once the robots generate $\sigma^{\text{next}}$ they should stay idle at their current locations $K-1$ time steps to reach $q_B^{\text{next}}$. Thus, formally,  transition to $q_B^{\text{next}}$ will occur at the time instant $T+K-1$.}% since at time $T$ $q_B^{\text{next}}$ can be reached from $q_B(t)$. 


%To show this result, it suffices to show that there exists a time instant $T$ so that $b^{\text{inv}}$ is satisfied during the time interval $[t,T)$ and $b^{\text{inv}}$ is satisfied at time $T$. 


%The reason is that if $b^{\text{inv}}$ is satisfied, then the robots can always remain in $q_B(t)$ for all $t'\in [t,T)$. If the robots remain in $q_B(t)$ for all $t'\in [t,T)$, then at the time instant $T=\max_j \{T_j\}$, the transition from $q_B(t)$ to $q_B^{\text{next}}$ can be enabled, since at that time the robots $j\in\ccalN^{\text{next}}$ will generate the symbol $\sigma^{\text{next}}$ by construction of Algorithm \ref{alg:RRT}.\footnote{Note that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is, in general, a multi-hop transition. Thus, formally, if the length of the this transition is $K$ hops, then once the robots generate $\sigma^{\text{next}}$ they should wait $K-1$ time steps to reach $q_B^{\text{next}}$.} %[\red{explain the last sentence a bit more; add 1-2 sentences}].

%Recall that the symbol $\sigma^{\text{next}}$ satisfies the Boolean formula $b^{\text{next}}$ defined in \eqref{eq:b}. 
%
%Since $q_B(t)\in\ccalV$ and $\sigma^{\text{next}}\models b^{\text{next}}$, where $b^{\text{next}}$ is defined in \eqref{eq:b},
By construction of Algorithm \ref{alg:RRT}, we have that once the robots reach any state in $q_B\in\ccalV$, the corresponding Boolean formula $b^{q_B,q_B}$ is satisfied by definition of \eqref{eq:b}. Thus, at time $t$ the multi-robot state $\bbp(t)$ satisfies the Boolean formula $b^{\text{inv}}$ is satisfied. As a result, if all robots in the set $\ccalN^{\text{inv}}$ (i.e., the robots that appear in $b^{\text{inv}}$) remain idle, the Boolean formula $b^{\text{inv}}$ will remain satisfied. Recall that robots $j\in\ccalN^{\text{next}}$ navigate the environment by following paths design as per \eqref{eq:localProb} 
%and executing them as discussed in Section \ref{sec:exec}.
while it may hold that $\ccalN^{\text{next}}\cap\ccalN^{\text{inv}}\neq \emptyset$. In what follows, we show that $q_B(t)=q_B(t')$ for all $t'\in[t,T)$. %Let $R_j^t$ be the region $r_i$ that the robots lie in at the time instant $t$. If  robot $j$ does not belong to any region $r_i$, i.e., $L(\bbp_{j}(t))=\varnothing$, then $R_j^t$ is not defined i.e., $R_j^t=\varnothing$. 
%
To show this, first recall that the robots $j\in\ccalR^{\text{inv}}\subseteq\ccalN^{\text{inv}}$ stay idle by construction of Alg. \ref{alg:RRT} and, therefore, they cannot violate $b^{\text{inv}}$. Thus. it suffices to show that the robots $j\in\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}$, where $\bar{\ccalR}^{\text{inv}}=\ccalN^{\text{inv}}\setminus\ccalR^{\text{inv}}$ will not violate $b^{\text{inv}}$. To show this we consider two cases. 

First, assume that $\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}=\emptyset$. Then this means that all robots in $\ccalN^{\text{inv}}$ will stay idle and, therefore, $b^{\text{inv}}$ will not be violated. Second assume that there exist robots $j\in\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}$. By construction of the set $\bar{\ccalR}^{\text{inv}}$ we have that atomic predicates $\pi_j^{\ell_e}$ associated with robots $j\in\bar{\ccalR}^{\text{inv}}$ and for some regions $\ell_e$ appear in $b^{\text{inv}}$ only with a negation operator in front of them (i.e., in the following form $\neg\pi_j^{\ell_e}$). In other words, robots $j\in\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}$ will violate $b^{\text{inv}}$ only if they visit certain regions of interest as they move towards locations $\bbq\in\Omega$, where no atomic predicates are satisfied. Nevertheless, this is precluded by the first constraint in \eqref{eq:localProb} meaning that at time $T$ transition from $q_B(t)$ to $q_B^{\text{next}}$ will be activated. Finally, note that this result holds even if the robots execute their paths asynchronously, i.e., if the (continuous) time required to move from $\bbp_j(t)$ to $\bbp_j(t+1)$ is different across the robots. The reason is that (i) generation of $\sigma_{\text{next}}$ does not depend on the order where the robots arrive at their goal locations $L_{j}^{\text{next}}$, (ii) satisfaction of $b^{\text{inv}}$ cannot be affected by the asynchronous execution of paths $\bbp_{j,t:T_j}$,  $j\in\ccalN^{\text{next}}$. The latter is true because 
in $b^{\text{inv}}$, there are no Boolean variables associated with robots $j\in\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}$ and, therefore,
the (synchronous or asynchronous) actions of these robots does not play any role in satisfying $b^{\text{inv}}$. Also, as discussed before, the (synchronous or asynchronous) actions of the robots $j\in\bar{\ccalR}^{\text{inv}}$ cannot violate $b^{\text{inv}}$ as long as they avoid certain regions, which is guaranteed by construction of the paths completing the proof.\end{proof}




{\bf{Proof of Proposition \ref{thm:completeness}:}} To show this result it suffices to show that eventually the accepting condition of the NBA is satisfied, i.e., the robots will visit at least one the final NBA states $q_F$ infinitely often. 
Equivalently, as discussed on Section \ref{sec:dist}, it suffices to show that accepting edges $(q_B,q_B')\in\ccalE$, where $q_B,q_B'\in\ccalV$ are traversed infinitely often. 

First, consider an infinite sequence of time instants $\bbt=t_0,t_1,\dots,t_k,\dots$ where $t_{k+1}\geq t_k$, so that an edge in $\ccalG$, defined in Section \ref{sec:dist}, is traverses at every time instant $t_k$. Let $e(t_k)\in\ccalE$ denote the edge that is traversed at time $t_k$. Thus, $\bbt$ yields the following sequence of edges $\bbe=e(t_0),e(t_1),\dots,e(t_k)\dots$ where $e(t_k)=(q_B(t_{k}),q_B(t_{k+1}))$, $q_B(t_0)=q_B^{\text{aux}}$, $q_B(t_k)\in\ccalV$, and the state $q_B^{k+1}$ is defined based on the following two cases. 
%
If $q_B(t_k)\notin \ccalV_F$, then the state $q_B(t_{k+1})$ is closer to $\ccalV_F$ than $q_B(t_k)$ is, i.e., $d_F(q_B(t_{k+1}),\ccalV_F)=d_F(q_B(t_{k}),\ccalV_F)-1$, where $d_F$ is defined in \eqref{eq:distF}. If $q_B(t_{k})\in\ccalV_F$, then $q_B(t_{k+1})$  is selected so that an accepting edge originating from $q_B(t_{k})$ is traversed. By definition of $q_B(t_{k})$, the `distance' to $\ccalV_F$ decreases as $t_k$ increases, i.e., given any time instant $t_k$, there exists a time instant $t_k'\geq t_k$ so that $q_B(t_{k}')\in\ccalV_F$ and then at the next time instant an accepting edge is traversed. This means that $\bbe$ includes an infinite number of accepting edges. This sequence $\bbe$ exists by assumption (a). Note that if assumption (a) does not hold, Algorithm \ref{alg:RRT} cannot find a solution even if it exists.
%

Assume that there exists a solution to Problem \ref{prob}. Assume that the robots navigate the environment as per Algorithm \ref{alg:RRT} and update the graph $\ccalG$ by removing edges as described in Section \ref{sec:replan}. To show that Algorithm \ref{alg:RRT} is complete, it suffices to show that it can generate a infinite sequence of edges $\bbe$ as defined before.


%of edges in the graph $\ccalG$, defined in Section \ref{sec:dist}, defined as $\ccalE=e(0),e(t_1_,\dots,e(t_k)\dots$, that includes an infinite number of accepting edges associated with $q_F^{\text{loop}}\in\ccalQ_F^{\text{loop}}$ infinitely often, where $e(t_k)=(q_B(t_k-1),q_B^{k+1})$, $q_B^0=q_B^{\text{aux}}$, and the state $q_B^{k+1}$ is selected as discussed in Section \ref{sec:planning}. Specifically, if $q_B^k\neq q_F^{\text{loop}}$, then the state $q_B^{\text{next}}=q_B^{k+1}$ is selected so that it is closer to $q_F^{\text{loop}}$ than $q_B^k$ is, i.e., $d(q_B^{k+1},q_F^{\text{loop}})=d(q_B^{k},q_F^{\text{loop}})-1$. If $q_B^k= q_F^{\text{loop}}$, then $q_B^{k+1}$ is selected so that an accepting edge originating from $q_F^{\text{loop}}$ is traversed. 
%


We show that a sequence $\bbe$ exists by induction. Specifically, we show that if there exists a time instant $t_k$ when the robots reach an NBA state denoted by $q_B(t_k)\in\ccalV$ there exists a time instant $t_{k+1}\geq t_k$ when the robots will reach a new state $q_B(t_{k+1})=q_B^{\text{next}}\in\ccalV$ where $q_B(t_{k+1})$ satisfies the conditions discussed before. 
%
At time $t=0$, we have that $q_B(0)=q_B^{\text{aux}}\in\ccalV$. By construction of Algorithm \ref{alg:RRT} the robots select a new state $q_B^{\text{next}}$ that they should reach next in the same way as discussed before. 
%
%Let $\sigma^{\text{next}}$ be the symbol that the robots decided to generate to enable the transition from $q_B(0)$ to $q_B^{\text{next}}$. Paths $\bbp_{j,t:T_j}$ that should be followed to generate $\sigma^{\text{next}}$ are designed by solving \eqref{eq:localProb}.
%
Since  $q_B(0)\in\ccalV$ then due to Lemma \ref{lem:binv}, we have that if robot paths $\bbp_{j,t:T_j}$ that solve \eqref{eq:localProb} always exist, as the map is updated, i.e., the robots eventually reach their regions $L_j^{\text{next}}$, then transition from $q_B(t_0)$ to $q_B^{\text{next}}$ will be eventually enabled. 
%$\sigma^{\text{next}}$ satisfies the Boolean formula $b^{q_B(0),q_B^{\text{next}}}$ defined in \eqref{eq:b}, we have that the Boolean formula $b^{q_B^{\text{next}},q_B^{\text{next}}}$ is satisfied.
%
Note that \eqref{eq:localProb} is always feasible, as the map is updated, due to assumption (b); this also means that edges in the graph $\ccalG$ will be never deleted. Also, as the robots follow the paths as per Algorithm \ref{alg:RRT}, it will never hit an obstacle due to assumption (c). Particularly, by assumption (c) the robot is equipped with an omnidirectional sensor, as per \eqref{eq:sensor}. %, the robot will always be aware of all obstacles within range $R$. 
Thus, if the path $\bbp_{j,t:T_j}$ passes through an obstacle, robot $j$ will always detect it and will re-solve \eqref{eq:localProb} to update its path. 
%
Since \eqref{eq:localProb} is always feasible, we get that there exists a time instant $t_0\geq 0$ when the robots will reach a new state $q_B^{\text{next}}\in\ccalV$. The induction step follows. Assume that at a time instant $t_{k}$ the robots reach a state $q_B(t_{k})\in\ccalV$ from a state $q_B(t_{k-1})\in\ccalV$. Following the same logic as for $t_0$, we can show that there exists a time instant $t_{k+1}\geq t_k$ when the robots reach $q_B^{t_{k+1}}\in\ccalV$ completing the proof.



\subsection{Proof of Proposition \ref{thm:exist}}
By Assumption (a) we have that there exists an infinite sequence of edges $\bbe=e_0,e_1,\dots,e_k\dots$ in $\ccalG$ that includes an infinite number of accepting edges where, with slight abuse of notation,  $e_k=(q_B^k,q_B^{k+1})$, $q_B^k\in\ccalV$ for all $k\geq 0$. To show that a solution to Problem \ref{prob} exists, it suffices to show that there exists a sequence of paths in $\Omega$ that the robots can follow to enable all edges $e_k$. We show this by induction. % can be enabled without requiring the robots to instantaneously jump from one location to another or be in more than one location simultaneously while respecting the robot dynamics. We show this by induction. 

First, we focus on the transition $e_0=(q_B^0,q_B^1)$ where $q_B^0=q_B^{\text{aux}}$. By construction of $q_B^{\text{aux}}$, we have that the initial multi-robot state satisfies the Boolean formula $b^{q_B^0,q_B^0}$ associated with the self loop of $q_B^0$. Due to the fact that $e_0\in\ccalE$ we get that the corresponding transition $\delta_B^m(q_B^0,\cdot,q_B^1)$ is decomposable. Therefore there exist paths that can enable the transition from $q_B^0$ to $q_B^1$. Specifically, as shown in Lemma \ref{lem:binv}, such paths can be computed by solving local reachability problems as in \eqref{eq:localProb} where \eqref{eq:localProb} is always feasible by Assumption (b). Thus, eventually, the transition $e_0$ will  be enabled. The induction step follows. Assume that all edges $e_0$, $e_1, \dots,e_{k-1}$ have been enabled and paths that reach the state $q_B^k$  and activate the Boolean formula $b^{q_B^k,q_B^k}$ have been designed. Following the same logic as for the edge $e_0$, we can show that there exist paths that can enable the edge $e_k$ completing the proof. 

==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/proofs.tex <==
%In this section we provide the proof of Lemma \ref{lem:binv} required to prove that Algorithm \ref{alg:RRT} is complete. To prove this result, we need first to state the following results.

%First, we show that once the robots reach a DFA state $q_D^{\text{next}}$ they can remain in this state if they stay in their current configuration.

%\begin{lem}[Feasibility]\label{lem:feas}
%Assume that the robots reach a configuration $\bbp(t)$ that generates a word $\sigma=L(\bbp(t))$ which enables a transition to the DFA state $q_D^{\text{next}}$. Then, it holds that $\sigma\models b_{\text{inv}}$, where $b_{\text{inv}}$ is a Boolean formula that needs to be satisfied to remain in $q_D^{\text{next}}$. 
%\end{lem}

%\begin{proof}
%This result follows directly from the fact that the `next' operator is excluded from the syntax of the task specification language. Particularly, let $q_D^{\text{next}}$ denote the DFA state that the robots will reach from   $q_D^{\text{next}}$ if they stay put in $\bbp(t)$. In what follows, we show by contradiction that $q_{\text{next}}$ exists (i.e., staying in $\bbp(t)$ does not violate $\phi$) and  $q_D^{\text{next}}=q_D^{\text{next}}$. Assume that $q_D^{\text{next}}$ does not exist. This means that once the robots reach $\bbp(t)$ and the current DFA state becomes $q_D^{\text{next}}$, we have that $\delta(L(\bbp(t)),q_D^{\text{next}})=\varnothing$. This means that once the robots reach $\bbp(t)$ they should immediately leave it, beause otherwise the LTL formula is violated. This implies the existence of the `next' operator in the specification language which is not the case. Therefore, we conclude that $q_D^{\text{next}}$ exists.

%Next, we show that $q_D^{\text{next}}=q_D^{\text{next}}$. Assume $q_D^{\text{next}}\neq q_D^{\text{next}}$. This implies that once $L(\bbp(t))$ is generated and $q_D^{\text{next}}$ is reached, the robots should leave $\bbp(t)$ immediately in order to stay in $q_D^{\text{next}}$; otherwise $L(\bbp(t))$ will enable a subsequent transition to $q_D^{\text{next}}\neq q_D^{\text{next}}$. This also implies the existence of the `next' operator in the specification language which is not the case completing the proof.
%\end{proof}

%This implies that the same word $L(\bbp(t))$ enables first a transition from a DFA state $q_D$ to $q_D^{\text{next}}$ and second, once this happens, a transition from $q_D^{\text{next}}$ to $q_D^{\text{next}}$ is enabled immediately. This means that $q_D^{\text{next}}$ is a `dummy' state in the DFA which cannot happen 
%$\ccalR=\set{q\in\ccalQ_D~|~q=(L(\bbp(t)),q_D^{\text{next}})}$.
%
%if $\sigma\not\models b_{\text{inv}}$, then this means that once the robots reach the configuration $\bbp(t)$ and the current DFA state becomes $q_D(t)=q_D^{\text{next}}$, the robots should immediately leave from this configuration in order to stay in $q_D(t)$. This implies the existence of the `next' operator in the specification language which is not the case completing the proof.

%Next, let $\sigma_{\text{cur}}$ denote the word that the multi-robot system currently generates, i.e., $\sigma_{\text{cur}}=L(\bbp(t))$. Assume also that $\sigma_{\text{cur}}$ enables a transition from $q_D(t)$ to $q_D'\neq q_D(t)$. Let $b_{\text{inv}}$ be the Boolean formula that the robots should satisfy in order to remain in $q_D'$. Recall that in Lemma \ref{lem:feas}, we showed that  $\sigma_{\text{cur}}\models b_{\text{inv}}$, i.e., the robots can stay in the DFA state $q_D'$ as long as they stay idle. Next, we define the $\sigma_{\text{inv}}$ that is constructed by replacing in $\sigma_{\text{cur}}$ the maximum possible number of symbols with the empty string, so that $\sigma_{\text{inv}}$ still satisfies $b_{\text{inv}}$, i.e., $\sigma_{\text{inv}}\models b_{\text{inv}}$; see also Example \ref{ex4}. Let $\ccalR_{\text{inv}}$ be the robots that appear in $\sigma_{\text{inv}}$ and let $L_j^{\text{inv}}$ be the regions that robots $j\in\ccalR_{\text{inv}}$ have to belong to in order to generate $\sigma_{\text{inv}}$; see also Example \ref{ex4}. In the following lemma, we show that $\ccalR_{\text{inv}}$ and $\ccalR_{\text{next}}$ are disjoint sets.

%\begin{lem}[Conflict-free]\label{lem:confl}
%Let sets $\ccalR_{\text{inv}}$ be the set of robots that are responsible  and $\ccalR_{\text{next}}$ are disjoint. %If $\phi$ is satisfiable, then Algorithm \ref{alg:RRT} is conflict-free i.e., a robot $j\in\ccalR_{\text{inv}}$ that is required to stay idle will never have to solve \eqref{eq:localProb} to design a path towards a new region. 
%\end{lem}

%\begin{proof}
%Recall first that $\sigma_{\text{inv}}$ is the word with the minimum length that satisfies $b_{\text{inv}}$. This means that $\ccalR_{\text{inv}}$ does not involve `unnecessary' robots whose presence in a region $r_i$ does not affect the satisfaction of $b_{\text{inv}}$. The respective result also holds for $\sigma_{\text{next}}$. Note that this is important since otherwise, it is trivial to see that $\ccalR_{\text{inv}}$ and $\ccalR_{\text{next}}$ may not be disjoint.
%Given words $\sigma_{\text{inv}}$ and $\sigma_{\text{next}}$, assume that there exist a robot $j\in\ccalR_{\text{inv}}\cap\ccalR_{\text{next}}$. This means that according to the LTL task, robot $j$ has to be present in the region $L_j^{\text{inv}}$ for all time instants $t'\in[t,T)$ and in $L_{j}^{\text{next}}$ at the time instant $T$. Nevertheless, this is impossible to specify given that the `next' operator is not included in the task specification language.
%\end{proof}

 
%\begin{ex}[Construction of $\sigma_{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b_{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi_w^{r_2})\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$ (i.e., $\bbp_{j}\in r_1\cap r_2$). Then, we have that $\sigma_{\text{inv}}=\pi_j^{r_1}$, $\ccalR_{\text{inv}}=\set{j}$, and $L_j^{\text{inv}}=r_1$. Similarly, if $b_{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma_{\text{inv}}$ is an empty string and $\ccalR_{\text{inv}}=\emptyset$.
%\end{ex}
%, i.e., Algorithm \ref{alg:prune} will remove the multi-hop transition $q_B\rightarrow_B^K$ only if 

\begin{assumption}\label{as:cnf}
Let $b^{q_B,q_B^K}$ be a Boolean formula, defined in \eqref{eq:b}, written in conjunctive normal form (CNF) that enables a transition from $q_B$ to $q_B^K$. Assume that all literals in any given clause of $b^{q_B,q_B^K}$ are associated with only one robot, which is not necessarily the same across different clauses.
\end{assumption}

\begin{lem}\label{lem:fragmentLTL}
%Consider an LTL formula $\phi$ defined over atomic predicates $\pi_j^{\ell_i}$ where $j\in\ccalN$ and $\{\ell_i\}_{i\in\ccalL}$ denote disjoint regions of interest. 
Consider any finite run in the form of \eqref{eq:run}. Assume that there exists a symbol $\sigma^{q_B,q_B^K}$ that satisfies the corresponding Boolean formula $b^{q_B,q_B^K}$ defined in \eqref{eq:b}. Under Assumption \eqref{as:cnf}, the transition from $q_B$ to $q_B^K$ is always decomposable as per Definition \eqref{def:feas} unless this transition requires robots to instantaneously jump from one region of interest to another one which is impossible.
%%%
%Let $\bbp(t)$ and $\bbq_B(t)$ be the multi-robot and NBA state respectively at time $t$ and assume that $L(\bbp(t))\models b^{q_B(t),q_B(t)}$. Consider any transition $q_B(t)\rightarrow_B^K q_B'$, defined in Section \ref{sec:prune}.Let the corresponding Boolean formula $b^{q_B(t),q_B'}_K$ be written in conjunctive normal form (CNF). If every clause of $b^{q_B(t),q_B'}_K$ are associated with only one robot (not necessarily the same across different clauses), then Algorithm \ref{alg:prune} is not conservative.
%%%
%Assume that at time $t$ the current NBA state is $q_B(t)$ and the current multi-robot state $\bbp(t)$ satisfies $b_{q_B,q_B}$, i.e., $\bbp(t)\models b_{q_B,q_B}$. Let $b^{q_B,q_B'}_K$ denote the Boolean formula, defined in condition (i) Definition \ref{def:feas}, written in conjunctive normal form (CNF) that that needs to be satisfied to enable the NBA transition $q_B\rightarrow_B^K q_B'$. If the literals in any clause of $b^{q_B,q_B'}_K$ are associated with only one robot, then Algorithm \ref{alg:prune} is not conservative. % i.e., it will remove transition $q_B\rightarrow_B^K q_B'$ only if it can be enabled only if regions of interest were not disjoint.
%
%Also, let $b$ denote any Boolean sub-formula of $\phi$. Assume that there are no Boolean sub-formulas of the form $b=\vee_{j\in\ccalR}[\triangle_{r_{e_j}\in\ccalL}(\pi_j^{r_{e_j}})]$ with $|\ccalR|>1$ in $\phi$, where $\ccalR\subseteq\ccalN$ is set of robot indices and $\ccalL$ is set of regions of interest. %then the pruning approach as per Definition \ref{def:feas} is not conservative, i.e., only the non-physically realizable NBA transitions will be removed.
%
%Assume that the current NBA state is $q_B$ and the current multi-robot state $\bbp$ satisfies $b_{q_B,q_B}$. Then Algorithm \ref{alg:prune} has removed transitions originating from $q_B$ only if they can be enabled only if regions of interest were not disjoint.
%Consider any $q_B\rightarrow_B^K q_B'$ where $q_B,q_B'\in\ccalQ_B\setminus\hat{\ccalQ}_B$ and a. Under assumption (*), the pruning approach as per Algorithm \ref{alg:prune} is not conservative i.e., it will remove transitions that can be enabled only if regions of interest were not disjoint.
\end{lem}
\begin{proof}
%Consider the Boolean formula $b^{q_B,q_B^1}$ associated with any NBA transition $q_B\rightarrow_B q_B^1$ where $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$. Hereafter, 
%
%Recall that Definition \ref{def:feas} is not satisfied if transition from $q_B$ to $q_B'$ requires robots to jump from one region to another one  is conservative due to Def
%
Recall that Algorithm \ref{alg:prune} removes transitions in two cases. First, a transition $\delta_B(q_B\cdot,q_B')$, where $q_B,q_B'\in\ccalQ_B$, will be removed if $\Sigma^{q_B,q_B'}\neq\emptyset$, i.e., if this transition can be enabled only if at least one robot should be present in more than one location simultaneously. Second, a transition
$\delta_B(q_B\cdot,q_B^1)$, where $q_B\neq q_B^1$ is removed if it does not satisfy Definition \ref{def:feas} which, as discussed in Remark \ref{rem:conserv}, is conservative.

First, we show that condition (i) in Definition \ref{def:feas} is not conservative, in the sense that it only removes transitions that require robots to jump from one region of interest to another one (i.e., go from $r_e$ to $r_m$, $m\neq e$ with visiting any location $\bbq$ where $L(\bbq)=\varnothing$) or be physically present in more than one location which is impossible given that non-overlapping regions are considered. According to condition (i)-(A) of Definition \ref{def:feas}, a transition $\delta_B(q_B,\cdot, q_B^1)$, $q_B\neq q_B^1$, is feasible if there exists at least one symbol, denoted by $\sigma^{q_B,q_B^K}$ and a finite $K\geq 1$, so that $\sigma^{q_B,q_B^K}$ satisfies $b_{q_B,q_B^K}^K$, where
\begin{equation}\label{eq:bK}
    b_{q_B,q_B^K}=\underbrace{b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}}_{=b}\wedge b_{q_B^{K},q_B^{K}}.
\end{equation}
%Due to \eqref{eq:bqbqb2}, we can rewrite \eqref{eq:bK} as
%\begin{equation}\label{eq:bqbqb2}
%    b^{q_B,q_BK}=\bigwedge_{j=1}^N d_j^{q_b,q_B^K}.
%\end{equation}

Assume that condition (i)-(A) is not satisfied. There are three cases when this may happen:
(a) First, there may no states (other than the auxiliary states) with feasible self-loops, i.e., the Boolean formula $b_{q_B^{K}},q_B^{K}$ is not defined. This means that if the transition from $q_B$ to $q_B^1$ is activated then the only way to visit a final state is to instantaneously move/jump from one NBA state to another one, since no self-loops exist, unless condition (i)-(B) is true. In words, condition (i)-(B) requires that there exists a symbol that if it is repeated indefinitely after reaching $q_B$, a final state will be visited infinitely often. If (i)-(B) is not true, then in this case we have visiting a final state requires robots to `jump' from one region of interest to another one or be in more than one location simultaneously which is not possible. %Note that Then, clearly, if (B) is not satisfied either, there is no way after taking the transition from $q_B$ to $q_B^1$ to eventually visit a final state. [correctly removed regardless of B]
(b) Second, there may exist states with feasible self-loops but they cannot be reached, i.e., there does not exist a sequence of states $q_B^k$ towards any state $q_B^K$ that has a self-loop so that the corresponding $b$ formula is satisfied. Thus visiting states with self-loops requires the robot to jump from one region to another or be at more than one region simultaneously (in order to satisfy $b$ which is impossible. Thus, this means that after activating a transition from $q_B$ to $q_B^1$ (recall that $b_{q_B,q_B^1}$ does not require simultaneous presence in more than one location for any robot), the only way to visit a final state is to instantaneously move from one NBA state to another one which is not possible as discussed in (a) unless (B) is true.
%in order to reach a state and stay there (i.e., enable its corresponding self-loop) robots should be able to `jump' from one region of interest to another one or be in more than one location simultaneously which is not possible.
%final state In fact, this implies that there exists at least one %
%$b_{1,j}$ that cannot be satisfied, which may happen only if 
%robot $j$ that is required to be in more than one location simultaneously. If (B) does not hold either, there is no way after taking the transition from $q_B$ to $q_B^1$ to eventually visit a final state. [correctly removed]
(c) Third, there may exist states $q_B'$ with feasible self loops that can be reached while satisfying the respective $b$ but without satisfying $b_{q_B',q_B'}$. Following the same logic as above we conclude that after taking a transition from $q_B$ to $q_B^1$, the only way to visit a final state is to instantaneously move from one NBA state to another one which is not possible unless (B) is true.
Thus, we conclude that condition (i) is not conservative i.e., it will remove transitions from $q_B$ to $q_B^1$ that if activated then satisfying the accepting condition of the NBA requires the robots to jump from one region of interest to another one or be in more than one location simultaneously which is not possible. Note that this part of the proof does not rely in Assumption \ref{as:cnf}.

Second, we show that condition (ii) is not conservative if Assumption \ref{as:cnf} holds. To show this, first we express $b^{q_B,q_B'}$ in CNF, i.e., as a conjunction of $F$ Boolean formulas $b_f$, for some $F>0$, where $b_f$ is a disjunction of literals, i.e.,
\begin{equation}\label{eq:bqbqb}
    b^{q_B,q_B'}=\bigwedge_{f=1}^F b_f
\end{equation}
%Assume that all literals in a clause $b_f$ are associated with only one robot, for all $f\in\{1,\dots,F\}$. 
%In what follows, we show by contradiction that Algorithm \ref{alg:prune} is not conservative if every clause $b_f$ is associated with only one robot, for all $f\in\{1,\dots,F\}$.
By Assumption \ref{as:cnf} we have that every clause $b_f$ is associated with only one robot, for all $f\in\{1,\dots,F\}$. Let $\ccalF_j$ be a set that collects all indices $f\in\{1,\dots,F\}$ to formulas $b_f$ that are associated with robot $j$, where $\ccalF_j\cap\ccalF_i=\emptyset$, for all $i,j\in\ccalN$, by definition of $b_f$. Next we define the Boolean formula 
\begin{equation}\label{eq:dj}
    d_j^{q_b,q_B'}=\bigwedge_{j\in\ccalF_j}b_f,
\end{equation}
which is a conjunction of all Boolean formulas $b_f$ associated with robot $j$. Using \eqref{eq:dj} and the fact that $\ccalF_j\cap\ccalF_i=\emptyset$, for all $i,j\in\ccalN$, we can re-write \eqref{eq:bqbqb} as 
\begin{equation}\label{eq:bqbqb2}
    b^{q_B,q_B'}=\bigwedge_{j=1}^N d_j^{q_b,q_B'}.
\end{equation}
Thus, the Boolean formula $b^{q_B,q_B'}$ can be decomposed into local/decoupled sub-formulas $d_j^{q_b,q_B'}$. In other words, robot $j$ can make decisions to contribute to satisfaction of $b^{q_B,q_B'}$ independent from other robots by considering only the sub-formula $d_j^{q_b,q_B'}$. 

Due to the decomposition of the Boolean formulas as per \eqref{eq:bqbqb2}, we can apply condition (ii) of Definition \ref{def:feas} locally to each robot to prune the NBA as follows. %
For all symbols  $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}$, there should exist at least one of the symbols $\sigma^{q_B,q_B^K}_j$ that satisfy condition (i) and either (A) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^K}$. Note that since symbols $\sigma^{q_B,q_B^K}$ that satisfy condition (i) exist, this means $L_{j}^{q_B,q_B^K}$ is unique/well-defined for all robots $j\in\ccalR^{q_B,q_B^K}$. Assume that (ii) is not satisfied i.e., there exists at least one symbol $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}$ for which there are no $\sigma^{q_B,q_B^K}_j$ that satisfy either conditions (ii)-(A) or (ii)-B. This means that there exists $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B^K}\neq L_{j}^{q_B,q_B}$. Since $j\in\ccalR^{q_B,q_B}$, we have that transition towards the state $q_B$ was enabled because robot $j$ reached a region of interest $L_{j}^{q_B,q_B}$. Also, since $j\in\ccalR^{q_B,q_B^K}$, we get that transition from $q_B$ to $q_B^K$ will be enabled only if robot $j$ visits a region of interest denoted by $L_{j}^{q_B,q_B^K}$. By assumption $L_{j}^{q_B,q_B^K}\neq L_{j}^{q_B,q_B}$. Therefore, we conclude if condition (ii) is not satisfied then transition from $q_B$ to $q_B^K$ can be enabled only if robot $j$ keeps being in a region of interest $L_{j}^{q_B,q_B}$ until it reaches another region $L_{j}^{q_B,q_B^K}\neq L_{j}^{q_B,q_B}$, which is impossible given that all regions of interest are disjoint completing the proof.
%visiting the final states requires  this If (B) does not hold either, there is no way after taking the transition from $q_B$ to $q_B^1$ to eventually visit a final state. [correctly removed]
%
%(B.a) there are runs with loops but the loop does not include any final state (useless loop)
%(B.b) there are no runs 
%case (A.b) implies that there exists at least one $b_{1,j}$ that cannot be satisfied, which may happen only if robot $j$ is required to be in more than one location simultaneously. Then, this transition will be removed only if it does not satisfy (i-B). 
%case (A.c)
%
%b_{q_B,q_B^K}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}$. 
%
%
%$b_{q_B,q_B^1}$, $b_{q_B^k,q_B^{k+1}}$, for all $k\in\{1,\dots,K-1\}$, and $b_{q_B^K,q_B^{K}}$, while it does not satisfy $b_{q_B^k,q_B^{k}}$ (if it exists), for all $k\in\{1,\dots,K-1\}$.
%
%a transition $q_B\rightarrow_B^K q_B'$ is feasible if (i) for all symbols  $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}_j$ there exists at least one symbol denoted by $\sigma^{q_B,q_B^1}_j$ that enables a transition from $q_B$ to $q_B'$, i.e., $\sigma^{q_B,q_B'}_j\in\Sigma^{q_B,q_B^1}_j$ such that $\sigma^{q_B,q_B^1}_j\models d_{j,K}^{q_B,q_B'}$;
%\wedge_{k=1}^K d_j^{q_B^k,q_B^{k+1}}\wedge d_j^{q_B^K,q_B'}
%and 
%
%(ii) at least one of the symbols $\sigma^{q_B,q_B^1}_j$ that satisfy condition (ii) should satisfy either (a) $j\notin\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^1}$ or (b) $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^1}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^1}$.
%Specifically, following Definition \ref{def:feas}, a transition $(q_B,\cdot,q_B')$ is feasible if: (i) $\Sigma^{q_B,q_B}\neq \emptyset$ (i.e., $b^{{q_B,q_B}}$ is defined); (ii) for all symbols  $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}_j$ there exists at least one symbol $\sigma^{q_B,q_B'}_j\in\Sigma^{q_B,q_B'}_j$ such that $\sigma^{q_B,q_B'}_j\models d^{q_B',q_B'}_j$; and (iii) at least one of the symbols $\sigma^{q_B,q_B'}_j$ that satisfy condition (ii) should satisfy either (a) $j\notin\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ or (b) $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B'}=L_{j}^{q_B,q_B}$, where conditions (ii)-(iii) should hold for all robots $j$. In condition (ii), if $j\notin\ccalN_{q_B',q_B'}$, then $d^{q_B',q_B'}_j$ is not defined; in this case $\sigma^{q_B,q_B'}_j\models d^{q_B',q_B'}_j$ is trivially satisfied as robot $j$ does not play any role in satisfying $b^{q_B',q_B'}$.
%
%Using this result, in what follows we show that the proposed pruning method will remove NBA transitions only their activation requires overlapping regions. Assume that the transition $q_B\rightarrow_B^K q_B'$ does not satisfy conditions (i) and/or (ii). \textit{First}, assume that condition (i) is not satisfied, i.e., there do not exist any feasible symbols $\sigma^{q_B,q_B^1}_j\models d_{j,K}^{q_B,q_B'}$. This may happen only if $\Sigma^{q_B,q_B'}_j=\emptyset$ which means that $d^{q_B,q_B'}_j$ and, consequently, $b^{q_B,q_B'}$ requires robot $j$ to be present in more than one location simultaneously. %As a result, the transition $q_B\rightarrow_K^B q_B'$ cannot be enabled.
%(B) Assume that $\Sigma^{q_B,q_B'}_j\neq\emptyset$.
%Assume that for at least one symbol $\sigma^{q_B,q_B}_j\models d^{q_B,q_B}_j$, there do not exist $\sigma^{q_B,q_B'}_j$ such that $\sigma^{q_B,q_B'}_j\models d^{q_B',q_B'}_j$. This implies that once robot $j$ makes a certain observation as per the Boolean formula $d^{q_B,q_B'}_j$, it has to make another observation as per $d^{q_B',q_B'}_j$ at the next time instant. Nevertheless, this cannot happen as the `next' operator is excluded.
%
%Consider any transition $(q_B,\cdot,q_B')'$ with $\Sigma^{q_B,q_B}\neq \emptyset$ that does not satisfy conditions (ii) and/or (iii). \textit{First}, assume that condition (ii) is not satisfied. There are two cases under which condition (ii) is not satisfied: (A) assume there do not exist any symbols $\sigma^{q_B,q_B'}_j\in \Sigma^{q_B,q_B'}_j$. This may happen only if $d^{q_B,q_B'}_j$ and, consequently, $b^{q_B,q_B'}$ requires robot $j$ to be present in more than one location simultaneously.  (B) Assume that there exist at least one symbol $\sigma^{q_B,q_B'}_j\in \Sigma^{q_B,q_B'}_j$. Assume that for at least one symbol $\sigma^{q_B,q_B}_j\models d^{q_B,q_B}_j$, there do not exist $\sigma^{q_B,q_B'}_j$ such that $\sigma^{q_B,q_B'}_j\models d^{q_B',q_B'}_j$. This implies that once robot $j$ makes a certain observation as per the Boolean formula $d^{q_B,q_B'}_j$, it has to make another observation as per $d^{q_B',q_B'}_j$ at the next time instant. Nevertheless, this cannot happen as the `next' operator is excluded.
%
%
%Thus, a transition will be removed due to condition (i) only if at least one robot $j$ needs to be present in more than one location simultaneously. \textit{Second}, assuming that condition (i) is satisfied, we show by contradiction that condition (ii) is always satisfied unless it requires a robot to `jump' from one region of interest. Assume that (ii) is not satisfied. This means that $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B^1}\neq L_{j}^{q_B,q_B}$. Since $j\in\ccalR^{q_B,q_B}$, this means that transition towards the state $q_B$ was enabled because robot $j$ reached a region of interest $L_{j}^{q_B,q_B}$. Also, since $j\in\ccalR^{q_B,q_B^1}$, this means that transition from $q_B$ to $q_B^1$ will be enabled only if robot $j$ visits a region of interest denoted by $L_{j}^{q_B,q_B^1}$. By assumption $L_{j}^{q_B,q_B^1}\neq L_{j}^{q_B,q_B}$. Therefore, transition from $q_B$ to $q_B'$ will be enabled if robot $j$ keeps being in $L_{j}^{q_B,q_B}$ until it reaches $L_{j}^{q_B,q_B^1}$, which is impossible given that all regions of interest are disjoint completing the proof.
%once robot $j$ reaches a region of interest $L_j^{q_B,q_B}=r_e$, it has to stay within this region until another region of interest $L_j^{q_B,q_B'}=r_m$ is reached. This transition cannot be enabled in practice since disjoint regions of interest are assumed which contradicts the assumption that (iii) is not satisfied completing the proof. %If condition (iii) is not satisfied, then this means that there exists at least one robot $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. In other words, at least on robot $j$ has to instantaneously move from one region of interest to another one which is impossible which completes the proof.
%$\cap \Sigma^{q_B,q_B}_j$. This means that $\Sigma^{q_B,q_B'}_j\cap \Sigma^{q_B,q_B}_j=\emptyset$, i.e., once robot $j$ reaches a region required to 
%
%that do not satisfy condition (iii) but they are physically realizable. Since they do not satisfy (iii), this means that $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$, i.e., robot $j$ has to instantaneously move from one region of interest to another one which is impossible which completes the proof.
%
%If there are no Boolean sub-formulas of the form $b=\vee_{j\in\ccalR}[\triangle_{r_{e_j}\in\ccalL}(\pi_j^{r_{e_j}})]$ with $|\ccalR|>1$, then this means that to
\end{proof}
%(i.e. the only NBA transitions that will be removed are the ones that require a robot does not include any Boolean subformula of the form $\vee_{j\ccalR}(\pi_j)$

%Given the above results, we can state the following result.
\begin{lem}\label{lem:binv}
assume that at time $t$ the robots reach state $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$ and design paths $\bbp_{j,t:T_j}$ to reach  $q_B^{\text{next}}$.
%Assume that there are no regions $r_i$ and $r_j$, such that $r_i\subseteq r_j$. Then,  %% condition for feasibility
As the robots execute the paths $\bbp_{j,t:T_j}$, as per Section \ref{sec:exec}, the transition $q_B\rightarrow_B^K q_B^{\text{next}}$ will be activated at the time instant $T=\max_j T_j$.
\end{lem}


\begin{proof}
To show this result, it suffices to show that $b_{\text{inv}}$ is satisfied during the time interval $[t,T)$, where recall that $b_{\text{inv}}$ is the Boolean formula should be satisfied to enable a loop around $q_B(t)$. The reason is that if $b_{\text{inv}}$ is satisfied, then the robots can always remain in $q_B(t)$ for all $t'\in [t,T)$. If the robots remain in $q_B(t)$ for all $t'\in [t,T)$, then at the time instant $T=\max_j T_j$, the transition from $q_B(t)$ to $q_B^{\text{next}}$ will be enabled, since at that time the robots will generate the symbol $\sigma_{\text{next}}$ by construction of Algorithm \ref{alg:RRT} [\red{explain the last sentence a bit more; add 1-2 sentences}].

By construction of the pruned NBA, we have that when a new NBA state $q_B(t)$ is reached at time $t$, the corresponding Boolean formula $b_{\text{inv}}$ is satisfied (see condition (ii) in Definition \ref{def:feas}). As a result, if all robots in the set $\ccalN_{\text{inv}}$ (i.e., the robots that appear in $b_{\text{inv}}$) remain idle, the Boolean $b_{\text{inv}}$ will be satisfied. Nevertheless, robots $j\ccalN_{\text{next}}$ navigate the environment as per \eqref{eq:localProb} while it may hold that $\ccalN_{\text{next}}\cap\ccalN_{\text{inv}}$. In what follows, we show that $q_D(t)=q_D(t')$ for all $t'\in[t,T)$. %Let $R_j^t$ be the region $r_i$ that the robots lie in at the time instant $t$. If  robot $j$ does not belong to any region $r_i$, i.e., $L(\bbp_{j}(t))=\varnothing$, then $R_j^t$ is not defined i.e., $R_j^t=\varnothing$. 
%
To show this, first recall that the robots $j\in\ccalR_{\text{inv}}\subseteq\ccalN_{\text{inv}}$ stay idle by construction of Alg. \ref{alg:RRT} and, therefore, they cannot violate $b_{\text{inv}}$. Thus it suffices to show that the robots $j\in\bar{\ccalR}_{\text{inv}}\cap\ccalN_{\text{next}}$, where $\bar{\ccalR}_{\text{inv}}=\ccalN_{\text{inv}}\setminus\ccalR_{\text{inv}}$ will not violate $b_{\text{inv}}$. To show this we consider two cases. 

First, assume that $\bar{\ccalR}_{\text{inv}}\cap\ccalN_{\text{next}}=\emptyset$. Then this means that all robots in $\ccalN_{\text{inv}}$ will stay idle and, therefore, $b_{\text{inv}}$ will not be violated. Second assume that there exist robots $j\in\bar{\ccalR}_{\text{inv}}\cap\ccalN_{\text{next}}$. By construction of the set $\bar{\ccalR}_{\text{inv}}$ we have that atomic predicates $\pi_j^{r_e}$ associated with robots $j\in\bar{\ccalR}_{\text{inv}}$ and for some regions $r_e$ appear in $b_{\text{inv}}$ only with a negation operator in front of them (i.e., in the following form $\neg\pi_j^{r_e}$). In other words, robots $j\in\bar{\ccalR}_{\text{inv}}\cap\ccalN_{\text{next}}$ will violate $b_{\text{inv}}$ only if they visit certain regions of interest as they move towards locations $\bbq\in\Omega$, where no atomic predicate is satisfied. Nevertheless, this is precluded by the first constraint in \eqref{eq:localProb} completing the proof. 
\end{proof}

==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/proofs_short_Aug8.tex <==

%Given the above results, we can state the following result.
\begin{lem}\label{lem:binv}
Let $q_D(t)$ be the current DFA state and $\bbp_{j,t:T_j}$ be the paths that the robots designed to reach  $q_D^{\text{next}}$.
%Assume that there are no regions $r_i$ and $r_j$, such that $r_i\subseteq r_j$. Then,  %% condition for feasibility
As the robots execute the paths $\bbp_{j,t:T_j}$, as per Section \ref{sec:exec}, the only DFA transition that will be enabled is from $q_D(t)$ to $q_D^{\text{next}}$ at the time instant $T=\max_j T_j$.
\end{lem}


\begin{proof}
To show this result it suffices to show that $b_{\text{inv}}$ is satisfied during the time interval $[t,T)$, where recall that $b_{\text{inv}}$ is the Boolean formula that needs to satisfied so that the robots remain in $q_D(t)$. The reason is that if $b_{\text{inv}}$ is satisfied, then due to the deterministic nature of the DFA, it holds that the robots remain in $q_D(t)$ for all $t'\in [t,T)$. If the robots remain in $q_D(t)$ for all $t'\in [t,T)$, then at the time instant $T=\max_j T_j$, the transition from $q_D(t)$ to $q_D^{\text{next}}$ happens since the robots generate the symbol $\sigma_{\text{next}}$ which completes the proof.

By construction of the pruned DFA, we have that the first time, denoted by $t$, that the robots reach a state $q_D'$, i.e. $q_D(t)=q_D'$, then the corresponding Boolean formula $b_{\text{inv}}$ is satisfied (see condition (ii) in Definition \ref{def:feas}). In what follows, we show that $q_D(t)=q_D(t')$ for all $t'\in[t,T)$. %Let $R_j^t$ be the region $r_i$ that the robots lie in at the time instant $t$. If  robot $j$ does not belong to any region $r_i$, i.e., $L(\bbp_{j}(t))=\varnothing$, then $R_j^t$ is not defined i.e., $R_j^t=\varnothing$. 
%
To show this result, we consider two cases (i) $R_j^t=\varnothing$, for all robots $j\in\ccalR_{\text{next}}$; and (ii) $R_j^t\neq\varnothing$, for at least one robot $j\in\ccalR_{\text{next}}$. Recall that $R_j^t$ is the region $r_i$ that the robot $j$ lies in at the time instant $t$.

In the first case, if $R_j^t=\varnothing$, for all robots $j\in\ccalR_{\text{next}}$, then by construction of $\bbp_{j,t:T_j}$, we have that $L(\bbp(t'))=L(\bbp(t))$, for all $t'\in [t,T)$, since the robots $j\in\ccalR_{\text{next}}$ will not observe anything during the time interval $[t,T)$, by construction and execution of their paths (see constraint \eqref{constrLoc1}) and the robots $j\in\ccalR_{\text{inv}}$ stay idle at their current location. Then, since $L(\bbp(t))\models b_{\text{inv}}$ and due to the deterministic nature of the DFA, we have that the robots will remain in $q_D(t)$ for all $t'\in [t,T)$.

In the second case, we have that $R_j^t\neq\varnothing$, for at least one robot $j\in\ccalR_{\text{next}}$. In what follows, we show that a transition to another state $q_D'\neq q_D(t)$ will never happen at some $t'\in [t,T)$, as the robots $j\in\ccalR_{\text{next}}$ exit (asynchronously) the regions $R_j^t$. In other words, we show that the symbols $\sigma\neq\sigma_{\text{inv}}$, where $\sigma_{\text{inv}}=L(\bbp(t))$, that may be generated as the robots leave asynchronously their regions $R_j^t$ will not enable a transition from $q_D(t)$ to a new DFA state $q_D''$. 
%
%In what follows, we show that this can never happen. Specifically, we consider two cases. First, if $L(\bbp_j(t))=\varnothing$, for all $j\notin\ccalR_{\text{inv}}$, then it holds that for all time instants $t'\in [t,T_j^{-}]$ the robots only generate the word $\sigma_{\text{inv}}$ by construction of their paths. Due to the deterministic nature of the DFA, we have that the robots will remain in the DFA state $q_D(t)$, for all $t'\in [t,T_j^{-}]$. 
%
%Second, we consider the case where there exists at least one robot that is inside a region $R_j(t)$, i.e.,  $L(\bbp_j(t))\neq \varnothing$. 
To show this, we first rewrite $b_{\text{inv}}$ so that the atomic propositions that appear with a negation operator in front of them are separated from those that the negation operator does not exist in front of them. Specifically, using De Morgan's law, we re-write $b_{\text{inv}}$ in the following general form:
\begin{equation}\label{eq:inv1}
    b_{\text{inv}} = b_{\text{inv}}^{\text{goal}} \wedge [(\neg b_{\text{inv}}^{\text{avoid},1} )]\vee [(\neg b_{\text{inv}}^{\text{avoid},2})],
\end{equation}
%\red{[++more explanation on the subformuals++say that $b_{\text{inv}}$ exists because next operator does not exist]}
where the Boolean formulas $b_{\text{inv}}^{\text{goal}}$, $b_{\text{inv}}^{\text{avoid},1}$, and $b_{\text{inv}}^{\text{avoid},2}$ are defined so that the negation operator does not appear in front of any atomic proposition that comprise them. Since $\sigma_{\text{inv}}\models b_{\text{inv}}$ we have that either (i) $\sigma_{\text{inv}}\not\models b_{\text{inv}}^{\text{avoid},2}$, or (ii) $\sigma_{\text{inv}}\models b_{\text{inv}}^{\text{goal}} \wedge [(\neg b_{\text{inv}}^{\text{avoid},1} )]$ (or both). In case (i), the exit of robots from their regions $R_j^t$ means that symbols in $\sigma_{\text{inv}}$ are replaced with the empty string giving rise to a new symbol $\sigma$. 

Due to Lemma \ref{lem:logic}, we have that if $\sigma_{\text{inv}}\not\models b_{\text{inv}}^{\text{avoid},2}$ then $\sigma\not\models b_{\text{inv}}^{\text{avoid},2}$ or, equivalently $\sigma\models b_{\text{inv}}$ which means that the robots remain in $q_D(t)$ due to the deterministic structure of the DFA. 
%
For the same reason, in case (ii), if $\sigma_{\text{inv}}\models b_{\text{inv}}^{\text{goal}} \wedge [(\neg b_{\text{inv}}^{\text{avoid},1} )]$, we get that $\sigma\not\models b_{\text{inv}}^{\text{avoid},1}$. In case (ii), we also have that $\sigma\models b_{\text{inv}}^{\text{goal}}$, since the robots in $\ccalR_{\text{next}}$ are not responsible for generating the word $\sigma_{\text{inv}}$ (i.e., atomic propositions of the form $\pi_j^{r_i}$, where $j\in\ccalR_{\text{next}}$, do not exist in $b_{\text{inv}}^{\text{goal}}$) or if they are, then it suffices to remain put (see the third requirement in Definition \ref{def:feas}), as they do by construction of Algorithm \ref{alg:RRT}. Therefore, robots $j\in\ccalR_{\text{next}}$ cannot violate $b_{\text{inv}}^{\text{goal}}$. Thus in case (ii), we also get $\sigma\models b_{\text{inv}}$ which means that the robots remain in $q_D(t)$ due to the deterministic structure of the DFA for all $t'\in [t,T)$. At the time instant $T$, the robots $j\in\ccalR_{\text{next}}$ synchronously satisfy $L(\bbp_j(T))=\pi_j^{L_j^{\text{next}}}$ and the word $\sigma_{\text{next}}$ is generated enabling the transition from $q_D(t)$ to $q_D^{\text{next}}$ completing the proof.%. Note that $L(\bbp_j(T))=\pi_j^{L_j^{\text{next}}}$ is possible, is that there 
\end{proof}

==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/sim.tex <==

%\begin{figure}
%    \centering
%     \includegraphics[width=0.5\linewidth]{figures/Horizon_VS_R_VS_NumRobots.png}
%    \caption{Effect of the sensing range $R$ on the terminal horizon $H$ that solves \eqref{eq:Prob2}.}
%    \label{fig:horizon}
%\end{figure}

\begin{figure*}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[$t=315$]{
    \label{fig:315}
  \includegraphics[width=0.3\linewidth]{figures/t315.pdf}}
  \subfigure[$t=342$]{
    \label{fig:342}
  \includegraphics[width=0.3\linewidth]{figures/t342.pdf}}
    \subfigure[$t=411$]{
    \label{fig:411}
  \includegraphics[width=0.3\linewidth]{figures/t411.pdf}}
  \caption{Case $N=1$, $R=0.3$: Figures \ref{fig:315}-\ref{fig:411} illustrate the robot trajectory while aiming to satisfy $\Diamond(\pi_1^{\ell_5}\vee\pi_1^{\ell_4})$, i.e., to visit either region $\ell_5$ or $\ell_4$. At time instant $t=315$ (Fig. \ref{fig:315}) the robot is heading towards $\ell_5$ and at $t=342$ (Fig. \ref{fig:342}) it realizes, based on the constructed occupancy grid map, that $\ell_5$ is surrounded by obstacles and, therefore, not reachable. As a result, it moves towards $\ell_4$ ((Fig. \ref{fig:411})) and arrives there at $t=411$. The blue circle denotes the sensing range and rhe red squares stands for the grid cells of the map $M(t)$ that are occupied by obstacles. The gray region corresponds to unknown obstacles. %Figure \ref{fig:effect} illustrates the effect of the sensing radius on the terminal horizon.
  }
  \label{fig:env1}
\end{figure*}


\begin{table*}[t]
\caption{Scalability Analysis-Comparative Results}
\label{tab:scale}
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
      & \multicolumn{2}{c|}{Average Re-planning Time (secs)} & \multicolumn{3}{c|}{Algorithm \ref{alg:RRT}} \\ \hline
      Number of Robots   & Algorithm \ref{alg:RRT}        & STyLuS         & Local Map Update (secs)  & $t_F^1$(iteration/time(hrs))  & $t_F^2$(iteration/time(hrs))  \\ \hline
N=1   & 0.05                   & 4.12        & 0.007                                               &    883~/~0.012               & 1065~/~0.015               \\ \hline
N=20  & 0.03                   & 313.69     & 0.007                                               &      952~/~0.17               &   1032~/~0.18                  \\ \hline
N=100 & 0.03                   & 1349.54        &0.009                                               &    1088~/~0.49                 &   1124~/~0.57                  \\ \hline
N=200 & 0.04                   & 2883.52        & 0.01                                              &   1028~/~1.13                  &    1067~/~1.23                 \\ \hline
N=500 & 0.05                   & 9271.57        & 0.008                                              & 1032~/~2.7                    & 1070~/~2.9                     \\ \hline
\end{tabular}
\end{table*}

In this section, we present simulations and hardware experiments that illustrate the efficiency of the proposed algorithm. Simulations have been implemented using MATLAB R2016b on a computer with Intel Core i7 3.1GHz and 16Gb RAM. \red{to be added: gazebo simulations}

%In this section, we present simulations and experiments that illustrate the efficiency of the proposed algorithm. 

\subsection{Numerical Experiments}\label{sec:sim1}
{\bf{Map-based Planning in Unknown Environments with Unreachable Regions:}} 
%vs Map-free
In what follows, we consider a single robot with differential drive dynamics equipped with a sensor of sensing range $R=1.2$. The robot resides in a $10\times10$ environment shown in Figure \ref{fig:env1} and is tasked with a surveillance mission that requires to visit regions of interest eventually or infinitely often
while always avoiding obstacles. This task is captured by the following LTL formula
\begin{equation}\label{task1}
 \phi= (\bigwedge_{e=1}^{2}\square\Diamond\xi_e)\wedge(\bigwedge_{e=3}^6\Diamond\xi_e)\wedge(\neg\xi_3\ccalU\xi_4)\wedge(\square\neg\xi_{\text{obs}})
\end{equation}
where $\xi_e$ is a Boolean formula that requires the robot to visit a specific regions of interest, for all $e\in\{1,\dots,6\}$, and $\xi_{\text{obs}}$ is true if the robot hits any obstacle. In particular, the Boolean formulas $\xi_e$ are defined as: (i) $\xi_1=(\pi_1^{\ell_6}\vee\pi_1^{\ell_3})$; (ii) $\xi_2=\pi_1^{\ell_1}$; (iii) $\xi_3=\pi_1^{\ell_2}$; (iv) $\xi_4=(\pi_1^{\ell_5}\vee\pi_1^{\ell_4})$; (v) $\xi_5=\pi_1^{\ell_8}$; and (vi) $\xi_6=\pi_1^{\ell_9}$. In words, \eqref{task1} requires (a) the Boolean formulas $\xi_1$ and $\xi_2$ to be satisfied infinitely often, (b) the Boolean formulas $\xi_3$, $\xi_4$, $\xi_5$, and $\xi_6$ to be satisfied eventually, (c) never satisfy $\xi_3$ until $\xi_4$ is satisfied, and (d) always avoid obstacles. This formula corresponds to a NBA with $14$ states and $61$ transitions. The corresponding pruned automaton has $37$ transitions while all of them are decomposable; see Definition \ref{def:feas} and Proposition \ref{lem:fragmentLTL}. The runtime to prune this automaton was $0.15$ seconds approximately. 

Figure \ref{fig:env1} illustrates the benefit of using online learned maps for planning in unknown environments. Specifically, incorporating mapping into the control loop allows robots to reason about the environment and make appropriate control decisions to accomplish the assigned task which would be quite challenging using map-free approaches e.g., \cite{guzzi2013human,bansal2019combining}
Particularly, Figure \ref{fig:env1} shows the trajectory that the robot follows to eventually satisfy $\xi_1=(\pi_1^{\ell_5}\vee\pi_1^{\ell_4})$ that requires robot $1$ to visit either location $\ell_5$ or $\ell_4$. Observe in Figure \ref{fig:env1} that $\ell_5$ is surrounded by obstacles and, therefore, it is not accessible. Initially, robot $1$ is moving towards $\ell_5$ and as it builds the map of the environment it realizes that $\ell_5$ is not reachable. When this happens, a new symbol that satisfies $\xi_1$ is selected and, therefore, robot $1$ decides to move towards $\ell_4$. A similar behavior is observed when the Boolean formula $\xi_1=(\pi_1^{\ell_6}\vee\pi_1^{\ell_3})$ needs to be satisfied. 

{\bf{Scalability Analysis:}} Next, we examine the performance of Algorithm \ref{alg:RRT} with respect to the number of robots and we provide comparative simulation studies against state-of-the-art centralized algorithms \cite{kantaros2018text,guo2013revising} that can be used for re-planning as the map of the environment is continuously learned. 

We consider a team of $N\in\{1,20,100,200,500\}$ robots with differential drive dynamics that reside in the environment shown in Figure \ref{fig:env1} while all robots are equipped with omnidirectional sensors of limited range $R=1.2$. The robots are tasked with accomplishing the task captured in \eqref{task1}. The difference is that the Boolean formulas $\xi_e$ require collaboration between multiple-robots. For instance, when $N=20$, we have that $\xi_1=\wedge_{j=1}^{15}(\pi_j^{\ell_6}\vee\pi_j^{\ell_3})$ which requires all robots with index $j\in\{1,\dots, 15\}$ to visit either region $\ell_3$ or $\ell_6$ and $\xi_2=\wedge_{j=8}^{20}(\pi_j^{\ell_2}\vee\pi_j^{\ell_3})$ which requires all robots with index $j\in\{8,\dots, 20\}$ to visit either region $\ell_2$ or $\ell_3$. 

Table \ref{tab:scale} summarizes the scalability analysis of the proposed algorithm. Specifically, the first column shows the number of robots, the second column shows the average time required for a robot to design a new path as the map is updated. To design paths we solve \eqref{eq:localProb} using the $\text{A}^*$ algorithm \cite{russell2002artificial}. Specifically, we represent the learned occupancy grid map, which consists of $10,000$ cells, as a graph and we apply $\text{A}^*$ on it to design paths towards the goal regions. Then, we synthesize controllers to follow the designed path. 
%
Note that the runtime to design new paths ranges between $0.03$ and $0.06$ seconds showing that Algorithm \ref{alg:RRT} can design new paths very fast for large-scale multi-robot systems with hundred of robots due to its decentralized nature. The third collumn shows the average runtime required if existing centralized methods are used for replanning \cite{guo2013revising,kantaros2018text}. Specifically, \cite{guo2013revising} employs partially known transition systems to model the interaction of the robot and environment which are updated as the environment is discovered. Motion plans are synthesized by composing the transition systems with the NBA giving rise to a product automaton. When the transition system is updated, the product automaton is locally updated and new paths are designed by computing new paths in the product automaton from the current product state to a final product state. To compare Algorithm \ref{alg:RRT} against this approach, we use a graph-based representation of the occupancy grid map as the transition system. Our implementation of \cite{guo2013revising} required more than $1$ hour to design a path over the product automaton for a single-robot system and ran out of memory for case studies with more than one robot. To enhance \cite{guo2013revising}, we integrate it with STyLuS* \cite{kantaros2018text}, a recently proposed temporal logic planning method that scales well with the number of robots. Specifically, we use \cite{kantaros2018text} to design paths, instead of building a product automaton and computing paths over it. The third column in Table \ref{tab:scale} shows the average runtime required for STyLuS* to design new paths. To compute this runtime, we consider cases where $q_B(t)=q_B^0$, i.e., the robots are still in the initial NBA state, and new paths towards a final NBA state need to be computed as in \cite{guo2013revising}. Observe in the third column of Table \ref{tab:scale} that STyLuS* can also handle large-scale multi-robot systems but the runtime required for replanning using Algorithm \ref{alg:RRT} is significantly smaller due to its decentralized nature and the decomposition of the LTL task into `smaller' and local tasks.

The fourth column shows the average time required per robot to update the map as per \eqref{eq:updMap}. The fifth and sixth column present the number of discrete time instants required to visit a final NBA state for the first and the second time respectively. These columns also include the corresponding total runtime required by Alg. \ref{alg:RRT}. Note that Alg. \ref{alg:RRT} has been implemented on a single computer and, therefore, control decisions are made sequentially, instead of in parallel, across the robots which explains why the runtime increases significantly as the number of robots increases.  




% ----------- simulation of N=50 robots ------------
%Moreover when $N=50$, we divide the robots into $9$ sub-teams $\ccalT_m$. Then, the specification $\phi$ requires (i) the sub-team $\ccalT_1$ to visit either the hostage $8$ or $5$ and the sub-team $\ccalT_2$ to visit either the hostage $7$, $4$, or $3$ ($\xi_1$); then %
%(ii) $\ccalT_3$ to visit either $7$ or $4$ and $\ccalT_4$ to visit $5$ ($\xi_2$); then (iii) $\ccalT_5$ to visit $1$ and $\ccalT_5$ to visit either $2$ or $6$ ($\xi_3$); then (iv) $\ccalT_6$ to visit $3$ and $\ccalT_7$ to visit either $6$ ($\xi_4$); then (v) $\ccalT_8$ to visit $4$ and $\ccalT_9$ to visit either $5$, $7$, or $8$ ($\xi_5$);
%
%while $\square\neg\xi_6$ requires teams $\ccalT_1$ and $\ccalT_2$ to always avoid hostages $1$ and $2$ respectively, since they carry supplies that are dangerous to them. After pruning the corresponding DFA, we get that $d(q_0,q_F)=5$, i.e., the assigned task is feasible. Specifically, to follow the shortest path that connects $q_0$ to $q_F$, 
%
%denoted by $\bbq_D=q_0,q_1,q_2,q_3,q_4,q_F$ the following requirements need to be met (a) satisfaction of (i) to reach $q_1$ from $q_0$, (b) satisfaction of (ii) to reach $q_2$ from $q_1$, (c) satisfaction of (iii) to reach $q_3$ from $q_2$, (d) satisfaction of (iv) and (v) at the same time to reach $q_4$ from $q_3$, and (e) satisfaction of $\xi_{\text{exit}}$ to reach $q_F$ from $q_4$. Note that the teams $\ccalT_6$, $\ccalT_7$, $\ccalT_8$, and $\ccalT_9$ do not share any common robots and, therefore, simultaneous satisfaction of (iv) and (v) to reach $q_4$ from $q_3$ is feasible; see Def. \ref{def:feas}.
%----------------------------------------------------
%
%


{\bf{Effect of Sensing Range:}}  In our simulations, we consider a team of $N\in\{1,5,10,25, 50\}$ robots with differential drive dynamics that reside in an unknown $10\times 10$ environment; see Fig. \ref{fig:340}. The robots are equipped with omnidirectional sensors of limited range $R\in\set{0.3,0.75,1.1, 2}$. %Note that the sensing range $0.3$ is significantly smaller than the dimension of the environment to model visually-degraded areas \cite{khattak2019visual}.
%
The robots are tasked with providing delivery services to known locations, in a user-specified order, while always avoiding obstacles and dangerous regions. Once and only when services are provided, the robots should exit the building. This task is captured by the following LTL formula
%$\phi=\Diamond(\xi_1\wedge\Diamond(\xi_2\wedge\Diamond(\xi_3\wedge(\Diamond\xi_4 \wedge (\Diamond\xi_5))))) \wedge(\wedge_{e\in\set{1,2,3,4,5}} (\neg \xi_{\text{exit}}\ccalU \xi_e)) \wedge (\square\neg \xi_6) \wedge (\square\neg \xi_{\text{obs}})$
\begin{align}\label{eq:task}
    \phi&=\Diamond(\xi_1\wedge\Diamond(\xi_2\wedge\Diamond(\xi_3\wedge(\Diamond\xi_4 \wedge (\Diamond\xi_5))))) \wedge\nonumber \\&\wedge (\square\neg \xi_6) \wedge (\square\neg \xi_{\text{obs}}) \wedge (\Diamond\square\xi_{\text{exit}})
\end{align}
where $\xi_e$ is a Boolean formula that requires a sub-team of robots to visit a specific region to provide e.g., supplies, for all $e\in\{1,\dots,6\}$, while $\xi_{\text{exit}}$ is true if all robots visit the exit of the building. For instance, when $N=1$, the Boolean formulas $\xi_e$ are defined as: (i) $\xi_1=(\pi_1^8\vee\pi_1^5)$; (ii) $\xi_2=\pi_1^7$; (iii) $\xi_3=\pi_1^4$; (iv) $\xi_4=(\pi_1^1\vee\pi_1^2)$; (v) $\xi_5=\pi_1^6$;  and (vi) $\square\neg \xi_6$ requires the robot to always  keep a distance of at least $0.3$ from region $3$. This LTL formula corresponds to a NBA with $17$ states $103$ transitions while the pruned automaton has $43$ transitions.
%
Figure \ref{fig:340} depicts the trajectory that a robot follows to reach $\ell_7$ as it learns the occupancy grid map through a sensor with a range $R=0.3$. Figure \ref{fig:effect} shows that as the sensing range $R$ increases, the total number of discrete time instants required to visit a final state for the first time decreases, since the larger the sensing range, the faster the robots can learn the map of the environment.  The simulation videos can be found in \cite{icra20_video}. 


\begin{figure}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
  \includegraphics[width=0.8\linewidth]{figures/340.png}
  \caption{Case $N=1$, $R=0.3$: Figure \ref{fig:340} illustrate the robot position (discs) and actions (arrows) while it is heading towards region $7$. The green circle denotes the sensing range. At time $t=190$ the robot is not aware of the horizontal obstacle that is between it and region $7$. As a result it moves toward the obstacle, until it is fully discovered. Then, a new obstacle-free path is eventually discovered to reach region $7$ ($t=340$). The red squares stands for the grid cells of the map $M(t)$ that are occupied by obstacles. %Figure \ref{fig:effect} illustrates the effect of the sensing radius on the terminal horizon.
  }
  \label{fig:340}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/HorizonVSSensing.png}
  \caption{Effect of sensing range. %Figure \ref{fig:effect} illustrates the effect of the sensing radius on the terminal horizon.
  }
 \label{fig:effect}
\end{figure}

% ----------- simulation of N=50 robots ------------
%Moreover when $N=50$, we divide the robots into $9$ sub-teams $\ccalT_m$. Then, the specification $\phi$ requires (i) the sub-team $\ccalT_1$ to visit either the hostage $8$ or $5$ and the sub-team $\ccalT_2$ to visit either the hostage $7$, $4$, or $3$ ($\xi_1$); then %
%(ii) $\ccalT_3$ to visit either $7$ or $4$ and $\ccalT_4$ to visit $5$ ($\xi_2$); then (iii) $\ccalT_5$ to visit $1$ and $\ccalT_5$ to visit either $2$ or $6$ ($\xi_3$); then (iv) $\ccalT_6$ to visit $3$ and $\ccalT_7$ to visit either $6$ ($\xi_4$); then (v) $\ccalT_8$ to visit $4$ and $\ccalT_9$ to visit either $5$, $7$, or $8$ ($\xi_5$);
%
%while $\square\neg\xi_6$ requires teams $\ccalT_1$ and $\ccalT_2$ to always avoid hostages $1$ and $2$ respectively, since they carry supplies that are dangerous to them. After pruning the corresponding DFA, we get that $d(q_0,q_F)=5$, i.e., the assigned task is feasible. Specifically, to follow the shortest path that connects $q_0$ to $q_F$, 
%
%denoted by $\bbq_D=q_0,q_1,q_2,q_3,q_4,q_F$ the following requirements need to be met (a) satisfaction of (i) to reach $q_1$ from $q_0$, (b) satisfaction of (ii) to reach $q_2$ from $q_1$, (c) satisfaction of (iii) to reach $q_3$ from $q_2$, (d) satisfaction of (iv) and (v) at the same time to reach $q_4$ from $q_3$, and (e) satisfaction of $\xi_{\text{exit}}$ to reach $q_F$ from $q_4$. Note that the teams $\ccalT_6$, $\ccalT_7$, $\ccalT_8$, and $\ccalT_9$ do not share any common robots and, therefore, simultaneous satisfaction of (iv) and (v) to reach $q_4$ from $q_3$ is feasible; see Def. \ref{def:feas}.
%----------------------------------------------------
%


%Note that an alternative approach to solve the considered planning problem in unknown environments is to use existing abstraction-free approaches for LTL planning \cite{vasile2013sampling,luo2019abstraction} to continuously update the robot paths as the map of the environment is learned. Nevertheless, such methods require searching over a large product automaton space to design paths that reach the final DFA state, a task that is computationally challenging to perform at runtime. To the contrary, the proposed method is more efficient as it searches over only the physical state-space to design paths that solve reachability planning problems; see \eqref{eq:localProb}. %that reach DFA states that are one-hop away from the current state.

\subsection{Hardware Experiments}
The proposed reactive algorithm was also evaluated experimentally to test its efficiency in real-time re-planning and reactivity. Specifically, Alg. \ref{alg:RRT} was implemented in MatLab with ROS and run on the Scarab platform developed at the University of Pennsylvania \cite{michael2008experimental}. The Scarab is a differential drive robot equipped with a Hokuyo UTM-30LX scanning laser that can obtain range measurements in a $270^0$ field-of-view up to a distance of $30$m and an Intel RealSense camera with a $180^0$ field-of-view. Laser-based sensing is used for robot localization and for building an occupancy grid map using the gmapping ROS package implementing the SLAM approach presented in \cite{grisetti2007improved}. A video with the conducted experiments can be found in \cite{icra_exp}. \red{[videos to  be updated]}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.95
    \linewidth]{figures/env1rbt.jpg}
    %\subfigure[]{
    %\includegraphics[width=0.95
    %\linewidth]{figures/env1rbt.jpg}}
    %    \subfigure[]{
    %\includegraphics[width=0.95
    %\linewidth]{figures/env2rbt.jpg}}
    \caption{Experiment setup: A differential drive robot equipped with a LiDAR sensor navigates indoor environments with unknown and static obstacles.}
    \label{fig:exp}
\end{figure}
%to accomplish a complex mission while adapting planning to the continuously learned map
{\bf{LiDAR-based \& Map-based Planning:}} First, we validated Alg. \ref{alg:RRT} in two complex indoor environments with \textit{unknown} and \textit{static} obstacles shown in Figure \ref{fig:exp}. The robot is responsible for accomplishing a surveillance task captured by the following LTL formula: 
\begin{align}\label{task3}
    \phi=&\Diamond(\pi_1^{\ell_4})\wedge\Diamond(\pi_1^{r_1})\wedge\Diamond(\pi_1^{r_2}\vee\pi_1^{r_5})\wedge\Diamond(\pi_1^{r_6}\vee\pi_1^{r_4})\nonumber\\& \wedge\Diamond(\pi_1^{r_7}\vee\pi_1^{r_5})\wedge (\neg \pi_1^{r_1}\ccalU \pi_1^{r_3})\wedge(\square \neg \xi^{\text{obs}}),
\end{align}
The task in \eqref{task3} requires the robot to eventually visit the locations $\ell_4$, $\ell_1$, either $\ell_2$ or $\ell_5$, either $\ell_6$ or $\ell_4$, either $\ell_7$ or $\ell_5$ and never visit $\ell_1$ until $\ell_3$ is visited while always avoiding the a priori unknown obstacles. Observe in Figure \ref{fig:exp} that obstacles can be both convex and non-convex. 
To ensure that the robot paths never go too close to the obstacles, paths are designed as per \eqref{eq:localProb} after inflating the obstacles. As anticipated, the few failures we recorded were associated with the inability of the SLAM approach to accurately localize the robot in long missions. 

%certain regions of interest while always avoiding obstacles. Note that in this experiment setup, we do not consider an omnidirectional sensor as required in Proposition \ref{thm:completeness}; nevertheless, the robot successfully accomplished the assigned mission in two different environments. 
%
%Second, we also considered \textit{unknown} and \textit{dynamic/unexpected} obstacles. Recall that Alg. \ref{alg:RRT} is specifically designed for environments with static obstacles; the same also holds for the theoretical guarantees provided in Section \ref{sec:complOpt}. Here, we present preliminary experimental results that show that Alg. \ref{alg:RRT} can be applied to dynamic environments as well. To this end, to account for unknown and dynamic obstacles, we solve the point-to-point navigation problem \eqref{eq:localProb} using the motion planning algorithm proposed in \cite{guzzi2013human}; note that \cite{guzzi2013human} does not require building a map of the environment. In this set of experiments, we consider two robots that need to coordinate to accomplish a collaborative task while also avoiding collisions with each other. %Finally, note that in this experiment, the robots are allowed to move asynchronously. 

%the robot successfully accomplished the assigned mission, the robot is not equipped with omnidirectional sensor
%Unlike the simulation results and the assumptions of Proposition \ref{thm:completeness}, the sensor is imperfect while there is localization error that grows over time. The latter may result in hitting obstacles especially in long-horizon missions. To mitigate this issue, we inflate the detected obstacles before applying Alg. \ref{alg:RRT}.

%Second, we also considered \textit{unknown} and \textit{dynamic} obstacles. Recall that Alg. \ref{alg:RRT} is specifically designed for environments with static obstacles; the same also holds for the theoretical guarantees provided in Section \ref{sec:complOpt}. Here, we present preliminary experimental results that show that Alg. \ref{alg:RRT} can be applied to dynamic environments as well. To this end, to account for unknown and dynamic obstacles, we solve the point-to-point navigation problem \eqref{eq:localProb} using the motion planning algorithm proposed in \cite{guzzi2013human}; note that \cite{guzzi2013human} does not require building a map of the environment. In this set of experiments, we consider two robots that need to coordinate to accomplish a collaborative task while also avoiding collisions with each other. %Finally, note that in this experiment, the robots are allowed to move asynchronously. 


%The proposed algorithm has also been validated experimentally for robots that that reside in complex indoor environments with \textit{unknown} and \textit{static} obstacles; see Fig. \ref{fig:exp}. In the experiments, the robot are equipped with a LiDAR sensor with $180^{o}$ field-of-view, which violates the assumption of Proposition \ref{thm:completeness}, since it is not an omnidirectional sensor. The task of the robot is captured by the following LTL formula: $\phi=\Diamond(\pi_1^{r_2}\vee \pi_1^{r_5})\wedge\Diamond(\pi_1^{r_1})\wedge\Diamond(\pi_1^{r_4}\vee\pi_1^{r_3})\wedge\Diamond(\pi_1^{r_7}\vee\pi_1^{r_5})\wedge(\wedge\Diamond(\pi_1^{r_8}\vee\pi_1^{r_6}) \wedge (\neg \pi_1^{r_9}\ccalU \pi_1^{r_8})\wedge(\square \neg \xi^{\text{obs}})$, which requires the robot to eventually visit certain regions of interest while always avoiding obstacles. This experiment has been conducted in two different environments. 
%F(p1) & F(p2) & F(p3) & F(p4) & F(p5) & FG(p6)
%

%{\bf{Experiments in Dynamic Environments:}} We have also validated experimentally Algorithm \ref{alg:RRT} in dynamic environments. Specifically, to solve the navigation problem in \eqref{eq:localProb} in the presence of \textit{unknown} and \textit{dynamic} obstacles, we employ the motion planning algorithm proposed in \cite{guzzi2013human}.  We consider two robots that need to coordinate to accomplish a collaborative task while also avoiding collisions with each other. Note that in this experiment, the robots move asynchronously as opposed to the majority of relevant works.
%




{\bf{Vision-based \& Map-Free Planning:}} 
In the second set of experiments we consider a team of two robots that have to accomplish the following task
\begin{align}\label{task4}
    \phi=&\Diamond(\pi_2^{\ell_2})\wedge\Diamond(\pi_1^{\ell_1}\wedge\Diamond(\pi_1^{\ell_3}\wedge\pi_2^{\ell_3}))\nonumber\\&\wedge\Diamond\square(\pi_1^{\ell_4})\wedge\Diamond\square(\pi_2^{\ell_4})\wedge(\square \neg \xi^{\text{obs}}).
\end{align}
The LTL task in \eqref{task4} requires robot $1$ and robot $2$ to eventually visit locations $\ell_1$ and $\ell_2$, respectively, e.g., to collect data. Then the robots should meet in $\ell_3$ e.g., to exchange their collected data or upload it to a data center, and then go to the exit $\ell_4$ of the room and stay there forever. 

In this set of experiments, to solve \eqref{eq:localProb}, i.e., to design reactive robot paths towards regions of interest, we rely on a vision-based approach proposed in \cite{guzzi2013human}. Specifically, \cite{guzzi2013human} proposes a heuristic approach to avoid dynamic obstacles such as other mobile robots or humans. Using visual information the heading of dynamic obstacles is estimated which is then used to compute the robot velocity so that all visible obstacles and robots are avoided within a time horizon. Figures \ref{fig:expMulti1} and \ref{fig:expMulti2} show cases where the robots react to unexpected obstacles that are placed in front of them at runtime. We would like to emphasize again that Algorithm \ref{alg:RRT} allows the robots to react to unknown structure of the environment quickly which would be impossible using available centralized temporal logic planning methods.

Note that \cite{guzzi2013human} is map-free i.e., it does not rely on building maps; instead navigation is accomplished using visual feedback. This allows to navigate dynamic environments as opposed to the purely map-based approach considered in the previous set of experiments.
Nevertheless, map-based approaches allows the robots to reason about the structure of the environment and make appropriate control decisions to accomplish their tasks as discussed in \ref{sec:sim1}. Integration of map-based and vision-based planning methods is part of our future work.
%In our future work, integra map-based approaches allow the robots to reaso


\begin{figure*}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Initial state]{
    \label{fig:a1}
  \includegraphics[width=0.32\linewidth]{figures/multiInit.jpg}}
  \subfigure[Unexpected obstacle]{
    \label{fig:b1}
  \includegraphics[width=0.32\linewidth]{figures/multiIBef.jpg}}
    %\subfigure[Reactive Planning]{
    %\label{fig:c1}
  %\includegraphics[width=0.47\linewidth]{figures/multiIAvoid1.jpg}}
      \subfigure[Reactive Planning]{
    \label{fig:d1}
  \includegraphics[width=0.32\linewidth]{figures/multiIAvoid2.jpg}}
  \caption{Camera-based planning in unknown environments: Robot $1$ and $2$ are heading towards locations $1$ and $2$ respectively. Obstacles are placed at run-time in the workspace. The robots adapt planning to these unexpected changes in the environment using visual feedback.\red{[Figs need some editing-hard to see what is happening]}
  }
  \label{fig:expMulti1}
\end{figure*}

\begin{figure*}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Heading towards $\ell_3$]{
    \label{fig:a2}
  \includegraphics[width=0.32\linewidth]{figures/multi2Bef2.jpg}}
    \subfigure[Unexpected Obstacle]{
    \label{fig:b2}
  \includegraphics[width=0.32\linewidth]{figures/multi2after2.jpg}}
      \subfigure[Reactive Planning]{
    \label{fig:c2}
  \includegraphics[width=0.32\linewidth]{figures/multi2avoid2.jpg}}
  \caption{Robot $1$ and $2$ are heading towards location $3$. Obstacles are placed at run-time in the workspace. The robots adapt planning to these unexpected changes in the environment using visual feedback. \red{[Figs need some editing-hard to see what is happening]}
  }
  \label{fig:expMulti2}
\end{figure*}


==> Robust Motion Planning in the Presence of Estimation Uncertainty/files/theory_final.tex <==
%\red{[TO BE UPDATED SOON!]}

%\begin{prop}[Correctness]
%If Algorithm \ref{alg:RRT} terminates successfully, then the resulting path $\bbp_{0:H}$ satisfies the LTL property $\phi$.
%\end{prop}
%\begin{proof}
%This result is true by construction of Algorithm \ref{alg:RRT}. Specifically, while the robots navigate in the workspace to reach the target DFA state $q_D^{\text{next}}$ from the current DFA state $q_D(t)$, they always check if the next observation $L(\bbp(t+1))$ violates the LTL formula $\phi$. If this is not the case, for all $t\geq 0$, the robots will eventually reach all subsequent target DFA states. Since the target DFA states are selected so that they are always one hop closer to the final state $q_F^{\text{feas}}$ than $q_D(t)$ is (see \eqref{eq:targetDFA}), this means that eventually the robots will reach $q_F^{\text{feas}}$ and, therefore, they will satisfy $\phi$ completing the proof.
%\end{proof}
 
 
%(ii) there do not exist regions $r_i$ and $r_e$, such that $r_i\subseteq r_e$ and 
%and (ii) there do not exist regions $r_i$ that are accessible only after visiting first
%\red{[the statements need to become more clear..]}
In this section, we examine correctness of the proposed reactive algorithm. First, recall from Algorithm \ref{alg:RRT} that once the robots reach a state $q_B(t)\in\ccalV$ a new state $q_B^{\text{next}}\in\ccalV$ is selected to be reached next.
%
This state is selected from the set $\ccalQ_{q_B(t)}^{\text{next}}\subseteq\ccalV$ that collects all states $q_B^{\text{next}}$ for which the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable, as per Definition \ref{def:feas}, and therefore, this transition can be enabled by solving local reachability tasks. As discussed in Remark \ref{rem:conserv}, Definition \ref{def:feas} is conservative, in the sense that there may be states that can be reached from $q_B(t)$ but they do not satisfy the conditions of Definition \ref{def:feas}; see e.g., Figure \ref{fig:conserv}.  As a result, such states are not included in the set $\ccalQ_{q_B(t)}^{\text{next}}$ and, therefore, a solution to Problem \ref{prob} may not be found even if it exists. 
%
First, we show that there exists a fragment of LTL for which any NBA transition $\delta_B^m(q_B,\cdot,q_B')$ associated with a run defined in \eqref{eq:run} always satisfies Definition \ref{def:feas}. In other words, all transitions $\delta_B^m(q_B,\cdot,q_B')$ are decomposable and can be enabled by solving local reachability problems \eqref{eq:localProb}. To show this we need make the following assumption.

%\subsection{Correctness of Algorithm \ref{alg:prune}}\label{sec:corPr}

%Given that the infeasible transitions are removed from the NBA, we have that the only reason there may not exist symbol $\sigma^{q_B,q_B^K}$ that satisfies $b^{q_B,q_B^K}$ is if the transition from $q_B$ to $q_B^K$ requires a robot to instantaneously jump from one region of interest to another one; see e.g., Figure \ref{fig:feas1}. 


%First of all note that for any state $q_B\in\ccalQ_B^{\text{loop}}$ there has to exist at least one state $q_B^K$ so that a run in the form of \eqref{eq:run} can be generated. If there exists no such runs, then the only way to visit a final state after visiting $q_B$ is by instantaneously jumping from one NBA state to another one i.e., without staying in any of them. Nevertheless, such transitions cannot exist, as they would require new observations to be made every time a new NBA state is visited which is impossible to specify given that the `next' operator is omitted. 

%In what follows we provide conditions under which Definition \ref{def:feas}, which Algorithm \ref{alg:prune} relies on, is not conservative. For this, we need first to state the following assumption.


\begin{assumption}\label{as:cnf}
Let $b^{q_B,q_B'}$ be a Boolean formula written in conjunctive normal form (CNF) associated with any NBA transition $\delta_B(q_B,\cdot,q_B')$. Assume that all literals in any given clause of $b^{q_B,q_B'}$ are associated with only one robot, which is not necessarily the same across different clauses.
\end{assumption}

\begin{lem}[From Global LTL to Local Tasks]\label{lem:fragmentLTL}
%Consider an LTL formula $\phi$ defined over atomic predicates $\pi_j^{\ell_i}$ where $j\in\ccalN$ and $\{\ell_i\}_{i\in\ccalL}$ denote disjoint regions of interest. 
%Consider any finite run in the form of \eqref{eq:run} from
%
Consider any two states $q_B,q_B'\in\ccalV$ for which there exists a symbol $\sigma^{q_B,q_B'}$ that satisfies the corresponding Boolean formula $b^{q_B,q_B'}$ defined in \eqref{eq:b}. Under Assumption \ref{as:cnf}, the transition $\delta_B^{m}(q_B,\cdot,q_B')$ is always decomposable, as per Definition \ref{def:feas}, unless this transition requires robots to instantaneously jump from one region of interest to another one which is impossible given that the regions of interest are disjoint.
\end{lem}

In other words, according to Lemma \ref{lem:fragmentLTL}, if all Boolean sub-formulas (expressed in CNF) that appear in an LTL formula satisfy Assumption \ref{as:cnf}, the global LTL formula can be decomposed into local reachability tasks.\footnote{The Boolean sub-formulas can be obtained after removing all temporal operators in an LTL formula.} Also, Lemma \ref{lem:fragmentLTL} implies that single-agent LTL tasks can always be decomposed into reachability tasks; see also Example \ref{ex:localTasks}.


%never couples two or more atomic predicates associated with different robots with the `or' operator, then Definition \ref{def:feas} is not conservative and, therefore, the global LTL formula can be decomposed into local reachability tasks. Also, Lemma \ref{lem:fragmentLTL} implies that Definition \ref{def:feas} is never conservative for single-robot tasks.

%\begin{rem}[Non-Emptiness of $\ccalQ_{q_B}^{\text{next}}$]
%By Definition $\ccalQ_{q_B}^{\text{next}}$ we have that $q_B\in\ccalQ_{q_B}^{\text{next}}$ for all $q_B\in\ccalQ_{q_B}^{\text{loop}}$. Also, we have that $\ccalQ_{q_B}^{\text{next}}\setminus\{q_B\}\neq\emptyset$ for all states $q_B\in\ccalQ_B^{\text{loop}}$ (assuming $\phi$ is satisfiable), since otherwise the only way to visit the final state after visiting $q_B$ is by instantaneously jumping from one NBA state to another one i.e., without staying in any of them. Nevertheless, such transitions cannot exist, as they would require new observations to be made every time a new NBA state is visited which is impossible to specify given that the `next' operator is omitted. 
%\end{rem}

%\subsection{Completeness of Algorithm \ref{alg:RRT}}\label{sec:corPl}


%\begin{lem}[Non-Existence of Solution]\label{thm:nonexist}
%Assume that (a) all Boolean subformulas that appear in an LTL formula satisfy Assumption \ref{as:cnf}, and (b) there does not exist an infinite path in $\ccalG$ that includes an infinite number of accepting edges defined in Definition \ref{def:accEdges}. Under assumptions (a)-(b), there does not exist a solution to Problem \ref{prob}.
%%%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. If at least one of these paths respects the robot dynamics \eqref{eq:rdynamics}, then Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
%\end{lem}

%\begin{lem}[Existence of Solution]\label{thm:exist}
%Assume that (a) all Boolean subformulas that appear in an LTL formula satisfy Assumption \ref{as:cnf}, and (b) there exists at least one robot path that respects the robot dynamics \eqref{eq:rdynamics} and connects any location $\bbq\in\Omega$ to any region $\ell_i$ without crossing any region $\ell_e\neq \ell_i$ and obstacles. Under assumptions (a)-(b), there exists a solution to Problem \ref{prob}.
%%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. If at least one of these paths respects the robot dynamics \eqref{eq:rdynamics}, then Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
%\end{lem}


Next we provide conditions that ensure that Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then a solution will be found.


%In the following proposition, we provide conditions under which Algorithm \ref{alg:RRT} is complete is complete.%, we need first to state the following Lemma. The proof is omitted due to space limitations.
%\begin{lem}\label{lem:binv}
%Let $q_D$ be the DFA state at time $t$ and $\bbp_{j,t:T_j}$ be the paths that the robots designed to reach  $q_D^{\text{next}}$.
%%Assume that there are no regions $r_i$ and $r_j$, such that $r_i\subseteq r_j$. Then,  %% condition for feasibility
%If all robots execute the paths $\bbp_{j,t:T_j}$, as per Section \ref{sec:planning}, and if all robots $j\in\ccalR_{\text{next}}$ reach their assigned regions $L_j^{\text{next}}$, then the robots remain in $q_D$ during the time interval $[t,T-1]$ and reach $q_D^{\text{next}}$ at the time instant $T=\max_j\{ T_j\}$.
%\end{lem}

%The following result presents conditions under which the pruning of the DFA is not conservative as discussed in Sec. \ref{sec:planning}.

%\begin{lem}\label{lem:cnt}
%Consider Boolean formulas $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$ in negation normal form. If the disjunction operator does not appear in either of these formulas, then Definition \ref{def:feas} is not conservative, i.e., if there exists at least one pair of symbols $\sigma_{\text{inv}}^{q_D}\in\Sigma_{\text{inv}}^{q_D}\cap\Sigma_{\text{feas}}$ and $\sigma_{\text{next}}^{q_D,q_D'}\in\Sigma_{\text{next}}^{q_D,q_D'}\cap \Sigma_{\text{inv}}^{q_D'}\cap\Sigma_{\text{feas}}$, then for any $\sigma_{\text{inv}}^{q_D}\in\Sigma_{\text{inv}}^{q_D}\cap\Sigma_{\text{feas}}$ there always exists $\sigma_{\text{next}}^{q_D,q_D'}\in\Sigma_{\text{next}}^{q_D,q_D'}\cap \Sigma_{\text{inv}}^{q_D'}\cap\Sigma_{\text{feas}}$ such that transition from $q_D$ to $q_D'$ can be cast as a reachability problem.
%\end{lem}


%The above lemma states that when the robots reach any DFA state $q_D'$, there always exist symbols $\sigma_{\text{inv}}$ and $\sigma_{\text{next}}$ to that will drive the robots towards another DFA state $q_D''$, as long as this transition is feasible. This essentially ensures that \eqref{eq:localProb} is always well defined. This is required in the proof of the following result.



\begin{prop}[Completeness]\label{thm:completeness}
Assume that (a) there exists at least one infinite path in $\ccalG$ that starts from $q_B^{\text{aux}}$ and traverses at least one accepting edge infinitely often,
%such that the disjunction operator does not appear in any of the formulas $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$, for all $q_D,q_D'$. %
(b) there exists at least one robot path that respects the robot dynamics \eqref{eq:rdynamics} and connects any location $\bbq\in\Omega$ to any region $\ell_i$ without crossing any region $\ell_e\neq \ell_i$ and obstacles, and (c)  \eqref{eq:sensor} models an omnidirectional sensor. Under assumptions (a)-(c), Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. If at least one of these paths respects the robot dynamics \eqref{eq:rdynamics}, then Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
\end{prop}

\red{[discuss why the assumptions are not too strong..and when then can be relaxed]}

Finally, in the next proposition we show that under the assumptions (a)-(b) of Proposition \ref{thm:completeness}, a solution to Problem \ref{prob} always exists.

\begin{prop}[Existence of Solution]\label{thm:exist}
If Assumptions (a)-(b) of Proposition \ref{thm:completeness} hold, then there exists a solution to Problem \ref{prob}.
%Assume that (a) there exists at least one infinite path in $\ccalG$ that starts from $q_B^{\text{aux}}$ and traverses at least one accepting edge, defined in Definition \ref{def:accEdges}, infinitely often, and (b) there exists at least one robot path that respects the robot dynamics \eqref{eq:rdynamics} and connects any location $\bbq\in\Omega$ to any region $\ell_i$ without crossing any region $\ell_e\neq \ell_i$ and obstacles. Under assumptions (a)-(b), there exists a solution to Problem \ref{prob}.
%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. If at least one of these paths respects the robot dynamics \eqref{eq:rdynamics}, then Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
\end{prop}

\begin{ex}[From Global LTL to Local Tasks]\label{ex:localTasks}
Consider the LTL formula $\phi=\square(\pi_1^{\ell_0}\vee\pi_2^{\ell_0}) \wedge \Diamond \pi_2^{\ell_1}\wedge \Diamond \pi_2^{\ell_1}$ corresponding to the NBA shown in Figure \ref{fig:conserv}. This LTL formula has three Boolean subformulas: (i) $\pi_1^{\ell_0}\vee\pi_2^{\ell_0}$, (ii) $\pi_2^{\ell_1}$ , and (iii) $\pi_2^{\ell_1}$. Observe that the Boolean subformula $\pi_1^{\ell_0}\vee\pi_2^{\ell_0}$ violates Assumption \ref{as:cnf} and therefore it cannot be decomposed into local reachability tasks. On the other hand, the LTL formula $\phi=\Diamond[(\pi_1^{\ell_0}\vee\pi_1^{\ell_2})\wedge\pi_1^{\ell_0}] \wedge \square\Diamond \pi_2^{\ell_1}\wedge \square\Diamond \pi_2^{\ell_1}$
satisfies Assumption \ref{as:cnf}. More examples of LTL formulas that satisfy Assumption \ref{as:cnf} are provided in Section \ref{sec:Sim}.
%and can be decomposed into local reachability tasks.
\end{ex}


%\begin{rem}[Checking satisfiability of $\phi$]
%Note that if in the pruned DFA there is no path that connects at least one pair of initial and accepting states, then this means that there is no solution to Problem \ref{prob}. One the other hand, if there exists at least one such path, then this means that there exists a solution to Problem \ref{prob} assuming simple enough dynamics transitions from one region $r_i$ to any other region $r_e$ can be accomplished while avoiding regions (e.g., obstacles) as determined by $\phi$.\footnote{\red{this is intuitively correct. It'd be great if we add a formal proof}} 
%\end{rem}

%\begin{prop}[Satisfiability]\label{prop:sat}
%%Consider robots with single-integrator dynamics. Also, 
%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$ and obstacles. 
%Consider a co-safe temporal logic formula such that the disjunction operator does not appear in any of the formulas $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$, for all $q_D,q_D'$. Assume that there exists at least one path that connects any location $\bbq\in\Omega$ to any region $r_i$ without crossing any region $r_e\neq r_i$ and obstacles. Also, assume that at least one of these paths satisfies the robot dynamics \eqref{eq:rdynamics}. Then, given the corresponding pruned DFA, it holds that $\phi$ cannot be satisfied if $d(q_0,q_F)=\infty$. If $d(q_0,q_F)\neq\infty$, then there exists $\bbp_{0:H}$ that satisfies $\phi$.
%\end{prop}

%\begin{proof} %This result can be proved by following the same logic as in the proof of Proposition \ref{thm:completeness}. 
%If $d(q_0,q_F)=\infty$, then by Definition \ref{def:feas}, we conclude that there exist robots that either have to be present in more than one disjoint region simultaneously or have to instantaneously move from one region to another region (see condition (ii) in Definition \ref{def:feas}) so that $\phi$ is satisfied. Thus, robot paths $\bbp_{0:H}$ that can satisfy $\phi$ do not exist. Note that condition (iii) in Definition \ref{def:feas} holds for all DFA transitions, if $\vee$ is excluded from the syntax, as shown in Lemma \ref{lem:cnt}. %and therefore no transition will be deleted due to condition(iii)
%%
%%
%If $d(q_0,q_F)\neq\infty$, then following the same logic as in the proof of Proposition \ref{thm:completeness}, we conclude that there exist robot paths $\bbp_{0:H}$ such that $\bbp_{0:H}\models\phi$ under the considered assumptions on the robot dynamics and the structure of the environment.
%%%
%, if there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$ and obstacles and at least one of these paths satisfies the robot dynamics.
%First, note that every DFA state $q_D$ has a (non-empty) Boolean formula $b_{\text{inv}}^{q_D}$ that if satisfied, transition from $q_D$ to $q_D$ (self-loop) is activated. The reason is that the `next' temporal operator is not included in the task specification language. Also, as the robots `follow' a path $\bbq_D$, when they reach a configuration $\bbp\in\Omega^N$ that enables a transition from $q_D$ to $q_D'$, we have that $L(\bbp)\models b_{\text{inv}}^{q_D'}$ by construction of the DFA. In other symbols, if the DFA will not move to another state until the robots observe something new that will either violate $\phi$ (and in this case there is no outgoing transition from $q_D'$ to another DFA state based on the current observation) or enable a transition to another state $q_D''$. 
%%%
%Second, assume that the multi-robot system has currently reached $q_D$ and as discussed before, the current multi-robot robot state $\bbp$ satisfies $L(\bbp)\models b_{\text{inv}}^{q_D}$. In what follows, we show by contradiction that $q_D'$ can be reached. Assume that the robots cannot reach $q_D'$. This means that the robots can never satisfy the Boolean formula $b_{\text{next}}^{q_D,q_D'}$. However, by Lemma \ref{lem:feas}, we have that there exist paths for all robots that can reach $q_D'$ assuming simple dynamics and that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. Thus, under these assumptions it is not possible that $q_D'$ cannot be reached. Therefore, we conclude that $q_D$ can be reached completing the proof.
%\end{proof}

%\begin{rem}[Boolean Operator OR]
%Note that the completeness and satisfiability result can be extended to cases where the $\vee$ operator is included in the syntax; however, a full characterization of the LTL formulas for which Alg. \ref{alg:RRT} is complete is omitted due to space limitation. For instance, the above results hold, if $\vee$ appears in $\phi$ but never associates atomic predicates of different robots (i.e., Boolean statements of the form $\pi_j^{r_e}\vee\pi_r^{r_m}$ never appear in $\phi$). This also implies that if $N=1$ then the above results hold even if $\vee$ is included. Such cases are included in the simulation/experimental results.
%\end{rem}


==> algorithm2e.tex <==
%  algorithm2e.sty --- style file for algorithms
%                      almost everything can be customized by users. See the document for more explanations
%% Copyright 1996-2015 Christophe Fiorio
%
% This work may be distributed and/or modified under the conditions of the LaTeX Project
% Public License, either version 1.3 of this license or (at your option) any later version.
% The latest version of this license is in http://www.latex-project.org/lppl.txt and
% version 1.3 or later is part of all distributions of LaTeX version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is M. Christophe Fiorio
%
% This work consists of the files algorithm2e.sty and algorithm2e.tex 
% and the associated example files algorithm2e_exAlgoDisjdecomp.tex,
% algorithm2e_exIR.tex, algorithm2e_ex01.tex, algorithm2e_exProg.tex,
% algorithm2e_ex02.tex, algorithm2e_exfor.tex, algorithm2e_ex03.tex,
% algorithm2e_exgeneric.tex, algorithm2e_ex04.tex,  algorithm2e_exgeneric2.tex,
% algorithm2e_ex05.tex, algorithm2e_exnlsty.tex, algorithm2e_ex06.tex,
% algorithm2e_exrepeat.tex, algorithm2e_ex07.tex, algorithm2e_exswitch.tex
%  
%  Report bugs and comments to:
%  - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
%  - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
%  subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
%
%  $Id: algorithm2e.sty,v 5.1 2015/10/18 21:37:30 cfiorio Exp $
%
%  PACKAGES REQUIRED:
%
%  - float   (in contrib/supported/float)
%  - ifthen  (in base)
%  - xspace  (in packages/tools)
%  - relsize (in contrib/misc/relsize.sty)
%
%%%%%%%%%%%%%%%  Release 5.1
%
%   Package options: 
%   ---------------
%   - oldcommands                      : to use old command names
%   - french, english, german, ngerman
%      portuguese, czech, italiano,
%      slovak, croatian, spanish       : for the name of the algorithm and some keyword code
%   - onelanguage                      : to simply switch keyword from one language to another without changing
%                                        keyword commands
%   - boxed, boxruled, ruled, tworuled, 
%     algoruled, plain                 : layout of the algorithm
%   - algo2e                           : environment is algorithm2e instead of algorithms and \listofalgorithmes
%                                        instead of \listofalgorithms
%   - slide                            : to use when making slides
%   - noline,lined,vlined              : how block are designed.
%   - shortend, longend, noend         : short or long end keyword as endif for e.g.
%   - linesnumbered                    : auto numbering of the algorithm's lines
%   - linesnumberedhidden              : to hide autonumbered lines (show number on a line with \ShowLn
%   - commentsnumbered, inoutnumbered  : to autonumber comments and inout keywords (by defaut not numbered)
%   - rightnl                          : to have line number on the right instead of on the left as default
%   - algonl                           : line numbers preceded by algo number
%   - scright, scleft                  : right or left justified side comments
%   - fillcomment, nofillcomment       : end mark of comment is flushed to the right so comments fill the line
%   - dotocloa                         : add an entry in the toc for list of algorithms (require tocbibind package)
%   - endfloat                         : add algoendfloat environment pushing algorithm so written to the end of document
%   - resetcount, noresetcount         : start value of line numbers.
%   - algopart,algochapter,algosection : algo numbering within part, chapter or section
%   - titlenumbered,titlenotnumbered   : numbering of title set by \Titleofalgo
%   - figure                           : algorithms are figures, numbered as figures, and put in the list of figures.
%   - procnumbered                     : procedure or function are numbered as algorithm
%   - nokwfunc                         : procedure or function name doens't become a command
%   - norelsize                        : don't use relsize package (useful if it breaks the compatibily)
%   - displayblockmarkers              : display begin, end keywords at start of each block
%  
%   defaults are; english,plain,resetcount,titlenotnumbered
%
%%%%%%%%%%%%%%
%
%   Short summary  
%   -------------
%  
%   algorithm is an environment for writing algorithm in LaTeX2e.
%   Almost all is customizable. You can add keywords, change style, change the layout, ...
%   It provide macros that allow you to create differents sorts of key words, therefore a set of predefined key
%   word is gived.
%
%   IT should be used as follows
%
%   \begin{algorithm}
%       ...
%       ...
%   \end{algorithm}
%
%
%   IMPORTANT : each line MUST end with \;
%
%   Note that if you define macros outside algorithm environment they
%   are avaible in all the document and particulary you can use then
%   inside all algorithms without re-define them.
%  
%   an example:
%
%   \begin{algorithm}
%     \SetAlgoLined
%     \KwIn{this text}
%     \KwOut{how to write algorithm with \LaTeX2e }
%     
%     initialization\;
%     \While{not at end of this document}{
%       read current section\;
%       \eIf{understand}{
%         go to next section\;
%         current section becomes this one\;
%         }{
%         go back to the beginning of current section\;
%         }
%       }
%     \caption{How to write algorithm}
%   \end{algorithm}
%
%
%%%%%%%%%%%%%%         predefined keywords
%
%     \KwIn{input}
%     \KwOut{output}
%     \KwData{input}
%     \KwResult{output}
%     \KwTo                                       % a simple keyword
%     \KwFrom                                     % a simple keyword
%     \KwRet{[value]}
%     \Return{[value]}
%     \Begin{block inside}
%     \eIf{condition}{Then Block}{Else block}     % in blocks
%     \If{condition}{Then block}                  % in a block
%     \uIf{condition}{Then block}                 % in a block unended
%     \lIf{condition}{Else text}                  % on the same line
%     \Else{inside Else}                          % in a block
%     \lElse{Else text}                           % on the same line        
%     \uElse{Else text}                           % in a block unended
%     \ElseIf{inside Elseif}                      % in a block
%     \lElseIf{Elseif text}                       % on the same line        
%     \uElseIf{Elseif text}                       % in a block unended
%     \Switch{Condition}{Switch block}
%     \Case{a case}{case block}                   % in a block
%     \lCase{a case}{case text}                   % on the same line
%     \Other{otherwise block}                     % in a block
%     \lOther{otherwise block}                    % on the same line
%     \For{condition}{text loop}                  % in a block
%     \lFor{condition}{text}                      % on the same line
%     \ForEach{condition}{text loop}              % in a block
%     \lForEach{condition}{text}                  % on the same line
%     \ForPar{condition}{text loop}               % in a block
%     \lForPar{condition}{text}                   % on the same line
%     \While{condition}{text loop}                % in a block
%     \lWhile{condition}{text loop}               % on the same line
%     \Repeat{End condition}{text loop}           % in a block
%     \lRepeat{condition}{text}                   % on the same line
%
%%%%%%%%%%%%%%
%
%   History: 
%
%   -  October 19 2015 - revision 5.1
%                   * CHANGE/ADD: l commands  (the ones as \lIf) can now be used with a
%                              star. If done, no end of line are done, so you can enclose
%                              l command into another one. For example, you can write:
%                              \lForEach{$i$}{\lIf*{foo}{bar}}.
%                               Note that when you use a star, side comments are not allowed.
%                   * CHANGE/ADD: Now you can have a side comment at end of macros which
%                               have a block. For example you can do : 
%                               \Begin(\tcc*[h]{side comment for begin}{text}(\tcc*[h]{side comment after end})
%                               Note: there are some side effects for some commands:
%                              \SetKwProg : macro defined thanks to \SetKwProg are allowed
%                                                   to have no end marker. In this case,
%                                                   beware to end side comment, this can
%                                                   do weird output (but no error)
%                   * CHANGE: \SetKwSwitch defines also an \uOther command which was not
%                               the case until this release.
%                   * CHANGE: \SetStartEndCondition{typo1}{typo2}{typo3} defined two end
%                               conditions (type2 and typo3) : typo3 is no more used for
%                               case condition as typo2 is used which is more consistent
%                               since there is a condition followed by a keyword as for
%                               if-then or other command that are defined using typo2.
%                   * CHANGE: keywords was not language dependant to allow to use multiple
%                               languages in the same document, but some keywords in
%                               different language were having the same keyword that lead
%                               last one declared to replace first one and so you could have some
%                               spanish keywords printed as you were in portuguese. So
%                               this behavior is changed from now:
%                               - localized keywords are defined if according language
%                                  option is defined ; 
%                               - if you want to keep old behaviour and use localized
%                                  keywords without using language option (keep old
%                                  behavior), you can use languagekw option
%                                  (e.g. frenchkw, germankw, ...). Note that you can use
%                                  multiple languagekw options at the same time, in
%                                  contrary of language option. Note also that if you use
%                                  multiple languagekw options, you can get back the same
%                                  problem as previously when keywords was not language
%                                  dependant.
%                   * ADD: new typo styles:
%                               - Arguments of functions have now their own style. By
%                                  default, FuncArgSty is the same as ArgSty. 
%                               - Name of KwProg have now their own sty (they used ArgSty
%                                  previously). By default, ProgSty is still ArgSty.
%                               As usual, \SetFuncArgSty{}, FuncArgSty{} and
%                               \SetProgSty{}, ProgSty{} are macros to set and use these
%                               typo styles.
%                   * ADD: Options to manage algorithm hangindent
%                            Until this revision, long statement acts as classical text and
%                            continue on next line starting from the same point. This makes
%                            difficult to notice that the new lines of text is not a new
%                            statement. Now, hangindent is managed and when a long
%                            statement continue on next lines, lines, except the first,
%                            are indented.
%                            Option: noalgohanging
%                               By default, long statement are indented on subsequent
%                               lines; with this option you get old behavior and lines are
%                               no more indented
%                            Option: hangingcomment 
%                               Comment that are alone on a line (not side comment) are
%                               not driven by algo hanging: subsequent lines of long
%                               comments are indented according to width of start comment
%                               marker. With this option, comment are indented like normal
%                               statement.
%                            Option: hanginginout
%                               As for comment, by default, in/out keywords and input
%                               keywords (defined by \SetKwInOut or \SetKwInput) are not
%                               indented by algorithm hangindent. They are indented
%                               according to width of input keyword. If you want that these
%                               keywords acts like normal statement, use this option.
%                            \SetAlgoHangIndent{length}
%                               This macro allows you to set your own indent length. By
%                               default, \SetAlgoHangIndent{0.5em}
%                   * ADD: Group markers. 
%                            This option is related to block markers of release 5.0. Some
%                            have ask to put also block markers for single line
%                            command. This new feature has been implemented to do this.
%                            So, you can now ask package to put begin and end keywords
%                            automatically at start and end of single line command (see
%                            example in documentation).
%                            These new group markers macros are:
%                            - \AlgoDisplayGroupMarkers and \AlgoDontDisplayGroupMarkers
%                            Note that a new option has also been added: displaygroupmarkers
%                   * ADD: \SetCustomAlgoRuledWidth{length}
%                             set a custom ruled width of ruled and algoruled options ;
%                             note that by the moment you use this macro, rules will have
%                             this fixed length: this can cause strange behavior in
%                             multicolumn mode or other layout that change the line
%                             width. 
%                   * ADD: turkish language option
%                   * FIX: a spurious whitespace which results in a spurious indent in the
%                            user's text right after the end of the algorithm environment
%                            was introduced  in release 5.0. This is fixed now thanks to
%                            Alexander Malkis.
%                   * FIX: there was a problem with margins in caption when option figure
%                            was use with caption package. This is fixed.
%                   * FIX: when changing font size in caption with, interline skip stayed
%                            unchanged and so with a small font was to large. This is fixed.
%                   * FIX: in contrary of that is written in the documentation, ':' what
%                            not in KwSty typo for KwIn and KwOut command. This is fixed. 
%                   * FIX: strange behaviour with label and lines numbered: @currentlabel
%                            was updated according to algo line number not in all
%                            situation. For e.g, with hyperref package, always updated ;
%                            with \nlset also updated, but with \nl or linesnumbered
%                            option, not updated. This "feature" causes different output
%                            with \label command according to options used which is not
%                            that one want. This is solved now, and @currentlabel is
%                            always updated so \label command works always is the same way.
%                   * FIX: some czech keywords
%                   * FIX: some spanish keywords
%                   * FIX: some croatian keywords
%                   * FIX: krantz class changes definition of chapter and get one more
%                            option that classical classes as book.cls or report.cls and
%                            broke fix for hyperref on chapter definition. This is now
%                            fixed and algorithm detects use of krantz class and use then
%                            a definition of chapter working with krantz class.
%                   * FIX: an issue with internal macro which causes ([Q]) use as argument
%                            of some environment to be misprinted (thanks to Martin Schr?der).
%                   * FIX: mispelled name of hyperrefcounter inside internal macro.
%
%   - January 06 2013 - revision 5.0
%                     * CHANGE: SetKwSwitch takes now 9 args: 9th arg is the same as
%                                previous 8th arg ('end of switch' keyword). New 8th arg is
%                                'end of case' keyword. This is due to change of release
%                                3.2 which introduce end after case block... as I never
%                                test with longend option, I never see that the 'end
%                                switch' used for case was not good.
%                     * CHANGE: when no end keyword is defined in a block macro, then
%                                algorithm2e does no more try to print it. So even with lined or noline
%                                option, no empty line is printed (before: a blank end was
%                                printed, so a blank line appeared)
%                     * Internal Change: add some internal function to improve readibility
%                                        (thanks to Philip K. F. H\?lzenspies)
%                     * ADD: Block markers. 
%                            You can now ask package to put begin and end keywords automatically at begin
%                            and end of blocks, it means each group of commands shifted and enclosed in
%                            braces.
%                            This is tricky to use but, combined with \SetStartEndCondition and
%                            redefinition of keywords, you should be abble to simulate any syntax. See
%                            examples in documentation where a generic example is derived in pseudo-code,
%                            python and C by keeping code and changing only style using block markers
%                            macros, \SetStartEndCondition and some redefinition of keywords.
%                            These new block markers macros are:
%                            - \AlgoDisplayBlockMarkers and \AlgoDontDisplayBlockMarkers
%                            - \SetAlgoBlockMarkers{begin marker}{end marker}
%                            - \BlockMarkersSty{text} and \SetBlockMarkersSty
%                            Note that a new option has also been added: displayblockmarkers
%                     * ADD: \leIf macro automatically defined by \SetKwIF: allow to define
%                            an if-then-else on a single line.
%                     * ADD: new macro \SetStartEndCondition{typo1}{typo2}{typo3} which
%                            sets typo around condition in For, If, Switch, Case and
%                            Repeat macros. First two are used around For, If, Swith
%                            conditions, First and third are used for Case and Repeat
%                            condition where condition ends the line. Default definition
%                            is \SetStartEndCondition{ }{ }{}. 
%                            A common alternative is \SetStartEndCondition{ (}{) }{)}
%                            Can also be used to remove space around condition, for
%                            example if you want python style commands:
%                            \SetStartEndCondition{ }{}{} and \SetKwFor{For}{for}{:}{}
%                     * ADD: new environment algomathdisplay which allow display math (like inside \[ \] or $$ $$) 
%                            handling end line and line number
%                     * ADD: new command \SetKwProg{Env}{Title}{is}{end} which defines a macro
%                            \Env{args}{text}. Env is a block with 'Title' (in \CapSty) at the beginning
%                            followed by args followed by 'is' then 'text' is put below inside a block ended
%                            by 'end'. If no 'end' is specified, nothing is written (no
%                            blank line is inserted). Useful to typeset function or prog for example:
%                            \SetKwProg{Fn}{Function}{ is}{end} makes \Fn{afunc(i: int) : int}{return 0\;}                    
%                            writes: 
%                            Function afunc(i: int) : int is
%                            | return 0;
%                            end
%                            or \SetKwProg{Def}{def}{:}{} makes \Def{afunc(i: int)}{return 0\;} writes:
%                            def afunc(i: int):
%                            | return 0
%                            Tip: combine it with \SetKwFunction to write recursive function algorithm. With
%                            example above, you could define \SetKwFunction{\Afunc}{afunc} and then write:
%                            \Def{\Afunc{i:int}{\eIf{i>0}{\KwRet \Afunc{i-1}}{\KwRet 0\;}} that writes:
%                            def afunc(i: int):
%                            | if(i>0):
%                            |     return afunc(i-1)
%                            | else:
%                            |     return 0
%                            with appropriate typo.
%                     * ADD: option croatian: croatian keywords (thanks to Ivan Gavran)
%                     * ADD: option ngerman: same as german option but so can be used with global option ngerman
%                            of babel
%                     * ADD: option spanish: Spanish support (thanks to Mario Abarca)
%                     * ADD: unterminated block: useful to add part separator that doesn't necessary need an end
%                            keyword.  
%                            Designed on the pattern of unterminated if (see \uIf macro) allowing to
%                            add a block that is not terminated by a keyword. Such block are defined in the same
%                            time as a block is defined by adding a macro beginning with u. So, for example,
%                            predefined \SetKwBlock{Begin}{begin}{end} defines now two commands:
%                            - \Begin{} as previously which print a begin - end block
%                            - \uBegin{} that defines a begin only block
%                     * FIX: problem when numbering line inside until condition of
%                            \SetKwRepeat macro: line number was not correctly aligned.
%                     * FIX: dotocloa option which was broken
%                     * FIX: uIf and uCase didn't have same behavior when used with
%                            noline, vlined or lined option. This is fixed. Side effect: no empty
%                            line after an uIf or uCase when used with options lined or vlined
%                     * FIX: a bug with Repeat Until command when use with side comment on Until
%                     * FIX: a bug with side text -- text put into () -- of command macro (SetKwIf and so on)
%                            which was always setting a ';' even after a \DontPrintSemicolon
%                     * FIX: a bug with hyperref and chapter definition (thanks to Hubert Meier)
%                     * FIX: bugs with l macro and side comment
%                     * FIX: revision number
%                     * FIX: fix non ascii character (utf8 not yet recognized by all latex engine)
%                     * FIX: fnum@algocf had an useless parameter which sometimes broke expansion and output an error
%                     * FIX: works now with multicol package
%
%   - december 14 2009 - revision 4.1
%                     * ADD: new command \SetKwHangingKw{Name}{text} (hanging indent with keyword): This creates a
%                            hanging indent much like \texttt{SetKwInput}, except that it removes the trailing `:'
%                            and does not reset numbering (thanks to Nathan Tallent)
%
%   - november 17 2009  - revision 4.00 -
%
%                      * CHANGE: IMPORTANT: some commands have been renamed to have consistent naming (CamlCase
%                                syntax) and old commands are no more available. If you doesn't want to change
%                                your mind or use old latex files, you can use oldcommands option to enable old
%                                commands back.
%                                text. Here are these commands:
%                                - \SetNoLine becomes \SetAlgoNoLine
%                                - \SetVline  becomes \SetAlgoVlined
%                                - \Setvlineskip  becomes \SetVlineSkip
%                                - \SetLine   becomes \SetAlgoLined
%                                - \dontprintsemicolon becomes \DontPrintSemicolon
%                                - \printsemicolon becomes \PrintSemicolon
%                                - \incmargin becomes \IncMargin
%                                - \decmargin becomes \DecMargin
%                                - \setnlskip becomes \SetNlSkip
%                                - \Setnlskip becomes \SetNlSkip
%                                - \setalcapskip becomes \SetAlCapSkip
%                                - \setalcaphskip becomes \SetAlCapHSkip
%                                - \nlSty becomes \NlSty
%                                - \Setnlsty becomes \SetNlSty
%                                - \linesnumbered becomes \LinesNumbered
%                                - \linesnotnumbered becomes \LinesNotNumbered
%                                - \linesnumberedhidden becomes \LinesNumberedHidden
%                                - \showln becomes \ShowLn
%                                - \showlnlabel becomes \ShowLnLabel
%                                - \nocaptionofalgo becomes \NoCaptionOfAlgo
%                                - \restorecaptionofalgo becomes \RestoreCaptionOfAlgo
%                                - \restylealgo becomes \RestyleAlgo
%                                - gIf macros and so on do no more exist
%                      * NEW: - Compatibily with other packages improven by changing name of internal
%                               macros. Algorithm2e can now be used with arabtex for example, if this last is
%                               loaded after algorithm2e package.
%                      * ADD: - OPTION endfloat: endfloat packages doesn't allow float environment inside other
%                               environment. So using it with figure option of algorithm2e makes error. This
%                               option enables a new environment algoendfloat to be used instead of algorithm
%                               environment that put algorithm at the end. algoendfloat environment make
%                               algorithm acting as endfloat figures. This option requires endfloat packages.
%                      * ADD: - OPTION norelsize: starting from this release (v4.00), algorithm2e package uses
%                               relsize package in order to get relative size for lines numbers; but it seems
%                               that some rare classes (such as inform1.cls) are not compatible with relsize; to
%                               have algorithm2e working, this option makes algorithm2e not to load relsize
%                               package and go back to previous definition by using \scriptsize font for lines
%                               numbers.
%                      * ADD: - OPTION onelanguage: allow, if using standard keywords listed below, to switch
%                               from one language to another without changing keywords by using appropriate
%                               language option:
%                               . KwIn, KwOut, KwData, KwResult
%                               . KwTo KwFrom
%                               . KwRet, Return
%                               . Begin
%                               . Repeat
%                               . If, ElseIf, Else
%                               . Switch, Case, Other
%                               . For, ForPar, ForEach, ForAll, While
%                               .
%                      * ADD: - OPTION rightnl: put lines numbers to the right of the algorithm instead of left.
%                      * ADD:   new commands \setRightLinesNumbers and \setLeftLinesNumbers which sets the lines
%                               numbers to the right or to the left of the algorithm.
%                      * ADD: - new kind of keywords: KwArray used to define arrays:
%                               \SetKwArray{Kw}{array} defines an array keywords Kw called array and printed in
%                               DataSty style when call with \Kw. It can be used with one argument which
%                               denotes the element index: \Kw{n} prints array[n] with array in DataSty and n in
%                               ArgSty.
%                      * ADD/FIX: rules of ruled, algoruled, tworuled styles used rules of different sizes! This
%                                 is now fixed. Moreover size of the rules is now controlled by a length and so
%                                 can be customized by the user.
%                                 \algoheightrule is the height of the rules and can be changed via \setlength
%                                 \algoheightruledefault is the default height of he rules (0.8pt)
%                                 \algotitleheightrule is the height of the rule that comes just after the
%                                 caption in ruled and algoruled style; it can be changed via \setlength
%                                 \algotitleheightruledefault is the default height of this rules (0.8pt)
%                                 Thanks to Philippe Dumas who reports the bug and make the suggestion.
%                      * ADD: - \SetAlgoCaptionSeparator which sets the separator between Algorithm 1 and the
%                               title. By default it's ':' and caption looks like "Algorithm 2: title" but now
%                               you can change it by using for example \SetAlgoCaptionSeparator{.} which will
%                               give "Algorithm 3. title"
%                      * ADD: - \SetAlgoLongEnd and \SetAlgoShortEnd and \SetAlgoNoEnd commands which act as
%                               corresponding package options
%                      * ADD: - OPTIONS italiano and slovak as new language (thanks to Roberto Posenato and
%                               Miroslav Binas) 
%                      * CHANGE: - Fnt and Sty macro to have consistent use and naming (see below)
%                      * ADD: - \AlCapSty, \AlCapNameSty, \AlCapFnt, \AlCapNameFnt, \ProcSty, \ProcFnt,
%                               \ProcNameSty, \ProcNameFnt, \ProcArgSty, ProcArgFnt and corresponding "set macro" 
%                               \SetAlCapSty, \SetAlCapNameSty, \SetAlCapFnt, \SetAlCapNameFnt, \SetProcSty,
%                               \SetProcFnt, \SetProcNameSty, \SetProcNameFnt, \SetProcArgSty, \SetProcArgFnt which
%                               control the way caption is printed. Sty macro use command taking one parameter as
%                               argument, Fnt macros use directly command. In Fact caption is printed as follow:
%                               \AlCapSty{\AlCapFnt Algorithm 1:}\AlCapNameSty{\AlCapNameFnt my algorithm}
%                               By default, \AlCapSty is textbf and \AlCapFnt is nothing. \AlCapNameSty keep text 
%                               as it is, and \AlCapNameFnt do nothing also.
%                               You can redefine \AlCapFnt and \AlCapNameFnt by giving macro to \Set commands. For
%                               example, you can do \SetAlCapFnt{\large} to see Algorithm printed in \large font.
%                               You can redefine \AlCapSty, \AlCapFnt, \AlCapNameSty and \AlCapNameFnt with the
%                               corresponding \Set command. For the Sty commands, you have to give in parameter
%                               name of a macro (whithout \)  which takes one argument. For example,
%                               \SetAlCapFnt{textbf} defines the default behaviour. If you want to do more
%                               complicated thing, you should define your own macro and give it to \SetAlCapFnt or
%                               \SetAlCapNameFnt. Here are two examples:
%                               - \newcommand{\mycapsty}[1]{\tiny #1}\SetAlCapNameSty{mycapsty}
%                               - \newcommand{\mycapsty}[1]{\textsl{\small #1}}\SetAlCapNameSty{mycapsty}
%                               Or you can combine the two, for the last example you can also do:
%                               \SetAlCapNameSty{textsl}\SetAlCapNameFnt{\small}
%                               Thanks to Jan Stilhammer who gives me the idea of \AlCapNameFnt.
%                      * CHANGE \AlTitleFnt to match definition of all other Fnt macros and add a \AlTitleSty 
%                               macro (see below) . Now you set \AlTitleFnt by calling \SetAlTitleFnt with 
%                               directly a macro without parameter in argument:
%                               Example: \SetAlTitleFnt{\small} to set title in small font.
%                      * ADD: - \AlTitleSty and \SetAlTitleSty commands to set a style for title. These commands
%                               are defined from a macro taking the text in argument, as \textbf for example. 
%                               To set the TitleSty you have to give name of the macro (without the '\') 
%                               to \SetAlTitleSty. For example \SetAlTitleSty{textbf} to set \textbf style.
%                      * ADD: - new command \SetAlgorithmName{algorithmname}{list of algorithms name} which
%                               redefines name of the algorithms and the sentence list of algorithms. Second
%                               argument is the name that \autoref, from hyperref package, will use. Example:
%                               \SetAlgorithmName{Protocol}{List of protocols} if you prefer protocol than
%                               algorithm.
%                      * ADD: - new \SetAlgoRefName{QXY} which change the default ref (number of the algorithm) by
%                               the name given in parameter (QXY in the example). 
%                      * ADD: - new command \SetAlgoRefRelativeSize{-2} which sets the output size of refs, defined
%                               by \SetAlgoRefName, used in list of algorithms.
%                      * ADD: - two dimensions to control the layout of caption in ruled, algoruled and boxruled
%                               algorithms:
%                               - interspacetitleruled (2pt by defaut) which controls the vertical space between
%                                 rules and title in ruled and algoruled algorithms.
%                               - interspaceboxruled (2\lineskip by default) which controls the vertical space
%                                 between rules and title in boxruled algorithms.
%                               These two dimensions can be changed by using \setlength command.
%                      * ADD: - With the fix (see below) of procedure and function environments, a new feature has
%                               been added: the name of the procedure or function set in caption is automatically
%                               defined as a KwFunction and so can be used as a macro. For example, if inside a
%                               procedure environment you set \caption{myproc()}, you can use \myproc macro in you
%                               main text. Beware that the macro is only defined after the \caption!
%                      * ADD: - OPTION nokwfunc to unable the new feature described above in function and
%                               procedure environment. Useful if you use name of procedure or function that cannot
%                               be a command name as a math display for example.
%                      * ADD: - \SetAlgoNlRelativeSize{number} command which sets the relative size of line
%                               numbers. By default, line numbers are two size smaller than algorithm text. Use
%                               this macro to change this behavior. For example, \SetAlgoNlRelativeSize{0} sets it
%                               to the same size, \SetAlgoNlRelativeSize{-1} to one size smaller and
%                               \SetAlgoNlRelativeSize{1} to one size bigger
%                      * ADD: - \SetAlgoProcName{aname} command which sets the name of Procedure printed by
%                               procedure environment (the environment prints Procedure by default). Second
%                               argument is the name that \autoref, from hyperref package, will use.
%                      * ADD: - \SetAlgoFuncName{aname} command which sets the name of Function printed by
%                               procedure environment (the environment prints Function by default). Second
%                               argument is the name that \autoref, from hyperref package, will use. 
%                      * ADD: - \SetAlgoCaptionLayout{style} command which sets style of the caption; style must
%                               be the name of a macro taking one argument (the text of the caption). Examples
%                               below show how to use it:
%                               . \SetAlgoCaptionLayout{centerline} to have centered caption
%                               . \SetAlgoCaptionLayout{textbf} to have bold caption
%                               If you want to apply two styles in the same time, such as centered bold, you have
%                               to define you own macro and then use \SetAlgoCaptionLayout with its name.
%                      * ADD: - OPTION procnumbered: which makes the procedure and function to be numbered as
%                               algorithm
%                      * ADD: - OPTIONS tworuled and boxruled
%                               these are two new layouts: tworuled acts like ruled but doesn't put a line after
%                               caption ; boxruled surround algorithm by a box, puts caption above and add a line
%                               after caption.
%                      * REMOVE: - SetKwInParam has been deleted since not useful itself because of different
%                                macros which can do the same in a better and a more consistent way as
%                                SetKwFunction or SetKw.
%                      * FIX: - line number is now correctly vertically aligned with math display.
%                      * FIX: - references with hyperref. No more same identifier or missing name error. BUT now
%                               you must NOT use naturalnames option of hyperref packages if you do PdfLaTeX
%                      * FIX: - autoref with hyperref package (thanks to J?rg Sommer who notices the problem).
%                      * FIX: - titlenumbered was not working! fixed.
%                      * FIX: - Else(){} acted like uElse. Corrected.
%                      * FIX: - noend management: when a block was inside another and end of block was following
%                               each other, a blank line was added: it's now corrected.
%                      * FIX: - Function and Procedure environment was no more working as defined originally: the
%                               label was no more name of the procedure, it acts always as if procumbered option
%                               has been used.
%                      * FIX: - line numbers had a fixed size which can be bigger than algorithm text accordingly
%                               to \AlFnt set (see also new command \SetAlgoNlRelativeSize above)
%                      * FIX: - semicolon in comments when dontprintsemicolon is used.
%                      * FIX: - listofalgorithms adds a vertical space before first algo of a chapter as for
%                               listoffigures or listoftables
%                      * FIX: - listofalgorithms with twocolumns mode and some classes which don't allow onecolumn
%                               and so don't define \if@restonecol as prescribed in LaTeX (sig-alternate for
%                               example)
%                      * FIX: - algorithm2e now works with elsart cls and some more classes.
%                      * FIX: - blocks defined by SetKwBlock act now as other blocks (if for instance) and don't
%                               write end in vlined mode, instead they print a small horizontal line as required
%                               by the option.
%                      * FIX: - underfull hbox warning at each end of algorithm environment removed.
%
%                      * INTERNAL CHANGE: - short end keyword are deduce from long end keyword by keeping the
%                                           first one. Allows to avoid double definition.
%                      * INTERNAL CHANGE: - procedure, function and algorithm are now resolved by the same
%                               environment to avoid code duplication. 
%
%   - October  04 2005  - revision 3.9 -
%                      * ADD: - \setalcaphskip command which sets the horizontal skip before Algorithm: in caption
%                               when used in ruled algorithm.
%                      * ADD: - \SetAlgoInsideSkip command which allows to add an extra vertical space before and
%                               after the core of the algorithm (ie: \SetAlgoInsideSkip{bigskip}) 
%                      * CHANGE: - caption, when used with figure option, is no more controlled by algorithm2e
%                                  package and so follows the exact behaviour of figures. The drawback is that you
%                                  cannot change the typo with AlTitleFnt or CapFnt. The avantage is that if you
%                                  use caption package, it works.
%                      * FIX: - problem with numbering line and pdflatex
%                      * FIX: - error when algorithm2e package was used with beamer and listings together
%   - February 12 2005  - revision 3.8 -
%                      * FIX: - extra line with noend option.
%   - February 10 2005  - revision 3.7 -
%                      * ADD: - sidecomment: different macros allowing to put text right after code on the same
%                               line. They are defined in the same time comment macros are defined with a star
%                               after the macro name. By default comments are right justified but this can be
%                               change with appropriate option in the macro. Ex:
%                               . default: \tcc*{side comment}
%                               . same as previous: \tcc*[r]{side comment}
%                               . left justify: \tcc*[l]{side comment}
%                               . here: \tcc*[h]{side comment} don't put the end of line mark before
%                                       comment (; by default) and don't end the line.
%                               . flushed: \tcc*[f]{side comment} same as the precedent but right
%                                 justified
%                      * ADD: - OPTION scright (default): right justified side comments (side comments
%                               are flushed to the righr)
%                      * ADD: - OPTION scleft: left justified side comments (side comments are put right after the
%                               code line)
%                      * ADD: - \SetSideCommentLeft acts as scleft option
%                      * ADD: - \SetSideCommentRight acts as scright option
%                      * ADD: - block like macro side text: all macro defining a block allows now to put text right
%                               after key words by putting text into (). Done to be used with sidecomment macros,
%                               but all text can be used. 
%                               Ex: \eIf(\tcc*[f]{then comment}){test}{then text}(else side text){else text}
%                      * ADD: - OPTION fillcomment (default): end mark of comment is flushed to the right so
%                               comments fill all the width of text.
%                      * ADD: - OPTION nofillcomment: end mark of comment is put right after the comment.
%                      * ADD: - \SetNoFillComment acts as nofillcomment option.
%                      * ADD: - \SetFillComment acts as fillcomment option.
%                      * ADD: - OPTION dotocloa: which adds an entry in the toc for the list of algorithms. This
%                               option load package tocbibind if not already done and so list of figures and list
%                               of tables are also added in the toc. If you want to control which ones of the lists
%                               will be added in the toc, please load package tocbibind before package algorithm
%                               and give it the options you want.
%                      * FIX: - vertical spacing for uif macro with noend option
%                      * FIX: - all the compatibility problems between caption and other packages
%                      * FIX: - typographical differences between list of algorithms and other lists  when in
%                               report or book 
%
%   - January 24 2005  - revision 3.6 -
%                      * FIX: - vertical spacing and space characters at the beginning or end of comments.
%                               line numbers of comments not in the NlSty.
%                               Thanks to Arnaud Giersch for his comments and suggestions.
%                      * FIX: - Set*Sty macro: the styles defined was not protected and was modified by surrounding
%                               context. For example KwTo in a \For{}{} was in bold AND italic instead of just in
%                               bold.
%                      * FIX: - line number misplacement after \Indp
%
%   - January 21 2005  - revision 3.5 -
%                      * ADD: - hidden numbering of the lines. Lines are auto-numbered but numbers are shown only
%                               on lines you specify:
%                               * linesnumberedhidden option or \LinesNumberedHidden macro activate this
%                                 functionnality.
%                               * \ShowLn and \ShowLnLabel{lab} macros make the number visible on the
%                               line. \ShowLnLabel{lab} allows to set a label for this line. 
%                               Thanks to Samson de Jager who makes this suggestion and provides the macros.
%                      * ADD: - \AlCapFnt and \SetAlCapFnt which allow to have a different font for
%                               caption. Works like \AlFnt and \SetAlFnt and by default is the same.
%                      * ADD: - \AlCapSkip skip length. This vertical space is added before caption in plain ou
%                               boxed mode. It allows to change distance between text and caption.
%                      * FIX: - caption compatible with IEEEtran class. 
%                      * FIX: - some vertical spacing error with \uIf macros (Thanks to Arnaud Giersch)
%                      * FIX: - Procedure and Function: lines are also numbered like algorithms
%                      * FIX: - CommentSty was not used for Comments
%
%   - January 10 2005  - revision 3.4 -
%                      * FIX: - caption compatible with new release of Beamer class. 
%
%   - June 16 2004     - revision 3.3 - 
%                      * FIX: - Hyperlink references of Hyperref package works now if compiled with pdflatex 
%                               and [naturalnames] option of hyperref package is used.
%                      * FIX: - algorithm[H] had problem in an list environment - corrected
%                      * FIX: - interline was not so regular in nested blocks - corrected
%                      * ADD  - \SetVlineSkip macro which sets the vertical skip after the little horizontal 
%                               rule which closes a block in Vlined mode. By default 0.8ex
%
%   - June 11 2004     - revision 3.2 - AUTO NUMBERING LINES !!!
%                      * ADD: auto numbering of the lines (the so asked and so long awaiting feature)
%                             this feature is managed by 3 options and 3 commands:
%                             - linesnumbered option: lines of the algo are numbered except for comments and
%                               input/output (KwInput and KwInOut)
%                             - commentsnumbered option: makes comments be numbered
%                             - inoutnumbered option: makes data input/output be numbered
%                             - \nllabel{lab} labels the line so you can cite with \ref{lab}
%                             - \LinesNumbered make the following algorithms having auto-numbered lines
%                             - \linesnotnumbered make the following algorithms having no auto-numbered lines
%                      * Change: algo2e option renames listofalgorithms in listofalgorithmes
%                      * FIX: new solution for compatibility with color package, more robust and not tricky.
%                             Many thanks to David Carlisle for his advices
%
%   - June 09 2004     - revision 3.1 -
%                      * Change: \SetKwSwitch command defines an additionnal macro \uCase and \Case prints end
%                      * Change: now macros SetKw* do a renewcommand if the keyword is already defined. So you can
%                                redefine default definition at your own convenience or change your definition
%                                without introducing a new macro and changing your text.
%                      * ADD: new macro \SetKwIF which do \SetKwIf and
%                             \SetKwIfElseIf.The following default definition has been added:
%                             \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
%                             and so you get the macros;
%                             \If \eIf \lIf \uIf \ElseIf \uElseIf \lElseIf \Else \uElse \lElse
%                      * ADD: new macro \SetAlgoSkip which allow to fix the vertical skip before and after the
%                             algorithms. Default is smallskip, do \SetAlgoSkip{} if you don't want an extra space
%                             or \SetAlgoSkip{medskip} or \SetAlgoSkip{bigskip} if you want bigger space.
%                      * ADD: macro \SetKwIf defines in addition a new macro \uElse  (depending on wat name you
%                             have given in #2 arg).
%                      * ADD: macro \SetKwIfElseIf defines in addition a new macro \uElse and \ugElseIf (depending
%                             on what name you have given in #2 and #3 arg).
%                      * Change: baseline of algorithm is now top, so two algorithms can be put side by side.
%                      * FIX: Compatibility with color package solved. The problem was due to a redefinition of
%                             standard macros by color package. This solves compatibility problem with other
%                             packages as pstcol or colortbl. (notified by Dirk Fressmann, Antti Tarvainen and Koby
%                             Crammer)
%                      * Fix: extra little shift to the right with boxed style algorithm removed (notified by
%                             P. Tanovski)
%                      * Fix: algoln option was buggy (notified bye Jiaying Shen)
%                      * Fix: german and portuges option didn't work due to bad typo (notified by Martin Sievers,
%                             Thorsten Vitt and Jeronimo Pellegrini)
%                      
%   - February 13 2004 - revision 3.0 -
%                      * Major revision which makes the package independent from float.sty, so now
%                        - algorithm* works better, in particular can be used in multicols environments
%                        - (known bug corrected)
%                          [H] works now for all sort of environment but is handled differently for classic
%                          environment and star environment (algorithm, figure, procedure and function). For star
%                          environment, H acts like for classical figure environment, so it doesn't stay here
%                          absolutely.
%                        - (known bug corrected)
%                          you can use now floatflt package with algorithm package and even with figure
%                          option. Beware that if you want to put an algorithm inside a floatingfigure, it cannot
%                          be floating, so [H] is required and then figure option should not be used, since
%                          standard figure[H] are still floating with LaTeX.
%                      * boxruled: a new style added. Possible now since no style no more defined by the float
%                        package.
%                      * nocaptionofalgo: dosen't print Algorithm #: in the caption for algorithm in ruled or
%                        algoruled style.
%                        note: this is just documentation of a macro which was already in the package.
%   - December 14 2003 - revision 2.52 -
%                      * output message shorter
%                      * French keyword macro \PourTous was missing for longend option, it has been added.
%                      * TitleofAlgo prints Function or Procedure in corresponding environments.
%
%   - October 27 2003  - revision 2.51 - Revision submitted to CTAN archive
%                      * correction of a minor which make caption in procedure
%                        and function to be blanck with pdfscreen package
%                        (thanks to Joel Gossens for the notification)
%                      * add two internal definition to avoid some errors when
%                        used with Hyperref package (Hyperref package need to
%                        define new counter macro from existing ones, and
%                        don't do it for algorithm2e package, so we do it)
%
%   - October 17 2003  - revision 2.50 - first revision for CTAN archive
%                      * add \AlFnt and \SetAlFnt{font} macros: \AlFnt is used at the beginning of the caption and
%                        the body of algorithm in order to define the fonts used for typesetting algorithms. You
%                        can use it elsewhere you want to typeset text as algorithm. For example you can do
%                        \SetAlFnt{\small\sf} to have algorithms typeset in small sf font. Default is nothing so
%                        algorithm is typeset as the text of the document.
%                      * add \AlTitleFnt{text} and \SetAlTitleFnt{font} macros: The {Algorithm: } in the caption is
%                        typeset with \AlTitleFnt{Algorithm:}. You can use it to have text typeset as {Algorithm:}
%                        of captions. Default is textbf.  Default can be redefined by \SetAlTitleFnt{font}, for
%                        example you can do \SetAlTitleFnt{emph}
%                      * add CommentSty typo for text comment.  
%                      * add some compatibility with hyperref package (still an error on multiply defined refs but
%                        pdf correctly generated)
%                      * flush text to left in order to have correct indentation even with class as amsart which
%                        center all figures
%                      * add german, portuguese and czech options for title of algorithms and typo.
%                      * add portuguese translation of predefined keywords * add czech translation of some
%                        predefined keywords
%
%   - December 23 2002 - revision 2.40
%                      * add some French keyword missing
%                      * add function* and procedure* environment like algorithme* environment: print in one column
%                        even if twocolumn option is specified for the document.
%                      * add a new macro \SetKwComment to define macro which writes comments in the text. First
%                        argument is the name of the macro, second is the text put before the comment, third is the
%                        text put at the end of the comment.Default are \tcc and \tcp
%                      * add new options to change the way algo are numbered:
%                        [algopart] algo are numbered within part (counter must exist)
%                        [algochapter] algo are numbered within chapter
%                        [algosection] algo are numbered within section
%
%   - March 27 2002   - revision 2.39
%                      * Gilles Geeraerts: added the \SetKwIfElseIf to manage
%                        if (c)
%                             i;
%                        else if (c)
%                             i;
%                        ...
%                        else
%                             i;
%                        end
%                      * Also added \gIf \gElseIf \gElse.
%
%   - January 02 2001 - revision 2.38
%                      * bugs related to the caption in procedure and function
%                        environment are corrected.
%                      * bug related to option noend (extra vertical space added
%                        after block command as If or For) is corrected.
%                      * czech option language added (thanks to Libor Bus: l.bus@sh.cvut.cz).
%  
%   - October 16 2000 - revision 2.37
%                      * option algo2e added: change the name of environment
%                        algorithm into algorithm2e. So allow to use the package
%                        with some journal style which already define an algorithm
%                        environment.
%  
%   - September 13 2000 - revision 2.36
%                      * option slide added: require package color
%                      * Hack for slide class in order to have correct
%                        margins
%  
%   - November 25 1999 - revision 2.35
%                      * revision number match RCS number
%                      * Thanks to David A. Bader, a new option is added:
%                        noend: no end keywords are printed.
%  
%   - November 19 1999 - revision 2.32
%                      * minor bug on longend option corrected.
%  
%   - August 26 1999 - revision 2.31
%                      * add an option: figure
%                        this option makes algorithms be figure and so are numbered
%                        as figures, have Figure as caption and are put in 
%                        the \listoffigures
%  
%   - January 21 1999 - revision 2.3 beta
%                    add 2 new environments: procedure and function.
%                    These environments works like algorithm environment but:
%                    - the ruled (or algoruled) style is imperative.
%                    - the caption now writes Procedure name....
%                    - the syntax of the \caption command is restricted as
%                      follow: you MUST put a name followed by 2 braces like
%                      this ``()''. You can put arguments inside the braces and
%                      text after. If no argument is given, the braces will be
%                      removed in the title. 
%                    - label now puts the name (the text before the braces in the
%                      caption) of the procedure or function as reference (not
%                      the number like a classic algorithm environment).
%                    There are also two new styles: ProcNameSty and
%                    ProcArgSty. These style are by default the same as FuncSty
%                    and ArgSty but are used in the caption of a procedure or a
%                    function.
%                    
%   - November 28 1996 - revision 2.22
%                    add a new macro \SetKwInParam{arg1}{arg2}{arg3}:
%                    it defines a macro \arg1{name}{arg} which prints name in keyword
%                    style followed byt arg surrounded by arg2 and arg3. The main
%                    application is to a function working as \SetKwInput to be used
%                    in the head of the algorithm. For example
%                    \SetKwInParam{Func}{(}{)} allows
%                    \Func{functionname}{list of arguments} which prints:
%                    \KwSty{functioname(}list of arguments\KwSty{)}
%       
%
%   - November 27 1996 - revision 2.21:
%                    minor bug in length of InOut boxes fixed.
%                    add algorithm* environment.
%
%   - July 12 1996 - revision 2.2: \SetArg and \SetKwArg macros removed.
%                        
%                    \SetArg has been removed since it never has been
%                    documented.
%                    \SetKwArg has been removed since \SetKw can now
%                    take an argument in order to be consistent with
%                    \SetKwData and \SetKwFunction macros.
%
%   - July 04 1996 - revision 2.1: still more LaTeX2e! Minor compatibility break
%
%                    Macros use now \newcommand instead of \def, use of \setlength, 
%                    \newsavebox, ... and other LaTeX2e specific stuff.
%                    The compatibility break:
%                    - \SetData becomes \SetKwData to be more consistent. So the old 
%                      \SetKwData becomes \SetKwInput
%                    - old macros \titleofalgo, \Freetitleofalgo and \freetitleofalgo
%                      from LaTeX209 version which did print a warning message and call 
%                      \Titleofalgo in version 2.0 are now removed!
%
%   - March 13 1996 - revision 2.0: first official major revision.
%   
%
%%%%%%%%%%%%%%
%
%   Known bugs: 
%   -----------
%   - horizontal spacing (indent) doesn't work with revtex4 class.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% for more complete informations you can see algorithm2e.tex
%
%
%%%%%%%%%%%%%%%%%%%%%%%% Identification Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
%
\ProvidesPackage{algorithm2e}[2013/01/06 v5.00 algorithms environments]
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Initial Code %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\@makeother\*% some package redefined it as a letter (as color.sty)
\def\@firstword#1 #2\@nil{#1}% an useful fonction
%%%%%%% Utilities:
% \ifArgumentEmpty<c><t><e> ; if c is empty, i.e. {}, then t, else e.
%    Function used internally, but may as well expose it to the user; it's useful
\begingroup
\catcode`\Q=3
\catcode`\T=3
\long\gdef\ALGOCF@argemptyaux#1#2Q#3#4#5T{#4}
\long\gdef\ifArgumentEmpty#1{%
  \begingroup\long\edef\@tempa{\endgroup
    \ALGOCF@argemptyaux#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T%
  }\@tempa
}
\endgroup
% \long\def\ifArgumentEmpty#1{\bgroup
% 	\catcode`\Q=3
% 	\catcode`\T=3
% 	\long\def\@tempa##1##2Q##3##4##5T{##4}%
% 	\xdef\@tempa{\@tempa#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T}%
% \egroup\@tempa}
%%%%%%%%%%%
%
% \algocf@longdef -> shorthand to reduce
%    \expandafter\long\expandafter\def
% to
%    \expandafter\algocf@longdef
% may look insignificant, but reads that much better ;)
\def\algocf@longdef{\long\def}
%
% \algocf@newcommand (and helper \algocf@new@command) behaves like LaTeX's newcommand,
% with two differences:
%  - the argument is not "\<name>", but rather "<name>"; i.e. one level of indirection
%  - if the command exists already, then \renewcommand, rather than \newcommand
\def\algocf@newcommand#1{\expandafter\algocf@new@command\csname#1\endcsname}
\def\algocf@new@command#1{%
	\begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
	\expandafter\@ifundefined\@gtempa\newcommand\renewcommand#1}%
%
% \algocf@newcmdside<name><arity><body>
%   The largest time-saver; many commands we define have the pattern:
%     \<name>(<side_text>)<argX><argY>...
%   where "(<side_text>)" is optional. By defining them with this function,
%   the arguments are parsed and renumbered, i.e. the body works as if the
%   command was:
%     \<name><side_text><argX><argY>...
%   and can use \ifArgumentEmpty to see whether its #1 exists (default case
%   for the side text is (), so there's no difference between calling
%     \foo{bar}
%   or
%     \foo(){bar}
%   Technically this is new behaviour, but it shouldn't really occur...
\algocf@longdef\algocf@newcmdside#1#2#3{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3}%
}
%
% a serie of newcmdside macro for block that allows a comment after the end
%     \<name>(<side_text>)<argX><argY>...(<side_text>)% 
%
% 1. kind of begin-end : for command with only one block as begin-end 
\algocf@longdef\algocf@newcmdside@kobe#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2{\csname algocf@#1checkcomfol\endcsname{##1}{##2}}%
  % now check for last side comment; args are : <first side com (could be empty)>, <body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}}{\csname algocf@#1noendcom\endcsname{##1}{##2}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2(##3){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2{%
    \csname algocf@#1main\endcsname{##1}{##2}{}}%
  \algocf@newcommand{algocf@#1main}[3]{#2}%
}%
%
% 2. kind of if-else : for command with two blocks as if-then-else 
\algocf@longdef\algocf@newcmdside@koif#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2##3{\csname algocf@#1checkcomfol\endcsname{##1}{##2}{##3}}%
  % now check for last side comment; args are : <1st side com>, <1st body of cmd>, <2nd body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2##3{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}{##3}}{\csname algocf@#1noendcom\endcsname{##1}{##2}{##3}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2##3(##4){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{##4}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2##3{%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{}}%
  \algocf@newcommand{algocf@#1main}[4]{#2}%
}%
%
% \algocf@newcmdsides<name><arity><body><tail><closing>
%   Like the command above, but with an optional side text at the end
%   of the command as well, i.e.:
%     \<name>(<side_text>)<argX><argY>(<end_text>)
%   It may be a bit confusing that <arity> doesn't count <end_text>,
%   but since it is for internal use, the naming can be a little more
%   fuzzy. This function behaves as if:
%     <body'> = <body><if end_text: tail{end_text}><closing>
\algocf@longdef\algocf@newcmdsides#1#2#3#4#5{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3\@ifnextchar({\csname algocf@#1end\endcsname}{#4#5}}%
	\expandafter\algocf@longdef\csname algocf@#1end\endcsname(##1){#4{##1}\strut\par}%
}%
%
% definition of commands which can be redefined in options of the package.
%
\newcounter{AlgoLine}%
\setcounter{AlgoLine}{0}%
%
\newcommand{\algocf@algocfref}{\relax}%
\newcommand{\listalgorithmcfname}{}%
\newcommand{\algorithmcfname}{}%
\@ifundefined{algorithmautorefname}{\newcommand{\algorithmautorefname}{algorithm}}{\renewcommand{\algorithmautorefname}{algorithm}}%
\newcommand{\algorithmcflinename}{}%
\newcommand{\algocf@typo}{}%
\newcommand{\@algocf@procname}{}\newcommand{\procedureautorefname}{}%
\newcommand{\SetAlgoProcName}[2]{\renewcommand{\@algocf@procname}{#1}\renewcommand{\procedureautorefname}{#2}}%
\newcommand{\@algocf@funcname}{}\newcommand{\functionautorefname}{}%
\newcommand{\SetAlgoFuncName}[2]{\renewcommand{\@algocf@funcname}{#1}\renewcommand{\functionautorefname}{#2}}%
\newcommand{\@algocf@titleofalgoname}{\algorithmcfname}%
\newcommand{\@algocf@algotitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algorithmcfname}}%
\newcommand{\@algocf@proctitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algocf@procname}}%
%
\newcommand{\algocf@style}{plain}%
\newcommand{\@ResetCounterIfNeeded}{}%
\newcommand{\@titleprefix}{}%
%
\newcommand{\algocf@numbering}[1]{\newcommand{\algocf@within}{#1}}%
%
\newcommand{\defaultsmacros@algo}{\algocf@defaults@shortend}%
%
\newcommand{\algocf@list}{loa}%
\newcommand{\algocf@float}{algocf}%
%
\newcommand{\algocf@envname}{algorithm}%
\newcommand{\algocf@listofalgorithms}{listofalgorithms}%
%
%
%% redefine chapter so that it adds a vspace in the loa as the original does for lof and lot
% \let\algocf@original@chapter=\chapter%
% \def\chapter{\expandafter\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}%
%
% bug correction with hyperref submitted by Hubert Meier
\begingroup\expandafter\expandafter\expandafter\endgroup 
\expandafter\ifx\csname @chapter\endcsname\relax\else 
% \let\algocf@original@chapter=\chapter% 
% \def\chapter{\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}% 
\let\algocf@original@chapter=\@chapter%
\@ifclassloaded{krantz}{%
\def\@chapter[#1][#2]#3{\algocf@original@chapter[#1][#2]{#3}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}{%
\def\@chapter[#1]#2{\algocf@original@chapter[#1]{#2}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}%
\fi
%
%% if@restonecol is defined in article and book but some other classes don't define it and we need it, so we do
\ifx\if@restonecol\relax\else\newif\if@restonecol\fi%
%
%
%%%%%%%%%%%%%%%%%%%%%% Declaration of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\RequirePackage{ifthen}%
%
\newboolean{algocf@displayblockmarkers}\setboolean{algocf@displayblockmarkers}{false}%
\DeclareOption{displayblockmarkers}{%
  \setboolean{algocf@displayblockmarkers}{true}%
}
\newboolean{algocf@displaygroupmarkers}{\setboolean{algocf@displaygroupmarkers}{false}
\DeclareOption{displaygroupmarkers}{%
  \setboolean{algocf@displaygroupmarkers}{true}%
}
%
\newboolean{algocf@nokwfunc}\setboolean{algocf@nokwfunc}{false}%
\DeclareOption{nokwfunc}{%
  \setboolean{algocf@nokwfunc}{true}%
}%
%
\newboolean{algocf@oldcommands}\setboolean{algocf@oldcommands}{false}%
\DeclareOption{oldcommands}{%
  \setboolean{algocf@oldcommands}{true}%
}%
%
\newboolean{algocf@leftlinenumber}\setboolean{algocf@leftlinenumber}{true}%
\newcommand{\setLeftLinesNumbers}{\setboolean{algocf@leftlinenumber}{true}}%
\newcommand{\setRightLinesNumbers}{\setboolean{algocf@leftlinenumber}{false}}%
\DeclareOption{rightnl}{%
  \setRightLinesNumbers%
}%
%
\newboolean{algocf@endfloat}\setboolean{algocf@endfloat}{false}%
\DeclareOption{endfloat}{%
  \setboolean{algocf@endfloat}{true}%
  \newcounter{postalgo}\setcounter{postalgo}{0}%
}%
%
\newboolean{algocf@procnumbered}\setboolean{algocf@procnumbered}{false}%
\DeclareOption{procnumbered}{%
  \setboolean{algocf@procnumbered}{true}%
}%
%
\DeclareOption{algo2e}{%
  \renewcommand{\algocf@envname}{algorithm2e}%
  \renewcommand{\algocf@listofalgorithms}{listofalgorithmes}%
}%
%
\newboolean{algocf@slide}\setboolean{algocf@slide}{false}%
\DeclareOption{slide}{%
  \setboolean{algocf@slide}{true}%
}%
%
\newboolean{algocf@figurecaption}\setboolean{algocf@figurecaption}{false}%
\DeclareOption{figure}{%
\renewcommand{\algocf@list}{lof}%
\renewcommand{\algocf@float}{figure}%
\AtBeginDocument{\@ifpackageloaded{caption}{\setboolean{algocf@figurecaption}{true}}{}}%
}%
%
\newboolean{algocf@optonelanguage}\setboolean{algocf@optonelanguage}{false}%
\DeclareOption{onelanguage}{\setboolean{algocf@optonelanguage}{true}}%
%
\newcommand{\algocf@languagechoosen}{english}%
\newboolean{algocf@localkw@english}\setboolean{algocf@localkw@english}{true}%
\DeclareOption{englishkw}{%
\setboolean{algocf@localkw@english}{true}%
}%
%
\DeclareOption{english}{%
\renewcommand{\listalgorithmcfname}{List of Algorithms}%
\renewcommand{\algorithmcfname}{Algorithm}%
\renewcommand{\algorithmautorefname}{algorithm}%
\renewcommand{\algorithmcflinename}{line}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedure}%
\renewcommand{\@algocf@funcname}{Function}%
\renewcommand{\procedureautorefname}{procedure}%
\renewcommand{\functionautorefname}{function}%
\renewcommand{\algocf@languagechoosen}{english}%
}%
%
%----
\newboolean{algocf@localkw@french}\setboolean{algocf@localkw@french}{false}%
\DeclareOption{frenchkw}{%
\setboolean{algocf@localkw@french}{true}%
}%
%
\DeclareOption{french}{%
\renewcommand{\listalgorithmcfname}{Liste des Algorithmes}%
\renewcommand{\algorithmcfname}{Algorithme}%
\renewcommand{\algorithmautorefname}{algorithme}%
\renewcommand{\algorithmcflinename}{ligne}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Proc\'edure}%
\renewcommand{\@algocf@funcname}{Fonction}%
\renewcommand{\procedureautorefname}{proc\'edure}%
\renewcommand{\functionautorefname}{fonction}%
\renewcommand{\algocf@languagechoosen}{french}%
}%
%
%----
\newboolean{algocf@localkw@czech}\setboolean{algocf@localkw@czech}{false}%
\DeclareOption{czechkw}{%
\setboolean{algocf@localkw@czech}{true}%
}%
%
\DeclareOption{czech}{%
\renewcommand{\listalgorithmcfname}{Seznam algoritm\r{u}}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkce}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{czech}%
}%
%
%----
\newboolean{algocf@localkw@german}\setboolean{algocf@localkw@german}{false}%
\DeclareOption{germankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{german}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\DeclareOption{ngermankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{ngerman}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\newboolean{algocf@localkw@portuguese}\setboolean{algocf@localkw@portuguese}{false}%
\DeclareOption{portuguesekw}{%
\setboolean{algocf@localkw@portuguese}{true}%
}%
%
\DeclareOption{portuguese}{%
\renewcommand{\listalgorithmcfname}{Lista de Algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{linha}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimento}%
\renewcommand{\@algocf@funcname}{Fun\c{c}\~{a}o}%
\renewcommand{\procedureautorefname}{procedimento}%
\renewcommand{\functionautorefname}{fun\c{c}\~{a}o}%
\renewcommand{\algocf@languagechoosen}{portuguese}%
}%
%
%----
\newboolean{algocf@localkw@italiano}\setboolean{algocf@localkw@italiano}{false}%
\DeclareOption{italianokw}{%
\setboolean{algocf@localkw@italiano}{true}%
}%
%
\DeclareOption{italiano}{%
\renewcommand{\listalgorithmcfname}{Elenco degli algoritmi}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{riga}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funzione}%
\renewcommand{\procedureautorefname}{procedura}%
\renewcommand{\functionautorefname}{funzione}%
\renewcommand{\algocf@languagechoosen}{italiano}%
}%
%----
\newboolean{algocf@localkw@spanish}\setboolean{algocf@localkw@spanish}{false}%
\DeclareOption{spanishkw}{%
\setboolean{algocf@localkw@spanish}{true}%
}%
%
\DeclareOption{spanish}{%
\renewcommand{\listalgorithmcfname}{\'Indice de algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{l\'inea}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimiento}%
\renewcommand{\@algocf@funcname}{Funci\'on}%
\renewcommand{\procedureautorefname}{procedimiento}%
\renewcommand{\functionautorefname}{funci\'on}%
\renewcommand{\algocf@languagechoosen}{spanish}%
}%
%----
\newboolean{algocf@localkw@slovak}\setboolean{algocf@localkw@slovak}{false}%
\DeclareOption{slovakkw}{%
\setboolean{algocf@localkw@slovak}{true}%
}%
%
\DeclareOption{slovak}{%
\renewcommand{\listalgorithmcfname}{Zoznam algoritmov}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Proced\'{u}ra}%
\renewcommand{\@algocf@funcname}{Funkcia}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{slovak}%
}%
%
%----
\newboolean{algocf@localkw@croatian}\setboolean{algocf@localkw@croatian}{false}%
\DeclareOption{croatiankw}{%
\setboolean{algocf@localkw@croatian}{true}%
}%
%
\DeclareOption{croatian}{%
\renewcommand{\listalgorithmcfname}{Popis algoritama}%
\renewcommand{\algorithmcfname}{Algoritam}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{redak}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkcija}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{croatian}%
}%
%%% adding 'turkish' option customization
%
%----
\newboolean{algocf@localkw@turkish}\setboolean{algocf@localkw@turkish}{false}%
\DeclareOption{turkishkw}{%
\setboolean{algocf@localkw@turkish}{true}%
}%
\DeclareOption{turkish}{%
\renewcommand{\listalgorithmcfname}{Algoritma Listesi}%
\renewcommand{\algorithmcfname}{Algoritma}%
\renewcommand{\algorithmautorefname}{algoritma}%
\renewcommand{\algorithmcflinename}{?izgi}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Prosed?r}%
\renewcommand{\@algocf@funcname}{Fonksiyon}%
\renewcommand{\procedureautorefname}{prosed?r}%
\renewcommand{\functionautorefname}{fonksiyon}%
\renewcommand{\algocf@languagechoosen}{turkish}%
}%
%
% OPTIONs plain, boxed, ruled, algoruled & boxruled
%
\newcommand{\algocf@style@plain}{\renewcommand{\algocf@style}{plain}}%
\newcommand{\algocf@style@boxed}{\renewcommand{\algocf@style}{boxed}}%
\newcommand{\algocf@style@ruled}{\renewcommand{\algocf@style}{ruled}}%
\newcommand{\algocf@style@algoruled}{\renewcommand{\algocf@style}{algoruled}}%
\newcommand{\algocf@style@boxruled}{\renewcommand{\algocf@style}{boxruled}}%
\newcommand{\algocf@style@tworuled}{\renewcommand{\algocf@style}{tworuled}}%
\newcommand{\algocf@style@plainruled}{\renewcommand{\algocf@style}{plainruled}}%
\newcommand{\RestyleAlgo}[1]{\csname algocf@style@#1\endcsname}%
\DeclareOption{plain}{\algocf@style@plain}%
\DeclareOption{plainruled}{\algocf@style@plainruled}%
\DeclareOption{boxed}{\algocf@style@boxed}%
\DeclareOption{ruled}{\algocf@style@ruled}%
\DeclareOption{algoruled}{\algocf@style@algoruled}%
\DeclareOption{boxruled}{\algocf@style@boxruled}%
\DeclareOption{tworuled}{\algocf@style@tworuled}%
%
% OPTIONs algopart,algochapter & algosection
%
\DeclareOption{algopart}{\algocf@numbering{part}}%       %algo part numbered
\DeclareOption{algochapter}{\algocf@numbering{chapter}}% %algo chapter numbered
\DeclareOption{algosection}{\algocf@numbering{section}}% %algo section numbered
%
% OPTIONs resetcount & noresetcount
%
\DeclareOption{resetcount}{\renewcommand{\@ResetCounterIfNeeded}{\setcounter{AlgoLine}{0}}}%
\DeclareOption{noresetcount}{\renewcommand{\@ResetCounterIfNeeded}{}}%
%
% OPTIONs algorithm hanging for long lines
%
\newlength{\algocf@hangindent}\setlength{\algocf@hangindent}{.5em}
\newcommand{\SetAlgoHangIndent}[1]{\setlength{\algocf@hangindent}{#1}}
%
\newboolean{algocf@hanging}\setboolean{algocf@hanging}{true}% hanging is handle by default
\newboolean{algocf@hanginginout}\setboolean{algocf@hanginginout}{false}% inout are managed as previously: hanging set by inout keywords
\newboolean{algocf@hangingcomment}\setboolean{algocf@hangingcomment}{false}% comment that are not side comment are indented accordingly to comment mark, not as normal text
\newcommand{\algocf@everyparnl}{\relax}%
\newcommand{\algocf@everyparhanging}{\hangafter=1\hangindent=\algocf@hangindent\relax}%
\newcommand{\algocf@everypar}{\algocf@everyparnl\algocf@everyparhanging}%
\newcommand{\algocf@seteverypar}{%
  \ifthenelse{\boolean{algocf@hanging}}{\everypar{\algocf@everypar}}{\relax}%
}%
%
\newcommand{\algocf@seteveryparnl}[1]{\renewcommand{\algocf@everyparnl}{#1}\everypar{\algocf@everypar}}%
\newcommand{\algocf@seteveryparhanging}[1]{%
\let\algocf@oldeveryparhanging=\algocf@everyparhanging%
\renewcommand{\algocf@everyparhanging}{#1}\everypar{\algocf@everypar}%
}%
\newcommand{\algocf@reseteveryparhanging}{%
\let\algocf@everyparhanging=\algocf@oldeveryparhanging%
\everypar{\algocf@everypar}%
}%
\DeclareOption{hanginginout}{\setboolean{algocf@hanginginout}{true}}%
\DeclareOption{hangingcomment}{\setboolean{algocf@hangingcomment}{true}}%
\DeclareOption{noalgohanging}{%
  \setboolean{algocf@hanginginout}{false}%
  \setboolean{algocf@hangingcomment}{false}%
  \setboolean{algocf@hanging}{false}%
}%
%\newcommand{
%
%
% OPTION linesnumbered
%
\newboolean{algocf@linesnumbered}\setboolean{algocf@linesnumbered}{false}%
\newcommand{\algocf@linesnumbered}{\relax}%
\DeclareOption{linesnumbered}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}%
}%
%
% OPTION linesnumberedhidden
%
\DeclareOption{linesnumberedhidden}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}%
}%
%
% OPTION commentsnumbered inoutnumbered
%
\newboolean{algocf@commentsnumbered}\setboolean{algocf@commentsnumbered}{false}%
\DeclareOption{commentsnumbered}{\setboolean{algocf@commentsnumbered}{true}}%
\newboolean{algocf@inoutnumbered}\setboolean{algocf@inoutnumbered}{false}%
\DeclareOption{inoutnumbered}{\setboolean{algocf@inoutnumbered}{true}}%
%
% OPTIONs titlenumbered & titlenotnumbered
%
\DeclareOption{titlenumbered}{%
  \renewcommand{\@titleprefix}{%
    \refstepcounter{\algocf@float}%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\ \expandafter\csname the\algocf@float\endcsname\algocf@typo: }%
  }%
}%
%
\DeclareOption{titlenotnumbered}{\renewcommand{\@titleprefix}{%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\algocf@typo: }}%
}%
%
% OPTIONs algonl
% line numbered with the counter of the algorithm
%
\DeclareOption{algonl}{\renewcommand{\theAlgoLine}{\expandafter\csname the\algocf@float\endcsname.\arabic{AlgoLine}}}%
%
% OPTIONs lined, vlined & noline
%
\DeclareOption{lined}{\AtBeginDocument{\SetAlgoLined}}%   \SetAlgoLined (default)
\DeclareOption{vlined}{\AtBeginDocument{\SetAlgoVlined}}% \SetAlgoVlined
\DeclareOption{noline}{\AtBeginDocument{\SetAlgoNoLine}}%\SetAlgoNoLine
%
% OPTIONs longend, shotend & noend
%
\DeclareOption{longend}{\AtBeginDocument{\SetAlgoLongEnd}}%  \SetAlgoLongEnd
\DeclareOption{shortend}{\AtBeginDocument{\SetAlgoShortEnd}}%\SetAlgoShortEnd
\DeclareOption{noend}{\AtBeginDocument{\SetAlgoNoEnd}}%      \SetAlgoNoEnd
%
\DeclareOption{nosemicolon}{\AtBeginDocument{\DontPrintSemicolon}}%      \SetAlgoNoEnd
%
% OPTION dotoc
%
\newboolean{algocf@dotocloa}\setboolean{algocf@dotocloa}{false}%
\DeclareOption{dotocloa}{%
  \setboolean{algocf@dotocloa}{true}%
}
%
% OPTION comments
%
\newboolean{algocf@optfillcomment}\setboolean{algocf@optfillcomment}{true}%
\DeclareOption{nofillcomment}{%
  \setboolean{algocf@optfillcomment}{false}%
}%
\DeclareOption{fillcomment}{%
  \setboolean{algocf@optfillcomment}{true}%
}%
%
% OPTION sidecommments
%
\newboolean{algocf@scleft}\setboolean{algocf@scleft}{false}%
\DeclareOption{scleft}{%
  \setboolean{algocf@scleft}{true}%
}%
\DeclareOption{sright}{% default
  \setboolean{algocf@scleft}{false}%
}%
%
% OPTION norelsize
%
\newboolean{algocf@norelsize}\setboolean{algocf@norelsize}{false}%
\DeclareOption{norelsize}{%
  \setboolean{algocf@norelsize}{true}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%% Execution of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ExecuteOptions{english,plain,resetcount,titlenotnumbered,lined,shortend}%
%
\ProcessOptions%
%
\@algocf@algotitleofalgo% fix name for \TitleOfAlgo to \algorithmcfname by default
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Package Loading %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\RequirePackage{xspace}%
%
\ifthenelse{\boolean{algocf@endfloat}}{%
  \RequirePackage{endfloat}%
}{\relax}%
%
\ifthenelse{\boolean{algocf@norelsize}}{%
  \newcommand{\relsize}[1]{\scriptsize}%
}{%
  \RequirePackage{relsize}%
}%
%
\ifthenelse{\boolean{algocf@slide}}{\RequirePackage{color}}{}%
%
%
\AtEndOfPackage{%
  \ifthenelse{\boolean{algocf@dotocloa}}{%
    \renewcommand{\listofalgorithms}{\tocfile{\listalgorithmcfname}{loa}}%
  }{\relax}%
}%
%
% if loa in toc required, load tocbibind package if not already done.
\ifthenelse{\boolean{algocf@dotocloa}}{%
  \ifx\@tocextra\undefined%
  \RequirePackage{tocbibind}%
  \fi%
}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Main Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\algocf@name}{algorithm2e}%
\newcommand{\algocf@date}{october 19 2015}%
\newcommand{\algocf@version}{Release 5.1}%
\newcommand{\algocf@id}{\algocf@version\space -- \algocf@date\space --}%
\typeout{********************************************************^^JPackage `\algocf@name'\space\algocf@id^^J%
         - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
         - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
         subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
         - Author: Christophe Fiorio (christophe.fiorio@umontpellier.fr)^^J********************************************************}%
%%
%%
%%
%%
%%
%%
%%%% hyperref compatibility tricks: Hyperref package defines H counters from
   % standard counters (i.e \theHpage from \thepage) and check some particular
   % counters of some packages, unfortunately it doesn't do the same for
   % algorithm2e package but act as Hcounter was defined. To avoid errors we
   % defined \theHalgocf ourself
%%%%
%
\@ifundefined{theHalgocf}{\def\theHalgocf{\thealgocf}}{}%
\@ifundefined{theHAlgoLine}{\def\theHAlgoLine{\theAlgoLine}}{}%
\@ifundefined{theHalgocfproc}{\def\theHalgocfproc{0}}{}%
\@ifundefined{theHalgocffunc}{\def\theHalgocffunc{0}}{}%
\@ifundefined{toclevel@algocf}{\def\toclevel@algocf{0}}{}%
%
% autoref from hyperref needs an autorefname, so we give it.
\def\AlgoLineautorefname{\algorithmcflinename}%
\def\algocfautorefname{\algorithmautorefname}%
\def\algocfprocautorefname{\procedureautorefname}%
\def\algocffuncautorefname{\functionautorefname}%
%%
%%
%%
\newcommand{\@defaultskiptotal}{0.5em}%
\newskip\skiptotal\skiptotal=0.5em%
\newskip\skiplinenumber\skiplinenumber=\hsize\advance\skiplinenumber by-\skiptotal%
\newskip\skiprule%
\newskip\skiphlne%
\newskip\skiptext%
\newskip\skiplength%
\newskip\algomargin%
\newskip\skipalgocfslide\skipalgocfslide=1em%
\newdimen\algowidth%
\newdimen\inoutsize%
\newdimen\inoutindent%
\newdimen\interspacetitleruled\setlength{\interspacetitleruled}{2pt}%
\newdimen\interspacealgoruled\setlength{\interspacealgoruled}{2pt}%
\newdimen\interspacetitleboxruled\setlength{\interspacetitleboxruled}{2\lineskip}%
%
\newcommand{\@algoskip}{\smallskip}%
\newcommand{\SetAlgoSkip}[1]{\renewcommand{\@algoskip}{\csname#1\endcsname}}%
\newcommand{\@algoinsideskip}{\relax}%
\newcommand{\SetAlgoInsideSkip}[1]{\renewcommand{\@algoinsideskip}{\csname#1\endcsname}}%
%
% ruledwidth
%
\newlength{\algocf@ruledwidth}\setlength{\algocf@ruledwidth}{\linewidth}%
\newboolean{algocf@customruledwidth}\setboolean{algocf@customruledwidth}{false}%
\newcommand{\SetCustomAlgoRuledWidth}[1]{%
  \setboolean{algocf@customruledwidth}{true}%
  \ifthenelse{\boolean{algocf@customruledwidth}}{\setlength{\algocf@ruledwidth}{#1}}{\relax}%
}%
%
\newsavebox{\algocf@inoutbox}%
\newsavebox{\algocf@inputbox}%
%%
%%
\newcommand{\arg@e}{}%
\newcommand{\arg@space}{\ }%
\newcommand{\BlankLine}{\vskip 1ex}%
%%
\newcommand{\vespace}{1ex}%
\newcommand{\SetInd}[2]{%
\skiprule=#1%
\skiptext=#2%
\skiplength=\skiptext\advance\skiplength by \skiprule\advance\skiplength by 0.4pt}%
\SetInd{0.5em}{1em}
\algomargin=\leftskip\advance\algomargin by \parindent%
\newcommand{\IncMargin}[1]{\advance\algomargin by #1}%
\newcommand{\DecMargin}[1]{\advance\algomargin by -#1}%
\newcommand{\SetNlSkip}[1]{%
  \renewcommand{\@defaultskiptotal}{#1}%
  \setlength{\skiptotal}{#1}}%
%%
\newskip\AlCapSkip\AlCapSkip=0ex%
\newskip\AlCapHSkip\AlCapSkip=0ex%
\newcommand{\SetAlCapSkip}[1]{\setlength{\AlCapSkip}{#1}}%
\newcommand{\SetAlCapHSkip}[1]{\setlength{\AlCapHSkip}{#1}}%
\SetAlCapHSkip{.5\algomargin}%
%%
%%
\newskip\algoskipindent
\newcommand{\algocf@adjustskipindent}{%
  \algoskipindent=\skiprule%
  \advance\algoskipindent by \skiptext\advance\algoskipindent by 0.4pt}
\algocf@adjustskipindent%
%
\newcommand{\Indentp}[1]{\advance\leftskip by #1}%
\newcommand{\Indp}{\algocf@adjustskipindent\advance\leftskip by \algoskipindent}
\newcommand{\Indpp}{\advance\leftskip by 0.5em}%
\newcommand{\Indm}{\algocf@adjustskipindent\advance\leftskip by -\algoskipindent}
\newcommand{\Indmm}{\advance\leftskip by -0.5em}%
%
%%
%%
%% Line Numbering
%%
%%
% number line style
\newcommand{\algocf@nlrelsize}{-2}\newcommand{\SetAlgoNlRelativeSize}[1]{\renewcommand{\algocf@nlrelsize}{#1}}%
\newcommand{\NlSty}[1]{\textnormal{\textbf{\relsize{\algocf@nlrelsize}#1}}}% default definition
\newcommand{\SetNlSty}[3]{\renewcommand{\NlSty}[1]{\textnormal{\csname#1\endcsname{\relsize{\algocf@nlrelsize}#2##1#3}}}}%
%
% nl definitions
%
\newsavebox{\algocf@nlbox}%
\newcommand{\algocf@printnl}[1]{%
  \ifthenelse{\boolean{algocf@leftlinenumber}}{%
    \skiplinenumber=\skiptotal\advance\skiplinenumber by\leftskip%
    \strut\raisebox{0pt}{\llap{\NlSty{#1}\kern\skiplinenumber}}\ignorespaces%
  }{%
    \sbox\algocf@nlbox{\NlSty{#1}}%
    \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip\advance\skiplinenumber by-\skiptext%
    \advance\skiplinenumber by\algomargin\advance\skiplinenumber by.3em\advance\skiplinenumber by-\wd\algocf@nlbox%
    % to handle particular case of until: printnl is after 'until' keyword has been writen, so we need to substract length of this keyword
    \advance\skiplinenumber by-\algocf@skipuntil%
    \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\NlSty{#1\ignorespaces}}}\ignorespaces%
  }%
}%
\newcommand{\algocf@nl@sethref}[1]{%
  \renewcommand{\theHAlgoLine}{\thealgocfproc.#1}%
  \hyper@refstepcounter{AlgoLine}\gdef\@currentlabel{#1}%
}%
\newcommand{\nl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \algocf@printnl{\theAlgoLine}%
}%
%
\newcommand{\nllabel}[1]{\label{#1}}%
%
\newcommand{\enl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip%
  \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\strut\NlSty{\theAlgoLine}}}\ignorespaces%
}%
%% nlset
\newcommand{\nlset}[1]{%
  \@ifundefined{hyper@refstepcounter}{\protected@edef\@currentlabel{#1}}{\algocf@nl@sethref{#1}}\algocf@printnl{#1}%
}%
%
%% lnl definitions
\newcommand{\lnl}[1]{\nl\label{#1}\ignorespaces}%
%
%% lnlset
\newcommand{\lnlset}[2]{\nlset{#2}\label{#1}}%
%
% set char put at end of each line
%
\newcommand{\algocf@endline}{\string;}
\newcommand{\SetEndCharOfAlgoLine}[1]{\renewcommand{\algocf@endline}{#1}}
%
% end of line definition
%
\newcommand{\@endalgocfline}{\algocf@endline}% default definition: printsemicolon
\newcommand{\DontPrintSemicolon}{\renewcommand{\@endalgocfline}{\relax}}%
\newcommand{\PrintSemicolon}{\renewcommand{\@endalgocfline}{\algocf@endline}}%
\newcommand{\@endalgoln}{\@endalgocfline\hfill\strut\par}%
%
% line numbering
%
\newcommand{\LinesNumbered}{\setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}}%
\newcommand{\LinesNotNumbered}{%
  \setboolean{algocf@linesnumbered}{false}%
  \renewcommand{\algocf@linesnumbered}{\relax}%
}%
%
\newcommand{\LinesNumberedHidden}{%
  \setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}}%
\newcommand{\ShowLn}{\nlset{\theAlgoLine}\ignorespaces}% display the line number on this line (without labelling)
\newcommand{\ShowLnLabel}[1]{\lnlset{#1}{\theAlgoLine}\ignorespaces}% display the line number and label this line
%
%%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Styling text commands
%
\newcommand{\AlFnt}{\relax}% default definition
\newcommand{\SetAlFnt}[1]{\renewcommand{\AlFnt}{#1}}%
\newcommand{\AlTitleFnt}{\relax}% default definition
\newcommand{\SetAlTitleFnt}[1]{\renewcommand{\AlTitleFnt}{#1}}%
%
\newcommand{\AlCapFnt}{\relax}% default definition
\newcommand{\SetAlCapFnt}[1]{\renewcommand{\AlCapFnt}{#1}}%
\newcommand{\AlCapNameFnt}{\relax}% default definition
\newcommand{\SetAlCapNameFnt}[1]{\renewcommand{\AlCapNameFnt}{#1}}%
%
\newcommand{\ProcFnt}{\relax}% default definition
\newcommand{\SetProcFnt}[1]{\renewcommand{\ProcFnt}{#1}}%
\newcommand{\ProcNameFnt}{\relax}% default definition
\newcommand{\SetProcNameFnt}[1]{\renewcommand{\ProcNameFnt}{#1}}%
\newcommand{\ProcArgFnt}{\relax}% default definition
\newcommand{\SetProcArgFnt}[1]{\renewcommand{\ProcArgFnt}{#1}}%
%
\newcommand{\AlTitleSty}[1]{\textbf{#1}\unskip}% default definition
\newcommand{\SetAlTitleSty}[1]{\renewcommand{\AlTitleSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetAlCapSty}[1]{\renewcommand{\AlCapSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapNameSty}[1]{\textnormal{#1}\unskip}% default definition
\newcommand{\SetAlCapNameSty}[1]{\renewcommand{\AlCapNameSty}[1]{\textnormal{\csname #1\endcsname{##1}}\unskip}}%
%
\newcommand{\ProcSty}[1]{\AlCapSty{#1}}%
\newcommand{\SetProcSty}[1]{\renewcommand{\ProcSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcNameSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcNameSty}[1]{\renewcommand{\ProcNameSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcArgSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcArgSty}[1]{\renewcommand{\ProcArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
\newcommand{\KwSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetKwSty}[1]{\renewcommand{\KwSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetArgSty{emph}
\newcommand{\SetArgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetFuncArgSty{emph}
\newcommand{\SetFuncArgSty}[1]{\renewcommand{\FuncArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncSty}[1]{\textnormal{\texttt{#1}}\unskip}%\SetFuncSty{texttt}
\newcommand{\SetFuncSty}[1]{\renewcommand{\FuncSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetProgSty{emphg}
\newcommand{\SetProgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\DataSty}[1]{\textnormal{\textsf{#1}}\unskip}%%\SetDataSty{textsf}
\newcommand{\SetDataSty}[1]{\renewcommand{\DataSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\CommentSty}[1]{\textnormal{\texttt{#1}}\unskip}%%\SetDataSty{texttt}
\newcommand{\SetCommentSty}[1]{\renewcommand{\CommentSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\TitleSty}[1]{#1\unskip}%\SetTitleSty{}{}
\newcommand{\SetTitleSty}[2]{\renewcommand{\TitleSty}[1]{%
\csname#1\endcsname{\csname#2\endcsname##1}}\unskip}%
\newcommand{\BlockMarkersSty}[1]{\KwSty{#1}}%
\newcommand{\SetBlockMarkersSty}[1]{\renewcommand{\BlockMarkersSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Block basic commands
%
\newcommand{\algocf@push}[1]{\advance\skiptotal by #1\moveright #1}%
\newcommand{\algocf@pop}[1]{\advance\skiptotal by -#1}%
\newcommand{\algocf@addskiptotal}{\advance\skiptotal by 0.4pt\advance\hsize by -0.4pt\advance\hsize by -\skiplength}% 0.4 pt=width of \vrule
\newcommand{\algocf@subskiptotal}{\advance\skiptotal by -0.4pt\advance\hsize by 0.4pt\advance\hsize by \skiplength}% 0.4 pt=width of \vrule
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% group of instructions definition
%
\skiphlne=.8ex%
\newcommand{\SetVlineSkip}[1]{\skiphlne=#1}%
\newcommand{\algocf@bblock}{\BlockMarkersSty{begin}}%
\newcommand{\algocf@eblock}{\BlockMarkersSty{end}}%
\newcommand{\AlgoDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{true}}%
\newcommand{\AlgoDontDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{false}}%
\newcommand{\AlgoDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{true}}%
\newcommand{\AlgoDontDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{false}}%
\newcommand{\algocf@bblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@bblock\par}{\relax}%
}%
\newcommand{\algocf@eblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@eblock\par}{\relax}%
}%
\newcommand{\algocf@bgroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@bblock}{\relax}%
}%
\newcommand{\algocf@egroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@eblock}{\relax}%
}%
\newcommand{\SetAlgoBlockMarkers}[2]{%
  \ifArgumentEmpty{#1}{%
    \renewcommand{\algocf@bblock}{\relax}%
  }{%
    \renewcommand{\algocf@bblock}{\BlockMarkersSty{#1}}%
  }% begin marker set
  \ifArgumentEmpty{#2}{%
    \renewcommand{\algocf@eblock}{\relax}%
  }{%
    \renewcommand{\algocf@eblock}{\BlockMarkersSty{#2}}%
  }% end marker set
}
%
%%%%%%%%% block with a vertical line end by a little horizontal line
\newcommand{\algocf@Vline}[1]{%     no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}\Hlne}}\vskip\skiphlne% inside the block
  \algocf@pop{\skiprule}%\algocf@subskiptotal% restore indentation
  \nointerlineskip}% no vskip after
%
%%%%%%%%% block with a vertical line
\newcommand{\algocf@Vsline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%               the vertical rule
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}% restore indentation
  \algocf@eblockcode%
}
%
\newcommand{\algocf@Hlne}{\hrule height 0.4pt depth 0pt width .5em}%
%
%%%%%%%%%  block without line
\newcommand{\algocf@Noline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%
  \hbox{%
    \vtop{\algocf@push{\skiptext}%
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}%
  \algocf@eblockcode%
  % \nointerlineskip% no vskip after
}%
%%%%%%%%%
%
%% default=NoLine
%
\newcommand{\algocf@group}[1]{\algocf@Noline{#1}}% group: set of instruction depending from another (ex: then part of the If)
\newcommand{\algocf@@@eblock}[2]{#1\ifArgumentEmpty{#2}{\relax}{\KwSty{\@algocf@endoption{#2}}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@@block}[3]{#1\ifArgumentEmpty{#2}{\ifArgumentEmpty{#3}{\relax}{ #3\relax}}{\KwSty{\@algocf@endoption{#2}}\ifArgumentEmpty{#3}{\relax}{ #3}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@block}[3]{\algocf@@@block{#1}{#2}{#3}}% block: group with a end keyword.
\newcommand{\algocf@block}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
%\newcommand{\algocf@nblock}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
\newcommand{\algocf@setBlock}{%
  \ifthenelse{\boolean{algocf@optnoend}}{%     if no end option
    \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%     block will be a group
  }{%                                          else
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}% block stays a block
  }%
}%
%
\newcommand{\Hlne}{}% little hrizontal line ending a block in vline mode
%
\newcommand{\@algocf@endoption}[1]{#1}%
\newboolean{algocf@optnoend}\setboolean{algocf@optnoend}{false}%
%
\newcommand{\SetAlgoLongEnd}{%%%%%%%%%%%%%%%%%%%%%%%%% Long End
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{##1}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoShortEnd}{%%%%%%%%%%%%%%%%%%%%%%%% ShortEnd
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{\@firstword##1 \@nil}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoEnd}{%%%%%%%%%%%%%%%%%%%%%%%%%%% NoEnd
  \setboolean{algocf@optnoend}{true}%
  \renewcommand{\@algocf@endoption}[1]{}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoLine}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\algocf@Noline{##1}}{##2}}%
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetAlgoVlined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Vline
\renewcommand{\algocf@@block}[2]{\algocf@Vline{##1}}%
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{\algocf@Hlne}}%
%
\newcommand{\SetAlgoLined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\strut\algocf@Vsline{##1}}{##2}}% no skip after a block so garantie at least one line
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetNothing}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@Noline{##1}\par}%
%\long
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
%%
%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ``Input:'''s like command 
%
%%%
% text staying at the right of the longer keyword of KwInOut commands 
% (text of KwInOut commands are all vertically aligned)
%
\newcommand{\algocf@newinout}{\par\parindent=\inoutindent}% to put right indentation after a \\ in the KwInOut
\newcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2\algocf@typo:}}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else% else keep the larger dimension
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi% the dimension of the box is now defined.
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
%
%% allow to ajust the skip size of InOut
%%
\newcommand{\ResetInOut}[1]{%
  \sbox\algocf@inoutbox{\hbox{\KwSty{#1\algocf@typo:}\ }}%
  \setlength{\inoutsize}{\wd\algocf@inoutbox}%
  }%
%
% 
%%%
% text staying at the right of the keyword.
%
\newcommand{\algocf@newinput}{\par\parindent=\wd\algocf@inputbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwInput}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@inputbox{\hbox{\KwSty{#2\algocf@typo:} }}%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
    {\let\\\algocf@newinput\hangindent=\wd\algocf@inputbox\hangafter=1\unhbox\algocf@inputbox##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
\newcommand{\SetKwData}[2]{%
  \algocf@newcommand{@#1}[1]{\DataSty{#2(}\ArgSty{##1}\DataSty{)}}%
  \algocf@newcommand{#1}{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
  }%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tallent:
%
% Add following macros:
%   \SetKwHangingKw:  [kw] ------------   <= hanging determined by [kw]
%                          ------------
% Should act like a combination of \SetKwInput and \SetKw.
% Based on \SetKwInput:
%   - remove ':' at end of keyword
%   - do not reset numbering
%   - use separate savebox
\newsavebox{\algocf@hangingbox}
\newcommand{\algocf@newhanging}{\par\parindent=\wd\algocf@hangingbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwHangingKw}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@hangingbox{\hbox{\KwSty{#2}\algocf@typo\ }}%
    {\let\\\algocf@newhanging\hangindent=\wd\algocf@hangingbox\hangafter=1\unhbox\algocf@hangingbox##1\;}%
  }%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Comments macros
%
%%%%
% comment in the text, first argument is the name of the macro, second is
% the text put before the comment, third is the text put at the end of the
% comment.
%
% first side comment justification
\newcommand{\SetSideCommentLeft}{\setboolean{algocf@scleft}{true}}%
\newcommand{\SetSideCommentRight}{\setboolean{algocf@scleft}{false}}%
\newcommand{\SetNoFillComment}{\setboolean{algocf@optfillcomment}{false}}%
\newcommand{\SetFillComment}{\setboolean{algocf@optfillcomment}{true}}%
%
% next comment and side comment
%
\newcommand{\algocf@endmarkcomment}{\relax}%
\newcommand{\algocf@fillcomment}{%
  \ifthenelse{\boolean{algocf@optfillcomment}}{\hfill}{\relax}}%
%
\newcommand{\algocf@startcomment}{%
  \hangindent=\wd\algocf@inputbox\hangafter=1\usebox\algocf@inputbox}%
\newcommand{\algocf@endcomment}{\algocf@fillcomment\algocf@endmarkcomment\ignorespaces\par}%
\newcommand{\algocf@endstartcomment}{\algocf@endcomment\algocf@startcomment\ignorespaces}%
%
\newboolean{algocf@sidecomment}%
\newboolean{algocf@altsidecomment}\setboolean{algocf@altsidecomment}{false}%
\newcommand{\algocf@scpar}{\ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\par}}%
\newcommand{\algocf@sclfill}{\ifthenelse{\boolean{algocf@scleft}}{\algocf@fillcomment}{\relax}}%
\newcommand{\algocf@scrfill}{\ifthenelse{\boolean{algocf@scleft}}{\relax}{\hfill}}%
\newcommand{\algocf@startsidecomment}{\usebox\algocf@inputbox}%
\newcommand{\algocf@endsidecomment}{\algocf@endmarkcomment\algocf@scpar}%
\newcommand{\algocf@endstartsidecomment}{%
  \algocf@sclfill\algocf@endsidecomment%
  \algocf@scrfill\algocf@startsidecomment\ignorespaces}%
%
\newcommand{\SetKwComment}[3]{%
  \algocf@newcommand{#1}{\@ifstar{\csname algocf@#1@star\endcsname}{\csname algocf@#1\endcsname}}%
	\algocf@newcommand{algocf@#1}[1]{%
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@seteveryparhanging{\relax}}%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {\renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartcomment%
        \algocf@startcomment\CommentSty{%
          \strut\ignorespaces##1\strut\algocf@fillcomment#3}\par}%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@reseteveryparhanging}%
    }%
  %%% side comment definitions
	\algocf@newcommand{algocf@#1@star}[2][]{%
      \ifArgumentEmpty{##1}\relax{% TODO: Is this even necessary, with all those \ifx's?
        \ifthenelse{\boolean{algocf@scleft}}{\setboolean{algocf@sidecomment}{true}}{\setboolean{algocf@sidecomment}{false}}%
        \ifx##1h\setboolean{algocf@altsidecomment}{true}\SetSideCommentLeft\fi%
        \ifx##1f\setboolean{algocf@altsidecomment}{true}\SetSideCommentRight\fi%
        \ifx##1l\setboolean{algocf@altsidecomment}{false}\SetSideCommentLeft\fi%
        \ifx##1r\setboolean{algocf@altsidecomment}{false}\SetSideCommentRight\fi%
      }%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {%
        \renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartsidecomment%
        % here is the comment
        \ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\@endalgocfline\ }%
        \algocf@scrfill\algocf@startsidecomment\CommentSty{%
          \strut\ignorespaces##2\strut\algocf@sclfill#3}\algocf@scpar%
      }%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifArgumentEmpty{##1}\relax{%
        \ifthenelse{\boolean{algocf@sidecomment}}{\setboolean{algocf@scleft}{true}}{\setboolean{algocf@scleft}{false}}%
        \setboolean{algocf@altsidecomment}{false}%
      }%
	}%
  }%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwProg
%
\newcommand{\SetKwProg}[4]{%\SetKwProg{Env}{Title}{is}{end} 
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\ifArgumentEmpty{#2}\relax{\ }\ProgSty{##2}\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode\@endalgocfline\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Kw
%
\newcommand{\SetKw}[2]{%
	\algocf@newcommand{@#1}[1]{\KwSty{#2} \ArgSty{##1}}
	\algocf@newcommand{#1}{\@ifnextchar\bgroup{\csname @#1\endcsname}{\KwSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwFunction
%
\newcommand{\SetKwFunction}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\FuncSty{#2(}\FuncArgSty{##1}\FuncSty{)}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\FuncSty{#2}\xspace}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwTab
%
\newcommand{\SetKwArray}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\DataSty{#2[}\ArgSty{##1}\DataSty{]}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwBlock
%
\newcommand{\SetKwBlock}[3]{%
	\algocf@newcmdside@kobe{#1}%
    {\KwSty{#2}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#3}{##3}\par}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% condition typo
%
\newcommand{\algocf@scond}{\ }
\newcommand{\algocf@econd}{\ }
\newcommand{\algocf@ucond}{}
\newcommand{\SetStartEndCondition}[3]{%
  \renewcommand{\algocf@scond}{#1}\renewcommand{\algocf@econd}{#2}\renewcommand{\algocf@ucond}{#3}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For Switch
%
\newcommand{\SetKwSwitch}[9]{% #1=\Switch #2=\Case #3=\Other #4=switch #5=do #6=case #7=otherwise #8=endcase #9=endsw
%	\algocf@newcmdside{#1}{3}%
	\algocf@newcmdside@koif{#1}%
		{\KwSty{#4}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#9} {##4\relax}}%
%%%% Case
	\algocf@newcmdside@koif{#2}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#8}{##4\relax}}%
    %uCase
	\algocf@newcmdside{u#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##3}}%
    %lcase
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\ \relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
%%%% Other 
	\algocf@newcmdside@kobe{#3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#8}{##3\relax}}%
    %lOther
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\algocf@egroupcode}%
    %uOther
	\algocf@newcmdside{u#3}{3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##2}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% If macros
%
\newcommand{\SetKwIF}[8]{% #1=\If #2=\ElseIf #3=\Else #4=if #5=then #6=elseif #7=else #8=endif
% 
% common text
	\algocf@newcommand{#1@ifthen}[1]{\KwSty{#4}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#1@endif} [2]{\algocf@block{##1}{#8}{##2}}%
	\algocf@newcommand{#1@noend} [1]{\algocf@group{##1}}%
	\algocf@newcommand{#1@else}  [1]{\algocf@group{##1}\KwSty{#7}}%
	\algocf@newcommand{#2@elseif}[1]{\KwSty{#6}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#3@else}     {\KwSty{#7}}%
%%%% If then { } endif
	\algocf@newcmdside@koif{#1}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% If then {} else {} endif
    % first command to handle optional side comment of else (so just after first braces)
 	\algocf@newcmdside@kobe{algocf@e#1thenelse}{\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##2}{##3}}%
    % the definition of if-then-else command using command above 
	\algocf@newcmdside{e#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@else\endcsname{##3}\csname algocf@e#1thenelse\endcsname}%
    %%% leif
    \algocf@newcommand{le#1}{\@ifstar{\csname algocf@le#1star\endcsname}{\csname algocf@le#1\endcsname}}%
    \algocf@newcmdside{algocf@le#1}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\@endalgocfline\ \algocf@egroupcode\ifArgumentEmpty{##1}\relax{##1}\strut\par}%
    \algocf@newcmdside{algocf@le#1star}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\algocf@egroupcode}%
%%%% If then 
	% \algocf@newcmdside{l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\
    % ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@noend\endcsname{##3}}%
%%%% ElseIf {} endif
	\algocf@newcmdside@koif{#2}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% ElseIf
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#2}{3}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{##1}\csname #1@noend\endcsname{##3}}%
%%%% Else {} endif
	\algocf@newcmdside@kobe{#3}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ ##1\csname #1@endif\endcsname{##2}{##3\relax}}%
%%%% Else 
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\algocf@egroupcode}%
	\algocf@newcmdside{u#3}{2}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ {##1\relax}\csname #1@noend\endcsname{##2}}%
}% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For macros
%
\newcommand{\SetKwFor}[4]{%
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4\relax}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Repeat macros
%
\newsavebox{\algocf@untilbox}% to handle width of until keyword needed to have good skip
  % for line numbers
\newskip\algocf@skipuntil
\newcommand{\SetKwRepeat}[3]{%
	\algocf@newcmdsides{#1}{3}{%
      \sbox\algocf@untilbox{\KwSty{#3}\algocf@scond}\algocf@skipuntil=\wd\algocf@untilbox%
      \KwSty{#2}\ifArgumentEmpty{##1}\relax{##1}\algocf@group{##3}%
      \KwSty{#3}\algocf@scond% until keyword and start condition typo
      %\advance\skiptotal by\algocf@skipuntil%
      \ArgSty{##2}%
      %\advance\skiptotal by-\algocf@skipuntil%
      \algocf@ucond%
      \algocf@skipuntil=0pt% reset counter
    }{\@endalgocfline}{\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond\@endalgocfline\ifArgumentEmpty{##1}\relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond}%
}%
%
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%        Environments definitions     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%
%% Caption management
%%
% for the following macros:
% #1 is given by caption and is equal to fnum@algocf
% #2 is the text given in argument by the user in the \caption macro
%
%%%%% text of caption
\newcommand{\algocf@captionlayout}[1]{#1}%
\newcommand{\SetAlgoCaptionLayout}[1]{%
  \renewcommand{\algocf@captionlayout}[1]{\csname #1\endcsname{##1}}}%
\newcommand{\algocf@capseparator}{:}%
\newcommand{\SetAlgoCaptionSeparator}[1]{\renewcommand{\algocf@capseparator}{#1}}%
\newcommand{\algocf@captiontext}[2]{%
  \algocf@captionlayout{\AlCapSty{\AlCapFnt #1\algocf@typo\algocf@capseparator}\nobreakspace%
    \AlCapNameSty{\AlCapNameFnt{}#2\endgraf}}}% text of caption
%
%%%%% default caption of algorithm: used if no specific style caption is defined
\newcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}%
%
\newsavebox\algocf@capbox%
\newcommand{\algocf@makecaption@plain}[2]{%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}}%
\newcommand{\algocf@makecaption@boxed}[2]{%
  \addtolength{\hsize}{-\algomargin}%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}%
  \addtolength{\hsize}{\algomargin}%
 }%
%
\newcommand{\algocf@makecaption@plainruled}[2]{\algocf@makecaption@plain{#1}{#2}}%
\newcommand{\algocf@makecaption@tworuled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@algoruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@boxruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@ruled}[2]{%
  \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}}% then caption is not centered
}%
%
\newlength{\algoheightruledefault}\setlength{\algoheightruledefault}{0.8pt}%
\newlength{\algoheightrule}\setlength{\algoheightrule}{\algoheightruledefault}%
\newlength{\algotitleheightruledefault}\setlength{\algotitleheightruledefault}{0.8pt}%
\newlength{\algotitleheightrule}\setlength{\algotitleheightrule}{\algotitleheightruledefault}%
\newcommand{\algocf@caption@plain}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@plainruled}{\algocf@caption@plain}%
\newcommand{\algocf@caption@boxed}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@ruled}{\box\algocf@capbox\kern\interspacetitleruled\hrule
  width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@tworuled}{\box\algocf@capbox\hrule  height0pt depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@algoruled}{\algocf@caption@ruled}%
\newcommand{\algocf@caption@boxruled}{%
  \addtolength{\hsize}{-0.8pt}%
  \hbox to\hsize{%
    \vrule%\hskip-0.35pt%
    \vbox{%
      \hrule\vskip\interspacetitleboxruled%
      \hbox to\hsize{\unhbox\algocf@capbox\hfill}\vskip\interspacetitleboxruled%
    }% 
    %\hskip-0.35pt%
    \vrule%
  }\nointerlineskip%
  \addtolength{\hsize}{0.8pt}%
}%
%
%
%%%% set caption for the environment
\newcommand{\algocf@captionref}{%
  \renewcommand{\fnum@algocf}[1]{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\algocf@algocfref}}%
  \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
  \let\old@thealgocf=\thealgocf\renewcommand{\thealgocf}{{\relsize{\algocf@refrelsize}\algocf@algocfref}}%
  \gdef\@currentlabel{\algocf@algocfref}% let the label use the new ref
}%
%
% Unfortunatly, we also need our own caption to set some specific stuff for special references. But after these
% settings, we call the original caption.
%
\long\def\algocf@caption@algo#1[#2]#3{%
  \ifthenelse{\equal{\algocf@algocfref}{\relax}}{}{\algocf@captionref}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\equal{\algocf@algocfref}{\relax}}{\renewcommand{\theHalgocf}{\thealgocf}}{% take algocf as Href
      \renewcommand{\theHalgocf}{\algocf@algocfref}}%else if SetAlgoRefName done, take this name as ref.
    \hyper@refstepcounter{algocf}%set algocf as category of ref
  }%
   \algocf@latexcaption{#1}[{#2}]{{#3}}% call original caption
}%
%
% beamer define is own caption overrinding latex caption!
% as we need it, we have put here the original definition
% to handle manual ref, unfortunately we have to add one line to handle algocf@algocfref
\long\def\algocf@latexcaption#1[#2]#3{% original definition of caption
  \par%
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
  {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup%
  \@parboxrestore%
  \if@minipage%
    \@setminipage%
  \fi%
  \normalsize%
  \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par%
  \endgroup%
}%
%
% \ifx\beamer@makecaption\undefined%
% \else% beamer detected
\ifx\@makecaption\undefined%
\newcommand{\@makecaption}[2]{\relax}%
\fi%
%%

%
% more and more packages redefine \@caption instead of just \@makecaption which makes algorithm2e
% caption not works since based on standard \@caption. So we force the definition of \@caption to be
% the standard one (the one from LaTeX) inside algorithm environment.
%
% unfortunately, makecaption is called with \ignorespace #3 so 
% we can't do the @currentlabel definition inside \algocf@captionproctext
\long\def\algocf@caption@proc#1[#2]#3{%
  \ifthenelse{\boolean{algocf@nokwfunc}}{\relax}{%
    \SetKwFunction{\algocf@captname#3@}{\algocf@captname#3@}%
  }%
  % we tell hyperref to use algocfproc as category and to take the appropriate ref.
  \ifthenelse{\boolean{algocf@func}}{\def\@proc@func{algocffunc}}{\def\@proc@func{algocfproc}}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\boolean{algocf@procnumbered}}{% 
      \expandafter\def\csname theH\@proc@func\endcsname{\thealgocf}%if procnumbered, take \thealgocf as ref
    }{%
      \expandafter\def\csname theH\@proc@func\endcsname{\algocf@captname#3@}%else take procedure or function name
    }%
    \hyper@refstepcounter{\@proc@func}%
  }%
  \ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
    \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
    \gdef\@currentlabel{\algocf@captname#3@}% let the label be the name of the function, not the counter
  }%
  \ifthenelse{\equal{\algocf@captparam#2@}{\arg@e}}{% if no paramater, we remove the ()
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace\algocf@captname#2@]{#3}%
  }{%                                                 else we give the complete name
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace#2]{#3}%
  }%
}%
%%
%%% setcaption
\newcommand{\algocf@setcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment, caption text must be changed
    \let\algocf@oldcaptiontext=\algocf@captiontext%
    \renewcommand{\algocf@captiontext}[2]{%
      \algocf@captionproctext{##1}{##2}%
    }%
  }{}%
  \let\algocf@savecaption=\@caption%
  \ifthenelse{\boolean{algocf@procenvironment}}{\let\@caption=\algocf@caption@proc}{\let\@caption=\algocf@caption@algo}%
  \let\algocf@oldmakecaption=\@makecaption%
  \renewcommand{\@makecaption}[2]{%
    \expandafter\csname algocf@makecaption@\algocf@style\endcsname{##1}{##2}%
  }%
}%
%
%%%%% reset caption
%
% since we have force the LaTeX caption for algorithm environment, we must go back to the caption
% used in the text.
\newcommand{\algocf@resetcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment
    \let\thealgocf=\old@thealgocf% restore normal counter printing
    \let\algocf@captiontext=\algocf@oldcaptiontext% restore normal caption text
  }{}%
  \let\@caption=\algocf@savecaption% now restore caption outside algo/proc/func environment
  \let\@makecaption=\algocf@oldmakecaption% and restore makecaption outside outside algo/proc/func environment
  \algocf@resetfnum%
}%
%
%%%%% nocaptionofalgo and restorecaptionofalgo --
\newcommand{\NoCaptionOfAlgo}{%
  \let\@old@algocf@captiontext=\algocf@captiontext%
  \renewcommand{\algocf@captiontext}[2]{\AlCapNameSty{\AlCapNameFnt{}##2}}%
}%
\newcommand{\RestoreCaptionOfAlgo}{%
  \let\algocf@captiontext=\@old@algocf@captiontext%
}%
%
% ----------------------  algocf environment
%
\newcounter{algocfline}%                    % new counter to make lines numbers be internally 
\setcounter{algocfline}{0}%                 % different in different algorithms
\newcounter{algocfproc}% counter to count all algo environment (proc, func), just used by hyperref to avoir "same
\setcounter{algocfproc}{0}% identifier" error caused by algocf being set to '-' for procedure or function or not
  % changed if no caption is given.
%
\expandafter\ifx\csname algocf@within\endcsname\relax% if \algocf@within doesn't exist
\newcounter{algocf}%                        % just define a new counter
\renewcommand{\thealgocf}{\@arabic\c@algocf}% and the way it is printed
\else%                                     else
\newcounter{algocf}[\algocf@within]%        % counter is numbered within \algocf@within
\renewcommand\thealgocf{\csname the\algocf@within\endcsname.\@arabic\c@algocf}%
\fi%
%
\def\fps@algocf{htbp}%        % default
\def\ftype@algocf{10}%        % float type
\def\ext@algocf{\algocf@list} % loa by default, lof if figure option used
\newcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}%
\newcommand{\algocf@resetfnum}{\renewcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}}%
\newenvironment{algocf}%      % float environment for algorithms
               {\@float{algocf}}%
               {\end@float}%
\newenvironment{algocf*}%     % float* environment for algorithms
               {\@dblfloat{algocf}}%
               {\end@dblfloat}%
%
\def\algocf@seclistalgo{}%
\ifx\l@chapter\undefined\let\algocf@seclistalgo=\section\else\let\algocf@seclistalgo=\chapter\fi%
\@ifundefined{if@restonecol}{\newif\if@restonecol}\relax%
\newcommand\listofalgocfs{%
     \ifx\algocf@seclistalgo\chapter%
      \if@twocolumn\@restonecoltrue\onecolumn\else\@restonecolfalse\fi%
    \fi%
     \algocf@seclistalgo*{\listalgorithmcfname}%
       \@mkboth{\MakeUppercase\listalgorithmcfname}%
               {\MakeUppercase\listalgorithmcfname}%
     \@starttoc{loa}%
    \ifx\algocf@seclistalgo\chapter%
      \if@restonecol\twocolumn\fi%
    \fi%
}
%
\newcommand*\l@algocf{\@dottedtocline{1}{1em}{2.3em}}% line of the list
%
% ----------------------  algorithm environment
%
%%%%%%%
%%
%% Algorithm environment definition
%%
%%%%%%%
%%
%
\newsavebox\algocf@algoframe%
\def\@algocf@pre@plain{\relax}%  action to be done before printing the algo.
\def\@algocf@post@plain{\relax}% action to be done after printing the algo.
\def\@algocf@capt@plain{bottom}% where the caption should be localized.
\def\@algocf@pre@boxed{\noindent\begin{lrbox}{\algocf@algoframe}}
\def\@algocf@post@boxed{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxed{under}%
\def\@algocf@pre@ruled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@ruled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@ruled{top}%
\def\@algocf@pre@algoruled{\hrule width\algocf@ruledwidth height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@algoruled{\kern\interspacealgoruled\hrule width\algocf@ruledwidth height\algoheightrule \relax}%
\def\@algocf@capt@algoruled{top}%
\def\@algocf@pre@tworuled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@tworuled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@tworuled{top}%
\def\@algocf@pre@boxruled{\noindent\begin{lrbox}{\algocf@algoframe}}%
\def\@algocf@post@boxruled{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxruled{above}%
\def\@algocf@pre@plainruled{\@algocf@pre@ruled}%  action to be done before printing the algo.
\def\@algocf@post@plainruled{\@algocf@post@ruled\kern\interspacealgoruled}%  action to be done before printing the algo.
\def\@algocf@capt@plainruled{under}%
%
\newcommand{\noalgocaption}{\def\@algocf@capt@ruled{none}}
%
%% before algocf environment (not figure environment)
\newcommand{\@algocf@init@caption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if we are inside a procedure/function environment
    \@algocf@proctitleofalgo% set Titleofalgo to Procedure: or Function:
                            % accordingly to the environment
    \let\old@thealgocf=\thealgocf\ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
      \renewcommand{\thealgocf}{-}}%
  }{% else inside environment algorithm
    \@algocf@algotitleofalgo% fix name for \Titleofalgo to \algorithmcfname
  }%
  \algocf@setcaption%       set caption to our caption style
}%
%
\newcommand{\@algofloatboxreset}{\@setminipage}
\newcommand{\@algocf@init}{%
  \refstepcounter{algocfline}%
  \stepcounter{algocfproc}%to have a different counter for each environment and being abble to make the difference
    %between href of algoline in different algorithms.
  \ifthenelse{\boolean{algocf@optnoend}}{%
      \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%
    }{%
      \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
    }%
}%
%% after the end of algocf or figure environment
\newcommand{\@algocf@term@caption}{%
  \algocf@resetcaption% restore original caption
}%
%
\newcommand{\@algocf@term}{%
  \setboolean{algocf@algoH}{false}% no H by default
  \ifthenelse{\boolean{algocf@optnoend}}{%
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
  }{%
    \renewcommand{\algocf@block}[2]{\algocf@group{##1}}%
  }%
  \SetAlgoRefName{\relax}%
}%
%
%%%%%%%%%%%%%%%%%
%% makethealgo: macro which print effectively the algo in its box
%% 
\newsavebox\algocf@algobox%
\newcommand{\algocf@makethealgo}{%
  \vtop{%
    % place caption above if needed  bye the style
    \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{above}}%
    {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    % precommand according to the style
    \csname @algocf@pre@\algocf@style\endcsname%
    % place caption at top if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{top}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    \box\algocf@algobox% the algo
    % place caption at bottom if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{bottom}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    % postcommand according to the style
    \csname @algocf@post@\algocf@style\endcsname%
    % place caption under if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{under}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
  }%
}%
%%%%%%%%%%%%%%%%%%%
%
%% at the beginning of algocf or figure environment
\newenvironment{algomathdisplay}{\[}{\@endalgocfline\]\ifthenelse{\boolean{algocf@linesnumbered}}{\nl}{\relax}}%
\newcommand{\@algocf@start}{%
  \@algoskip%
  \begin{lrbox}{\algocf@algobox}%
  \setlength{\algowidth}{\hsize}%
  \vbox\bgroup% save all the algo in a box
  \hbox to\algowidth\bgroup\hbox to \algomargin{\hfill}\vtop\bgroup%
  \ifthenelse{\boolean{algocf@slide}}{\parskip 0.5ex\color{black}}{}%
  % initialization
  \addtolength{\hsize}{-1.5\algomargin}%
  \let\@mathsemicolon=\;\def\;{\ifmmode\@mathsemicolon\else\@endalgoln\fi}%
  \raggedright\AlFnt{}%
  \ifthenelse{\boolean{algocf@slide}}{\IncMargin{\skipalgocfslide}}{}%
  \@algoinsideskip%
%   \let\@emathdisplay=\]\def\]{\algocf@endline\@emathdisplay\nl}%
}%
%
%% at the end of algocf or figure environment
\newcommand{\@algocf@finish}{%
  \@algoinsideskip%
  \egroup%end of vtop which contain all the text
  \hfill\egroup%end of hbox wich contains [margin][vtop]
  \ifthenelse{\boolean{algocf@slide}}{\DecMargin{\skipalgocfslide}}{}%
  %
  \egroup%end of main vbox
  \end{lrbox}%
  \algocf@makethealgo% print the algo
  \@algoskip%
  % restore dimension and macros
  \setlength{\hsize}{\algowidth}%
  \lineskip\normallineskip\setlength{\skiptotal}{\@defaultskiptotal}%
  \let\;=\@mathsemicolon%  
  \let\]=\@emathdisplay%
}%
%
%%%%%%%%%%%%%%%%%%%%
%% basic definition of the environment algorithm
%%
%
\newboolean{algocf@procenvironment}\setboolean{algocf@procenvironment}{false}%
\newboolean{algocf@func}\setboolean{algocf@func}{false}%
\newboolean{algocf@algoH}\setboolean{algocf@algoH}{false}%
\newboolean{algocf@algostar}\setboolean{algocf@algostar}{false}%
%
%%% environment for {algorithm}[H]
\newenvironment{algocf@Here}{\noindent%
  \def\@captype{algocf}% if not defined, caption exit with an error
  \begin{minipage}{\hsize}%
}{%
  \end{minipage}%\par%
}%
%%% real algorithm environment which manages H and * option
%    \let\algocf@originalfloatboxreset=\@floatboxreset%
%    \let\@floatboxreset=\@algofloatboxreset%
\newenvironment{algocf@algorithm}[1][htbp]{%
   \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@figurecaption}}{\captionsetup{margin={-\algomargin,\algomargin}}}{}%
   }{}%
   \@algocf@init%
   \ifthenelse{\equal{\algocf@float}{figure}}{% if option figure set
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \begin{figure*}[#1]% call figure*
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else algorithm environment with figure option
       \begin{figure}[#1]%  call figure
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
          \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }%
   }{% else normal algorithm environment
     \@algocf@init@caption%
     \ifthenelse{\equal{#1}{H}}{% if [H] algorithm
       \if@twocolumn\@latex@error{[H] in two columns mode is not allowed for algorithms}\fi% TODO: SCREAM if H in two colums!
       \setboolean{algocf@algoH}{true}\begin{algocf@Here}% call corresponding environment
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \begin{algocf*}[#1]% call algocf*
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }{% else algorithm environment
         \begin{algocf}[#1]%  call algcf
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }%
     }%
   }% fin test option figure ou pas
   \@algocf@start% 
   \@ResetCounterIfNeeded%
   \algocf@linesnumbered\ignorespaces%
}{%
  \@algocf@finish%
  \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure*}% call figure*
     }{% else algorithm environment with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure}%  call figure
     }%
  }{%
    \@algocf@term@caption%
    \ifthenelse{\boolean{algocf@algoH}}{% if [H] algorithm
      \let\everypar=\algocf@oldeverypar%
      \end{algocf@Here}\par% call corresponding environment
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \let\everypar=\algocf@oldeverypar%
         \end{algocf*}% call algocf*
       }{% else algorithm environment
         \let\everypar=\algocf@oldeverypar%
         \end{algocf}%  call algocf
       }%
     }%
  }%
  \@algocf@term\ignorespacesafterend%
}%
%
%%% user algorithm environment
\newenvironment{\algocf@envname}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%%% user algorithm* environment
\newenvironment{\algocf@envname*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%
%%%
%
\expandafter\newcommand\csname\algocf@listofalgorithms\endcsname{%
  \ifthenelse{\equal{\algocf@float}{figure}}{\listoffigures}{\listofalgocfs}%
}%
%%%
%%%
%
% ----------------------  procedure and function environments
%
%
% -- new style (used in particular in the caption of function and procedure environments)
%
% three macros to extract parts of the caption
\gdef\algocf@captname#1(#2)#3@{#1}  % keep characters before the first brace
\gdef\algocf@captparam#1(#2)#3@{#2} % keep character in between the braces
\gdef\algocf@captother#1(#2)#3@{#3} % keep character after the braces
%
%%% Text of caption for Procedure or Function
\newcommand{\algocf@captionproctext}[2]{%
  {%
    \ProcSty{\ProcFnt\algocf@procname\ifthenelse{\boolean{algocf@procnumbered}}{\nobreakspace\thealgocf\algocf@typo\algocf@capseparator}{\relax}}%
    \nobreakspace\ProcNameSty{\ProcNameFnt\algocf@captname #2@}% Name of the procedure in ProcName Style. 
    \ifthenelse{\equal{\algocf@captparam #2@}{\arg@e}}{}{% if no argument, write nothing
      \ProcNameSty{\ProcNameFnt(}\ProcArgSty{\ProcArgFnt\algocf@captparam #2@}\ProcNameSty{\ProcNameFnt)}%else put arguments in ProcArgSty:
    }% endif
    \algocf@captother #2@%
  }%
}%
%
%
% -- procedure and function environments are defined from algocf@algorithm environment
%
\newenvironment{procedure}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
\newenvironment{procedure*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%
%%%%%%%%%%%%%%%%%%%%
%% definition of algondfloat environment
%%
\ifthenelse{\boolean{algocf@endfloat}}{% if endfloat option then
\newcommand{\algoplace}{% macro which is used to writhe algorithm about there
   \begin{center}%
     [\algorithmcfname~\thepostfig\ about here.]%
   \end{center}%
}%
\newcommand{\algoendfloat}{% use as a \begin{algoendfloat} environment to start scanning of line
%  \immediate\openout\@mainfff\jobname.fff%
  \efloat@condopen{fff}
  \efloat@iwrite{fff}{\string\begin{\algocf@envname}}%
    \if@domarkers%
       \ifthenelse{\equal{\algocf@list}{lof}}{%
         \addtocounter{postfig}{1}%
       }{%
         \addtocounter{postalgo}{1}%
       }%
       \algoplace%
    \fi%
    \bgroup%
    \let\do\ef@makeinnocent\dospecials%
    \ef@makeinnocent\^^L% and whatever other special cases
    \endlinechar`\^^M \catcode`\^^M=12 \ef@xalgocfendfloat}%
}{\relax}%%%% end of endfloat option ifthenelse
%% some macros useful for endfloat option that cannot be defined inside the ifthenelse
%scan algoendfloat algorithm and write the text into .fff file
{\catcode`\^^M=12 \endlinechar=-1 %
 \gdef\ef@xalgocfendfloat#1^^M{% scan the lines inside algoendfloat environment being read by latex
   \def\test{#1}% test is the line being currently scan by latex
   \ifx\test\ef@endalgocftest% if it is \end{algoendfloat}
     \def\next{% define next as to not continue the scan and write \end{algorithm} into .fff file
       \egroup\end{algoendfloat}%
       \efloat@iwrite{fff}{\string\end{\algocf@envname}}%
       \efloat@iwrite{fff}{\string\efloatseparator}%
       \efloat@iwrite{fff}{ }%
     }%
     \else% else write the current line being scanned by latex and set next to continue the scan
       \efloat@iwrite{fff}{#1}%
       \let\next\ef@xalgocfendfloat%
     \fi% endif
     \next}% next is continue if it was else condition, else it does not continue the scan and write end to file
}%
% test if the scan is finish by looking at the string \end{algoendfloat}
{\escapechar=-1%
 \xdef\ef@endalgocftest{\string\\end\string\{algoendfloat\string\}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
\newcommand{\TitleOfAlgo}[1]{\@titleprefix\ 
  \TitleSty{#1}\par\smallskip}%
%
\newcommand{\SetAlgorithmName}[3]{%
  \renewcommand{\listalgorithmcfname}{#3}%
  \renewcommand{\algorithmcfname}{#1}%
  \renewcommand{\algorithmautorefname}{#2}%
}%
%
\newcommand{\algocf@refrelsize}{-2}\newcommand{\SetAlgoRefRelativeSize}[1]{\renewcommand{\algocf@refrelsize}{#1}}%
\newcommand{\SetAlgoRefName}[1]{%
  \renewcommand{\algocf@algocfref}{#1}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
% -------------------------   Default Definitions
%
%%
%%
%
\SetKwComment{tcc}{/* }{ */}%
\SetKwComment{tcp}{// }{}%
%
%\newcommand{\algocf@defaults@common}{
%
%
% english keywords (default)
%
\SetKwHangingKw{KwHData}{Data$\rightarrow$}
\SetKwInput{KwIn}{Input}%
\SetKwInput{KwOut}{Output}%
\SetKwInput{KwData}{Data}%
\SetKwInput{KwResult}{Result}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
%
% French keywords
%
\ifthenelse{\boolean{algocf@localkw@french}\OR\equal{\algocf@languagechoosen}{french}}{%
%\SetKwInOut{AlgDonnees}{Donn\'ees}\SetKwInOut{AlgRes}{R\'esultat}
\SetKwHangingKw{HDonnees}{Donnees$\rightarrow$}
\SetKwInput{Donnees}{Donn\'ees}%
\SetKwInput{Res}{R\'esultat}%
\SetKwInput{Entree}{Entr\'ees}%
\SetKwInput{Sortie}{Sorties}%
\SetKw{KwA}{\`a}%
\SetKw{Retour}{retourner}%
\SetKwBlock{Deb}{d\'ebut}{fin}%
\SetKwRepeat{Repeter}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{Si}{SinonSi}{Sinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Suivant}{Cas}{Autre}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{Pour}{pour}{faire}{fin pour}%
\SetKwFor{PourPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{PourCh}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{PourTous}{pour tous les}{faire}{fin pour tous}%
\SetKwFor{Tq}{tant que}{faire}{fin tq}%
}{}%
%
% --- German keywords
%
\ifthenelse{\boolean{algocf@localkw@german}\OR\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{Ein}{Eingabe}%KwIn
\SetKwInput{Aus}{Ausgabe}%KwOut
\SetKwInput{Daten}{Daten}%KwData
\SetKwInput{Ergebnis}{Ergebnis}%KwResult
\SetKw{Bis}{bis}%KwTo
\SetKw{KwZurueck}{zur\"uck}%KwRet
\SetKw{Zurueck}{zur\"uck}%Return
\SetKwBlock{Beginn}{Beginn}{Ende}%Begin
\SetKwRepeat{Wiederh}{wiederhole}{bis}%Repeat
%
\SetKwIF{Wenn}{SonstWenn}{Sonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Unterscheide}{Fall}{Anderes}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{Fuer}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{FuerPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{FuerJedes}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{FuerAlle}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{Solange}{solange}{tue}{Ende solange}%While
}{}%
%
% --- Czech keywords
%
\ifthenelse{\boolean{algocf@localkw@czech}\OR\equal{\algocf@languagechoosen}{czech}}{%
\SetKwInput{Vst}{Vstup}%
\SetKwInput{Vyst}{V\'{y}stup}%
\SetKwInput{Vysl}{V\'{y}sledek}%
}{}%
%
% --- Portuguese keywords
%
\ifthenelse{\boolean{algocf@localkw@portuguese}\OR\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{Entrada}{Entrada}%
\SetKwInput{Saida}{Sa\'{i}da}%
\SetKwInput{Dados}{Dados}%
\SetKwInput{Resultado}{Resultado}%
\SetKw{Ate}{at\'{e}}
\SetKw{KwRetorna}{retorna}%
\SetKw{Retorna}{retorna}%
\SetKwBlock{Inicio}{in\'{i}cio}{fim}%
\SetKwRepeat{Repita}{repita}{at\'{e}}%
%
\SetKwIF{Se}{SenaoSe}{Senao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Selec}{Caso}{Outro}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{Para}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ParaPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ParaCada}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ParaTodo}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{Enqto}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
%
% --- Italian keywords
%
\ifthenelse{\boolean{algocf@localkw@italiano}\OR\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIng}{Ingresso}%
\SetKwInput{KwUsc}{Uscita}%
\SetKwInput{KwDati}{Dati}%
\SetKwInput{KwRisult}{Risultato}%
\SetKw{KwA}{a}%
\SetKw{KwRitorna}{ritorna}%
\SetKw{Ritorna}{ritorna}%
\SetKwBlock{Inizio}{inizio}{fine}%
\SetKwRepeat{Ripeti}{ripeti}{finch\'e}%
%
\SetKwIF{Sea}{AltSe}{Altrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{Per}{per}{fai}{fine per}%
\SetKwFor{PerPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{PerCiascun}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{PerTutti}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{Finche}{finch\'e}{fai}{fine finch\'e}%
}{}%
%
% --- Spanish keywords
%
\ifthenelse{\boolean{algocf@localkw@spanish}\OR\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{Datos}{Datos}
\SetKwInput{Resultado}{Resultado}
\SetKwInput{Entrada}{Entrada}
\SetKwInput{Salida}{Salida}
\SetKw{KwA}{a}
\SetKw{KwDevolver}{devolver}
\SetKw{Devolver}{devolver}
\SetKwBlock{Inicio}{inicio}{fin}
\SetKwIF{SSi}{EnOtroCasoSi}{EnOtroCaso}{si}{entonces}{sin\'o, si}{sin\'o}{fin si}
\SetKwSwitch{Seleccionar}{Caso}{Otro}{seleccionar}{hacer}{caso}{sin\'o}{fin caso}{fin seleccionar}
\SetKwFor{Para}{para}{hacer}{fin para}
\SetKwFor{ParaPara}{par}{hacer en paralelo}{fin para}
\SetKwFor{EnParalelo}{para}{hacer en paralelo}{fin para}
\SetKwFor{Mientras}{mientras}{hacer}{fin mientras}
\SetKwFor{ParaCada}{para cada}{hacer}{fin para cada}
\SetKwFor{ParaTodo}{para todo}{hacer}{fin para todo}
\SetKwRepeat{Repetir}{repetir}{hasta que}
}{}%
%
% Croatian keywords
%
\ifthenelse{\boolean{algocf@localkw@croatian}\OR\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwUlaz}{Ulaz}%KwIn
\SetKwInput{KwIzlaz}{Izlaz}%KwOut
\SetKwInput{KwPodaci}{Podaci}%KwData
\SetKwInput{KwRezultat}{Rezultat}%KwResult
\SetKw{KwDo}{do}%KwTo
\SetKw{KwVrati}{vrati}%KwRet
\SetKw{Vrati}{vrati}%Return
\SetKwBlock{Pocetak}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Ponavljaj}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{Ako}{InaceAko}{Inace}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Granaj}{Slucaj}{OstaliSlucajevi}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{Za}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ZaPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ZaSvaki}{za svaki}{\v{c}ini}{kraj za svaki}%mForEach
\SetKwFor{ZaSvaku}{za svaku}{\v{c}ini}{kraj za svaku}%fForEach
\SetKwFor{ZaSvako}{za svako}{\v{c}ini}{kraj za svako}%nForEach
\SetKwFor{ZaSve}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{Dok}{dok}{\v{c}ini}{kraj dok}%While
}{}%

%
% --- Turkish keywords
%
\ifthenelse{\boolean{algocf@localkw@turkish}\OR\equal{\algocf@languagechoosen}{turkish}}{%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
% %
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
% --- End 
%}
%
%\algocf@defaults@common
%
% option onelanguage redefinition
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{french}}{%
\SetKwInput{KwIn}{Entr\'ees}%
\SetKwInput{KwOutSortie}{Sorties}%
\SetKwInput{KwData}{Donn\'ees}%
\SetKwInput{KwResult}{R\'esultat}%
\SetKw{KwTo}{\`a}%
\SetKw{KwRet}{retourner}%
\SetKw{Return}{retourner}%
\SetKwBlock{Begin}{d\'ebut}{fin}%
\SetKwRepeat{Repeat}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Switch}{Case}{Other}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{For}{pour}{faire}{fin pour}%
\SetKwFor{ForPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{ForEach}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{ForAll}{pour tous}{faire}{fin pour tous}%
\SetKwFor{While}{tant que}{faire}{fin tq}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{KwIn}{Eingabe}%KwIn
\SetKwInput{KwOut}{Ausgabe}%KwOut
\SetKwInput{KwData}{Daten}%KwData
\SetKwInput{KwResult}{Ergebnis}%KwResult
\SetKw{KwTo}{bis}%KwTo
\SetKw{KwRet}{zur\"uck}%KwRet
\SetKw{Return}{zur\"uck}%Return
\SetKwBlock{Begin}{Beginn}{Ende}%Begin
\SetKwRepeat{Repeat}{wiederhole}{bis}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Switch}{Case}{Other}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{For}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{ForPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{ForEach}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{ForAll}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{While}{solange}{tue}{Ende solange}%While
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Sa\'{i}da}%
\SetKwInput{KwData}{Dados}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{at\'{e}}
\SetKw{KwRet}{retorna}%
\SetKw{Return}{retorna}%
\SetKwBlock{Begin}{in\'{i}cio}{fim}%
\SetKwRepeat{Repeat}{repita}{at\'{e}}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Switch}{Case}{Other}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{For}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ForPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ForEach}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ForAll}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{While}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIn}{Ingresso}%
\SetKwInput{KwOut}{Uscita}%
\SetKwInput{KwData}{Dati}%
\SetKwInput{KwResult}{Risultato}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{ritorna}%
\SetKw{Return}{ritorna}%
\SetKwBlock{Begin}{inizio}{fine}%
\SetKwRepeat{Repeat}{ripeti}{finch\'e}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{For}{per}{fai}{fine per}%
\SetKwFor{ForPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{ForEach}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{ForAll}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{While}{finch\'e}{fai}{fine finch\'e}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Salida}%
\SetKwInput{KwData}{Datos}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{devolver}%
\SetKw{Return}{devolver}%
\SetKwBlock{Begin}{inicio}{fin}%
\SetKwRepeat{Repeat}{repetir}{hasta que}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{entonces}{si no, si}{en otro caso}{fin si}
\SetKwSwitch{Switch}{Case}{Other}{seleccionar}{hacer}{caso}{si no}{fin caso}{fin seleccionar}
\SetKwFor{For}{para}{hacer}{fin para}%
\SetKwFor{ForPar}{para}{hacer in paralelo}{fin para}%
\SetKwFor{ForEach}{para cada}{hacer}{fin para cada}
\SetKwFor{ForAll}{para todo}{hacer}{fin para todo}
\SetKwFor{While}{mientras}{hacer}{fin mientras}
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwIn}{Ulaz}%KwIn
\SetKwInput{KwOut}{Izlaz}%KwOut
\SetKwInput{KwData}{Podaci}%KwData
\SetKwInput{KwResult}{Rezultat}%KwResult
\SetKw{KwTo}{do}%KwTo
\SetKw{KwRet}{vrati}%KwRet
\SetKw{Return}{vrati}%Return
\SetKwBlock{Begin}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Repeat}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Switch}{Case}{Other}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{For}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ForPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ForEach}{za svaki}{\v{c}ini}{kraj za svaki}%ForEach
\SetKwFor{ForAll}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{While}{dok}{\v{c}ini}{kraj dok}%While
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{turkish}}{%
%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
%
%%%% old commands compatibility
%
\ifthenelse{\boolean{algocf@oldcommands}}{%
\newcommand{\SetNoLine}{\SetAlgoNoLine}%
\newcommand{\SetNoline}{\SetAlgoNoLine}%
\newcommand{\SetVline}{\SetAlgoVlined}%
\newcommand{\SetLine}{\SetAlgoLined}%
%
\newcommand{\dontprintsemicolon}{\DontPrintSemicolon}%
\newcommand{\printsemicolon}{\PrintSemicolon}%
\newcommand{\incmargin}[1]{\IncMargin{#1}}%
\newcommand{\decmargin}[1]{\DecMargin{-#1}}%
\newcommand{\setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\Setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\setalcapskip}[1]{\SetAlCapSkip{#1}}%
\newcommand{\setalcaphskip}[1]{\SetAlCapHSkip{#1}}%
\newcommand{\nlSty}[1]{\NlSty{#1}}%
\newcommand{\Setnlsty}[3]{\SetNlSty{#1}{#2}{#3}}%
\newcommand{\linesnumbered}{\LinesNumbered}%
\newcommand{\linesnotnumbered}{\LinesNotNumbered}%
\newcommand{\linesnumberedhidden}{\LinesNumberedHidden}%
\newcommand{\showln}{\ShowLn}%
\newcommand{\showlnlabel}[1]{\ShowLnLabel{#1}}%
\newcommand{\nocaptionofalgo}{\NoCaptionOfAlgo}%
\newcommand{\restorecaptionofalgo}{\RestoreCaptionOfAlgo}%
\newcommand{\restylealgo}[1]{\RestyleAlgo{#1}}%
%
\newcommand{\Titleofalgo}[1]{\TitleOfAlgo{#1}}%
% \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
\newcommand{\SetKwIf}[6]{\SetKwIF{#1}{#2#1}{#2}{#3}{#4}{#5 #1}{#5}{#6}}
%
\SetKwIF{gSi}{gSinonSi}{gSinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwIF{gIf}{gElsIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gIf}{gElseIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gWenn}{gSonstWenn}{gSonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwIF{gSe}{gSenaoSe}{gSenao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwIF{gSea}{gAltSe}{gAltrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKw{Ret}{return}%
\SetKwInput{Data}{Data}%
\SetKwInput{Result}{Result}%
}{%
  \relax%
}%
%
%
%
%%
%%%
%%%% END

==> files/Intro.tex <==
%\red{(needs to be polished quite a bit..)}


Temporal logic motion planning has emerged as one of the main approaches for specifying a richer class of robot tasks than the classical point-to-point navigation and can capture temporal and Boolean requirements, such as sequencing, surveillance or coverage
\cite{fainekos2005hybrid,kress2007s,smith2011optimal,tumova2016multi,chen2012formal,ulusoy2013optimality,ulusoy2014optimal,shoukry2017linear,shoukry2018smc,vasile2013sampling,kantaros2017Csampling,kantaros2018text}. Common in these works is that they typically assume robots with \textit{known} dynamics operating in \textit{known} environments that are modeled using discrete abstractions, e.g., transition systems. 
%Nevertheless, constructing expressive discrete abstractions makes the synthesis problem computationally expensive. 
As a result, these methods cannot be applied to scenarios where the environment is initially unknown and, therefore, online re-planning may be required as environmental maps are constructed;  resulting in limited applicability. To mitigate this issue, learning-based approaches have also been proposed that consider robots with \textit{unknown} dynamics operating in \textit{unknown} environments. These approaches learn policies that directly map on-board sensor readings to control commands in a trial-and-error fashion; see e.g., \cite{dorsa2014learning,li2017reinforcement,jones,gao2019reduced,hasanbeig2019reinforcement}. However, learning approaches, in addition to being data inefficient, are specialized to the  environment they were trained on and do not generalize well to previously unseen environments. %On the other hand, learning-free approaches typically rely on repeatedly re-planning trajectories towards intermediate goals within the robot’s known environment, with the expectation that the robot will eventually fulfill its assigned mission \cite{bekris2007greedy,guo2013revising,guo2015multi}. However, such planning strategies are not necessarily complete, i.e., a solution may not be found even if it exists, and their computational cost increases as the size of the environment or the number of robots increases which restricts their applicability.

%is shortsighted in that it does not reason about the map beyond the observed environment, resulting in greedy and inefficient trajectories


%%%%%

This paper addresses a motion planning problem for multiple robots with \textit{known} dynamics that need to accomplish collaborative complex tasks in \textit{unknown} environments. We consider robots that are tasked with accomplishing collaborative tasks captured by global Linear Temporal Logic (LTL) formulas in complex environments with unknown obstacles. To address this problem, we propose the first reactive, abstraction-free, and distributed temporal logic planning algorithm for complex mission planning in unknown environments. The robots are equipped with sensors that allow them to continuously learn an individual or shared occupancy grid map of the environment, using existing Simultaneous Localization and Mapping (SLAM) methods \cite{elfes1989using,thrun2001learning,thrun2005probabilistic,grisetti2007improved}, while reacting and adapting mission planning to the updated map.
%
Furthermore, the proposed algorithm is abstraction-free i.e., it does not rely on any discrete abstraction of the robot dynamics (e.g., transition systems) and distributed in the sense that the temporal logic task is decomposed into local point-to-point navigation tasks. These local tasks are formulated online based on the continuously learned map and can be solved using existing approaches 
\cite{karaman2011sampling,guzzi2013human,liu2016high,otte2016rrtx,bansal2019combining,vasilopoulos2018sensor,ryll2019efficient,tordesillas2020faster}.
%\cite{karaman2011sampling,guzzi2013human,pivtoraiko2013incremental,liu2016high,otte2016rrtx,bansal2019combining,ryll2019efficient,elhafsi2019map,zhai2019path,tordesillas2020faster}. 
The decomposition of the global LTL task into local reachability tasks allows for efficient re-planning as the robots can make decisions locally to accomplish the assigned LTL task while communicating intermittently with each other when new reachability tasks need to be designed. 
%, a task that is particularly challenging in unknown environments.
%To achieve that, we first translate the LTL specification into an automaton which is then pruned by removing transitions that can never be enabled (e.g., transitions that are enabled if a robot is simultaneously present in more than one location). Then, as the robots navigate the workspace they collaboratively select the automaton state they should reach next so that they move closer to the accepting/final automaton states (i.e., so that they make progress towards accomplishing the assigned task). By appropriately decomposing the Boolean formula that enables this automaton transition, every robot selects locations that they need to visit next to reach the desired automaton state. Then, every robot solves a \textit{local} shortest-path optimal control problem to design paths that reach the desired location in space and, consequently, the desired automaton state. These paths are locally revised online as  the map of the environment is updated as per sensor measurements. 
%Unlike the majority of relevant works, we show that by appropriately introducing delays in the execution of the synthesized motion plans, the robots can move asynchronously in the workspace. 
Theoretically, we show there exists a fragment of LTL formulas for which decomposition into local reachability tasks is always possible. Furthermore, we show that the paths designed to address these reachability sub-tasks can be executed asynchronously(?) across the robots. Finally, we prove that under mild assumptions on the coarse structure of the environment and the sensor model, the proposed planning algorithm is complete. 

%\subsection{Temporal Logic Planning in Known Environments}
%Control synthesis for mobile robots under complex tasks, captured by LTL formulas, build upon either bottom-up approaches when independent LTL expressions are assigned to robots \cite{kress2009temporal,kress2007s,bhatia2010sampling,smith2011optimal,fu2016optimal,tumova2016multi} or top-down approaches when a global LTL formula describing a collaborative task is assigned to a team of robots \cite{chen2011synthesis,chen2012formal,kloetzer2010automatic,ulusoy2012robust,ulusoy2013optimality,ulusoy2014optimal}, as in this work. %Common in the above works is that they rely on model checking tools \cite{baier2008principles,clarke1999model} to design correct-by-construction paths that satisfy the LTL tasks. 
%Common in these works is that optimal paths are synthesized for every robot using the individual transition systems that capture robot mobility and an automaton that represents the global LTL specification. Specifically, by taking the synchronous product among the transition systems and the NBA, a synchronous product automaton can be constructed \cite{baier2008principles,clarke1999model}. Then, representing the latter automaton as a graph and using graph-search techniques, optimal motion plans can be derived that satisfy the global LTL specification and optimize a cost function. As the number of robots or the size of the automaton increases, the state-space of the product automaton grows exponentially and, as a result, graph-search techniques become intractable. Consequently, these motion planning algorithms scale poorly with the number of robots and the complexity of the assigned task. Temporal logic planning algorithms for large-scale multi-robot systems have recently been proposed that rely on decomposing the automaton into local smaller automata \cite{schillinger2016decomposition}, SMT methods \cite{shoukry2017linear,shoukry2018smc}, or sampling-based techniques \cite{vasile2013sampling,kantaros2017Csampling,kantaros2018text,kantaros2018temporal}. Common in all the above works is that they assume that the environment is \textit{a priori} known, and, therefore, motion plans can be synthesized offline. 


%{\bf{Temporal Logic Tasks in Unknown Environments:}} 
%{\bf{Related Research:}}
\subsection{Related Research}
%Temporal logic planning has been studied extensively in \cite{fainekos2005hybrid,kress2007s,smith2011optimal,tumova2016multi,chen2012formal,ulusoy2013optimality,ulusoy2014optimal,shoukry2017linear,shoukry2018smc,vasile2013sampling,kantaros2017Csampling,kantaros2018text}. Common in these works is that they consider known environments while the majority of them rely on the application of graph search methods on a product automaton to compute correct-by-construction paths. Due to the centralized nature of these algorithms, their computational cost increases as the number of robots, the complexity of the task, or the size of the environment increases. 
%of these temporal logic planning approaches As a result, their application in unknown environments raises computational challenges, since they need to be re-executed online to design new robot paths as the environmental map is learned.\footnote{\red{[this paragraph is possibly not needed]}}%In fact, their computational cost increases as the number of robots, the complexity of the task, or the size of the environment increases. 

Reactive temporal logic planning algorithms that can account for map uncertainty in terms of incomplete environment models have been developed  in \cite{guo2013revising,guo2015multi,maly2013iterative,lahijanian2016iterative,livingston2012backtracking,livingston2013patching,kress2009temporal,alonso2018reactive}. Particularly, \cite{guo2013revising,guo2015multi} model the environment as transition systems which are partially known. Then discrete controllers are designed by applying graph search methods on a product automaton. As the environment, i.e., the transition system, is updated, the product automaton is locally updated as well, and new paths are re-designed by applying graph search approaches on the revised automaton. %However, construction of a product automaton and application of graph search techniques is computationally expensive.
A conceptually similar approach is proposed in \cite{maly2013iterative,lahijanian2016iterative} as well. The works in \cite{livingston2012backtracking,livingston2013patching} propose methods to locally patch paths as transition systems, modeling the environment, change so that GR(1) (General Reactivity of Rank 1) specifications are satisfied. Reactive to LTL specifications planning algorithms are proposed in \cite{kress2009temporal,alonso2018reactive}, as well. Specifically, in \cite{kress2009temporal,alonso2018reactive} the robot reacts to the environment while the task specification captures this reactivity. Correctness of these algorithms is guaranteed if the robot operates in an environment that satisfies the assumptions that were explicitly modeled in the task specification. 
%
Common in all these works is that, unlike our approach, they rely on discrete abstractions of the robot dynamics  \cite{belta2005discrete,pola2008approximately}. Thus, correctness of the generated motion plans is guaranteed with respect to the discrete abstractions resulting in a gap between  the generated discrete motion plans and their physical low-level implementation \cite{desaisoter}.
%
Moreover, the reactive algorithms proposed in \cite{guo2013revising,guo2015multi,maly2013iterative,lahijanian2016iterative,livingston2012backtracking,livingston2013patching,kress2009temporal,alonso2018reactive} are centralized as they rely on constructing a product automaton among all robots to synthesize motion plans. As a result, their their computational cost for online re-planning increases as the number of robots, the complexity of the task, or the size of the environment increase.
%also supported by our comparative simulation studies.
To the contrary, our algorithm is highly scalable due to its distributed nature and the fact that it avoids altogether the construction of a product automaton. %Specifically, we show that there exists a fragment of LTL that can decomposed into a sequence of \textit{local} reachability tasks that can be efficiently solved online as the map of the environment is learned using existing methods  \cite{karaman2011sampling,guzzi2013human,otte2016rrtx,bansal2019combining,ryll2019efficient,elhafsi2019map,zhai2019path,tordesillas2020faster}. 
%
%
Finally, note that decomposition of fragments of LTL formulas into reachability tasks has been investigated in \cite{fainekos2006translating,bisoffi2018hybrid,jagtap2019formal}, as well, assuming robots that operate in known environments. %For instance, \cite{fainekos2006translating} considers flat LTL formulas while \cite{bisoffi2018hybrid,jagtap2019formal}  considers safe-LTL formulas satisfied by finite traces. 
Common in these works is that temporal logic tasks are decomposed into \textit{global/multi-agent} reachability tasks. As a result, these methods face scaling challenges as the number of robots increases and require synchronous motion among all agents. Our proposed method mitigates these issues by decomposing temporal logic tasks  into \textit{local} reachability tasks. %We emphasize that this is the first temporal logic planning algorithm over continuously learned occupancy grid maps.

%cite{fainekos2006translating} as well. However, in these works temporal logic tasks are decomposed into \textit{global/multi-agent} reachability tasks while the computational cost of solving global reachability tasks increases as the number of robots increases. %As a result, it is computationally
%
%To the contrary, our approach does not rely on abstractions of the robot dynamics and, therefore, avoids altogether the construction of a product automaton and scales well with the number of robots. 

\subsection{Contribution}
%{\bf{Contributions:}}
The contribution of this paper can be summarized as follows.
\textit{First}, we propose the \textit{first} temporal logic planning algorithm over continuously learned occupancy grid maps. The proposed algorithm is reactive, distributed, and abstraction-free. \textit{Second}, we show that the proposed algorithm is complete under assumptions on the coarse structure of the environment and the sensor model. \textit{Third}, we provide extensive comparative simulation studies and hardware experiments that corroborate the efficacy and scalability of the proposed algorithm.



%The rest of the paper is organized as follows. The problem formulation is presented Section \ref{sec:PF} while the proposed distributed algorithm for LTL planning is presented in Section \ref{sec:planning}. Correctness of the proposed algorithm is dicussed in Section \ref{sec:complOpt}. In Section \ref{sec:Sim}, we provide numerical experiments. Conclusive remarks are provided in the last section.

==> files/PF.tex <==

% ------------------------------------------------------------------------------- %
%\subsection{Robot \& Sensor Model}
Consider $N$ mobile robots that reside in an environment $\Omega\subset \reals^d$ with non-overlapping and known regions of interest, denoted  by $\ell_i\subset \Omega$, and \textit{static} but \textit{unknown} obstacles $O\subset\Omega$, where $d$ is the dimension of the workspace. The robots are governed by the following dynamics: $\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$,
% 
%\begin{equation}\label{eq:rdynamics}
%\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t)),
%\end{equation}
for all $j\in\ccalN:=\{1,\dots,N\}$, where $\bbp_{j}(t) \in\mathbb{R}^n$ stands for the state (e.g., position and orientation) of robot $j$ at time $t\geq 0$, $\bbu_{j}(t)$. %stands for a control input in a \textit{finite} space of admissible controls $\ccalU_j$. %\NA{state that time is discrete}
%Note that the state $\bbp_{j}$ may belong to a higher dimensional space than $\Omega_{\text{free}}$. For example, this is the case if $\bbp_j(t)$ includes the position and the orientation of robot $j$. Nevertheless, throughout the rest of the paper, for simplicity of notations we denote $\bbp_{j}(t) \in \Omega_{\text{free}}$.\BS{Can we make this into a  remark or just remove it? It's extra clutter for something that is fairly straightforward.} 
%Also, note that the considered dynamics can range from simple graph-based dynamics to arbitrary nonlinear discrete dynamics\NA{This sentence could be removed}. 
Hereafter, we compactly denote the dynamics of all robots as 
\begin{equation}\label{eq:rdynamics}
\bbp(t+1)=\bbf(\bbp(t),\bbu(t)),
\end{equation}
where $\bbp(t)\in \mathbb{R}^{n\times N}$, $\forall t\geq 0$. %, and $\bbu(t)\in\ccalU:=\ccalU_1\times\dots\times\ccalU_N$.

Moreover, we assume that the robots are equipped with sensors (e.g., LiDAR or camera) to detect if a given location $\bbq\in\Omega$ belongs to the obstacle-free space. Specifically, we consider the following deterministic sensor model:
\begin{equation}\label{eq:sensor}
   s(\bbp_j(t),\bbq)=
            \begin{cases}
               1~\text{if~}(\bbq\in O) \wedge (\lVert \bbp_j(t)-\bbq \rVert\leq R),\\
              0~\text{otherwise}.
            \end{cases} 
\end{equation}

\noindent In words, given a location $\bbq\in\Omega$ that lies within the sensing range $R$ of robot $j$, we have that $s(\bbp_j(t),\bbq)=1$ if $\bbq$ belongs to the obstacle-space, i.e., $\bbq\in O$; otherwise, $s(\bbp_j(t),\bbq)=0$. 

Using sensor measurements as per \eqref{eq:sensor}, the robots collectively build a shared (binary) occupancy grid map defined as follows. First, the workspace $\Omega$ is partitioned into $K$ grid cells denoted by $c_i\subset\Omega$. Then, given $C=\{c_1,c_2,\dots,c_K\}$, we define
a function a function $g: C\times \bbs_{0:t} \rightarrow \set{0,1}^K$ that maps each grid cell $c_i$ to $0$ or $1$, given all robot measurements up to time $t$, denoted by $\bbs_{0:t}$. 
%
The function $g$ is defined as follows:
\begin{equation}\label{eq:updMap}
   g(c_i,\bbs_{0:t})=
            \begin{cases}
               1~\text{if~}\exists j, \bbq\in c_i,~t'\leq t~\text{s.t}~s(\bbp_j(t'),\bbq)=1,\\
              0~\text{otherwise}.
            \end{cases} 
\end{equation}
In words, if there exists at least one robot $j$ that took a measurement at any past time instant $t'\leq t$ indicating that there exists an obstacle within the grid cell $c_i$ (i.e., $s(\bbp_j(t'),\bbq)=1$), then $g(c_i,\bbs_{0:t})=1$, i.e., $c_i$ is considered an obstacle. Otherwise, $g(c_i,\bbs_{0:t})=0$, which means that $c_i$ is either obstacle-free or no measurement associated with $c_i$ has been taken up to the current time instant $t$. As a result, $g$ produces a binary occupancy grid map $M(t)=\{m_1(t),m_2(t),\dots,m_K(t)\}$, where (i) $m_i(t)=1$ if $g(c_i,\bbs_{0:t})=1$ (ii) and $m_i(t)=0$ if $g(c_i,\bbs_{0:t})=0$. 
%
%
%
%For simplicity of notation, we assume that all robots can exchange their sensor measurements at any time $t$ through a connected communication network and, therefore, they have access to same global map $M(t)$.\footnote{The proposed algorithm can straightforwardly be extended to the case where each robot $j$ builds its own map $M_j$ and adapts its planning to $M_j$.} %if $\bbq$ belongs to the obstacle-free space, for all locations $\bbq$ that lie with the sensing range $R$ of robot $i$.
%\red{here we need to define the occupancy grid map that we build... otherwise it is unlcear what exactly $q$ is.}
Note that the occupancy grid map is constructed as per \eqref{eq:updMap} assuming deterministic and noiseless sensor models as in \eqref{eq:sensor}. In practice, to account for noisy sensors, the function $g$ in \eqref{eq:updMap} can be determined by inference methods (e.g., particle filters) giving rise to probabilistic maps which are then thresholded yielding binary maps $M(t)$ as e.g., in \cite{elfes1989using,thrun2001learning,thrun2005probabilistic,grisetti2007improved}. Moreover, for simplicity of notation, we assume that all robots build a shared map $M(t)$. This can be relaxed by allowing each robot to build its own local map $M_j(t)$, based on its individual sensor measurements.
%in \eqref{eq:updMap} we assume that all robots can exchange their sensor measurements at any time through a connected communication network and, therefore, they have access to same global map $M(t)$. Nevertheless, this can be relaxed by allowing each robot to build its own local map $M_j$, based on its individual sensor measurements. %Also, in Section \ref{sec:Sim}, we show that the proposed algorithm can be applied even without building maps, by leveraging recently proposed algorithms that consider point-to-point navigation problems in the presence of unknown obstacles \cite{guzzi2013human,vasilopoulos2018sensor,bansal2019combining}.
%, and adapt its planning to $M_j$ instead of $M$ 
%\footnote{The proposed algorithm can straightforwardly be extended to the case where each robot $j$ builds its own map $M_j$ and adapts its planning to $M_j$.} 
%Second, we consider deterministic and noiseless sensor models in \eqref{eq:sensor}. In practice, to account for noisy sensors, the function $g$ can be determined by inference methods (e.g., particle filters) giving rise to probabilistic maps which are then thresholded yielding binary maps $M(t)$ as e.g., in \cite{elfes1989using,thrun2001learning,thrun2005probabilistic,grisetti2007improved}. 

%\subsection{Task Specification using Linear Temporal Logic}
The goal of the robots is to accomplish a complex collaborative task captured by a global Linear Temporal Logic (LTL) specification $\phi$. The assigned task $\phi$ is defined over a set of atomic propositions $\mathcal{AP}=\cup_{\forall j}\mathcal{AP}_j$ where $\mathcal{AP}_j=\cup_i\set{\pi_{j}^{\ell_i},\pi_j^{O}}$, and $\pi_{j}^{\ell_i}$ and $\pi_{j}^{O}$ are atomic predicates that are true when robot $j$ is within region $\ell_i$ and hits an obstacle, respectively.
%
In what follows, we briefly present the syntax and semantics of LTL. A detailed overview of this theory can be found in \cite{baier2008principles}. The basic ingredients of LTL are a set of atomic propositions $\mathcal{AP}$, the boolean operators, i.e., conjunction $\wedge$, and negation $\neg$, and two temporal operators, next $\bigcirc$ and until $\mathcal{U}$. LTL formulas over a set $\mathcal{AP}$ can be constructed based on the following grammar: $\phi::=\text{true}~|~\pi~|~\phi_1\wedge\phi_2~|~\neg\phi~|~\bigcirc\phi~|~\phi_1~\mathcal{U}~\phi_2$, where $\pi\in\mathcal{AP}$. For brevity we abstain from presenting the derivations of other Boolean and temporal operators, e.g., \textit{always} $\square$, \textit{eventually} $\lozenge$, \textit{implication} $\Rightarrow$, which can be found in \cite{baier2008principles}. 
%
%An infinite \textit{word} $\sigma$ over the alphabet $2^{\mathcal{AP}}$ is defined as an infinite sequence  $\sigma=\pi_0\pi_1\pi_2\dots\in (2^{\mathcal{AP}})^{\omega}$, where $\omega$ denotes an infinite repetition and $\pi_k\in2^{\mathcal{AP}}$, $\forall k\in\mathbb{N}$. The language $\texttt{Words}(\phi)=\left\{\sigma\in (2^{\mathcal{AP}})^{\omega}|\sigma\models\phi\right\}$ is defined as the set of words that satisfy the LTL formula $\phi$, where $\models\subseteq (2^{\mathcal{AP}})^{\omega}\times\phi$ is the satisfaction relation.
%
%Any LTL formula $\phi$ can be translated into a Nondeterministic B$\ddot{\text{u}}$chi Automaton (NBA) over $(2^{\mathcal{AP}})^{\omega}$ denoted by $B$ \cite{vardi1986automata}, which is defined as follows:
%\begin{definition}
%A \textit{Nondeterministic B$\ddot{\text{u}}$chi Automaton} (NBA) $B$ over $2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\Sigma,\rightarrow_B,\mathcal{Q}_B^F\right)$, where $\ccalQ_{B}$ is the set of states, $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is a set of initial states, $\Sigma=2^{\mathcal{AP}}$ is an alphabet, $\rightarrow_{B}\subseteq\ccalQ_{B}\times \Sigma\times\ccalQ_{B}$ is the transition relation, and $\ccalQ_B^F\subseteq\ccalQ_{B}$ is a set of accepting/final states. 
%\end{definition}
%
%An \textit{infinite run} $\rho_B$ of $B$ over an infinite word $\sigma=\pi_0\pi_1\pi_2\dots$, where $\pi_k\in\Sigma$, for all $ k\in\mathbb{N}$, is a sequence $\rho_B=q_B^0q_B^1q_B^2\dots$ such that $q_B^0\in\ccalQ_B^0$ and $(q_B^{k},\pi_k,q_B^{k+1})\in\rightarrow_{B}$, $\forall k\in\mathbb{N}$. An infinite run $\rho_B$ is called \textit{accepting} if $\texttt{Inf}(\rho_B)\cap\ccalQ_B^F\neq\varnothing$, where $\texttt{Inf}(\rho_B)$ represents the set of states that appear in $\rho_B$ infinitely often. The words $\sigma$ that result in an accepting run of $B$ constitute the accepted language of $B$, denoted by $\ccalL_B$. It is proven \cite{baier2008principles} that the accepted language of $B$ is equivalent to the words of $\phi$, i.e., $\ccalL_B=\texttt{Words}(\phi)$. 
%
%Hereafter, we assume that in $\Omega$ there are non-overlapping regions of interest, denoted by $\ell_i\subseteq \Omega$ with known locations.\footnote{\red{explain why it is trivial to consider overlapping regions..}} However, the locations of obstacles are \textit{a priori} unknown. 
An example of an LTL specification is: $\phi=\Diamond(\pi_1^{\ell_1}\wedge (\pi_1^{\ell_2}\wedge (\Diamond \pi_1^{\ell_3}))) \wedge\Box (\neg(\pi_1^{O}\vee \pi_{1}^{\ell_{4}})) $, which requires the robot to (i) eventually visit locations $\ell_1$, $\ell_2$, and $\ell_{3}$ in this order; and (ii) avoid all a priori unknown obstacles and region $\ell_{4}$ since hostile units may exist there. %until robot $2$ visit location $\ell_3$, captured by $\neg\pi_1^{\ell_1}\ccalU \pi_1^{\ell_3}$; and (iii) both robots to avoid hitting any obstacle captured by $\Box (\wedge_{j}(\vee_{\ell_{\text{obs}}}\pi_j^{\ell_{\text{obs}}}))$. %Note that the robots know the coordinates of the target locations $\ell_1$ and $\ell_3$ but they are not aware of the locations of obstacles denoted by $\ell_{\text{obs}}$. Specifically, throughout the paper, we assume that the coordinates of all target locations $\ell_i$ are known but the coordinates of obstacles are completely unknown.
%
Hereafter, we exclude the `next' operator $\bigcirc$ from the syntax, since it is not meaningful for practical robotics applications; this is common in relevant works, see, e.g., \cite{kloetzer2008fully} and the references therein. LTL formulas are satisfied by discrete plans $\tau$ that are
infinite sequences of locations of $N$ robots in $\Omega$. i.e., $\tau=\bbp(0),\bbp(1),\dots,\bbp(t),\dots$ \cite{baier2008principles}. %Given an LTL formula $\phi$, if there exists a plan $\tau$ satisfying $\phi$, then it can be written in a finite representation, called prefix-suffix structure, i.e., $\tau=\tau_{\text{pre}}[\tau_{\text{suf}}]^{\omega}$, where the  prefix part $\tau_{\text{pre}}=\bbp(0),\bbp(1),\dots,\bbp(K)$ is executed only once followed by the indefinite execution of the suffix part $\tau_{\text{suf}}=\bbp(K+1),\bbp(\bbp(K+2)),\dots,\bbp(K+S)$, where $\bbp(K+S)=\bbp(K)$ and $\omega$ denotes the indefinite execution of $\tau_{\text{suf}}$. 
%
%In order to interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times M(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current robot system state $\bbp(t)\in\mathbb{R}^{n\times N}$ and the current map $M(t)$ of the environment.
%%%%%%%%%%%%%%
%
%\subsection{Mission Planning Problem in Unknown Environments}
%Given a task specification $\phi$, our goal is to select a stopping time $H$ and a sequence $\bbu_{0:H}$ of control inputs $\bbu(t)$, for all $t\in\set{0,\dots,H}$, that satisfies $\phi$ while minimizing a motion cost. This gives rise to the following optimal control problem:
%
%\footnotesize
%\begin{subequations}
%\label{eq:Prob2}
%\begin{align}
%& \min_{\substack{H, \bbu_{0:H}}} \left[J(H,\bbu_{0:H}) = %\int_{t=0}^{H}  w(\bbp(t),\bbu(t))dt \right] \label{obj2}\\
%& \ \ \ \ \ \ \ \ \ \ \  \bbp_{0:H}\models\phi  \label{constr1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \dot{\bbp}(t) = \bbf(\bbp(t),\bbu(t)). %\label{constr2}
%\end{align}
%\end{subequations}
%
%\normalsize
%where $w(\bbp(t),\bbu(t))\geq 0$ is a motion cost function that captures e.g., the energy consumption or control effort, and $\bbp_{0:H}$ is the path of the multi-robot system until the time instant $H$. 
The problem addressed in this paper can be summarized as follows:
\begin{problem} \label{prob}
Given an initial robot configuration $\bbp(0)$ in an environment with unknown obstacles, the robot dynamics \eqref{eq:rdynamics}, sensor models \eqref{eq:sensor}, and a task specification captured by an LTL formula $\phi$ (which also requires obstacle avoidance), compute a plan $\tau$ that satisfies $\phi$ and respects the robot dynamics.% as per \eqref{eq:Prob2}.
\end{problem}

Problem \ref{prob} can be solved by applying existing abstraction-free approaches for LTL planning, e.g., \cite{vasile2013sampling,luo2019abstraction}, at runtime to continuously update the robot paths as the map of the environment is continuously learned. These methods require searching over a large product automaton space, a task that is computationally challenging to perform at runtime. To mitigate this challenge, we propose a new reactive LTL planning algorithm that does not rely on searching over a product automaton space. In particular, in Section \ref{sec:aut}, we decompose the temporal logic task into a sequence of local point-to-point navigation problems which allows for efficient and fast re-planning. These navigation problems are formulated and solved online while adapting to the updated map of the environment; see Sec. \ref{sec:planning}.

%\begin{rem}
%Note that in this section, we made two main assumptions. First, we assume that all robots can exchange their sensor measurements at any time through a connected communication network and, therefore, they have access to same global map $M(t)$. This can be relaxed by allowing each robot to build its own local map $M_j$, based on its individual sensor measurements. %Also, in Section \ref{sec:Sim}, we show that the proposed algorithm can be applied even without building maps, by leveraging recently proposed algorithms that consider point-to-point navigation problems in the presence of unknown obstacles \cite{guzzi2013human,vasilopoulos2018sensor,bansal2019combining}.
%, and adapt its planning to $M_j$ instead of $M$ 
%\footnote{The proposed algorithm can straightforwardly be extended to the case where each robot $j$ builds its own map $M_j$ and adapts its planning to $M_j$.} 
%Second, we consider deterministic and noiseless sensor models in \eqref{eq:sensor}. In practice, to account for noisy sensors, the function $g$ can be determined by inference methods (e.g., particle filters) giving rise to probabilistic maps which are then thresholded yielding binary maps $M(t)$ as e.g., in \cite{elfes1989using,thrun2001learning,thrun2005probabilistic,grisetti2007improved}. 
%\end{rem}

==> files/alg_April8_2020.tex <==
%
In this section, we provide an algorithm to decompose global LTL task into local reachability tasks. This process occurs offline i.e., before deploying the robots in the unknown environment. Specifically, in Section \ref{sec:nba} we translate the LTL formula into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA). In Section \ref{sec:prune} we prune this automaton by removing infeasible transitions i.e., transitions that can be activated only if a robot is present in more than one location simultaneously. Then, in Section \ref{sec:dec} we provide conditions under which feasible NBA transitions can be enabled by solving local reachability tasks. Such transitions are called decomposable. In Section \ref{sec:dist}, using the definition of feasible and decomposable transitions, we define a distance metric over the NBA that measures how far the robots are from fulfilling the assigned mission. This metric will be used in Section \ref{sec:planning} to guide and adapt planning to the continuously learned map of the environment.


\subsection{From LTL formulas to Automata}\label{sec:nba}

First, we translate the specification $\phi$, constructed using a set of atomic predicates $\mathcal{AP}$, into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA), defined as follows \cite{baier2008principles}. %Given a temporal logic formula $\phi$ , with syntax and semantics as described in Definitions \ref{syntax} and \ref{semantics}, respectively, a DFA is defined as follows:

\begin{definition}[NBA]
A Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\delta_B, \ccalQ_F\right)$, where (i) $\ccalQ_{B}$ is the set of states;
(ii) $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is the initial state; (iii) $\delta_B:\ccalQ_B\times\Sigma\rightarrow\ccalQ_B$ is a non-deterministic transition relation, and $\ccalQ_F\subseteq\ccalQ_{B}$ is a set of accepting/final state. 
\end{definition}

To interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times M(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current multi-robot state $\bbp(t)\in\mathbb{R}^{n\times N}$ and the current map $M(t)$ of the environment. An infinite-length discrete plan $\tau=\bbp(0)\bbp(1)\dots$ satisfies $\phi$, denoted by $\tau\models\phi$, if the word $\sigma=L(\bbp(0), M(0))L(\bbp(1),M(1))\dots$ yields an accepting NBA run defined as follows. First, a run of $\rho_B$ of $B$ over an infinite word $\sigma=\sigma(1)\sigma(2)\dots\sigma(t)\dots\in(2^{\mathcal{AP}})^{\omega}$, is a sequence $\rho_B=q_B(0)q_B(1)q_B(2)\dots,q_B(t),\dots$, where $q_B(0)\in\ccalQ_B^0$ and $\delta_B(q_B(t),\sigma(t),q_B(t+1)$, $\forall t\in\mathbb{N}$. %Hereafter, we equivalently denote $\delta_B(q_B(t),\sigma(t),q_B(t+1)$ as $q_B(t)\rightarrow_B q_B(t+1)$.
A run $\rho_B$ is called \textit{accepting} if at least one final state appears infinitely often in it. In words, an infinite-length discrete plan $\tau$ satisfies an LTL formula $\phi$ if it can generate at least one accepting NBA run. Hereafter, for simplicity we replace $L(\bbp(t),M(t))$ with $L(\bbp(t))$.
%The symbols $\sigma$ that result in an accepting run of $D$ constitute the accepted language of $D$.

%The proposed reactive algorithm builds online (i.e., as the robots navigate the environment) paths that live in the infinite-dimensional space $\Omega^N\times\ccalQ_D$. The synthesized paths are updated as the map of the environment is updated. 

%Specifically, let $q_B(t)\in\ccalQ_B$ denote the NBA state that the multi-robot system has reached at time $t$ given all observations that have been made (i.e., all atomic predicates that have been satisfied) until $t$, where $q_B(0)\in\ccalQ_B^0$ [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. 

%In Section \ref{sec:planning}, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task. Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task. To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that (i) it is  one-hop reachable from $q_B(t)$, (ii) the transition from $q_B(t)$ to $q_B^{\text{next}}$ is feasible, i.e., observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously, and (iii) $q_B^{\text{next}}$ is `closer' to the final states than $q_B(t)$ is. %Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. 
%In what follows, we describe these steps in detail.
%In Section \ref{sec:prune} we define when an NBA transition is feasible and when it is decomposable i.e., it can be enabled via solving local reachability-avoidance problems. In Section \ref{sec:dist}, we define a distance metric over the NBA that measures how far each NBA state is from the set of final states.

%Next, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task; see Algorithm \ref{alg:RRT}. Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task. To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that it is (i) one-hop reachable from $q_B(t)$, (ii) `closer' to the final states than $q_B(t)$ is according to a distance function defined over the NBA, and (iii) observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously. Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. In what follows, we describe these steps in detail.


%Once this transition is enabled, the robots update the target DFA state $q_D^{\text{next}}$ until they reach a final DFA state.%\footnote{In case the DFA has more than one initial state, then there is more than one state $\bbq(0)$ that can be used as a root. In this case, a separate tree is build for each one of possible roots.}
%For this, we assume that the initial robot configuration allows the robots to stay in $q_B(0)$.
%

%By convention the cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = 0$, while the cost of a node $\bbq(t+1)=[\bbp(t+1), q_D]\in\ccalV$, given its parent node $\bbq(t)=[\bbp(t),q_D']\in\ccalV$, is computed as 
%\begin{equation}\label{eq:costUpd}
%J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq(t)) +  w(\bbp(t),\bbp(t+1)).
%\end{equation}
%Observe that by applying \eqref{eq:costUpd} recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:Prob2}.

 
%Given the current DFA state $q_D(t)$, the robots first select a DFA state $q_D^{\text{next}}\in\ccalQ_D$ that is `closer' to the final state $q_F$ than $q_D(t)$ is and observations that generate a transition from $q_D(t)$ to $q_D^{\text{next}}$ can be generated. Therefore,
%\subsection{Selecting the Next DFA State}\label{sec:targetDFA}

%{\bf{Pruning the DFA:}}
\subsection{Pruning Infeasible NBA Transitions}\label{sec:prune}
%Given the current NBA state $q_B(t)$, a new state $q_B^{\text{next}}$ is selected so that it is closer to the final states. Thus, to select $q_B^{\text{next}}$, we need to define a distance function over the state-space of the NBA that measures how far each state is from the final state. %(in terms of the number feasible transitions/hops required to reach $q_F$). 
%To achieve that, we first prune the NBA $B$ by removing transitions that cannot be enabled [line \ref{rrt:prune}, Alg. \ref{alg:RRT}]. %This is required to define a distance function over the state-space of the DFA. %
%
%Specifically, the pruned NBA is constructed by removing all infeasible NBA transitions. 
In what follows, we define the \textit{feasible/infeasible} NBA transitions $\delta_B(q_B,\cdot,q_B')$. Transitions that are infeasible are removed giving rise to a pruned automaton. To formally define the \textit{feasible} NBA transitions we first need to introduce the following definitions. %\cite{kantaros2018text}.
%
%We also rewrite $b^{\text{inv}}^{q_D}$ and $b^{\text{next}}^{q_D,q_D'}$ as follows:
%\begin{equation}\label{eq:eq1}
%    b^{\text{inv}}^{q_D} = b^{\text{inv}}^{\text{goal}} \triangle (\neg b^{\text{inv}}^{\text{avoid}} ),
%\end{equation}

%\begin{equation}\label{eq:eq2}
%    b^{\text{next}}^{q_D,q_D'} = b^{\text{next}}^{\text{goal}} \triangle (\neg b^{\text{next}}^{\text{avoid}} ),
%\end{equation}
%where in the Boolean formulas  $b^{\text{next}}^{\text{goal}}$, $b^{\text{next}}^{\text{avoid}}$, $b^{\text{inv}}^{\text{goal}}$ and $b^{\text{inv}}^{\text{avoid}}$ the negation operator does not appear in front of any atomic proposition. Also, in \eqref{eq:eq1} and \eqref{eq:eq2}, $\triangle$ denotes either the logical AND ($\wedge$) or the logical OR $(\vee)$ operator.

% defined in \ref{defn:wTS}.%\footnote{Recall from Definition \ref{defn:wTS} that $\text{wTS}_i$ is defined over $\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma_i=2^{\mathcal{AP}_i}$. Also, recall from Definition \ref{def:pts} that the PTS is defined over $\mathcal{AP}=\bigcup_{i=1}^N\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma=2^{\mathcal{AP}}$. Also, throughout the paper, we denote the finite symbols by $\sigma^*\in\Sigma$ and the infinite symbols by $\sigma\in\Sigma^{\omega}$.}
\begin{definition}[Feasible symbols $\sigma_j\in\Sigma_j$]\label{defn:infTSi}
A symbol $\sigma_j\in\Sigma_j:=2^{\mathcal{AP}_j}$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, where $b_j^{\text{inf}}$ is a Boolean formula defined as 
\begin{equation}\label{bInfTSi}
b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e}(\pi_j^{r_i}\wedge\pi_j^{r_e})).
%b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e})),
\end{equation}
where $b_j^{\text{inf}}$ requires robot $j$ to be present simultaneously in more than one disjoint region.
\end{definition}

%We also need to define when a symbol $\sigma\in\Sigma$ is \textit{feasible}, i.e., when it can be generated by the multi-robot system. To this end, we first need to define the
%In other symbols $\sigma_j\in\Sigma_j=2^{\mathcal{AP}_j}$ that are feasible, i.e, the symbols that can be generated by robot $j$ \cite{kantaros2018text}. 


Note that the Boolean formula $b_j^{\text{inf}}$ is satisfied by any finite symbol $\sigma_j\in\Sigma_j$ that requires robot $j$ to be present in two or more disjoint regions, simultaneously. For instance, the symbol $\sigma_j=\pi_j^{r_i}\pi_j^{r_e}$ satisfies $b_j^{\text{inf}}$ if $r_i$ and $r_e$ are disjoint regions. %\footnote{Note that if we consider regions $r_i$ that are not necessarily disjoint, then the Boolean formula $b_j^{\text{inf}}$ is defined as $b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e}))$. Note also that definition of infeasible symbols depends on the problem at hand, i.e, the definition of atomic propositions included in the sets $\mathcal{AP}_j$.} % if there is an overlap between regions $r_i$ and $r_e$. 
Next, we define the feasible symbols $\sigma\in\Sigma$.

\begin{definition}[Feasible symbols $\sigma\in\Sigma$]\label{defn:infPTS}
A symbol $\sigma\in\Sigma$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, for all robots $j$,
where $\sigma_j=\Pi|_{\Sigma_j}\sigma$, $b_j^{\text{inf}}$ is defined in \eqref{bInfTSi}, and $\Pi|_{\Sigma_j}\sigma$ stands for the projection of the symbol $\sigma$ onto $\Sigma_j$.\footnote{For instance, $\Pi|_{\Sigma_j}(\pi_j^{r_e}\pi_m^{r_h})=\pi_j^{r_e}$.} We denote by $\Sigma_{\text{feas}}\subseteq\Sigma$ the set of all feasible symbols $\sigma\in\Sigma$. 
\end{definition}


%%%
%%%
%Next, we define the $\Sigma(q_D)=\{s\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D)\in\rightarrow_D)\}$ that collects all symbols that the robots can generate to remain in the state $q_D$. We also define the set $\Sigma(q_D,q_D')=\{\sigma\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D')\in\rightarrow_D)\}$ that collects all symbols that enable a transition from $q_D$ to $q_D'$.
%
%Moreover, for each state $q_D$, we define the set $\Sigma(q_D|p)$ that collects all symbols $\sigma$ that robots may observe if they reach $q_D$ through a path $p=q_D^0,\dots,q_D$, i.e., a sequence of states in $\ccalQ_D$ that starts at the initial state $q_D^0$ and ends at the state $q_D$. Note that there may be multiple paths that can reach $q_D$ from $q_D^0$ and, therefore, each state $q_D$ may be associated with more than one set $\Sigma(q_D|p)$. For the initial state, $q_D^0$, there is only one such set  defined as $\Sigma(q_D^0|p)=\Sigma(q_D^0)$, since in a DFA the only path $p$ to reach $q_D^0$ from $q_D^0$ is the self-loop of $q_D^0$.

%To prune the DFA we need first to construct the sets $\Sigma(q_D|p)$. Starting from $q_D^{0}$, we execute the following process for each state $q_D$ that is reachable within one hop from $q_D^0$

%First, we select a state $q_D\in\ccalQ_D$, for which all corresponding sets $\Sigma(q_D|p)$ have been constructed
%%%
%%%
%\red{unclear here..}
%To solve Problem \ref{prob}, we first decompose the assigned task into local point-to-point planning problems. Motion plans that solve these point-to-point navigation problems are locally designed online while adapting to the map of the environment that is built by the robots. The proposed algorithm is summarized in Algorithm \ref{alg:RRT}. 
%


%\begin{algorithm}[t]
%%\footnotesize
%\caption{Pruning a NBA}
%\LinesNumbered
%\label{alg:prune}
%\KwIn{NBA}
%\KwOut{Pruned NBA}
%Remove infeasible transitions (see Definition \ref{def:feas1})\label{prune:inf}\;
%Add auxiliary states and transitions\label{prune:aux}\;
%Initialize $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$, $\ccalQ_B^\text{checked}=\emptyset$, $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$\;\label{prune:init}
%Compute $\ccalQ_{q_B}^{\text{next}}$ for all $q_B\in\ccalQ_B^\text{loop}$\;
%\While{$|\ccalQ_B^{\text{not-checked}}|\neq\emptyset$}{
%    \For{$q_B\in\ccalQ_B^{\text{not-checked}}$}{
%        Compute $\ccalQ_{q_B}^{\text{next}}$\;\label{prune:nextS}
%        \For{$q_B^K\in\ccalQ_{q_B}^{\text{next}}$}{\label{prune:FornextS}
%            Replicate transition $\delta_B^K(q_B,q_B^K)$\;\label{prune:repl}
%            \If{$\delta_B^K(q_B,q_B^K)$ is decomposable (Def. \ref{def:feas})}{
%                $\ccalQ_B^{\text{dec}}=\ccalQ_B^{\text{dec}}\cup\{q_B^K\}$\;\label{prune:UpdLoop} 
%            }
%            \Else{
%                Remove transition $\delta_B^K(q_B,\cdot,q_B^K)$ from the NBA and the set $\ccalP_{q_B}^{\text{next}}$\;\label{prune:remNonDec}
%            }
%        }
%        One-hop transitions $\delta_B(q_B,\cdot,q_B')$ that are not part of any run in $\ccalP_{q_B}^{\text{next}}$ are removed\;\label{prune:prune2}
%    }
%    $\ccalQ_{B}^{\text{checked}}=\ccalQ_{B}^{\text{not-checked}}$\;
%    $\ccalQ_{B}^{\text{not-checked}}=\ccalQ_B^{\text{dec}}\setminus\ccalQ_{B}^{\text{checked}}$\;
%}
%%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
%\end{algorithm}

\begin{algorithm}[t]
%\footnotesize
\caption{Computing Decomposable Transitions}
\LinesNumbered
\label{alg:prune}
\KwIn{Pruned NBA}
\KwOut{Sets $\ccalQ_{q_B}^{\text{next}}$, $\Sigma^{q_B,q_B'}_{\text{dec}}$, $\forall q_B\in\ccalD_{q_B^\text{aux}}$}
%Remove infeasible transitions (see Definition \ref{def:feas1})\label{prune:inf}\;
Add auxiliary states and transitions\label{prune:aux}\;
Compute the set $\ccalD_{q_B^{\text{aux}}}$\;\label{prune:reachAux}
\For{$q_B\in\ccalD_{q_B^{\text{aux}}}$}{
    Initialize $\ccalQ_{q_B}^{\text{next}}=\emptyset$\;
    \For{each run \eqref{eq:run}}{\label{prune:forRun}%that ends in a state $q_B'\in\ccalD_{q_B^{\text{aux}}}$
        \If{$\delta_B^m(q_B,\cdot,q_B')$ is decomposable (Def. \ref{def:feas1})}{\label{prune:ifDec}
        $\ccalQ_{q_B}^{\text{next}}=\ccalQ_{q_B}^{\text{next}}\cup\{q_B'\}$\;\label{prune:upd1}
        }
         Collect in $\Sigma^{q_B,q_B'}_{\text{dec}}$ all symbols $\sigma^{q_B,q_B'}$ that satisfy Def. \ref{def:feas1} \;\label{prune:upd2}
        }

    }
$\ccalQ_B^{\text{dec}}=\bigcup_{q_B\in\ccalD_{q_B^{\text{aux}}}}\ccalQ_{q_B}^{\text{next}}$\;
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}





Next, we define the sets that collect all feasible symbols that enable a transition from an NBA state $q_B$ to another, not necessarily different, NBA state $q_B'$; see also Example \ref{ex:exFeasSets}. This definition relies on the fact that transition from a state $q_B$ to a state $q_B'$ is enabled if a Boolean formula, denoted by $b^{q_B,q_B'}$ and defined over the set of atomic predicates $\mathcal{AP}$, is satisfied.  %The set of all atomic predicates associated with robots $j\in\mathcal{N}_{q_B,q_B'}$ is defined by $\mathcal{AP}_{q_B,q_B'}=\bigcup_{j\in\mathcal{N}_{q_B,q_B'}}\mathcal{AP}_j$.

\begin{definition}[Sets of Feasible Symbols]
Let $\mathcal{AP}_{q_B,q_B'}$ be a set that collects all atomic predicates that appear in the Boolean formula $b^{q_B,q_B'}$ associated with an NBA transition $\delta_B(q_B,\cdot, q_B')$. Given $b^{q_B,q_B'}$, we define the set $\Sigma^{q_B,q_B'}\subseteq 2^{\mathcal{AP}_{q_B,q_B'}}$ 
that collects all symbols $\sigma$ that (i) satisfy the corresponding Boolean formula $b^{q_B,q_B'}$, i.e., $\sigma\models b^{q_B,q_B'}$; and (ii) $\sigma\in\Sigma_{\text{feas}}$. %; and (iii) are associated with robots that appear in $b^{q_B,q_B'}$. 
%If the empty symbol $\varnothing$ satisfies (i), then $\Sigma^{q_B,q_B'}=\set{\varnothing}$. 
%The set $\mathcal{AP}_{q_B,q_B'}$ collects all atomic predicates that appear in $b^{q_B,q_B'}$.
\label{defn:feasSet}
\end{definition}

%Moreover, let $b^{\text{inv}}^{q_D}$ denote the Boolean formula that needs to be satisfied to enable a loop around $q_D$, i.e., a transition from $q_D$ to $q_D$.\footnote{Note that $b^{\text{inv}}^{q_D}$ exists for all states $q_D$, since the `next' operator is excluded from the syntax. Also, the Boolean formulas that should be satisfied to enable a  transition from a state $q_D$ to $q_D'$ can be provided by tools that convert temporal logic formulas to automata.} Let also $\Sigma^{\text{inv}}^{q_D}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b^{\text{inv}}^{q_D}$. 
%
%Let also $b^{\text{next}}^{q_D,q_D'}$ denote the Boolean formula that needs to be satisfied to enable a transition from $q_D$ to $q_D'$ and $\Sigma^{\text{next}}^{q_D,q_D'}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b^{\text{next}}^{q_D,q_D'}$.
%Also, from $\Sigma_{\text{text}}^{q_D,q_D'}$, we exclude symbols associated with robots that do not play any role in satisfying $b^{\text{next}}^{q_D,q_D'}$. For instance, if $b^{\text{next}}^{q_D,q_D'}=\pi_j^{r_e}\vee\pi_j^{r_m}$, then $\Sigma_{\text{text}}^{q_D,q_D'}$ is defined as $\Sigma_{\text{text}}^{q_D,q_D'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$, i.e., it does not include any symbol associated with other robots $i\neq j$ that may also satisfy $b^{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_i^{r_f}$). The same also holds for $\Sigma^{\text{inv}}^{q_D}$; see also Example \ref{ex:feas}. %Additionally, in case the empty symbol, denoted by $\varnothing$ belongs to 
%

Given the sets $\Sigma^{q_B,q_B'}$, we define the infeasible NBA transitions defined as follows:

\begin{definition}[Infeasible NBA Transitions]\label{def:feas1}
A transition $\delta_B(q_B,\cdot,q_B')$ is infeasible if $\Sigma^{q_B,q_B'}=\emptyset$.
\end{definition}

In words, an NBA transition is infeasible if it is enabled only when at least one robot is present in more than one location in the environment simultaneously. All infeasible NBA transitions are pruned; see e.g., Figure \ref{fig:prune}. % line \ref{prune:inf}, Alg. \ref{alg:prune}]. 
%we remove all NBA transitions with $\Sigma_{q_B,q_B'}=\emptyset$, i.e., all transitions that are enabled if at least one robot is present in more than one location in the environment simultaneously [. 



%Next we remove NBA transitions that require robots to move from one region of interest $\ell_i$ to another one $\ell_e$ without visiting any location $\bbq$ in the environment outside $\ell_i$. Such transitions are considered infeasible as they require robots to `jump' from one region of interest to another one. For instance, consider the LTL formula $\phi=\pi_1^{r_1}\ccalU\pi_1^{r_2}$ that requires robot $1$ to be in region $r_1$ until it enters $r_2$. The corresponding NBA is illustrated in Figure \ref{fig:NBA1}. Assume that the initial condition of the robot satisfies $b^{q_B^0,q_B^0}=\pi_1^{r_1}$, i.e., that robot $1$ is initially located in $r_1$. Then the transition from the initial to the final state is considered infeasible as it requires the robot to `jump' from one region of interest to another one. 


\begin{figure}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Original NBA]{
    \label{fig:origNBA}
  \includegraphics[width=0.46\linewidth]{figures/feas1_bf.png}}
  \subfigure[Pruned NBA (Def. \ref{def:feas1})]{
    \label{fig:feas1}
  \includegraphics[width=0.38\linewidth]{figures/NBA2.png}}
%  \caption{FEASIBLE 1}
%  \label{fig:tow7}
%\end{figure}
%
%\begin{figure}[t]
%  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      %\subfigure[Replicating NBA states]{
    %\label{fig:repl}
 % \includegraphics[width=0.3\linewidth]{figures/NBA3.png}}
  \caption{Graphical illustration of Algorithm \ref{alg:prune} applied to the NBA corresponding to $\phi=\square\Diamond(\pi_1^{\ell_1})\wedge\square\Diamond(\pi_1^{\ell_2})$. This formula requires robot $1$ to visit infinitely often $\ell_1$ and $\ell_2$. Figure \ref{fig:origNBA} shows the original NBA where the states $q_B^0$ and $q_F$ correspond to the initial and final state of the NBA. The red dashed transitions are infeasible, as per Definition \ref{def:feas}, as they require robot $1$ to be in $\ell_1$ and $\ell_2$ simultaneously.  These transitions are removed  yielding the pruned NBA shown in Figure \ref{fig:feas1}. An auxiliary state $q_B^{\text{aux}}$ is added to the pruned NBA; see Figure \ref{fig:feas1}.
  Observe in Figure \ref{fig:feas1} that $\ccalD_{q_B^{\text{aux}}}=\{q_B^{\text{aux}},q_B^0,q_B\}$. Also, there are two runs in the form \eqref{eq:run} originating from $q_B$: $\rho_1=q_Bq_B$ and $\rho_2=q_B q_F q_B^0$. Note that the run $\rho=q_B q_F q_B$ cannot be generated as there is no feasible symbol that satisfies $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$. In fact, this run requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$ instantaneously. %Due to $\rho_2$, the intermediate state $q_F$ is replicated so that it has one incoming transition from $q_B$ and one outgoing transition to $q_B^0$; see Figure \ref{fig:repl}. The transition from $q_B$ to the original $q_F$ is removed. 
  Thus $\ccalQ_{q_B}^{\text{next}}=\{q_B,q_B^0\}$. Similarly, for $q_B^0$ there are two runs in the form \eqref{eq:run}: $\rho_1=q_B^0q_B^0$ and $\rho_2=q_B^0 q_B$ and $\ccalQ_{q_B^0}^{\text{next}}=\{q_B,q_B^0\}$.% The set $\ccalQ_B^{\text{dec}}$  constructed by alg. \ref{alg:prune} is $\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}},q_B^0,q_B\}$. 
  %
  %Observe in Figure \ref{fig:feas1} that there is no self-loop for the final state $q_F$. Thus, $q_F$ is replicated twice since it has one incoming and two outgoing transitions as shown in Figure \ref{fig:repl}. In Figure \ref{fig:repl} the multi-hop transition $q_B\rightarrow_B q_F\rightarrow_B q_B$ is removed since there are no symbols that satisfy $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$ (condition (i)-Defn. \ref{def:feas}); in fact this transition requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$. The resulting pruned NBA generated by Algorithm \ref{alg:prune} is shown in Figure \ref{fig:finalPrune}.  
  }
  \label{fig:prune}
\end{figure}

\begin{figure}
    \centering
     %\includegraphics[width=0.6\linewidth]{figures/p1Up2.png}
       \subfigure[Original NBA]{
    \label{fig:origNBAU}
  \includegraphics[width=0.45\linewidth]{figures/NBA1u.png}}
    \subfigure[Pruned NBA]{
    \label{fig:finalNBA2}
  \includegraphics[width=0.45\linewidth]{figures/NBAU.png}}
    %\subfigure[Pruned NBA]{
   % \label{fig:finalNBA3}
  %\includegraphics[width=0.3\linewidth]{figures/nba3u.png}}
    \caption{Effect of the initial robot state in computing decomposable transitions. Figure \ref{fig:origNBAU} depicts the NBA corresponding to $\phi=\pi_1^{\ell_1}\ccalU\pi_1^{\ell_2}$. All transitions are feasible as per Def. \ref{def:feas1}. Observe in Figure \ref{fig:finalNBA2} that if the initial robot state $\bbp(0)=\ell_1$, then $\ccalD_{q_B^{\text{aux}}}=\{q_B^{\text{aux}},q_B^0\}$. Note that the final state $q_F$ is not reachable from $q_B^0$. Also, $\ccalQ_{q_B^{\text{aux}}}^{\text{next}}=\{q_B^0,q_B^{\text{aux}}\}$ and $\ccalQ_{q_B^0}^{\text{next}}=\{q_B^0\}$. Note that the transition from $q_B^0$ to $q_F$ (red dashed line) does not satisfy Def. \ref{def:feas} and therefore the final state $q_F$ is not reachable. %In this case $\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}},q_B^0\}$. 
    If $\bbp(0)=\ell_2$, then $\ccalD_{q_B^{\text{aux}}}=\{q_B^{\text{aux}},q_F\}$, $\ccalQ_{q_B^{\text{aux}}}^{\text{next}}=\{q_B^{\text{aux}},q_F\}$, and $\ccalQ_{q_{F}}^{\text{next}}=\{q_F\}$. %, and $\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}},q_F\}$.
    %$\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}},q_B^0\}$. Also, there only decomposable transition originating from $q_B^0$ is its self-loop. As a result, the transition   Transition from the initial state $q_B^0$ to the final state $q_B^F$ is infeasible as robot $1$ is required to `jump' from $\ell_1$ to $\ell_2$ while $\ell_1$ and $\ell_2$ are disjoint regions.
    }
    \label{fig:NBA1}
\end{figure}


\subsection{Computing Decomposable NBA Transitions}\label{sec:dec}

In this section, we discuss when an NBA transition can be enabled by requiring each robot to solve a local reachability problem; such transitions are called decomposable. The process of determining which NBA transitions are decomposable is summarized in Algorithm \ref{alg:prune} and illustrated in Figures \ref{fig:prune}-\ref{fig:NBA1}.

First, to take into account the initial multi-robot state in this process, we introduce an auxiliary state $q_B^{\text{aux}}$ and transitions from $q_B^{\text{aux}}$ to all initial states $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=\wedge_{j\in\ccalN} L(\bbp_j(0))$, i.e., transition from $q_B^\text{aux}$ to $q_B^0$ can always be enabled; see also Figure \ref{fig:NBA1} [line \ref{prune:aux}, Alg. \ref{alg:prune}]. Hereafter, the auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA. %The set $\ccalQ_B^{\text{dec}}$ is initialized as $\ccalQ_B^{\text{dec}}=\{q_B^{\text{aux}}\}$ [line \ref{prune:init}, Alg. \ref{alg:prune}].


Let $\ccalD_{q_B^{\text{aux}}}$ a set that collects all NBA states $q_B$ with a feasible self-loop, as per Definition \ref{def:feas1}, for which there exists a finite and feasible word $w$, i.e., a finite sequence of feasible symbols, that can incur a finite NBA run $\rho_w$ that ends in $q_B$ and activate the self-loop of $q_B$ [line \ref{prune:reachAux}, Alg. \ref{alg:prune}]. In math, $\ccalD_{q_B^{\text{aux}}}$ is defined as:
%$\ccalD_{q_B^{\text{aux}}}$ is defined as:
\begin{align}\label{eq:reach}
    \ccalD_{q_B^{\text{aux}}}=&\{q_B\in\ccalQ_B|\\&(\Sigma^{q_B,q_B}\neq\emptyset)\wedge(\exists w~\text{s.t.}~\rho_{w}=q_B^{\text{aux}}\dots \bar{q}_B q_Bq_B)\nonumber\}.
\end{align}

By definition of $q_B^{\text{aux}}$, we have that $q_B^{\text{aux}}\in\ccalD_{q_B^{\text{aux}}}$. Consider any two states $q_B, q_B'\in\ccalD_{q_B^{\text{aux}}}$ for which there exists a symbol, denoted by $\sigma^{q_B,q_B'}$, the following run, starting from $q_B$, will be generated: 
\begin{equation}\label{eq:run}
    \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}q_B^{K},
\end{equation}
where $q_B'=q_B^K$. In \eqref{eq:run}, the run is defined so that (i) $q_B^k\neq q_B^{k+1}$, for all $k\in\{1,K-1\}$; (ii) $\delta_B(q_B^k,\sigma^{q_B,q_B'},q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$, i.e., the robots cannot remain in any of the intermediate states (if any) that connect $q_B$ to $q_B'$ either because a feasible self-loop does not exist or because $\sigma^{q_B,q_B'}$ cannot activate this self-loop; and (iii) $\delta_B(q_B',\sigma^{q_B,q_B'},q_B')$ i.e., there is a feasible loop associated with $q_B'$ that is activated by $\sigma^{q_B,q_B'}$ and, therefore, the robots can remain in $q_B'$ as long as $\sigma^{q_B,q_B'}$ is generated. The fact that the finite repetition of a \textit{single} symbol needs to generate the run \eqref{eq:run} precludes multi-hop transitions from $q_B$ to $q_B'$ that require a robot to jump from one region of interest to another one instantaneously as such transitions are not meaningful as discussed in Section \ref{sec:PF}; see e.g., Fig. \ref{fig:feas1}. Hereafter, we denote the multi-hop transition incurred due to the run \eqref{eq:run} by  $\delta_{B}^m(q_B,\cdot,q_B')$.

%Hereafter, we denote by $\delta_B^K(q_B,\cdot,q_B^K)$ the multi-hop NBA transition corresponding to the run \eqref{eq:run}. 
%
The symbol $\sigma^{q_B,q_B'}$ is selected from $\Sigma^{q_B,q_B'}$ that is constructed from the Boolean formula \eqref{eq:b} as per Definition \ref{defn:feasSet}.
\begin{equation}\label{eq:b}
   b^{q_B,q_B'}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}.  
\end{equation}
By definition of \eqref{eq:b}, if there exists a symbol $\sigma^{q_B,q_B'}$ that satisfies $b^{q_B,q_B'}$ then the finite word generated by repeating $K+1$ times the symbol $\sigma^{q_B,q_B'}$ can yield the run in \eqref{eq:run}. 
%
%
%
%Note that such a state $q_B^{K}$ can always be reached (assuming $\phi$ is satisfiable), since 
Note that given a state $q_B$, finding a symbol $\sigma^{q_B,q_B'}$ and a state $q_B'$ can be accomplished by viewing the NBA as a directed graph and applying graph-search methods on it.


%Next we define the decomposable transitions $\delta_B^{K_i}(q_B,q_B^{K_i})$; for simplicity of notation, when it is clear from the context we drop the index $i$. If $\delta_B^{K}(q_B,q_B^K)$ is not decomposable, then the multi-hop transition $\delta_B^{K}(q_B,q_B^{K})$ is removed. To define the decomposable transitions, we need first to introduce the following definition. 


%THE ROBOTS IN $\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$ GET OUT OF THEIR CURRENT REGIONS!
%q_B^K\in\ccalQ_B^{\text{dec}}

Next, we define when the multi-hop transition from $q_B$ to $q_B'$ is decomposable. To define this we need first to introduce the following definitions. First, given the Boolean formula $b^{q_B,q_B'}$ in \eqref{eq:b}, we define the set $\ccalN^{q_B,q_B'}\subseteq\ccalN$ that collects the indices of all robots that appear in $b^{q_B,q_B'}$. Also, given a symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$, we define the set $\ccalR^{q_B,q_B'}\subseteq\ccalN^{q_B,q_B'}$ that collects the indices $j$ of the robots that are involved in generating $\sigma^{q_B,q_B'}$. Also, we denote by $L_{j}^{q_B,q_B'}$ the location that robot $j\in\ccalN^{q_B,q_B'}$ should be located to generate $\sigma^{q_B,q_B'}$. Note that for robots $j\in\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$, $L_{j}^{q_B,q_B'}$ corresponds to any location $\bbq\in\Omega$ where no atomic predicates are satisfied; see also Example \ref{ex:exFeasSets}. 



\begin{definition}[Decomposable NBA transitions]\label{def:feas}
A transition $\delta_{B}^m(q_B,\cdot,q_B')$ corresponding to a run as in \eqref{eq:run} is decomposable if for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$, there exists at least one symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$
such that either (A) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}=\emptyset$ or (B) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B'}$.
\end{definition}

Observe that Definition \ref{def:feas} allows us to cast transition from $q_B$ to states $q_B'$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B'}$ needs to move to a region of interest $L_{j}^{q_B,q_B'}$ while avoiding obstacles and/or other regions of interest so that the symbol $\sigma^{q_B,q_B'}$ is generated; this will be discussed in detail in Section \ref{sec:planning}. This decomposition of the temporal logic task allows for computationally and efficient re-planning as the map of the environment is continuously learned.

Moreover, note that there may be more than one (if any) decomposable transitions originating from $q_B\in\ccalD_{q_B^{\text{aux}}}$ [line \ref{prune:forRun}, Alg. \ref{alg:prune}]. Hereafter, we collect all these states in a set $\ccalQ_{q_B}^{\text{next}}$ [line \ref{prune:upd1}, Alg. \ref{alg:prune}], i.e.,
\begin{equation}
    \ccalQ_{q_B}^{\text{next}}=\{q_B'\in\ccalD_{q_B^{\text{aux}}}~|~\delta_B^m(q_B,\cdot,q_B')~\text{is decomposable}\}.
\end{equation}

Also, there may be more than one symbol $\sigma^{q_B,q_B'}$ that satisfies both $b^{q_B,q_B'}$ in \eqref{eq:b} and Definition \ref{def:feas}. As a result, there may be more than one symbol $\sigma^{q_B,q_B'}$ that can enable the decomposable transition from $q_B$ to $q_B'$.  Hereafter, we collect all these symbols in the set $\Sigma_{\text{dec}}^{q_B,q_B'}\subseteq \Sigma^{q_B,q_B'}$ [line \ref{prune:upd2}, Alg. \ref{alg:prune}]. 

\begin{figure}
    \centering
     \includegraphics[width=1\linewidth]{figures/conserv.png}
    \caption{Decomposing global LTL tasks into local reachability tasks is not always possible. This figure shows the NBA corresponding to $\phi=\square(\pi_1^{\ell_0}\vee\pi_2^{\ell_0}) \wedge \Diamond \pi_2^{\ell_1}\wedge \Diamond \pi_2^{\ell_1}$. This formula requires either robot $1$ or $2$ to always be in $\ell_0$ and eventually robots $1$ and $2$ to visit, not necessarily simultaneously, $\ell_1$. Transition from $q_B^0$ to $q_B^F$ is removed as it requires robots to visit more than one location at the same time. Observe that the transitions from $q_B$ to $q_F$ and from $q_B'$ to $q_F$ do not satisfy  Definition \ref{def:feas}, i.e., $\ccalQ_{q_B}^{\text{next}}=\{q_B\}$ and $\ccalQ_{q_B'}^{\text{next}}=\{q_B'\}$, resulting in a disconnected graph $\ccalG$. For instance, consider the transition from $q_B$ to $q_F$. 
    %Assuming that both robots are initially in $\ell_0$, 
    Observe that transition from $q_B$ to $q_F$ cannot be cast as two independent reachability-avoidance problems. In fact, it requires coordination among the robots that is specific to the Boolean formula $b^{q_B,q_F}$. Specifically, when the robots reach $q_B$, we have that robot $1$ is in $\ell_0$ and robot $2$ is in $\ell_1$. To eventually satisfy $b^{q_B,q_F}=(\pi_1^{\ell_0}\wedge\pi_2^{\ell_1})\vee(\pi_2^{\ell_0}\wedge\pi_2^{\ell_1})$, first robot $2$ is required to return in $\ell_0$ while in the meantime robot $1$ should stay in $\ell_0$. Once robot $2$ returns in $\ell_0$, robot $1$ should move to $\ell_1$ enabling the transition to the final state $q_F$.}
    \label{fig:conserv}
\end{figure}
%Nevertheless, a solution exists, as these two transitions can be enabled in practice. 

\begin{rem}[Definition \ref{def:feas}]
Consider any transition $\delta_B^{m}(q_B,\cdot,q_B')$ associated with the finite run \eqref{eq:run}. If $\delta_B^{m}(q_B,\cdot,q_B')$ does not satisfy Definition \ref{def:feas} then this means that the transition from $q_B$ to $q_B'$ may be either feasible to enable but not in a local-reachability fashion (see Figure \ref{fig:conserv}) or impossible to activate as it may require robots to jump from one region of interest to another one (see Figure \ref{fig:NBA1}). %Conditions under which Definition \ref{def:feas} is not conservative are discussed in Section \ref{sec:complOpt}. Specifically, we show that there exists a fragment of LTL so that if Definition \ref{def:feas} is not satisfied then transition from $q_B$ to $q_B'$ is impossible to activate as it requires robots to instantaneously jump from one region of interest to another one.
%Nevertheless, conservative pruning ensures that when the robots reach a state $q_D$, they will always be able to make progress towards accomplishing their task (i.e., reach a new state $q_D'$) regardless of the symbols they have generated to reach $q_D$ by solving local point-to-point navigation problems. A fragment of LTL for which the proposed approach is not conservative is discussed in Section \ref{sec:complOpt}.
\end{rem}

\begin{ex}(Sets of Feasible Symbols)
(a) Consider the Boolean formula $b^{q_B,q_B'}=(\pi_j^{\ell_e}\vee\pi_j^{\ell_m})\wedge(\neg \pi_i^{\ell_e})$, then $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\pi_j^{\ell_e},\pi_j^{\ell_m}, \pi_j^{\ell_e}\pi_j^{\ell_m}\}$. %, i.e., it does not include any symbol associated with other robots $k\neq j$ that may also satisfy $b^{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{\ell_e}\pi_k^{\ell_f}$).
Given the Boolean formula $b^{q_B,q_B'}$, we have that $\ccalN^{q_B,q_B'}=\set{j,i}$.
%
Also, for $\sigma^{q_B,q_B'}=\pi_j^{\ell_e}$, we have that $\ccalR^{q_B,q_B'}=\set{j}$, $L_{j}^{q_B,q_B'}=\ell_e$. (b) Consider the Boolean formula $b^{q_B,q_B'}=\neg \pi_i^{\ell_e}$. In this case $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\varnothing\}$, where $\varnothing$ denotes an empty symbol and is generated when a robot is outside all regions interests and does hit any obstacles. Also, we have that $\ccalN^{q_B,q_B'}=\set{i}$, $\sigma^{q_B,q_B'}=\varnothing$, $\ccalR^{q_B,q_B'}=\emptyset$, and while $L_{i}^{q_B,q_B'}$ corresponds to any location $\bbq$ in the workspace where no atomic predicates are satisfied. 
\label{ex:exFeasSets}
\end{ex}

%\begin{ex}[Feasible DFA transitions]\label{ex:feas}
%(a) Consider the case, where $b^{q_B,q_B}=1$ and $b^{q_B,q_B'}=\pi_j^{\ell_{m}}$. By definition of $\Sigma^{q_B,q_B}$ and $\Sigma^{q_B,q_B'}$, we have that $\Sigma^{q_B,q_B}=\{\varnothing\}$, where $\varnothing$ stands for the empty symbol, and $\Sigma^{q_B,q_B'} =\{\pi_j^{\ell_{m}}\}$. Transition from $q_B$ to $q_B'$ is feasible as per Definition \ref{def:feas}. Recall that the sets $\Sigma^{q_B,q_B}, \Sigma^{q_B,q_B'}$ collect symbols that are associated with robots that play a role in satisfying the respective Boolean formulas. This precludes cases where, e.g., a symbol $\pi_j^{\ell_e}$, $e\neq m$ is included in $\Sigma^{q_B,q_B}$ resulting in erroneously characterizing the transition from $q_D$ to $q_D'$ as infeasible due to condition (iii). 
%%%(b) Consider the following Boolean conditions: $b^{\text{inv}}^{q_D}=b^{\text{inv}}^{q_D'}=\pi_j^{\ell_i}$ and $b^{\text{next}}^{q_D,q_D'}=\pi_j^{\ell_i}\wedge \pi_m^{\ell_h}$. Then the transition from $q_D$ to $q_D'$ is feasible since it satisfies Definition \ref{def:feas}. 
%(b) Consider also the Boolean formulas  $b^{q_B,q_B}=b^{q_B',q_B'}=\pi_j^{\ell_i}$ and $b^{q_B,q_B'}=\pi_j^{\ell_e}\wedge \pi_m^{\ell_h}$, then the transition from $q_B$ to $q_B'$ is infeasible, since it holds that $j\in \ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and, $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. In fact, transition from $q_B$ to $q_B'$ requires robot $j$ to instantaneously move from $\ell_i$ to $\ell_e$ which is not possible given that $\ell_i$ and $\ell_e$ are disjoint regions. 
%\end{ex}

\subsection{Distance Metric Over the Pruned NBA}\label{sec:dist}
Given the pruned NBA, we define a function to compute how far an NBA state is from the set of final states. This metric will be used in Section \ref{sec:planning} to guide planning towards NBA states that are closer to the final states.
%By construction of the pruned automaton, for every a state $q_B\in\ccalQ_B^{\text{dec}}$ there exists a symbol that if repeated a finite number of times then another state $q_B'\in\ccalQ_B^{\text{dec}}$ can be visited while this symbol allows to remain in $q_B'$. Also, as discussed before, transition from $q_B$ to $q_B'$ will occur while possibly going through intermediate states but self-loops are
To this end, we construct a directed graph $\ccalG=\{\ccalV,\ccalE\}$ where $\ccalV$ is the set of nodes defined as $\ccalV=\ccalD_{q_B^{\text{aux}}}$ and $\ccalE\subseteq\ccalV\times\ccalV$ is the set of edges. Specifically, there exists an edge from node $q_B\in\ccalV$ to $q_B'\in\ccalV$ if $\Sigma^{q_B,q_B'}_{\text{dec}}\neq\emptyset$, i.e., if there exists a decomposable transition from $q_B$ to $q_B'$ as per Definition \ref{def:feas}; see Figure \ref{fig:graphG}. 

Given the graph $\ccalG$, we define the distance metric
$d:\ccalV\times\ccalV\rightarrow \mathbb{N}$ that returns the minimum number of transitions among states in $\ccalV$ that are required to reach a state $q_B'\in\ccalV$ starting from a state $q_B\in\ccalV$. %This function will be used to guide the robots towards locations in the workspace so that eventually a final DFA state is visited, i.e., the LTL formula is satisfied.
%
Particularly, we define the distance function $d: \ccalV \times \ccalV \rightarrow \mathbb{N}$ as follows
\begin{equation}\label{eq:dist}
d(q_B,q_B')=\left\{
                \begin{array}{ll}
                  |SP_{q_B,q_B'}|, \mbox{if $SP_{q_B,q_B'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_B,q_B'}$ denotes the shortest path (in terms of hops) in $\ccalG$ from $q_B$ to $q_B'$ and $|SP_{q_B,q_B'}|$ stands for its cost (number of hops). %\footnote{In Section \ref{sec:complOpt}, we provide conditions under which if $d(q_D^0,q_F)=\infty$ then the assigned co-safe LTL task is infeasible}. %; see Sections \ref{sec:targetDFA}-\ref{sec:paths}.
%
Next, we define the final/accepting edges in $\ccalG$.
\begin{definition}[Final/Accepting Edges]\label{def:accEdges}
An edge $(q_B,q_B')\in\ccalE$ is called final or accepting if the corresponding multi-hop NBA transition $\delta_B^m(q_B,\cdot,q_B')$ includes at least one final state $q_F\in\ccalQ_F$.
\end{definition}

Based on the definition of accepting edges, we define the set $\ccalV_F\subseteq \ccalV$ that collects all states $q_B\in\ccalV$ from which an accepting edge originates, i.e.,
\begin{equation}\label{eq:accNode}
    \ccalV_F = \{q_B\in\ccalV~|~\exists~ \text{accepting edge}~(q_B,q_B')\in\ccalE \}.
\end{equation}
By definition of the accepting condition of the NBA, we have that if at least one of the accepting edges is traversed infinitely often, then the corresponding LTL formula is satisfied. %States $q_B\in\ccalQ_B^{\text{dec}}$ for which there are accepting edges $(q_B,q_B')\in\ccalE$ are collected in a set $\ccalQ_F^{\text{dec}}$.%, i.e.,

Similar to \cite{bisoffi2018hybrid}, we define the distance of any state $q_B\in\ccalV$ to the set $\ccalV_F\subseteq \ccalV$ as
\begin{equation}\label{eq:distF}
d_F(q_B,\ccalV_F)=\min_{q_B'\in\ccalV_F}d(q_B,q_B'),
\end{equation}
where $d(q_B,q_B')$ is defined in \eqref{eq:dist} and $\ccalV_F$ is defined in \eqref{eq:accNode}; see Figure \ref{fig:graphG}.

\begin{figure}
    \centering
     %\includegraphics[width=0.6\linewidth]{figures/p1Up2.png}
  \includegraphics[width=0.7\linewidth]{figures/graphG.png}
    \caption{Graph $\ccalG$ constructed for the NBA shown in Figure \ref{fig:feas1}. The red dashed line corresponds to an accepting edge. Also, we have that $\ccalV_F=\{q_B\}$, $d_F(q_B^{\text{aux}},\ccalV_F)=2$, $d_F(q_B^{0},\ccalV_F)=1$, and $d_F(q_B,\ccalV_F)=0$.
    }
    \label{fig:graphG}
\end{figure}

\section{From Automata to Reactive Planning\\in Unknown Occupancy Grid Maps}\label{sec:planning}

%The pruning process described in Section \ref{sec:prune} occurs offline, i.e., before deploying the robots in the workspace. In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

In this section, we present a distributed reactive temporal logic algorithm for robots that operate in unknown environments modeled as occupancy grid maps. The proposed algorithm is summarized in Algorithm \ref{alg:RRT} and requires as an input the output of the Algorithm \ref{alg:prune} that was executed offline. The main idea of Algorithm \ref{alg:RRT} is that the robots select NBA states they should visit next, using the continuously learned map, so that the distance to the final states as per \eqref{eq:distF} decreases over time giving rise to local reachability planning problems. %sets $\ccalQ_{q_B}^{\text{next}}$ and the set of of symbols $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, for all $q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}$ and for all $q_B\in\ccalV$. 
%Recall that $\ccalQ_{q_B}^{\text{next}}$ collects all states, denoted by $q_B^{\text{next}}$, that can reached from $q_B$ in a decomposable fashion, as per Definition \ref{def:feas}, using a symbol selected from $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$. These sets are computed offline by Algorithm \ref{alg:prune} described in Section \ref{sec:aut}.

%for all $q_B\in\ccalQ_B^{\text{dec}}$,  In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

\subsection{Distributed Construction of Robot Paths}\label{sec:paths}
Let $q_B(t)\in\ccalV$ be the NBA state that the robots have reached at time $t$ after following paths, denoted by $\bbp_{j,[0:t]}$ so that the robots can remain in $q_B(t)$ using the current symbol $L(\bbp(t))$, i.e., $L(\bbp(t))\models b^{q_{B}(t),q_{B}(t)}$.
%
At time $t=0$, $q_B(t)$ is initialized to be the initial/auxiliary state $q_B^{\text{aux}}$, introduced in Section \ref{sec:prune} [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. Recall that $q_B^{\text{aux}}\in\ccalV$ and $L(\bbp(0))\models b^{q_{B}(0),q_{B}(0)}$, by definition of $q_B^{\text{aux}}$. 
%


\begin{algorithm}[t]
%\footnotesize
\caption{Distributed LTL Control in Unknown Occupancy Grid Maps}
\LinesNumbered
\label{alg:RRT}
\KwIn{ (i) Initial robot configuration $\bbp(0)$, (ii) Sets $\ccalQ_{q_B}^{\text{next}}$, $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, $\forall q_B\in\ccalV$ provided by Alg. \ref{alg:prune}}
%\KwOut{Terminal horizon $H$, and control inputs $\bbu_{0:H}$}
%Convert $\phi$ into a DFA\label{rrt:dfa}\;
%Initial state $\bbq(0)=[\bbp(0), q_D^0]$;\label{rrt:init}
Initialize $t=0$, $q_B(0)=q_B^{\text{aux}}$\;\label{rrt:t0}
%Update current DFA state as $q_D(0)=\delta(q_D^0,L(\bbp(0)))$\;
%Prune DFA\;\label{rrt:prune}
%Select an initial state $q_D(0)=q_D^0$ and a feasible final state $q_F^{\text{feas}}$\;\label{rrt:feasFinal}
%Current DFA state $q_D(t)=q_D^0$\;\label{rrt:init}
%Compute distance from $q_D(t)$ to $q_D^F$\;
%\If{$d(q_D^0, q_F)= \infty$}{\label{rrt:unsat1}
%Error message: \textit{$\phi$ cannot be satisfied (see Proposition \ref{prop:sat})}\;}\label{rrt:unsat2}
%Initialize $\texttt{updateLoc}=0$ and $\texttt{updateDFA}=0$\;
Select the next NBA state $q_B^{\text{next}}\in\ccalQ_{q_B(t)}^{\text{next}}$\; Select $\sigma^{\text{next}}\in\Sigma_{\text{dec}}^{q_B(t),q_B^{\text{next}}}$\;\label{rrt:selTarget}%(see
Using $\sigma^{\text{next}}$, compute $\ccalN^{\text{next}}$\;\label{rrt:compN}
\While{accepting condition of NBA is not satisfied}{\label{rrt:sat}
%
%\For{$j\in\ccalN^{\text{next}}$}{\label{rrt:for1})
%Using $\sigma^{\text{next}}$, check if $j\in\ccalN^{\text{next}}$ $L_j^{\text{next}}$ \label{rrt:goals}\;
%and the set of robots $\ccalN^{\text{next}}$\;
\For{$j\in\ccalN^{\text{next}}$}{\label{rrt:for1}
Compute paths $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$; see \eqref{eq:localProb}\;\label{rrt:compPaths}%}
Follow paths, re-plan if needed, and update map\;\label{rrt:ExecReplan}%(see Section \ref{sec:exec})
%
\If{$\bbp_j(t)\in L_j^{\text{next}}$}{\label{rrt:T}
Wait until all other robots $j\in\ccalN^{\text{next}}$ reach their goal regions.\;}\label{rrt:wait}
\If{$\bbp_j(t)\in L_j^{\text{next}}, \forall i\in\ccalN^{\text{next}}$}{\label{rrt:nowait}
Update $q_B(t)=q_B^{\text{next}}$\;\label{rrt:updNBA}
Select a new NBA state $q_B^{\text{next}}$ and  $\sigma^{\text{next}}$\;\label{rrt:updTarget}
Using $\sigma^{\text{next}}$, update $\ccalN^{\text{next}}$\;\label{rrt:updN}
%
%Compute new $L_j^{\text{next}}$ and the set of robots $\ccalN^{\text{next}}$\;\label{rrt:UpdGoals}
}
}
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\normalsize

Given the current NBA state $\bbq_B(t)$, the robots coordinate to select a new NBA state, denoted by $q_B^{\text{next}}\in\ccalV$ that they should reach next to make progress towards accomplishing their task [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. This state is selected so that the transition from $q_B$ to $q_B^{\text{next}}$ is decomposable, as per Definition \ref{def:feas}, and progress towards reaching a final state is made. Therefore, the state $q_B^{\text{next}}$ is selected from the set $\ccalQ_{q_B(t)}^{\text{next}}$ based on the following two cases.
%
If $q_B(t)\notin \ccalV_F$, where $\ccalV_F$ is defined in \eqref{eq:accNode}, then among all the states in $\ccalQ_{q_B(t)}^{\text{next}}$ we select one that satisfies
%$q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}\subseteq \ccalQ_B^{\text{dec}}$
\begin{equation}\label{eq:minDist}
d_F(q_B^{\text{next}},\ccalV_F) =  d_F(q_B(t),\ccalV_F)-1,  
\end{equation}
i.e., a state that is one hop closer to the set $\ccalV_F$ than $q_B(t)$ is where $d_F$ is defined in \eqref{eq:distF}.  Under this policy of selecting $q_B^{\text{next}}$, we have that eventually $q_B(t)=\ccalV_F$; design of robot paths to ensure this property will be discussed next. If $q_B(t)\in\ccalV_F$, then the state $q_B^{\text{next}}$ is selected so that $(q_B(t),q_B^{\text{next}})$ is an accepting edge as per Definition \ref{def:accEdges}. This way we ensure that accepting edges are traversed infinitely often and, therefore, the assigned LTL task is satisfied.

%Note that there exists at least one $q_B^{\text{next}}$ that satisfies \eqref{eq:minDist} since any path (including the shortest path) in the pruned NBA that connects $q_B(t)$ to $q_F^{\text{feas}}$ goes through one of the states in $\ccalQ_{q_B(t)}^{\text{next}}$ by construction of the pruned automaton. %and the definition of the distance metric in \eqref{eq:dist}. 
%If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}].

%Given $q_B^{\text{next}}$


%every robot $j$ needs to locally design a path so that a DFA state that is closer to the final state $q_F$ than the current DFA state $q_D(t)$ is eventually reached. 
%The NBA state $q_B^{\text{next}}$ is selected as follows. First, we compute the distance $d(q_B(t),q_F^{\text{feas}})$, where $q_F^{\text{feas}}$ is a final NBA state that is selected offline and is reachable from its initial state $q_B^0$ in the pruned NBA, i.e., $d(q_B^0,q_F^{\text{feas}})\neq\infty$. Then, we select as $q_B^{\text{next}}$ a state that satisfies $d(q_B^{\text{next}},q_F^{\text{feas}}) < d(q_B(t),q_F^{\text{feas}})$,
%\begin{equation}\label{eq:targetDFA}
%   d(q_D^{\text{next}},q_F) = d(q_D(t),q_F) -1, 
%\end{equation}
%i.e., a state that is one hop closer to $q_F^{\text{feas}}$ than $q_B(t)$ is. If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}]. %; see  Sections \ref{sec:paths}. %or realize that a transition from $q_D(t)$ to $q_D^{\text{next}}$ is in fact infeasible; see next section.


%{\bf{Local Construction of Robot Paths:}}

To reach $q_B^{\text{next}}\in\ccalQ_{q_B(t)}^{\text{next}}$ the robots need to eventually generate a symbol from the set $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$; this symbol can be selected randomly. By construction of this symbol, we have that once the robots reach $q_B^{\text{next}}$ they will be able to stay in it as long as they keep generating this symbol; see \eqref{eq:b}.  %Among all such symbols $\sigma^{\text{next}}$, we select the one that yields the smallest set $\ccalN^{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
With slight abuse of notation, we denote the selected symbol by $\sigma^{\text{next}}$ [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. Also, for simplicity of notation we replace $b^{q_B(t),q_B^{\text{next}}}$ and $b^{q_B(t),q_B(t)}$ with $b^{\text{next}}$ and $b^{\text{inv}}$. The same simplification extends to all notation with the same superscripts.
%the corresponding set of robots $\ccalR^{q_B(t),q_B^{\text{next}}}$, $\ccalN^{q_B(t),q_B^{\text{next}}}$, $\ccalR^{q_B(t),q_B(t)}$, and $\ccalN^{q_B(t),q_B(t)}$.

%with $\ccalR^{\text{next}}$ and $\ccalN^{\text{next}}$.


In what follows, we discuss how to design robot paths $\bbp_{j,t:T_j}$, for all robots $j$, that should be followed within a time interval $[t,T_j]$ to ensure that eventually $\sigma^{\text{next}}$ is generated. Given $\sigma^{\text{next}}$, we compute for each robot $j\in\ccalN^{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma^{\text{next}}$. Recall that for robots $j\in\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma^{\text{next}}$  while for robots $j\in\ccalN^{\text{next}}\setminus\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%
Every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%the state $q_B^{\text{next}}$ will be eventually reached and once $q_B^{\text{next}}$ is reached the robots can remain in $q_B^{\text{next}}$ until new observations are made (i.e., until atomic predicates are satisfied/violated). 
%
%For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b^{\text{inv}}$ and $b^{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.
%
%Given the NBA state $q_B^{\text{next}}$, our goal is to design paths $\bbp_{j,t:T_j}$, for all robots $j$ that should be followed within a time interval $[t,T_j]$ so that the NBA transition from $q_B(t)$ to $q_B^{\text{next}}$ is activated. %%\footnote{With slight abuse of notation the subscript in $\bbp_{j,t:T_j}$ denotes the index of robot and the time interval $[t,T_j]$ within which the path should be followed.} 
%To achieve that, it suffices to ensure that the robots follow paths that (i) satisfy the Boolean formula $b^{q_B(t),q_B(t)}$ that allows them to stay in the current NBA state $q_B(t)$, until (ii) the Boolean formula $b^{q_B(t),q_B^{\text{next}}}$ that enables transition from $q_B(t)$ to $q_B^{\text{next}}$ is satisfied while (iii) while never satisfying Boolean formulas $b^{q_B(t),q_B''}$ other than the ones that are satisfied at time $t$.\footnote{At time $t$, the Boolean formula $b^{q_B(t),q_B(t)}$ is satisfied by construction of the pruned automaton. Nevertheless, other Boolean formulas $b^{q_B(t),q_B''}$ may be satisfied as well due to the non-deterministic nature of the NBA.}  For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b^{\text{inv}}$ and $b^{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.
%
%\red{[add reference to lines of the algorithm]}
%To design paths $\bbp_{j,t:T_j}$, \textit{first} the robots $j\in\ccalN^{\text{next}}$ \textit{communicate} to select a symbol $\sigma^{\text{next}}$ that satisfies conditions (i)-(ii) of Definition \ref{def:feas} given the current symbol  $\sigma^{\text{inv}}=L(\bbp(t))$ they are generating. %; see also Example \ref{ex3}. Note that such a symbol exists by construction of the pruned NBA for any symbol $\sigma^{\text{inv}}$. 
%%% \footnote{Note that it is possible that given the symbol that the robots generated to reach $q_D$ there may not exist a pair of symbols $\sigma^{\text{inv}}$ and $\sigma^{\text{next}}$ to reach a state $q_D^{\text{next}}$ that satisfy condition (iii) of Def. \ref{def:feas}. In other words, transition from $q_D$ to $q_D^{\text{next}}$ may not be cast as a point-to-point navigation problem as in \eqref{eq:localProb}.
%Consider e.g., the DFA that corresponds to $\phi=\square(\pi_1^{\ell_0}\vee\pi_2^{\ell_0})\wedge\Diamond(\pi_1^{\ell_1})\wedge\Diamond(\pi_2^{\ell_2})$. 
%Existence of such symbols is always guaranteed for a sub-class of co-safe LTL formulas as discussed in Lemma \ref{lem:cnt}.} %that satisfy $b^{\text{inv}}$ and $b^{\text{next}}$, respectively, i.e., $\sigma^{\text{next}}\models b^{\text{next}}$. This pair of symbols is selected so that condition (ii) of Definition \ref{def:feas} is satisfied; 
%Among all such symbols $\sigma^{\text{next}}$, we select the one that yields the smallest set $\ccalN^{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
%
%Given $\sigma^{\text{next}}$, we compute the set $\ccalR^{\text{next}}$ that collect the robots that need to move towards certain regions of interest $r_e$ in workspace to generate $\sigma^{\text{next}}$. 
%
%\textit{Second}, given $\sigma^{\text{next}}$,  we compute for each robot $j\in\ccalN^{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma^{\text{next}}$. Recall that for robots $j\in\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma^{\text{next}}$  while for robots $j\in\ccalN^{\text{next}}\setminus\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%\textit{Third}, we design the paths $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ for all robots $j\in\ccalN^{\text{next}}$. %First, all robots $j\notin\ccalR^{\text{inv}}$ stay put at their current locations until the state $q_B^{\text{next}}$ is reached. %
%\textit{Third}, every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%that if followed the symbol  $\sigma^{\text{next}}\models b^{\text{next}}$ is generated and the DFA state $q_D^{\text{next}}$ is reached
%In Section \ref{sec:complOpt}, we show that the multi-robot state $\bbp(t)$ already generates a symbol that satisfies $b^{\text{inv}}$. We also show that if (i) the robots that are involved in generating $\sigma^{\text{inv}}$, collected in a set $\ccalR^{\text{inv}}$, stay idle at their current locations $\bbp_j(t)$ and (ii) all other robots 
%
%
%\footnotesize
\begin{subequations}
\label{eq:localProb}
\begin{align}
%& \min_{\substack{T_j, \bbu_{j,t:T_j}}} \left[J(T_j,\bbu_{j,t:T_j}) = \int_{t'=t}^{T_j}  w(\bbp_j(t'),\bbu_j(t'))dt \right] \label{ObjLoc2}\\
& \text{Compute:~}{T_j, \bbu_{j,t:T_j}}~\text{such that}  \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ [L(\bbp_j(t'))=L(\bbp_j(t))] \vee [L(\bbp_j(t'))=\varnothing] \nonumber\\
%& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \vee [L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}],~\forall t'\in[t,T_j] \label{constrLoc1} \\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \cup_i\set{r_i}\setminus (R_j^t\cup L_j^{\text{next}}), \forall t'\in[t,T_j] \label{constrLoc1}\\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \hat{O}(t), \forall t'\in[t,T_j] \label{constrLocObs}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j) \in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin \ccalA_j^{\text{avoid}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
\end{align}
\end{subequations}
%\normalsize

\noindent In \eqref{constrLoc1}, $R_j^t$ denotes the region that robot $j$ lies in at time $t$. The first constraint \eqref{constrLoc1} requires that robot $j$ should not visit any region $r_i$ excluding $R_j^t$ and the target region $L_j^{\text{next}}$, for all $t'\in[t,T_j]$. If at time $t$ robot $j$ does not lie in any of the regions $r_i$, then $R_j^t=\emptyset$. This ensures that the multi-robot system can always remain in $q_B(t)$ as the robots $j\in\ccalN^{\text{next}}$ navigate the workspace; see Lemma \ref{lem:binv}. This constraint can be relaxed by requiring  robot $j\in\ccalN^{\text{next}}$ to always avoid only regions that may result in violating $b^{\text{inv}}$. For instance, if $b^{\text{next}}=\neg(\pi_j^{r_e}\wedge\pi_i^{r_e}$), then it suffices to require robot $j$ to never visit $r_e$.  %\footnote{$T_j^{-}$ denotes a time instant right before $T_j$, i.e., $T_j^{-}=T_j-\epsilon$, for an arbitrarily small $\epsilon>0$.} 
Similarly, the second constraint in \eqref{constrLocObs} requires robot $j$ to avoid all obstacles, collected in $\hat{O}(t)$, that are known up to the time instant $t$. The third constraint in \eqref{constrLoc2} requires robot $j$ to be in region $L_j^{\text{next}}$ at a time instant $T_j\geq t$. %so that it generates $L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}$.%\footnote{Note that this prevents the robot from visiting parts of $L_j^{\text{next}}$ that are shared with other regions $r_i$.} 
This is required to eventually generate the symbol $\sigma^{\text{next}}$. The last constraint in \eqref{constrLoc3} captures the robot dynamics. Note that among all paths that satisfy these constraints, the optimal one, as a per a user-specified motion cost function, can be selected. 
%\textit{Third}, every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%In words, the optimal control problem \eqref{eq:localProb} requires robot $j$ to design a path $\bbp_{j,t:T_j}$ that reaches $L_j^{\text{next}}$ (see \eqref{constrLoc2}) while avoiding certain regions $r_i$ (see \eqref{constrLoc1}) and all detected obstacles denoted by $\hat{O}(t)$ (see \eqref{constrLocObs}). %Note that the robots that do not belong to $\ccalR^{\text{inv}}$ and also are not responsible to generate $\sigma^{\text{next}}$ do not have a target region $L_{j}^{\text{next}}$. These robots remain stationary in their current locations and they do not need to solve \eqref{eq:localProb}.
%
Observe that \eqref{eq:localProb} is a local reachability problem, and, therefore, existing point-to-point navigation algorithms can be used to solve it, e.g., \cite{karaman2011sampling}. Finally observe that given $L_j^{\text{next}}$, robot $j$ locally solves \eqref{eq:localProb} without communicating with any other robot. %Also, since the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable as per Definition \ref{def:feas}, there are no conflicts where a robot would have to stay idle at its current location and at the same time move towards a new location as per the solution to \eqref{eq:localProb}; see also Lemma \ref{lem:binv}. %there is no robot $j$ that belongs to $\ccalR^{\text{inv}}$ that is required to stay idle
%
%Correctness of Alg. \ref{alg:RRT} is discussed in Sec. \ref{sec:complOpt}. %Feasibility of such this problem is examined in 

%We design such paths in two stages. In the first stage, we design subpaths $\bbp_{j,t:\bar{T}_j}$ for some $t<\bar{T}_j<T$ and in the second stage we design paths $\bbp_{j,\bar{T}_j:T_j}$. In particular, \textit{in the first stage} all robots that are involved in generating $\sigma^{\text{inv}}$, collected in a set $\ccalR^{\text{inv}}$, and all other robots $j$ for which it hold $L(\bbp_j(t))=\varnothing$ (i.e., they are outside of all regions $r_i$) stay idle at their current locations $\bbp_j(t)$, i.e., $\bar{T}_j=t+1$ and $\bbp_{j,t:\bar{T}_j}=[\bbp_j(t),\bbp_j(t)]$ All other robots $j$ (i.e., the ones that satisfy $j\notin\ccalR^{\text{inv}}$ and $L(\bbp_j(t))\neq \varnothing$) solve the following optimal control problem to design paths $\bbp_{j,t:\bar{T}_j}$ that if followed then the robots will move outside the regions that they are currently located. %As it will bbe discusses in Section \ref{sec:exec}, these subpaths will be executed so that the robots will move outside their current regions simultaneously.

%\begin{subequations}
%\label{eq:localProb1}
%\begin{align}
%& \min_{\substack{\bar{T}_j, \bbu_{t:\bar{T}_j}}} \left[J(\bar{T}_j,\bbu_{t:\bar{T}_j}) = \sum_{t'=t}^{\bar{T}_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc1}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in R_j(t), \forall t\in\set{t,\dots,\bar{T}_j-1} \label{constrLoc1a} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in \ccalR_j^{\text{inv}}, \forall t\in\set{t,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(\bar{T}_j))=\varnothing \label{constrLoc2a}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   %\bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc2}
%\end{align}
%\end{subequations}
%where $R_j(t)$ denotes the region $r_i$ that robot $j$ lies in at time $t$. Observe that the first two constraints \eqref{constrLoc1a}-\eqref{constrLoc2a} require robot $j$ to move outside the region $\ccalR_j(t)$ where it is located at the time instant $t$. This happens at a time instant $\bar{T}_j$, i.e., $L(\bbp_j(\bar{T}_j))=\varnothing$. Note that robot $j$ locally solves \label{eq:localProb1} with communicating with other robots. Observe that execution of these subpaths ensures that the robots remain in the DFA state $q_D(t)$ since $b^{\text{inv}}$ is always satisfied as the robots $\ccalR^{\text{inv}}$ remain stationary in their current locations that generates  $\sigma^{\text{inv}}\models b^{\text{inv}}$.

%since the robots in $\ccalR^{\text{inv}}$

%In the \textit{second} stage, we construct the subpaths $\bbp_{j,\bar{T}_j:T_j}$ that will enable the transition from $q_D(t)$ to $q_D^{\text{next}}$. For robots $j\in\ccalR^{\text{inv}}$, we select $T_j=\bar{T}_j+1$ and $\bbp_{j,\bar{T}_j:T_j}=[\bbp_{j}(t),\bbp_{j}(t)]$, i.e., these robots still stay idle. In fact, due to the deterministic structure of the DFA, this ensures that the robots remain in the DFA state $q_D(t)$ until the symbol $\sigma^{\text{next}}$ is generated which will activate the transition towards $q_D^{\text{next}}$. To generate the symbol  $\sigma^{\text{next}}$, all other robots $j\notin\ccalR^{\text{inv}}$ design paths $\bbp_{j,\bar{T}_j:T_j}$ by solving the following optimal control problem:

%\begin{subequations}
%\label{eq:localProb}
%\begin{align}
%& \min_{\substack{T_j, \bbu_{\bar{T}_j:T_j}}} \left[J(T_j,\bbu_{\bar{T}_j:T_j}) = \sum_{t'=\bar{T}_j}^{T_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ L(\bbp_j(t'))=\varnothing, \forall t'\in\set{\bar{T}_j,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
%\end{align}
%\end{subequations}



 %This ensures that  transition to a DFA state $q_D'\neq q_D(t)$ that is not $q_D^{\text{next}}$. 
%In the meantime the robots in $\ccalR^{\text{inv}}$ ensure that the current DFA state remain the same in $[t,\bar{T}-1]$, since they stay idle and generate the symbol $\sigma^{\text{inv}}$. Also note that robots in $\ccalR^{\text{inv}}$ do not belong to the set of robots that need to move to another location to generate the symbol $\sigma$, since that would create a conflict; see also Remark \ref{rem:invariant}. 
%The second constraint in \eqref{constrLoc2} requires that at time instant $T_j$, all robots should be in their corresponding locations $L_j^\textbf{}$. Once this happens the symbol $\sigma^{\text{next}}$ is generated and the target DFA state is reached.
%
%Note that infeasibility of \eqref{eq:localProb} is due to the facts (i) the environment is unknown and, therefore, it is not possible to check offline which DFA transitions cannot be enabled because e.g., of the robot dynamics or the existence of obstacles.%; and (ii) the LTL formula $\phi$ is decomposed into local sub-tasks Problem \ref{prob} is solved in a distributed the proposed algorithm is distributed nature of the proposed 

%What if the problem is infeasible? update $\sigma$ i.e., $L_j$. If no other $L_j$. update target DFA state. If no other target DFA state report `current method failed (this does not mean that the task is unsatisfiable though)'

%\begin{ex}[Selection of $\sigma^{\text{next}}$ and $\sigma^{\text{inv}}$]\label{ex3}
%Consider the Boolean formulas $b^{\text{inv}}=\neg \pi_{\text{obs}}$ and $b^{\text{next}}=(\pi_j^{r_1}\vee \pi_j^{r_3} )\wedge\pi_e^{r_2}\wedge (\neg \pi_j^{r_2}) \wedge (\neg (\pi_j^{r_1}\wedge \pi_e^{r_1}))$, where the atomic predicate $\pi_{\text{obs}}$ is true of at least one robot hits an obstacle. A symbol $\sigma^{\text{next}}$ that satisfies $b^{\text{next}}$ is $\sigma^{\text{next}}=\pi_j^{r_1}\pi_e^{r_2}$ while $b^{\text{inv}}$ is satisfied by an empty string, i.e., $\sigma^{\text{inv}}=\varnothing$. Given this pair of symbols, we have that $\ccalR^{\text{inv}}=\emptyset$, $\ccalR^{\text{next}}=\set{j,e}$, $L_j^{\text{next}}=r_1$, and $L_e^{\text{next}}=r_2$.
%\end{ex}

%\begin{ex}[Construction of $\sigma^{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b^{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$. Then, we have that $\sigma^{\text{inv}}=\pi_j^{r_1}$ and $\ccalR^{\text{inv}}=\set{j}$. Similarly, if $b^{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma^{\text{inv}}$ is an empty string and $\ccalR^{\text{inv}}=\emptyset$.
%\end{ex}

%\begin{ex}
%--add automaton figure--and explain--
%\end{ex}
%\begin{rem}[Initialization of $q_B(t)$]
%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}
%\end{rem}
\subsection{Reacting to Map Uncertainty}\label{sec:replan}
%{\bf{Reactive Planning to Map Uncertainty:}}

As the robots follow their paths $\bbp_{j,t:T_j}$, the map $M(t)$ is continuously updated, as per \eqref{eq:updMap}, and the robot paths need to be accordingly revised [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. In fact, reactivity to the environment is required in two cases. First, as the robots follow their paths $\bbp_{j,t:T_j}$, they may discover new obstacles based on their sensor measurements; see \eqref{eq:sensor}. If the discovered obstacles intersect with their paths $\bbp_{j,t:T_j}$, for some $j\in\ccalR^{\text{next}}$, then these robots $j$ locally re-solve \eqref{eq:localProb} using the updated map to design new paths. Note that existing reactive planning algorithms that can address reachability navigation problems in the presence of unknown obstacles can also be used to solve \eqref{eq:localProb}; see e.g., \cite{karaman2011sampling,guzzi2013human,otte2016rrtx,bansal2019combining,ryll2019efficient,elhafsi2019map,zhai2019path,tordesillas2020faster}.

%is not reachable e.g., due to the robot dynamics or 
Second, as the the map $M(t)$ is constructed, goal regions $L_j^{\text{next}}$ may become unreachable because of the structure of the environment (e.g., regions of interest may be surrounded by obstacles). In this case, robots $j$ that cannot reach $L_j^{\text{next}}$ communicate with all other robots so that a new symbol $\sigma^{\text{next}}$ is selected. This process is repeated until a reachable region $L_j^{\text{next}}$ is selected.  %that makes \eqref{eq:localProb} feasible. 
If such a symbol $\sigma^{\text{next}}$ does not exist, then this means that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$, due to the a-priori unknown structure of the environment. Then, the graph $\ccalG$ is updated by removing this transition and a new NBA state $q_B^{\text{next}}$ is selected. If there do not exist any candidate NBA states to be selected as $q_B^{\text{next}}$, then the assigned task cannot be accomplished given the current multi-robot and NBA state. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
In fact, there may exist another sequence of NBA states for which Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible (i.e., paths towards selected goal regions always exist) and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.

%\begin{rem}[Feasibility of \eqref{eq:localProb}]
%Observe that \eqref{eq:localProb} may be \textit{infeasible}. This can be the case e.g., if the region $L_j^{\text{next}}$ is not reachable e.g., due to the robot dynamics or the structure of the environment. In this case, robot $j$ needs to communicate with all other robots so that a new symbol $\sigma^{\text{next}}$ is selected. This process is repeated until regions $L_j^{\text{next}}$ are selected that make \eqref{eq:localProb} feasible. If such a symbol $\sigma^{\text{next}}$ does not exist, then this means that the transition from $q_D(t)$ to $q_D^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$. Then, the pruned DFA is updated by removing this transition. Next, a new target DFA state is selected that is closer to the final state $q_F$ than $q_D(t)$ is. If there do not exist such DFA states then the robots cannot accomplish the assigned task. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
%In fact, there may exist another sequence of DFA states for which  Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
%Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.
%\end{rem}

%{\bf{Asynchronous Execution of Paths:}} 
\subsection{Asynchronous Execution of Paths}\label{sec:exec}
The robots $j\in\ccalR^{\text{next}}$ follow their paths $\bbp_{j,t:T_j}$ to eventually reach their goal regions $L_j^{\text{next}}$. By construction of these paths, the robots may not arrive at the same discrete time instant at their goal regions. To account for this, when a robot $j$ has traversed its path and has reached its goal region, it waits until
all other robots $e\in\ccalR^{\text{next}}$ reach their respective goal regions $L_e^{\text{next}}$ as well [line \ref{rrt:wait}, Alg. \ref{alg:RRT}]. When this happens, the symbol $\sigma^{\text{next}}$ is generated and the NBA state $q_B^{\text{next}}$ is reached as it will be shown in Section \ref{sec:complOpt}. Then a new NBA state is selected [lines \ref{rrt:nowait}-\ref{rrt:updN}, Alg. \ref{alg:RRT}]. This process is repeated indefinitely so that a final state is reached infinitely often [line \ref{rrt:sat}, Alg. \ref{alg:RRT}]. Note also that the robots can execute their paths asynchronously in the sense that the (continuous) time required to move from $\bbp_j(t)$ to $\bbp_j(t+1)$ may differ across the robots; see Sec. \ref{sec:complOpt}.

%transition  the paths can be executed since the robots are allowed to not arrive at the same discrete-time instant at their goal locations, 



%\textit{asynchronously}, i.e., the robots do not need to reach their goal regions at the same (continuous) time instant [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. In fact, when a robot $j$ has traversed its  path and has reached its goal region $L_j^{\text{next}}$, it has to wait until all other robots $e\in\ccalR^{\text{next}}$ reach their respective goal regions $L_e^{\text{next}}$ [line \ref{rrt:wait}, Alg. \ref{alg:RRT}]. When this happens, the symbol $\sigma^{\text{next}}$ is generated and the NBA state $q_B^{\text{next}}$ is reached as it will be shown in Section \ref{sec:complOpt}. Then a new NBA state is selected [lines \ref{rrt:nowait}-\ref{rrt:updN}, Alg. \ref{alg:RRT}]. This process is repeated indefinitely so that a final state is reached infinitely often [line \ref{rrt:sat}, Alg. \ref{alg:RRT}].

%The robots $j\in\ccalR^{\text{next}}$ execute their paths $\bbp_{j,t:T_j}$ \textit{asynchronously}, i.e., the robots do not need to reach their goal regions at the same (continuous) time instant [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. In fact, when a robot $j$ has traversed its  path and has reached its goal region $L_j^{\text{next}}$, it has to wait until all other robots $e\in\ccalR^{\text{next}}$ reach their respective goal regions $L_e^{\text{next}}$ [line \ref{rrt:wait}, Alg. \ref{alg:RRT}]. When this happens, the symbol $\sigma^{\text{next}}$ is generated and the NBA state $q_B^{\text{next}}$ is reached as it will be shown in Section \ref{sec:complOpt}. Then a new NBA state is selected [lines \ref{rrt:nowait}-\ref{rrt:updN}, Alg. \ref{alg:RRT}]. This process is repeated indefinitely so that a final state is reached infinitely often [line \ref{rrt:sat}, Alg. \ref{alg:RRT}].
%In Section \ref{sec:complOpt}, we show the robots remain in the NBA state $q_B(t)$ for all  $t'\in [t, T-1]$ and transition to $q_B^{\text{next}}$ occurs at the time instant $T$. Once this happens, the robots update their current DFA state and select the next DFA state [lines \ref{rrt:T}-\ref{rrt:UpdGoals}]. This process is repeated until the final state $q_F$ is reached.

%
%\begin{rem}\label{rem:invariant}
%Note that once the robots reach a new DFA $q_D$, they satisfy its respective Boolean condition $b^{\text{inv}}$, since the `next' temporal operator is excluded from the task specification. Particularly, if $b^{\text{inv}}$ is not satisfied this implies that once the robots are at locations that generate a symbol that triggers the transition to $q_D$, the robots should immediately leave their locations, which is impossible to specify unless the next operator is included in the specification language. 

%Recall that $\sigma^{\text{inv}}$ is selected to have the minimum length, this means that the minimum number of robots are involved to generate it. Therefore, robots that are required to generate the symbol $\sigma$ are not included in the set $\ccalR^{\text{inv}}$; see also Remark \ref{rem:invariant}.
%Similarly, robots that are responsible to satisfy $b^{\text{next}}$ cannot be responsible for generating the symbol $\sigma^{\text{inv}}$, since the next operator does not exist and all regions are assumed to be disjoint. %(unless there is an overlap..)
%\end{rem}


%\subsection{Online Re-planning}\label{sec:replan}






\begin{rem}[Communication]
%Note that Algorithm \ref{alg:RRT} requires all-time communication to ensure that all robots always have access to the same map $M(t)$. Nevertheless, this requirement can be straightforwardly relaxed by allowing each robot to build their local map $M_j(t)$. Moreover, 
Execution of the paths $\bbp_{j,t:T_j}$ does not require all-time communication among robots, which is typically the case in relevant temporal logic algorithms. Instead, communication is intermittent and is required only in the following two cases: (i) all robots need to communicate with each other to select and update the symbol $\sigma^{\text{next}}$ (ii) every robot $j\in\ccalR^{\text{next}}$ needs to send a message to all other robots in $\ccalR^{\text{next}}$ once it has reached region $L_{j}^{\text{next}}$. %; see Section \ref{sec:exec}.
\end{rem}

%Next, we define the set $\ccalL_j$ that collects all robot positions $\bbp_j$ that violate $b^{\text{inv}}$ regardless of the state of all other robots. For instance, if $b^{\text{inv}}=\neg (\pi_j^{r_e}\wedge \pi_z^{r_h})$, then $\ccalL_j=\emptyset$. On the other hand, if $b^{\text{inv}}=\neg (\pi_j^{r_e})\wedge (\neg \pi_z^{r_h})$ then  $\ccalL_j=\set{r_e}$. Formally, to construct the set, we express the negation of $b^{\text{inv}}$, denoted by $\bar{b}^{\text{inv}}=\neg b^{\text{inv}}$ as


\begin{rem}[Conservativeness]\label{rem:conserv}
Recall that once the robots reach a state $q_B(t)\in\ccalV$ a new state $q_B^{\text{next}}\in\ccalV$ is selected to be reached next.
%
This state is selected from the set $\ccalQ_{q_B(t)}^{\text{next}}\subseteq\ccalV$ that collects all states $q_B^{\text{next}}$ for which the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable, as per Definition \ref{def:feas}, and therefore, this transition can be enabled by solving local reachability tasks as per \eqref{eq:localProb}. Note that there may be states that can be reached from $q_B(t)$ but not in a local-reachability fashion according to Definition \ref{def:feas}; see e.g., Figure \ref{fig:conserv}. As a result, such states are not included in the set $\ccalQ_{q_B(t)}^{\text{next}}$ and, therefore, a solution to Problem \ref{prob} may not be found even if it exists. 
%
\end{rem}
%In Section \ref{sec:complOpt}, we show that there exists a fragment of LTL so that if Definition \ref{def:feas} is not satisfied for a transition $\delta_B^m(q_B,\cdot,q_B')$, then transition from $q_B$ to $q_B'$ is impossible to activate as it requires robots to instantaneously jump from one region of interest to another one. 

%Definition \ref{def:feas} is conservative %Particularly, there may exist (feasible) symbols $\sigma^{q_B,q_B'}$ that satisfy \eqref{eq:b} but they do not satisfy Definition \ref{def:feas}; see e.g., Figure \ref{fig:conserv}. 
%in the sense that if is not satisfied then transition from $q_B$ to $q_B'$ may be either possible but not in a local-reachability fashion (see Figure \ref{fig:conserv}) or impossible as it may require robots to jump from one region of interest to another one (see Figure \ref{fig:NBA1}). Conditions under which Definition \ref{def:feas} is not conservative are discussed in Section \ref{sec:complOpt}. Specifically, we show that there exists a fragment of LTL so that if Definition \ref{def:feas} is not satisfied then transition from $q_B$ to $q_B'$ is impossible to activate as it requires robots to instantaneously jump from one region of interest to another one.
%Nevertheless, conservative pruning ensures that when the robots reach a state $q_D$, they will always be able to make progress towards accomplishing their task (i.e., reach a new state $q_D'$) regardless of the symbols they have generated to reach $q_D$ by solving local point-to-point navigation problems. A fragment of LTL for which the proposed approach is not conservative is discussed in Section \ref{sec:complOpt}.

==> files/alg_Mar31_2020.tex <==
%
In this section, we provide an algorithm to decompose an LTL task into reachability tasks. This process occurs offline i.e., before deploying the robots in the unknown environment. Specifically, in Section \ref{sec:nba} we translate the LTL formula into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA). In Section \ref{sec:prune} we prune this automaton by removing infeasible transitions i.e., transitions that are activated if a robot is present in more than one location simultaneously. Then, in Section \ref{sec:dec} we provide conditions under which feasible NBA transitions can be enabled by solving local reachability tasks. Such transitions are called decomposable. Using the definition of feasible and decomposable transitions, in Section \ref{sec:dist} we define a distance metric over the NBA that measures how far the robots are from fulfilling the assigned mission. This metric will be used in Section \ref{sec:planning} to guide and adapt planning to the continuously learned map of the environment.


\subsection{From LTL formulas to Automata}\label{sec:nba}

First, we translate the specification $\phi$, constructed using a set of atomic predicates $\mathcal{AP}$, into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA), defined as follows \cite{baier2008principles} [line \ref{rrt:dfa}, Alg. \ref{alg:RRT}]. %Given a temporal logic formula $\phi$ , with syntax and semantics as described in Definitions \ref{syntax} and \ref{semantics}, respectively, a DFA is defined as follows:

\begin{definition}[NBA]
A Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\rightarrow_B, \ccalQ_F\right)$, where (i) $\ccalQ_{B}$ is the set of states;
(ii) $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is the initial state; (iii) $\delta_B:\ccalQ_B\times\Sigma\rightarrow\ccalQ_B$ is a non-deterministic transition relation, and $\ccalQ_F\subseteq\ccalQ_{B}$ is a set of accepting/final state. 
\end{definition}

To interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times M(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current multi-robot state $\bbp(t)\in\mathbb{R}^{n\times N}$ and the current map $M(t)$ of the environment. An infinite-length discrete plan $\tau=\bbp(0)\bbp(1)\dots$ satisfies $\phi$, denoted by $\tau\models\phi$, if the word $\sigma=L(\bbp(0), M(0))L(\bbp(1),M(1))\dots$ yields an accepting NBA run defined as follows. First, a run of $\rho_B$ of $B$ over an infinite word $\sigma=\sigma(1)\sigma(2)\dots\sigma(t)\dots\in(2^{\mathcal{AP}})^{\omega}$, is a sequence $\rho_B=q_B(0)q_B(1)q_B(2)\dots,q_B(t),\dots$, where $q_B(0)\in\ccalQ_B^0$ and $\delta_B(q_B(t),\sigma(t),q_B(t+1)$, $\forall t\in\mathbb{N}$. %Hereafter, we equivalently denote $\delta_B(q_B(t),\sigma(t),q_B(t+1)$ as $q_B(t)\rightarrow_B q_B(t+1)$.
A run $\rho_B$ is called \textit{accepting} if $\texttt{Inf}(\rho_B)\cap\ccalQ_F\neq\emptyset$, where $\texttt{Inf}(\rho_B)$ represents the set of states that appear infinitely often in $\rho_B$. In words, an infinite-length discrete plan $\tau$ satisfies an LTL formula $\phi$ if it can generate at least one accepting NBA run. Hereafter, for simplicity we replace $L(\bbp(t),M(t))$ with $L(\bbp(t))$.
%The symbols $\sigma$ that result in an accepting run of $D$ constitute the accepted language of $D$.

%The proposed reactive algorithm builds online (i.e., as the robots navigate the environment) paths that live in the infinite-dimensional space $\Omega^N\times\ccalQ_D$. The synthesized paths are updated as the map of the environment is updated. 

%Specifically, let $q_B(t)\in\ccalQ_B$ denote the NBA state that the multi-robot system has reached at time $t$ given all observations that have been made (i.e., all atomic predicates that have been satisfied) until $t$, where $q_B(0)\in\ccalQ_B^0$ [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. 

%In Section \ref{sec:planning}, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task. Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task. To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that (i) it is  one-hop reachable from $q_B(t)$, (ii) the transition from $q_B(t)$ to $q_B^{\text{next}}$ is feasible, i.e., observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously, and (iii) $q_B^{\text{next}}$ is `closer' to the final states than $q_B(t)$ is. %Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. 
%In what follows, we describe these steps in detail.
%In Section \ref{sec:prune} we define when an NBA transition is feasible and when it is decomposable i.e., it can be enabled via solving local reachability-avoidance problems. In Section \ref{sec:dist}, we define a distance metric over the NBA that measures how far each NBA state is from the set of final states.

%Next, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task; see Algorithm \ref{alg:RRT}. Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task. To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that it is (i) one-hop reachable from $q_B(t)$, (ii) `closer' to the final states than $q_B(t)$ is according to a distance function defined over the NBA, and (iii) observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously. Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. In what follows, we describe these steps in detail.


%Once this transition is enabled, the robots update the target DFA state $q_D^{\text{next}}$ until they reach a final DFA state.%\footnote{In case the DFA has more than one initial state, then there is more than one state $\bbq(0)$ that can be used as a root. In this case, a separate tree is build for each one of possible roots.}
%For this, we assume that the initial robot configuration allows the robots to stay in $q_B(0)$.
%

%By convention the cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = 0$, while the cost of a node $\bbq(t+1)=[\bbp(t+1), q_D]\in\ccalV$, given its parent node $\bbq(t)=[\bbp(t),q_D']\in\ccalV$, is computed as 
%\begin{equation}\label{eq:costUpd}
%J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq(t)) +  w(\bbp(t),\bbp(t+1)).
%\end{equation}
%Observe that by applying \eqref{eq:costUpd} recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:Prob2}.

 
%Given the current DFA state $q_D(t)$, the robots first select a DFA state $q_D^{\text{next}}\in\ccalQ_D$ that is `closer' to the final state $q_F$ than $q_D(t)$ is and observations that generate a transition from $q_D(t)$ to $q_D^{\text{next}}$ can be generated. Therefore,
%\subsection{Selecting the Next DFA State}\label{sec:targetDFA}

%{\bf{Pruning the DFA:}}
\subsection{Pruning Infeasible NBA Transitions}\label{sec:prune}
%Given the current NBA state $q_B(t)$, a new state $q_B^{\text{next}}$ is selected so that it is closer to the final states. Thus, to select $q_B^{\text{next}}$, we need to define a distance function over the state-space of the NBA that measures how far each state is from the final state. %(in terms of the number feasible transitions/hops required to reach $q_F$). 
%To achieve that, we first prune the NBA $B$ by removing transitions that cannot be enabled [line \ref{rrt:prune}, Alg. \ref{alg:RRT}]. %This is required to define a distance function over the state-space of the DFA. %
%
%Specifically, the pruned NBA is constructed by removing all infeasible NBA transitions. 
In what follows, we define the \textit{feasible/infeasible} NBA transitions $\delta_B(q_B,\cdot,q_B')$. Transitions that are infeasible are removed giving rise to a pruned automaton. To formally define the \textit{feasible} NBA transitions we first need to introduce the following definitions. %\cite{kantaros2018text}.
%
%We also rewrite $b^{\text{inv}}^{q_D}$ and $b^{\text{next}}^{q_D,q_D'}$ as follows:
%\begin{equation}\label{eq:eq1}
%    b^{\text{inv}}^{q_D} = b^{\text{inv}}^{\text{goal}} \triangle (\neg b^{\text{inv}}^{\text{avoid}} ),
%\end{equation}

%\begin{equation}\label{eq:eq2}
%    b^{\text{next}}^{q_D,q_D'} = b^{\text{next}}^{\text{goal}} \triangle (\neg b^{\text{next}}^{\text{avoid}} ),
%\end{equation}
%where in the Boolean formulas  $b^{\text{next}}^{\text{goal}}$, $b^{\text{next}}^{\text{avoid}}$, $b^{\text{inv}}^{\text{goal}}$ and $b^{\text{inv}}^{\text{avoid}}$ the negation operator does not appear in front of any atomic proposition. Also, in \eqref{eq:eq1} and \eqref{eq:eq2}, $\triangle$ denotes either the logical AND ($\wedge$) or the logical OR $(\vee)$ operator.

% defined in \ref{defn:wTS}.%\footnote{Recall from Definition \ref{defn:wTS} that $\text{wTS}_i$ is defined over $\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma_i=2^{\mathcal{AP}_i}$. Also, recall from Definition \ref{def:pts} that the PTS is defined over $\mathcal{AP}=\bigcup_{i=1}^N\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma=2^{\mathcal{AP}}$. Also, throughout the paper, we denote the finite symbols by $\sigma^*\in\Sigma$ and the infinite symbols by $\sigma\in\Sigma^{\omega}$.}
\begin{definition}[Feasible symbols $\sigma_j\in\Sigma_j$]\label{defn:infTSi}
A symbol $\sigma_j\in\Sigma_j:=2^{\mathcal{AP}_j}$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, where $b_j^{\text{inf}}$ is a Boolean formula defined as 
\begin{equation}\label{bInfTSi}
b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e}(\pi_j^{r_i}\wedge\pi_j^{r_e})).
%b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e})),
\end{equation}
where $b_j^{\text{inf}}$ requires robot $j$ to be present simultaneously in more than one disjoint region.
\end{definition}

%We also need to define when a symbol $\sigma\in\Sigma$ is \textit{feasible}, i.e., when it can be generated by the multi-robot system. To this end, we first need to define the
%In other symbols $\sigma_j\in\Sigma_j=2^{\mathcal{AP}_j}$ that are feasible, i.e, the symbols that can be generated by robot $j$ \cite{kantaros2018text}. 


Note that the Boolean formula $b_j^{\text{inf}}$ is satisfied by any finite symbol $\sigma_j\in\Sigma_j$ that requires robot $j$ to be present in two or more disjoint regions, simultaneously. For instance, the symbol $\sigma_j=\pi_j^{r_i}\pi_j^{r_e}$ satisfies $b_j^{\text{inf}}$ if $r_i$ and $r_e$ are disjoint regions. %\footnote{Note that if we consider regions $r_i$ that are not necessarily disjoint, then the Boolean formula $b_j^{\text{inf}}$ is defined as $b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e}))$. Note also that definition of infeasible symbols depends on the problem at hand, i.e, the definition of atomic propositions included in the sets $\mathcal{AP}_j$.} % if there is an overlap between regions $r_i$ and $r_e$. 
Next, we define the feasible symbols $\sigma\in\Sigma$.

\begin{definition}[Feasible symbols $\sigma\in\Sigma$]\label{defn:infPTS}
A symbol $\sigma\in\Sigma$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, for all robots $j$,
where $\sigma_j=\Pi|_{\Sigma_j}\sigma$, $b_j^{\text{inf}}$ is defined in \eqref{bInfTSi}, and $\Pi|_{\Sigma_j}\sigma$ stands for the projection of the symbol $\sigma$ onto $\Sigma_j$.\footnote{For instance, $\Pi|_{\Sigma_j}(\pi_j^{r_e}\pi_m^{r_h})=\pi_j^{r_e}$.} We denote by $\Sigma_{\text{feas}}\subseteq\Sigma$ the set of all feasible symbols $\sigma\in\Sigma$. 
\end{definition}


%%%
%%%
%Next, we define the $\Sigma(q_D)=\{s\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D)\in\rightarrow_D)\}$ that collects all symbols that the robots can generate to remain in the state $q_D$. We also define the set $\Sigma(q_D,q_D')=\{\sigma\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D')\in\rightarrow_D)\}$ that collects all symbols that enable a transition from $q_D$ to $q_D'$.
%
%Moreover, for each state $q_D$, we define the set $\Sigma(q_D|p)$ that collects all symbols $\sigma$ that robots may observe if they reach $q_D$ through a path $p=q_D^0,\dots,q_D$, i.e., a sequence of states in $\ccalQ_D$ that starts at the initial state $q_D^0$ and ends at the state $q_D$. Note that there may be multiple paths that can reach $q_D$ from $q_D^0$ and, therefore, each state $q_D$ may be associated with more than one set $\Sigma(q_D|p)$. For the initial state, $q_D^0$, there is only one such set  defined as $\Sigma(q_D^0|p)=\Sigma(q_D^0)$, since in a DFA the only path $p$ to reach $q_D^0$ from $q_D^0$ is the self-loop of $q_D^0$.

%To prune the DFA we need first to construct the sets $\Sigma(q_D|p)$. Starting from $q_D^{0}$, we execute the following process for each state $q_D$ that is reachable within one hop from $q_D^0$

%First, we select a state $q_D\in\ccalQ_D$, for which all corresponding sets $\Sigma(q_D|p)$ have been constructed
%%%
%%%
%\red{unclear here..}
%To solve Problem \ref{prob}, we first decompose the assigned task into local point-to-point planning problems. Motion plans that solve these point-to-point navigation problems are locally designed online while adapting to the map of the environment that is built by the robots. The proposed algorithm is summarized in Algorithm \ref{alg:RRT}. 
%


%\begin{algorithm}[t]
%%\footnotesize
%\caption{Pruning a NBA}
%\LinesNumbered
%\label{alg:prune}
%\KwIn{NBA}
%\KwOut{Pruned NBA}
%Remove infeasible transitions (see Definition \ref{def:feas1})\label{prune:inf}\;
%Add auxiliary states and transitions\label{prune:aux}\;
%Initialize $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$, $\ccalQ_B^\text{checked}=\emptyset$, $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$\;\label{prune:init}
%Compute $\ccalQ_{q_B}^{\text{next}}$ for all $q_B\in\ccalQ_B^\text{loop}$\;
%\While{$|\ccalQ_B^{\text{not-checked}}|\neq\emptyset$}{
%    \For{$q_B\in\ccalQ_B^{\text{not-checked}}$}{
%        Compute $\ccalQ_{q_B}^{\text{next}}$\;\label{prune:nextS}
%        \For{$q_B^K\in\ccalQ_{q_B}^{\text{next}}$}{\label{prune:FornextS}
%            Replicate transition $\delta_B^K(q_B,q_B^K)$\;\label{prune:repl}
%            \If{$\delta_B^K(q_B,q_B^K)$ is decomposable (Def. \ref{def:feas})}{
%                $\ccalQ_{B}^{\text{loop}}=\ccalQ_{B}^{\text{loop}}\cup\{q_B^K\}$\;\label{prune:UpdLoop} 
%            }
%            \Else{
%                Remove transition $\delta_B^K(q_B,\cdot,q_B^K)$ from the NBA and the set $\ccalP_{q_B}^{\text{next}}$\;\label{prune:remNonDec}
%            }
%        }
%        One-hop transitions $\delta_B(q_B,\cdot,q_B')$ that are not part of any run in $\ccalP_{q_B}^{\text{next}}$ are removed\;\label{prune:prune2}
%    }
%    $\ccalQ_{B}^{\text{checked}}=\ccalQ_{B}^{\text{not-checked}}$\;
%    $\ccalQ_{B}^{\text{not-checked}}=\ccalQ_{B}^{\text{loop}}\setminus\ccalQ_{B}^{\text{checked}}$\;
%}
%%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
%\end{algorithm}

\begin{algorithm}[t]
%\footnotesize
\caption{Computing Decomposable Transitions}
\LinesNumbered
\label{alg:prune}
\KwIn{Pruned NBA}
\KwOut{Sets $\ccalQ_{B}^{\text{loop}}$, $\ccalQ_{q_B}^{\text{next}}$, $\forall q_B\in\ccalQ_{B}^{\text{loop}}$}
%Remove infeasible transitions (see Definition \ref{def:feas1})\label{prune:inf}\;
Add auxiliary states and transitions\label{prune:aux}\;
Initialize $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$, $\ccalQ_B^\text{checked}=\emptyset$, $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$\;\label{prune:init}
Compute $\ccalQ_{q_B}^{\text{next}}$ for all $q_B\in\ccalQ_B^\text{loop}$\;
\While{$|\ccalQ_B^{\text{not-checked}}|\neq\emptyset$}{
    \For{$q_B\in\ccalQ_B^{\text{not-checked}}$}{
        $\ccalQ_{q_B}^{\text{next}}=\emptyset$\;\label{prune:initNext}
        Compute all runs \eqref{eq:run} starting from $q_B$\;\label{prune:run}
        \For{all runs}{\label{prune:FornextS}
            %Replicate transition $\delta_B^K(q_B,q_B^K)$\;\label{prune:repl}
            \If{$\delta_B^K(q_B,q_B^K)$ is decomposable (Def. \ref{def:feas})}{
                $\ccalQ_{B}^{\text{loop}}=\ccalQ_{B}^{\text{loop}}\cup\{q_B^K\}$\;\label{prune:UpdLoop1} 
                $\ccalQ_{q_B}^{\text{next}}=\ccalQ_{q_B}^{\text{next}}\cup\{q_B^K\}$\;\label{prune:UpdLoop2} 
            }
            %\Else{
             %   Remove transition $\delta_B^K(q_B,\cdot,q_B^K)$ from the NBA and the set $\ccalP_{q_B}^{\text{next}}$\;\label{prune:remNonDec}
            %}
        }
        %One-hop transitions $\delta_B(q_B,\cdot,q_B')$ that are not part of any run in $\ccalP_{q_B}^{\text{next}}$ are removed\;\label{prune:prune2}
    }
    $\ccalQ_{B}^{\text{checked}}=\ccalQ_{B}^{\text{not-checked}}$\;\label{prune:checked} 
    $\ccalQ_{B}^{\text{not-checked}}=\ccalQ_{B}^{\text{loop}}\setminus\ccalQ_{B}^{\text{checked}}$\;\label{prune:notchecked} 
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}





Next, we define the sets that collect all feasible symbols that enable a transition from an NBA state $q_B$ to another, not necessarily different, NBA state $q_B'$; see also Example \ref{ex:exFeasSets}. This definition relies on the fact that transition from a state $q_B$ to a state $q_B'$ is enabled if a Boolean formula, denoted by $b^{q_B,q_B'}$ and defined over the set of atomic predicates $\mathcal{AP}$, is satisfied.  %The set of all atomic predicates associated with robots $j\in\mathcal{N}_{q_B,q_B'}$ is defined by $\mathcal{AP}_{q_B,q_B'}=\bigcup_{j\in\mathcal{N}_{q_B,q_B'}}\mathcal{AP}_j$.

\begin{definition}[Sets of Feasible Symbols]
Let $\mathcal{AP}_{q_B,q_B'}$ be a set that collects all atomic predicates that appear in the Boolean formula $b^{q_B,q_B'}$ associated with an NBA transition $\delta_B(q_B,\cdot, q_B')$. Given $b^{q_B,q_B'}$, we define the set $\Sigma^{q_B,q_B'}\subseteq 2^{\mathcal{AP}_{q_B,q_B'}}$ 
that collects all symbols $\sigma$ that (i) satisfy the corresponding Boolean formula $b^{q_B,q_B'}$, i.e., $\sigma\models b^{q_B,q_B'}$; and (ii) $\sigma\in\Sigma_{\text{feas}}$. %; and (iii) are associated with robots that appear in $b^{q_B,q_B'}$. 
%If the empty symbol $\varnothing$ satisfies (i), then $\Sigma^{q_B,q_B'}=\set{\varnothing}$. 
%The set $\mathcal{AP}_{q_B,q_B'}$ collects all atomic predicates that appear in $b^{q_B,q_B'}$.
\label{defn:feasSet}
\end{definition}

%Moreover, let $b^{\text{inv}}^{q_D}$ denote the Boolean formula that needs to be satisfied to enable a loop around $q_D$, i.e., a transition from $q_D$ to $q_D$.\footnote{Note that $b^{\text{inv}}^{q_D}$ exists for all states $q_D$, since the `next' operator is excluded from the syntax. Also, the Boolean formulas that should be satisfied to enable a  transition from a state $q_D$ to $q_D'$ can be provided by tools that convert temporal logic formulas to automata.} Let also $\Sigma^{\text{inv}}^{q_D}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b^{\text{inv}}^{q_D}$. 
%
%Let also $b^{\text{next}}^{q_D,q_D'}$ denote the Boolean formula that needs to be satisfied to enable a transition from $q_D$ to $q_D'$ and $\Sigma^{\text{next}}^{q_D,q_D'}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b^{\text{next}}^{q_D,q_D'}$.
%Also, from $\Sigma_{\text{text}}^{q_D,q_D'}$, we exclude symbols associated with robots that do not play any role in satisfying $b^{\text{next}}^{q_D,q_D'}$. For instance, if $b^{\text{next}}^{q_D,q_D'}=\pi_j^{r_e}\vee\pi_j^{r_m}$, then $\Sigma_{\text{text}}^{q_D,q_D'}$ is defined as $\Sigma_{\text{text}}^{q_D,q_D'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$, i.e., it does not include any symbol associated with other robots $i\neq j$ that may also satisfy $b^{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_i^{r_f}$). The same also holds for $\Sigma^{\text{inv}}^{q_D}$; see also Example \ref{ex:feas}. %Additionally, in case the empty symbol, denoted by $\varnothing$ belongs to 
%

Given the sets $\Sigma^{q_B,q_B'}$, we define the infeasible NBA transitions defined as follows:

\begin{definition}[Infeasible NBA Transitions]\label{def:feas1}
A transition $\delta_B(q_B,\cdot,q_B')$ is infeasible if $\Sigma_{q_B,q_B'}=\emptyset$.
\end{definition}

In words, an NBA transition is infeasible if it is enabled only when at least one robot is present in more than one location in the environment simultaneously. All infeasible NBA transitions are pruned; see e.g., Figure \ref{fig:prune}. % line \ref{prune:inf}, Alg. \ref{alg:prune}]. 
%we remove all NBA transitions with $\Sigma_{q_B,q_B'}=\emptyset$, i.e., all transitions that are enabled if at least one robot is present in more than one location in the environment simultaneously [. 



%Next we remove NBA transitions that require robots to move from one region of interest $\ell_i$ to another one $\ell_e$ without visiting any location $\bbq$ in the environment outside $\ell_i$. Such transitions are considered infeasible as they require robots to `jump' from one region of interest to another one. For instance, consider the LTL formula $\phi=\pi_1^{r_1}\ccalU\pi_1^{r_2}$ that requires robot $1$ to be in region $r_1$ until it enters $r_2$. The corresponding NBA is illustrated in Figure \ref{fig:NBA1}. Assume that the initial condition of the robot satisfies $b^{q_B^0,q_B^0}=\pi_1^{r_1}$, i.e., that robot $1$ is initially located in $r_1$. Then the transition from the initial to the final state is considered infeasible as it requires the robot to `jump' from one region of interest to another one. 


\begin{figure}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Original NBA]{
    \label{fig:origNBA}
  \includegraphics[width=0.46\linewidth]{figures/feas1_bf.png}}
  \subfigure[Pruned NBA (Def. \ref{def:feas1})]{
    \label{fig:feas1}
  \includegraphics[width=0.38\linewidth]{figures/NBA2.png}}
%  \caption{FEASIBLE 1}
%  \label{fig:tow7}
%\end{figure}
%
%\begin{figure}[t]
%  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      %\subfigure[Replicating NBA states]{
    %\label{fig:repl}
 % \includegraphics[width=0.3\linewidth]{figures/NBA3.png}}
  \caption{Graphical illustration of Algorithm \ref{alg:prune} applied to the NBA corresponding to $\phi=\square\Diamond(\pi_1^{\ell_1})\wedge\square\Diamond(\pi_1^{\ell_2})$. This formula requires robot $1$ to visit infinitely often $\ell_1$ and $\ell_2$. Figure \ref{fig:origNBA} shows the original NBA where the states $q_B^0$ and $q_F$ correspond to the initial and final state of the NBA. The red dashed transitions are infeasible, as per Definition \ref{def:feas}, as they require robot $1$ to be in $\ell_1$ and $\ell_2$ simultaneously.  These transitions are removed  yielding the pruned NBA shown in Figure \ref{fig:feas1}. An auxiliary state $q_B^{\text{aux}}$ is added to the pruned NBA; see Figure \ref{fig:feas1}. Observe in Figure \ref{fig:feas1} that there are two runs in the form \eqref{eq:run} originating from $q_B$: $\rho_1=q_Bq_B$ and $\rho_2=q_B q_F q_B^0$. Note that the run $\rho=q_B q_F q_B$ cannot be generated as there is no feasible symbol that satisfies $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$. In fact, this run requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$ instantaneously. %Due to $\rho_2$, the intermediate state $q_F$ is replicated so that it has one incoming transition from $q_B$ and one outgoing transition to $q_B^0$; see Figure \ref{fig:repl}. The transition from $q_B$ to the original $q_F$ is removed. 
  Thus $\ccalQ_{q_B}^{\text{next}}={q_B,q_B^0}$. Similarly, for $q_B^0$ there are two runs in the form \eqref{eq:run}: $\rho_1=q_B^0q_B^0$ and $\rho_2=q_B^0 q_B$. The set $\ccalQ_{B}^{\text{loop}}$  constructed by alg. \ref{alg:prune} is $\ccalQ_{B}^{\text{loop}}=\{q_B^{\text{aux}},q_B^0,q_B\}$. 
  %
  %Observe in Figure \ref{fig:feas1} that there is no self-loop for the final state $q_F$. Thus, $q_F$ is replicated twice since it has one incoming and two outgoing transitions as shown in Figure \ref{fig:repl}. In Figure \ref{fig:repl} the multi-hop transition $q_B\rightarrow_B q_F\rightarrow_B q_B$ is removed since there are no symbols that satisfy $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$ (condition (i)-Defn. \ref{def:feas}); in fact this transition requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$. The resulting pruned NBA generated by Algorithm \ref{alg:prune} is shown in Figure \ref{fig:finalPrune}.  
  }
  \label{fig:prune}
\end{figure}

\begin{figure}
    \centering
     %\includegraphics[width=0.6\linewidth]{figures/p1Up2.png}
       \subfigure[Original NBA]{
    \label{fig:origNBAU}
  \includegraphics[width=0.45\linewidth]{figures/NBA1u.png}}
    \subfigure[Pruned NBA]{
    \label{fig:finalNBA2}
  \includegraphics[width=0.45\linewidth]{figures/NBAU.png}}
    %\subfigure[Pruned NBA]{
   % \label{fig:finalNBA3}
  %\includegraphics[width=0.3\linewidth]{figures/nba3u.png}}
    \caption{Effect of the initial robot state in computing decomposable transitions. Figure \ref{fig:origNBAU} depicts the NBA corresponding to $\phi=\pi_1^{\ell_1}\ccalU\pi_1^{\ell_2}$. All transitions are feasible as per Def. \ref{def:feas1}. Observe in Figure \ref{fig:finalNBA2} that if the initial robot state $\bbp(0)=\pi_1^{\ell_1}$, then $\ccalQ_{q_B^{\text{aux}}}^{\text{next}}=\{q_B^0,q_B^{\text{aux}}\}$ and $\ccalQ_{q_B^0}^{\text{next}}=\{q_B^0\}$. In other words, the transition from $q_B^0$ to $q_F$ (red dashed line) does not satisfy Def. \ref{def:feas} and therefore the final state $q_F$ is not reachable. In this case $\ccalQ_{B}^{\text{loop}}=\{q_B^{\text{aux}},q_B^0\}$. If $\bbp(0)=\pi_1^{\ell_2}$, then $\ccalQ_{q_B^{\text{aux}}}^{\text{next}}=\{q_B^{\text{aux}},q_F\}$, $\ccalQ_{q_B^{F}}^{\text{next}}=\{q_F\}$, and $\ccalQ_{B}^{\text{loop}}=\{q_B^{\text{aux}},q_F\}$.
    %$\ccalQ_{B}^{\text{loop}}=\{q_B^{\text{aux}},q_B^0\}$. Also, there only decomposable transition originating from $q_B^0$ is its self-loop. As a result, the transition   Transition from the initial state $q_B^0$ to the final state $q_B^F$ is infeasible as robot $1$ is required to `jump' from $\ell_1$ to $\ell_2$ while $\ell_1$ and $\ell_2$ are disjoint regions.
    }
    \label{fig:NBA1}
\end{figure}


\subsection{Computing Decomposable NBA Transitions}\label{sec:dec}

Given any Boolean formula $b^{q_B,q_B'}$, we define the set $\ccalN^{q_B,q_B'}\subseteq\ccalN$ that collects the indices of all robots that appear in $b^{q_B,q_B'}$. Also, given a symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$, we define the set $\ccalR^{q_B,q_B'}\subseteq\ccalN^{q_B,q_B'}$ that collects the indices $j$ of the robots that are involved in generating $\sigma_{q_B,q_B'}$. Also, we denote by $L_{j}^{q_B,q_B'}$ the location that robot $j\in\ccalN^{q_B,q_B'}$ should be located to generate $\sigma^{q_B,q_B'}$. Note that for robots $j\in\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$, $L_{j}^{q_B,q_B'}$ corresponds to any location $\bbq\in\Omega$ where no atomic predicates are satisfied; see also Example \ref{ex:exFeasSets}. 

Consider an NBA state $q_B$ with a feasible self-loop, as per Definition \ref{def:feas1}, that is reachable from the initial state. Given $q_B$, compute a finite $K\geq 1$ so that if a symbol, denoted by $\sigma^{q_B,q_B^K}$, is repeated $K$ times the following finite run will be generated:
\begin{equation}\label{eq:run}
    \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K},
\end{equation}
starting from $q_B$. In \eqref{eq:run}, the run is defined so that (i) $q_B^k\neq q_B^{k+1}$, for all $k\in\{1,K-1\}$; (ii) $\delta_B(q_B^k,\sigma^{q_B,q_B^K},q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$, i.e., the robots cannot remain in any of the intermediate states (if any) that connect $q_B$ to $q_B^K$ either because a feasible self-loop does not exist or because $\sigma^{q_B,q_B^K}$ cannot activate this self-loop; and (iii) $\delta_B(q_B^K,\sigma^{q_B,q_B^K},q_B^{K})$ i.e., there is a feasible loop associated with $q_B^K$ that is activated by $\sigma^{q_B,q_B^K}$ and, therefore, the robots can remain in $q_B^K$ as long as $\sigma^{q_B,q_B^K}$ is generated. The fact that the finite repetition of a \textit{single} symbol needs to generate the run \eqref{eq:run} precludes multi-hop transitions from $q_B$ to $q_B^K$ that require a robot to jump from one region of interest to another one instantaneously as such transitions are not meaningful as discussed in Section \ref{sec:PF}; see e.g., Fig. \ref{fig:feas1}. 

%Hereafter, we denote by $\delta_B^K(q_B,\cdot,q_B^K)$ the multi-hop NBA transition corresponding to the run \eqref{eq:run}. 
%
The symbol $\sigma^{q_B,q_B^K}$ is selected from $\Sigma^{q_B,q_B^K}$ that is constructed from the Boolean formula \eqref{eq:b} as per Definition \ref{defn:feasSet}.
\begin{equation}\label{eq:b}
   b^{q_B,q_B^K}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}.  
\end{equation}
By definition of \eqref{eq:b}, if there exists a symbol $\sigma^{q_B,q_B^K}$ that satisfies $b^{q_B,q_B^K}$ then the finite word generated by repeating $K$ times the symbol $\sigma^{q_B,q_B^K}$ will yield the run in \eqref{eq:run}. 
%
%
%
%Note that such a state $q_B^{K}$ can always be reached (assuming $\phi$ is satisfiable), since 
Finding such a symbol $\sigma^{q_B,q_B^K}$ and a state $q_B^K$ can be accomplished by viewing the NBA as a directed graph and applying graph-search methods on it.


%Next we define the decomposable transitions $\delta_B^{K_i}(q_B,q_B^{K_i})$; for simplicity of notation, when it is clear from the context we drop the index $i$. If $\delta_B^{K}(q_B,q_B^K)$ is not decomposable, then the multi-hop transition $\delta_B^{K}(q_B,q_B^{K})$ is removed. To define the decomposable transitions, we need first to introduce the following definition. 


%THE ROBOTS IN $\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$ GET OUT OF THEIR CURRENT REGIONS!
%q_B^K\in\ccalQ_B^{\text{loop}}
\begin{definition}[Decomposable NBA transitions]\label{def:feas}
A transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ corresponding to a run as in \eqref{eq:run} is decomposable if for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$, there exists at least one symbols $\sigma^{q_B,q_B^{K}}\in\Sigma^{q_B,q_B^K}$
such that $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^K}$.
\end{definition}

Observe that Definition \ref{def:feas} allows us to cast transition from $q_B$ to states $q_B^K$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B^K}$ needs to move to a region of interest $L_{j}^{q_B,q_B^K}$ while avoiding obstacles and/or other regions of interest. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is continuously learned; see Section \ref{sec:planning}. 
%
Moreover, note that it is possible that there is more than one such state $q_B^{K}$ that can be reached from $q_B$ and possibly more than one paths/runs to reach the same $q_B^K$. All (feasible) symbols that can generate a run in the form of \eqref{eq:run} towards a state $q_B^K$ are collected in a set $\Sigma^{q_B,q_B^{K}}_{\text{dec}}$.


Recall that Definition \ref{def:feas} is applied to all states $q_B\in\ccalQ_B^{\text{loop}}$ with feasible self-loops that can be reached from the initial state.  In what follows, we discuss how to compute the set $\ccalQ_B^{\text{loop}}$ which is summarized in Algorithm \ref{alg:prune}. As discussed before, the $\ccalQ_B^{\text{loop}}$ is initialized as $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$ [line \ref{prune:init}, Alg. \ref{alg:prune}]. 
%
All states $q_B\in\ccalQ_B^{\text{loop}}$ for which Definition \ref{def:feas} has been checked are collected in the set $\ccalQ_B^{\text{checked}}\subseteq\ccalQ_B^{\text{loop}}$ and the remaining states of $\ccalQ_B^{\text{loop}}$ are collected in $\ccalQ_B^{\text{not-checked}}$, i.e., $\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$. 
%
These sets are initialized as $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$ and $\ccalQ_B^\text{checked}=\emptyset$  [line \ref{prune:init}, Alg. \ref{alg:prune}]. Next we compute all possible finite runs starting from $q_B$ as defined in \eqref{eq:run} [line \ref{prune:run}, Alg. \ref{alg:prune}]. For each run \eqref{eq:run}, we examine if the corresponding multi-hop transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ is decomposable as per Definition \ref{def:feas} [lines \ref{prune:FornextS}-\ref{prune:UpdLoop2}, Alg. \ref{alg:prune}]. If it is decomposable then we update the set $\ccalQ_B^{\text{loop}}$ as: $\ccalQ_B^{\text{loop}}=\ccalQ_B^{\text{loop}}\cup\{q_B^K\}$ [line \ref{prune:UpdLoop1}, Alg. \ref{alg:prune}]. Also, we update the set $\ccalQ_B^{\text{next}}$ as $\ccalQ_B^{\text{next}}=\ccalQ_B^{\text{next}}\cup\{q_B^K\}$ [line \ref{prune:UpdLoop2}, Alg. \ref{alg:prune}]. The set $\ccalQ_B^{\text{next}}$ is initialized as $\ccalQ_B^{\text{next}}=\emptyset$ and collects all states $q_B^K\in\ccalQ_B^{\text{loop}}$ associated with $q_B$. 
%
Once all runs are examined, we update the set $\ccalQ_B^{\text{checked}}$ as $\ccalQ_B^{\text{checked}}=\ccalQ_B^{\text{checked}}\cup\ccalQ_B^{\text{checked}}\cup\{q_B\}$ and the set $\ccalQ_B^{\text{not-checked}}$ as
$\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$ [lines \ref{prune:checked}-\ref{prune:notchecked}, Alg. \ref{alg:prune}]. This process is repeated for all states $q_B\in\ccalQ_B^{\text{not-checked}}$ and terminates when $\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}=\emptyset$.


%Let also $ \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}$ be a run/path in the NBA that connects. Let also $ \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}$ be a $K$-hop path in the automaton (after removing infeasible transitions) that connect $q_B$ to $q_B^K=q_B'$. Hereafter, we denote a $K$-hop NBA transition as $\delta_B(q_B,\cdot,q_B^K)$. 

---------------------
%Let $q_B$ and $q_B'$ be NBA states with feasible self-loops, i.e., $\Sigma_{q_B,q_B}=\emptyset$ and $\Sigma_{q_B',q_B'}=\emptyset$. Let also $ \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K}$ be a $K$-hop path in the automaton (after removing infeasible transitions) that connect $q_B$ to $q_B^K=q_B'$. Hereafter, we denote a $K$-hop NBA transition as $\delta_B(q_B,\cdot,q_B^K)$. 

In Section \ref{sec:planning}, we use the pruned NBA to guide planning as follows. Specifically, assume that at time $t$ the robots reach a state $q_B$ with a feasible self-loop that is activated, i.e., $L(\bbp(t))\models b^{q_B,q_B}$ (i.e., the current observations allow the robots to remain in $q_B$). Then the robots coordinate to select a new state $q_B'\neq q_B$ with a feasible self-loop that will also be activated when the robots reach it at a time $t'>t$. The state $q_B'$ is selected so that progress towards accomplishing the assigned mission is made; this process will be discussed in detail in Section \ref{sec:planning}. Such transitions are called decomposable. Note that transition from $q_B$ to $q_B'$ may be a multi-hop NBA transition. Hereafter, we denote a $K$-hop NBA transition from $q_B$ to $q_B'$ as $\delta_B^K(q_B,\cdot,q_B^K)$, where $q_B^K=q_B'$. %
%
In this section, we define conditions under which transition from $q_B$ to $q_B'$ is decomposable. 
%Transitions $\delta_B^K(q_B,\cdot,q_B^K)$ that cannot be enabled by solving local reachability-avoidance planning problems are called non-decomposable. %and are removed from the NBA.
%
%Next, we remove a transition $\delta_B(q_B,\cdot,q_B')$ only if transition from $q_B$ to $q_B'$ and from $q_B'$ to $q_B'$ can be decomposed into local reachability-avoid tasks per robot. This concept is formalized next. To take into account the initial multi-robot state in this pruning process, first, we introduce auxiliary states $q_B^{\text{aux}}$ and transitions $q_B^{\text{aux}}\rightarrow_B q_B^0$ for all $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=\wedge_j\in\ccalN L(\bbp_j(0))$, i.e., transition from $q_B^\text{aux}$ to $q_B^0$ can always be enabled. Hereafter, the auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA %and are introduced to take into account the initial multi-robot state as it may also result in infeasible NBA transitions; see e.g., Figure \ref{fig:NBA1}. 
%
%Consider any NBA state $q_B$ for which a feasible self-loop (as per Definition \ref{def:feas1}) exists. Also assume that there exists a sequence of observations, i.e., atomic predicates, that the robots can satisfy to reach $q_B$ from an initial state and stay in it, i.e., activate its self-loop. All such states $q_B$ are collected in the set $\ccalQ_B^{\text{loop}}$; computation of $\ccalQ_B^{\text{loop}}$ will be discussed later and summarized in Algorithm \ref{alg:prune}. %Let $q_B^1$ be an NBA state that is within one-hop reachable from $q_B$. %The following process is repeated for all such states $q_B$ and for each transition $\delta_{B}(q_B,\cdot,q_B^1)$ that originates from $q_B$. 
%In what follows, we discuss when $\delta_{B}(q_B,\cdot,q_B^1)$ is non-decomposable and therefore it should be removed. 


All states $q_B$ with feasible self-loops (Definition \ref{def:feas1}) that can reached from the initial state by following decomposable transitions and then stay in it, i.e., activate its self loop, are collected in a set denoted $\ccalQ_B^{\text{loop}}$. Construction of this set is summarized in Algorithm \ref{alg:prune} and will be discussed later. In what follows, we examine if there any decomposable transitions $\delta_{B}^K(q_B,\cdot,q_B^K)$ from a state $q_B\in\ccalQ_B^{\text{loop}}$ towards states $q_B'=q_B^K\in\ccalQ_B^{\text{loop}}$. 
%collects all NBA states with feasible self-loops (Definition \ref{def:feas1}) that can reached from the initial state by following decomposable transitions (Definition \ref{def:feas}).
%If there are no decomposable transitions originating from $q_B\in\ccalQ_B^{\text{loop}}$,
Examples illustrating this process are provided in Figures \ref{fig:prune} and \ref{fig:NBA1}.    %All one-hop transitions $\delta_{B}(q_B,\cdot,q_B')$ that are not part of any decomposable transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ are removed. 

First, to take into account the initial multi-robot state in this process, we introduce auxiliary states $q_B^{\text{aux}}$ and transitions $\delta_B(q_B^{\text{aux}},\cdot, q_B^0)$ for all $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=\wedge_{j\in\ccalN} L(\bbp_j(0))$, i.e., transition from $q_B^\text{aux}$ to $q_B^0$ can always be enabled; see also Figure \ref{fig:NBA1} [line \ref{prune:aux}, Alg. \ref{alg:prune}]. Hereafter, the auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA. The set $\ccalQ_B^{\text{loop}}$ is initialized as $\ccalQ_B^{\text{loop}}=\{q_B^{\text{aux}}\}$ [line \ref{prune:init}, Alg. \ref{alg:prune}].

Given any state $q_B\in\ccalQ_B^{\text{loop}}$, we compute a finite $K\geq 1$ so that if a symbol, denoted by $\sigma^{q_B,q_B^K}$, is repeated $K$ times the following finite run will be generated:
\begin{equation}\label{eq:run}
    \rho=q_B q_B^1\dots q_B^{K-1}q_B^{K},
\end{equation}
starting from $q_B$. In \eqref{eq:run}, the run is defined so that (i) $q_B^k\neq q_B^{k+1}$, for all $k\in\{1,K-1\}$; (ii) $\delta_B(q_B^k,\sigma^{q_B,q_B^K},q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$, i.e., the robots cannot remain in any of the intermediate states (if any) that connect $q_B$ to $q_B^K$ either because a feasible self-loop does not exist or because $\sigma^{q_B,q_B^K}$ cannot activate this self-loop; and (iii) $\delta_B(q_B^K,\sigma^{q_B,q_B^K},q_B^{K})$ i.e., there is a feasible loop associated with $q_B^K$ that is activated by $\sigma^{q_B,q_B^K}$ and, therefore, the robots can remain in $q_B^K$ as long as $\sigma^{q_B,q_B^K}$ is generated. The fact that the finite repetition of a \textit{single} symbol needs generate the run \eqref{eq:run} precludes multi-hop transitions from $q_B$ to $q_B^K$ that require a robot to jump from one region of interest to another one instantaneously as such transitions are not meaningful as discussed in Section \ref{sec:PF}; see e.g., Fig. \ref{fig:feas1}. 

%Hereafter, we denote by $\delta_B^K(q_B,\cdot,q_B^K)$ the multi-hop NBA transition corresponding to the run \eqref{eq:run}. 
%
The symbol $\sigma^{q_B,q_B^K}$ is selected from $\Sigma^{q_B,q_B^K}$ that is constructed from the Boolean formula 
\begin{equation}\label{eq:b}
   b^{q_B,q_B^K}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}.  
\end{equation}
By definition of \eqref{eq:b}, if there exists a symbol $\sigma^{q_B,q_B^K}$ that satisfies $b^{q_B,q_B^K}$ then the finite word generated by repeating $K$ times the symbol $\sigma^{q_B,q_B^K}$ will yield the run in \eqref{eq:run}. 
%
%
%
%Note that such a state $q_B^{K}$ can always be reached (assuming $\phi$ is satisfiable), since 
Finding such a symbol $\sigma^{q_B,q_B^K}$ and a state $q_B^K$ can be accomplished  by viewing the NBA as a directed graph and applying graph-search methods on it.


To define when a transition $\delta_B^K(q_B,\cdot,q_B^K)$ is decomposable, we need first to introduce the following definitions. Given a Boolean formula $b^{q_B,q_B'}$, we define the set $\ccalN^{q_B,q_B'}\subseteq\ccalN$ that collects the indices of all robots that appear in $b^{q_B,q_B'}$. Also, given a symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$, we define the set $\ccalR^{q_B,q_B'}\subseteq\ccalN^{q_B,q_B'}$ that collects the indices $j$ of the robots that are involved in generating $\sigma_{q_B,q_B'}$. Also, we denote by $L_{j}^{q_B,q_B'}$ the location that robot $j\in\ccalN^{q_B,q_B'}$ should be located to generate $\sigma^{q_B,q_B'}$. Note that for robots $j\in\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$, $L_{j}^{q_B,q_B'}$ corresponds to any location $\bbq\in\Omega$ where no atomic predicates are satisfied; see also Example \ref{ex:exFeasSets}.   

%Next we define the decomposable transitions $\delta_B^{K_i}(q_B,q_B^{K_i})$; for simplicity of notation, when it is clear from the context we drop the index $i$. If $\delta_B^{K}(q_B,q_B^K)$ is not decomposable, then the multi-hop transition $\delta_B^{K}(q_B,q_B^{K})$ is removed. To define the decomposable transitions, we need first to introduce the following definition. 


%THE ROBOTS IN $\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$ GET OUT OF THEIR CURRENT REGIONS!
%q_B^K\in\ccalQ_B^{\text{loop}}
\begin{definition}[Decomposable NBA transitions]\label{def:feas}
A transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ corresponding to a run as in \eqref{eq:run} is decomposable if for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$, there exists at least one symbols $\sigma^{q_B,q_B^{K}}\in\Sigma^{q_B,q_B^K}$
such that $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^K}$.
\end{definition}

Observe that Definition \ref{def:feas} allows us to cast transition from $q_B$ to states $q_B^K$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B^K}$ needs to move to a region of interest $L_{j}^{q_B,q_B^K}$ while avoiding obstacles and/or other regions of interest. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is continuously learned; see Section \ref{sec:planning}. 
%
Moreover, note that it is possible that there is more than one such state $q_B^{K}$ that can be reached from $q_B$ and possibly more than one paths/runs to reach the same $q_B^K$. All (feasible) symbols that can generate a run in the form of \eqref{eq:run} towards a state $q_B^K$ are collected in a set $\Sigma^{q_B,q_B^{K}}_{\text{dec}}$.

%All such states are appended to $\ccalQ_{B}^{\text{loop}}$. Thus, the above process is repeated for all finite runs in the form of \eqref{eq:run}. Also, 
%Thus, we define the set $\ccalP_{q_B}^{\text{next}}$ that collects all finite runs, denoted by $\rho_i=q_B q_B^{1,i}\dots q_B^{k_i}\dots q_B^{K_i}$, in the form of \eqref{eq:run} that originate from $q_B\in\ccalQ_B^{\text{loop}}$ and the set $\ccalQ_{q_B}^{\text{next}}$ that collects all states $q_B^{K_i}$. Also, there may be more than one word that can yield the same run $\rho_i$. Thus, we collect in a set $\Sigma^{q_B,q_B^{K_i}}$ all symbols that can yield the run $\rho_i$, i.e., all symbols that satisfy the corresponding formula \eqref{eq:b}. Next, we delete the transition from $q_B$ to $q_B^{1,i}$ and we replicate all intermediate states that connect $q_B$ to $q_B^{K_i}$ so that for each state $q_B^{k_i}$ there is only one incoming transition from $q_B^{k_i-1}$ and one outgoing transition to $q_B^{k_i+1}$. This step allows us to examine each multi-hop transition independently as it is possible that more than one multi-hop transition shares common states.

%or more than one symbol that can be used to reach $q_B^{K}$. For every state $q_B\in\ccalQ_B^{\text{loop}}$, we define the set $\ccalP_{q_B}^{\text{next}}$ that collects all pairs of sets of feasible symbols and states, where the $i$-th pair is denoted by $(\Sigma^{q_B,q_B^{K_i}},q_B^{K_i})$, so that a symbol $\sigma^{q_B,q_B^{K_i}}\in\Sigma^{q_B,q_B^{K_i}}$ satisfies the corresponding formula \eqref{eq:b}, i.e.,
%\begin{align}\label{eq:pairs}
%    \ccalP_{q_B}^{\text{next}} = \{&(\Sigma^{q_B,q_B^{K_i}},q_B^{K_i})~|~\nonumber\\&\sigma^{q_B,q_B^{K_i}}\models b^{q_B,q_B^{K_i}}, \forall \sigma^{q_B,q_B^{K_i}}\in\Sigma^{q_B,q_B^{K_i}}\}
%\end{align}
%


%conditions under which conditions a symbol $\sigma^{q_B,q_B^{K_i}}$ can be generated by solving local/independent reachability-avoid tasks for each robot. If $\sigma^{q_B,q_B^{K_i}}$ can be generated in this way then we call the multi-hop transition from $q_B$ to $q_B^{K_i}$, denoted by $\delta_B^K(q_B,q_B^{K_i})$






%This concept is formalized in lines ??? in Algorithm \ref{alg:prune}. First, we introduce auxiliary states $q_B^{\text{aux}}$ and transitions $q_B^{\text{aux}}\rightarrow_B q_B^0$ for all $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=L(\bbp(0))$. The auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA and are introduced to take into account the initial multi-robot state as it may also result in infeasible NBA transitions; see e.g., Figure \ref{fig:NBA1}. 
%
%The key idea in lines ?? -?? is the following. Consider an NBA $q_B$ for which a feasible self-loop (as per Def??) exists. Assume that there exists a sequence of observations, i.e., atomic predicates that the robots can satisfy to reach $q_B$ from $q_B^{\text{aux}}$. Determining which states $q_B$ satisfy this condition will be discussed later. The following process is repeated for all such states $q_B$. We remove transitions $\delta_{B}(q_B,\cdot,q_B^1)$ (i) if after enabling this transition the robots are required to `jump' from one region of interest to another one so that they eventually visit and remain in another state with a feasible self-loop or (ii) if activation of $\delta_{B}(q_B,\cdot,q_B^1)$ cannot be cast as local reachability-avoid planning tasks per robot; as it will be discussed next condition (ii) is conservative. The latter is formalized in the following definition.

%\begin{definition}[Feasible NBA transitions]\label{def:feas}
%A transition $\delta_{B}(q_B,\cdot,q_B^1)$, $q_B\neq q_B^1$ is feasible if the following two conditions hold. (i) There exists at least one symbol denoted by $\sigma^{q_B,q_B^K}$ and a finite $K\geq 1$ so that the infinite word $w=[\sigma^{q_B,q_B^K}]^\omega$ enables either (A) a run of the form $\rho=q_B q_B^1\dots q_B^{K-1}[q_B^{K}]^\omega$, where $\delta_B(q_B^k,w(k),q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K-1\}$ or (B) an accepting run $\rho$. The symbol $\sigma^{q_B,q_B^K}$ is selected from $\Sigma^{q_B,q_B^K}$ that is constructed from the Boolean formula $b^{q_B,q_B^K}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}$.
%%$\rho=q_B q_B^1\dots q_B^{m-1}[q_B^{m}\dots q_B^{K-1}q_B^{K}]^\omega$, where $\delta_B(q_B^k,w(k),q_B^{k})$ is not valid for all $\forall k\in\{1,\dots,K\}$ and at least one of the final states is appears infinitely often in $\rho$. 
%(ii) For all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$, there exists at least one of the symbols $\sigma^{q_B,q_B^K}$ that satisfy condition (i) and either (A) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^1}$. %%The symbol $\sigma^{q_B,q_B^K}$ is selected from $\Sigma^{q_B,q_B^K}$ which %If $K=0$, conditions (i)-(ii) are applied by replacing $q_B^1$ with $q_B'$. %conditions (i)-(ii) assume
%\end{definition}

%If $\delta_{B}(q_B,\cdot,q_B^1)$ does not satisfy Definition \ref{def:feas}, then it is removed. Note that condition (i)-(A) requires that once robots reach a state $q_B$ with a self-loop and remain in this state, they will always be able to make progress towards accomplishing the assigned task by moving towards a new NBA state $q_B^K$ with a self-loop and remain in it as well. If such states $q_B^K$ do not exist, i.e., if after enabling a transition from $q_B$ to $q_B^1$ the robots will never be able to reach and remain in a state with self-loop, then this means final states can be reached by `instantaneously' moving from one NBA state to another one. Clearly, this requires the robots to jump from one region of interest to enable such transitions unless there is a symbol that if repeated indefinitely, at least one final state will be visited infinitely often. This is captured by condition (i)-(B).  Condition (ii) allows us to cast transition from $q_B$ to states $q_B^K$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B^K}$ needs to move to a region of interest while avoiding certain regions and obstacles. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is continuously learned. 
%
%Also, by construction of the pruned automaton we have that once the robots reach an NBA state $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$, i.e., an NBA state for which a self-loop exists, the robots can remain in this state given their current observations. To enforce this property from $t=0$, we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$. This property will be used in Section \ref{sec:planning} to design robot paths.


Recall that Definition \ref{def:feas} is applied to all states $q_B\in\ccalQ_B^{\text{loop}}$ with feasible self-loops that can be reached from the initial state.  In what follows, we discuss how to compute the set $\ccalQ_B^{\text{loop}}$ which is summarized in Algorithm \ref{alg:prune}. As discussed before, the $\ccalQ_B^{\text{loop}}$ is initialized as $\ccalQ_B^\text{loop}=\set{q_B^{\text{aux}}}$ [line \ref{prune:init}, Alg. \ref{alg:prune}]. 
%
All states $q_B\in\ccalQ_B^{\text{loop}}$ for which Definition \ref{def:feas} has been checked are collected in the set $\ccalQ_B^{\text{checked}}\subseteq\ccalQ_B^{\text{loop}}$ and the remaining states of $\ccalQ_B^{\text{loop}}$ are collected in $\ccalQ_B^{\text{not-checked}}$, i.e., $\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$. 
%
These sets are initialized as $\ccalQ_B^\text{not-checked}=\set{q_B^{\text{aux}}}$ and $\ccalQ_B^\text{checked}=\emptyset$  [line \ref{prune:init}, Alg. \ref{alg:prune}]. Next we compute all possible finite runs starting from $q_B$ as defined in \eqref{eq:run} [line \ref{prune:run}, Alg. \ref{alg:prune}]. For each run \eqref{eq:run}, we examine if the corresponding multi-hop transition $\delta_{B}^K(q_B,\cdot,q_B^K)$ is decomposable as per Definition \ref{def:feas} [lines \ref{prune:FornextS}-\ref{prune:UpdLoop2}, Alg. \ref{alg:prune}]. If it is decomposable then we update the set $\ccalQ_B^{\text{loop}}$ as: $\ccalQ_B^{\text{loop}}=\ccalQ_B^{\text{loop}}\cup\{q_B^K\}$ [line \ref{prune:UpdLoop1}, Alg. \ref{alg:prune}]. Also, we update the set $\ccalQ_B^{\text{next}}$ as $\ccalQ_B^{\text{next}}=\ccalQ_B^{\text{next}}\cup\{q_B^K\}$ [line \ref{prune:UpdLoop2}, Alg. \ref{alg:prune}]. The set $\ccalQ_B^{\text{next}}$ is initialized as $\ccalQ_B^{\text{next}}=\emptyset$ and collects all states $q_B^K\in\ccalQ_B^{\text{loop}}$ associated with $q_B$. 
%
Once all runs are examined, we update the set $\ccalQ_B^{\text{checked}}$ as $\ccalQ_B^{\text{checked}}=\ccalQ_B^{\text{checked}}\cup\ccalQ_B^{\text{checked}}\cup\{q_B\}$ and the set $\ccalQ_B^{\text{not-checked}}$ as
$\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$ [lines \ref{prune:checked}-\ref{prune:notchecked}, Alg. \ref{alg:prune}]. This process is repeated for all states $q_B\in\ccalQ_B^{\text{not-checked}}$ and terminates when $\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}=\emptyset$.
%all states $q_B^{K}$ that exist in $\ccalQ_{q_B}^{\text{next}}$ and can be reached through a symbol that satisfies Definition \ref{def:feas}. 
%Once all states in $\ccalQ_B^{\text{not-checked}}$ are examined, we update the set   $\ccalQ_B^{\text{not-checked}}$ as $\ccalQ_B^{\text{not-checked}}=\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}$. This process is repeated until $\ccalQ_B^{\text{loop}}\setminus\ccalQ_B^{\text{checked}}=\emptyset$. %Definition \ref{def:feas} has been applied to all transitions originated from states with feasible self-loops that can be reached from $q_B^{\text{aux}}$. 
Algorithm \ref{alg:prune} will terminate due to the finite set of NBA states and transitions. By construction of Algorithm \ref{alg:prune}, $\ccalQ_B^{\text{loop}}$ collects all NBA states with feasible self-loops (Definition \ref{def:feas1}) that can reached from the initial state by following decomposable transitions (Definition \ref{def:feas}).

%\begin{rem}[Non-emptiness of $\ccalQ_{q_B}^{\text{next}}$]
%Note that $\ccalQ_{q_B}^{\text{next}}\setminus\{q_B\}\neq\emptyset$ for all states $q_B\in\ccalQ_B^{\text{loop}}$ (assuming $\phi$ is satisfiable), since otherwise the only way to visit the final state after visiting $q_B$ is by instantaneously jumping from one NBA state to another one i.e., without staying in any of them. Nevertheless, such transitions cannot exist, as they would require new observations to be made every time a new NBA state is visited which is impossible to specify given that the `next' operator is omitted. %In case $\ccalQ_{q_B}^{\text{next}}=\emptyset$, then $\delta_B(q_B,\cdot,q_B^1)$ is removed.
%\end{rem}

%\begin{rem}[Conflict-free pruning]
%Note that if $\delta_{B}^K(q_B,\cdot,q_B^K)$ is decomposable as per Definition \ref{def:feas} then this means that there may exist states $q_B^k$, $k\in\{1,\dots,K-1\}$, with feasible self-loops without being activated by $\sigma^{q_B,q_B^K}$. Note that none of the transitions $\delta_B(q_B^k,\cdot,q_B^{k+1})$ should be removed at subsequent iterations of Algorithm \ref{alg:prune} since otherwise  $q_B^K$ may not be reachable from $q_B$. However, if there is a sequence of observations so that $q_B^k$ is reached from the initial state, then Definition \ref{def:feas} will be applied to the transition $\delta_B(q_B^k,\cdot,q_B^{k+1})$. If Definition \ref{def:feas} is not satisfied, then $\delta_B(q_B^k,\cdot,q_B^{k+1})$ should be removed which creates a conflict. To avoid such conflicts, if $\delta_{B}^K(q_B,\cdot,q_B^K)$ is decomposable, then we replicate all states $q_B^k$ with self-loops so that they have only one incoming transition which is  $\delta_{B}(q_B^{k-1},\cdot,q_B^k)$ and one outgoing transition which is $\delta_{B}(q_B^{k},\cdot,q_B^{k+1})$. By construction, the replicated state can be reached only through $q_B$ and therefore, it will never be removed. This is applied to all states $q_B^K$ collected in $\ccalQ_{q_B}^{\text{next}}$. Note that in our conducted experiments such conflicts never occurred.
%\end{rem}

%END END END


%In words, a transition from $q_B$ to $q_B'$ is feasible and, therefore, it is not removed (a) if the set $\Sigma^{q_B,q_B}$ is non-empty, i.e., there are feasible symbols that allow the robots to stay in state $q_B$; and (ii) for each possible symbol in $\Sigma^{q_B,q_B}$ that the robots may generate to reach $q_B'$, there exists a feasible symbol that will enable the robots to eventually reach a new state $q_B'$ from $q_B$ and stay in $q_B'$. Also, in (iii) we require the set of robots in $\ccalN^{q_B,q_B'}$ that to be either (a) disjoint from the set of robots in $\ccalR^{q_B,q_B}$ or (b) if there exist robots $j\in \ccalR^{q_B,q_B}\cap\ccalN^{\text{next}}^{q_B,q_B'}\neq\emptyset$ then these robots should suffice to stay in their current locations, i.e., $L_{j}^{q_B,q_B'}=L_{j}^{q_B,q_B}$, to `contribute' to satisfaction of $b^{\text{next}}^{q_D,q_D'}$. As it will be discussed later, this allows us to cast transition from $q_B$ to $q_B'$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalN^{q_B,q_B'}$ needs to move to a region of interest while avoiding certain regions and obstacles. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is learned.

%IN THE PRUNED AUTOMATON WE HAVE THAT ONCE WE VISIT A SELF-LOOP STATE WE CAN STAY IN IT MAKE PROGRESS I.E. VISIT NEW TASKS. This essentially allows us to avoid cases WHERE ROBOTS HAVE TO 'JUMP' FROM ONE REGION OF INTEREST TO ANOTHER ONE. WE USE THIS PROPERTY FOR PLANNING IN SECTION ?. TO ENFORCE THIS PROPERTY AT T=0, WE ASSUME THAT THE INITIAL CONDITION ALWAYS SATISFIES THE INITIAL SELF-LOOP IF IT EXISTS. 

%OR AVOID IT AND MENTION IT IN THE THEOREMS!!!

%IT IS POSSIBLE THAT THE INIT STATE DOES NOT HAVE A SELF LOOP OR THE INIT ROBOT STATE DOES NOT SATISFY.

%SAY HERE THAT OUR GOAL IS THAT ONCE WE VISIT A STATE WITH SELF LOOPS TO SATISFY THE RESPECTIVE CONDITION UNTIL WE MAKE NEW OBSERVATIONS THAT WILL ALLOWS US TO MAKE PROGRESS IE VISIT NEW TASKS


%\begin{ex}[Conservative Pruning]
%-Add figure and explain-
%\end{ex}
\begin{figure}
    \centering
     \includegraphics[width=1\linewidth]{figures/conserv.png}
    \caption{Example of conservativeness of Definition \ref{def:feas} for the NBA corresponding to $\phi=\square(\pi_1^{r_0}\vee\pi_1^{r_0}) \wedge \Diamond \pi_2^{r_1}\wedge \Diamond \pi_2^{r_1}$. This formula requires either robot $1$ or $2$ to always be in $\ell_0$ and eventually robots $1$ and $2$ to visit, not necessarily simultaneously, $\ell_1$. Transition from $q_B^0$ to $q_B^F$ is removed as it requires robots to visit more than one location at the same time. Transitions from $q_B$ to $q_F$ and from $q_B'$ to $q_F$ are removed as they violate both conditions of Definition \ref{def:feas} resulting in a disconnected pruned NBA, i.e., Algorithm \ref{alg:RRT} will not be able to find a solution. Nevertheless, a solution exists, as these two transitions can be enabled in practice. For instance, consider the transition from $q_B$ to $q_F$. %Assuming that both robots are initially in $\ell_0$, 
    Observe that transition from $q_B$ to $q_F$ cannot be cast as two independent reachability-avoidance problems. In fact, it requires coordination among the robots that is specific to the Boolean formula $b^{q_B,q_F}$. Specifically, when the robots reach $q_B$, we have that robot $1$ is in $\ell_0$ and robot $2$ is in $\ell_1$. To eventually satisfy $b^{q_B,q_F}=(\pi_1^{\ell_0}\wedge\pi_2^{\ell_1})\vee(\pi_2^{\ell_0}\wedge\pi_2^{\ell_1})$, first robot $2$ is required 
    to return in $\ell_0$ while in the meantime robot $1$ should stay in $\ell_0$. Once robot $2$ returns in $\ell_0$, robot $1$ should move to $\ell_1$ enabling the transition to the final state $q_F$.}
    \label{fig:conserv}
\end{figure}
%
%Conditions under which Definition \ref{def:feas} is not conservative are presented in Section \ref{sec:complOpt}.%, and/or (c) if it is (physically) impossible for the robots to stay in $q_D$ until the symbol $\sigma^{\text{next}}$, that triggers transition to $q_D'$, is generated; the latter happens if condition (iii) is not true (see also Ex. \ref{ex:feas}). 


\begin{rem}[Conservativeness]\label{rem:conserv}
%First, note that requiring a multi-hop transition to be enabled if the Boolean formula \eqref{eq:b} is satisfied is not conservative, since if \eqref{eq:b} is not satisfied then, this means that to enable this transition at least one robot has to instantaneously move from o
Algorithm \ref{alg:prune} is conservatice due to Definition \ref{def:feas}. Particularly, there may exist (feasible) symbols $\sigma^{q_B,q_B^K}$ that satisfy \eqref{eq:b} but they do not satisfy Definition \ref{def:feas}; see e.g., Figure \ref{fig:conserv}. Conditions under which Definition \ref{def:feas} and, consequently Algorithm \ref{alg:prune}, is not conservative are discussed in Section \ref{sec:complOpt}.
%Nevertheless, conservative pruning ensures that when the robots reach a state $q_D$, they will always be able to make progress towards accomplishing their task (i.e., reach a new state $q_D'$) regardless of the symbols they have generated to reach $q_D$ by solving local point-to-point navigation problems. A fragment of LTL for which the proposed approach is not conservative is discussed in Section \ref{sec:complOpt}.
\end{rem}

\begin{ex}(Sets of Feasible Symbols)
(a) Consider the Boolean formula $b^{q_B,q_B'}=(\pi_j^{r_e}\vee\pi_j^{r_m})\wedge(\neg \pi_i^{r_e})$, then $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$. %, i.e., it does not include any symbol associated with other robots $k\neq j$ that may also satisfy $b^{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_k^{r_f}$).
Given the Boolean formula $b^{q_B,q_B'}$, we have that $\ccalN^{q_B,q_B'}=\set{j,i}$.
%
Also, for $\sigma^{q_B,q_B'}=\pi_j^{r_e}$, we have that $\ccalR^{q_B,q_B'}=\set{j}$, $L_{j}^{q_B,q_B'}=r_e$. (b) Consider the Boolean formula $b^{q_B,q_B'}=\neg \pi_i^{r_e}$. In this case $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\varnothing\}$, where $\varnothing$ denotes an empty symbol and is generated when a robot is outside all regions interests and does hit any obstacles. Also, we have that $\ccalN^{q_B,q_B'}=\set{i}$, $\sigma^{q_B,q_B'}=\varnothing$, $\ccalR^{q_B,q_B'}=\emptyset$, and while $L_{i}^{q_B,q_B'}$ corresponds to any location $\bbq$ in the workspace where no atomic predicates are satisfied. 
\label{ex:exFeasSets}
\end{ex}

\subsection{Distance Metric Over the Pruned NBA}\label{sec:dist}
Given the pruned NBA, we define a function to compute how far two NBA states that belong to $\ccalQ_B^{\text{loop}}$ are. This metric will be used in Section \ref{sec:planning} to guide planning towards states in $\ccalQ_B^{\text{loop}}$ that are closer to the final states.
%By construction of the pruned automaton, for every a state $q_B\in\ccalQ_B^{\text{loop}}$ there exists a symbol that if repeated a finite number of times then another state $q_B'\in\ccalQ_B^{\text{loop}}$ can be visited while this symbol allows to remain in $q_B'$. Also, as discussed before, transition from $q_B$ to $q_B'$ will occur while possibly going through intermediate states but self-loops are
To this end, we construct a directed graph $\ccalG=\{\ccalV,\ccalE\}$ where $\ccalV$ is the set of nodes defined as $\ccalV=\ccalQ_B^{\text{loop}}$ and $\ccalE\subseteq\ccalV\times\ccalV$ is the set of edges. Specifically, there exists an edge from node $q_B\in\ccalV$ to $q_B'\in\ccalV$ if $\Sigma^{q_B,q_B^{K}}_{\text{dec}}\neq\emptyset$, i.e., if there exists a decomposable transition from $q_B$ to $q_B'$ as per Definition \ref{def:feas}. 

Given the graph $\ccalG$, we define the distance metric
$d:\ccalV\times\ccalV\rightarrow \mathbb{N}$ that returns the minimum number of transitions among states in $\ccalQ_B^{\text{loop}}$ that are required to reach a state $q_B'\in\ccalQ_B^{\text{loop}}$ starting from a state $q_B\in\ccalQ_B^{\text{loop}}$. %This function will be used to guide the robots towards locations in the workspace so that eventually a final DFA state is visited, i.e., the LTL formula is satisfied.
%
Particularly, we define the distance function $d: \ccalQ_B^{\text{loop}} \times \ccalQ_B^{\text{loop}} \rightarrow \mathbb{N}$ as follows
\begin{equation}\label{eq:dist}
d(q_B,q_B')=\left\{
                \begin{array}{ll}
                  |SP_{q_B,q_B'}|, \mbox{if $SP_{q_B,q_B'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_B,q_B'}$ denotes the shortest path (in terms of hops) in $\ccalG$ from $q_B$ to $q_B'$ and $|SP_{q_B,q_B'}|$ stands for its cost (number of hops).%\footnote{In Section \ref{sec:complOpt}, we provide conditions under which if $d(q_D^0,q_F)=\infty$ then the assigned co-safe LTL task is infeasible}. %; see Sections \ref{sec:targetDFA}-\ref{sec:paths}.

Next, we define the final/accepting edges in $\ccalG$.
\begin{definition}[Final/Accepting Edges]\label{def:accEdges}
An edge $(q_B,q_B')\in\ccalE$ is called final or accepting if the corresponding multi-hop NBA transition $\delta_B^K(q_B,\cdot,q_B')$ includes at least one final state $q_F$.
\end{definition}

Based on the definition of accepting edges, we define the set $\ccalQ_{F}^{\text{loop}}\subseteq \ccalQ_{B}^{\text{loop}}$ that collects all states $q_B\in\ccalQ_B^{\text{loop}}$ from which an accepting edge originates, i.e.,
\begin{equation}\label{eq:accNode}
    \ccalQ_{F}^{\text{loop}} = \{q_B\in\ccalQ_B^{\text{loop}}~|~\exists~ \text{accepting edge}~(q_B,q_B')\in\ccalE \}.
\end{equation}
By definition of the accepting condition of the NBA, we have that if at least one of the accepting edges is traversed infinitely often, then the corresponding LTL formula is satisfied. %States $q_B\in\ccalQ_{B}^{\text{loop}}$ for which there are accepting edges $(q_B,q_B')\in\ccalE$ are collected in a set $\ccalQ_{F}^{\text{loop}}$.%, i.e.,





%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}

%\begin{ex}[Feasible DFA transitions]\label{ex:feas}
%(a) Consider the case, where $b^{q_B,q_B}=1$ and $b^{q_B,q_B'}=\pi_j^{r_{m}}$. By definition of $\Sigma^{q_B,q_B}$ and $\Sigma^{q_B,q_B'}$, we have that $\Sigma^{q_B,q_B}=\{\varnothing\}$, where $\varnothing$ stands for the empty symbol, and $\Sigma^{q_B,q_B'} =\{\pi_j^{r_{m}}\}$. Transition from $q_B$ to $q_B'$ is feasible as per Definition \ref{def:feas}. Recall that the sets $\Sigma^{q_B,q_B}, \Sigma^{q_B,q_B'}$ collect symbols that are associated with robots that play a role in satisfying the respective Boolean formulas. This precludes cases where, e.g., a symbol $\pi_j^{r_e}$, $e\neq m$ is included in $\Sigma^{q_B,q_B}$ resulting in erroneously characterizing the transition from $q_D$ to $q_D'$ as infeasible due to condition (iii). 
%%%(b) Consider the following Boolean conditions: $b^{\text{inv}}^{q_D}=b^{\text{inv}}^{q_D'}=\pi_j^{r_i}$ and $b^{\text{next}}^{q_D,q_D'}=\pi_j^{r_i}\wedge \pi_m^{r_h}$. Then the transition from $q_D$ to $q_D'$ is feasible since it satisfies Definition \ref{def:feas}. 
%(b) Consider also the Boolean formulas  $b^{q_B,q_B}=b^{q_B',q_B'}=\pi_j^{r_i}$ and $b^{q_B,q_B'}=\pi_j^{r_e}\wedge \pi_m^{r_h}$, then the transition from $q_B$ to $q_B'$ is infeasible, since it holds that $j\in \ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and, $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. In fact, transition from $q_B$ to $q_B'$ requires robot $j$ to instantaneously move from $r_i$ to $r_e$ which is not possible given that $r_i$ and $r_e$ are disjoint regions. 
%\end{ex}




%\subsection{Selecting a Feasible DFA Final State}\label{sec:feasFinal}
%Given the pruned DFA, the distance function, and an initial DFA state $q_D(0)$, our next step is to select a \textit{feasible} final state $q_{F}\in\ccalQ_F$, i.e., a final state that is reachable from $q_D(0)$ in the pruned DFA [line \ref{rrt:feasFinal}, Alg. \ref{alg:RRT}]. In math, given an initial state  $q_D(0)$ feasible final states are the ones that satisfy  $d(q_D(0),q_{F})\neq \infty$. Among all final states that satisfy this condition, we select one randomly denoted by $q_F^{\text{feas}}$. If there do not exist such final states given the state $q_D(0)$, then we select another initial DFA state $q_D(0)$ from $\ccalQ_D^0$. If there do not exist initial states such that $d(q_D^0,q_{F})\neq \infty$, then the LTL formula can not be satisfied since the in the pruning process, only the DFA transitions that are impossible to enable are removed (i.e., the ones that require the robots to be physically present at more than one region simultaneously) [lines \ref{rrt:unsat1}-\ref{rrt:unsat2}, Alg. \ref{alg:RRT}].
%Next at any time $t\geq 0$, given the current DFA state $q_D(t)$, we select a target DFA state, denoted by $q_D^{\text{next}}$, that the robots should reach next. This state is selected so that it is one hop closer to $q_F^{\text{feas}}$ than $q_D(t)$ is, i.e.,

%\subsection{Selecting the Next NBA State}
%{\bf{Selecting the Next NBA State:}} 

\section{From Feasible Automata to Reactive Planning}\label{sec:planning}

%The pruning process described in Section \ref{sec:prune} occurs offline, i.e., before deploying the robots in the workspace. In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

In this section, we present a distributed reactive algorithm for LTL tasks. The proposed algorithm is summarized in Algorithm \ref{alg:RRT} and requires as input the sets $\ccalQ_{q_B}^{\text{next}}$ and the set of of symbols $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, for all $q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}$ and for all $q_B\in\ccalQ_B^{\text{loop}}$. Recall that $\ccalQ_{q_B}^{\text{next}}$ collects all states, denoted by $q_B^{\text{next}}$, that can reached from $q_B$ in a decomposable fashion, as per Definition \ref{def:feas}, using a symbol selected from $\Sigma_{\text{dec}}^{q_B,qq_B^{\text{next}}}$. These sets are computed offline by Algorithm \ref{alg:prune} described in Section \ref{sec:aut}.

%for all $q_B\in\ccalQ_B^{\text{loop}}$,  In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

\subsection{Distributed Construction of Robot Paths}\label{sec:paths}
Let $q_B(t)\in\ccalQ_B^{\text{loop}}$ be the NBA state that the robots have reached at time $t$ after following paths, denoted by $\bbp_{j,[0:t]}$. Assume also that $L(\bbp(t))\models b^{q_{B(t)},q_{B(t)}}$ i.e., the robots can remain in $q_B(t)$ as long as they remain idle in their current locations.
%
At time $t=0$, $q_B(t)$ is initialized to be the initial/auxiliary state $q_B^{\text{aux}}$, introduced in Section \ref{sec:prune} [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. Recall that $q_B^{\text{aux}}\in\ccalQ_B^{\text{loop}}$ and $L(\bbp(0))\models b^{q_{B(0)},q_{B(0)}}$, by definition of $q_B^{\text{aux}}$. 
%


\begin{algorithm}[t]
%\footnotesize
\caption{LTL Planning in Unknown Occupancy Grid Maps}
\LinesNumbered
\label{alg:RRT}
\KwIn{ (i) initial robot configuration $\bbp(0)$, (ii) Sets $\ccalQ_{q_B}^{\text{next}}$, $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$, $\forall q_B\in\ccalQ_{B}^{\text{loop}}$}
%\KwOut{Terminal horizon $H$, and control inputs $\bbu_{0:H}$}
%Convert $\phi$ into a DFA\label{rrt:dfa}\;
%Initial state $\bbq(0)=[\bbp(0), q_D^0]$;\label{rrt:init}
Initialize $t=0$, $q_B(0)=q_B^{\text{aux}}$\;\label{rrt:t0}
%Update current DFA state as $q_D(0)=\delta(q_D^0,L(\bbp(0)))$\;
%Prune DFA\;\label{rrt:prune}
%Select an initial state $q_D(0)=q_D^0$ and a feasible final state $q_F^{\text{feas}}$\;\label{rrt:feasFinal}
%Current DFA state $q_D(t)=q_D^0$\;\label{rrt:init}
%Compute distance from $q_D(t)$ to $q_D^F$\;
%\If{$d(q_D^0, q_F)= \infty$}{\label{rrt:unsat1}
%Error message: \textit{$\phi$ cannot be satisfied (see Proposition \ref{prop:sat})}\;}\label{rrt:unsat2}
Select the next NBA state $q_B^{\text{next}}$ and select $\sigma^{\text{next}}$\;\label{rrt:selTarget}%(see \eqref{eq:targetDFA})
Compute $L_j^{\text{next}}$ and the set of robots $\ccalN^{\text{next}}$\;\label{rrt:goals}
%Initialize $\texttt{updateLoc}=0$ and $\texttt{updateDFA}=0$\;
\While{accepting condition of NBA is not satisfied}{\label{rrt:sat}
%
\For{$j\in\ccalN^{\text{next}}$}{\label{rrt:for1}
Using $\sigma^{\text{next}}$ compute $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$; see \eqref{eq:localProb}\;}\label{rrt:compPaths}
Follow $\bbp_{j,t:T_j}$, re-plan if needed, and update  $M(t)$\;\label{rrt:ExecReplan}%(see Section \ref{sec:exec})
%
\If{$t=T$}{\label{rrt:T}
Update $q_B(t)=q_B^{\text{next}}$\;\label{rrt:updcurDFA}
Select a new NBA state $q_B^{\text{next}}$ and  $\sigma^{\text{next}}$\;\label{rrt:updTarget}
%
Compute new $L_j^{\text{next}}$ and the set of robots $\ccalN^{\text{next}}$\;\label{rrt:UpdGoals}
}
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\normalsize

Given the current NBA state $\bbq_B(t)$, the robots coordinate to select a new NBA state, denoted by $q_B^{\text{next}}$ that they should reach next to make progress towards accomplishing their task [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. This state is selected so that the transition from $q_B$ to $q_B^{\text{next}}$ is decomposable, as per Definition \ref{def:feas}, and progress towards reaching a final state is made. Therefore, the state $q_B^{\text{next}}$ is selected from the set $\ccalQ_{q_B(t)}^{\text{next}}$ based on the following two cases.
%
If $q_B(t)\notin \ccalQ_F^{\text{loop}}$, where $\ccalQ_F^{\text{loop}}$ is defined in \eqref{eq:accNode}, then among all the states in $\ccalQ_{q_B(t)}^{\text{next}}$ we select one that satisfies
%$q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}\subseteq \ccalQ_{B}^{\text{loop}}$

\begin{equation}\label{eq:minDist}
d(q_B^{\text{next}},q_F^{\text{loop}}) =  d(q_B(t),q_F^{\text{loop}})-1,    
\end{equation}
i.e., a state that is one hop closer to a given state $q_F^{\text{loop}}\in\ccalQ_F^{\text{loop}}$ than $q_B(t)$ is. The state $q_F^{\text{loop}}\in\ccalQ_F^{\text{loop}}$ is selected offline and used to guide planning towards traversing accepting edges infinitely often; see Definition \ref{def:accEdges}. Recall that $q_B^{\text{next}}\in\ccalQ_{q_B}^{\text{next}}\subseteq \ccalQ_{B}^{\text{loop}}$ and therefore, $d(q_B^{\text{next}},q_F)$ is well defined; see \eqref{eq:dist}. Under this policy of selecting $q_B^{\text{next}}$, we have that eventually $q_B(t)=q_F$; design of robot paths to ensure this property will be discussed next. If $q_B(t)=q_F^{\text{loop}}$, then the state $q_B^{\text{next}}$ is selected so that $(q_B(t),q_B^{\text{next}})$ is an accepting edge as per Definition \ref{def:accEdges}. This way we ensure that accepting edges are traversed infinitely often and, therefore, the assigned LTL task is satisfied.

%Note that there exists at least one $q_B^{\text{next}}$ that satisfies \eqref{eq:minDist} since any path (including the shortest path) in the pruned NBA that connects $q_B(t)$ to $q_F^{\text{feas}}$ goes through one of the states in $\ccalQ_{q_B(t)}^{\text{next}}$ by construction of the pruned automaton. %and the definition of the distance metric in \eqref{eq:dist}. 
%If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}].

%Given $q_B^{\text{next}}$


%every robot $j$ needs to locally design a path so that a DFA state that is closer to the final state $q_F$ than the current DFA state $q_D(t)$ is eventually reached. 
%The NBA state $q_B^{\text{next}}$ is selected as follows. First, we compute the distance $d(q_B(t),q_F^{\text{feas}})$, where $q_F^{\text{feas}}$ is a final NBA state that is selected offline and is reachable from its initial state $q_B^0$ in the pruned NBA, i.e., $d(q_B^0,q_F^{\text{feas}})\neq\infty$. Then, we select as $q_B^{\text{next}}$ a state that satisfies $d(q_B^{\text{next}},q_F^{\text{feas}}) < d(q_B(t),q_F^{\text{feas}})$,
%\begin{equation}\label{eq:targetDFA}
%   d(q_D^{\text{next}},q_F) = d(q_D(t),q_F) -1, 
%\end{equation}
%i.e., a state that is one hop closer to $q_F^{\text{feas}}$ than $q_B(t)$ is. If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}]. %; see  Sections \ref{sec:paths}. %or realize that a transition from $q_D(t)$ to $q_D^{\text{next}}$ is in fact infeasible; see next section.


%{\bf{Local Construction of Robot Paths:}}

To reach $q_B^{\text{next}}\in\ccalQ_{q_B(t)}^{\text{next}}$ the robots need to eventually generate a symbol from the set $\Sigma_{\text{dec}}^{q_B,q_B^{\text{next}}}$; this symbol can be selected randomly. %Among all such symbols $\sigma^{\text{next}}$, we select the one that yields the smallest set $\ccalN^{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
With slight abuse of notation, we denote the selected symbol by $\sigma^{\text{next}}$ [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. Also, for simplicity of notation we replace $b^{q_B(t),q_B^{\text{next}}}$ and $b^{q_B(t),q_B(t)}$ with $b^{\text{next}}$ and $b^{\text{inv}}$. The same notation extends to  the corresponding set of robots $\ccalR^{q_B(t),q_B^{\text{next}}}$, $\ccalN^{q_B(t),q_B^{\text{next}}}$, $\ccalR^{q_B(t),q_B(t)}$, and $\ccalN^{q_B(t),q_B(t)}$.

%with $\ccalR^{\text{next}}$ and $\ccalN^{\text{next}}$.


In what follows, we discuss how to design robot paths $\bbp_{j,t:T_j}$, for all robots $j$, that should be followed within a time interval $[t,T_j]$ to ensure that eventually $\sigma^{\text{next}}$ is generated. Given $\sigma^{\text{next}}$, we compute for each robot $j\in\ccalN^{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma^{\text{next}}$. Recall that for robots $j\in\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma^{\text{next}}$  while for robots $j\in\ccalN^{\text{next}}\setminus\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%
Every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%the state $q_B^{\text{next}}$ will be eventually reached and once $q_B^{\text{next}}$ is reached the robots can remain in $q_B^{\text{next}}$ until new observations are made (i.e., until atomic predicates are satisfied/violated). 
%
%For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b^{\text{inv}}$ and $b^{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.
%
%Given the NBA state $q_B^{\text{next}}$, our goal is to design paths $\bbp_{j,t:T_j}$, for all robots $j$ that should be followed within a time interval $[t,T_j]$ so that the NBA transition from $q_B(t)$ to $q_B^{\text{next}}$ is activated. %%\footnote{With slight abuse of notation the subscript in $\bbp_{j,t:T_j}$ denotes the index of robot and the time interval $[t,T_j]$ within which the path should be followed.} 
%To achieve that, it suffices to ensure that the robots follow paths that (i) satisfy the Boolean formula $b^{q_B(t),q_B(t)}$ that allows them to stay in the current NBA state $q_B(t)$, until (ii) the Boolean formula $b^{q_B(t),q_B^{\text{next}}}$ that enables transition from $q_B(t)$ to $q_B^{\text{next}}$ is satisfied while (iii) while never satisfying Boolean formulas $b^{q_B(t),q_B''}$ other than the ones that are satisfied at time $t$.\footnote{At time $t$, the Boolean formula $b^{q_B(t),q_B(t)}$ is satisfied by construction of the pruned automaton. Nevertheless, other Boolean formulas $b^{q_B(t),q_B''}$ may be satisfied as well due to the non-deterministic nature of the NBA.}  For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b^{\text{inv}}$ and $b^{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.
%
%\red{[add reference to lines of the algorithm]}
%To design paths $\bbp_{j,t:T_j}$, \textit{first} the robots $j\in\ccalN^{\text{next}}$ \textit{communicate} to select a symbol $\sigma^{\text{next}}$ that satisfies conditions (i)-(ii) of Definition \ref{def:feas} given the current symbol  $\sigma^{\text{inv}}=L(\bbp(t))$ they are generating. %; see also Example \ref{ex3}. Note that such a symbol exists by construction of the pruned NBA for any symbol $\sigma^{\text{inv}}$. 
%%% \footnote{Note that it is possible that given the symbol that the robots generated to reach $q_D$ there may not exist a pair of symbols $\sigma^{\text{inv}}$ and $\sigma^{\text{next}}$ to reach a state $q_D^{\text{next}}$ that satisfy condition (iii) of Def. \ref{def:feas}. In other words, transition from $q_D$ to $q_D^{\text{next}}$ may not be cast as a point-to-point navigation problem as in \eqref{eq:localProb}.
%Consider e.g., the DFA that corresponds to $\phi=\square(\pi_1^{r_0}\vee\pi_2^{r_0})\wedge\Diamond(\pi_1^{r_1})\wedge\Diamond(\pi_2^{r_2})$. 
%Existence of such symbols is always guaranteed for a sub-class of co-safe LTL formulas as discussed in Lemma \ref{lem:cnt}.} %that satisfy $b^{\text{inv}}$ and $b^{\text{next}}$, respectively, i.e., $\sigma^{\text{next}}\models b^{\text{next}}$. This pair of symbols is selected so that condition (ii) of Definition \ref{def:feas} is satisfied; 
%Among all such symbols $\sigma^{\text{next}}$, we select the one that yields the smallest set $\ccalN^{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
%
%Given $\sigma^{\text{next}}$, we compute the set $\ccalR^{\text{next}}$ that collect the robots that need to move towards certain regions of interest $r_e$ in workspace to generate $\sigma^{\text{next}}$. 
%
%\textit{Second}, given $\sigma^{\text{next}}$,  we compute for each robot $j\in\ccalN^{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma^{\text{next}}$. Recall that for robots $j\in\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma^{\text{next}}$  while for robots $j\in\ccalN^{\text{next}}\setminus\ccalR^{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%\textit{Third}, we design the paths $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ for all robots $j\in\ccalN^{\text{next}}$. %First, all robots $j\notin\ccalR^{\text{inv}}$ stay put at their current locations until the state $q_B^{\text{next}}$ is reached. %
%\textit{Third}, every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%that if followed the symbol  $\sigma^{\text{next}}\models b^{\text{next}}$ is generated and the DFA state $q_D^{\text{next}}$ is reached
%In Section \ref{sec:complOpt}, we show that the multi-robot state $\bbp(t)$ already generates a symbol that satisfies $b^{\text{inv}}$. We also show that if (i) the robots that are involved in generating $\sigma^{\text{inv}}$, collected in a set $\ccalR^{\text{inv}}$, stay idle at their current locations $\bbp_j(t)$ and (ii) all other robots 
%
%
%\footnotesize
\begin{subequations}
\label{eq:localProb}
\begin{align}
%& \min_{\substack{T_j, \bbu_{j,t:T_j}}} \left[J(T_j,\bbu_{j,t:T_j}) = \int_{t'=t}^{T_j}  w(\bbp_j(t'),\bbu_j(t'))dt \right] \label{ObjLoc2}\\
& \text{Compute:~}{T_j, \bbu_{j,t:T_j}}~\text{such that}  \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ [L(\bbp_j(t'))=L(\bbp_j(t))] \vee [L(\bbp_j(t'))=\varnothing] \nonumber\\
%& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \vee [L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}],~\forall t'\in[t,T_j] \label{constrLoc1} \\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \cup_i\set{r_i}\setminus (R_j^t\cup L_j^{\text{next}}), \forall t'\in[t,T_j] \label{constrLoc1}\\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \hat{O}(t), \forall t'\in[t,T_j] \label{constrLocObs}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j) \in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin \ccalA_j^{\text{avoid}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'+1),\bbu_j(t'+1)), \label{constrLoc3}
\end{align}
\end{subequations}
%\normalsize

\noindent In \eqref{constrLoc1}, $R_j^t$ denotes the region that robot $j$ lies in at time $t$. The first constraint \eqref{constrLoc1} requires that robot $j$ should not visit any region $r_i$ excluding $R_j^t$ and the target region $L_j^{\text{next}}$, for all $t'\in[t,T_j]$. If at time $t$ robot $j$ does not lie in any of the regions $r_i$, then $R_j^t=\emptyset$. This ensures that the multi-robot system can always remain in $q_B(t)$ as the robots $j\in\ccalN^{\text{next}}$ navigate the workspace; see Lemma \ref{lem:binv}. This constraint can be relaxed by requiring  robot $j\in\ccalN^{\text{next}}$ to always avoid only regions that may result in violating $b^{\text{inv}}$. For instance, if $b^{\text{next}}=\neg(\pi_j^{r_e}\wedge\pi_i^{r_e}$), then it suffices to require robot $j$ to never visit $r_e$.  %\footnote{$T_j^{-}$ denotes a time instant right before $T_j$, i.e., $T_j^{-}=T_j-\epsilon$, for an arbitrarily small $\epsilon>0$.} 
Similarly, the second constraint in \eqref{constrLocObs} requires robot $j$ to avoid all obstacles, collected in $\hat{O}(t)$, that are known up to the time instant $t$. The third constraint in \eqref{constrLoc2} requires robot $j$ to be in region $L_j^{\text{next}}$ at a time instant $T_j\geq t$. %so that it generates $L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}$.%\footnote{Note that this prevents the robot from visiting parts of $L_j^{\text{next}}$ that are shared with other regions $r_i$.} 
This is required to eventually generate the symbol $\sigma^{\text{next}}$. The last constraint in \eqref{constrLoc3} captures the robot dynamics. Note that among all paths that satisfy these constraints, the optimal one, as a per a user-specified motion cost function, can be selected. 
%\textit{Third}, every robot $j\in\ccalN^{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%In words, the optimal control problem \eqref{eq:localProb} requires robot $j$ to design a path $\bbp_{j,t:T_j}$ that reaches $L_j^{\text{next}}$ (see \eqref{constrLoc2}) while avoiding certain regions $r_i$ (see \eqref{constrLoc1}) and all detected obstacles denoted by $\hat{O}(t)$ (see \eqref{constrLocObs}). %Note that the robots that do not belong to $\ccalR^{\text{inv}}$ and also are not responsible to generate $\sigma^{\text{next}}$ do not have a target region $L_{j}^{\text{next}}$. These robots remain stationary in their current locations and they do not need to solve \eqref{eq:localProb}.
%
Observe that \eqref{eq:localProb} is a  point-to-point navigation problem, and, therefore, any of the traditional motion planning algorithms, such as $\text{A}^*$, RRT, $\text{RRT}^*$, RRG, or PRM, can be used to solve it \cite{karaman2011sampling}. Finally observe that given $L_j^{\text{next}}$, robot $j$ locally solves \eqref{eq:localProb} without communicating with any other robot. %Also, since the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable as per Definition \ref{def:feas}, there are no conflicts where a robot would have to stay idle at its current location and at the same time move towards a new location as per the solution to \eqref{eq:localProb}; see also Lemma \ref{lem:binv}. %there is no robot $j$ that belongs to $\ccalR^{\text{inv}}$ that is required to stay idle
%
%Correctness of Alg. \ref{alg:RRT} is discussed in Sec. \ref{sec:complOpt}. %Feasibility of such this problem is examined in 

%We design such paths in two stages. In the first stage, we design subpaths $\bbp_{j,t:\bar{T}_j}$ for some $t<\bar{T}_j<T$ and in the second stage we design paths $\bbp_{j,\bar{T}_j:T_j}$. In particular, \textit{in the first stage} all robots that are involved in generating $\sigma^{\text{inv}}$, collected in a set $\ccalR^{\text{inv}}$, and all other robots $j$ for which it hold $L(\bbp_j(t))=\varnothing$ (i.e., they are outside of all regions $r_i$) stay idle at their current locations $\bbp_j(t)$, i.e., $\bar{T}_j=t+1$ and $\bbp_{j,t:\bar{T}_j}=[\bbp_j(t),\bbp_j(t)]$ All other robots $j$ (i.e., the ones that satisfy $j\notin\ccalR^{\text{inv}}$ and $L(\bbp_j(t))\neq \varnothing$) solve the following optimal control problem to design paths $\bbp_{j,t:\bar{T}_j}$ that if followed then the robots will move outside the regions that they are currently located. %As it will bbe discusses in Section \ref{sec:exec}, these subpaths will be executed so that the robots will move outside their current regions simultaneously.

%\begin{subequations}
%\label{eq:localProb1}
%\begin{align}
%& \min_{\substack{\bar{T}_j, \bbu_{t:\bar{T}_j}}} \left[J(\bar{T}_j,\bbu_{t:\bar{T}_j}) = \sum_{t'=t}^{\bar{T}_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc1}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in R_j(t), \forall t\in\set{t,\dots,\bar{T}_j-1} \label{constrLoc1a} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in \ccalR_j^{\text{inv}}, \forall t\in\set{t,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(\bar{T}_j))=\varnothing \label{constrLoc2a}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   %\bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc2}
%\end{align}
%\end{subequations}
%where $R_j(t)$ denotes the region $r_i$ that robot $j$ lies in at time $t$. Observe that the first two constraints \eqref{constrLoc1a}-\eqref{constrLoc2a} require robot $j$ to move outside the region $\ccalR_j(t)$ where it is located at the time instant $t$. This happens at a time instant $\bar{T}_j$, i.e., $L(\bbp_j(\bar{T}_j))=\varnothing$. Note that robot $j$ locally solves \label{eq:localProb1} with communicating with other robots. Observe that execution of these subpaths ensures that the robots remain in the DFA state $q_D(t)$ since $b^{\text{inv}}$ is always satisfied as the robots $\ccalR^{\text{inv}}$ remain stationary in their current locations that generates  $\sigma^{\text{inv}}\models b^{\text{inv}}$.

%since the robots in $\ccalR^{\text{inv}}$

%In the \textit{second} stage, we construct the subpaths $\bbp_{j,\bar{T}_j:T_j}$ that will enable the transition from $q_D(t)$ to $q_D^{\text{next}}$. For robots $j\in\ccalR^{\text{inv}}$, we select $T_j=\bar{T}_j+1$ and $\bbp_{j,\bar{T}_j:T_j}=[\bbp_{j}(t),\bbp_{j}(t)]$, i.e., these robots still stay idle. In fact, due to the deterministic structure of the DFA, this ensures that the robots remain in the DFA state $q_D(t)$ until the symbol $\sigma^{\text{next}}$ is generated which will activate the transition towards $q_D^{\text{next}}$. To generate the symbol  $\sigma^{\text{next}}$, all other robots $j\notin\ccalR^{\text{inv}}$ design paths $\bbp_{j,\bar{T}_j:T_j}$ by solving the following optimal control problem:

%\begin{subequations}
%\label{eq:localProb}
%\begin{align}
%& \min_{\substack{T_j, \bbu_{\bar{T}_j:T_j}}} \left[J(T_j,\bbu_{\bar{T}_j:T_j}) = \sum_{t'=\bar{T}_j}^{T_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ L(\bbp_j(t'))=\varnothing, \forall t'\in\set{\bar{T}_j,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
%\end{align}
%\end{subequations}



 %This ensures that  transition to a DFA state $q_D'\neq q_D(t)$ that is not $q_D^{\text{next}}$. 
%In the meantime the robots in $\ccalR^{\text{inv}}$ ensure that the current DFA state remain the same in $[t,\bar{T}-1]$, since they stay idle and generate the symbol $\sigma^{\text{inv}}$. Also note that robots in $\ccalR^{\text{inv}}$ do not belong to the set of robots that need to move to another location to generate the symbol $\sigma$, since that would create a conflict; see also Remark \ref{rem:invariant}. 
%The second constraint in \eqref{constrLoc2} requires that at time instant $T_j$, all robots should be in their corresponding locations $L_j^\textbf{}$. Once this happens the symbol $\sigma^{\text{next}}$ is generated and the target DFA state is reached.
%
%Note that infeasibility of \eqref{eq:localProb} is due to the facts (i) the environment is unknown and, therefore, it is not possible to check offline which DFA transitions cannot be enabled because e.g., of the robot dynamics or the existence of obstacles.%; and (ii) the LTL formula $\phi$ is decomposed into local sub-tasks Problem \ref{prob} is solved in a distributed the proposed algorithm is distributed nature of the proposed 

%What if the problem is infeasible? update $\sigma$ i.e., $L_j$. If no other $L_j$. update target DFA state. If no other target DFA state report `current method failed (this does not mean that the task is unsatisfiable though)'

%\begin{ex}[Selection of $\sigma^{\text{next}}$ and $\sigma^{\text{inv}}$]\label{ex3}
%Consider the Boolean formulas $b^{\text{inv}}=\neg \pi_{\text{obs}}$ and $b^{\text{next}}=(\pi_j^{r_1}\vee \pi_j^{r_3} )\wedge\pi_e^{r_2}\wedge (\neg \pi_j^{r_2}) \wedge (\neg (\pi_j^{r_1}\wedge \pi_e^{r_1}))$, where the atomic predicate $\pi_{\text{obs}}$ is true of at least one robot hits an obstacle. A symbol $\sigma^{\text{next}}$ that satisfies $b^{\text{next}}$ is $\sigma^{\text{next}}=\pi_j^{r_1}\pi_e^{r_2}$ while $b^{\text{inv}}$ is satisfied by an empty string, i.e., $\sigma^{\text{inv}}=\varnothing$. Given this pair of symbols, we have that $\ccalR^{\text{inv}}=\emptyset$, $\ccalR^{\text{next}}=\set{j,e}$, $L_j^{\text{next}}=r_1$, and $L_e^{\text{next}}=r_2$.
%\end{ex}

%\begin{ex}[Construction of $\sigma^{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b^{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$. Then, we have that $\sigma^{\text{inv}}=\pi_j^{r_1}$ and $\ccalR^{\text{inv}}=\set{j}$. Similarly, if $b^{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma^{\text{inv}}$ is an empty string and $\ccalR^{\text{inv}}=\emptyset$.
%\end{ex}

%\begin{ex}
%--add automaton figure--and explain--
%\end{ex}
%\begin{rem}[Initialization of $q_B(t)$]
%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}
%\end{rem}
\subsection{Reacting to Map Uncertainty}\label{sec:exec}
%{\bf{Reactive Planning to Map Uncertainty:}}

As the robots follow their paths $\bbp_{j,t:T_j}$, the map $M(t)$ is continuously updated, as per \eqref{eq:updMap}, and the robot paths need to be accordingly revised [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. In fact, reactivity to the environment is required in two cases. First, as the robots follow their paths $\bbp_{j,t:T_j}$, they may discover new obstacles based on their sensor measurements; see \eqref{eq:sensor}. If the discovered obstacles intersect with their paths $\bbp_{j,t:T_j}$, for some $j\in\ccalR^{\text{next}}$, then these robots $j$ locally re-solve \eqref{eq:localProb} using the updated map to design new paths. Note that existing reactive planning algorithms that can address reachability navigation problems in the presence of unknown obstacles can also be used to solve \eqref{eq:localProb}; see e.g., \cite{guzzi2013human,vasilopoulos2018sensor,bansal2019combining,ryll2019efficient}.

%is not reachable e.g., due to the robot dynamics or 
Second, as the the map $M(t)$ is constructed, goal regions $L_j^{\text{next}}$ may become unreachable because of the structure of the environment (e.g., regions of interest may be surrounded by obstacles). In this case, robots $j$ that cannot reach $L_j^{\text{next}}$ communicate with all other robots so that a new symbol $\sigma^{\text{next}}$ is selected. This process is repeated until a reachable region $L_j^{\text{next}}$ is selected.  %that makes \eqref{eq:localProb} feasible. 
If such a symbol $\sigma^{\text{next}}$ does not exist, then this means that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$, due to the a-priori unknown structure of the environment. Then, the pruned NBA is updated by removing this transition and a new NBA state $q_B^{\text{next}}$ is selected. If there do not exist any candidate NBA states to be selected as $q_B^{\text{next}}$, then the assigned task cannot be accomplished given the current multi-robot and NBA state. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
In fact, there may exist another sequence of NBA states for which Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible (i.e., paths towards selected goal regions always exist) and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.

%\begin{rem}[Feasibility of \eqref{eq:localProb}]
%Observe that \eqref{eq:localProb} may be \textit{infeasible}. This can be the case e.g., if the region $L_j^{\text{next}}$ is not reachable e.g., due to the robot dynamics or the structure of the environment. In this case, robot $j$ needs to communicate with all other robots so that a new symbol $\sigma^{\text{next}}$ is selected. This process is repeated until regions $L_j^{\text{next}}$ are selected that make \eqref{eq:localProb} feasible. If such a symbol $\sigma^{\text{next}}$ does not exist, then this means that the transition from $q_D(t)$ to $q_D^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$. Then, the pruned DFA is updated by removing this transition. Next, a new target DFA state is selected that is closer to the final state $q_F$ than $q_D(t)$ is. If there do not exist such DFA states then the robots cannot accomplish the assigned task. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
%In fact, there may exist another sequence of DFA states for which  Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
%Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.
%\end{rem}

%{\bf{Asynchronous Execution of Paths:}} 
\subsection{Asynchronous Execution of Paths}
The robots $j\in\ccalR^{\text{next}}$ execute their paths $\bbp_{j,t:T_j}$ \textit{asynchronously} until the time instant $T_j$, i.e., until they reach their respective target regions $L_j^{\text{next}}$ [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. At time $T_j$, robot $j$ waits for all other robots $e\in\ccalR^{\text{next}}$ with $T_e>T_j$. At time instant $T=\max_{j\in\ccalN^{\text{next}}}\{T_j\}$, i.e., when \textit{all} robots $j\in\ccalN^{\text{next}}$ have reached their respective regions $L_j^{\text{next}}$, the symbol $\sigma^{\text{next}}$ is generated. Then, the multi-robot system reaches the NBA state $q_B^{\text{next}}$ and a new NBA state is selected [lines \ref{rrt:T}-\ref{rrt:UpdGoals}, Alg. \ref{alg:RRT}]. This process is repeated indefinitely so that a final state is reached infinitely often [line \ref{rrt:sat}, Alg. \ref{alg:RRT}].
%In Section \ref{sec:complOpt}, we show the robots remain in the NBA state $q_B(t)$ for all  $t'\in [t, T-1]$ and transition to $q_B^{\text{next}}$ occurs at the time instant $T$. Once this happens, the robots update their current DFA state and select the next DFA state [lines \ref{rrt:T}-\ref{rrt:UpdGoals}]. This process is repeated until the final state $q_F$ is reached.

%
%\begin{rem}\label{rem:invariant}
%Note that once the robots reach a new DFA $q_D$, they satisfy its respective Boolean condition $b^{\text{inv}}$, since the `next' temporal operator is excluded from the task specification. Particularly, if $b^{\text{inv}}$ is not satisfied this implies that once the robots are at locations that generate a symbol that triggers the transition to $q_D$, the robots should immediately leave their locations, which is impossible to specify unless the next operator is included in the specification language. 

%Recall that $\sigma^{\text{inv}}$ is selected to have the minimum length, this means that the minimum number of robots are involved to generate it. Therefore, robots that are required to generate the symbol $\sigma$ are not included in the set $\ccalR^{\text{inv}}$; see also Remark \ref{rem:invariant}.
%Similarly, robots that are responsible to satisfy $b^{\text{next}}$ cannot be responsible for generating the symbol $\sigma^{\text{inv}}$, since the next operator does not exist and all regions are assumed to be disjoint. %(unless there is an overlap..)
%\end{rem}


%\subsection{Online Re-planning}\label{sec:replan}






\begin{rem}[Communication]
%Note that Algorithm \ref{alg:RRT} requires all-time communication to ensure that all robots always have access to the same map $M(t)$. Nevertheless, this requirement can be straightforwardly relaxed by allowing each robot to build their local map $M_j(t)$. Moreover, 
Execution of the paths $\bbp_{j,t:T_j}$ does not require all-time communication among robots, which is typically the case in relevant temporal logic algorithms. Instead, communication is intermittent and is required only in the following two cases: (i) all robots need to communicate with each other to select and update the symbol $\sigma^{\text{next}}$ (ii) every robot $j\in\ccalR^{\text{next}}$ needs to send a message to all other robots in $\ccalR^{\text{next}}$ once it has reached region $L_{j}^{\text{next}}$. %; see Section \ref{sec:exec}.
\end{rem}

%Next, we define the set $\ccalL_j$ that collects all robot positions $\bbp_j$ that violate $b^{\text{inv}}$ regardless of the state of all other robots. For instance, if $b^{\text{inv}}=\neg (\pi_j^{r_e}\wedge \pi_z^{r_h})$, then $\ccalL_j=\emptyset$. On the other hand, if $b^{\text{inv}}=\neg (\pi_j^{r_e})\wedge (\neg \pi_z^{r_h})$ then  $\ccalL_j=\set{r_e}$. Formally, to construct the set, we express the negation of $b^{\text{inv}}$, denoted by $\bar{b}^{\text{inv}}=\neg b^{\text{inv}}$ as




==> files/alg_final.tex <==




%ASSUMPTIONS

%Disjoint regions? no reachable regions? not in the PF but possibly needed to ensure completeness separable regions? only for completeness


%%%%%%%%







%%%%%%%%%


%\subsection{Planning for Information Acquisition}
%\red{(we need figures)}

Problem \ref{prob} can be solved by applying existing abstraction-free approaches for LTL planning, e.g., \cite{vasile2013sampling,luo2019abstraction}, at runtime to continuously update the robot paths as the map of the environment is continuously learned. Nevertheless, such methods require searching over a large product automaton space, a task that is computationally challenging to perform at runtime. To mitigate this challenge, we propose a new reactive LTL planning algorithm summarized in Algorithm \ref{alg:RRT} that does not rely on searching over a product automaton space. The main idea of Algorithm \ref{alg:RRT} is to decompose the temporal logic task into a sequence of local point-to-point navigation problems that are formulated and solved online while adapting to the updated map $M(t)$ of the environment.
%

\subsection{From LTL formulas to Automata}



To this end, first, we translate the specification $\phi$, constructed using a set of atomic predicates $\mathcal{AP}$, into a Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA), defined as follows \cite{baier2008principles} [line \ref{rrt:dfa}, Alg. \ref{alg:RRT}]. %Given a temporal logic formula $\phi$ , with syntax and semantics as described in Definitions \ref{syntax} and \ref{semantics}, respectively, a DFA is defined as follows:

\begin{definition}[NBA]
A Non-deterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\rightarrow_B, \ccalQ_F\right)$, where (i) $\ccalQ_{B}$ is the set of states;
(ii) $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is the initial state; (iii) $\rightarrow_B:\ccalQ_B\times\Sigma\rightarrow\ccalQ_B$ is a non-deterministic transition relation, and $\ccalQ_F\subseteq\ccalQ_{B}$ is a set of accepting/final state. 
\end{definition}

To interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\mathbb{R}^{n\times N}\times M(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current multi-robot state $\bbp(t)\in\mathbb{R}^{n\times N}$ and the current map $M(t)$ of the environment. An infinite-length discrete plan $\tau=\bbp(0)\bbp(1)\dots$ satisfies $\phi$, denoted by $\tau\models\phi$, if the word $\sigma=L(\bbp(0), M(0))L(\bbp(1),M(1))\dots$ yields an accepting NBA run defined as follows.\footnote{Hereafter, for simplicity we denote $L(\bbp(t),M(t))$ by $L(\bbp(t))$.} First, a run of $\rho_B$ of $B$ over an infinite word $\sigma=\sigma(1)\sigma(2)\dots\sigma(t)\dots\in(2^{\mathcal{AP}})^{\omega}$, is a sequence $\rho_B=q_B(0)q_B(1)q_B(2)\dots,q_B(t),\dots$, where $q_B(0)\in\ccalQ_B^0$ and $(q_B(t),\sigma(t),q_B(t+1)\in\rightarrow_B$, $\forall t\in\mathbb{N}$. Hereafter, we equivalently denote $(q_B(t),\sigma(t),q_B(t+1)\in\rightarrow_B$ as $q_B(t)\rightarrow_B q_B(t+1)$. A run $\rho_B$ is called \textit{accepting} if $\texttt{Inf}(\rho_B)\cap\ccalQ_F\neq\emptyset$, where $\texttt{Inf}(\rho_B)$ represents the set of states that appear infinitely often in $\rho_B$. In words, an infinite-length discrete plan $\tau$ satisfies an LTL formula $\phi$ if its corresponding NBA run visits at least one of the final states infinitely often.
%The symbols $\sigma$ that result in an accepting run of $D$ constitute the accepted language of $D$.

%The proposed reactive algorithm builds online (i.e., as the robots navigate the environment) paths that live in the infinite-dimensional space $\Omega^N\times\ccalQ_D$. The synthesized paths are updated as the map of the environment is updated. 
Next, we use the NBA to guide planning in a distributed way towards regions of interest that contribute to satisfaction of the assigned LTL task; see Algorithm \ref{alg:RRT}. %Specifically, let $q_B(t)\in\ccalQ_B$ denote the NBA state that the multi-robot system has reached at time $t$ given all observations that have been made (i.e., all atomic predicates that have been satisfied) until $t$, where $q_B(0)\in\ccalQ_B^0$ [line \ref{rrt:t0}, Alg. \ref{alg:RRT}]. 
Specifically, at any time $t$, given the NBA state $q_B(t)$ that the robots have reached given all observations that have been made (i.e., all atomic predicates that have been satisfied) until time $t$, where $q_B(0)\in\ccalQ_B^0$, the robots navigate the environment so that they make progress towards accomplishing the assigned task.
%eventually visit a new NBA state, denoted by $q_B^{\text{next}}$, i.e., they make progress towards accomplishing the assigned task. 
To this end, once the robots reach a state $q_B(t)$, they collaboratively select a new NBA state, denoted by $q_B^{\text{next}}$, that they should eventually reach. The state $q_B^{\text{next}}$ is selected so that it is (i) one-hop reachable from $q_B(t)$, (ii) `closer' to the final states than $q_B(t)$ is according to a distance function defined over the NBA, and (iii) observations that can trigger a transition from $q_B(t)$ to $q_B^{\text{next}}$ can be `physically' generated by the robots; for instance, a transition from $q_B(t)$ to $q_B^{\text{next}}$ cannot be generated if it requires a robot to be present in more than one location simultaneously. Given the state $q_B^{\text{next}}$, the robots move towards locations in the workspace that will trigger the transition from $q_B(t)$ to $q_B^{\text{next}}$. In the meantime, the robots update the current map $M(t)$ and revise their paths, if needed, to avoid previously unseen obstacles. This process is repeated so that at least one of the final NBA states is visited infinitely often, i.e., the LTL task is accomplished. In what follows, we describe these steps in detail.%Once this transition is enabled, the robots update the target DFA state $q_D^{\text{next}}$ until they reach a final DFA state.%\footnote{In case the DFA has more than one initial state, then there is more than one state $\bbq(0)$ that can be used as a root. In this case, a separate tree is build for each one of possible roots.}
%For this, we assume that the initial robot configuration allows the robots to stay in $q_B(0)$.
%

%By convention the cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = 0$, while the cost of a node $\bbq(t+1)=[\bbp(t+1), q_D]\in\ccalV$, given its parent node $\bbq(t)=[\bbp(t),q_D']\in\ccalV$, is computed as 
%\begin{equation}\label{eq:costUpd}
%J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq(t)) +  w(\bbp(t),\bbp(t+1)).
%\end{equation}
%Observe that by applying \eqref{eq:costUpd} recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:Prob2}.

 
%Given the current DFA state $q_D(t)$, the robots first select a DFA state $q_D^{\text{next}}\in\ccalQ_D$ that is `closer' to the final state $q_F$ than $q_D(t)$ is and observations that generate a transition from $q_D(t)$ to $q_D^{\text{next}}$ can be generated. Therefore,
%\subsection{Selecting the Next DFA State}\label{sec:targetDFA}

%{\bf{Pruning the DFA:}}
\subsection{Pruning the NBA}\label{sec:prune}
Given the current NBA state $q_B(t)$, a new state $q_B^{\text{next}}$ is selected so that it is closer to the final states. Thus, to select $q_B^{\text{next}}$, we need to define a distance function over the state-space of the NBA that measures how far each state is from the final state. %(in terms of the number feasible transitions/hops required to reach $q_F$). 
To achieve that, we first prune the NBA $B$ by removing transitions that cannot be enabled [line \ref{rrt:prune}, Alg. \ref{alg:RRT}]. %This is required to define a distance function over the state-space of the DFA. %
%
Specifically, the pruned NBA is constructed by removing all infeasible NBA transitions. To formally define the \textit{feasible/infeasible} DFA transitions we first need to introduce the following definitions. %\cite{kantaros2018text}.
%
%We also rewrite $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$ as follows:
%\begin{equation}\label{eq:eq1}
%    b_{\text{inv}}^{q_D} = b_{\text{inv}}^{\text{goal}} \triangle (\neg b_{\text{inv}}^{\text{avoid}} ),
%\end{equation}

%\begin{equation}\label{eq:eq2}
%    b_{\text{next}}^{q_D,q_D'} = b_{\text{next}}^{\text{goal}} \triangle (\neg b_{\text{next}}^{\text{avoid}} ),
%\end{equation}
%where in the Boolean formulas  $b_{\text{next}}^{\text{goal}}$, $b_{\text{next}}^{\text{avoid}}$, $b_{\text{inv}}^{\text{goal}}$ and $b_{\text{inv}}^{\text{avoid}}$ the negation operator does not appear in front of any atomic proposition. Also, in \eqref{eq:eq1} and \eqref{eq:eq2}, $\triangle$ denotes either the logical AND ($\wedge$) or the logical OR $(\vee)$ operator.

% defined in \ref{defn:wTS}.%\footnote{Recall from Definition \ref{defn:wTS} that $\text{wTS}_i$ is defined over $\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma_i=2^{\mathcal{AP}_i}$. Also, recall from Definition \ref{def:pts} that the PTS is defined over $\mathcal{AP}=\bigcup_{i=1}^N\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma=2^{\mathcal{AP}}$. Also, throughout the paper, we denote the finite symbols by $\sigma^*\in\Sigma$ and the infinite symbols by $\sigma\in\Sigma^{\omega}$.}
\begin{definition}[Feasible symbols $\sigma_j\in\Sigma_j$]\label{defn:infTSi}
A symbol $\sigma_j\in\Sigma_j:=2^{\mathcal{AP}_j}$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, where $b_j^{\text{inf}}$ is a Boolean formula defined as 
\begin{equation}\label{bInfTSi}
b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e}(\pi_j^{r_i}\wedge\pi_j^{r_e})).
%b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e})),
\end{equation}
where $b_j^{\text{inf}}$ requires robot $j$ to be present simultaneously in more than one disjoint region.
\end{definition}

%We also need to define when a symbol $\sigma\in\Sigma$ is \textit{feasible}, i.e., when it can be generated by the multi-robot system. To this end, we first need to define the
%In other symbols $\sigma_j\in\Sigma_j=2^{\mathcal{AP}_j}$ that are feasible, i.e, the symbols that can be generated by robot $j$ \cite{kantaros2018text}. 


Note that the Boolean formula $b_j^{\text{inf}}$ is satisfied by any finite symbol $\sigma_j\in\Sigma_j$ that requires robot $j$ to be present in two or more disjoint regions, simultaneously. For instance, the symbol $\sigma_j=\pi_j^{r_i}\pi_j^{r_e}$ satisfies $b_j^{\text{inf}}$ if $r_i$ and $r_e$ are disjoint regions. %\footnote{Note that if we consider regions $r_i$ that are not necessarily disjoint, then the Boolean formula $b_j^{\text{inf}}$ is defined as $b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e}))$. Note also that definition of infeasible symbols depends on the problem at hand, i.e, the definition of atomic propositions included in the sets $\mathcal{AP}_j$.} % if there is an overlap between regions $r_i$ and $r_e$. 
Next, we define the feasible symbols $\sigma\in\Sigma$.

\begin{definition}[Feasible symbols $\sigma\in\Sigma$]\label{defn:infPTS}
A symbol $\sigma\in\Sigma$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, for all robots $j$,
where $\sigma_j=\Pi|_{\Sigma_j}\sigma$, $b_j^{\text{inf}}$ is defined in \eqref{bInfTSi}, and $\Pi|_{\Sigma_j}\sigma$ stands for the projection of the symbol $\sigma$ onto $\Sigma_j$.\footnote{For instance, $\Pi|_{\Sigma_j}(\pi_j^{r_e}\pi_m^{r_h})=\pi_j^{r_e}$.} We denote by $\Sigma_{\text{feas}}\subseteq\Sigma$ the set of all feasible symbols $\sigma\in\Sigma$. 
\end{definition}


%%%
%%%
%Next, we define the $\Sigma(q_D)=\{s\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D)\in\rightarrow_D)\}$ that collects all symbols that the robots can generate to remain in the state $q_D$. We also define the set $\Sigma(q_D,q_D')=\{\sigma\in 2^{\mathcal{AP}}|(q_D,\sigma,q_D')\in\rightarrow_D)\}$ that collects all symbols that enable a transition from $q_D$ to $q_D'$.
%
%Moreover, for each state $q_D$, we define the set $\Sigma(q_D|p)$ that collects all symbols $\sigma$ that robots may observe if they reach $q_D$ through a path $p=q_D^0,\dots,q_D$, i.e., a sequence of states in $\ccalQ_D$ that starts at the initial state $q_D^0$ and ends at the state $q_D$. Note that there may be multiple paths that can reach $q_D$ from $q_D^0$ and, therefore, each state $q_D$ may be associated with more than one set $\Sigma(q_D|p)$. For the initial state, $q_D^0$, there is only one such set  defined as $\Sigma(q_D^0|p)=\Sigma(q_D^0)$, since in a DFA the only path $p$ to reach $q_D^0$ from $q_D^0$ is the self-loop of $q_D^0$.

%To prune the DFA we need first to construct the sets $\Sigma(q_D|p)$. Starting from $q_D^{0}$, we execute the following process for each state $q_D$ that is reachable within one hop from $q_D^0$

%First, we select a state $q_D\in\ccalQ_D$, for which all corresponding sets $\Sigma(q_D|p)$ have been constructed
%%%
%%%
%\red{unclear here..}
%To solve Problem \ref{prob}, we first decompose the assigned task into local point-to-point planning problems. Motion plans that solve these point-to-point navigation problems are locally designed online while adapting to the map of the environment that is built by the robots. The proposed algorithm is summarized in Algorithm \ref{alg:RRT}. 
%


\begin{algorithm}[t]
%\footnotesize
\caption{Pruning a NBA}
\LinesNumbered
\label{alg:prune}
\KwIn{NBA}
\KwOut{Pruned NBA}
Remove transitions that are activated only by infeasible symbols (see Definition \ref{defn:infPTS})\label{prune:inf}\;
Collect all states $q_B\in\ccalQ_B$ for which a self-loop does not exist in the set $\hat{\ccalQ}_B$\label{prune:noloop}\;
Collect in a set $\ccalP_{q_B}=\{[(q_B^{\text{in},n},q_B),(q_B,q_B^{\text{out},m})]\}_{n=1,m=1}^{n=\bar{n},m=\bar{m}}$ \;%all possible pairs of incoming and outgoing transitions associated with
\For{$q_B\in\ccalQ_B$}{\label{prune:for1}
    \For{each pair in $\ccalP_{q_B}$}{
    Replicate $q_B$ so that its copy has only one incoming and only one outgoing transition as per the selected pair of edges\;\label{prune:repl}
    Remove the pair of edges from $\ccalP_{q_B}$\;\label{prune:rem}} 
}
\For {$q_B\in\ccalQ_B$ with $\Sigma^{q_B,q_B}\neq\emptyset$}{
Apply Definition \ref{def:feas}
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\begin{algorithm}[t]
%\footnotesize
\caption{LTL Planning in Unknown Environments}
\LinesNumbered
\label{alg:RRT}
\KwIn{ (i) initial robot configuration $\bbp(0)\models b^{q_B^0,q_B^0}$, (ii) LTL formula $\phi$}
%\KwOut{Terminal horizon $H$, and control inputs $\bbu_{0:H}$}
Convert $\phi$ into a DFA\label{rrt:dfa}\;
%Initial state $\bbq(0)=[\bbp(0), q_D^0]$;\label{rrt:init}
Initialize $t=0$, $q_D(0)=q_D^0$\;\label{rrt:t0}
%Update current DFA state as $q_D(0)=\delta(q_D^0,L(\bbp(0)))$\;
Prune DFA\;\label{rrt:prune}
%Select an initial state $q_D(0)=q_D^0$ and a feasible final state $q_F^{\text{feas}}$\;\label{rrt:feasFinal}
%Current DFA state $q_D(t)=q_D^0$\;\label{rrt:init}
%Compute distance from $q_D(t)$ to $q_D^F$\;
%\If{$d(q_D^0, q_F)= \infty$}{\label{rrt:unsat1}
%Error message: \textit{$\phi$ cannot be satisfied (see Proposition \ref{prop:sat})}\;}\label{rrt:unsat2}
Select the next DFA state $q_D^{\text{next}}$ that should be reached\;\label{rrt:selTarget}%(see \eqref{eq:targetDFA})
Compute $L_j^{\text{next}}$ and the set of robots $\ccalR_{\text{next}}$\;\label{rrt:goals}
%Initialize $\texttt{updateLoc}=0$ and $\texttt{updateDFA}=0$\;
\While{$q_B(t)\neq q_F$}{
%
\For{$j\in\ccalR_{\text{next}}$}{\label{rrt:for1}
Compute $\bbp_{j,t:T_j}$ as per \eqref{eq:localProb}\;}\label{rrt:compPaths}
Execute paths $\bbp_{j,t:T_j}$, re-plan if needed, and update map $M(t)$\;\label{rrt:ExecReplan}%(see Section \ref{sec:exec})
%
\If{$t=T$}{\label{rrt:T}
Update $q_D(t)=q_D^{\text{next}}$\;\label{rrt:updcurDFA}
Select a new DFA state $q_D^{\text{next}}$\;\label{rrt:updTarget}
%
Compute new $L_j^{\text{next}}$ and the set of robots $\ccalR_{\text{next}}$\;\label{rrt:UpdGoals}
}
}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\normalsize


Next, we define the sets that collect all feasible symbols that enable a transition from an NBA state $q_B$ to another, not necessarily different, NBA state $q_B'$. This definition relies on the fact that transitions among automaton states are enabled if Boolean formulas, denoted by $b^{q_B,q_B'}$ and defined over the set of atomic predicates $\mathcal{AP}$, are satisfied.  %The set of all atomic predicates associated with robots $j\in\mathcal{N}_{q_B,q_B'}$ is defined by $\mathcal{AP}_{q_B,q_B'}=\bigcup_{j\in\mathcal{N}_{q_B,q_B'}}\mathcal{AP}_j$.

\begin{definition}[Sets of Feasible Symbols]
Let $\mathcal{AP}_{q_B,q_B'}$ be a set that collects all atomic predicates that appear in the Boolean formula $b^{q_B,q_B'}$ associated with an NBA transition $q_B\rightarrow q_B'$. Given $b^{q_B,q_B'}$, we define the set $\Sigma^{q_B,q_B'}\subseteq 2^{\mathcal{AP}_{q_B,q_B'}}$ 
that collects all symbols $\sigma$ that (i) satisfy the corresponding Boolean formula $b^{q_B,q_B'}$, i.e., $\sigma\models b^{q_B,q_B'}$; and (ii) $\sigma\in\Sigma_{\text{feas}}$. %; and (iii) are associated with robots that appear in $b^{q_B,q_B'}$. 
%If the empty symbol $\varnothing$ satisfies (i), then $\Sigma^{q_B,q_B'}=\set{\varnothing}$. 
%The set $\mathcal{AP}_{q_B,q_B'}$ collects all atomic predicates that appear in $b^{q_B,q_B'}$.
\label{defn:feasSet}
\end{definition}

%Moreover, let $b_{\text{inv}}^{q_D}$ denote the Boolean formula that needs to be satisfied to enable a loop around $q_D$, i.e., a transition from $q_D$ to $q_D$.\footnote{Note that $b_{\text{inv}}^{q_D}$ exists for all states $q_D$, since the `next' operator is excluded from the syntax. Also, the Boolean formulas that should be satisfied to enable a  transition from a state $q_D$ to $q_D'$ can be provided by tools that convert temporal logic formulas to automata.} Let also $\Sigma_{\text{inv}}^{q_D}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b_{\text{inv}}^{q_D}$. 
%
%Let also $b_{\text{next}}^{q_D,q_D'}$ denote the Boolean formula that needs to be satisfied to enable a transition from $q_D$ to $q_D'$ and $\Sigma_{\text{next}}^{q_D,q_D'}\subseteq\Sigma$ be a set that collects all symbols that satisfy $b_{\text{next}}^{q_D,q_D'}$.
%Also, from $\Sigma_{\text{text}}^{q_D,q_D'}$, we exclude symbols associated with robots that do not play any role in satisfying $b_{\text{next}}^{q_D,q_D'}$. For instance, if $b_{\text{next}}^{q_D,q_D'}=\pi_j^{r_e}\vee\pi_j^{r_m}$, then $\Sigma_{\text{text}}^{q_D,q_D'}$ is defined as $\Sigma_{\text{text}}^{q_D,q_D'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$, i.e., it does not include any symbol associated with other robots $i\neq j$ that may also satisfy $b_{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_i^{r_f}$). The same also holds for $\Sigma_{\text{inv}}^{q_D}$; see also Example \ref{ex:feas}. %Additionally, in case the empty symbol, denoted by $\varnothing$ belongs to 
%
Given a Boolean formula $b^{q_B,q_B'}$, we define the set $\ccalN^{q_B,q_B'}\subseteq\ccalN$ that collects the indices of all robots that appear in $b^{q_B,q_B'}$. Also, given a symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$, we define the set $\ccalR^{q_B,q_B'}\subseteq\ccalN^{q_B,q_B'}$ that collects the indices $j$ of the robots that are involved in generating $\sigma_{q_B,q_B'}$. Also, we denote by $L_{j}^{q_B,q_B'}$ the location that robot $j\in\ccalN^{q_B,q_B'}$ should be located to generate $\sigma^{q_B,q_B'}$. Note that for robots $j\in\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$, $L_{j}^{q_B,q_B'}$ corresponds to any location $\bbq\in\Omega$ where no atomic predicates are satisfied; see also Example \ref{ex:exFeasSets}. 


%THE ROBOTS IN $\ccalN^{q_B,q_B'}\setminus\ccalR^{q_B,q_B'}$ GET OUT OF THEIR CURRENT REGIONS!

\begin{ex}(Sets of Feasible Symbols)
(a) Consider the Boolean formula $b^{q_B,q_B'}=(\pi_j^{r_e}\vee\pi_j^{r_m})\wedge(\neg \pi_i^{r_e})$, then $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\pi_j^{r_e},\pi_j^{r_m}, \pi_j^{r_e}\pi_j^{r_m}\}$. %, i.e., it does not include any symbol associated with other robots $k\neq j$ that may also satisfy $b_{\text{next}}^{q_D,q_D'}$ (as e.g., $\pi_j^{r_e}\pi_k^{r_f}$).
Given the Boolean formula $b^{q_B,q_B'}$, we have that $\ccalN^{q_B,q_B'}=\set{j,i}$.
%
Also, for $\sigma^{q_B,q_B'}=\pi_j^{r_e}$, we have that $\ccalR^{q_B,q_B'}=\set{j}$, $L_{j}^{q_B,q_B'}=r_e$. (b) Consider the Boolean formula $b^{q_B,q_B'}=\neg \pi_i^{r_e}$. In this case $\Sigma^{q_B,q_B'}$ is defined as $\Sigma^{q_B,q_B'}=\{\varnothing\}$, where $\varnothing$ denotes an empty symbol and is generated when a robot is outside all regions interests and does hit any obstacles. Also, we have that $\ccalN^{q_B,q_B'}=\set{i}$, $\sigma^{q_B,q_B'}=\varnothing$, $\ccalR^{q_B,q_B'}=\emptyset$, and while $L_{i}^{q_B,q_B'}$ corresponds to any location $\bbq$ in the workspace where no atomic predicates are satisfied. 
\label{ex:exFeasSets}
\end{ex}

Given the sets $\Sigma_{q_B,q_B'}$, we remove all NBA transitions with $\Sigma_{q_B,q_B'}=\emptyset$, i.e., all transitions that are require robots to be present in more than one locations in the environment simultaneously [line \ref{prune:inf}, Alg. \ref{alg:prune}]. Next we remove NBA transitions that require robots to move from one region of interest $\ell_i$ to another one $\ell_e$ without visiting any location $\bbq$ in the environment outside $\ell_i$. Such transitions are considered infeasible as they require robots to `jump' from one region of interest to another one.
%without robots to move to new regions of interest. Such transitions are removed as in practice they cannot be activated given that the regions of interest are disjoint. 
For instance, consider the LTL formula $\phi=\pi_1^{r_1}\ccalU\pi_1^{r_2}$ that requires robot $1$ to be in region $r_1$ until it enters $r_2$. The corresponding NBA is illustrated in Figure \ref{fig:NBA1}. Assume that the initial condition of the robot satisfies $b^{q_B^0,q_B^0}=\pi_1^{r_1}$, i.e., that robot $1$ is initially located in $r_1$. Then the transition from the initial to the final state is considered infeasible as it requires the robot to `jump' from one region of interest to another one. 

\begin{figure}
    \centering
     \includegraphics[width=0.6\linewidth]{figures/p1Up2.png}
    \caption{Example of an infeasible transition in the NBA corresponding to $\phi=\pi_1^{r_1}\ccalU\pi_1^{r_2}$. Transition from the initial state $q_B^0$ to the final state $q_B^F$ is infeasible as robot $1$ is required to `jump' from $\ell_1$ to $\ell_2$ while $\ell_1$ and $\ell_2$ are disjoint regions.}
    \label{fig:NBA1}
\end{figure}

\begin{figure}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Original NBA]{
    \label{fig:origNBA}
  \includegraphics[width=0.48\linewidth]{figures/feas1_bf.png}}
  \subfigure[Pruned NBA (Def. \ref{defn:feasSet})]{
    \label{fig:feas1}
  \includegraphics[width=0.34\linewidth]{figures/feas1_after.png}}
%  \caption{FEASIBLE 1}
%  \label{fig:tow7}
%\end{figure}
%
%\begin{figure}[t]
%  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Replicating NBA states]{
    \label{fig:repl}
  \includegraphics[width=0.5\linewidth]{figures/feas2_after.png}}
  \subfigure[Pruned NBA (Def. \ref{def:feas})]{
    \label{fig:finalPrune}
  \includegraphics[width=0.42\linewidth]{figures/feas2_pruned.png}}
  \caption{Graphical illustration of Algorithm \ref{alg:prune} applied to the NBA corresponding to $\phi=\square\Diamond(\pi_1^{\ell_1})\wedge\square\Diamond(\pi_1^{\ell_2})$. This formula requires robot $1$ to visit infinitely often $\ell_1$ and $\ell_2$. Figure \ref{fig:origNBA} shows the NBA   where the red dashed transitions are removed, as per Definition \ref{defn:feasSet}, as they require robot $1$ to be in $\ell_1$ and $\ell_2$ simultaneously yielding the pruned NBA shown in Figure \ref{fig:feas1}. Observe in Figure \ref{fig:feas1} that there is no self-loop for the final state $q_F$. Thus, $q_F$ is replicated twice since it has one incoming and two outgoing transitions as shown in Figure \ref{fig:repl}. In Figure \ref{fig:repl} the multi-hop transition $q_B\rightarrow_B q_F\rightarrow_B q_B$ is removed since there are no symbols that satisfy $\pi_1^{\ell_1}\wedge\pi_1^{\ell_2}$ (condition (i)-Defn. \ref{def:feas}); in fact this transition requires robot $1$ to `jump' from $\ell_1$ to $\ell_2$. The resulting pruned NBA generated by Algorithm \ref{alg:prune} is shown in Figure \ref{fig:finalPrune}.  
  }
  \label{fig:prune}
\end{figure}



To formalize this concept, we first %need to take into account the initial multi-robot state as it may also result in infeasible NBA transitions; see e.g., Figure \ref{fig:NBA1}. To this end, we introduce auxiliary states $q_B^{\text{aux}}$ and transitions $q_B^{\text{aux}}\rightarrow_B q_B^0$ for all $q_B^0\in\ccalQ_B^0$ so that $b^{q_B^{\text{aux}},q_B^{\text{aux}}}=1$ and $b^{q_B^{\text{aux}},q_B^{0}}=L(\bbp(0))$. The auxiliary states $q_B^{\text{aux}}$ are considered the initial states of the resulting NBA. For
%In this way, we also ensure that the robots can remain in the initial states 
define the set $\hat{\ccalQ}_B\subseteq\ccalQ_B$ that collects all NBA states $q_B$ for which there exist feasible symbols (as per Definition \ref{defn:infPTS}) that allow a transition from $q_B$ to $q_B$, i.e., $\Sigma^{q_B,q_B}\neq\emptyset$, i.e., 
\begin{equation}
    \hat{\ccalQ}_B=\{q_B\in\ccalQ_B|\Sigma^{q_B,q_B}\neq\emptyset\},
\end{equation}
where $\Sigma^{q_B,q_B}$ is defined in Definition \ref{defn:feasSet}. Let $i_{q_B}$ and $o_{q_B}$ be the number of incoming and outgoing transitions for $q_B\in\hat{\ccalQ}_B$. For each state $q_B\in\hat{\ccalQ}_B$, we define the set $\ccalP_{q_B}$ that collects all possible pairs of incoming and outgoing transitions for $q_B$, i.e.,  
\begin{equation}\label{eq:pairs}
    \ccalP_{q_B}=\{[(q_B^{\text{in},i},q_B),(q_B,q_B^{\text{out},o})]\}_{i=1,o=1}^{i_{q_B},o_{q_B}}
\end{equation}
where with slight abuse of notation $(q_B^{\text{in},i},q_B)$ and $(q_B,q_B^{\text{out},o})$ denote an incoming and outgoing transition for $q_B$ respectively.
%$\ccalP_{q_B}=\{[(q_B^{\text{in},n},q_B),(q_B,q_B^{\text{out},m})]\}_{n=1,m=1}^{n=\bar{n},m=\bar{m}}$ that collects all possible pairs of incoming and outgoing transitions for $q_B$. 
Next we replicate all states $q_B\in\hat{\ccalQ}_B$ $i_{q_B}\times o_{q_B}$ times, so that each copy of $q_B$ has only one and unique pair of incoming and outgoing transitions; see Example \red{(????)}. 

Next for each state $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$ we compute all, possibly multi-hop, transitions that start from $q_B$ and end at states $q_B'\in q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$, $q_B'\neq q_B$ so that all, if any, intermediate NBA states that connect $q_B$ to $q_B'$ belong to $\hat{\ccalQ}_B$. Formally, these multi-hop transitions are defined as $q_B\rightarrow_B q_B^1\rightarrow_B q_B^2\rightarrow_B\dots\rightarrow_B q_B^K\rightarrow_B q_B'$, where $q_B^k\in\hat{\ccalQ}_B, k\in\{1,\dots,K\}$, and $K\geq 0$; see also Figure \red{(????)}. We compactly denote such a multi hop transition by $q_B\rightarrow_B^K q_B'$.%\footnote{Note that $q_B\rightarrow_B^0 q_B'$ corresponds to the one hop transition $q_B\rightarrow_B q_B'$.}

Given the above definitions, we define the feasible NBA transitions as follows; see also Example \ref{ex:feas}.
\begin{definition}[Feasible NBA transitions]\label{def:feas}
A transition $q_B\rightarrow_B^K q_B'$, where $q_B,q_B'\in\ccalQ_B\setminus\hat{\ccalQ}_B$, is feasible if (i) for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$ there exists at least one symbol $\sigma^{q_B,q_B^1}\in\Sigma^{q_B,q_B^1}$ that enables the multi-hop transition $q_B\rightarrow_B^K q_B'$, i.e.,
$\sigma^{q_B,q_B^1}\models b^{q_B,q_B'}_K$, where 
$b^{q_B,q_B'}_K=b^{q_B,q_B^1}\wedge b^{q_B^1,q_B^{2}}\wedge\dots\wedge b^{q_B^{K-1},q_B^{K}}\wedge b^{q_B^K,q_B'}\wedge b^{q_B',q_B'}$; and 
%
(ii) at least one of the symbols $\sigma^{q_B,q_B^1}$ that satisfy condition (i) should satisfy either (a) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^1}=\emptyset$ or (b) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^1}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^1}$. If $K=0$, conditions (i)-(ii) are applied by replacing $q_B^1$ with $q_B'$. %conditions (i)-(ii) assume
\end{definition}
%A transition $(q_B,\cdot,q_B')$ is feasible if (i) $\Sigma^{q_B,q_B}\neq \emptyset$; (ii) for all symbols  $\sigma^{q_B,q_B}\in\Sigma^{q_B,q_B}$ there exists at least one symbol $\sigma^{q_B,q_B'}\in\Sigma^{q_B,q_B'}$ such that $\sigma^{q_B,q_B'}\models b^{q_B',q_B'}$; and (iii) at least one of the symbols $\sigma^{q_B,q_B'}$ that satisfy condition (ii) should satisfy either (a) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}=\emptyset$ or (b) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}\neq\emptyset$ and $L_{j}^{q_B,q_B'}=L_{j}^{q_B,q_B}$.

Then, we prune the NBA by removing transitions that are not feasible, as per Definition \ref{def:feas}. Note that condition (i) ensures that once robots reach a state $q_B$, they will always be able to make progress towards accomplishing the assigned task by moving towards a new NBA state $q_B'$. Also, due to condition (i), this will be achieved without requiring robots to be present in more than one location simultaneously (since $\sigma^{q_B,q_B^1}\in\Sigma^{q_B,q_B^1}$) or jump from one region of interest to another (since $\sigma^{q_B,q_B^1}\models b^{q_B,q_B'}_K$). Also, condition (ii) allows us to cast transition from $q_B$ to $q_B'$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalR^{q_B,q_B'}$ needs to move to a region of interest while avoiding certain regions and obstacles. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is continuously learned. 
%
Also, by construction of the pruned automaton we have that once the robots reach an NBA state $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$, i.e., an NBA state for which a self-loop exists, the robots can remain in this state given their current observations. To enforce this property from $t=0$, we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$. This property will be used in Section \ref{sec:planning} to design robot paths.
\begin{assumption}[Initial Robot State]
Assume that the initial multi-robot state $\bbp(0)$ satisfies $b^{q_B^0,q_B^0}$, i.e, $L(\bbp(0))\models b^{q_B^0,q_B^0}$ for at least one initial state $q_B^0\in\ccalQ_B^0$.
\end{assumption}

%In words, a transition from $q_B$ to $q_B'$ is feasible and, therefore, it is not removed (a) if the set $\Sigma^{q_B,q_B}$ is non-empty, i.e., there are feasible symbols that allow the robots to stay in state $q_B$; and (ii) for each possible symbol in $\Sigma^{q_B,q_B}$ that the robots may generate to reach $q_B'$, there exists a feasible symbol that will enable the robots to eventually reach a new state $q_B'$ from $q_B$ and stay in $q_B'$. Also, in (iii) we require the set of robots in $\ccalN^{q_B,q_B'}$ that to be either (a) disjoint from the set of robots in $\ccalR^{q_B,q_B}$ or (b) if there exist robots $j\in \ccalR^{q_B,q_B}\cap\ccalN_{\text{next}}^{q_B,q_B'}\neq\emptyset$ then these robots should suffice to stay in their current locations, i.e., $L_{j}^{q_B,q_B'}=L_{j}^{q_B,q_B}$, to `contribute' to satisfaction of $b_{\text{next}}^{q_D,q_D'}$. As it will be discussed later, this allows us to cast transition from $q_B$ to $q_B'$ as \textit{local/independent} reachability-avoidance problems, where each robot involved in $\ccalN^{q_B,q_B'}$ needs to move to a region of interest while avoiding certain regions and obstacles. This decomposition of the temporal logic task allows for computationally efficient re-planning as the map of the environment is learned.

%IN THE PRUNED AUTOMATON WE HAVE THAT ONCE WE VISIT A SELF-LOOP STATE WE CAN STAY IN IT MAKE PROGRESS I.E. VISIT NEW TASKS. This essentially allows us to avoid cases WHERE ROBOTS HAVE TO 'JUMP' FROM ONE REGION OF INTEREST TO ANOTHER ONE. WE USE THIS PROPERTY FOR PLANNING IN SECTION ?. TO ENFORCE THIS PROPERTY AT T=0, WE ASSUME THAT THE INITIAL CONDITION ALWAYS SATISFIES THE INITIAL SELF-LOOP IF IT EXISTS. 

%OR AVOID IT AND MENTION IT IN THE THEOREMS!!!

%IT IS POSSIBLE THAT THE INIT STATE DOES NOT HAVE A SELF LOOP OR THE INIT ROBOT STATE DOES NOT SATISFY.

%SAY HERE THAT OUR GOAL IS THAT ONCE WE VISIT A STATE WITH SELF LOOPS TO SATISFY THE RESPECTIVE CONDITION UNTIL WE MAKE NEW OBSERVATIONS THAT WILL ALLOWS US TO MAKE PROGRESS IE VISIT NEW TASKS


%\begin{ex}[Conservative Pruning]
%-Add figure and explain-
%\end{ex}
\begin{figure}
    \centering
     \includegraphics[width=1\linewidth]{figures/conserv.png}
    \caption{Example of conservative pruning for the NBA corresponding to $\phi=\square(\pi_1^{r_0}\vee\pi_1^{r_0}) \wedge \Diamond \pi_2^{r_1}\wedge \Diamond \pi_2^{r_1}$. This formula requires either robot $1$ or $2$ to always be in $\ell_0$ and eventually robots $1$ and $2$ to visit, not necessarily simultaneously, $\ell_1$. Transition from $q_B^0$ to $q_B^F$ is removed as it requires robots to visit more than one location at the same time. Transitions from $q_B$ to $q_F$ and from $q_B'$ to $q_F$ are removed as they violate both conditions of Definition \ref{def:feas} resulting in a disconnected pruned NBA, i.e., Algorithm \ref{alg:RRT} will not be able to find a solution. Nevertheless, a solution exists, as these two transitions can be enabled in practice. For instance, consider the transition from $q_B$ to $q_F$. %Assuming that both robots are initially in $\ell_0$, 
    Observe that transition from $q_B$ to $q_F$ cannot be cast as two independent reachability-avoidance problems (condition (ii)). Instead it requires coordination among the robots that is specific to the Boolean formula $b^{q_B,q_F}$. Specifically, when the robots reach $q_B$, we have that robot $1$ is in $\ell_0$ and robot $2$ is in $\ell_1$. To eventually satisfy $b^{q_B,q_F}=(\pi_1^{\ell_0}\wedge\pi_2^{\ell_1})\vee(\pi_2^{\ell_0}\wedge\pi_2^{\ell_1})$, first robot $2$ is required 
    to return in $\ell_0$ while in the meantime robot $1$ should stay in $\ell_0$. Once robot $2$ returns in $\ell_0$, robot $1$ should move to $\ell_1$ enabling the transition to the final state $q_F$.}
    \label{fig:conserv}
\end{figure}
%
%Conditions under which Definition \ref{def:feas} is not conservative are presented in Section \ref{sec:complOpt}.%, and/or (c) if it is (physically) impossible for the robots to stay in $q_D$ until the symbol $\sigma_{\text{next}}$, that triggers transition to $q_D'$, is generated; the latter happens if condition (iii) is not true (see also Ex. \ref{ex:feas}). 

On the pruned DFA, we define a function $d:\ccalQ_D\times\ccalQ_D\rightarrow \mathbb{N}$ that returns the minimum number of \textit{feasible} DFA transitions that are required to reach a state $q_D'\in\ccalQ_D$ starting from a state $q_D\in\ccalQ_D$. %This function will be used to guide the robots towards locations in the workspace so that eventually a final DFA state is visited, i.e., the LTL formula is satisfied.
%
Particularly, we define the distance function $d: \ccalQ_D \times \ccalQ_D \rightarrow \mathbb{N}$ as follows
\begin{equation}
d(q_D,q_D')=\left\{
                \begin{array}{ll}
                  |SP_{q_D,q_D'}|, \mbox{if $SP_{q_D,q_D'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_D,q_D'}$ denotes the shortest path (in terms of hops) in the  pruned DFA from $q_D$ to $q_D'$ and $|SP_{q_D,q_D'}|$ stands for its cost (number of hops).%\footnote{In Section \ref{sec:complOpt}, we provide conditions under which if $d(q_D^0,q_F)=\infty$ then the assigned co-safe LTL task is infeasible}. %; see Sections \ref{sec:targetDFA}-\ref{sec:paths}.
\begin{rem}[Conservative Pruning]\label{rem:conserv}
Notice that the proposed pruning approach for the NBA, as per Definition \ref{def:feas}, is conservative. For instance, there may exist feasible symbols (as per Definition \ref{defn:infPTS}) that enable a transition from $q_B$ to $q_B'$ that may not satisfy conditions (i)-(ii); see e.g., Figure \ref{fig:conserv}. Conditions under which the proposed pruning approach is not conservative are discussed in Section \ref{sec:complOpt}.
%Nevertheless, conservative pruning ensures that when the robots reach a state $q_D$, they will always be able to make progress towards accomplishing their task (i.e., reach a new state $q_D'$) regardless of the symbols they have generated to reach $q_D$ by solving local point-to-point navigation problems. A fragment of LTL for which the proposed approach is not conservative is discussed in Section \ref{sec:complOpt}.
\end{rem}


%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}

%\begin{ex}[Feasible DFA transitions]\label{ex:feas}
%(a) Consider the case, where $b^{q_B,q_B}=1$ and $b^{q_B,q_B'}=\pi_j^{r_{m}}$. By definition of $\Sigma^{q_B,q_B}$ and $\Sigma^{q_B,q_B'}$, we have that $\Sigma^{q_B,q_B}=\{\varnothing\}$, where $\varnothing$ stands for the empty symbol, and $\Sigma^{q_B,q_B'} =\{\pi_j^{r_{m}}\}$. Transition from $q_B$ to $q_B'$ is feasible as per Definition \ref{def:feas}. Recall that the sets $\Sigma^{q_B,q_B}, \Sigma^{q_B,q_B'}$ collect symbols that are associated with robots that play a role in satisfying the respective Boolean formulas. This precludes cases where, e.g., a symbol $\pi_j^{r_e}$, $e\neq m$ is included in $\Sigma^{q_B,q_B}$ resulting in erroneously characterizing the transition from $q_D$ to $q_D'$ as infeasible due to condition (iii). 
%%%(b) Consider the following Boolean conditions: $b_{\text{inv}}^{q_D}=b_{\text{inv}}^{q_D'}=\pi_j^{r_i}$ and $b_{\text{next}}^{q_D,q_D'}=\pi_j^{r_i}\wedge \pi_m^{r_h}$. Then the transition from $q_D$ to $q_D'$ is feasible since it satisfies Definition \ref{def:feas}. 
%(b) Consider also the Boolean formulas  $b^{q_B,q_B}=b^{q_B',q_B'}=\pi_j^{r_i}$ and $b^{q_B,q_B'}=\pi_j^{r_e}\wedge \pi_m^{r_h}$, then the transition from $q_B$ to $q_B'$ is infeasible, since it holds that $j\in \ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and, $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. In fact, transition from $q_B$ to $q_B'$ requires robot $j$ to instantaneously move from $r_i$ to $r_e$ which is not possible given that $r_i$ and $r_e$ are disjoint regions. 
%\end{ex}




%\subsection{Selecting a Feasible DFA Final State}\label{sec:feasFinal}
%Given the pruned DFA, the distance function, and an initial DFA state $q_D(0)$, our next step is to select a \textit{feasible} final state $q_{F}\in\ccalQ_F$, i.e., a final state that is reachable from $q_D(0)$ in the pruned DFA [line \ref{rrt:feasFinal}, Alg. \ref{alg:RRT}]. In math, given an initial state  $q_D(0)$ feasible final states are the ones that satisfy  $d(q_D(0),q_{F})\neq \infty$. Among all final states that satisfy this condition, we select one randomly denoted by $q_F^{\text{feas}}$. If there do not exist such final states given the state $q_D(0)$, then we select another initial DFA state $q_D(0)$ from $\ccalQ_D^0$. If there do not exist initial states such that $d(q_D^0,q_{F})\neq \infty$, then the LTL formula can not be satisfied since the in the pruning process, only the DFA transitions that are impossible to enable are removed (i.e., the ones that require the robots to be physically present at more than one region simultaneously) [lines \ref{rrt:unsat1}-\ref{rrt:unsat2}, Alg. \ref{alg:RRT}].
%Next at any time $t\geq 0$, given the current DFA state $q_D(t)$, we select a target DFA state, denoted by $q_D^{\text{next}}$, that the robots should reach next. This state is selected so that it is one hop closer to $q_F^{\text{feas}}$ than $q_D(t)$ is, i.e.,

%\subsection{Selecting the Next NBA State}
%{\bf{Selecting the Next NBA State:}} 
\subsection{Distributed Construction of Robot Paths}\label{sec:paths}
The pruning process described in Section \ref{sec:prune} occurs offline, i.e., before deploying the robots in the workspace. In what follows, we present the online part of Algorithm \ref{alg:RRT}. The pruned automaton is used at runtime to guide planning in a distributed way towards regions of interest so the assigned LTL task is accomplished.

Let $q_B(t)$ be the NBA state that the robots have reached at time $t$ after following paths, denoted by $\bbp_{j,[0:t]}$, and starting from an initial NBA state $q_B^0\in\ccalQ_B^0$. At time $t=0$, $q_B(0)$ is initialized to be one of the initial states $q_B^0$ of the NBA. Given the current NBA state $\bbq_B(t)$, the robots coordinate to select a new NBA state, denoted by $q_B^{\text{next}}$, that they should reach next to make progress towards accomplishing their task.
%every robot $j$ needs to locally design a path so that a DFA state that is closer to the final state $q_F$ than the current DFA state $q_D(t)$ is eventually reached. 
The NBA state $q_B^{\text{next}}$ is selected as follows. First, we compute the distance $d(q_BB(t),q_F^{\text{feas}})$, where $q_F^{\text{feas}}$ is a final NBA state that is reachable from its initial state $q_B^0$ in the pruned NBA, i.e., $d(q_B^0,q_F^{\text{feas}})\neq\infty$. Then, we select as $q_B^{\text{next}}$ a state that satisfies $d(q_B^{\text{next}},q_F^{\text{feas}}) = d(q_B(t),q_F^{\text{feas}}) -1$,
%\begin{equation}\label{eq:targetDFA}
%   d(q_D^{\text{next}},q_F) = d(q_D(t),q_F) -1, 
%\end{equation}
i.e., a state that is one hop closer to $q_F^{\text{feas}}$ than $q_B(t)$ is. If there is more than one state that satisfies this condition, we select one randomly [line \ref{rrt:selTarget}, Alg. \ref{alg:RRT}]. The state $q_B^{\text{next}}$ is updated when the robots reach it, i.e., at a time instant $t'\geq t$ that satisfies $q_D(t')=q_D^{\text{next}}$ [lines \ref{rrt:T}-\ref{rrt:updTarget}, Alg. \ref{alg:RRT}]. %; see  Sections \ref{sec:paths}. %or realize that a transition from $q_D(t)$ to $q_D^{\text{next}}$ is in fact infeasible; see next section.


%{\bf{Local Construction of Robot Paths:}}
Given the NBA state $q_B^{\text{next}}$, our goal is to design paths $\bbp_{j,t:T_j}$, for all robots $j$ that should be followed within a time interval $[t,T_j]$ so that the NBA transition from $q_B(t)$ to $q_B^{\text{next}}$ is activated. %\footnote{With slight abuse of notation the subscript in $\bbp_{j,t:T_j}$ denotes the index of robot and the time interval $[t,T_j]$ within which the path should be followed.} 
To achieve that, it suffices to ensure that the robots follow paths that (i) satisfy the Boolean formula $b^{q_B(t),q_B(t)}$ that allows them to stay in the current NBA state $q_B(t)$, until (ii) the Boolean formula $b^{q_B(t),q_B^{\text{next}}}$ that enables transition from $q_B(t)$ to $q_B^{\text{next}}$ is satisfied while (iii) while never satisfying Boolean formulas $b^{q_B(t),q_B''}$ other than the ones that are satisfied at time $t$.\footnote{At time $t$, the Boolean formula $b^{q_B(t),q_B(t)}$ is satisfied by construction of the pruned automaton. Nevertheless, other Boolean formulas $b^{q_B(t),q_B''}$ may be satisfied as well due to the non-deterministic nature of the NBA.} 
For simplicity, in what follows, we replace $b^{q_B(t),q_B(t)}$ and $b^{q_B(t),q_B^{\text{next}}}$ with $b_{\text{inv}}$ and $b_{\text{next}}$ respectively. The same notation extends to the symbols $\sigma^{q_B,q_B'}$ and the sets of robot indices $\ccalN^{q_B,q_B'}$, $\ccalR^{q_B,q_B'}$.

\red{[add reference to lines of the algorithm]}
To design paths $\bbp_{j,t:T_j}$, \textit{first} the robots $j\in\ccalN_{\text{next}}$ \textit{communicate} to select a symbol $\sigma_{\text{next}}$ that satisfies conditions (i)-(ii) of Definition \ref{def:feas} given the current symbol  $\sigma_{\text{inv}}=L(\bbp(t))$ they are generating. %; see also Example \ref{ex3}. 
Note that such a symbol exists by construction of the pruned NBA for any symbol $\sigma_{\text{inv}}$. % \footnote{Note that it is possible that given the symbol that the robots generated to reach $q_D$ there may not exist a pair of symbols $\sigma_{\text{inv}}$ and $\sigma_{\text{next}}$ to reach a state $q_D^{\text{next}}$ that satisfy condition (iii) of Def. \ref{def:feas}. In other words, transition from $q_D$ to $q_D^{\text{next}}$ may not be cast as a point-to-point navigation problem as in \eqref{eq:localProb}.
%Consider e.g., the DFA that corresponds to $\phi=\square(\pi_1^{r_0}\vee\pi_2^{r_0})\wedge\Diamond(\pi_1^{r_1})\wedge\Diamond(\pi_2^{r_2})$. 
%Existence of such symbols is always guaranteed for a sub-class of co-safe LTL formulas as discussed in Lemma \ref{lem:cnt}.} %that satisfy $b_{\text{inv}}$ and $b_{\text{next}}$, respectively, i.e., $\sigma_{\text{next}}\models b_{\text{next}}$. This pair of symbols is selected so that condition (ii) of Definition \ref{def:feas} is satisfied; 
Among all such symbols $\sigma_{\text{next}}$, we select the one that yields the smallest set $\ccalN_{\text{next}}$ to minimize the number of robots required to navigate the workspace to reach the state $q_B^{\text{next}}$; however any symbol can be selected. 
%
%Given $\sigma_{\text{next}}$, we compute the set $\ccalR_{\text{next}}$ that collect the robots that need to move towards certain regions of interest $r_e$ in workspace to generate $\sigma_{\text{next}}$. 
%
\textit{Second}, given $\sigma_{\text{next}}$,  we compute for each robot $j\in\ccalN_{\text{next}}$ the location $L_j^{\text{next}}$ that it should visit to generate  $\sigma_{\text{next}}$. Recall that for robots $j\in\ccalR_{\text{next}}$, $L_j^{\text{next}}$ corresponds to a certain region of interest determined by $\sigma_{\text{next}}$  while for robots $j\in\ccalN_{\text{next}}\setminus\ccalR_{\text{next}}$, $L_j^{\text{next}}$ corresponds to any location in the workspace where no atomic predicates are satisfied. 
%\textit{Third}, we design the paths $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ for all robots $j\in\ccalN_{\text{next}}$. %First, all robots $j\notin\ccalR_{\text{inv}}$ stay put at their current locations until the state $q_B^{\text{next}}$ is reached. %
\textit{Third}, every robot $j\in\ccalN_{\text{next}}$ locally solves the feasibility problem \eqref{eq:localProb} to design its respective path $\bbp_{j,t:T_j}$ towards $L_j^{\text{next}}$ while all other robots stay put at their current locations [lines \ref{rrt:for1}-\ref{rrt:compPaths}, Alg. \ref{alg:RRT}].
%that if followed the symbol  $\sigma_{\text{next}}\models b_{\text{next}}$ is generated and the DFA state $q_D^{\text{next}}$ is reached
%In Section \ref{sec:complOpt}, we show that the multi-robot state $\bbp(t)$ already generates a symbol that satisfies $b_{\text{inv}}$. We also show that if (i) the robots that are involved in generating $\sigma_{\text{inv}}$, collected in a set $\ccalR_{\text{inv}}$, stay idle at their current locations $\bbp_j(t)$ and (ii) all other robots 
%
%
%\footnotesize
\begin{subequations}
\label{eq:localProb}
\begin{align}
%& \min_{\substack{T_j, \bbu_{j,t:T_j}}} \left[J(T_j,\bbu_{j,t:T_j}) = \int_{t'=t}^{T_j}  w(\bbp_j(t'),\bbu_j(t'))dt \right] \label{ObjLoc2}\\
& \text{Compute:~}{T_j, \bbu_{j,t:T_j}}~\text{such that}  \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ [L(\bbp_j(t'))=L(\bbp_j(t))] \vee [L(\bbp_j(t'))=\varnothing] \nonumber\\
%& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \vee [L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}],~\forall t'\in[t,T_j] \label{constrLoc1} \\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \cup_i\set{r_i}\setminus (R_j^t\cup L_j^{\text{next}}), \forall t'\in[t,T_j] \label{constrLoc1}\\
& \ \ \ \ \ \ \ \ \ \ \  \bbp_j(t') \notin \hat{O}(t), \forall t'\in[t,T_j] \label{constrLocObs}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j) \in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin \ccalA_j^{\text{avoid}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'+1),\bbu_j(t'+1)), \label{constrLoc3}
\end{align}
\end{subequations}
%\normalsize

\noindent In \eqref{constrLoc1}, $R_j^t$ denotes the region that robot $j$ lies in at time $t$. The first constraint \eqref{constrLoc1} requires that robot $j$ should not visit any region $r_i$ excluding $R_j^t$ and the target region $L_j^{\text{next}}$, for all $t'\in[t,T_j]$. If at time $t$ robot $j$ does not lie in any of the regions $r_i$, then $R_j^t=\emptyset$. This ensures that the multi-robot system can always remain in $q_B(t)$ as the robots $j\in\ccalN_{\text{next}}$ navigate the workspace; see Lemma \ref{lem:binv}. This constraint can be relaxed by requiring  robot $j\in\ccalN_\text{next}$ to always avoid only regions that may result in violating $b_{\text{inv}}$. For instance, if $b_{\text{next}}=\neg(\pi_j^{r_e}\wedge\pi_i^{r_e}$), then it suffices to require robot $j$ to never visit $r_e$.  %\footnote{$T_j^{-}$ denotes a time instant right before $T_j$, i.e., $T_j^{-}=T_j-\epsilon$, for an arbitrarily small $\epsilon>0$.} 
Similarly, the second constraint in \eqref{constrLocObs} requires robot $j$ to avoid all obstacles, collected in $\hat{O}(t)$, that are known up to the time instant $t$. The third constraint in \eqref{constrLoc2} requires robot $j$ to be in region $L_j^{\text{next}}$ at a time instant $T_j\geq t$. %so that it generates $L(\bbp_j(T_j)) =\pi_j^{L_j^{\text{next}}}$.%\footnote{Note that this prevents the robot from visiting parts of $L_j^{\text{next}}$ that are shared with other regions $r_i$.} 
This is required to eventually generate the symbol $\sigma_{\text{next}}$. The last constraint in \eqref{constrLoc3} captures the robot dynamics. Note that among all paths that satisfy these constraints, the optimal one, as a per a user-specified motion cost function, can be selected. %In words, the optimal control problem \eqref{eq:localProb} requires robot $j$ to design a path $\bbp_{j,t:T_j}$ that reaches $L_j^{\text{next}}$ (see \eqref{constrLoc2}) while avoiding certain regions $r_i$ (see \eqref{constrLoc1}) and all detected obstacles denoted by $\hat{O}(t)$ (see \eqref{constrLocObs}). %Note that the robots that do not belong to $\ccalR_{\text{inv}}$ and also are not responsible to generate $\sigma_{\text{next}}$ do not have a target region $L_{j}^{\text{next}}$. These robots remain stationary in their current locations and they do not need to solve \eqref{eq:localProb}.
%
Observe that \eqref{eq:localProb} is a  point-to-point navigation problem, and, therefore, any of the traditional motion planning algorithms, such as $\text{A}^*$, RRT, $\text{RRT}^*$, RRG, or PRM, can be used to solve it \cite{karaman2011sampling}. Finally observe that given $L_j^{\text{next}}$, robot $j$ locally solves \eqref{eq:localProb} without communicating with any other robot. %Correctness of Alg. \ref{alg:RRT} is discussed in Sec. \ref{sec:complOpt}. %Feasibility of such this problem is examined in 

%We design such paths in two stages. In the first stage, we design subpaths $\bbp_{j,t:\bar{T}_j}$ for some $t<\bar{T}_j<T$ and in the second stage we design paths $\bbp_{j,\bar{T}_j:T_j}$. In particular, \textit{in the first stage} all robots that are involved in generating $\sigma_{\text{inv}}$, collected in a set $\ccalR_{\text{inv}}$, and all other robots $j$ for which it hold $L(\bbp_j(t))=\varnothing$ (i.e., they are outside of all regions $r_i$) stay idle at their current locations $\bbp_j(t)$, i.e., $\bar{T}_j=t+1$ and $\bbp_{j,t:\bar{T}_j}=[\bbp_j(t),\bbp_j(t)]$ All other robots $j$ (i.e., the ones that satisfy $j\notin\ccalR_{\text{inv}}$ and $L(\bbp_j(t))\neq \varnothing$) solve the following optimal control problem to design paths $\bbp_{j,t:\bar{T}_j}$ that if followed then the robots will move outside the regions that they are currently located. %As it will bbe discusses in Section \ref{sec:exec}, these subpaths will be executed so that the robots will move outside their current regions simultaneously.

%\begin{subequations}
%\label{eq:localProb1}
%\begin{align}
%& \min_{\substack{\bar{T}_j, \bbu_{t:\bar{T}_j}}} \left[J(\bar{T}_j,\bbu_{t:\bar{T}_j}) = \sum_{t'=t}^{\bar{T}_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc1}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in R_j(t), \forall t\in\set{t,\dots,\bar{T}_j-1} \label{constrLoc1a} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in \ccalR_j^{\text{inv}}, \forall t\in\set{t,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(\bar{T}_j))=\varnothing \label{constrLoc2a}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   %\bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc2}
%\end{align}
%\end{subequations}
%where $R_j(t)$ denotes the region $r_i$ that robot $j$ lies in at time $t$. Observe that the first two constraints \eqref{constrLoc1a}-\eqref{constrLoc2a} require robot $j$ to move outside the region $\ccalR_j(t)$ where it is located at the time instant $t$. This happens at a time instant $\bar{T}_j$, i.e., $L(\bbp_j(\bar{T}_j))=\varnothing$. Note that robot $j$ locally solves \label{eq:localProb1} with communicating with other robots. Observe that execution of these subpaths ensures that the robots remain in the DFA state $q_D(t)$ since $b_{\text{inv}}$ is always satisfied as the robots $\ccalR_{\text{inv}}$ remain stationary in their current locations that generates  $\sigma_{\text{inv}}\models b_{\text{inv}}$.

%since the robots in $\ccalR_{\text{inv}}$

%In the \textit{second} stage, we construct the subpaths $\bbp_{j,\bar{T}_j:T_j}$ that will enable the transition from $q_D(t)$ to $q_D^{\text{next}}$. For robots $j\in\ccalR_{\text{inv}}$, we select $T_j=\bar{T}_j+1$ and $\bbp_{j,\bar{T}_j:T_j}=[\bbp_{j}(t),\bbp_{j}(t)]$, i.e., these robots still stay idle. In fact, due to the deterministic structure of the DFA, this ensures that the robots remain in the DFA state $q_D(t)$ until the symbol $\sigma_{\text{next}}$ is generated which will activate the transition towards $q_D^{\text{next}}$. To generate the symbol  $\sigma_{\text{next}}$, all other robots $j\notin\ccalR_{\text{inv}}$ design paths $\bbp_{j,\bar{T}_j:T_j}$ by solving the following optimal control problem:

%\begin{subequations}
%\label{eq:localProb}
%\begin{align}
%& \min_{\substack{T_j, \bbu_{\bar{T}_j:T_j}}} \left[J(T_j,\bbu_{\bar{T}_j:T_j}) = \sum_{t'=\bar{T}_j}^{T_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ L(\bbp_j(t'))=\varnothing, \forall t'\in\set{\bar{T}_j,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{next}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
%\end{align}
%\end{subequations}



 %This ensures that  transition to a DFA state $q_D'\neq q_D(t)$ that is not $q_D^{\text{next}}$. 
%In the meantime the robots in $\ccalR_{\text{inv}}$ ensure that the current DFA state remain the same in $[t,\bar{T}-1]$, since they stay idle and generate the symbol $\sigma_{\text{inv}}$. Also note that robots in $\ccalR_{\text{inv}}$ do not belong to the set of robots that need to move to another location to generate the symbol $\sigma$, since that would create a conflict; see also Remark \ref{rem:invariant}. 
%The second constraint in \eqref{constrLoc2} requires that at time instant $T_j$, all robots should be in their corresponding locations $L_j^\textbf{}$. Once this happens the symbol $\sigma_{\text{next}}$ is generated and the target DFA state is reached.
%
%Note that infeasibility of \eqref{eq:localProb} is due to the facts (i) the environment is unknown and, therefore, it is not possible to check offline which DFA transitions cannot be enabled because e.g., of the robot dynamics or the existence of obstacles.%; and (ii) the LTL formula $\phi$ is decomposed into local sub-tasks Problem \ref{prob} is solved in a distributed the proposed algorithm is distributed nature of the proposed 

%What if the problem is infeasible? update $\sigma$ i.e., $L_j$. If no other $L_j$. update target DFA state. If no other target DFA state report `current method failed (this does not mean that the task is unsatisfiable though)'

%\begin{ex}[Selection of $\sigma_{\text{next}}$ and $\sigma_{\text{inv}}$]\label{ex3}
%Consider the Boolean formulas $b_{\text{inv}}=\neg \pi_{\text{obs}}$ and $b_{\text{next}}=(\pi_j^{r_1}\vee \pi_j^{r_3} )\wedge\pi_e^{r_2}\wedge (\neg \pi_j^{r_2}) \wedge (\neg (\pi_j^{r_1}\wedge \pi_e^{r_1}))$, where the atomic predicate $\pi_{\text{obs}}$ is true of at least one robot hits an obstacle. A symbol $\sigma_{\text{next}}$ that satisfies $b_{\text{next}}$ is $\sigma_{\text{next}}=\pi_j^{r_1}\pi_e^{r_2}$ while $b_{\text{inv}}$ is satisfied by an empty string, i.e., $\sigma_{\text{inv}}=\varnothing$. Given this pair of symbols, we have that $\ccalR_{\text{inv}}=\emptyset$, $\ccalR_{\text{next}}=\set{j,e}$, $L_j^{\text{next}}=r_1$, and $L_e^{\text{next}}=r_2$.
%\end{ex}

%\begin{ex}[Construction of $\sigma_{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b_{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$. Then, we have that $\sigma_{\text{inv}}=\pi_j^{r_1}$ and $\ccalR_{\text{inv}}=\set{j}$. Similarly, if $b_{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma_{\text{inv}}$ is an empty string and $\ccalR_{\text{inv}}=\emptyset$.
%\end{ex}

%\begin{ex}
%--add automaton figure--and explain--
%\end{ex}
%\begin{rem}[Initialization of $q_B(t)$]
%we assume that the initial multi-robot state $\bbp(0)$ satisfies the Boolean condition $b^{q_B^0,q_B^0}$.\footnote{Note that if $b^{q_B^0,q_B^0}$ is not defined or if $L(\bbp(0))\not\models b^{q_B^0,q_B^0}$, then $q_B(0)$ can be selected to be a state $q_B$ that can be reached from $q_B^0$ given $L(\bbp(0))$ that satisfies $b^{q_B,q_B}$. If such a state does not exist then $\phi$ cannot be satisfied given the initial multi-robot state. For instance, in Figure \ref{fig:NBA1}, if robot $1$ is initially in $\ell_2$, then $q_B(0)=q_F$. For simplicity, throughout the paper we assume that we assume that $\bbp(0)\models b^{q_B^0,q_B^0}$, for at least one initial state.}
%\end{rem}
\subsection{Reacting to Map Uncertainty}\label{sec:exec}
%{\bf{Reactive Planning to Map Uncertainty:}}

The robots need to adapt their control actions to the continuously learned occupancy grid map. In fact, reactivity to the environment is required in two cases. First, as the robots follow their paths $\bbp_{j,t:T_j}$, they may discover new obstacles based on their sensor measurements; see \eqref{eq:sensor}. If the discovered obstacles intersect with their paths $\bbp_{j,t:T_j}$, for some $j\in\ccalR_{\text{next}}$, then these robots $j$ locally re-solve \eqref{eq:localProb} using the updated map to design new paths. Note that existing reactive planning algorithms that can address reachability navigation problems in the presence of unknown obstacles can also be used to solve \eqref{eq:localProb}; see e.g., \cite{guzzi2013human,vasilopoulos2018sensor,bansal2019combining,ryll2019efficient}.

%is not reachable e.g., due to the robot dynamics or 
Second, as the the map $M(t)$ is constructed, goal regions $L_j^{\text{next}}$ may become unreachable because of the structure of the environment (e.g., regions of interest may be surrounded by obstacles). In this case, robots $j$ that cannot reach $L_j^{\text{next}}$ communicate with all other robots so that a new symbol $\sigma_{\text{next}}$ is selected. This process is repeated until a reachable region $L_j^{\text{next}}$ is selected.  %that makes \eqref{eq:localProb} feasible. 
If such a symbol $\sigma_{\text{next}}$ does not exist, then this means that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$, due to the a-priori unknown structure of the environment. Then, the pruned NBA is updated by removing this transition and a new NBA state $q_B^{\text{next}}$. If there do not exist any candidate NBA states to be selected as $q_B^{\text{next}}$, then the assigned task cannot be accomplished given the current multi-robot and NBA state. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
In fact, there may exist another sequence of NBA states for which  Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible (i.e., paths towards selected goal regions always exist) and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.

%\begin{rem}[Feasibility of \eqref{eq:localProb}]
%Observe that \eqref{eq:localProb} may be \textit{infeasible}. This can be the case e.g., if the region $L_j^{\text{next}}$ is not reachable e.g., due to the robot dynamics or the structure of the environment. In this case, robot $j$ needs to communicate with all other robots so that a new symbol $\sigma_{\text{next}}$ is selected. This process is repeated until regions $L_j^{\text{next}}$ are selected that make \eqref{eq:localProb} feasible. If such a symbol $\sigma_{\text{next}}$ does not exist, then this means that the transition from $q_D(t)$ to $q_D^{\text{next}}$ is infeasible, given the current multi-robot state $\bbp(t)$. Then, the pruned DFA is updated by removing this transition. Next, a new target DFA state is selected that is closer to the final state $q_F$ than $q_D(t)$ is. If there do not exist such DFA states then the robots cannot accomplish the assigned task. Note that this does not necessarily mean that Problem \ref{prob} is infeasible. %that there do not exist paths that satisfy the assigned LTL specification. 
%In fact, there may exist another sequence of DFA states for which  Problem \ref{prob} is always feasible. %; see also Section \ref{sec:complOpt}.
%Conditions under which \eqref{eq:localProb} (and, consequently, Problem \ref{prob}) is always feasible and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}.
%\end{rem}

%{\bf{Asynchronous Execution of Paths:}} 
\subsection{Asynchronous Execution of Paths}
The robots $j\in\ccalR_{\text{next}}$ execute their paths $\bbp_{j,t:T_j}$ \textit{asynchronously} until the time instant $T_j$, i.e., until they reach their respective target regions $L_j^{\text{next}}$ [line \ref{rrt:ExecReplan}, Alg. \ref{alg:RRT}]. At time $T_j$, robot $j$ waits for all other robots $e\in\ccalR_{\text{next}}$ with $T_e>T_j$. At time instant $T=\max_{j\in\ccalN_{\text{next}}}\{T_j\}$, i.e., when \textit{all} robots $j\in\ccalN_{\text{next}}$ have reached their respective regions $L_j^{\text{next}}$, the symbol $\sigma_{\text{next}}$ is generated. Then, the multi-robot system reaches the NBA state $q_B^{\text{next}}$ and a new NBA state is selected [lines \ref{rrt:T}-\ref{rrt:UpdGoals}]. This process is repeated indefinitely so that a final state is reached infinitely often.
%In Section \ref{sec:complOpt}, we show the robots remain in the NBA state $q_B(t)$ for all  $t'\in [t, T-1]$ and transition to $q_B^{\text{next}}$ occurs at the time instant $T$. Once this happens, the robots update their current DFA state and select the next DFA state [lines \ref{rrt:T}-\ref{rrt:UpdGoals}]. This process is repeated until the final state $q_F$ is reached.

%
%\begin{rem}\label{rem:invariant}
%Note that once the robots reach a new DFA $q_D$, they satisfy its respective Boolean condition $b_{\text{inv}}$, since the `next' temporal operator is excluded from the task specification. Particularly, if $b_{\text{inv}}$ is not satisfied this implies that once the robots are at locations that generate a symbol that triggers the transition to $q_D$, the robots should immediately leave their locations, which is impossible to specify unless the next operator is included in the specification language. 

%Recall that $\sigma_{\text{inv}}$ is selected to have the minimum length, this means that the minimum number of robots are involved to generate it. Therefore, robots that are required to generate the symbol $\sigma$ are not included in the set $\ccalR_{\text{inv}}$; see also Remark \ref{rem:invariant}.
%Similarly, robots that are responsible to satisfy $b_{\text{next}}$ cannot be responsible for generating the symbol $\sigma_{\text{inv}}$, since the next operator does not exist and all regions are assumed to be disjoint. %(unless there is an overlap..)
%\end{rem}


%\subsection{Online Re-planning}\label{sec:replan}






\begin{rem}[Communication]
%Note that Algorithm \ref{alg:RRT} requires all-time communication to ensure that all robots always have access to the same map $M(t)$. Nevertheless, this requirement can be straightforwardly relaxed by allowing each robot to build their local map $M_j(t)$. Moreover, 
Execution of the paths $\bbp_{j,t:T_j}$ does not require all-time communication among robots, which is typically the case in relevant temporal logic algorithms. Instead, communication is intermittent and is required only in the following two cases: (i) all robots need to communicate with each other to select the symbol $\sigma_{\text{next}}$ (ii) every robot $j\in\ccalR_{\text{next}}$ needs to send a message to all other robots in $\ccalR_{\text{next}}$ once it is ready to step into the region $L_{j}^{\text{next}}$. %; see Section \ref{sec:exec}.
\end{rem}

%Next, we define the set $\ccalL_j$ that collects all robot positions $\bbp_j$ that violate $b_{\text{inv}}$ regardless of the state of all other robots. For instance, if $b_{\text{inv}}=\neg (\pi_j^{r_e}\wedge \pi_z^{r_h})$, then $\ccalL_j=\emptyset$. On the other hand, if $b_{\text{inv}}=\neg (\pi_j^{r_e})\wedge (\neg \pi_z^{r_h})$ then  $\ccalL_j=\set{r_e}$. Formally, to construct the set, we express the negation of $b_{\text{inv}}$, denoted by $\bar{b}_{\text{inv}}=\neg b_{\text{inv}}$ as




==> files/proof2.tex <==
%In this section we provide the proof of Lemma \ref{lem:binv} required to prove that Algorithm \ref{alg:RRT} is complete. To prove this result, we need first to state the following results.

%First, we show that once the robots reach a DFA state $q_D^{\text{next}}$ they can remain in this state if they stay in their current configuration.

%\begin{lem}[Feasibility]\label{lem:feas}
%Assume that the robots reach a configuration $\bbp(t)$ that generates a word $\sigma=L(\bbp(t))$ which enables a transition to the DFA state $q_D^{\text{next}}$. Then, it holds that $\sigma\models b^{\text{inv}}$, where $b^{\text{inv}}$ is a Boolean formula that needs to be satisfied to remain in $q_D^{\text{next}}$. 
%\end{lem}

%\begin{proof}
%This result follows directly from the fact that the `next' operator is excluded from the syntax of the task specification language. Particularly, let $q_D^{\text{next}}$ denote the DFA state that the robots will reach from   $q_D^{\text{next}}$ if they stay put in $\bbp(t)$. In what follows, we show by contradiction that $q^{\text{next}}$ exists (i.e., staying in $\bbp(t)$ does not violate $\phi$) and  $q_D^{\text{next}}=q_D^{\text{next}}$. Assume that $q_D^{\text{next}}$ does not exist. This means that once the robots reach $\bbp(t)$ and the current DFA state becomes $q_D^{\text{next}}$, we have that $\delta(L(\bbp(t)),q_D^{\text{next}})=\varnothing$. This means that once the robots reach $\bbp(t)$ they should immediately leave it, beause otherwise the LTL formula is violated. This implies the existence of the `next' operator in the specification language which is not the case. Therefore, we conclude that $q_D^{\text{next}}$ exists.

%Next, we show that $q_D^{\text{next}}=q_D^{\text{next}}$. Assume $q_D^{\text{next}}\neq q_D^{\text{next}}$. This implies that once $L(\bbp(t))$ is generated and $q_D^{\text{next}}$ is reached, the robots should leave $\bbp(t)$ immediately in order to stay in $q_D^{\text{next}}$; otherwise $L(\bbp(t))$ will enable a subsequent transition to $q_D^{\text{next}}\neq q_D^{\text{next}}$. This also implies the existence of the `next' operator in the specification language which is not the case completing the proof.
%\end{proof}

%This implies that the same word $L(\bbp(t))$ enables first a transition from a DFA state $q_D$ to $q_D^{\text{next}}$ and second, once this happens, a transition from $q_D^{\text{next}}$ to $q_D^{\text{next}}$ is enabled immediately. This means that $q_D^{\text{next}}$ is a `dummy' state in the DFA which cannot happen 
%$\ccalR=\set{q\in\ccalQ_D~|~q=(L(\bbp(t)),q_D^{\text{next}})}$.
%
%if $\sigma\not\models b^{\text{inv}}$, then this means that once the robots reach the configuration $\bbp(t)$ and the current DFA state becomes $q_D(t)=q_D^{\text{next}}$, the robots should immediately leave from this configuration in order to stay in $q_D(t)$. This implies the existence of the `next' operator in the specification language which is not the case completing the proof.

%Next, let $\sigma_{\text{cur}}$ denote the word that the multi-robot system currently generates, i.e., $\sigma_{\text{cur}}=L(\bbp(t))$. Assume also that $\sigma_{\text{cur}}$ enables a transition from $q_D(t)$ to $q_D'\neq q_D(t)$. Let $b^{\text{inv}}$ be the Boolean formula that the robots should satisfy in order to remain in $q_D'$. Recall that in Lemma \ref{lem:feas}, we showed that  $\sigma_{\text{cur}}\models b^{\text{inv}}$, i.e., the robots can stay in the DFA state $q_D'$ as long as they stay idle. Next, we define the $\sigma^{\text{inv}}$ that is constructed by replacing in $\sigma_{\text{cur}}$ the maximum possible number of symbols with the empty string, so that $\sigma^{\text{inv}}$ still satisfies $b^{\text{inv}}$, i.e., $\sigma^{\text{inv}}\models b^{\text{inv}}$; see also Example \ref{ex4}. Let $\ccalR^{\text{inv}}$ be the robots that appear in $\sigma^{\text{inv}}$ and let $L_j^{\text{inv}}$ be the regions that robots $j\in\ccalR^{\text{inv}}$ have to belong to in order to generate $\sigma^{\text{inv}}$; see also Example \ref{ex4}. In the following lemma, we show that $\ccalR^{\text{inv}}$ and $\ccalR^{\text{next}}$ are disjoint sets.

%\begin{lem}[Conflict-free]\label{lem:confl}
%Let sets $\ccalR^{\text{inv}}$ be the set of robots that are responsible  and $\ccalR^{\text{next}}$ are disjoint. %If $\phi$ is satisfiable, then Algorithm \ref{alg:RRT} is conflict-free i.e., a robot $j\in\ccalR^{\text{inv}}$ that is required to stay idle will never have to solve \eqref{eq:localProb} to design a path towards a new region. 
%\end{lem}

%\begin{proof}
%Recall first that $\sigma^{\text{inv}}$ is the word with the minimum length that satisfies $b^{\text{inv}}$. This means that $\ccalR^{\text{inv}}$ does not involve `unnecessary' robots whose presence in a region $r_i$ does not affect the satisfaction of $b^{\text{inv}}$. The respective result also holds for $\sigma^{\text{next}}$. Note that this is important since otherwise, it is trivial to see that $\ccalR^{\text{inv}}$ and $\ccalR^{\text{next}}$ may not be disjoint.
%Given words $\sigma^{\text{inv}}$ and $\sigma^{\text{next}}$, assume that there exist a robot $j\in\ccalR^{\text{inv}}\cap\ccalR^{\text{next}}$. This means that according to the LTL task, robot $j$ has to be present in the region $L_j^{\text{inv}}$ for all time instants $t'\in[t,T)$ and in $L_{j}^{\text{next}}$ at the time instant $T$. Nevertheless, this is impossible to specify given that the `next' operator is not included in the task specification language.
%\end{proof}

 
%\begin{ex}[Construction of $\sigma^{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b^{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi_w^{r_2})\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$ (i.e., $\bbp_{j}\in r_1\cap r_2$). Then, we have that $\sigma^{\text{inv}}=\pi_j^{r_1}$, $\ccalR^{\text{inv}}=\set{j}$, and $L_j^{\text{inv}}=r_1$. Similarly, if $b^{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma^{\text{inv}}$ is an empty string and $\ccalR^{\text{inv}}=\emptyset$.
%\end{ex}
%, i.e., Algorithm \ref{alg:prune} will remove the multi-hop transition $q_B\rightarrow_B^K$ only if 

\subsection{Proof of Lemma \ref{lem:fragmentLTL}}
%\begin{proof}
To show this result, first we express all Boolean formulas $b^{q_B,q_B'}$ associated with any NBA transition $\delta(q_B,\cdot,q_B')$ in CNF, i.e., as a conjunction of $F$ Boolean formulas $b_f$, for some $F>0$, where $b_f$ is a disjunction of literals, i.e.,
\begin{equation}\label{eq:bqbqb}
    b^{q_B,q_B'}=\bigwedge_{f=1}^F b_f.
\end{equation}
%Assume that all literals in a clause $b_f$ are associated with only one robot, for all $f\in\{1,\dots,F\}$. 
%In what follows, we show by contradiction that Algorithm \ref{alg:prune} is not conservative if every clause $b_f$ is associated with only one robot, for all $f\in\{1,\dots,F\}$.
By Assumption \ref{as:cnf} we have that every clause $b_f$ is associated with only one robot, for all $f\in\{1,\dots,F\}$. Let $\ccalF_j$ be a set that collects all indices $f\in\{1,\dots,F\}$ to formulas $b_f$ that are associated with robot $j$, where $\ccalF_j\cap\ccalF_i=\emptyset$, for all $i,j\in\ccalN$, by definition of $b_f$. Next we define the Boolean formula 
\begin{equation}\label{eq:dj}
    d_j^{q_B,q_B'}=\bigwedge_{j\in\ccalF_j}b_f,
\end{equation}
which is a conjunction of all Boolean formulas $b_f$ associated with robot $j$ that appear in \eqref{eq:bqbqb}. Using \eqref{eq:dj} and the fact that $\ccalF_j\cap\ccalF_i=\emptyset$, for all $i,j\in\ccalN$, we can re-write \eqref{eq:bqbqb} as 
\begin{equation}\label{eq:bqbqb2}
    b^{q_B,q_B'}=\bigwedge_{j=1}^N d_j^{q_B,q_B'}.
\end{equation}
Thus, if Assumption \ref{as:cnf} holds, then the Boolean formula $b^{q_B,q_B'}$ defined in \eqref{eq:b} can be decomposed into local/decoupled sub-formulas $d_j^{q_B,q_B'}$ as in \eqref{eq:bqbqb2}. In other words, robot $j$ can make decisions to contribute to satisfaction of $b^{q_B,q_B'}$ independent from other robots by considering only the sub-formula $d_j^{q_B,q_B'}$. 

Due to the decomposition of \eqref{eq:b} as per \eqref{eq:bqbqb2}, we can apply Definition \ref{def:feas} locally to each robot as follows. %
Specifically, a transition $\delta_B^m(q_B,\cdot,q_B')$ is decomposable if the following condition holds for all robots $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$. For all symbols $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}_j$, there should exist at least one symbol $\sigma^{q_B,q_B'}_j$ that satisfies $d_j^{q_B,q_B^K}$ (i) and either (A) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B'}$. 
%Note that since symbols $\sigma^{q_B,q_B^K}$ that satisfy condition (i) exist, this means $L_{j}^{q_B,q_B^K}$ is unique/well-defined for all robots $j\in\ccalR^{q_B,q_B^K}$.
Assume that there exists at least one robot $j$ for which this condition is not satisfied i.e., there exists at least one symbol $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}_j$ for which there are no such $\sigma^{q_B,q_B'}_j$. This means that there exists $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. Since $j\in\ccalR^{q_B,q_B}$, we have that transition towards the state $q_B$ was enabled because robot $j$ reached a region of interest $L_{j}^{q_B,q_B}$. Also, since $j\in\ccalR^{q_B,q_B'}$, we get that transition from $q_B$ to $q_B'$ will be enabled only if robot $j$ visits a region of interest denoted by $L_{j}^{q_B,q_B'}$. By assumption we have that $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. Therefore, we conclude that if Definition \ref{def:feas} is not satisfied then transition from $q_B$ to $q_B'$ can be enabled only if robot $j$ keeps being in a region of interest $L_{j}^{q_B,q_B}$ until it reaches another region $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$, which is impossible given that all regions of interest are disjoint completing the proof.
%\end{proof}
%(i.e. the only NBA transitions that will be removed are the ones that require a robot does not include any Boolean subformula of the form $\vee_{j\ccalR}(\pi_j)$

%\subsection{Proof of Lemma \ref{thm:nonexist}}
%We show this result by contradiction. Assume that there exists a solution to Problem \ref{prob}. If there exists a solution to Problem \ref{prob} and Assumption (b) holds then we have that in $\ccalG$ there are states $q_B,q_B'\in\ccalV$ for which there does not exist a corresponding edge $(q_B,q_B')\notin\ccalE$ while the corresponding transitions $\delta_B^m(q_B,\cdot,q_B')$ can be enabled by the robots, i.e., without requiring them to instantaneously jump from one location to another one or being present in more than one location at the same time. Let $\delta_B^m(q_B,\cdot,q_B')$ be such a transition.
%
%Since $(q_B,q_B')\notin\ccalE$ this means that either (i) there does not exists a (feasible) symbol $\sigma^{q_B,q_B'}$ that satisfies $b^{q_B,q_B'}$ defined in \eqref{eq:b} or (ii) there exist symbols $\sigma^{q_B,q_B'}$ that satisfy $b^{q_B,q_B'}$ but none of them satisfies Definition \ref{def:feas}. By definition of $b^{q_B,q_B'}$ we have that in case (i), the state  $q_B'$ can be reached from $q_B$ only if the robots can instantaneously jump from one location to another one. Nevertheless, this contradicts the assumption that $\delta_B^m(q_B,\cdot,q_B')$ can be enabled without requiring the robots to instantaneously jump from one location to another one. Thus, case (i) cannot happen i.e., there exists at least one symbol  $\sigma^{q_B,q_B'}$ that satisfies $b^{q_B,q_B'}$. Due to assumption (a) and since case (i) cannot happen, we get from Lemma \ref{lem:fragmentLTL} that $\delta_B^m(q_B,\cdot,q_B')$ satisfies the condition mentioned in Definition \ref{def:feas} and, therefore, case (ii) cannot happen either. Thus, $\ccalG$ collects all edges that correspond to transitions $\delta_B^m(q_B,\cdot,q_B')$ that can be enabled by the robots which contradicts the assumption that there exists a solution to Problem \ref{prob}.

\subsection{Proof Of Proposition \ref{thm:completeness}}

To prove that Algorithm \ref{alg:RRT} is complete, we need first to state the following Lemma. The proof is omitted due to space limitations.
%Given the above results, we can state the following result.
\begin{lem}\label{lem:binv}
Assume that at time $t$ the robots reach a state $q_B(t)\in\ccalV$ and design paths $\bbp_{j,t:T_j}$ to reach  $q_B^{\text{next}}\in\ccalV$.
%Assume that there are no regions $r_i$ and $r_j$, such that $r_i\subseteq r_j$. Then,  %% condition for feasibility
If the robots execute and update the paths $\bbp_{j,t:T_j}$, as per Section \ref{sec:exec}, and eventually they reach their goal regions $L_j^{\text{next}}$ then the transition from $q_B$ to $q_B^{\text{next}}$ will be activated. % at the time instant $T=\max_{j\in\ccalN^{\text{next}}} \{T_j\}$.
\end{lem}


\begin{proof}
For simplicity of notation, let $b^{\text{inv}}$ and $b^{\text{next}}$ denote the Boolean formulas that should be true to enable a transition from $q_B$ to $q_B$ and from $q_B$ to $q_B^{\text{next}}$, respectively. Once the robots reach $q_B(t)$, they coordinate to select symbol $\sigma^{\text{next}}$ that satisfies $b^{\text{next}}$. By assumption, all robots will eventually reach their assigned locations $L_{j}^{\text{next}}$ but not necessarily at the same time instant. When this happens, a time instant $T$, the symbol $\sigma^{\text{next}}$ that satisfies $b^{\text{next}}$ will be generated.
%By construction of Algorithm \ref{alg:RRT} there exists a time instant $T$ when the symbol $\sigma^{\text{next}}$ will be generated. Specifically, since the environment is static, we have that re-planning will be required a finite number of times. As a result, all robots $\ccalN^{\text{next}}$ will eventually reach their assigned locations $L_{j}^{\text{next}}$ and the symbol $\sigma^{\text{next}}$ will be generated. 
Thus, to show that at time $T$ the transition from $q_B$ to $q_B^{\text{next}}$ will be enabled, it suffices to show that $b^{\text{inv}}$ is satisfied for all $t'\in [t,T)$.\footnote{Note that the transition from $q_B$ to $q_B^{\text{next}}$ is, in general, a multi-hop transition; see \eqref{eq:run}. Thus, formally, if the length of the this transition is $K$ hops, then once the robots generate $\sigma^{\text{next}}$ they should stay idle at their current locations $K-1$ time steps to reach $q_B^{\text{next}}$. Thus, formally,  transition to $q_B^{\text{next}}$ will occur at the time instant $T+K-1$.}% since at time $T$ $q_B^{\text{next}}$ can be reached from $q_B(t)$. 


%To show this result, it suffices to show that there exists a time instant $T$ so that $b^{\text{inv}}$ is satisfied during the time interval $[t,T)$ and $b^{\text{inv}}$ is satisfied at time $T$. 


%The reason is that if $b^{\text{inv}}$ is satisfied, then the robots can always remain in $q_B(t)$ for all $t'\in [t,T)$. If the robots remain in $q_B(t)$ for all $t'\in [t,T)$, then at the time instant $T=\max_j \{T_j\}$, the transition from $q_B(t)$ to $q_B^{\text{next}}$ can be enabled, since at that time the robots $j\in\ccalN^{\text{next}}$ will generate the symbol $\sigma^{\text{next}}$ by construction of Algorithm \ref{alg:RRT}.\footnote{Note that the transition from $q_B(t)$ to $q_B^{\text{next}}$ is, in general, a multi-hop transition. Thus, formally, if the length of the this transition is $K$ hops, then once the robots generate $\sigma^{\text{next}}$ they should wait $K-1$ time steps to reach $q_B^{\text{next}}$.} %[\red{explain the last sentence a bit more; add 1-2 sentences}].

%Recall that the symbol $\sigma^{\text{next}}$ satisfies the Boolean formula $b^{\text{next}}$ defined in \eqref{eq:b}. 
%
%Since $q_B(t)\in\ccalV$ and $\sigma^{\text{next}}\models b^{\text{next}}$, where $b^{\text{next}}$ is defined in \eqref{eq:b},
By construction of Algorithm \ref{alg:RRT}, we have that once the robots reach any state in $q_B\in\ccalV$, the corresponding Boolean formula $b^{q_B,q_B}$ is satisfied by definition of \eqref{eq:b}. Thus, at time $t$ the multi-robot state $\bbp(t)$ satisfies the Boolean formula $b^{\text{inv}}$ is satisfied. As a result, if all robots in the set $\ccalN^{\text{inv}}$ (i.e., the robots that appear in $b^{\text{inv}}$) remain idle, the Boolean formula $b^{\text{inv}}$ will remain satisfied. Recall that robots $j\in\ccalN^{\text{next}}$ navigate the environment by following paths design as per \eqref{eq:localProb} 
%and executing them as discussed in Section \ref{sec:exec}.
while it may hold that $\ccalN^{\text{next}}\cap\ccalN^{\text{inv}}\neq \emptyset$. In what follows, we show that $q_B(t)=q_B(t')$ for all $t'\in[t,T)$. %Let $R_j^t$ be the region $r_i$ that the robots lie in at the time instant $t$. If  robot $j$ does not belong to any region $r_i$, i.e., $L(\bbp_{j}(t))=\varnothing$, then $R_j^t$ is not defined i.e., $R_j^t=\varnothing$. 
%
To show this, first recall that the robots $j\in\ccalR^{\text{inv}}\subseteq\ccalN^{\text{inv}}$ stay idle by construction of Alg. \ref{alg:RRT} and, therefore, they cannot violate $b^{\text{inv}}$. Thus. it suffices to show that the robots $j\in\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}$, where $\bar{\ccalR}^{\text{inv}}=\ccalN^{\text{inv}}\setminus\ccalR^{\text{inv}}$ will not violate $b^{\text{inv}}$. To show this we consider two cases. 

First, assume that $\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}=\emptyset$. Then this means that all robots in $\ccalN^{\text{inv}}$ will stay idle and, therefore, $b^{\text{inv}}$ will not be violated. Second assume that there exist robots $j\in\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}$. By construction of the set $\bar{\ccalR}^{\text{inv}}$ we have that atomic predicates $\pi_j^{\ell_e}$ associated with robots $j\in\bar{\ccalR}^{\text{inv}}$ and for some regions $\ell_e$ appear in $b^{\text{inv}}$ only with a negation operator in front of them (i.e., in the following form $\neg\pi_j^{\ell_e}$). In other words, robots $j\in\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}$ will violate $b^{\text{inv}}$ only if they visit certain regions of interest as they move towards locations $\bbq\in\Omega$, where no atomic predicates are satisfied. Nevertheless, this is precluded by the first constraint in \eqref{eq:localProb} meaning that at time $T$ transition from $q_B(t)$ to $q_B^{\text{next}}$ will be activated. Finally, note that this result holds even if the robots execute their paths asynchronously, i.e., if the (continuous) time required to move from $\bbp_j(t)$ to $\bbp_j(t+1)$ is different across the robots. The reason is that (i) generation of $\sigma_{\text{next}}$ does not depend on the order where the robots arrive at their goal locations $L_{j}^{\text{next}}$, (ii) satisfaction of $b^{\text{inv}}$ cannot be affected by the asynchronous execution of paths $\bbp_{j,t:T_j}$,  $j\in\ccalN^{\text{next}}$. The latter is true because 
in $b^{\text{inv}}$, there are no Boolean variables associated with robots $j\in\bar{\ccalR}^{\text{inv}}\cap\ccalN^{\text{next}}$ and, therefore,
the (synchronous or asynchronous) actions of these robots does not play any role in satisfying $b^{\text{inv}}$. Also, as discussed before, the (synchronous or asynchronous) actions of the robots $j\in\bar{\ccalR}^{\text{inv}}$ cannot violate $b^{\text{inv}}$ as long as they avoid certain regions, which is guaranteed by construction of the paths completing the proof.\end{proof}




{\bf{Proof of Proposition \ref{thm:completeness}:}} To show this result it suffices to show that eventually the accepting condition of the NBA is satisfied, i.e., the robots will visit at least one the final NBA states $q_F$ infinitely often. 
Equivalently, as discussed on Section \ref{sec:dist}, it suffices to show that accepting edges $(q_B,q_B')\in\ccalE$, where $q_B,q_B'\in\ccalV$ are traversed infinitely often. 

First, consider an infinite sequence of time instants $\bbt=t_0,t_1,\dots,t_k,\dots$ where $t_{k+1}\geq t_k$, so that an edge in $\ccalG$, defined in Section \ref{sec:dist}, is traverses at every time instant $t_k$. Let $e(t_k)\in\ccalE$ denote the edge that is traversed at time $t_k$. Thus, $\bbt$ yields the following sequence of edges $\bbe=e(t_0),e(t_1),\dots,e(t_k)\dots$ where $e(t_k)=(q_B(t_{k}),q_B(t_{k+1}))$, $q_B(t_0)=q_B^{\text{aux}}$, $q_B(t_k)\in\ccalV$, and the state $q_B^{k+1}$ is defined based on the following two cases. 
%
If $q_B(t_k)\notin \ccalV_F$, then the state $q_B(t_{k+1})$ is closer to $\ccalV_F$ than $q_B(t_k)$ is, i.e., $d_F(q_B(t_{k+1}),\ccalV_F)=d_F(q_B(t_{k}),\ccalV_F)-1$, where $d_F$ is defined in \eqref{eq:distF}. If $q_B(t_{k})\in\ccalV_F$, then $q_B(t_{k+1})$  is selected so that an accepting edge originating from $q_B(t_{k})$ is traversed. By definition of $q_B(t_{k})$, the `distance' to $\ccalV_F$ decreases as $t_k$ increases, i.e., given any time instant $t_k$, there exists a time instant $t_k'\geq t_k$ so that $q_B(t_{k}')\in\ccalV_F$ and then at the next time instant an accepting edge is traversed. This means that $\bbe$ includes an infinite number of accepting edges. This sequence $\bbe$ exists by assumption (a). Note that if assumption (a) does not hold, Algorithm \ref{alg:RRT} cannot find a solution even if it exists.
%

Assume that there exists a solution to Problem \ref{prob}. Assume that the robots navigate the environment as per Algorithm \ref{alg:RRT} and update the graph $\ccalG$ by removing edges as described in Section \ref{sec:replan}. To show that Algorithm \ref{alg:RRT} is complete, it suffices to show that it can generate a infinite sequence of edges $\bbe$ as defined before.


%of edges in the graph $\ccalG$, defined in Section \ref{sec:dist}, defined as $\ccalE=e(0),e(t_1_,\dots,e(t_k)\dots$, that includes an infinite number of accepting edges associated with $q_F^{\text{loop}}\in\ccalQ_F^{\text{loop}}$ infinitely often, where $e(t_k)=(q_B(t_k-1),q_B^{k+1})$, $q_B^0=q_B^{\text{aux}}$, and the state $q_B^{k+1}$ is selected as discussed in Section \ref{sec:planning}. Specifically, if $q_B^k\neq q_F^{\text{loop}}$, then the state $q_B^{\text{next}}=q_B^{k+1}$ is selected so that it is closer to $q_F^{\text{loop}}$ than $q_B^k$ is, i.e., $d(q_B^{k+1},q_F^{\text{loop}})=d(q_B^{k},q_F^{\text{loop}})-1$. If $q_B^k= q_F^{\text{loop}}$, then $q_B^{k+1}$ is selected so that an accepting edge originating from $q_F^{\text{loop}}$ is traversed. 
%


We show that a sequence $\bbe$ exists by induction. Specifically, we show that if there exists a time instant $t_k$ when the robots reach an NBA state denoted by $q_B(t_k)\in\ccalV$ there exists a time instant $t_{k+1}\geq t_k$ when the robots will reach a new state $q_B(t_{k+1})=q_B^{\text{next}}\in\ccalV$ where $q_B(t_{k+1})$ satisfies the conditions discussed before. 
%
At time $t=0$, we have that $q_B(0)=q_B^{\text{aux}}\in\ccalV$. By construction of Algorithm \ref{alg:RRT} the robots select a new state $q_B^{\text{next}}$ that they should reach next in the same way as discussed before. 
%
%Let $\sigma^{\text{next}}$ be the symbol that the robots decided to generate to enable the transition from $q_B(0)$ to $q_B^{\text{next}}$. Paths $\bbp_{j,t:T_j}$ that should be followed to generate $\sigma^{\text{next}}$ are designed by solving \eqref{eq:localProb}.
%
Since  $q_B(0)\in\ccalV$ then due to Lemma \ref{lem:binv}, we have that if robot paths $\bbp_{j,t:T_j}$ that solve \eqref{eq:localProb} always exist, as the map is updated, i.e., the robots eventually reach their regions $L_j^{\text{next}}$, then transition from $q_B(t_0)$ to $q_B^{\text{next}}$ will be eventually enabled. 
%$\sigma^{\text{next}}$ satisfies the Boolean formula $b^{q_B(0),q_B^{\text{next}}}$ defined in \eqref{eq:b}, we have that the Boolean formula $b^{q_B^{\text{next}},q_B^{\text{next}}}$ is satisfied.
%
Note that \eqref{eq:localProb} is always feasible, as the map is updated, due to assumption (b); this also means that edges in the graph $\ccalG$ will be never deleted. Also, as the robots follow the paths as per Algorithm \ref{alg:RRT}, it will never hit an obstacle due to assumption (c). Particularly, by assumption (c) the robot is equipped with an omnidirectional sensor, as per \eqref{eq:sensor}. %, the robot will always be aware of all obstacles within range $R$. 
Thus, if the path $\bbp_{j,t:T_j}$ passes through an obstacle, robot $j$ will always detect it and will re-solve \eqref{eq:localProb} to update its path. 
%
Since \eqref{eq:localProb} is always feasible, we get that there exists a time instant $t_0\geq 0$ when the robots will reach a new state $q_B^{\text{next}}\in\ccalV$. The induction step follows. Assume that at a time instant $t_{k}$ the robots reach a state $q_B(t_{k})\in\ccalV$ from a state $q_B(t_{k-1})\in\ccalV$. Following the same logic as for $t_0$, we can show that there exists a time instant $t_{k+1}\geq t_k$ when the robots reach $q_B^{t_{k+1}}\in\ccalV$ completing the proof.



\subsection{Proof of Proposition \ref{thm:exist}}
By Assumption (a) we have that there exists an infinite sequence of edges $\bbe=e_0,e_1,\dots,e_k\dots$ in $\ccalG$ that includes an infinite number of accepting edges where, with slight abuse of notation,  $e_k=(q_B^k,q_B^{k+1})$, $q_B^k\in\ccalV$ for all $k\geq 0$. To show that a solution to Problem \ref{prob} exists, it suffices to show that there exists a sequence of paths in $\Omega$ that the robots can follow to enable all edges $e_k$. We show this by induction. % can be enabled without requiring the robots to instantaneously jump from one location to another or be in more than one location simultaneously while respecting the robot dynamics. We show this by induction. 

First, we focus on the transition $e_0=(q_B^0,q_B^1)$ where $q_B^0=q_B^{\text{aux}}$. By construction of $q_B^{\text{aux}}$, we have that the initial multi-robot state satisfies the Boolean formula $b^{q_B^0,q_B^0}$ associated with the self loop of $q_B^0$. Due to the fact that $e_0\in\ccalE$ we get that the corresponding transition $\delta_B^m(q_B^0,\cdot,q_B^1)$ is decomposable. Therefore there exist paths that can enable the transition from $q_B^0$ to $q_B^1$. Specifically, as shown in Lemma \ref{lem:binv}, such paths can be computed by solving local reachability problems as in \eqref{eq:localProb} where \eqref{eq:localProb} is always feasible by Assumption (b). Thus, eventually, the transition $e_0$ will  be enabled. The induction step follows. Assume that all edges $e_0$, $e_1, \dots,e_{k-1}$ have been enabled and paths that reach the state $q_B^k$  and activate the Boolean formula $b^{q_B^k,q_B^k}$ have been designed. Following the same logic as for the edge $e_0$, we can show that there exist paths that can enable the edge $e_k$ completing the proof. 

==> files/proofs.tex <==
%In this section we provide the proof of Lemma \ref{lem:binv} required to prove that Algorithm \ref{alg:RRT} is complete. To prove this result, we need first to state the following results.

%First, we show that once the robots reach a DFA state $q_D^{\text{next}}$ they can remain in this state if they stay in their current configuration.

%\begin{lem}[Feasibility]\label{lem:feas}
%Assume that the robots reach a configuration $\bbp(t)$ that generates a word $\sigma=L(\bbp(t))$ which enables a transition to the DFA state $q_D^{\text{next}}$. Then, it holds that $\sigma\models b_{\text{inv}}$, where $b_{\text{inv}}$ is a Boolean formula that needs to be satisfied to remain in $q_D^{\text{next}}$. 
%\end{lem}

%\begin{proof}
%This result follows directly from the fact that the `next' operator is excluded from the syntax of the task specification language. Particularly, let $q_D^{\text{next}}$ denote the DFA state that the robots will reach from   $q_D^{\text{next}}$ if they stay put in $\bbp(t)$. In what follows, we show by contradiction that $q_{\text{next}}$ exists (i.e., staying in $\bbp(t)$ does not violate $\phi$) and  $q_D^{\text{next}}=q_D^{\text{next}}$. Assume that $q_D^{\text{next}}$ does not exist. This means that once the robots reach $\bbp(t)$ and the current DFA state becomes $q_D^{\text{next}}$, we have that $\delta(L(\bbp(t)),q_D^{\text{next}})=\varnothing$. This means that once the robots reach $\bbp(t)$ they should immediately leave it, beause otherwise the LTL formula is violated. This implies the existence of the `next' operator in the specification language which is not the case. Therefore, we conclude that $q_D^{\text{next}}$ exists.

%Next, we show that $q_D^{\text{next}}=q_D^{\text{next}}$. Assume $q_D^{\text{next}}\neq q_D^{\text{next}}$. This implies that once $L(\bbp(t))$ is generated and $q_D^{\text{next}}$ is reached, the robots should leave $\bbp(t)$ immediately in order to stay in $q_D^{\text{next}}$; otherwise $L(\bbp(t))$ will enable a subsequent transition to $q_D^{\text{next}}\neq q_D^{\text{next}}$. This also implies the existence of the `next' operator in the specification language which is not the case completing the proof.
%\end{proof}

%This implies that the same word $L(\bbp(t))$ enables first a transition from a DFA state $q_D$ to $q_D^{\text{next}}$ and second, once this happens, a transition from $q_D^{\text{next}}$ to $q_D^{\text{next}}$ is enabled immediately. This means that $q_D^{\text{next}}$ is a `dummy' state in the DFA which cannot happen 
%$\ccalR=\set{q\in\ccalQ_D~|~q=(L(\bbp(t)),q_D^{\text{next}})}$.
%
%if $\sigma\not\models b_{\text{inv}}$, then this means that once the robots reach the configuration $\bbp(t)$ and the current DFA state becomes $q_D(t)=q_D^{\text{next}}$, the robots should immediately leave from this configuration in order to stay in $q_D(t)$. This implies the existence of the `next' operator in the specification language which is not the case completing the proof.

%Next, let $\sigma_{\text{cur}}$ denote the word that the multi-robot system currently generates, i.e., $\sigma_{\text{cur}}=L(\bbp(t))$. Assume also that $\sigma_{\text{cur}}$ enables a transition from $q_D(t)$ to $q_D'\neq q_D(t)$. Let $b_{\text{inv}}$ be the Boolean formula that the robots should satisfy in order to remain in $q_D'$. Recall that in Lemma \ref{lem:feas}, we showed that  $\sigma_{\text{cur}}\models b_{\text{inv}}$, i.e., the robots can stay in the DFA state $q_D'$ as long as they stay idle. Next, we define the $\sigma_{\text{inv}}$ that is constructed by replacing in $\sigma_{\text{cur}}$ the maximum possible number of symbols with the empty string, so that $\sigma_{\text{inv}}$ still satisfies $b_{\text{inv}}$, i.e., $\sigma_{\text{inv}}\models b_{\text{inv}}$; see also Example \ref{ex4}. Let $\ccalR_{\text{inv}}$ be the robots that appear in $\sigma_{\text{inv}}$ and let $L_j^{\text{inv}}$ be the regions that robots $j\in\ccalR_{\text{inv}}$ have to belong to in order to generate $\sigma_{\text{inv}}$; see also Example \ref{ex4}. In the following lemma, we show that $\ccalR_{\text{inv}}$ and $\ccalR_{\text{next}}$ are disjoint sets.

%\begin{lem}[Conflict-free]\label{lem:confl}
%Let sets $\ccalR_{\text{inv}}$ be the set of robots that are responsible  and $\ccalR_{\text{next}}$ are disjoint. %If $\phi$ is satisfiable, then Algorithm \ref{alg:RRT} is conflict-free i.e., a robot $j\in\ccalR_{\text{inv}}$ that is required to stay idle will never have to solve \eqref{eq:localProb} to design a path towards a new region. 
%\end{lem}

%\begin{proof}
%Recall first that $\sigma_{\text{inv}}$ is the word with the minimum length that satisfies $b_{\text{inv}}$. This means that $\ccalR_{\text{inv}}$ does not involve `unnecessary' robots whose presence in a region $r_i$ does not affect the satisfaction of $b_{\text{inv}}$. The respective result also holds for $\sigma_{\text{next}}$. Note that this is important since otherwise, it is trivial to see that $\ccalR_{\text{inv}}$ and $\ccalR_{\text{next}}$ may not be disjoint.
%Given words $\sigma_{\text{inv}}$ and $\sigma_{\text{next}}$, assume that there exist a robot $j\in\ccalR_{\text{inv}}\cap\ccalR_{\text{next}}$. This means that according to the LTL task, robot $j$ has to be present in the region $L_j^{\text{inv}}$ for all time instants $t'\in[t,T)$ and in $L_{j}^{\text{next}}$ at the time instant $T$. Nevertheless, this is impossible to specify given that the `next' operator is not included in the task specification language.
%\end{proof}

 
%\begin{ex}[Construction of $\sigma_{\text{inv}}$]\label{ex4}
%Consider the Boolean formula  $b_{\text{inv}}=(\pi_j^{r_1}\vee \pi_e^{r_3} )\wedge (\neg \pi_w^{r_2})\wedge (\neg \pi^{\text{obs}})$, where $\pi^{\text{obs}}$ is true if at least one of the robots hits an obstacle. Also, assume that $\sigma_{\text{cur}}=\pi_j^{r_1}\pi_j^{r_2}\pi_e^{r_3}$ (i.e., $\bbp_{j}\in r_1\cap r_2$). Then, we have that $\sigma_{\text{inv}}=\pi_j^{r_1}$, $\ccalR_{\text{inv}}=\set{j}$, and $L_j^{\text{inv}}=r_1$. Similarly, if $b_{\text{inv}}= (\neg \pi^{\text{obs}})$, then $\sigma_{\text{inv}}$ is an empty string and $\ccalR_{\text{inv}}=\emptyset$.
%\end{ex}
%, i.e., Algorithm \ref{alg:prune} will remove the multi-hop transition $q_B\rightarrow_B^K$ only if 

\begin{assumption}\label{as:cnf}
Let $b^{q_B,q_B^K}$ be a Boolean formula, defined in \eqref{eq:b}, written in conjunctive normal form (CNF) that enables a transition from $q_B$ to $q_B^K$. Assume that all literals in any given clause of $b^{q_B,q_B^K}$ are associated with only one robot, which is not necessarily the same across different clauses.
\end{assumption}

\begin{lem}\label{lem:fragmentLTL}
%Consider an LTL formula $\phi$ defined over atomic predicates $\pi_j^{\ell_i}$ where $j\in\ccalN$ and $\{\ell_i\}_{i\in\ccalL}$ denote disjoint regions of interest. 
Consider any finite run in the form of \eqref{eq:run}. Assume that there exists a symbol $\sigma^{q_B,q_B^K}$ that satisfies the corresponding Boolean formula $b^{q_B,q_B^K}$ defined in \eqref{eq:b}. Under Assumption \eqref{as:cnf}, the transition from $q_B$ to $q_B^K$ is always decomposable as per Definition \eqref{def:feas} unless this transition requires robots to instantaneously jump from one region of interest to another one which is impossible.
%%%
%Let $\bbp(t)$ and $\bbq_B(t)$ be the multi-robot and NBA state respectively at time $t$ and assume that $L(\bbp(t))\models b^{q_B(t),q_B(t)}$. Consider any transition $q_B(t)\rightarrow_B^K q_B'$, defined in Section \ref{sec:prune}.Let the corresponding Boolean formula $b^{q_B(t),q_B'}_K$ be written in conjunctive normal form (CNF). If every clause of $b^{q_B(t),q_B'}_K$ are associated with only one robot (not necessarily the same across different clauses), then Algorithm \ref{alg:prune} is not conservative.
%%%
%Assume that at time $t$ the current NBA state is $q_B(t)$ and the current multi-robot state $\bbp(t)$ satisfies $b_{q_B,q_B}$, i.e., $\bbp(t)\models b_{q_B,q_B}$. Let $b^{q_B,q_B'}_K$ denote the Boolean formula, defined in condition (i) Definition \ref{def:feas}, written in conjunctive normal form (CNF) that that needs to be satisfied to enable the NBA transition $q_B\rightarrow_B^K q_B'$. If the literals in any clause of $b^{q_B,q_B'}_K$ are associated with only one robot, then Algorithm \ref{alg:prune} is not conservative. % i.e., it will remove transition $q_B\rightarrow_B^K q_B'$ only if it can be enabled only if regions of interest were not disjoint.
%
%Also, let $b$ denote any Boolean sub-formula of $\phi$. Assume that there are no Boolean sub-formulas of the form $b=\vee_{j\in\ccalR}[\triangle_{r_{e_j}\in\ccalL}(\pi_j^{r_{e_j}})]$ with $|\ccalR|>1$ in $\phi$, where $\ccalR\subseteq\ccalN$ is set of robot indices and $\ccalL$ is set of regions of interest. %then the pruning approach as per Definition \ref{def:feas} is not conservative, i.e., only the non-physically realizable NBA transitions will be removed.
%
%Assume that the current NBA state is $q_B$ and the current multi-robot state $\bbp$ satisfies $b_{q_B,q_B}$. Then Algorithm \ref{alg:prune} has removed transitions originating from $q_B$ only if they can be enabled only if regions of interest were not disjoint.
%Consider any $q_B\rightarrow_B^K q_B'$ where $q_B,q_B'\in\ccalQ_B\setminus\hat{\ccalQ}_B$ and a. Under assumption (*), the pruning approach as per Algorithm \ref{alg:prune} is not conservative i.e., it will remove transitions that can be enabled only if regions of interest were not disjoint.
\end{lem}
\begin{proof}
%Consider the Boolean formula $b^{q_B,q_B^1}$ associated with any NBA transition $q_B\rightarrow_B q_B^1$ where $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$. Hereafter, 
%
%Recall that Definition \ref{def:feas} is not satisfied if transition from $q_B$ to $q_B'$ requires robots to jump from one region to another one  is conservative due to Def
%
Recall that Algorithm \ref{alg:prune} removes transitions in two cases. First, a transition $\delta_B(q_B\cdot,q_B')$, where $q_B,q_B'\in\ccalQ_B$, will be removed if $\Sigma^{q_B,q_B'}\neq\emptyset$, i.e., if this transition can be enabled only if at least one robot should be present in more than one location simultaneously. Second, a transition
$\delta_B(q_B\cdot,q_B^1)$, where $q_B\neq q_B^1$ is removed if it does not satisfy Definition \ref{def:feas} which, as discussed in Remark \ref{rem:conserv}, is conservative.

First, we show that condition (i) in Definition \ref{def:feas} is not conservative, in the sense that it only removes transitions that require robots to jump from one region of interest to another one (i.e., go from $r_e$ to $r_m$, $m\neq e$ with visiting any location $\bbq$ where $L(\bbq)=\varnothing$) or be physically present in more than one location which is impossible given that non-overlapping regions are considered. According to condition (i)-(A) of Definition \ref{def:feas}, a transition $\delta_B(q_B,\cdot, q_B^1)$, $q_B\neq q_B^1$, is feasible if there exists at least one symbol, denoted by $\sigma^{q_B,q_B^K}$ and a finite $K\geq 1$, so that $\sigma^{q_B,q_B^K}$ satisfies $b_{q_B,q_B^K}^K$, where
\begin{equation}\label{eq:bK}
    b_{q_B,q_B^K}=\underbrace{b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}}_{=b}\wedge b_{q_B^{K},q_B^{K}}.
\end{equation}
%Due to \eqref{eq:bqbqb2}, we can rewrite \eqref{eq:bK} as
%\begin{equation}\label{eq:bqbqb2}
%    b^{q_B,q_BK}=\bigwedge_{j=1}^N d_j^{q_b,q_B^K}.
%\end{equation}

Assume that condition (i)-(A) is not satisfied. There are three cases when this may happen:
(a) First, there may no states (other than the auxiliary states) with feasible self-loops, i.e., the Boolean formula $b_{q_B^{K}},q_B^{K}$ is not defined. This means that if the transition from $q_B$ to $q_B^1$ is activated then the only way to visit a final state is to instantaneously move/jump from one NBA state to another one, since no self-loops exist, unless condition (i)-(B) is true. In words, condition (i)-(B) requires that there exists a symbol that if it is repeated indefinitely after reaching $q_B$, a final state will be visited infinitely often. If (i)-(B) is not true, then in this case we have visiting a final state requires robots to `jump' from one region of interest to another one or be in more than one location simultaneously which is not possible. %Note that Then, clearly, if (B) is not satisfied either, there is no way after taking the transition from $q_B$ to $q_B^1$ to eventually visit a final state. [correctly removed regardless of B]
(b) Second, there may exist states with feasible self-loops but they cannot be reached, i.e., there does not exist a sequence of states $q_B^k$ towards any state $q_B^K$ that has a self-loop so that the corresponding $b$ formula is satisfied. Thus visiting states with self-loops requires the robot to jump from one region to another or be at more than one region simultaneously (in order to satisfy $b$ which is impossible. Thus, this means that after activating a transition from $q_B$ to $q_B^1$ (recall that $b_{q_B,q_B^1}$ does not require simultaneous presence in more than one location for any robot), the only way to visit a final state is to instantaneously move from one NBA state to another one which is not possible as discussed in (a) unless (B) is true.
%in order to reach a state and stay there (i.e., enable its corresponding self-loop) robots should be able to `jump' from one region of interest to another one or be in more than one location simultaneously which is not possible.
%final state In fact, this implies that there exists at least one %
%$b_{1,j}$ that cannot be satisfied, which may happen only if 
%robot $j$ that is required to be in more than one location simultaneously. If (B) does not hold either, there is no way after taking the transition from $q_B$ to $q_B^1$ to eventually visit a final state. [correctly removed]
(c) Third, there may exist states $q_B'$ with feasible self loops that can be reached while satisfying the respective $b$ but without satisfying $b_{q_B',q_B'}$. Following the same logic as above we conclude that after taking a transition from $q_B$ to $q_B^1$, the only way to visit a final state is to instantaneously move from one NBA state to another one which is not possible unless (B) is true.
Thus, we conclude that condition (i) is not conservative i.e., it will remove transitions from $q_B$ to $q_B^1$ that if activated then satisfying the accepting condition of the NBA requires the robots to jump from one region of interest to another one or be in more than one location simultaneously which is not possible. Note that this part of the proof does not rely in Assumption \ref{as:cnf}.

Second, we show that condition (ii) is not conservative if Assumption \ref{as:cnf} holds. To show this, first we express $b^{q_B,q_B'}$ in CNF, i.e., as a conjunction of $F$ Boolean formulas $b_f$, for some $F>0$, where $b_f$ is a disjunction of literals, i.e.,
\begin{equation}\label{eq:bqbqb}
    b^{q_B,q_B'}=\bigwedge_{f=1}^F b_f
\end{equation}
%Assume that all literals in a clause $b_f$ are associated with only one robot, for all $f\in\{1,\dots,F\}$. 
%In what follows, we show by contradiction that Algorithm \ref{alg:prune} is not conservative if every clause $b_f$ is associated with only one robot, for all $f\in\{1,\dots,F\}$.
By Assumption \ref{as:cnf} we have that every clause $b_f$ is associated with only one robot, for all $f\in\{1,\dots,F\}$. Let $\ccalF_j$ be a set that collects all indices $f\in\{1,\dots,F\}$ to formulas $b_f$ that are associated with robot $j$, where $\ccalF_j\cap\ccalF_i=\emptyset$, for all $i,j\in\ccalN$, by definition of $b_f$. Next we define the Boolean formula 
\begin{equation}\label{eq:dj}
    d_j^{q_b,q_B'}=\bigwedge_{j\in\ccalF_j}b_f,
\end{equation}
which is a conjunction of all Boolean formulas $b_f$ associated with robot $j$. Using \eqref{eq:dj} and the fact that $\ccalF_j\cap\ccalF_i=\emptyset$, for all $i,j\in\ccalN$, we can re-write \eqref{eq:bqbqb} as 
\begin{equation}\label{eq:bqbqb2}
    b^{q_B,q_B'}=\bigwedge_{j=1}^N d_j^{q_b,q_B'}.
\end{equation}
Thus, the Boolean formula $b^{q_B,q_B'}$ can be decomposed into local/decoupled sub-formulas $d_j^{q_b,q_B'}$. In other words, robot $j$ can make decisions to contribute to satisfaction of $b^{q_B,q_B'}$ independent from other robots by considering only the sub-formula $d_j^{q_b,q_B'}$. 

Due to the decomposition of the Boolean formulas as per \eqref{eq:bqbqb2}, we can apply condition (ii) of Definition \ref{def:feas} locally to each robot to prune the NBA as follows. %
For all symbols  $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}$, there should exist at least one of the symbols $\sigma^{q_B,q_B^K}_j$ that satisfy condition (i) and either (A) $\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}=\emptyset$ or (B) $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^K}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^K}$. Note that since symbols $\sigma^{q_B,q_B^K}$ that satisfy condition (i) exist, this means $L_{j}^{q_B,q_B^K}$ is unique/well-defined for all robots $j\in\ccalR^{q_B,q_B^K}$. Assume that (ii) is not satisfied i.e., there exists at least one symbol $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}$ for which there are no $\sigma^{q_B,q_B^K}_j$ that satisfy either conditions (ii)-(A) or (ii)-B. This means that there exists $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B^K}\neq L_{j}^{q_B,q_B}$. Since $j\in\ccalR^{q_B,q_B}$, we have that transition towards the state $q_B$ was enabled because robot $j$ reached a region of interest $L_{j}^{q_B,q_B}$. Also, since $j\in\ccalR^{q_B,q_B^K}$, we get that transition from $q_B$ to $q_B^K$ will be enabled only if robot $j$ visits a region of interest denoted by $L_{j}^{q_B,q_B^K}$. By assumption $L_{j}^{q_B,q_B^K}\neq L_{j}^{q_B,q_B}$. Therefore, we conclude if condition (ii) is not satisfied then transition from $q_B$ to $q_B^K$ can be enabled only if robot $j$ keeps being in a region of interest $L_{j}^{q_B,q_B}$ until it reaches another region $L_{j}^{q_B,q_B^K}\neq L_{j}^{q_B,q_B}$, which is impossible given that all regions of interest are disjoint completing the proof.
%visiting the final states requires  this If (B) does not hold either, there is no way after taking the transition from $q_B$ to $q_B^1$ to eventually visit a final state. [correctly removed]
%
%(B.a) there are runs with loops but the loop does not include any final state (useless loop)
%(B.b) there are no runs 
%case (A.b) implies that there exists at least one $b_{1,j}$ that cannot be satisfied, which may happen only if robot $j$ is required to be in more than one location simultaneously. Then, this transition will be removed only if it does not satisfy (i-B). 
%case (A.c)
%
%b_{q_B,q_B^K}=b_{q_B,q_B^1}\wedge b_{q_B^2,q_B^3}\wedge\dots b_{q_B^{K-1},q_B^{K}}\wedge b_{q_B^{K},q_B^{K}}$. 
%
%
%$b_{q_B,q_B^1}$, $b_{q_B^k,q_B^{k+1}}$, for all $k\in\{1,\dots,K-1\}$, and $b_{q_B^K,q_B^{K}}$, while it does not satisfy $b_{q_B^k,q_B^{k}}$ (if it exists), for all $k\in\{1,\dots,K-1\}$.
%
%a transition $q_B\rightarrow_B^K q_B'$ is feasible if (i) for all symbols  $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}_j$ there exists at least one symbol denoted by $\sigma^{q_B,q_B^1}_j$ that enables a transition from $q_B$ to $q_B'$, i.e., $\sigma^{q_B,q_B'}_j\in\Sigma^{q_B,q_B^1}_j$ such that $\sigma^{q_B,q_B^1}_j\models d_{j,K}^{q_B,q_B'}$;
%\wedge_{k=1}^K d_j^{q_B^k,q_B^{k+1}}\wedge d_j^{q_B^K,q_B'}
%and 
%
%(ii) at least one of the symbols $\sigma^{q_B,q_B^1}_j$ that satisfy condition (ii) should satisfy either (a) $j\notin\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^1}$ or (b) $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B^1}\neq\emptyset$ and $L_{j}^{q_B,q_B}=L_{j}^{q_B,q_B^1}$.
%Specifically, following Definition \ref{def:feas}, a transition $(q_B,\cdot,q_B')$ is feasible if: (i) $\Sigma^{q_B,q_B}\neq \emptyset$ (i.e., $b^{{q_B,q_B}}$ is defined); (ii) for all symbols  $\sigma^{q_B,q_B}_j\in\Sigma^{q_B,q_B}_j$ there exists at least one symbol $\sigma^{q_B,q_B'}_j\in\Sigma^{q_B,q_B'}_j$ such that $\sigma^{q_B,q_B'}_j\models d^{q_B',q_B'}_j$; and (iii) at least one of the symbols $\sigma^{q_B,q_B'}_j$ that satisfy condition (ii) should satisfy either (a) $j\notin\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ or (b) $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B'}=L_{j}^{q_B,q_B}$, where conditions (ii)-(iii) should hold for all robots $j$. In condition (ii), if $j\notin\ccalN_{q_B',q_B'}$, then $d^{q_B',q_B'}_j$ is not defined; in this case $\sigma^{q_B,q_B'}_j\models d^{q_B',q_B'}_j$ is trivially satisfied as robot $j$ does not play any role in satisfying $b^{q_B',q_B'}$.
%
%Using this result, in what follows we show that the proposed pruning method will remove NBA transitions only their activation requires overlapping regions. Assume that the transition $q_B\rightarrow_B^K q_B'$ does not satisfy conditions (i) and/or (ii). \textit{First}, assume that condition (i) is not satisfied, i.e., there do not exist any feasible symbols $\sigma^{q_B,q_B^1}_j\models d_{j,K}^{q_B,q_B'}$. This may happen only if $\Sigma^{q_B,q_B'}_j=\emptyset$ which means that $d^{q_B,q_B'}_j$ and, consequently, $b^{q_B,q_B'}$ requires robot $j$ to be present in more than one location simultaneously. %As a result, the transition $q_B\rightarrow_K^B q_B'$ cannot be enabled.
%(B) Assume that $\Sigma^{q_B,q_B'}_j\neq\emptyset$.
%Assume that for at least one symbol $\sigma^{q_B,q_B}_j\models d^{q_B,q_B}_j$, there do not exist $\sigma^{q_B,q_B'}_j$ such that $\sigma^{q_B,q_B'}_j\models d^{q_B',q_B'}_j$. This implies that once robot $j$ makes a certain observation as per the Boolean formula $d^{q_B,q_B'}_j$, it has to make another observation as per $d^{q_B',q_B'}_j$ at the next time instant. Nevertheless, this cannot happen as the `next' operator is excluded.
%
%Consider any transition $(q_B,\cdot,q_B')'$ with $\Sigma^{q_B,q_B}\neq \emptyset$ that does not satisfy conditions (ii) and/or (iii). \textit{First}, assume that condition (ii) is not satisfied. There are two cases under which condition (ii) is not satisfied: (A) assume there do not exist any symbols $\sigma^{q_B,q_B'}_j\in \Sigma^{q_B,q_B'}_j$. This may happen only if $d^{q_B,q_B'}_j$ and, consequently, $b^{q_B,q_B'}$ requires robot $j$ to be present in more than one location simultaneously.  (B) Assume that there exist at least one symbol $\sigma^{q_B,q_B'}_j\in \Sigma^{q_B,q_B'}_j$. Assume that for at least one symbol $\sigma^{q_B,q_B}_j\models d^{q_B,q_B}_j$, there do not exist $\sigma^{q_B,q_B'}_j$ such that $\sigma^{q_B,q_B'}_j\models d^{q_B',q_B'}_j$. This implies that once robot $j$ makes a certain observation as per the Boolean formula $d^{q_B,q_B'}_j$, it has to make another observation as per $d^{q_B',q_B'}_j$ at the next time instant. Nevertheless, this cannot happen as the `next' operator is excluded.
%
%
%Thus, a transition will be removed due to condition (i) only if at least one robot $j$ needs to be present in more than one location simultaneously. \textit{Second}, assuming that condition (i) is satisfied, we show by contradiction that condition (ii) is always satisfied unless it requires a robot to `jump' from one region of interest. Assume that (ii) is not satisfied. This means that $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B^1}\neq L_{j}^{q_B,q_B}$. Since $j\in\ccalR^{q_B,q_B}$, this means that transition towards the state $q_B$ was enabled because robot $j$ reached a region of interest $L_{j}^{q_B,q_B}$. Also, since $j\in\ccalR^{q_B,q_B^1}$, this means that transition from $q_B$ to $q_B^1$ will be enabled only if robot $j$ visits a region of interest denoted by $L_{j}^{q_B,q_B^1}$. By assumption $L_{j}^{q_B,q_B^1}\neq L_{j}^{q_B,q_B}$. Therefore, transition from $q_B$ to $q_B'$ will be enabled if robot $j$ keeps being in $L_{j}^{q_B,q_B}$ until it reaches $L_{j}^{q_B,q_B^1}$, which is impossible given that all regions of interest are disjoint completing the proof.
%once robot $j$ reaches a region of interest $L_j^{q_B,q_B}=r_e$, it has to stay within this region until another region of interest $L_j^{q_B,q_B'}=r_m$ is reached. This transition cannot be enabled in practice since disjoint regions of interest are assumed which contradicts the assumption that (iii) is not satisfied completing the proof. %If condition (iii) is not satisfied, then this means that there exists at least one robot $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$. In other words, at least on robot $j$ has to instantaneously move from one region of interest to another one which is impossible which completes the proof.
%$\cap \Sigma^{q_B,q_B}_j$. This means that $\Sigma^{q_B,q_B'}_j\cap \Sigma^{q_B,q_B}_j=\emptyset$, i.e., once robot $j$ reaches a region required to 
%
%that do not satisfy condition (iii) but they are physically realizable. Since they do not satisfy (iii), this means that $j\in\ccalR^{q_B,q_B}\cap\ccalR^{q_B,q_B'}$ and $L_{j}^{q_B,q_B'}\neq L_{j}^{q_B,q_B}$, i.e., robot $j$ has to instantaneously move from one region of interest to another one which is impossible which completes the proof.
%
%If there are no Boolean sub-formulas of the form $b=\vee_{j\in\ccalR}[\triangle_{r_{e_j}\in\ccalL}(\pi_j^{r_{e_j}})]$ with $|\ccalR|>1$, then this means that to
\end{proof}
%(i.e. the only NBA transitions that will be removed are the ones that require a robot does not include any Boolean subformula of the form $\vee_{j\ccalR}(\pi_j)$

%Given the above results, we can state the following result.
\begin{lem}\label{lem:binv}
assume that at time $t$ the robots reach state $q_B\in\ccalQ_B\setminus\hat{\ccalQ}_B$ and design paths $\bbp_{j,t:T_j}$ to reach  $q_B^{\text{next}}$.
%Assume that there are no regions $r_i$ and $r_j$, such that $r_i\subseteq r_j$. Then,  %% condition for feasibility
As the robots execute the paths $\bbp_{j,t:T_j}$, as per Section \ref{sec:exec}, the transition $q_B\rightarrow_B^K q_B^{\text{next}}$ will be activated at the time instant $T=\max_j T_j$.
\end{lem}


\begin{proof}
To show this result, it suffices to show that $b_{\text{inv}}$ is satisfied during the time interval $[t,T)$, where recall that $b_{\text{inv}}$ is the Boolean formula should be satisfied to enable a loop around $q_B(t)$. The reason is that if $b_{\text{inv}}$ is satisfied, then the robots can always remain in $q_B(t)$ for all $t'\in [t,T)$. If the robots remain in $q_B(t)$ for all $t'\in [t,T)$, then at the time instant $T=\max_j T_j$, the transition from $q_B(t)$ to $q_B^{\text{next}}$ will be enabled, since at that time the robots will generate the symbol $\sigma_{\text{next}}$ by construction of Algorithm \ref{alg:RRT} [\red{explain the last sentence a bit more; add 1-2 sentences}].

By construction of the pruned NBA, we have that when a new NBA state $q_B(t)$ is reached at time $t$, the corresponding Boolean formula $b_{\text{inv}}$ is satisfied (see condition (ii) in Definition \ref{def:feas}). As a result, if all robots in the set $\ccalN_{\text{inv}}$ (i.e., the robots that appear in $b_{\text{inv}}$) remain idle, the Boolean $b_{\text{inv}}$ will be satisfied. Nevertheless, robots $j\ccalN_{\text{next}}$ navigate the environment as per \eqref{eq:localProb} while it may hold that $\ccalN_{\text{next}}\cap\ccalN_{\text{inv}}$. In what follows, we show that $q_D(t)=q_D(t')$ for all $t'\in[t,T)$. %Let $R_j^t$ be the region $r_i$ that the robots lie in at the time instant $t$. If  robot $j$ does not belong to any region $r_i$, i.e., $L(\bbp_{j}(t))=\varnothing$, then $R_j^t$ is not defined i.e., $R_j^t=\varnothing$. 
%
To show this, first recall that the robots $j\in\ccalR_{\text{inv}}\subseteq\ccalN_{\text{inv}}$ stay idle by construction of Alg. \ref{alg:RRT} and, therefore, they cannot violate $b_{\text{inv}}$. Thus it suffices to show that the robots $j\in\bar{\ccalR}_{\text{inv}}\cap\ccalN_{\text{next}}$, where $\bar{\ccalR}_{\text{inv}}=\ccalN_{\text{inv}}\setminus\ccalR_{\text{inv}}$ will not violate $b_{\text{inv}}$. To show this we consider two cases. 

First, assume that $\bar{\ccalR}_{\text{inv}}\cap\ccalN_{\text{next}}=\emptyset$. Then this means that all robots in $\ccalN_{\text{inv}}$ will stay idle and, therefore, $b_{\text{inv}}$ will not be violated. Second assume that there exist robots $j\in\bar{\ccalR}_{\text{inv}}\cap\ccalN_{\text{next}}$. By construction of the set $\bar{\ccalR}_{\text{inv}}$ we have that atomic predicates $\pi_j^{r_e}$ associated with robots $j\in\bar{\ccalR}_{\text{inv}}$ and for some regions $r_e$ appear in $b_{\text{inv}}$ only with a negation operator in front of them (i.e., in the following form $\neg\pi_j^{r_e}$). In other words, robots $j\in\bar{\ccalR}_{\text{inv}}\cap\ccalN_{\text{next}}$ will violate $b_{\text{inv}}$ only if they visit certain regions of interest as they move towards locations $\bbq\in\Omega$, where no atomic predicate is satisfied. Nevertheless, this is precluded by the first constraint in \eqref{eq:localProb} completing the proof. 
\end{proof}

==> files/proofs_short_Aug8.tex <==

%Given the above results, we can state the following result.
\begin{lem}\label{lem:binv}
Let $q_D(t)$ be the current DFA state and $\bbp_{j,t:T_j}$ be the paths that the robots designed to reach  $q_D^{\text{next}}$.
%Assume that there are no regions $r_i$ and $r_j$, such that $r_i\subseteq r_j$. Then,  %% condition for feasibility
As the robots execute the paths $\bbp_{j,t:T_j}$, as per Section \ref{sec:exec}, the only DFA transition that will be enabled is from $q_D(t)$ to $q_D^{\text{next}}$ at the time instant $T=\max_j T_j$.
\end{lem}


\begin{proof}
To show this result it suffices to show that $b_{\text{inv}}$ is satisfied during the time interval $[t,T)$, where recall that $b_{\text{inv}}$ is the Boolean formula that needs to satisfied so that the robots remain in $q_D(t)$. The reason is that if $b_{\text{inv}}$ is satisfied, then due to the deterministic nature of the DFA, it holds that the robots remain in $q_D(t)$ for all $t'\in [t,T)$. If the robots remain in $q_D(t)$ for all $t'\in [t,T)$, then at the time instant $T=\max_j T_j$, the transition from $q_D(t)$ to $q_D^{\text{next}}$ happens since the robots generate the symbol $\sigma_{\text{next}}$ which completes the proof.

By construction of the pruned DFA, we have that the first time, denoted by $t$, that the robots reach a state $q_D'$, i.e. $q_D(t)=q_D'$, then the corresponding Boolean formula $b_{\text{inv}}$ is satisfied (see condition (ii) in Definition \ref{def:feas}). In what follows, we show that $q_D(t)=q_D(t')$ for all $t'\in[t,T)$. %Let $R_j^t$ be the region $r_i$ that the robots lie in at the time instant $t$. If  robot $j$ does not belong to any region $r_i$, i.e., $L(\bbp_{j}(t))=\varnothing$, then $R_j^t$ is not defined i.e., $R_j^t=\varnothing$. 
%
To show this result, we consider two cases (i) $R_j^t=\varnothing$, for all robots $j\in\ccalR_{\text{next}}$; and (ii) $R_j^t\neq\varnothing$, for at least one robot $j\in\ccalR_{\text{next}}$. Recall that $R_j^t$ is the region $r_i$ that the robot $j$ lies in at the time instant $t$.

In the first case, if $R_j^t=\varnothing$, for all robots $j\in\ccalR_{\text{next}}$, then by construction of $\bbp_{j,t:T_j}$, we have that $L(\bbp(t'))=L(\bbp(t))$, for all $t'\in [t,T)$, since the robots $j\in\ccalR_{\text{next}}$ will not observe anything during the time interval $[t,T)$, by construction and execution of their paths (see constraint \eqref{constrLoc1}) and the robots $j\in\ccalR_{\text{inv}}$ stay idle at their current location. Then, since $L(\bbp(t))\models b_{\text{inv}}$ and due to the deterministic nature of the DFA, we have that the robots will remain in $q_D(t)$ for all $t'\in [t,T)$.

In the second case, we have that $R_j^t\neq\varnothing$, for at least one robot $j\in\ccalR_{\text{next}}$. In what follows, we show that a transition to another state $q_D'\neq q_D(t)$ will never happen at some $t'\in [t,T)$, as the robots $j\in\ccalR_{\text{next}}$ exit (asynchronously) the regions $R_j^t$. In other words, we show that the symbols $\sigma\neq\sigma_{\text{inv}}$, where $\sigma_{\text{inv}}=L(\bbp(t))$, that may be generated as the robots leave asynchronously their regions $R_j^t$ will not enable a transition from $q_D(t)$ to a new DFA state $q_D''$. 
%
%In what follows, we show that this can never happen. Specifically, we consider two cases. First, if $L(\bbp_j(t))=\varnothing$, for all $j\notin\ccalR_{\text{inv}}$, then it holds that for all time instants $t'\in [t,T_j^{-}]$ the robots only generate the word $\sigma_{\text{inv}}$ by construction of their paths. Due to the deterministic nature of the DFA, we have that the robots will remain in the DFA state $q_D(t)$, for all $t'\in [t,T_j^{-}]$. 
%
%Second, we consider the case where there exists at least one robot that is inside a region $R_j(t)$, i.e.,  $L(\bbp_j(t))\neq \varnothing$. 
To show this, we first rewrite $b_{\text{inv}}$ so that the atomic propositions that appear with a negation operator in front of them are separated from those that the negation operator does not exist in front of them. Specifically, using De Morgan's law, we re-write $b_{\text{inv}}$ in the following general form:
\begin{equation}\label{eq:inv1}
    b_{\text{inv}} = b_{\text{inv}}^{\text{goal}} \wedge [(\neg b_{\text{inv}}^{\text{avoid},1} )]\vee [(\neg b_{\text{inv}}^{\text{avoid},2})],
\end{equation}
%\red{[++more explanation on the subformuals++say that $b_{\text{inv}}$ exists because next operator does not exist]}
where the Boolean formulas $b_{\text{inv}}^{\text{goal}}$, $b_{\text{inv}}^{\text{avoid},1}$, and $b_{\text{inv}}^{\text{avoid},2}$ are defined so that the negation operator does not appear in front of any atomic proposition that comprise them. Since $\sigma_{\text{inv}}\models b_{\text{inv}}$ we have that either (i) $\sigma_{\text{inv}}\not\models b_{\text{inv}}^{\text{avoid},2}$, or (ii) $\sigma_{\text{inv}}\models b_{\text{inv}}^{\text{goal}} \wedge [(\neg b_{\text{inv}}^{\text{avoid},1} )]$ (or both). In case (i), the exit of robots from their regions $R_j^t$ means that symbols in $\sigma_{\text{inv}}$ are replaced with the empty string giving rise to a new symbol $\sigma$. 

Due to Lemma \ref{lem:logic}, we have that if $\sigma_{\text{inv}}\not\models b_{\text{inv}}^{\text{avoid},2}$ then $\sigma\not\models b_{\text{inv}}^{\text{avoid},2}$ or, equivalently $\sigma\models b_{\text{inv}}$ which means that the robots remain in $q_D(t)$ due to the deterministic structure of the DFA. 
%
For the same reason, in case (ii), if $\sigma_{\text{inv}}\models b_{\text{inv}}^{\text{goal}} \wedge [(\neg b_{\text{inv}}^{\text{avoid},1} )]$, we get that $\sigma\not\models b_{\text{inv}}^{\text{avoid},1}$. In case (ii), we also have that $\sigma\models b_{\text{inv}}^{\text{goal}}$, since the robots in $\ccalR_{\text{next}}$ are not responsible for generating the word $\sigma_{\text{inv}}$ (i.e., atomic propositions of the form $\pi_j^{r_i}$, where $j\in\ccalR_{\text{next}}$, do not exist in $b_{\text{inv}}^{\text{goal}}$) or if they are, then it suffices to remain put (see the third requirement in Definition \ref{def:feas}), as they do by construction of Algorithm \ref{alg:RRT}. Therefore, robots $j\in\ccalR_{\text{next}}$ cannot violate $b_{\text{inv}}^{\text{goal}}$. Thus in case (ii), we also get $\sigma\models b_{\text{inv}}$ which means that the robots remain in $q_D(t)$ due to the deterministic structure of the DFA for all $t'\in [t,T)$. At the time instant $T$, the robots $j\in\ccalR_{\text{next}}$ synchronously satisfy $L(\bbp_j(T))=\pi_j^{L_j^{\text{next}}}$ and the word $\sigma_{\text{next}}$ is generated enabling the transition from $q_D(t)$ to $q_D^{\text{next}}$ completing the proof.%. Note that $L(\bbp_j(T))=\pi_j^{L_j^{\text{next}}}$ is possible, is that there 
\end{proof}

==> files/sim.tex <==

%\begin{figure}
%    \centering
%     \includegraphics[width=0.5\linewidth]{figures/Horizon_VS_R_VS_NumRobots.png}
%    \caption{Effect of the sensing range $R$ on the terminal horizon $H$ that solves \eqref{eq:Prob2}.}
%    \label{fig:horizon}
%\end{figure}

\begin{figure*}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[$t=315$]{
    \label{fig:315}
  \includegraphics[width=0.3\linewidth]{figures/t315.pdf}}
  \subfigure[$t=342$]{
    \label{fig:342}
  \includegraphics[width=0.3\linewidth]{figures/t342.pdf}}
    \subfigure[$t=411$]{
    \label{fig:411}
  \includegraphics[width=0.3\linewidth]{figures/t411.pdf}}
  \caption{Case $N=1$, $R=0.3$: Figures \ref{fig:315}-\ref{fig:411} illustrate the robot trajectory while aiming to satisfy $\Diamond(\pi_1^{\ell_5}\vee\pi_1^{\ell_4})$, i.e., to visit either region $\ell_5$ or $\ell_4$. At time instant $t=315$ (Fig. \ref{fig:315}) the robot is heading towards $\ell_5$ and at $t=342$ (Fig. \ref{fig:342}) it realizes, based on the constructed occupancy grid map, that $\ell_5$ is surrounded by obstacles and, therefore, not reachable. As a result, it moves towards $\ell_4$ ((Fig. \ref{fig:411})) and arrives there at $t=411$. The blue circle denotes the sensing range and rhe red squares stands for the grid cells of the map $M(t)$ that are occupied by obstacles. The gray region corresponds to unknown obstacles. %Figure \ref{fig:effect} illustrates the effect of the sensing radius on the terminal horizon.
  }
  \label{fig:env1}
\end{figure*}


\begin{table*}[t]
\caption{Scalability Analysis-Comparative Results}
\label{tab:scale}
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
      & \multicolumn{2}{c|}{Average Re-planning Time (secs)} & \multicolumn{3}{c|}{Algorithm \ref{alg:RRT}} \\ \hline
      Number of Robots   & Algorithm \ref{alg:RRT}        & STyLuS         & Local Map Update (secs)  & $t_F^1$(iteration/time(hrs))  & $t_F^2$(iteration/time(hrs))  \\ \hline
N=1   & 0.05                   & 4.12        & 0.007                                               &    883~/~0.012               & 1065~/~0.015               \\ \hline
N=20  & 0.03                   & 313.69     & 0.007                                               &      952~/~0.17               &   1032~/~0.18                  \\ \hline
N=100 & 0.03                   & 1349.54        &0.009                                               &    1088~/~0.49                 &   1124~/~0.57                  \\ \hline
N=200 & 0.04                   & 2883.52        & 0.01                                              &   1028~/~1.13                  &    1067~/~1.23                 \\ \hline
N=500 & 0.05                   & 9271.57        & 0.008                                              & 1032~/~2.7                    & 1070~/~2.9                     \\ \hline
\end{tabular}
\end{table*}

In this section, we present simulations and hardware experiments that illustrate the efficiency of the proposed algorithm. Simulations have been implemented using MATLAB R2016b on a computer with Intel Core i7 3.1GHz and 16Gb RAM. \red{to be added: gazebo simulations}

%In this section, we present simulations and experiments that illustrate the efficiency of the proposed algorithm. 

\subsection{Numerical Experiments}\label{sec:sim1}
{\bf{Map-based Planning in Unknown Environments with Unreachable Regions:}} 
%vs Map-free
In what follows, we consider a single robot with differential drive dynamics equipped with a sensor of sensing range $R=1.2$. The robot resides in a $10\times10$ environment shown in Figure \ref{fig:env1} and is tasked with a surveillance mission that requires to visit regions of interest eventually or infinitely often
while always avoiding obstacles. This task is captured by the following LTL formula
\begin{equation}\label{task1}
 \phi= (\bigwedge_{e=1}^{2}\square\Diamond\xi_e)\wedge(\bigwedge_{e=3}^6\Diamond\xi_e)\wedge(\neg\xi_3\ccalU\xi_4)\wedge(\square\neg\xi_{\text{obs}})
\end{equation}
where $\xi_e$ is a Boolean formula that requires the robot to visit a specific regions of interest, for all $e\in\{1,\dots,6\}$, and $\xi_{\text{obs}}$ is true if the robot hits any obstacle. In particular, the Boolean formulas $\xi_e$ are defined as: (i) $\xi_1=(\pi_1^{\ell_6}\vee\pi_1^{\ell_3})$; (ii) $\xi_2=\pi_1^{\ell_1}$; (iii) $\xi_3=\pi_1^{\ell_2}$; (iv) $\xi_4=(\pi_1^{\ell_5}\vee\pi_1^{\ell_4})$; (v) $\xi_5=\pi_1^{\ell_8}$; and (vi) $\xi_6=\pi_1^{\ell_9}$. In words, \eqref{task1} requires (a) the Boolean formulas $\xi_1$ and $\xi_2$ to be satisfied infinitely often, (b) the Boolean formulas $\xi_3$, $\xi_4$, $\xi_5$, and $\xi_6$ to be satisfied eventually, (c) never satisfy $\xi_3$ until $\xi_4$ is satisfied, and (d) always avoid obstacles. This formula corresponds to a NBA with $14$ states and $61$ transitions. The corresponding pruned automaton has $37$ transitions while all of them are decomposable; see Definition \ref{def:feas} and Proposition \ref{lem:fragmentLTL}. The runtime to prune this automaton was $0.15$ seconds approximately. 

Figure \ref{fig:env1} illustrates the benefit of using online learned maps for planning in unknown environments. Specifically, incorporating mapping into the control loop allows robots to reason about the environment and make appropriate control decisions to accomplish the assigned task which would be quite challenging using map-free approaches e.g., \cite{guzzi2013human,bansal2019combining}
Particularly, Figure \ref{fig:env1} shows the trajectory that the robot follows to eventually satisfy $\xi_1=(\pi_1^{\ell_5}\vee\pi_1^{\ell_4})$ that requires robot $1$ to visit either location $\ell_5$ or $\ell_4$. Observe in Figure \ref{fig:env1} that $\ell_5$ is surrounded by obstacles and, therefore, it is not accessible. Initially, robot $1$ is moving towards $\ell_5$ and as it builds the map of the environment it realizes that $\ell_5$ is not reachable. When this happens, a new symbol that satisfies $\xi_1$ is selected and, therefore, robot $1$ decides to move towards $\ell_4$. A similar behavior is observed when the Boolean formula $\xi_1=(\pi_1^{\ell_6}\vee\pi_1^{\ell_3})$ needs to be satisfied. 

{\bf{Scalability Analysis:}} Next, we examine the performance of Algorithm \ref{alg:RRT} with respect to the number of robots and we provide comparative simulation studies against state-of-the-art centralized algorithms \cite{kantaros2018text,guo2013revising} that can be used for re-planning as the map of the environment is continuously learned. 

We consider a team of $N\in\{1,20,100,200,500\}$ robots with differential drive dynamics that reside in the environment shown in Figure \ref{fig:env1} while all robots are equipped with omnidirectional sensors of limited range $R=1.2$. The robots are tasked with accomplishing the task captured in \eqref{task1}. The difference is that the Boolean formulas $\xi_e$ require collaboration between multiple-robots. For instance, when $N=20$, we have that $\xi_1=\wedge_{j=1}^{15}(\pi_j^{\ell_6}\vee\pi_j^{\ell_3})$ which requires all robots with index $j\in\{1,\dots, 15\}$ to visit either region $\ell_3$ or $\ell_6$ and $\xi_2=\wedge_{j=8}^{20}(\pi_j^{\ell_2}\vee\pi_j^{\ell_3})$ which requires all robots with index $j\in\{8,\dots, 20\}$ to visit either region $\ell_2$ or $\ell_3$. 

Table \ref{tab:scale} summarizes the scalability analysis of the proposed algorithm. Specifically, the first column shows the number of robots, the second column shows the average time required for a robot to design a new path as the map is updated. To design paths we solve \eqref{eq:localProb} using the $\text{A}^*$ algorithm \cite{russell2002artificial}. Specifically, we represent the learned occupancy grid map, which consists of $10,000$ cells, as a graph and we apply $\text{A}^*$ on it to design paths towards the goal regions. Then, we synthesize controllers to follow the designed path. 
%
Note that the runtime to design new paths ranges between $0.03$ and $0.06$ seconds showing that Algorithm \ref{alg:RRT} can design new paths very fast for large-scale multi-robot systems with hundred of robots due to its decentralized nature. The third collumn shows the average runtime required if existing centralized methods are used for replanning \cite{guo2013revising,kantaros2018text}. Specifically, \cite{guo2013revising} employs partially known transition systems to model the interaction of the robot and environment which are updated as the environment is discovered. Motion plans are synthesized by composing the transition systems with the NBA giving rise to a product automaton. When the transition system is updated, the product automaton is locally updated and new paths are designed by computing new paths in the product automaton from the current product state to a final product state. To compare Algorithm \ref{alg:RRT} against this approach, we use a graph-based representation of the occupancy grid map as the transition system. Our implementation of \cite{guo2013revising} required more than $1$ hour to design a path over the product automaton for a single-robot system and ran out of memory for case studies with more than one robot. To enhance \cite{guo2013revising}, we integrate it with STyLuS* \cite{kantaros2018text}, a recently proposed temporal logic planning method that scales well with the number of robots. Specifically, we use \cite{kantaros2018text} to design paths, instead of building a product automaton and computing paths over it. The third column in Table \ref{tab:scale} shows the average runtime required for STyLuS* to design new paths. To compute this runtime, we consider cases where $q_B(t)=q_B^0$, i.e., the robots are still in the initial NBA state, and new paths towards a final NBA state need to be computed as in \cite{guo2013revising}. Observe in the third column of Table \ref{tab:scale} that STyLuS* can also handle large-scale multi-robot systems but the runtime required for replanning using Algorithm \ref{alg:RRT} is significantly smaller due to its decentralized nature and the decomposition of the LTL task into `smaller' and local tasks.

The fourth column shows the average time required per robot to update the map as per \eqref{eq:updMap}. The fifth and sixth column present the number of discrete time instants required to visit a final NBA state for the first and the second time respectively. These columns also include the corresponding total runtime required by Alg. \ref{alg:RRT}. Note that Alg. \ref{alg:RRT} has been implemented on a single computer and, therefore, control decisions are made sequentially, instead of in parallel, across the robots which explains why the runtime increases significantly as the number of robots increases.  




% ----------- simulation of N=50 robots ------------
%Moreover when $N=50$, we divide the robots into $9$ sub-teams $\ccalT_m$. Then, the specification $\phi$ requires (i) the sub-team $\ccalT_1$ to visit either the hostage $8$ or $5$ and the sub-team $\ccalT_2$ to visit either the hostage $7$, $4$, or $3$ ($\xi_1$); then %
%(ii) $\ccalT_3$ to visit either $7$ or $4$ and $\ccalT_4$ to visit $5$ ($\xi_2$); then (iii) $\ccalT_5$ to visit $1$ and $\ccalT_5$ to visit either $2$ or $6$ ($\xi_3$); then (iv) $\ccalT_6$ to visit $3$ and $\ccalT_7$ to visit either $6$ ($\xi_4$); then (v) $\ccalT_8$ to visit $4$ and $\ccalT_9$ to visit either $5$, $7$, or $8$ ($\xi_5$);
%
%while $\square\neg\xi_6$ requires teams $\ccalT_1$ and $\ccalT_2$ to always avoid hostages $1$ and $2$ respectively, since they carry supplies that are dangerous to them. After pruning the corresponding DFA, we get that $d(q_0,q_F)=5$, i.e., the assigned task is feasible. Specifically, to follow the shortest path that connects $q_0$ to $q_F$, 
%
%denoted by $\bbq_D=q_0,q_1,q_2,q_3,q_4,q_F$ the following requirements need to be met (a) satisfaction of (i) to reach $q_1$ from $q_0$, (b) satisfaction of (ii) to reach $q_2$ from $q_1$, (c) satisfaction of (iii) to reach $q_3$ from $q_2$, (d) satisfaction of (iv) and (v) at the same time to reach $q_4$ from $q_3$, and (e) satisfaction of $\xi_{\text{exit}}$ to reach $q_F$ from $q_4$. Note that the teams $\ccalT_6$, $\ccalT_7$, $\ccalT_8$, and $\ccalT_9$ do not share any common robots and, therefore, simultaneous satisfaction of (iv) and (v) to reach $q_4$ from $q_3$ is feasible; see Def. \ref{def:feas}.
%----------------------------------------------------
%
%


{\bf{Effect of Sensing Range:}}  In our simulations, we consider a team of $N\in\{1,5,10,25, 50\}$ robots with differential drive dynamics that reside in an unknown $10\times 10$ environment; see Fig. \ref{fig:340}. The robots are equipped with omnidirectional sensors of limited range $R\in\set{0.3,0.75,1.1, 2}$. %Note that the sensing range $0.3$ is significantly smaller than the dimension of the environment to model visually-degraded areas \cite{khattak2019visual}.
%
The robots are tasked with providing delivery services to known locations, in a user-specified order, while always avoiding obstacles and dangerous regions. Once and only when services are provided, the robots should exit the building. This task is captured by the following LTL formula
%$\phi=\Diamond(\xi_1\wedge\Diamond(\xi_2\wedge\Diamond(\xi_3\wedge(\Diamond\xi_4 \wedge (\Diamond\xi_5))))) \wedge(\wedge_{e\in\set{1,2,3,4,5}} (\neg \xi_{\text{exit}}\ccalU \xi_e)) \wedge (\square\neg \xi_6) \wedge (\square\neg \xi_{\text{obs}})$
\begin{align}\label{eq:task}
    \phi&=\Diamond(\xi_1\wedge\Diamond(\xi_2\wedge\Diamond(\xi_3\wedge(\Diamond\xi_4 \wedge (\Diamond\xi_5))))) \wedge\nonumber \\&\wedge (\square\neg \xi_6) \wedge (\square\neg \xi_{\text{obs}}) \wedge (\Diamond\square\xi_{\text{exit}})
\end{align}
where $\xi_e$ is a Boolean formula that requires a sub-team of robots to visit a specific region to provide e.g., supplies, for all $e\in\{1,\dots,6\}$, while $\xi_{\text{exit}}$ is true if all robots visit the exit of the building. For instance, when $N=1$, the Boolean formulas $\xi_e$ are defined as: (i) $\xi_1=(\pi_1^8\vee\pi_1^5)$; (ii) $\xi_2=\pi_1^7$; (iii) $\xi_3=\pi_1^4$; (iv) $\xi_4=(\pi_1^1\vee\pi_1^2)$; (v) $\xi_5=\pi_1^6$;  and (vi) $\square\neg \xi_6$ requires the robot to always  keep a distance of at least $0.3$ from region $3$. This LTL formula corresponds to a NBA with $17$ states $103$ transitions while the pruned automaton has $43$ transitions.
%
Figure \ref{fig:340} depicts the trajectory that a robot follows to reach $\ell_7$ as it learns the occupancy grid map through a sensor with a range $R=0.3$. Figure \ref{fig:effect} shows that as the sensing range $R$ increases, the total number of discrete time instants required to visit a final state for the first time decreases, since the larger the sensing range, the faster the robots can learn the map of the environment.  The simulation videos can be found in \cite{icra20_video}. 


\begin{figure}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
  \includegraphics[width=0.8\linewidth]{figures/340.png}
  \caption{Case $N=1$, $R=0.3$: Figure \ref{fig:340} illustrate the robot position (discs) and actions (arrows) while it is heading towards region $7$. The green circle denotes the sensing range. At time $t=190$ the robot is not aware of the horizontal obstacle that is between it and region $7$. As a result it moves toward the obstacle, until it is fully discovered. Then, a new obstacle-free path is eventually discovered to reach region $7$ ($t=340$). The red squares stands for the grid cells of the map $M(t)$ that are occupied by obstacles. %Figure \ref{fig:effect} illustrates the effect of the sensing radius on the terminal horizon.
  }
  \label{fig:340}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/HorizonVSSensing.png}
  \caption{Effect of sensing range. %Figure \ref{fig:effect} illustrates the effect of the sensing radius on the terminal horizon.
  }
 \label{fig:effect}
\end{figure}

% ----------- simulation of N=50 robots ------------
%Moreover when $N=50$, we divide the robots into $9$ sub-teams $\ccalT_m$. Then, the specification $\phi$ requires (i) the sub-team $\ccalT_1$ to visit either the hostage $8$ or $5$ and the sub-team $\ccalT_2$ to visit either the hostage $7$, $4$, or $3$ ($\xi_1$); then %
%(ii) $\ccalT_3$ to visit either $7$ or $4$ and $\ccalT_4$ to visit $5$ ($\xi_2$); then (iii) $\ccalT_5$ to visit $1$ and $\ccalT_5$ to visit either $2$ or $6$ ($\xi_3$); then (iv) $\ccalT_6$ to visit $3$ and $\ccalT_7$ to visit either $6$ ($\xi_4$); then (v) $\ccalT_8$ to visit $4$ and $\ccalT_9$ to visit either $5$, $7$, or $8$ ($\xi_5$);
%
%while $\square\neg\xi_6$ requires teams $\ccalT_1$ and $\ccalT_2$ to always avoid hostages $1$ and $2$ respectively, since they carry supplies that are dangerous to them. After pruning the corresponding DFA, we get that $d(q_0,q_F)=5$, i.e., the assigned task is feasible. Specifically, to follow the shortest path that connects $q_0$ to $q_F$, 
%
%denoted by $\bbq_D=q_0,q_1,q_2,q_3,q_4,q_F$ the following requirements need to be met (a) satisfaction of (i) to reach $q_1$ from $q_0$, (b) satisfaction of (ii) to reach $q_2$ from $q_1$, (c) satisfaction of (iii) to reach $q_3$ from $q_2$, (d) satisfaction of (iv) and (v) at the same time to reach $q_4$ from $q_3$, and (e) satisfaction of $\xi_{\text{exit}}$ to reach $q_F$ from $q_4$. Note that the teams $\ccalT_6$, $\ccalT_7$, $\ccalT_8$, and $\ccalT_9$ do not share any common robots and, therefore, simultaneous satisfaction of (iv) and (v) to reach $q_4$ from $q_3$ is feasible; see Def. \ref{def:feas}.
%----------------------------------------------------
%


%Note that an alternative approach to solve the considered planning problem in unknown environments is to use existing abstraction-free approaches for LTL planning \cite{vasile2013sampling,luo2019abstraction} to continuously update the robot paths as the map of the environment is learned. Nevertheless, such methods require searching over a large product automaton space to design paths that reach the final DFA state, a task that is computationally challenging to perform at runtime. To the contrary, the proposed method is more efficient as it searches over only the physical state-space to design paths that solve reachability planning problems; see \eqref{eq:localProb}. %that reach DFA states that are one-hop away from the current state.

\subsection{Hardware Experiments}
The proposed reactive algorithm was also evaluated experimentally to test its efficiency in real-time re-planning and reactivity. Specifically, Alg. \ref{alg:RRT} was implemented in MatLab with ROS and run on the Scarab platform developed at the University of Pennsylvania \cite{michael2008experimental}. The Scarab is a differential drive robot equipped with a Hokuyo UTM-30LX scanning laser that can obtain range measurements in a $270^0$ field-of-view up to a distance of $30$m and an Intel RealSense camera with a $180^0$ field-of-view. Laser-based sensing is used for robot localization and for building an occupancy grid map using the gmapping ROS package implementing the SLAM approach presented in \cite{grisetti2007improved}. A video with the conducted experiments can be found in \cite{icra_exp}. \red{[videos to  be updated]}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.95
    \linewidth]{figures/env1rbt.jpg}
    %\subfigure[]{
    %\includegraphics[width=0.95
    %\linewidth]{figures/env1rbt.jpg}}
    %    \subfigure[]{
    %\includegraphics[width=0.95
    %\linewidth]{figures/env2rbt.jpg}}
    \caption{Experiment setup: A differential drive robot equipped with a LiDAR sensor navigates indoor environments with unknown and static obstacles.}
    \label{fig:exp}
\end{figure}
%to accomplish a complex mission while adapting planning to the continuously learned map
{\bf{LiDAR-based \& Map-based Planning:}} First, we validated Alg. \ref{alg:RRT} in two complex indoor environments with \textit{unknown} and \textit{static} obstacles shown in Figure \ref{fig:exp}. The robot is responsible for accomplishing a surveillance task captured by the following LTL formula: 
\begin{align}\label{task3}
    \phi=&\Diamond(\pi_1^{\ell_4})\wedge\Diamond(\pi_1^{r_1})\wedge\Diamond(\pi_1^{r_2}\vee\pi_1^{r_5})\wedge\Diamond(\pi_1^{r_6}\vee\pi_1^{r_4})\nonumber\\& \wedge\Diamond(\pi_1^{r_7}\vee\pi_1^{r_5})\wedge (\neg \pi_1^{r_1}\ccalU \pi_1^{r_3})\wedge(\square \neg \xi^{\text{obs}}),
\end{align}
The task in \eqref{task3} requires the robot to eventually visit the locations $\ell_4$, $\ell_1$, either $\ell_2$ or $\ell_5$, either $\ell_6$ or $\ell_4$, either $\ell_7$ or $\ell_5$ and never visit $\ell_1$ until $\ell_3$ is visited while always avoiding the a priori unknown obstacles. Observe in Figure \ref{fig:exp} that obstacles can be both convex and non-convex. 
To ensure that the robot paths never go too close to the obstacles, paths are designed as per \eqref{eq:localProb} after inflating the obstacles. As anticipated, the few failures we recorded were associated with the inability of the SLAM approach to accurately localize the robot in long missions. 

%certain regions of interest while always avoiding obstacles. Note that in this experiment setup, we do not consider an omnidirectional sensor as required in Proposition \ref{thm:completeness}; nevertheless, the robot successfully accomplished the assigned mission in two different environments. 
%
%Second, we also considered \textit{unknown} and \textit{dynamic/unexpected} obstacles. Recall that Alg. \ref{alg:RRT} is specifically designed for environments with static obstacles; the same also holds for the theoretical guarantees provided in Section \ref{sec:complOpt}. Here, we present preliminary experimental results that show that Alg. \ref{alg:RRT} can be applied to dynamic environments as well. To this end, to account for unknown and dynamic obstacles, we solve the point-to-point navigation problem \eqref{eq:localProb} using the motion planning algorithm proposed in \cite{guzzi2013human}; note that \cite{guzzi2013human} does not require building a map of the environment. In this set of experiments, we consider two robots that need to coordinate to accomplish a collaborative task while also avoiding collisions with each other. %Finally, note that in this experiment, the robots are allowed to move asynchronously. 

%the robot successfully accomplished the assigned mission, the robot is not equipped with omnidirectional sensor
%Unlike the simulation results and the assumptions of Proposition \ref{thm:completeness}, the sensor is imperfect while there is localization error that grows over time. The latter may result in hitting obstacles especially in long-horizon missions. To mitigate this issue, we inflate the detected obstacles before applying Alg. \ref{alg:RRT}.

%Second, we also considered \textit{unknown} and \textit{dynamic} obstacles. Recall that Alg. \ref{alg:RRT} is specifically designed for environments with static obstacles; the same also holds for the theoretical guarantees provided in Section \ref{sec:complOpt}. Here, we present preliminary experimental results that show that Alg. \ref{alg:RRT} can be applied to dynamic environments as well. To this end, to account for unknown and dynamic obstacles, we solve the point-to-point navigation problem \eqref{eq:localProb} using the motion planning algorithm proposed in \cite{guzzi2013human}; note that \cite{guzzi2013human} does not require building a map of the environment. In this set of experiments, we consider two robots that need to coordinate to accomplish a collaborative task while also avoiding collisions with each other. %Finally, note that in this experiment, the robots are allowed to move asynchronously. 


%The proposed algorithm has also been validated experimentally for robots that that reside in complex indoor environments with \textit{unknown} and \textit{static} obstacles; see Fig. \ref{fig:exp}. In the experiments, the robot are equipped with a LiDAR sensor with $180^{o}$ field-of-view, which violates the assumption of Proposition \ref{thm:completeness}, since it is not an omnidirectional sensor. The task of the robot is captured by the following LTL formula: $\phi=\Diamond(\pi_1^{r_2}\vee \pi_1^{r_5})\wedge\Diamond(\pi_1^{r_1})\wedge\Diamond(\pi_1^{r_4}\vee\pi_1^{r_3})\wedge\Diamond(\pi_1^{r_7}\vee\pi_1^{r_5})\wedge(\wedge\Diamond(\pi_1^{r_8}\vee\pi_1^{r_6}) \wedge (\neg \pi_1^{r_9}\ccalU \pi_1^{r_8})\wedge(\square \neg \xi^{\text{obs}})$, which requires the robot to eventually visit certain regions of interest while always avoiding obstacles. This experiment has been conducted in two different environments. 
%F(p1) & F(p2) & F(p3) & F(p4) & F(p5) & FG(p6)
%

%{\bf{Experiments in Dynamic Environments:}} We have also validated experimentally Algorithm \ref{alg:RRT} in dynamic environments. Specifically, to solve the navigation problem in \eqref{eq:localProb} in the presence of \textit{unknown} and \textit{dynamic} obstacles, we employ the motion planning algorithm proposed in \cite{guzzi2013human}.  We consider two robots that need to coordinate to accomplish a collaborative task while also avoiding collisions with each other. Note that in this experiment, the robots move asynchronously as opposed to the majority of relevant works.
%




{\bf{Vision-based \& Map-Free Planning:}} 
In the second set of experiments we consider a team of two robots that have to accomplish the following task
\begin{align}\label{task4}
    \phi=&\Diamond(\pi_2^{\ell_2})\wedge\Diamond(\pi_1^{\ell_1}\wedge\Diamond(\pi_1^{\ell_3}\wedge\pi_2^{\ell_3}))\nonumber\\&\wedge\Diamond\square(\pi_1^{\ell_4})\wedge\Diamond\square(\pi_2^{\ell_4})\wedge(\square \neg \xi^{\text{obs}}).
\end{align}
The LTL task in \eqref{task4} requires robot $1$ and robot $2$ to eventually visit locations $\ell_1$ and $\ell_2$, respectively, e.g., to collect data. Then the robots should meet in $\ell_3$ e.g., to exchange their collected data or upload it to a data center, and then go to the exit $\ell_4$ of the room and stay there forever. 

In this set of experiments, to solve \eqref{eq:localProb}, i.e., to design reactive robot paths towards regions of interest, we rely on a vision-based approach proposed in \cite{guzzi2013human}. Specifically, \cite{guzzi2013human} proposes a heuristic approach to avoid dynamic obstacles such as other mobile robots or humans. Using visual information the heading of dynamic obstacles is estimated which is then used to compute the robot velocity so that all visible obstacles and robots are avoided within a time horizon. Figures \ref{fig:expMulti1} and \ref{fig:expMulti2} show cases where the robots react to unexpected obstacles that are placed in front of them at runtime. We would like to emphasize again that Algorithm \ref{alg:RRT} allows the robots to react to unknown structure of the environment quickly which would be impossible using available centralized temporal logic planning methods.

Note that \cite{guzzi2013human} is map-free i.e., it does not rely on building maps; instead navigation is accomplished using visual feedback. This allows to navigate dynamic environments as opposed to the purely map-based approach considered in the previous set of experiments.
Nevertheless, map-based approaches allows the robots to reason about the structure of the environment and make appropriate control decisions to accomplish their tasks as discussed in \ref{sec:sim1}. Integration of map-based and vision-based planning methods is part of our future work.
%In our future work, integra map-based approaches allow the robots to reaso


\begin{figure*}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Initial state]{
    \label{fig:a1}
  \includegraphics[width=0.32\linewidth]{figures/multiInit.jpg}}
  \subfigure[Unexpected obstacle]{
    \label{fig:b1}
  \includegraphics[width=0.32\linewidth]{figures/multiIBef.jpg}}
    %\subfigure[Reactive Planning]{
    %\label{fig:c1}
  %\includegraphics[width=0.47\linewidth]{figures/multiIAvoid1.jpg}}
      \subfigure[Reactive Planning]{
    \label{fig:d1}
  \includegraphics[width=0.32\linewidth]{figures/multiIAvoid2.jpg}}
  \caption{Camera-based planning in unknown environments: Robot $1$ and $2$ are heading towards locations $1$ and $2$ respectively. Obstacles are placed at run-time in the workspace. The robots adapt planning to these unexpected changes in the environment using visual feedback.\red{[Figs need some editing-hard to see what is happening]}
  }
  \label{fig:expMulti1}
\end{figure*}

\begin{figure*}[t]
  \centering
    %\subfigure[$t=190$]{
    %\label{fig:190}
  %\includegraphics[width=0.485\linewidth]{figures/190.png}}
      \subfigure[Heading towards $\ell_3$]{
    \label{fig:a2}
  \includegraphics[width=0.32\linewidth]{figures/multi2Bef2.jpg}}
    \subfigure[Unexpected Obstacle]{
    \label{fig:b2}
  \includegraphics[width=0.32\linewidth]{figures/multi2after2.jpg}}
      \subfigure[Reactive Planning]{
    \label{fig:c2}
  \includegraphics[width=0.32\linewidth]{figures/multi2avoid2.jpg}}
  \caption{Robot $1$ and $2$ are heading towards location $3$. Obstacles are placed at run-time in the workspace. The robots adapt planning to these unexpected changes in the environment using visual feedback. \red{[Figs need some editing-hard to see what is happening]}
  }
  \label{fig:expMulti2}
\end{figure*}


==> files/theory_final.tex <==
%\red{[TO BE UPDATED SOON!]}

%\begin{prop}[Correctness]
%If Algorithm \ref{alg:RRT} terminates successfully, then the resulting path $\bbp_{0:H}$ satisfies the LTL property $\phi$.
%\end{prop}
%\begin{proof}
%This result is true by construction of Algorithm \ref{alg:RRT}. Specifically, while the robots navigate in the workspace to reach the target DFA state $q_D^{\text{next}}$ from the current DFA state $q_D(t)$, they always check if the next observation $L(\bbp(t+1))$ violates the LTL formula $\phi$. If this is not the case, for all $t\geq 0$, the robots will eventually reach all subsequent target DFA states. Since the target DFA states are selected so that they are always one hop closer to the final state $q_F^{\text{feas}}$ than $q_D(t)$ is (see \eqref{eq:targetDFA}), this means that eventually the robots will reach $q_F^{\text{feas}}$ and, therefore, they will satisfy $\phi$ completing the proof.
%\end{proof}
 
 
%(ii) there do not exist regions $r_i$ and $r_e$, such that $r_i\subseteq r_e$ and 
%and (ii) there do not exist regions $r_i$ that are accessible only after visiting first
%\red{[the statements need to become more clear..]}
In this section, we examine correctness of the proposed reactive algorithm. First, recall from Algorithm \ref{alg:RRT} that once the robots reach a state $q_B(t)\in\ccalV$ a new state $q_B^{\text{next}}\in\ccalV$ is selected to be reached next.
%
This state is selected from the set $\ccalQ_{q_B(t)}^{\text{next}}\subseteq\ccalV$ that collects all states $q_B^{\text{next}}$ for which the transition from $q_B(t)$ to $q_B^{\text{next}}$ is decomposable, as per Definition \ref{def:feas}, and therefore, this transition can be enabled by solving local reachability tasks. As discussed in Remark \ref{rem:conserv}, Definition \ref{def:feas} is conservative, in the sense that there may be states that can be reached from $q_B(t)$ but they do not satisfy the conditions of Definition \ref{def:feas}; see e.g., Figure \ref{fig:conserv}.  As a result, such states are not included in the set $\ccalQ_{q_B(t)}^{\text{next}}$ and, therefore, a solution to Problem \ref{prob} may not be found even if it exists. 
%
First, we show that there exists a fragment of LTL for which any NBA transition $\delta_B^m(q_B,\cdot,q_B')$ associated with a run defined in \eqref{eq:run} always satisfies Definition \ref{def:feas}. In other words, all transitions $\delta_B^m(q_B,\cdot,q_B')$ are decomposable and can be enabled by solving local reachability problems \eqref{eq:localProb}. To show this we need make the following assumption.

%\subsection{Correctness of Algorithm \ref{alg:prune}}\label{sec:corPr}

%Given that the infeasible transitions are removed from the NBA, we have that the only reason there may not exist symbol $\sigma^{q_B,q_B^K}$ that satisfies $b^{q_B,q_B^K}$ is if the transition from $q_B$ to $q_B^K$ requires a robot to instantaneously jump from one region of interest to another one; see e.g., Figure \ref{fig:feas1}. 


%First of all note that for any state $q_B\in\ccalQ_B^{\text{loop}}$ there has to exist at least one state $q_B^K$ so that a run in the form of \eqref{eq:run} can be generated. If there exists no such runs, then the only way to visit a final state after visiting $q_B$ is by instantaneously jumping from one NBA state to another one i.e., without staying in any of them. Nevertheless, such transitions cannot exist, as they would require new observations to be made every time a new NBA state is visited which is impossible to specify given that the `next' operator is omitted. 

%In what follows we provide conditions under which Definition \ref{def:feas}, which Algorithm \ref{alg:prune} relies on, is not conservative. For this, we need first to state the following assumption.


\begin{assumption}\label{as:cnf}
Let $b^{q_B,q_B'}$ be a Boolean formula written in conjunctive normal form (CNF) associated with any NBA transition $\delta_B(q_B,\cdot,q_B')$. Assume that all literals in any given clause of $b^{q_B,q_B'}$ are associated with only one robot, which is not necessarily the same across different clauses.
\end{assumption}

\begin{lem}[From Global LTL to Local Tasks]\label{lem:fragmentLTL}
%Consider an LTL formula $\phi$ defined over atomic predicates $\pi_j^{\ell_i}$ where $j\in\ccalN$ and $\{\ell_i\}_{i\in\ccalL}$ denote disjoint regions of interest. 
%Consider any finite run in the form of \eqref{eq:run} from
%
Consider any two states $q_B,q_B'\in\ccalV$ for which there exists a symbol $\sigma^{q_B,q_B'}$ that satisfies the corresponding Boolean formula $b^{q_B,q_B'}$ defined in \eqref{eq:b}. Under Assumption \ref{as:cnf}, the transition $\delta_B^{m}(q_B,\cdot,q_B')$ is always decomposable, as per Definition \ref{def:feas}, unless this transition requires robots to instantaneously jump from one region of interest to another one which is impossible given that the regions of interest are disjoint.
\end{lem}

In other words, according to Lemma \ref{lem:fragmentLTL}, if all Boolean sub-formulas (expressed in CNF) that appear in an LTL formula satisfy Assumption \ref{as:cnf}, the global LTL formula can be decomposed into local reachability tasks.\footnote{The Boolean sub-formulas can be obtained after removing all temporal operators in an LTL formula.} Also, Lemma \ref{lem:fragmentLTL} implies that single-agent LTL tasks can always be decomposed into reachability tasks; see also Example \ref{ex:localTasks}.


%never couples two or more atomic predicates associated with different robots with the `or' operator, then Definition \ref{def:feas} is not conservative and, therefore, the global LTL formula can be decomposed into local reachability tasks. Also, Lemma \ref{lem:fragmentLTL} implies that Definition \ref{def:feas} is never conservative for single-robot tasks.

%\begin{rem}[Non-Emptiness of $\ccalQ_{q_B}^{\text{next}}$]
%By Definition $\ccalQ_{q_B}^{\text{next}}$ we have that $q_B\in\ccalQ_{q_B}^{\text{next}}$ for all $q_B\in\ccalQ_{q_B}^{\text{loop}}$. Also, we have that $\ccalQ_{q_B}^{\text{next}}\setminus\{q_B\}\neq\emptyset$ for all states $q_B\in\ccalQ_B^{\text{loop}}$ (assuming $\phi$ is satisfiable), since otherwise the only way to visit the final state after visiting $q_B$ is by instantaneously jumping from one NBA state to another one i.e., without staying in any of them. Nevertheless, such transitions cannot exist, as they would require new observations to be made every time a new NBA state is visited which is impossible to specify given that the `next' operator is omitted. 
%\end{rem}

%\subsection{Completeness of Algorithm \ref{alg:RRT}}\label{sec:corPl}


%\begin{lem}[Non-Existence of Solution]\label{thm:nonexist}
%Assume that (a) all Boolean subformulas that appear in an LTL formula satisfy Assumption \ref{as:cnf}, and (b) there does not exist an infinite path in $\ccalG$ that includes an infinite number of accepting edges defined in Definition \ref{def:accEdges}. Under assumptions (a)-(b), there does not exist a solution to Problem \ref{prob}.
%%%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. If at least one of these paths respects the robot dynamics \eqref{eq:rdynamics}, then Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
%\end{lem}

%\begin{lem}[Existence of Solution]\label{thm:exist}
%Assume that (a) all Boolean subformulas that appear in an LTL formula satisfy Assumption \ref{as:cnf}, and (b) there exists at least one robot path that respects the robot dynamics \eqref{eq:rdynamics} and connects any location $\bbq\in\Omega$ to any region $\ell_i$ without crossing any region $\ell_e\neq \ell_i$ and obstacles. Under assumptions (a)-(b), there exists a solution to Problem \ref{prob}.
%%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. If at least one of these paths respects the robot dynamics \eqref{eq:rdynamics}, then Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
%\end{lem}


Next we provide conditions that ensure that Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then a solution will be found.


%In the following proposition, we provide conditions under which Algorithm \ref{alg:RRT} is complete is complete.%, we need first to state the following Lemma. The proof is omitted due to space limitations.
%\begin{lem}\label{lem:binv}
%Let $q_D$ be the DFA state at time $t$ and $\bbp_{j,t:T_j}$ be the paths that the robots designed to reach  $q_D^{\text{next}}$.
%%Assume that there are no regions $r_i$ and $r_j$, such that $r_i\subseteq r_j$. Then,  %% condition for feasibility
%If all robots execute the paths $\bbp_{j,t:T_j}$, as per Section \ref{sec:planning}, and if all robots $j\in\ccalR_{\text{next}}$ reach their assigned regions $L_j^{\text{next}}$, then the robots remain in $q_D$ during the time interval $[t,T-1]$ and reach $q_D^{\text{next}}$ at the time instant $T=\max_j\{ T_j\}$.
%\end{lem}

%The following result presents conditions under which the pruning of the DFA is not conservative as discussed in Sec. \ref{sec:planning}.

%\begin{lem}\label{lem:cnt}
%Consider Boolean formulas $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$ in negation normal form. If the disjunction operator does not appear in either of these formulas, then Definition \ref{def:feas} is not conservative, i.e., if there exists at least one pair of symbols $\sigma_{\text{inv}}^{q_D}\in\Sigma_{\text{inv}}^{q_D}\cap\Sigma_{\text{feas}}$ and $\sigma_{\text{next}}^{q_D,q_D'}\in\Sigma_{\text{next}}^{q_D,q_D'}\cap \Sigma_{\text{inv}}^{q_D'}\cap\Sigma_{\text{feas}}$, then for any $\sigma_{\text{inv}}^{q_D}\in\Sigma_{\text{inv}}^{q_D}\cap\Sigma_{\text{feas}}$ there always exists $\sigma_{\text{next}}^{q_D,q_D'}\in\Sigma_{\text{next}}^{q_D,q_D'}\cap \Sigma_{\text{inv}}^{q_D'}\cap\Sigma_{\text{feas}}$ such that transition from $q_D$ to $q_D'$ can be cast as a reachability problem.
%\end{lem}


%The above lemma states that when the robots reach any DFA state $q_D'$, there always exist symbols $\sigma_{\text{inv}}$ and $\sigma_{\text{next}}$ to that will drive the robots towards another DFA state $q_D''$, as long as this transition is feasible. This essentially ensures that \eqref{eq:localProb} is always well defined. This is required in the proof of the following result.



\begin{prop}[Completeness]\label{thm:completeness}
Assume that (a) there exists at least one infinite path in $\ccalG$ that starts from $q_B^{\text{aux}}$ and traverses at least one accepting edge infinitely often,
%such that the disjunction operator does not appear in any of the formulas $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$, for all $q_D,q_D'$. %
(b) there exists at least one robot path that respects the robot dynamics \eqref{eq:rdynamics} and connects any location $\bbq\in\Omega$ to any region $\ell_i$ without crossing any region $\ell_e\neq \ell_i$ and obstacles, and (c)  \eqref{eq:sensor} models an omnidirectional sensor. Under assumptions (a)-(c), Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. If at least one of these paths respects the robot dynamics \eqref{eq:rdynamics}, then Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
\end{prop}

\red{[discuss why the assumptions are not too strong..and when then can be relaxed]}

Finally, in the next proposition we show that under the assumptions (a)-(b) of Proposition \ref{thm:completeness}, a solution to Problem \ref{prob} always exists.

\begin{prop}[Existence of Solution]\label{thm:exist}
If Assumptions (a)-(b) of Proposition \ref{thm:completeness} hold, then there exists a solution to Problem \ref{prob}.
%Assume that (a) there exists at least one infinite path in $\ccalG$ that starts from $q_B^{\text{aux}}$ and traverses at least one accepting edge, defined in Definition \ref{def:accEdges}, infinitely often, and (b) there exists at least one robot path that respects the robot dynamics \eqref{eq:rdynamics} and connects any location $\bbq\in\Omega$ to any region $\ell_i$ without crossing any region $\ell_e\neq \ell_i$ and obstacles. Under assumptions (a)-(b), there exists a solution to Problem \ref{prob}.
%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. If at least one of these paths respects the robot dynamics \eqref{eq:rdynamics}, then Algorithm \ref{alg:RRT} is complete, i.e., if there exists a solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will find it.
\end{prop}

\begin{ex}[From Global LTL to Local Tasks]\label{ex:localTasks}
Consider the LTL formula $\phi=\square(\pi_1^{\ell_0}\vee\pi_2^{\ell_0}) \wedge \Diamond \pi_2^{\ell_1}\wedge \Diamond \pi_2^{\ell_1}$ corresponding to the NBA shown in Figure \ref{fig:conserv}. This LTL formula has three Boolean subformulas: (i) $\pi_1^{\ell_0}\vee\pi_2^{\ell_0}$, (ii) $\pi_2^{\ell_1}$ , and (iii) $\pi_2^{\ell_1}$. Observe that the Boolean subformula $\pi_1^{\ell_0}\vee\pi_2^{\ell_0}$ violates Assumption \ref{as:cnf} and therefore it cannot be decomposed into local reachability tasks. On the other hand, the LTL formula $\phi=\Diamond[(\pi_1^{\ell_0}\vee\pi_1^{\ell_2})\wedge\pi_1^{\ell_0}] \wedge \square\Diamond \pi_2^{\ell_1}\wedge \square\Diamond \pi_2^{\ell_1}$
satisfies Assumption \ref{as:cnf}. More examples of LTL formulas that satisfy Assumption \ref{as:cnf} are provided in Section \ref{sec:Sim}.
%and can be decomposed into local reachability tasks.
\end{ex}


%\begin{rem}[Checking satisfiability of $\phi$]
%Note that if in the pruned DFA there is no path that connects at least one pair of initial and accepting states, then this means that there is no solution to Problem \ref{prob}. One the other hand, if there exists at least one such path, then this means that there exists a solution to Problem \ref{prob} assuming simple enough dynamics transitions from one region $r_i$ to any other region $r_e$ can be accomplished while avoiding regions (e.g., obstacles) as determined by $\phi$.\footnote{\red{this is intuitively correct. It'd be great if we add a formal proof}} 
%\end{rem}

%\begin{prop}[Satisfiability]\label{prop:sat}
%%Consider robots with single-integrator dynamics. Also, 
%Assume that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$ and obstacles. 
%Consider a co-safe temporal logic formula such that the disjunction operator does not appear in any of the formulas $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$, for all $q_D,q_D'$. Assume that there exists at least one path that connects any location $\bbq\in\Omega$ to any region $r_i$ without crossing any region $r_e\neq r_i$ and obstacles. Also, assume that at least one of these paths satisfies the robot dynamics \eqref{eq:rdynamics}. Then, given the corresponding pruned DFA, it holds that $\phi$ cannot be satisfied if $d(q_0,q_F)=\infty$. If $d(q_0,q_F)\neq\infty$, then there exists $\bbp_{0:H}$ that satisfies $\phi$.
%\end{prop}

%\begin{proof} %This result can be proved by following the same logic as in the proof of Proposition \ref{thm:completeness}. 
%If $d(q_0,q_F)=\infty$, then by Definition \ref{def:feas}, we conclude that there exist robots that either have to be present in more than one disjoint region simultaneously or have to instantaneously move from one region to another region (see condition (ii) in Definition \ref{def:feas}) so that $\phi$ is satisfied. Thus, robot paths $\bbp_{0:H}$ that can satisfy $\phi$ do not exist. Note that condition (iii) in Definition \ref{def:feas} holds for all DFA transitions, if $\vee$ is excluded from the syntax, as shown in Lemma \ref{lem:cnt}. %and therefore no transition will be deleted due to condition(iii)
%%
%%
%If $d(q_0,q_F)\neq\infty$, then following the same logic as in the proof of Proposition \ref{thm:completeness}, we conclude that there exist robot paths $\bbp_{0:H}$ such that $\bbp_{0:H}\models\phi$ under the considered assumptions on the robot dynamics and the structure of the environment.
%%%
%, if there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$ and obstacles and at least one of these paths satisfies the robot dynamics.
%First, note that every DFA state $q_D$ has a (non-empty) Boolean formula $b_{\text{inv}}^{q_D}$ that if satisfied, transition from $q_D$ to $q_D$ (self-loop) is activated. The reason is that the `next' temporal operator is not included in the task specification language. Also, as the robots `follow' a path $\bbq_D$, when they reach a configuration $\bbp\in\Omega^N$ that enables a transition from $q_D$ to $q_D'$, we have that $L(\bbp)\models b_{\text{inv}}^{q_D'}$ by construction of the DFA. In other symbols, if the DFA will not move to another state until the robots observe something new that will either violate $\phi$ (and in this case there is no outgoing transition from $q_D'$ to another DFA state based on the current observation) or enable a transition to another state $q_D''$. 
%%%
%Second, assume that the multi-robot system has currently reached $q_D$ and as discussed before, the current multi-robot robot state $\bbp$ satisfies $L(\bbp)\models b_{\text{inv}}^{q_D}$. In what follows, we show by contradiction that $q_D'$ can be reached. Assume that the robots cannot reach $q_D'$. This means that the robots can never satisfy the Boolean formula $b_{\text{next}}^{q_D,q_D'}$. However, by Lemma \ref{lem:feas}, we have that there exist paths for all robots that can reach $q_D'$ assuming simple dynamics and that there exist obstacle-free paths that connect any two regions $r_i$ and $r_e$ without crossing any other region $r_m$. Thus, under these assumptions it is not possible that $q_D'$ cannot be reached. Therefore, we conclude that $q_D$ can be reached completing the proof.
%\end{proof}

%\begin{rem}[Boolean Operator OR]
%Note that the completeness and satisfiability result can be extended to cases where the $\vee$ operator is included in the syntax; however, a full characterization of the LTL formulas for which Alg. \ref{alg:RRT} is complete is omitted due to space limitation. For instance, the above results hold, if $\vee$ appears in $\phi$ but never associates atomic predicates of different robots (i.e., Boolean statements of the form $\pi_j^{r_e}\vee\pi_r^{r_m}$ never appear in $\phi$). This also implies that if $N=1$ then the above results hold even if $\vee$ is included. Such cases are included in the simulation/experimental results.
%\end{rem}

